Finding Convincing Arguments Using Scalable Bayesian Preference Learning

We introduce a scalable Bayesian preference learning method for identifying convincing arguments in the absence of gold-standard rat- ings or rankings. In contrast to previous work, we avoid the need for separate methods to perform quality control on training data, predict rankings and perform pairwise classification. Bayesian approaches are an effective solution when faced with sparse or noisy training data, but have not previously been used to identify convincing arguments. One issue is scalability, which we address by developing a stochastic variational inference method for Gaussian process (GP) preference learning. We show how our method can be applied to predict argument convincingness from crowdsourced data, outperforming the previous state-of-the-art, particularly when trained with small amounts of unreliable data. We demonstrate how the Bayesian approach enables more effective active learning, thereby reducing the amount of data required to identify convincing arguments for new users and domains. While word embeddings are principally used with neural networks, our results show that word embeddings in combination with linguistic features also benefit GPs when predicting argument convincingness.

==> figures/features2/feature_table.tex <==
Emb_dimension_250 & 0.40719 \nonumber\\
Emb_dimension_19 & 0.48545 \nonumber\\
Emb_dimension_205 & 0.51810 \nonumber\\
Emb_dimension_291 & 0.58783 \nonumber\\
Emb_dimension_173 & 0.59443 \nonumber\\
Emb_dimension_60 & 0.61096 \nonumber\\
Emb_dimension_180 & 0.61138 \nonumber\\
Emb_dimension_111 & 0.61279 \nonumber\\
Emb_dimension_227 & 0.61656 \nonumber\\
Emb_dimension_86 & 0.62554 \nonumber\\
Emb_dimension_296 & 0.62627 \nonumber\\
sentimentPositive & 0.63554 \nonumber\\
Emb_dimension_115 & 0.63737 \nonumber\\
Emb_dimension_107 & 0.63794 \nonumber\\
Emb_dimension_16 & 0.64628 \nonumber\\
Emb_dimension_271 & 0.65794 \nonumber\\
Emb_dimension_27 & 0.66930 \nonumber\\
Emb_dimension_133 & 0.67488 \nonumber\\
Emb_dimension_217 & 0.67495 \nonumber\\
Emb_dimension_220 & 0.67785 \nonumber\\
Emb_dimension_241 & 0.67956 \nonumber\\
Emb_dimension_122 & 0.68083 \nonumber\\
Emb_dimension_150 & 0.68644 \nonumber\\
Emb_dimension_89 & 0.68824 \nonumber\\
Emb_dimension_156 & 0.69151 \nonumber\\
Emb_dimension_191 & 0.69477 \nonumber\\
Emb_dimension_40 & 0.69500 \nonumber\\
Emb_dimension_61 & 0.70342 \nonumber\\
Emb_dimension_166 & 0.71249 \nonumber\\
Emb_dimension_85 & 0.71321 \nonumber\\
Emb_dimension_80 & 0.71853 \nonumber\\
Emb_dimension_197 & 0.72274 \nonumber\\
Emb_dimension_10 & 0.72288 \nonumber\\
Emb_dimension_224 & 0.72498 \nonumber\\
Emb_dimension_222 & 0.73112 \nonumber\\
word_more_6_letters_ratio & 0.73443 \nonumber\\
Emb_dimension_101 & 0.73894 \nonumber\\
Emb_dimension_130 & 0.73920 \nonumber\\
Emb_dimension_54 & 0.74126 \nonumber\\
Emb_dimension_192 & 0.74763 \nonumber\\
Emb_dimension_285 & 0.75383 \nonumber\\
Emb_dimension_256 & 0.75705 \nonumber\\
Emb_dimension_212 & 0.76352 \nonumber\\
Emb_dimension_290 & 0.76364 \nonumber\\
Emb_dimension_248 & 0.76468 \nonumber\\
Emb_dimension_165 & 0.76705 \nonumber\\
Emb_dimension_152 & 0.77348 \nonumber\\
Emb_dimension_170 & 0.77892 \nonumber\\
Emb_dimension_282 & 0.77986 \nonumber\\
Emb_dimension_114 & 0.78577 \nonumber\\
Emb_dimension_168 & 0.78688 \nonumber\\
Emb_dimension_38 & 0.78828 \nonumber\\
Emb_dimension_99 & 0.78851 \nonumber\\
Emb_dimension_65 & 0.79290 \nonumber\\
Emb_dimension_284 & 0.79360 \nonumber\\
Emb_dimension_245 & 0.79444 \nonumber\\
Emb_dimension_43 & 0.79485 \nonumber\\
Emb_dimension_211 & 0.79632 \nonumber\\
Emb_dimension_70 & 0.80108 \nonumber\\
Emb_dimension_275 & 0.80770 \nonumber\\
Emb_dimension_63 & 0.80896 \nonumber\\
Emb_dimension_79 & 0.80983 \nonumber\\
Emb_dimension_186 & 0.82495 \nonumber\\
Emb_dimension_265 & 0.82559 \nonumber\\
Emb_dimension_48 & 0.82641 \nonumber\\
Emb_dimension_244 & 0.82784 \nonumber\\
Emb_dimension_49 & 0.83437 \nonumber\\
Emb_dimension_235 & 0.83741 \nonumber\\
Emb_dimension_257 & 0.83909 \nonumber\\
sentimentVeryNegative & 0.84163 \nonumber\\
Emb_dimension_105 & 0.84226 \nonumber\\
Emb_dimension_172 & 0.84413 \nonumber\\
Emb_dimension_289 & 0.84472 \nonumber\\
Emb_dimension_267 & 0.84529 \nonumber\\
Emb_dimension_229 & 0.84587 \nonumber\\
Emb_dimension_174 & 0.84678 \nonumber\\
Emb_dimension_260 & 0.84737 \nonumber\\
Emb_dimension_7 & 0.85297 \nonumber\\
Emb_dimension_113 & 0.85399 \nonumber\\
Emb_dimension_110 & 0.85623 \nonumber\\
Emb_dimension_226 & 0.85752 \nonumber\\
Emb_dimension_1 & 0.85857 \nonumber\\
Emb_dimension_132 & 0.86007 \nonumber\\
Emb_dimension_121 & 0.86070 \nonumber\\
Emb_dimension_20 & 0.86174 \nonumber\\
Emb_dimension_251 & 0.86328 \nonumber\\
Emb_dimension_294 & 0.86450 \nonumber\\
Emb_dimension_155 & 0.86583 \nonumber\\
Emb_dimension_104 & 0.86649 \nonumber\\
Emb_dimension_36 & 0.86742 \nonumber\\
Emb_dimension_87 & 0.87023 \nonumber\\
Emb_dimension_218 & 0.87358 \nonumber\\
Emb_dimension_83 & 0.87705 \nonumber\\
Emb_dimension_232 & 0.87924 \nonumber\\
Emb_dimension_140 & 0.87968 \nonumber\\
Emb_dimension_237 & 0.89019 \nonumber\\
Emb_dimension_216 & 0.89452 \nonumber\\
Emb_dimension_299 & 0.89892 \nonumber\\
sentimentNeutral & 0.89984 \nonumber\\
Emb_dimension_22 & 0.90093 \nonumber\\
Emb_dimension_2 & 0.90831 \nonumber\\
Emb_dimension_28 & 0.91070 \nonumber\\
Emb_dimension_15 & 0.91220 \nonumber\\
Emb_dimension_204 & 0.91303 \nonumber\\
Emb_dimension_228 & 0.91389 \nonumber\\
Emb_dimension_9 & 0.91401 \nonumber\\
Emb_dimension_181 & 0.91477 \nonumber\\
Emb_dimension_252 & 0.91573 \nonumber\\
Emb_dimension_259 & 0.91651 \nonumber\\
Emb_dimension_127 & 0.91893 \nonumber\\
Emb_dimension_175 & 0.91963 \nonumber\\
Emb_dimension_153 & 0.92318 \nonumber\\
Emb_dimension_96 & 0.92508 \nonumber\\
Emb_dimension_26 & 0.92520 \nonumber\\
Emb_dimension_171 & 0.92598 \nonumber\\
Emb_dimension_84 & 0.92759 \nonumber\\
Emb_dimension_177 & 0.92797 \nonumber\\
Emb_dimension_144 & 0.93029 \nonumber\\
Emb_dimension_118 & 0.93448 \nonumber\\
Emb_dimension_193 & 0.93818 \nonumber\\
Emb_dimension_17 & 0.94029 \nonumber\\
SuperlativeRatioAdj & 0.94267 \nonumber\\
Emb_dimension_169 & 0.94541 \nonumber\\
Emb_dimension_288 & 0.94698 \nonumber\\
_pos_ngram_V_ADJ & 0.94990 \nonumber\\
Emb_dimension_283 & 0.95278 \nonumber\\
Emb_dimension_279 & 0.95345 \nonumber\\
Emb_dimension_199 & 0.95420 \nonumber\\
Emb_dimension_148 & 0.95444 \nonumber\\
Emb_dimension_31 & 0.95543 \nonumber\\
Emb_dimension_162 & 0.95742 \nonumber\\
Emb_dimension_3 & 0.95808 \nonumber\\
Emb_dimension_277 & 0.95839 \nonumber\\
Emb_dimension_57 & 0.95999 \nonumber\\
Emb_dimension_297 & 0.96056 \nonumber\\
Emb_dimension_116 & 0.96284 \nonumber\\
Emb_dimension_249 & 0.96338 \nonumber\\
Emb_dimension_270 & 0.96503 \nonumber\\
Emb_dimension_154 & 0.96650 \nonumber\\
Emb_dimension_194 & 0.96653 \nonumber\\
sentimentNegative & 0.96735 \nonumber\\
Emb_dimension_233 & 0.96771 \nonumber\\
Emb_dimension_149 & 0.96803 \nonumber\\
Emb_dimension_73 & 0.96985 \nonumber\\
Emb_dimension_163 & 0.97003 \nonumber\\
Emb_dimension_158 & 0.97138 \nonumber\\
Emb_dimension_292 & 0.97141 \nonumber\\
Emb_dimension_5 & 0.97351 \nonumber\\
_pos_ngram_PUNC_NN & 0.97402 \nonumber\\
Emb_dimension_13 & 0.97430 \nonumber\\
Emb_dimension_47 & 0.97552 \nonumber\\
_pos_ngram_PR_PUNC & 0.97704 \nonumber\\
ProductionRule_S->NP,VP,., & 0.97712 \nonumber\\
Emb_dimension_62 & 0.97969 \nonumber\\
_pos_ngram_PP_V_PR & 0.98053 \nonumber\\
. & 0.98115 \nonumber\\
_pos_ngram_NN_V_ADV & 0.98137 \nonumber\\
_pos_ngram_V_PP_PR & 0.98199 \nonumber\\
Emb_dimension_258 & 0.98203 \nonumber\\
_pos_ngram_PUNC_ART & 0.98243 \nonumber\\
word_more_6_letters & 0.98253 \nonumber\\
Emb_dimension_71 & 0.98340 \nonumber\\
Emb_dimension_64 & 0.98447 \nonumber\\
_pos_ngram_NN_CONJ & 0.98448 \nonumber\\
Emb_dimension_146 & 0.98507 \nonumber\\
_pos_ngram_ART_ADJ_NN & 0.98542 \nonumber\\
_pos_ngram_ADV_PP & 0.98564 \nonumber\\
InterjectionRate & 0.98584 \nonumber\\
_pos_ngram_NN_PUNC & 0.98586 \nonumber\\
_pos_ngram_ADJ_NN_PUNC & 0.98646 \nonumber\\
Emb_dimension_189 & 0.98671 \nonumber\\
SuperlativeRatioAdv & 0.98693 \nonumber\\
_pos_ngram_PP_PR_V & 0.98712 \nonumber\\
_pos_ngram_NP_V & 0.98770 \nonumber\\
Emb_dimension_238 & 0.98784 \nonumber\\
ProductionRule_S->NP,VP, & 0.98833 \nonumber\\
de.tudarmstadt.ukp.dkpro.core.api.ner.type.Location & 0.98875 \nonumber\\
_pos_ngram_V_V & 0.98895 \nonumber\\
_pos_ngram_PP_PP & 0.98903 \nonumber\\
_pos_ngram_ADJ_NN & 0.98905 \nonumber\\
to & 0.98927 \nonumber\\
Emb_dimension_44 & 0.98939 \nonumber\\
_pos_ngram_NN_V_V & 0.98952 \nonumber\\
in & 0.98974 \nonumber\\
it & 0.98976 \nonumber\\
_pos_ngram_ADJ_PP_V & 0.99057 \nonumber\\
smog & 0.99058 \nonumber\\
_pos_ngram_V_ADJ_PP & 0.99065 \nonumber\\
_pos_ngram_PUNC & 0.99078 \nonumber\\
not & 0.99085 \nonumber\\
_pos_ngram_PP_V & 0.99100 \nonumber\\
_pos_ngram_V_PP_PP & 0.99126 \nonumber\\
_pos_ngram_NN_PUNC_ART & 0.99130 \nonumber\\
_pos_ngram_V_NN & 0.99142 \nonumber\\
Emb_dimension_55 & 0.99143 \nonumber\\
_pos_ngram_V_PP & 0.99149 \nonumber\\
_pos_ngram_PP_PR_NN & 0.99169 \nonumber\\
_pos_ngram_ADV_V_PP & 0.99170 \nonumber\\
QuestionRatio & 0.99175 \nonumber\\
ProductionRule_SBAR->IN,S, & 0.99179 \nonumber\\
_pos_ngram_NN_PP_V & 0.99187 \nonumber\\
a & 0.99192 \nonumber\\
_pos_ngram_NN_PUNC_NN & 0.99196 \nonumber\\
Emb_dimension_137 & 0.99206 \nonumber\\
_pos_ngram_ADJ_NN_PP & 0.99211 \nonumber\\
_pos_ngram_NN_V & 0.99216 \nonumber\\
_pos_ngram_CONJ_NN & 0.99217 \nonumber\\
_pos_ngram_V_ADJ_NN & 0.99225 \nonumber\\
_pos_ngram_PP_NP & 0.99230 \nonumber\\
_pos_ngram_ART_NN_V & 0.99249 \nonumber\\
Emb_dimension_266 & 0.99255 \nonumber\\
_pos_ngram_V_PP_ADJ & 0.99257 \nonumber\\
_pos_ngram_CARD & 0.99270 \nonumber\\
_pos_ngram_PP_NN_PUNC & 0.99284 \nonumber\\
_pos_ngram_PUNC_NN_V & 0.99293 \nonumber\\
_pos_ngram_V_V_ADJ & 0.99308 \nonumber\\
_pos_ngram_PP_ADJ_NN & 0.99308 \nonumber\\
_pos_ngram_V_ART_ADJ & 0.99328 \nonumber\\
and & 0.99331 \nonumber\\
_pos_ngram_V_PR_PUNC & 0.99334 \nonumber\\
argument & 0.99341 \nonumber\\
Emb_dimension_8 & 0.99344 \nonumber\\
_pos_ngram_V_ADV & 0.99355 \nonumber\\
Emb_dimension_239 & 0.99363 \nonumber\\
_pos_ngram_O_O & 0.99370 \nonumber\\
_pos_ngram_CARD_NN & 0.99375 \nonumber\\
can & 0.99381 \nonumber\\
the & 0.99399 \nonumber\\
_pos_ngram_PR_ADV & 0.99420 \nonumber\\
_pos_ngram_NP_PP & 0.99422 \nonumber\\
Emb_dimension_11 & 0.99451 \nonumber\\
_pos_ngram_ADJ & 0.99454 \nonumber\\
_pos_ngram_V & 0.99456 \nonumber\\
why & 0.99466 \nonumber\\
there & 0.99480 \nonumber\\
_pos_ngram_PP_V_ADJ & 0.99488 \nonumber\\
with & 0.99499 \nonumber\\
ProductionRule_NP->JJ,NN, & 0.99502 \nonumber\\
_pos_ngram_PR_V_ART & 0.99507 \nonumber\\
_pos_ngram_V_ADV_ADV & 0.99512 \nonumber\\
know & 0.99535 \nonumber\\
_pos_ngram_PP_NN_NN & 0.99542 \nonumber\\
_pos_ngram_V_V_NN & 0.99568 \nonumber\\
_pos_ngram_PP & 0.99571 \nonumber\\
_pos_ngram_NN & 0.99574 \nonumber\\
_pos_ngram_NN_ADJ & 0.99574 \nonumber\\
Emb_dimension_32 & 0.99577 \nonumber\\
_pos_ngram_PP_ADJ & 0.99586 \nonumber\\
_pos_ngram_NN_V_PP & 0.99596 \nonumber\\
_pos_ngram_PP_V_V & 0.99601 \nonumber\\
_pos_ngram_PR_NN_PP & 0.99601 \nonumber\\
_pos_ngram_CONJ_PR & 0.99603 \nonumber\\
_pos_ngram_V_ADV_PP & 0.99603 \nonumber\\
_pos_ngram_CONJ & 0.99606 \nonumber\\
_pos_ngram_ADV_V_PUNC & 0.99606 \nonumber\\
do & 0.99609 \nonumber\\
_pos_ngram_ADJ_PP & 0.99619 \nonumber\\
other & 0.99620 \nonumber\\
_pos_ngram_NN_CONJ_NN & 0.99620 \nonumber\\
._it & 0.99620 \nonumber\\
_pos_ngram_PR_V_PR & 0.99623 \nonumber\\
ProductionRule_NP->DT,NNS, & 0.99623 \nonumber\\
_pos_ngram_NN_PP_ADV & 0.99629 \nonumber\\
_pos_ngram_V_ADV_PR & 0.99662 \nonumber\\
be & 0.99663 \nonumber\\
_pos_ngram_PUNC_ART_NN & 0.99665 \nonumber\\
_pos_ngram_ART & 0.99665 \nonumber\\
ProductionRule_VP->VBG,NP, & 0.99670 \nonumber\\
_pos_ngram_V_PP_NP & 0.99681 \nonumber\\
_pos_ngram_NP_V_ART & 0.99682 \nonumber\\
_pos_ngram_V_V_ART & 0.99690 \nonumber\\
Emb_dimension_108 & 0.99690 \nonumber\\
_pos_ngram_ART_NP & 0.99700 \nonumber\\
_pos_ngram_PUNC_ART_V & 0.99701 \nonumber\\
ProductionRule_VP->VBZ,SBAR, & 0.99704 \nonumber\\
_pos_ngram_NN_O & 0.99704 \nonumber\\
_pos_ngram_PP_PR_PUNC & 0.99705 \nonumber\\
_pos_ngram_V_NN_PP & 0.99708 \nonumber\\
_pos_ngram_NP_NP & 0.99709 \nonumber\\
believe & 0.99710 \nonumber\\
_pos_ngram_PR & 0.99714 \nonumber\\
ProductionRule_SBAR->WHADVP,S, & 0.99716 \nonumber\\
because & 0.99721 \nonumber\\
_pos_ngram_NN_PUNC_ADV & 0.99729 \nonumber\\
_pos_ngram_PR_V_ADJ & 0.99733 \nonumber\\
_pos_ngram_ART_ADJ & 0.99734 \nonumber\\
ProductionRule_NP->PRP$,NN, & 0.99735 \nonumber\\
_pos_ngram_CONJ_NN_PUNC & 0.99736 \nonumber\\
_pos_ngram_PUNC_NP & 0.99738 \nonumber\\
_pos_ngram_PUNC_NP_V & 0.99738 \nonumber\\
it_be & 0.99738 \nonumber\\
debate & 0.99743 \nonumber\\
_pos_ngram_PUNC_V & 0.99754 \nonumber\\
_pos_ngram_PP_V_PUNC & 0.99756 \nonumber\\
_pos_ngram_PP_PR & 0.99762 \nonumber\\
also & 0.99763 \nonumber\\
_pos_ngram_PP_ART_NP & 0.99764 \nonumber\\
_pos_ngram_PR_PUNC_PR & 0.99765 \nonumber\\
_pos_ngram_V_CONJ & 0.99766 \nonumber\\
_pos_ngram_NN_PUNC_V & 0.99767 \nonumber\\
._the & 0.99770 \nonumber\\
_pos_ngram_ADV_ADV_V & 0.99773 \nonumber\\
_pos_ngram_NN_PP_NP & 0.99774 \nonumber\\
he_be & 0.99776 \nonumber\\
_pos_ngram_PUNC_NN_CONJ & 0.99781 \nonumber\\
about & 0.99789 \nonumber\\
this & 0.99791 \nonumber\\
_pos_ngram_ADJ_NN_CONJ & 0.99792 \nonumber\\
_pos_ngram_ADJ_PR & 0.99794 \nonumber\\
FutureVsPastVerbRatio & 0.99800 \nonumber\\
_pos_ngram_O_V & 0.99808 \nonumber\\
_pos_ngram_PR_ADJ_PP & 0.99810 \nonumber\\
de.tudarmstadt.ukp.dkpro.core.api.ner.type.Person & 0.99811 \nonumber\\
_pos_ngram_ART_NN & 0.99812 \nonumber\\
_pos_ngram_ADV_ADV & 0.99812 \nonumber\\
_pos_ngram_ADJ_CONJ_ADJ & 0.99812 \nonumber\\
anything & 0.99815 \nonumber\\
_pos_ngram_PP_PP_ART & 0.99816 \nonumber\\
_pos_ngram_ADV_PP_PR & 0.99817 \nonumber\\
_pos_ngram_CONJ_ADJ & 0.99820 \nonumber\\
_pos_ngram_NN_ADJ_NN & 0.99821 \nonumber\\
have_the & 0.99824 \nonumber\\
_pos_ngram_ART_V_V & 0.99824 \nonumber\\
_pos_ngram_NN_ADV & 0.99825 \nonumber\\
ProductionRule_VP->VBP,ADJP, & 0.99827 \nonumber\\
ProductionRule_VP->VBZ,NP, & 0.99828 \nonumber\\
_pos_ngram_ART_CARD & 0.99832 \nonumber\\
n't & 0.99834 \nonumber\\
_pos_ngram_CONJ_V_NN & 0.99836 \nonumber\\
_pos_ngram_ART_V_PR & 0.99840 \nonumber\\
ProductionRule_ADJP->JJ,PP, & 0.99840 \nonumber\\
be_to & 0.99841 \nonumber\\
like & 0.99841 \nonumber\\
_pos_ngram_ADV_PUNC & 0.99841 \nonumber\\
_pos_ngram_ART_ADJ_ADJ & 0.99842 \nonumber\\
oovWordsCount & 0.99842 \nonumber\\
i_have & 0.99842 \nonumber\\
_pos_ngram_ADV_PUNC_ADV & 0.99843 \nonumber\\
ProductionRule_VP->VBP,S, & 0.99843 \nonumber\\
_pos_ngram_CONJ_V & 0.99843 \nonumber\\
be_better & 0.99844 \nonumber\\
_pos_ngram_PP_NP_V & 0.99850 \nonumber\\
yourself & 0.99850 \nonumber\\
be_a & 0.99851 \nonumber\\
_pos_ngram_CONJ_ART_NN & 0.99851 \nonumber\\
child & 0.99851 \nonumber\\
_pos_ngram_V_PP_ART & 0.99851 \nonumber\\
sorry & 0.99853 \nonumber\\
ProductionRule_VP->MD,VP, & 0.99854 \nonumber\\
_pos_ngram_CONJ_ADV_V & 0.99855 \nonumber\\
for & 0.99856 \nonumber\\
,_i & 0.99856 \nonumber\\
_pos_ngram_NP & 0.99856 \nonumber\\
_pos_ngram_ART_NN_PP & 0.99859 \nonumber\\
but & 0.99859 \nonumber\\
_pos_ngram_ADV_PP_V & 0.99861 \nonumber\\
ProductionRule_VP->VBP,VP, & 0.99862 \nonumber\\
her & 0.99862 \nonumber\\
_pos_ngram_NP_ADV & 0.99863 \nonumber\\
better & 0.99863 \nonumber\\
_pos_ngram_ADV_PUNC_ART & 0.99864 \nonumber\\
_pos_ngram_NN_CONJ_ART & 0.99865 \nonumber\\
_pos_ngram_ADJ_PUNC & 0.99865 \nonumber\\
_pos_ngram_ART_V_ADJ & 0.99865 \nonumber\\
view & 0.99866 \nonumber\\
_pos_ngram_PR_NN_PUNC & 0.99867 \nonumber\\
_pos_ngram_NN_ART_ADJ & 0.99868 \nonumber\\
only & 0.99868 \nonumber\\
should & 0.99869 \nonumber\\
even & 0.99871 \nonumber\\
_pos_ngram_NN_ADV_PR & 0.99871 \nonumber\\
, & 0.99871 \nonumber\\
i_believe & 0.99871 \nonumber\\
but_if & 0.99873 \nonumber\\
it_. & 0.99873 \nonumber\\
help_other & 0.99875 \nonumber\\
_pos_ngram_V_ART & 0.99875 \nonumber\\
something & 0.99877 \nonumber\\
_pos_ngram_CONJ_PP_PR & 0.99879 \nonumber\\
ProductionRule_PP->TO,NP, & 0.99879 \nonumber\\
_pos_ngram_PUNC_PP_PR & 0.99881 \nonumber\\
way & 0.99881 \nonumber\\
he & 0.99881 \nonumber\\
_pos_ngram_NN_NN_NN & 0.99882 \nonumber\\
your & 0.99884 \nonumber\\
ModalVerbCan & 0.99885 \nonumber\\
_pos_ngram_NN_ADV_PUNC & 0.99888 \nonumber\\
yourself_. & 0.99888 \nonumber\\
become & 0.99890 \nonumber\\
_pos_ngram_CARD_NN_PUNC & 0.99890 \nonumber\\
_pos_ngram_ART_V & 0.99890 \nonumber\\
ProductionRule_VP->VB,SBAR, & 0.99891 \nonumber\\
ca & 0.99891 \nonumber\\
ca_n't & 0.99891 \nonumber\\
ProductionRule_VP->TO,VP, & 0.99892 \nonumber\\
need & 0.99892 \nonumber\\
ProductionRule_NP->DT,ADJP,NN, & 0.99893 \nonumber\\
_pos_ngram_ART_ART & 0.99893 \nonumber\\
_pos_ngram_NN_V_PR & 0.99894 \nonumber\\
wrong & 0.99894 \nonumber\\
word_per_sentence & 0.99895 \nonumber\\
_pos_ngram_PUNC_ADJ & 0.99896 \nonumber\\
_pos_ngram_ADJ_V & 0.99897 \nonumber\\
_pos_ngram_PUNC_PP_ADJ & 0.99897 \nonumber\\
_pos_ngram_ADV_PUNC_NN & 0.99898 \nonumber\\
_pos_ngram_ADV & 0.99898 \nonumber\\
their & 0.99898 \nonumber\\
love & 0.99899 \nonumber\\
first & 0.99899 \nonumber\\
_pos_ngram_PR_V & 0.99899 \nonumber\\
on_the & 0.99899 \nonumber\\
do_not & 0.99900 \nonumber\\
i & 0.99900 \nonumber\\
argue & 0.99901 \nonumber\\
,_because & 0.99901 \nonumber\\
_pos_ngram_CONJ_ADV & 0.99904 \nonumber\\
ProductionRule_NP->NN,NNS, & 0.99904 \nonumber\\
_pos_ngram_ART_NP_NP & 0.99905 \nonumber\\
_pos_ngram_ART_ART_NN & 0.99906 \nonumber\\
_pos_ngram_V_NP_NP & 0.99906 \nonumber\\
_pos_ngram_ADJ_NN_PR & 0.99906 \nonumber\\
_pos_ngram_V_O & 0.99906 \nonumber\\
while & 0.99907 \nonumber\\
_pos_ngram_ADV_V_V & 0.99907 \nonumber\\
_pos_ngram_V_ADV_CONJ & 0.99908 \nonumber\\
personal_pursuit & 0.99908 \nonumber\\
i_know & 0.99909 \nonumber\\
_pos_ngram_ADJ_PP_ADJ & 0.99909 \nonumber\\
_pos_ngram_NN_NN_CONJ & 0.99909 \nonumber\\
_pos_ngram_V_V_PR & 0.99910 \nonumber\\
_pos_ngram_V_PR & 0.99910 \nonumber\\
_pos_ngram_PUNC_CONJ_NN & 0.99910 \nonumber\\
pursuit & 0.99910 \nonumber\\
_pos_ngram_PUNC_ADV_PP & 0.99911 \nonumber\\
ProductionRule_ADJP->JJ,S, & 0.99911 \nonumber\\
want & 0.99912 \nonumber\\
_pos_ngram_PP_PP_NN & 0.99912 \nonumber\\
_pos_ngram_PP_ART_PP & 0.99912 \nonumber\\
because_you & 0.99913 \nonumber\\
an & 0.99913 \nonumber\\
personally & 0.99914 \nonumber\\
spank & 0.99914 \nonumber\\
by & 0.99914 \nonumber\\
believe_in & 0.99915 \nonumber\\
answer & 0.99915 \nonumber\\
ProductionRule_ADJP->JJ,SBAR, & 0.99915 \nonumber\\
_pos_ngram_ART_O & 0.99916 \nonumber\\
_pos_ngram_NP_PP_ART & 0.99916 \nonumber\\
it_' & 0.99916 \nonumber\\
be_in & 0.99917 \nonumber\\
what & 0.99917 \nonumber\\
it_do & 0.99917 \nonumber\\
_pos_ngram_NP_PUNC_PR & 0.99917 \nonumber\\
_pos_ngram_ADV_PUNC_PR & 0.99917 \nonumber\\
_pos_ngram_NN_PR_V & 0.99917 \nonumber\\
_pos_ngram_V_NN_O & 0.99917 \nonumber\\
._but & 0.99918 \nonumber\\
,_then & 0.99918 \nonumber\\
kill & 0.99918 \nonumber\\
_pos_ngram_V_PR_ART & 0.99918 \nonumber\\
ProductionRule_S->PP,NP,VP,., & 0.99918 \nonumber\\
_pos_ngram_NN_PR_NN & 0.99918 \nonumber\\
_pos_ngram_CONJ_ADJ_NN & 0.99918 \nonumber\\
ProductionRule_VP->VBD,NP, & 0.99918 \nonumber\\
_pos_ngram_PP_V_ADV & 0.99919 \nonumber\\
we_be & 0.99919 \nonumber\\
there_be & 0.99921 \nonumber\\
_pos_ngram_CARD_NN_PP & 0.99921 \nonumber\\
mistake & 0.99921 \nonumber\\
be_able & 0.99921 \nonumber\\
able_to & 0.99921 \nonumber\\
these & 0.99921 \nonumber\\
know_that & 0.99922 \nonumber\\
_pos_ngram_PP_PUNC_PP & 0.99922 \nonumber\\
_pos_ngram_ADV_ADV_PP & 0.99922 \nonumber\\
_pos_ngram_ART_PP & 0.99922 \nonumber\\
_pos_ngram_PR_ADV_V & 0.99923 \nonumber\\
_pos_ngram_PUNC_PP_V & 0.99923 \nonumber\\
_pos_ngram_PP_PR_ADV & 0.99923 \nonumber\\
you_be & 0.99923 \nonumber\\
be_. & 0.99924 \nonumber\\
_pos_ngram_V_CONJ_PR & 0.99925 \nonumber\\
_pos_ngram_PP_NP_PUNC & 0.99926 \nonumber\\
good & 0.99926 \nonumber\\
_pos_ngram_CONJ_PR_NN & 0.99927 \nonumber\\
_pos_ngram_NN_PP_ADJ & 0.99927 \nonumber\\
_pos_ngram_V_V_V & 0.99927 \nonumber\\
up & 0.99927 \nonumber\\
_pos_ngram_PUNC_CONJ_ADV & 0.99927 \nonumber\\
_pos_ngram_ADJ_PUNC_ADV & 0.99927 \nonumber\\
_pos_ngram_NN_CONJ_PR & 0.99927 \nonumber\\
_pos_ngram_ADJ_PP_NN & 0.99928 \nonumber\\
better_to & 0.99929 \nonumber\\
work & 0.99929 \nonumber\\
be_not & 0.99929 \nonumber\\
able & 0.99929 \nonumber\\
_pos_ngram_NP_NP_NP & 0.99929 \nonumber\\
_pos_ngram_V_NP_PP & 0.99929 \nonumber\\
to_help & 0.99930 \nonumber\\
_pos_ngram_ART_NN_O & 0.99930 \nonumber\\
decide & 0.99930 \nonumber\\
ProductionRule_VP->VB,PP, & 0.99930 \nonumber\\
_pos_ngram_ADV_CONJ & 0.99931 \nonumber\\
out_of & 0.99931 \nonumber\\
like_the & 0.99931 \nonumber\\
happy & 0.99931 \nonumber\\
ProductionRule_ADJP->RB,JJ, & 0.99931 \nonumber\\
_pos_ngram_ART_NN_CONJ & 0.99931 \nonumber\\
_pos_ngram_V_ADV_PUNC & 0.99931 \nonumber\\
_pos_ngram_V_NN_NN & 0.99932 \nonumber\\
for_a & 0.99932 \nonumber\\
_pos_ngram_PP_O & 0.99932 \nonumber\\
_pos_ngram_PP_ART_PUNC & 0.99932 \nonumber\\
most & 0.99932 \nonumber\\
._also & 0.99933 \nonumber\\
founder & 0.99933 \nonumber\\
_pos_ngram_PR_ADJ_PUNC & 0.99933 \nonumber\\
the_one & 0.99934 \nonumber\\
no & 0.99934 \nonumber\\
_pos_ngram_ART_CARD_NN & 0.99935 \nonumber\\
_pos_ngram_V_ADJ_ADJ & 0.99935 \nonumber\\
_pos_ngram_NN_PP & 0.99935 \nonumber\\
even_if & 0.99935 \nonumber\\
_pos_ngram_NP_PP_V & 0.99935 \nonumber\\
_pos_ngram_CONJ_NN_V & 0.99936 \nonumber\\
_pos_ngram_ADV_ADJ_PP & 0.99936 \nonumber\\
_pos_ngram_V_V_ADV & 0.99936 \nonumber\\
_pos_ngram_PUNC_PP_NN & 0.99936 \nonumber\\
hand & 0.99937 \nonumber\\
point & 0.99937 \nonumber\\
they_be & 0.99937 \nonumber\\
_pos_ngram_NN_ADV_ADV & 0.99937 \nonumber\\
argument_be & 0.99938 \nonumber\\
_pos_ngram_PR_NN_CONJ & 0.99938 \nonumber\\
_pos_ngram_NN_NN_V & 0.99938 \nonumber\\
_pos_ngram_PR_V_CONJ & 0.99938 \nonumber\\
ProductionRule_VP->VBZ,PP, & 0.99938 \nonumber\\
_pos_ngram_ADV_V_ART & 0.99938 \nonumber\\
_pos_ngram_PR_PP_ADJ & 0.99939 \nonumber\\
_pos_ngram_V_CONJ_V & 0.99939 \nonumber\\
_pos_ngram_PP_V_ART & 0.99939 \nonumber\\
_pos_ngram_PR_ART_NN & 0.99940 \nonumber\\
ProductionRule_PP->IN,S, & 0.99940 \nonumber\\
_pos_ngram_V_NN_ADV & 0.99940 \nonumber\\
plus & 0.99941 \nonumber\\
_pos_ngram_PR_V_NN & 0.99941 \nonumber\\
personal & 0.99941 \nonumber\\
_pos_ngram_O_PUNC & 0.99941 \nonumber\\
them & 0.99941 \nonumber\\
i_can & 0.99942 \nonumber\\
_pos_ngram_ADJ_ADV_V & 0.99942 \nonumber\\
be_lousy & 0.99942 \nonumber\\
_pos_ngram_CONJ_PR_V & 0.99942 \nonumber\\
_pos_ngram_CONJ_ART & 0.99942 \nonumber\\
now & 0.99942 \nonumber\\
ProductionRule_VP->VP,CC,VP, & 0.99942 \nonumber\\
_pos_ngram_ADV_ART_ADJ & 0.99942 \nonumber\\
i_really & 0.99942 \nonumber\\
she & 0.99942 \nonumber\\
tv_be & 0.99943 \nonumber\\
him_in & 0.99943 \nonumber\\
if & 0.99943 \nonumber\\
_pos_ngram_ART_V_ART & 0.99943 \nonumber\\
you_have & 0.99944 \nonumber\\
_pos_ngram_PR_V_PUNC & 0.99944 \nonumber\\
.... & 0.99944 \nonumber\\
_pos_ngram_ADV_NN & 0.99945 \nonumber\\
ProductionRule_VP->VBP,RB,VP, & 0.99945 \nonumber\\
ProductionRule_VP->VBD,NP,S, & 0.99945 \nonumber\\
3 & 0.99945 \nonumber\\
_pos_ngram_PUNC_V_PP & 0.99945 \nonumber\\
very & 0.99946 \nonumber\\
ProductionRule_NP->NP,PP,SBAR, & 0.99946 \nonumber\\
_pos_ngram_O_O_O & 0.99946 \nonumber\\
ProductionRule_VP->VB,VP, & 0.99946 \nonumber\\
_pos_ngram_NN_V_PUNC & 0.99946 \nonumber\\
_pos_ngram_ADJ_PR_V & 0.99947 \nonumber\\
_pos_ngram_PUNC_NN_NN & 0.99947 \nonumber\\
ProductionRule_NP->NNP,CC,NNP, & 0.99947 \nonumber\\
that_it & 0.99947 \nonumber\\
i_will & 0.99947 \nonumber\\
... & 0.99947 \nonumber\\
with_it & 0.99948 \nonumber\\
out_. & 0.99948 \nonumber\\
_pos_ngram_PUNC_NN_PP & 0.99948 \nonumber\\
_pos_ngram_V_PR_ADV & 0.99948 \nonumber\\
_pos_ngram_NN_ADV_ADJ & 0.99949 \nonumber\\
_pos_ngram_PR_CONJ_V & 0.99949 \nonumber\\
_pos_ngram_O_V_PR & 0.99949 \nonumber\\
ProductionRule_VP->VBZ,ADJP,PP, & 0.99949 \nonumber\\
over & 0.99949 \nonumber\\
_pos_ngram_NN_NN_PUNC & 0.99949 \nonumber\\
_pos_ngram_PP_PR_CONJ & 0.99949 \nonumber\\
ProductionRule_VP->VBZ,ADJP, & 0.99949 \nonumber\\
_pos_ngram_PP_PR_PP & 0.99949 \nonumber\\
_pos_ngram_V_ART_O & 0.99949 \nonumber\\
_pos_ngram_O_V_V & 0.99949 \nonumber\\
_pos_ngram_NN_V_CONJ & 0.99949 \nonumber\\
may_help & 0.99950 \nonumber\\
_pos_ngram_PP_PP_PUNC & 0.99950 \nonumber\\
ProductionRule_VP->VB,NP,SBAR, & 0.99950 \nonumber\\
_pos_ngram_PUNC_ADV_V & 0.99950 \nonumber\\
say & 0.99950 \nonumber\\
not_. & 0.99950 \nonumber\\
provide & 0.99950 \nonumber\\
full & 0.99950 \nonumber\\
_pos_ngram_V_ART_NN & 0.99951 \nonumber\\
i_do & 0.99951 \nonumber\\
_pos_ngram_V_V_PP & 0.99951 \nonumber\\
_pos_ngram_PP_PP_PR & 0.99951 \nonumber\\
? & 0.99951 \nonumber\\
_pos_ngram_ADV_ADJ_PR & 0.99952 \nonumber\\
_pos_ngram_O_PP & 0.99952 \nonumber\\
be_just & 0.99952 \nonumber\\
bid & 0.99952 \nonumber\\
on_this & 0.99952 \nonumber\\
not_a & 0.99952 \nonumber\\
common_good & 0.99952 \nonumber\\
_pos_ngram_PP_ADV_PUNC & 0.99952 \nonumber\\
_pos_ngram_PR_PP_PR & 0.99952 \nonumber\\
argument_on & 0.99952 \nonumber\\
hear & 0.99952 \nonumber\\
find & 0.99953 \nonumber\\
ProductionRule_S->NP,ADVP,VP, & 0.99953 \nonumber\\
_pos_ngram_V_PUNC_PP & 0.99953 \nonumber\\
ignore & 0.99953 \nonumber\\
_pos_ngram_ART_NN_PR & 0.99953 \nonumber\\
_pos_ngram_ART_NP_PP & 0.99953 \nonumber\\
know_what & 0.99953 \nonumber\\
and_a & 0.99953 \nonumber\\
_pos_ngram_ADJ_ADV & 0.99954 \nonumber\\
history & 0.99954 \nonumber\\
will_be & 0.99954 \nonumber\\
._sorry & 0.99954 \nonumber\\
actually & 0.99954 \nonumber\\
_pos_ngram_PP_NN_CONJ & 0.99954 \nonumber\\
_pos_ngram_PP_NN_O & 0.99954 \nonumber\\
_pos_ngram_V_ADV_ART & 0.99954 \nonumber\\
'_not & 0.99954 \nonumber\\
or & 0.99954 \nonumber\\
wrong_. & 0.99955 \nonumber\\
_pos_ngram_PR_ART_V & 0.99955 \nonumber\\
,_it & 0.99955 \nonumber\\
_pos_ngram_ADV_PR_ADV & 0.99955 \nonumber\\
year & 0.99955 \nonumber\\
_pos_ngram_O_NN_PP & 0.99955 \nonumber\\
might & 0.99955 \nonumber\\
_pos_ngram_PP_NN_ART & 0.99955 \nonumber\\
._if & 0.99955 \nonumber\\
'_argument & 0.99955 \nonumber\\
_pos_ngram_PR_PUNC_NN & 0.99955 \nonumber\\
_pos_ngram_ADV_V_O & 0.99955 \nonumber\\
_pos_ngram_CONJ_PP & 0.99955 \nonumber\\
may & 0.99956 \nonumber\\
or_do & 0.99956 \nonumber\\
but_you & 0.99956 \nonumber\\
1 & 0.99956 \nonumber\\
allow & 0.99956 \nonumber\\
think_about & 0.99956 \nonumber\\
big & 0.99956 \nonumber\\
in_my & 0.99957 \nonumber\\
_pos_ngram_V_NP & 0.99957 \nonumber\\
to_do & 0.99957 \nonumber\\
scientific & 0.99957 \nonumber\\
_pos_ngram_NP_CONJ & 0.99957 \nonumber\\
_pos_ngram_NN_O_PP & 0.99957 \nonumber\\
_pos_ngram_ADV_ADV_PUNC & 0.99957 \nonumber\\
_pos_ngram_PR_NN_ADV & 0.99957 \nonumber\\
_pos_ngram_PR_NN_ADJ & 0.99957 \nonumber\\
_pos_ngram_ADJ_PUNC_ADJ & 0.99958 \nonumber\\
_pos_ngram_PUNC_PP_ART & 0.99958 \nonumber\\
never & 0.99958 \nonumber\\
_pos_ngram_PR_NN_PR & 0.99958 \nonumber\\
ProductionRule_VP->VBZ,RB,NP, & 0.99958 \nonumber\\
against & 0.99958 \nonumber\\
grow & 0.99958 \nonumber\\
argument_to & 0.99959 \nonumber\\
something_you & 0.99959 \nonumber\\
ProductionRule_NP->PRP$,JJ,NN, & 0.99959 \nonumber\\
,_you & 0.99959 \nonumber\\
_pos_ngram_PP_ADV_PR & 0.99959 \nonumber\\
_pos_ngram_NN_ART_NN & 0.99959 \nonumber\\
,_" & 0.99959 \nonumber\\
ProductionRule_VP->VBZ,RB,VP, & 0.99959 \nonumber\\
_pos_ngram_ADV_ADJ_NN & 0.99959 \nonumber\\
_pos_ngram_PUNC_CONJ_PP & 0.99959 \nonumber\\
the_parent & 0.99960 \nonumber\\
those & 0.99960 \nonumber\\
_pos_ngram_V_PUNC_PR & 0.99960 \nonumber\\
kid & 0.99960 \nonumber\\
idea & 0.99960 \nonumber\\
argument_and & 0.99960 \nonumber\\
help & 0.99960 \nonumber\\
._a & 0.99960 \nonumber\\
from & 0.99960 \nonumber\\
my_wife & 0.99961 \nonumber\\
the_reason & 0.99961 \nonumber\\
_pos_ngram_PP_ART_ART & 0.99961 \nonumber\\
such & 0.99961 \nonumber\\
each & 0.99961 \nonumber\\
lead & 0.99961 \nonumber\\
sorry_. & 0.99961 \nonumber\\
bottle_water & 0.99961 \nonumber\\
politician & 0.99961 \nonumber\\
_pos_ngram_ADJ_NP_NN & 0.99961 \nonumber\\
to_go & 0.99961 \nonumber\\
of_debate & 0.99961 \nonumber\\
have_n't & 0.99961 \nonumber\\
_pos_ngram_NP_PUNC_ART & 0.99961 \nonumber\\
_pos_ngram_NN_PR & 0.99961 \nonumber\\
human & 0.99961 \nonumber\\
_pos_ngram_NP_O_NN & 0.99962 \nonumber\\
_pos_ngram_PP_ADV & 0.99962 \nonumber\\
ProductionRule_VP->VBD,VP, & 0.99962 \nonumber\\
second & 0.99962 \nonumber\\
_pos_ngram_PR_PUNC_CONJ & 0.99962 \nonumber\\
a_child & 0.99963 \nonumber\\
around & 0.99963 \nonumber\\
_pos_ngram_PP_NN_ADV & 0.99963 \nonumber\\
develop & 0.99963 \nonumber\\
_pos_ngram_PR_PR & 0.99963 \nonumber\\
_pos_ngram_ART_PUNC_PR & 0.99963 \nonumber\\
_pos_ngram_ADJ_NN_ADJ & 0.99963 \nonumber\\
the_need & 0.99963 \nonumber\\
you_, & 0.99963 \nonumber\\
_pos_ngram_O_PUNC_CONJ & 0.99963 \nonumber\\
to_someone & 0.99963 \nonumber\\
_pos_ngram_NN_V_CARD & 0.99963 \nonumber\\
that_you & 0.99963 \nonumber\\
_pos_ngram_NP_PR_V & 0.99963 \nonumber\\
wife & 0.99963 \nonumber\\
since & 0.99964 \nonumber\\
raffle_be & 0.99964 \nonumber\\
_pos_ngram_ART_PUNC & 0.99964 \nonumber\\
rebuttal & 0.99964 \nonumber\\
_pos_ngram_O_ART_NN & 0.99964 \nonumber\\
and_be & 0.99964 \nonumber\\
also_, & 0.99964 \nonumber\\
_pos_ngram_PR_NN_NN & 0.99964 \nonumber\\
_pos_ngram_PR_PP_PUNC & 0.99964 \nonumber\\
because_they & 0.99964 \nonumber\\
_pos_ngram_PP_NN_NP & 0.99964 \nonumber\\
really_do & 0.99964 \nonumber\\
believe_that & 0.99965 \nonumber\\
get & 0.99965 \nonumber\\
think_it & 0.99965 \nonumber\\
case & 0.99965 \nonumber\\
you_can & 0.99965 \nonumber\\
just_ignore & 0.99965 \nonumber\\
_pos_ngram_ART_V_ADV & 0.99965 \nonumber\\
_pos_ngram_V_ART_CARD & 0.99965 \nonumber\\
be_that & 0.99965 \nonumber\\
expect & 0.99965 \nonumber\\
_pos_ngram_NN_V_O & 0.99965 \nonumber\\
example & 0.99965 \nonumber\\
ProductionRule_UCP->NP,CC,S, & 0.99965 \nonumber\\
murder & 0.99965 \nonumber\\
kill_someone & 0.99966 \nonumber\\
_pos_ngram_ADV_PP_ART & 0.99966 \nonumber\\
to_you & 0.99966 \nonumber\\
ProductionRule_S->NP,VP,:, & 0.99966 \nonumber\\
you_would & 0.99966 \nonumber\\
through & 0.99966 \nonumber\\
_pos_ngram_ADJ_NP & 0.99966 \nonumber\\
_pos_ngram_NN_NP_NP & 0.99966 \nonumber\\
_pos_ngram_CONJ_V_PR & 0.99966 \nonumber\\
it_, & 0.99966 \nonumber\\
for_that & 0.99966 \nonumber\\
than & 0.99966 \nonumber\\
_pos_ngram_NP_NP_V & 0.99966 \nonumber\\
help_that & 0.99966 \nonumber\\
ProductionRule_VP->VBZ,PP,SBAR, & 0.99966 \nonumber\\
to_wear & 0.99967 \nonumber\\
sun & 0.99967 \nonumber\\
_pos_ngram_PR_V_NP & 0.99967 \nonumber\\
_pos_ngram_PR_PP_PP & 0.99967 \nonumber\\
_pos_ngram_PR_PUNC_ART & 0.99967 \nonumber\\
talk_about & 0.99967 \nonumber\\
to_write & 0.99967 \nonumber\\
to_think & 0.99967 \nonumber\\
love_. & 0.99967 \nonumber\\
_pos_ngram_NN_PUNC_NP & 0.99967 \nonumber\\
have_already & 0.99967 \nonumber\\
_pos_ngram_PR_PP_ADV & 0.99967 \nonumber\\
click & 0.99968 \nonumber\\
stay & 0.99968 \nonumber\\
_pos_ngram_PR_PR_NN & 0.99968 \nonumber\\
_pos_ngram_NN_PP_PR & 0.99968 \nonumber\\
,_or & 0.99968 \nonumber\\
_pos_ngram_ART_PP_ART & 0.99968 \nonumber\\
it_may & 0.99968 \nonumber\\
_pos_ngram_O_PUNC_PR & 0.99968 \nonumber\\
be_go & 0.99968 \nonumber\\
do_that & 0.99968 \nonumber\\
easier & 0.99968 \nonumber\\
baby & 0.99968 \nonumber\\
indium_be & 0.99968 \nonumber\\
they_have & 0.99968 \nonumber\\
_pos_ngram_NP_V_NP & 0.99968 \nonumber\\
country & 0.99968 \nonumber\\
_pos_ngram_ADV_ADV_ADV & 0.99968 \nonumber\\
else & 0.99968 \nonumber\\
on_you & 0.99968 \nonumber\\
be_ok & 0.99968 \nonumber\\
raise & 0.99969 \nonumber\\
question & 0.99969 \nonumber\\
goal & 0.99969 \nonumber\\
anything_. & 0.99969 \nonumber\\
say_that & 0.99969 \nonumber\\
woman & 0.99969 \nonumber\\
_pos_ngram_ADV_PP_NN & 0.99969 \nonumber\\
_pos_ngram_NN_NN_ART & 0.99969 \nonumber\\
about_it & 0.99969 \nonumber\\
_pos_ngram_V_NN_V & 0.99969 \nonumber\\
rebuttal_to & 0.99969 \nonumber\\
church_and & 0.99969 \nonumber\\
to_become & 0.99969 \nonumber\\
father & 0.99969 \nonumber\\
eliminate_the & 0.99970 \nonumber\\
history_of & 0.99970 \nonumber\\
a_less & 0.99970 \nonumber\\
themselve_by & 0.99970 \nonumber\\
a_history & 0.99970 \nonumber\\
_pos_ngram_ART_O_ADV & 0.99970 \nonumber\\
ProductionRule_VP->VB,RB,VP, & 0.99970 \nonumber\\
then_click & 0.99970 \nonumber\\
n't_or & 0.99970 \nonumber\\
respond_to & 0.99970 \nonumber\\
n't_respond & 0.99970 \nonumber\\
all_" & 0.99970 \nonumber\\
abortion_.... & 0.99970 \nonumber\\
against_. & 0.99970 \nonumber\\
here_, & 0.99970 \nonumber\\
on_here & 0.99970 \nonumber\\
that_singthestory & 0.99970 \nonumber\\
...._funny & 0.99970 \nonumber\\
explanation_of & 0.99970 \nonumber\\
their_argument & 0.99970 \nonumber\\
ignore_what & 0.99970 \nonumber\\
singthestory & 0.99970 \nonumber\\
singthestory_and & 0.99970 \nonumber\\
view_all & 0.99970 \nonumber\\
of_why & 0.99970 \nonumber\\
this_give & 0.99970 \nonumber\\
sibtiger_have & 0.99970 \nonumber\\
find_adoption & 0.99970 \nonumber\\
repeat_themselve & 0.99970 \nonumber\\
interest_that & 0.99970 \nonumber\\
by_address & 0.99970 \nonumber\\
_pos_ngram_PUNC_CARD_ADJ & 0.99970 \nonumber\\
sibtiger & 0.99970 \nonumber\\
thing_: & 0.99970 \nonumber\\
something_they & 0.99970 \nonumber\\
ProductionRule_VP->VBP,NP,UCP, & 0.99970 \nonumber\\
ProductionRule_ADVP->JJR,IN, & 0.99970 \nonumber\\
alternative & 0.99970 \nonumber\\
than_desirable & 0.99970 \nonumber\\
alternative_to & 0.99970 \nonumber\\
a_rebuttal & 0.99970 \nonumber\\
desirable & 0.99970 \nonumber\\
desirable_alternative & 0.99970 \nonumber\\
adoption_a & 0.99970 \nonumber\\
ProductionRule_S->FRAG,:,S,., & 0.99970 \nonumber\\
"_view & 0.99970 \nonumber\\
and_sibtiger & 0.99970 \nonumber\\
my_explanation & 0.99970 \nonumber\\
_pos_ngram_NP_ADV_NN & 0.99970 \nonumber\\
ProductionRule_NP->CD,JJR,NN, & 0.99970 \nonumber\\
funny_how & 0.99970 \nonumber\\
click_" & 0.99970 \nonumber\\
ProductionRule_FRAG->ADJP,,,NP, & 0.99970 \nonumber\\
need_for & 0.99970 \nonumber\\
already_address & 0.99970 \nonumber\\
more_thing & 0.99970 \nonumber\\
one_more & 0.99970 \nonumber\\
address_something & 0.99970 \nonumber\\
"_first & 0.99970 \nonumber\\
sorry_, & 0.99970 \nonumber\\
write_a & 0.99970 \nonumber\\
ProductionRule_NP->DT,JJ,NNS, & 0.99970 \nonumber\\
_pos_ngram_NP_V_ADV & 0.99970 \nonumber\\
_pos_ngram_CONJ_V_PP & 0.99970 \nonumber\\
the_common & 0.99970 \nonumber\\
_pos_ngram_ADV_V_NP & 0.99970 \nonumber\\
learn & 0.99970 \nonumber\\
_pos_ngram_NN_NN_ADV & 0.99970 \nonumber\\
your_argument & 0.99970 \nonumber\\
consider & 0.99970 \nonumber\\
._people & 0.99970 \nonumber\\
_pos_ngram_PP_CONJ & 0.99970 \nonumber\\
_pos_ngram_PUNC_PR_ADV & 0.99970 \nonumber\\
comment & 0.99970 \nonumber\\
my & 0.99970 \nonumber\\
agree & 0.99970 \nonumber\\
address_. & 0.99970 \nonumber\\
ProductionRule_VP->MD,RB, & 0.99970 \nonumber\\
'_interest & 0.99970 \nonumber\\
assume_that & 0.99970 \nonumber\\
because_the & 0.99970 \nonumber\\
all_. & 0.99970 \nonumber\\
_pos_ngram_O_PUNC_ART & 0.99970 \nonumber\\
funny & 0.99970 \nonumber\\
in_singapore & 0.99970 \nonumber\\
because_if & 0.99971 \nonumber\\
answer_. & 0.99971 \nonumber\\
'_a & 0.99971 \nonumber\\
to_repeat & 0.99971 \nonumber\\
repeat & 0.99971 \nonumber\\
who_you & 0.99971 \nonumber\\
find_out & 0.99971 \nonumber\\
how_people & 0.99971 \nonumber\\
and_they & 0.99971 \nonumber\\
_pos_ngram_PUNC_PR_ADJ & 0.99971 \nonumber\\
Emb_dimension_109 & 0.99971 \nonumber\\
the_family & 0.99971 \nonumber\\
_pos_ngram_NN_NP & 0.99971 \nonumber\\
wish & 0.99971 \nonumber\\
- & 0.99971 \nonumber\\
random & 0.99971 \nonumber\\
of_singapore & 0.99971 \nonumber\\
ok & 0.99971 \nonumber\\
that_' & 0.99971 \nonumber\\
a_lousy & 0.99971 \nonumber\\
and_i & 0.99971 \nonumber\\
_pos_ngram_PR_O & 0.99971 \nonumber\\
give & 0.99971 \nonumber\\
ProductionRule_ADJP->ADVP,JJ, & 0.99972 \nonumber\\
people_just & 0.99972 \nonumber\\
_pos_ngram_PUNC_ADJ_NN & 0.99972 \nonumber\\
do_it & 0.99972 \nonumber\\
_pos_ngram_NN_NN_O & 0.99972 \nonumber\\
sentence_length & 0.99972 \nonumber\\
do_anything & 0.99972 \nonumber\\
full_of & 0.99972 \nonumber\\
_pos_ngram_PR_ADV_PP & 0.99972 \nonumber\\
_pos_ngram_CONJ_ART_V & 0.99972 \nonumber\\
american & 0.99972 \nonumber\\
_pos_ngram_V_O_O & 0.99972 \nonumber\\
_pos_ngram_ADV_NN_ADV & 0.99972 \nonumber\\
mean & 0.99972 \nonumber\\
him & 0.99972 \nonumber\\
which_be & 0.99972 \nonumber\\
do_with & 0.99972 \nonumber\\
respond & 0.99972 \nonumber\\
which & 0.99972 \nonumber\\
the_founder & 0.99973 \nonumber\\
the_most & 0.99973 \nonumber\\
_pos_ngram_CARD_ADJ & 0.99973 \nonumber\\
_pos_ngram_V_NN_CONJ & 0.99973 \nonumber\\
its_better & 0.99973 \nonumber\\
_pos_ngram_PUNC_CARD_NN & 0.99973 \nonumber\\
debate_. & 0.99973 \nonumber\\
technique & 0.99973 \nonumber\\
person_to & 0.99973 \nonumber\\
you_ca & 0.99973 \nonumber\\
in_life & 0.99973 \nonumber\\
help_to & 0.99973 \nonumber\\
problem & 0.99973 \nonumber\\
_pos_ngram_ADJ_PUNC_CONJ & 0.99973 \nonumber\\
_pos_ngram_NN_PR_PP & 0.99973 \nonumber\\
ProductionRule_NP->NNP,NNP, & 0.99973 \nonumber\\
_pos_ngram_O_ADJ_O & 0.99973 \nonumber\\
your_family & 0.99973 \nonumber\\
who & 0.99973 \nonumber\\
_pos_ngram_PUNC_ART_O & 0.99973 \nonumber\\
information & 0.99973 \nonumber\\
i_say & 0.99973 \nonumber\\
_pos_ngram_ART_O_NN & 0.99973 \nonumber\\
to_kill & 0.99974 \nonumber\\
forever & 0.99974 \nonumber\\
anyone & 0.99974 \nonumber\\
_pos_ngram_ADJ_NN_ADV & 0.99974 \nonumber\\
_pos_ngram_NP_V_V & 0.99974 \nonumber\\
you_think & 0.99974 \nonumber\\
and_we & 0.99974 \nonumber\\
_pos_ngram_O_ADV_PUNC & 0.99974 \nonumber\\
eliminate & 0.99974 \nonumber\\
right_now & 0.99974 \nonumber\\
use_the & 0.99974 \nonumber\\
put & 0.99974 \nonumber\\
enough & 0.99974 \nonumber\\
much & 0.99974 \nonumber\\
would_be & 0.99974 \nonumber\\
advance & 0.99974 \nonumber\\
ProductionRule_NP->NP,S, & 0.99974 \nonumber\\
_pos_ngram_O_PUNC_NN & 0.99974 \nonumber\\
._there & 0.99974 \nonumber\\
ProductionRule_NP->NN,NNP,NNP, & 0.99974 \nonumber\\
to_eliminate & 0.99974 \nonumber\\
_pos_ngram_NN_PUNC_CARD & 0.99974 \nonumber\\
by_the & 0.99974 \nonumber\\
do_no & 0.99974 \nonumber\\
quality & 0.99974 \nonumber\\
you_do & 0.99974 \nonumber\\
think_that & 0.99974 \nonumber\\
_pos_ngram_V_ADJ_ADV & 0.99975 \nonumber\\
better_than & 0.99975 \nonumber\\
know_who & 0.99975 \nonumber\\
'_. & 0.99975 \nonumber\\
to_argue & 0.99975 \nonumber\\
be_so & 0.99975 \nonumber\\
_pos_ngram_O_CARD_NN & 0.99975 \nonumber\\
_pos_ngram_ADJ_CONJ_ADV & 0.99975 \nonumber\\
_pos_ngram_NN_PR_PUNC & 0.99975 \nonumber\\
your_claim & 0.99975 \nonumber\\
have_no & 0.99975 \nonumber\\
,_for & 0.99975 \nonumber\\
on_your & 0.99975 \nonumber\\
degrade & 0.99975 \nonumber\\
_pos_ngram_CONJ_NP_CONJ & 0.99975 \nonumber\\
ask & 0.99975 \nonumber\\
_pos_ngram_PUNC_PP_PP & 0.99975 \nonumber\\
sarcastic & 0.99975 \nonumber\\
happen & 0.99975 \nonumber\\
_pos_ngram_NP_V_PP & 0.99975 \nonumber\\
_pos_ngram_ADV_V_NN & 0.99975 \nonumber\\
should_be & 0.99975 \nonumber\\
religious & 0.99975 \nonumber\\
to_say & 0.99975 \nonumber\\
any & 0.99976 \nonumber\\
_pos_ngram_PUNC_ADJ_PUNC & 0.99976 \nonumber\\
_pos_ngram_V_PP_ADV & 0.99976 \nonumber\\
good_be & 0.99976 \nonumber\\
between & 0.99976 \nonumber\\
_pos_ngram_PUNC_ART_ADJ & 0.99976 \nonumber\\
realize & 0.99976 \nonumber\\
: & 0.99976 \nonumber\\
ProductionRule_ADJP->ADJP,SBAR, & 0.99976 \nonumber\\
however & 0.99976 \nonumber\\
blood & 0.99976 \nonumber\\
ModalVerbsUncertain & 0.99976 \nonumber\\
lifestyle & 0.99976 \nonumber\\
_pos_ngram_NP_NP_ADV & 0.99976 \nonumber\\
_pos_ngram_ART_O_O & 0.99976 \nonumber\\
_pos_ngram_NP_PUNC_V & 0.99976 \nonumber\\
still & 0.99976 \nonumber\\
experience & 0.99976 \nonumber\\
_pos_ngram_ART_ADV_V & 0.99976 \nonumber\\
we_would & 0.99976 \nonumber\\
_pos_ngram_ADV_O_PUNC & 0.99976 \nonumber\\
commit & 0.99976 \nonumber\\
under & 0.99976 \nonumber\\
sabrejimmy & 0.99976 \nonumber\\
na & 0.99976 \nonumber\\
commit_murder & 0.99976 \nonumber\\
cancer & 0.99976 \nonumber\\
_pos_ngram_NN_O_CARD & 0.99976 \nonumber\\
not_know & 0.99976 \nonumber\\
under_the & 0.99976 \nonumber\\
other_. & 0.99976 \nonumber\\
interest & 0.99976 \nonumber\\
ProductionRule_NP->DT,JJ,JJ,NN, & 0.99976 \nonumber\\
,_we & 0.99976 \nonumber\\
terrorist & 0.99977 \nonumber\\
side & 0.99977 \nonumber\\
no_matter & 0.99977 \nonumber\\
argue_against & 0.99977 \nonumber\\
pro & 0.99977 \nonumber\\
ProductionRule_NP->ADJP,NNS, & 0.99977 \nonumber\\
you_cant & 0.99977 \nonumber\\
early & 0.99977 \nonumber\\
around_. & 0.99977 \nonumber\\
talk & 0.99977 \nonumber\\
_pos_ngram_V_ADJ_CONJ & 0.99977 \nonumber\\
this_argument & 0.99977 \nonumber\\
time & 0.99977 \nonumber\\
a_better & 0.99977 \nonumber\\
_pos_ngram_CONJ_O & 0.99977 \nonumber\\
_pos_ngram_NP_NN_PUNC & 0.99977 \nonumber\\
i_find & 0.99977 \nonumber\\
may_be & 0.99977 \nonumber\\
can_show & 0.99977 \nonumber\\
_pos_ngram_V_PUNC_NP & 0.99977 \nonumber\\
ProductionRule_VP->VBN,NP, & 0.99977 \nonumber\\
" & 0.99977 \nonumber\\
example_, & 0.99977 \nonumber\\
problem_, & 0.99977 \nonumber\\
,_if & 0.99977 \nonumber\\
_pos_ngram_PP_ADJ_PUNC & 0.99978 \nonumber\\
just & 0.99978 \nonumber\\
they_ca & 0.99978 \nonumber\\
_pos_ngram_PUNC_PUNC_ADV & 0.99978 \nonumber\\
live & 0.99978 \nonumber\\
_pos_ngram_NN_NN_ADJ & 0.99978 \nonumber\\
less_than & 0.99978 \nonumber\\
right_to & 0.99978 \nonumber\\
to_a & 0.99978 \nonumber\\
first_before & 0.99978 \nonumber\\
be_you & 0.99978 \nonumber\\
commitment & 0.99978 \nonumber\\
need_at & 0.99978 \nonumber\\
_pos_ngram_PP_NP_PP & 0.99978 \nonumber\\
_pos_ngram_O_PP_ART & 0.99978 \nonumber\\
to_express & 0.99978 \nonumber\\
that_a & 0.99978 \nonumber\\
,_one & 0.99978 \nonumber\\
there_. & 0.99978 \nonumber\\
post & 0.99978 \nonumber\\
rights & 0.99978 \nonumber\\
_pos_ngram_NP_PUNC_NP & 0.99978 \nonumber\\
him_. & 0.99978 \nonumber\\
ProductionRule_NP->JJR,NNS, & 0.99978 \nonumber\\
_pos_ngram_NN_PUNC_CONJ & 0.99978 \nonumber\\
n't_understand & 0.99978 \nonumber\\
of_school & 0.99978 \nonumber\\
of_something & 0.99978 \nonumber\\
most_of & 0.99978 \nonumber\\
_pos_ngram_PR_ADV_PR & 0.99978 \nonumber\\
matter & 0.99978 \nonumber\\
waste & 0.99978 \nonumber\\
with_her & 0.99978 \nonumber\\
the_day & 0.99978 \nonumber\\
farquhar_. & 0.99978 \nonumber\\
sure_that & 0.99979 \nonumber\\
_pos_ngram_ADV_V_CONJ & 0.99979 \nonumber\\
ProductionRule_VP->VBZ,ADJP,NP, & 0.99979 \nonumber\\
_pos_ngram_ADJ_CONJ_PR & 0.99979 \nonumber\\
adoption & 0.99979 \nonumber\\
of_the & 0.99979 \nonumber\\
explanation & 0.99979 \nonumber\\
_pos_ngram_V_ART_PR & 0.99979 \nonumber\\
with_the & 0.99979 \nonumber\\
what_he & 0.99979 \nonumber\\
terrible & 0.99979 \nonumber\\
ProductionRule_PP->IN,SBAR, & 0.99979 \nonumber\\
about_other & 0.99979 \nonumber\\
i_make & 0.99979 \nonumber\\
same_time & 0.99979 \nonumber\\
_pos_ngram_PP_O_NN & 0.99979 \nonumber\\
be_much & 0.99979 \nonumber\\
that_human & 0.99979 \nonumber\\
room & 0.99979 \nonumber\\
_pos_ngram_CARD_ADJ_NN & 0.99979 \nonumber\\
who_say & 0.99979 \nonumber\\
why_we & 0.99979 \nonumber\\
,_there & 0.99979 \nonumber\\
greater & 0.99979 \nonumber\\
singapore & 0.99979 \nonumber\\
shape & 0.99979 \nonumber\\
new & 0.99979 \nonumber\\
_pos_ngram_CARD_V_ART & 0.99979 \nonumber\\
_pos_ngram_V_ADV_NN & 0.99979 \nonumber\\
issue & 0.99979 \nonumber\\
down & 0.99979 \nonumber\\
_pos_ngram_ADV_NN_V & 0.99979 \nonumber\\
_pos_ngram_O_PR & 0.99979 \nonumber\\
honestly & 0.99979 \nonumber\\
place & 0.99979 \nonumber\\
end & 0.99979 \nonumber\\
comment_. & 0.99979 \nonumber\\
matter_what & 0.99979 \nonumber\\
ProductionRule_VP->VBP,NP, & 0.99979 \nonumber\\
without & 0.99979 \nonumber\\
to_lead & 0.99979 \nonumber\\
_pos_ngram_ART_PP_PR & 0.99979 \nonumber\\
_pos_ngram_V_ART_PUNC & 0.99980 \nonumber\\
hit & 0.99980 \nonumber\\
,_why & 0.99980 \nonumber\\
you & 0.99980 \nonumber\\
as_someone & 0.99980 \nonumber\\
_pos_ngram_O_V_NN & 0.99980 \nonumber\\
would_have & 0.99980 \nonumber\\
the_debate & 0.99980 \nonumber\\
be_talk & 0.99980 \nonumber\\
father_as & 0.99980 \nonumber\\
nothing & 0.99980 \nonumber\\
something_then & 0.99980 \nonumber\\
before_anyone & 0.99980 \nonumber\\
that_family & 0.99980 \nonumber\\
be_relate & 0.99980 \nonumber\\
blood_. & 0.99980 \nonumber\\
member_out & 0.99980 \nonumber\\
relate & 0.99980 \nonumber\\
what_because & 0.99980 \nonumber\\
relate_to & 0.99980 \nonumber\\
be_blood & 0.99980 \nonumber\\
out_instead & 0.99980 \nonumber\\
time_as & 0.99980 \nonumber\\
just_something & 0.99980 \nonumber\\
anything_help & 0.99980 \nonumber\\
the_random & 0.99980 \nonumber\\
know_be & 0.99980 \nonumber\\
random_person & 0.99980 \nonumber\\
pursuit_should & 0.99980 \nonumber\\
_pos_ngram_V_NN_ADJ & 0.99980 \nonumber\\
_pos_ngram_ART_ADJ_PR & 0.99980 \nonumber\\
today & 0.99980 \nonumber\\
a_mother & 0.99980 \nonumber\\
if_he & 0.99980 \nonumber\\
of_their & 0.99980 \nonumber\\
there_have & 0.99980 \nonumber\\
completely & 0.99980 \nonumber\\
_pos_ngram_ART_NN_ART & 0.99980 \nonumber\\
attempt & 0.99980 \nonumber\\
the_" & 0.99980 \nonumber\\
religion_, & 0.99980 \nonumber\\
it_again & 0.99980 \nonumber\\
mind & 0.99980 \nonumber\\
ProductionRule_VP->VB,NP,PP, & 0.99980 \nonumber\\
come_first & 0.99980 \nonumber\\
! & 0.99980 \nonumber\\
focus & 0.99980 \nonumber\\
_pos_ngram_PUNC_V_ART & 0.99980 \nonumber\\
me_i & 0.99980 \nonumber\\
,_instead & 0.99980 \nonumber\\
attempt_to & 0.99980 \nonumber\\
guess & 0.99980 \nonumber\\
_pos_ngram_PUNC_NP_NN & 0.99980 \nonumber\\
_pos_ngram_V_CARD & 0.99980 \nonumber\\
_pos_ngram_V_NP_V & 0.99980 \nonumber\\
family_be & 0.99980 \nonumber\\
thousand & 0.99980 \nonumber\\
to_hit & 0.99980 \nonumber\\
deal & 0.99980 \nonumber\\
community & 0.99980 \nonumber\\
be_no & 0.99980 \nonumber\\
opposite & 0.99980 \nonumber\\
_pos_ngram_V_ART_ART & 0.99980 \nonumber\\
again_i & 0.99980 \nonumber\\
_pos_ngram_CONJ_NP & 0.99980 \nonumber\\
endeavor_. & 0.99980 \nonumber\\
achieve & 0.99980 \nonumber\\
happy_. & 0.99980 \nonumber\\
_pos_ngram_NP_NP_PUNC & 0.99980 \nonumber\\
farquhar_have & 0.99980 \nonumber\\
indisputable & 0.99980 \nonumber\\
self & 0.99980 \nonumber\\
ProductionRule_NP->DT,NN,NN, & 0.99981 \nonumber\\
any_way & 0.99981 \nonumber\\
form & 0.99981 \nonumber\\
understand_anything & 0.99981 \nonumber\\
you_just & 0.99981 \nonumber\\
soldier & 0.99981 \nonumber\\
you_in & 0.99981 \nonumber\\
the_potential & 0.99981 \nonumber\\
?_in & 0.99981 \nonumber\\
this_debate & 0.99981 \nonumber\\
the_same & 0.99981 \nonumber\\
?_i & 0.99981 \nonumber\\
common & 0.99981 \nonumber\\
_pos_ngram_O_ADV_PR & 0.99981 \nonumber\\
_pos_ngram_NN_ADJ_PUNC & 0.99981 \nonumber\\
look & 0.99981 \nonumber\\
to_not & 0.99981 \nonumber\\
change_. & 0.99981 \nonumber\\
1_. & 0.99981 \nonumber\\
advance_the & 0.99981 \nonumber\\
see_it & 0.99981 \nonumber\\
day_when & 0.99981 \nonumber\\
_pos_ngram_O_O_V & 0.99981 \nonumber\\
should_come & 0.99981 \nonumber\\
i_feel & 0.99981 \nonumber\\
_pos_ngram_NN_O_ADV & 0.99981 \nonumber\\
_pos_ngram_CARD_PUNC & 0.99981 \nonumber\\
_pos_ngram_NN_NN_PR & 0.99981 \nonumber\\
ProductionRule_VP->VBG,PP, & 0.99982 \nonumber\\
probably & 0.99982 \nonumber\\
_pos_ngram_V_V_NP & 0.99982 \nonumber\\
_pos_ngram_PUNC_CONJ_NP & 0.99982 \nonumber\\
choice_. & 0.99982 \nonumber\\
simply & 0.99982 \nonumber\\
_pos_ngram_PUNC_V_ADV & 0.99982 \nonumber\\
the_baby & 0.99982 \nonumber\\
someone & 0.99982 \nonumber\\
individuality_. & 0.99982 \nonumber\\
can_not & 0.99982 \nonumber\\
in_hand & 0.99982 \nonumber\\
become_a & 0.99982 \nonumber\\
_pos_ngram_ADV_PP_PP & 0.99982 \nonumber\\
people_on & 0.99982 \nonumber\\
be_n't & 0.99982 \nonumber\\
be_cool & 0.99982 \nonumber\\
ProductionRule_NP->NP,PP,PP, & 0.99982 \nonumber\\
then_again & 0.99982 \nonumber\\
;_) & 0.99982 \nonumber\\
ProductionRule_NP->NN,POS, & 0.99982 \nonumber\\
god_, & 0.99982 \nonumber\\
._book & 0.99982 \nonumber\\
all_the & 0.99982 \nonumber\\
wear_the & 0.99982 \nonumber\\
do_. & 0.99982 \nonumber\\
law & 0.99982 \nonumber\\
for_example & 0.99982 \nonumber\\
_pos_ngram_ADJ_PUNC_CARD & 0.99982 \nonumber\\
crap & 0.99982 \nonumber\\
focus_on & 0.99982 \nonumber\\
family_member & 0.99982 \nonumber\\
debate_be & 0.99982 \nonumber\\
how_come & 0.99982 \nonumber\\
_pos_ngram_ART_V_NN & 0.99982 \nonumber\\
_pos_ngram_PUNC_ADV_PUNC & 0.99982 \nonumber\\
my_father & 0.99982 \nonumber\\
_pos_ngram_PP_ART_CARD & 0.99982 \nonumber\\
:_i & 0.99982 \nonumber\\
be_out & 0.99983 \nonumber\\
way_to & 0.99983 \nonumber\\
_pos_ngram_V_PUNC_O & 0.99983 \nonumber\\
to_abortion & 0.99983 \nonumber\\
why_i & 0.99983 \nonumber\\
person_you & 0.99983 \nonumber\\
this_be & 0.99983 \nonumber\\
that_person & 0.99983 \nonumber\\
care_about & 0.99983 \nonumber\\
wonder & 0.99983 \nonumber\\
that_make & 0.99983 \nonumber\\
_pos_ngram_ART_PP_NN & 0.99983 \nonumber\\
_pos_ngram_PP_PP_V & 0.99983 \nonumber\\
write & 0.99983 \nonumber\\
morn & 0.99983 \nonumber\\
sure & 0.99983 \nonumber\\
ProductionRule_NP->DT,JJS,NN, & 0.99983 \nonumber\\
to_my & 0.99983 \nonumber\\
father_than & 0.99983 \nonumber\\
potential_to & 0.99983 \nonumber\\
_pos_ngram_NN_PR_PR & 0.99983 \nonumber\\
_pos_ngram_PUNC_ADJ_PP & 0.99983 \nonumber\\
someone_in & 0.99983 \nonumber\\
if_nothing & 0.99983 \nonumber\\
nothing_else & 0.99983 \nonumber\\
christianity & 0.99983 \nonumber\\
_pos_ngram_PR_ART & 0.99983 \nonumber\\
of_a & 0.99983 \nonumber\\
what_be & 0.99983 \nonumber\\
cool & 0.99983 \nonumber\\
be_easier & 0.99983 \nonumber\\
same & 0.99983 \nonumber\\
_pos_ngram_CONJ_V_ART & 0.99983 \nonumber\\
._who & 0.99983 \nonumber\\
in_any & 0.99983 \nonumber\\
_pos_ngram_PUNC_ADV_NP & 0.99983 \nonumber\\
._( & 0.99983 \nonumber\\
dumb & 0.99983 \nonumber\\
perfect & 0.99983 \nonumber\\
_pos_ngram_PP_NN_CARD & 0.99983 \nonumber\\
founder_of & 0.99983 \nonumber\\
like_tv & 0.99983 \nonumber\\
claim & 0.99983 \nonumber\\
she_have & 0.99983 \nonumber\\
else_' & 0.99983 \nonumber\\
2_. & 0.99983 \nonumber\\
ModalVerbsRatio & 0.99983 \nonumber\\
_pos_ngram_NP_NN_V & 0.99983 \nonumber\\
ProductionRule_VP->VB,ADVP, & 0.99983 \nonumber\\
i_guess & 0.99983 \nonumber\\
._and & 0.99983 \nonumber\\
will_have & 0.99983 \nonumber\\
here & 0.99983 \nonumber\\
species & 0.99983 \nonumber\\
possible & 0.99983 \nonumber\\
my_argument & 0.99983 \nonumber\\
_pos_ngram_PR_ADJ_NN & 0.99983 \nonumber\\
you_get & 0.99984 \nonumber\\
from_him & 0.99984 \nonumber\\
for_the & 0.99984 \nonumber\\
a_woman & 0.99984 \nonumber\\
ProductionRule_VP->VBZ,ADJP,SBAR, & 0.99984 \nonumber\\
sexual & 0.99984 \nonumber\\
._just & 0.99984 \nonumber\\
_pos_ngram_ADV_PR_PP & 0.99984 \nonumber\\
_pos_ngram_PP_PR_ART & 0.99984 \nonumber\\
_pos_ngram_PUNC_V_ADJ & 0.99984 \nonumber\\
lesbian & 0.99984 \nonumber\\
_pos_ngram_PP_PUNC & 0.99984 \nonumber\\
one & 0.99984 \nonumber\\
on_tv & 0.99984 \nonumber\\
child_. & 0.99984 \nonumber\\
because_a & 0.99984 \nonumber\\
know_, & 0.99984 \nonumber\\
get_to & 0.99984 \nonumber\\
all_i & 0.99984 \nonumber\\
understand & 0.99984 \nonumber\\
i_personally & 0.99984 \nonumber\\
of_argument & 0.99984 \nonumber\\
_pos_ngram_ADV_CARD_PUNC & 0.99984 \nonumber\\
_pos_ngram_CONJ_ADJ_PUNC & 0.99984 \nonumber\\
ProductionRule_S->ADVP,NP,VP,., & 0.99984 \nonumber\\
on_how & 0.99984 \nonumber\\
get_spank & 0.99984 \nonumber\\
almost & 0.99984 \nonumber\\
_pos_ngram_ART_NN_ADV & 0.99984 \nonumber\\
_pos_ngram_NP_V_NN & 0.99984 \nonumber\\
that_homosexuality & 0.99984 \nonumber\\
_pos_ngram_PP_V_NP & 0.99984 \nonumber\\
_pos_ngram_PP_PP_NP & 0.99984 \nonumber\\
anyone_else & 0.99984 \nonumber\\
_pos_ngram_CONJ_ADV_ADJ & 0.99984 \nonumber\\
that_personal & 0.99984 \nonumber\\
i_see & 0.99984 \nonumber\\
ProductionRule_SINV->MD,NP,VP, & 0.99984 \nonumber\\
_pos_ngram_ADV_PUNC_PP & 0.99984 \nonumber\\
culture & 0.99984 \nonumber\\
we_think & 0.99984 \nonumber\\
hand_. & 0.99984 \nonumber\\
_pos_ngram_V_PUNC_CONJ & 0.99984 \nonumber\\
pick & 0.99984 \nonumber\\
_pos_ngram_NN_CONJ_ADV & 0.99984 \nonumber\\
pursuit_, & 0.99984 \nonumber\\
in_your & 0.99984 \nonumber\\
lousy & 0.99984 \nonumber\\
to_decide & 0.99984 \nonumber\\
turn_him & 0.99984 \nonumber\\
_pos_ngram_PR_CONJ & 0.99984 \nonumber\\
_pos_ngram_ADJ_PUNC_NN & 0.99985 \nonumber\\
maintain & 0.99985 \nonumber\\
be_like & 0.99985 \nonumber\\
the_case & 0.99985 \nonumber\\
fatherless_be & 0.99985 \nonumber\\
involve_in & 0.99985 \nonumber\\
_pos_ngram_PP_NN_ADJ & 0.99985 \nonumber\\
member & 0.99985 \nonumber\\
other_in & 0.99985 \nonumber\\
your_personal & 0.99985 \nonumber\\
day_that & 0.99985 \nonumber\\
water & 0.99985 \nonumber\\
this_side & 0.99985 \nonumber\\
parent & 0.99985 \nonumber\\
the_work & 0.99985 \nonumber\\
his_superior & 0.99985 \nonumber\\
ProductionRule_NP->QP,NN, & 0.99985 \nonumber\\
and_to & 0.99985 \nonumber\\
feeling & 0.99985 \nonumber\\
fact_that & 0.99985 \nonumber\\
care & 0.99985 \nonumber\\
and_for & 0.99985 \nonumber\\
the_problem & 0.99985 \nonumber\\
parent_should & 0.99985 \nonumber\\
_pos_ngram_ADV_CONJ_V & 0.99985 \nonumber\\
ProductionRule_S->NP,ADVP,VP,., & 0.99985 \nonumber\\
generation & 0.99985 \nonumber\\
_pos_ngram_ADJ_V_ADV & 0.99985 \nonumber\\
better_for & 0.99985 \nonumber\\
_pos_ngram_NN_O_V & 0.99985 \nonumber\\
want_to & 0.99985 \nonumber\\
_pos_ngram_CONJ_V_V & 0.99985 \nonumber\\
fact & 0.99985 \nonumber\\
in_me & 0.99985 \nonumber\\
ProductionRule_NP->PRP$,NNS, & 0.99985 \nonumber\\
if_the & 0.99985 \nonumber\\
a_bid & 0.99985 \nonumber\\
ProductionRule_VP->VB,PP,SBAR, & 0.99985 \nonumber\\
_pos_ngram_ADV_NN_PR & 0.99985 \nonumber\\
how_can & 0.99985 \nonumber\\
would & 0.99985 \nonumber\\
and_you & 0.99985 \nonumber\\
_pos_ngram_CONJ_CARD & 0.99985 \nonumber\\
i_'d & 0.99985 \nonumber\\
ProductionRule_NP->JJR,NN, & 0.99985 \nonumber\\
think_i & 0.99985 \nonumber\\
._not & 0.99985 \nonumber\\
individuality & 0.99985 \nonumber\\
be_one & 0.99985 \nonumber\\
_pos_ngram_ART_ADV_ADJ & 0.99985 \nonumber\\
the_country & 0.99985 \nonumber\\
,_he & 0.99985 \nonumber\\
church & 0.99985 \nonumber\\
_pos_ngram_NP_PP_NP & 0.99985 \nonumber\\
then_we & 0.99985 \nonumber\\
discover & 0.99986 \nonumber\\
,_farquhar & 0.99986 \nonumber\\
need_to & 0.99986 \nonumber\\
your_time & 0.99986 \nonumber\\
waste_your & 0.99986 \nonumber\\
as_a & 0.99986 \nonumber\\
reach & 0.99986 \nonumber\\
human_nature & 0.99986 \nonumber\\
_pos_ngram_ADJ_PP_CONJ & 0.99986 \nonumber\\
lousy_father & 0.99986 \nonumber\\
safe & 0.99986 \nonumber\\
an_argument & 0.99986 \nonumber\\
it_come & 0.99986 \nonumber\\
n't_think & 0.99986 \nonumber\\
i_like & 0.99986 \nonumber\\
_pos_ngram_PR_PUNC_PP & 0.99986 \nonumber\\
we & 0.99986 \nonumber\\
you_realize & 0.99986 \nonumber\\
school_it & 0.99986 \nonumber\\
brisk & 0.99986 \nonumber\\
great_tv & 0.99986 \nonumber\\
day_you & 0.99986 \nonumber\\
lesbian_it & 0.99986 \nonumber\\
brisk_air & 0.99986 \nonumber\\
the_cool & 0.99986 \nonumber\\
cancer_it & 0.99986 \nonumber\\
morn_be & 0.99986 \nonumber\\
your_first & 0.99986 \nonumber\\
just_waste & 0.99986 \nonumber\\
time_read & 0.99986 \nonumber\\
cool_brisk & 0.99986 \nonumber\\
ProductionRule_VP->VBP,PRT,SBAR, & 0.99986 \nonumber\\
sun_in & 0.99986 \nonumber\\
air_on & 0.99986 \nonumber\\
realize_you & 0.99986 \nonumber\\
and_tv & 0.99986 \nonumber\\
tv_tv & 0.99986 \nonumber\\
womb_it & 0.99986 \nonumber\\
my_womb & 0.99986 \nonumber\\
air & 0.99986 \nonumber\\
diegnosedca_with & 0.99986 \nonumber\\
get_diegnosedca & 0.99986 \nonumber\\
with_cancer & 0.99986 \nonumber\\
ProductionRule_S->S,S,S,S, & 0.99986 \nonumber\\
diegnosedca & 0.99986 \nonumber\\
be_lesbian & 0.99986 \nonumber\\
the_sun & 0.99986 \nonumber\\
fatherless_would & 0.99986 \nonumber\\
_pos_ngram_ADV_PUNC_ADJ & 0.99986 \nonumber\\
_pos_ngram_V_ART_PP & 0.99986 \nonumber\\
dispute & 0.99986 \nonumber\\
out_that & 0.99986 \nonumber\\
ProductionRule_VP->VBN,VP, & 0.99986 \nonumber\\
then_why & 0.99986 \nonumber\\
father_you & 0.99986 \nonumber\\
they_should & 0.99986 \nonumber\\
like_that & 0.99986 \nonumber\\
gay_marriage & 0.99986 \nonumber\\
have_to & 0.99986 \nonumber\\
it_means & 0.99986 \nonumber\\
father_because & 0.99986 \nonumber\\
day_of & 0.99986 \nonumber\\
of & 0.99986 \nonumber\\
nature & 0.99986 \nonumber\\
rape & 0.99986 \nonumber\\
my_dad & 0.99986 \nonumber\\
in_. & 0.99986 \nonumber\\
a_personal & 0.99986 \nonumber\\
_pos_ngram_ADJ_PR_ADV & 0.99986 \nonumber\\
that_god & 0.99986 \nonumber\\
and_evolution & 0.99986 \nonumber\\
separate & 0.99986 \nonumber\\
ProductionRule_NP->PRP$,JJR, & 0.99986 \nonumber\\
if_we & 0.99986 \nonumber\\
_pos_ngram_ADV_PP_O & 0.99986 \nonumber\\
if_it & 0.99986 \nonumber\\
father_be & 0.99986 \nonumber\\
be_completely & 0.99986 \nonumber\\
ProductionRule_NP->FW,FW, & 0.99986 \nonumber\\
civil & 0.99986 \nonumber\\
._she & 0.99986 \nonumber\\
ProductionRule_VP->VBN,PP, & 0.99986 \nonumber\\
the_morn & 0.99986 \nonumber\\
ProductionRule_ADJP->ADJP,PP, & 0.99986 \nonumber\\
that_help & 0.99986 \nonumber\\
live_in & 0.99986 \nonumber\\
date & 0.99986 \nonumber\\
to_find & 0.99986 \nonumber\\
personal_experience & 0.99986 \nonumber\\
experience_, & 0.99986 \nonumber\\
people_to & 0.99986 \nonumber\\
someone_' & 0.99986 \nonumber\\
_pos_ngram_V_ADJ_ART & 0.99986 \nonumber\\
_pos_ngram_NP_PP_PR & 0.99986 \nonumber\\
me_, & 0.99986 \nonumber\\
first_day & 0.99986 \nonumber\\
not_god & 0.99986 \nonumber\\
make_sarcastic & 0.99986 \nonumber\\
sarcastic_comment & 0.99986 \nonumber\\
use_him & 0.99986 \nonumber\\
just_use & 0.99986 \nonumber\\
in_god & 0.99986 \nonumber\\
story & 0.99986 \nonumber\\
agree_with & 0.99986 \nonumber\\
see & 0.99986 \nonumber\\
as_the & 0.99986 \nonumber\\
physically & 0.99986 \nonumber\\
session & 0.99986 \nonumber\\
do_the & 0.99986 \nonumber\\
way_for & 0.99986 \nonumber\\
you_will & 0.99986 \nonumber\\
act & 0.99986 \nonumber\\
all_of & 0.99986 \nonumber\\
car & 0.99986 \nonumber\\
superior & 0.99986 \nonumber\\
_pos_ngram_CARD_V & 0.99986 \nonumber\\
and_have & 0.99986 \nonumber\\
because_of & 0.99986 \nonumber\\
._. & 0.99987 \nonumber\\
baby_in & 0.99987 \nonumber\\
be_full & 0.99987 \nonumber\\
_pos_ngram_PP_CARD & 0.99987 \nonumber\\
for_those & 0.99987 \nonumber\\
love_be & 0.99987 \nonumber\\
help_the & 0.99987 \nonumber\\
gon_na & 0.99987 \nonumber\\
gon & 0.99987 \nonumber\\
_pos_ngram_CARD_PUNC_ADV & 0.99987 \nonumber\\
_pos_ngram_ADV_ART_O & 0.99987 \nonumber\\
hour & 0.99987 \nonumber\\
_pos_ngram_ADJ_ART & 0.99987 \nonumber\\
american_endeavor & 0.99987 \nonumber\\
politician_who & 0.99987 \nonumber\\
screw_by & 0.99987 \nonumber\\
communism & 0.99987 \nonumber\\
endeavor_personal & 0.99987 \nonumber\\
fail_. & 0.99987 \nonumber\\
endeavor_advance & 0.99987 \nonumber\\
by_politician & 0.99987 \nonumber\\
communism_fail & 0.99987 \nonumber\\
good_; & 0.99987 \nonumber\\
everyone_endeavor & 0.99987 \nonumber\\
pursuit_than & 0.99987 \nonumber\\
why_communism & 0.99987 \nonumber\\
get_most & 0.99987 \nonumber\\
would_keep & 0.99987 \nonumber\\
by_someone & 0.99987 \nonumber\\
in_check & 0.99987 \nonumber\\
to_endeavor & 0.99987 \nonumber\\
who_endeavor & 0.99987 \nonumber\\
get_screw & 0.99987 \nonumber\\
;_which & 0.99987 \nonumber\\
keep_each & 0.99987 \nonumber\\
check_. & 0.99987 \nonumber\\
go_to & 0.99987 \nonumber\\
everywhere & 0.99987 \nonumber\\
abusive & 0.99987 \nonumber\\
every_time & 0.99987 \nonumber\\
look_like & 0.99987 \nonumber\\
then_i & 0.99987 \nonumber\\
ProductionRule_VP->VB,NP,ADVP,S, & 0.99987 \nonumber\\
him_, & 0.99987 \nonumber\\
it_also & 0.99987 \nonumber\\
ProductionRule_S->S,VP, & 0.99987 \nonumber\\
at_all & 0.99987 \nonumber\\
_pos_ngram_PP_ADV_PP & 0.99987 \nonumber\\
n't_even & 0.99987 \nonumber\\
to_stay & 0.99987 \nonumber\\
_pos_ngram_ADJ_CONJ_ART & 0.99987 \nonumber\\
better_endeavor & 0.99987 \nonumber\\
._when & 0.99987 \nonumber\\
_pos_ngram_PUNC_CONJ_O & 0.99987 \nonumber\\
clean & 0.99987 \nonumber\\
most_american & 0.99987 \nonumber\\
word_, & 0.99987 \nonumber\\
do_you & 0.99987 \nonumber\\
FutureVerbRatio & 0.99987 \nonumber\\
television_be & 0.99987 \nonumber\\
they_make & 0.99987 \nonumber\\
desire & 0.99987 \nonumber\\
be_of & 0.99987 \nonumber\\
although & 0.99987 \nonumber\\
normal & 0.99987 \nonumber\\
belief & 0.99987 \nonumber\\
a_load & 0.99987 \nonumber\\
sport & 0.99987 \nonumber\\
your_lousy & 0.99987 \nonumber\\
_pos_ngram_O_NN_ADV & 0.99987 \nonumber\\
god_. & 0.99987 \nonumber\\
end_up & 0.99987 \nonumber\\
what_' & 0.99987 \nonumber\\
_pos_ngram_CONJ_ADV_PUNC & 0.99987 \nonumber\\
pe & 0.99987 \nonumber\\
future & 0.99987 \nonumber\\
ridiculous & 0.99987 \nonumber\\
to_fall & 0.99987 \nonumber\\
_pos_ngram_PR_ADV_ADV & 0.99987 \nonumber\\
just_one & 0.99987 \nonumber\\
_pos_ngram_ART_NP_CONJ & 0.99987 \nonumber\\
ProductionRule_PP->JJ,IN,NP, & 0.99987 \nonumber\\
._most & 0.99987 \nonumber\\
_pos_ngram_ADJ_ART_NN & 0.99987 \nonumber\\
fall & 0.99987 \nonumber\\
christian & 0.99987 \nonumber\\
ProductionRule_NP->NP,ADVP, & 0.99987 \nonumber\\
_pos_ngram_ADV_PR_NN & 0.99987 \nonumber\\
for_some & 0.99987 \nonumber\\
_pos_ngram_V_ADJ_V & 0.99987 \nonumber\\
go & 0.99987 \nonumber\\
_pos_ngram_V_CARD_NN & 0.99987 \nonumber\\
ProductionRule_SBAR->IN,IN,S, & 0.99987 \nonumber\\
make_a & 0.99987 \nonumber\\
express & 0.99988 \nonumber\\
religious_institution & 0.99988 \nonumber\\
television & 0.99988 \nonumber\\
you_want & 0.99988 \nonumber\\
give_the & 0.99988 \nonumber\\
what_go & 0.99988 \nonumber\\
singapore_to & 0.99988 \nonumber\\
evidence & 0.99988 \nonumber\\
_pos_ngram_PUNC_ART_ADV & 0.99988 \nonumber\\
not_think & 0.99988 \nonumber\\
_pos_ngram_PUNC_ADJ_NP & 0.99988 \nonumber\\
take_a & 0.99988 \nonumber\\
_pos_ngram_O_NN_NN & 0.99988 \nonumber\\
easier_to & 0.99988 \nonumber\\
likely_to & 0.99988 \nonumber\\
you_tell & 0.99988 \nonumber\\
just_to & 0.99988 \nonumber\\
ProductionRule_VP->VB,NP,ADVP, & 0.99988 \nonumber\\
because_its & 0.99988 \nonumber\\
realize_that & 0.99988 \nonumber\\
ProductionRule_VP->VBN,ADVP, & 0.99988 \nonumber\\
_pos_ngram_PP_CARD_NN & 0.99988 \nonumber\\
of_people & 0.99988 \nonumber\\
for_at & 0.99988 \nonumber\\
_pos_ngram_O_ADJ & 0.99988 \nonumber\\
than_none & 0.99988 \nonumber\\
none_. & 0.99988 \nonumber\\
check & 0.99988 \nonumber\\
means_you & 0.99988 \nonumber\\
we_use & 0.99988 \nonumber\\
than_it & 0.99988 \nonumber\\
of_crap & 0.99988 \nonumber\\
be_actually & 0.99988 \nonumber\\
ProductionRule_NP->DT,JJR,NN, & 0.99988 \nonumber\\
_pos_ngram_ADV_V & 0.99988 \nonumber\\
to_your & 0.99988 \nonumber\\
low & 0.99988 \nonumber\\
_pos_ngram_ADJ_V_V & 0.99988 \nonumber\\
job_. & 0.99988 \nonumber\\
institution & 0.99988 \nonumber\\
lead_the & 0.99988 \nonumber\\
3_. & 0.99988 \nonumber\\
be_when & 0.99988 \nonumber\\
_pos_ngram_PR_NP & 0.99988 \nonumber\\
who_he & 0.99988 \nonumber\\
two & 0.99988 \nonumber\\
attend & 0.99988 \nonumber\\
from_what & 0.99988 \nonumber\\
require & 0.99988 \nonumber\\
water_. & 0.99988 \nonumber\\
,_a & 0.99988 \nonumber\\
fail & 0.99988 \nonumber\\
with_a & 0.99988 \nonumber\\
the_idea & 0.99988 \nonumber\\
_pos_ngram_PUNC_O_PR & 0.99988 \nonumber\\
good_idea & 0.99988 \nonumber\\
if_everyone & 0.99988 \nonumber\\
ProductionRule_PP->IN,PP, & 0.99988 \nonumber\\
corruption & 0.99988 \nonumber\\
indium_do & 0.99988 \nonumber\\
lowest & 0.99988 \nonumber\\
have_chat & 0.99988 \nonumber\\
i_dispute & 0.99988 \nonumber\\
lowest_common & 0.99988 \nonumber\\
attune_to & 0.99988 \nonumber\\
ProductionRule_NP->DT,JJS,JJ,NN, & 0.99988 \nonumber\\
denominator & 0.99988 \nonumber\\
indisputable_" & 0.99988 \nonumber\\
forum & 0.99988 \nonumber\\
yahoo_! & 0.99988 \nonumber\\
yahoo & 0.99988 \nonumber\\
forum_, & 0.99988 \nonumber\\
!_have & 0.99988 \nonumber\\
this_forum & 0.99988 \nonumber\\
degrade_this & 0.99988 \nonumber\\
style_of & 0.99988 \nonumber\\
means_what & 0.99988 \nonumber\\
it_disputable & 0.99988 \nonumber\\
"_indisputable & 0.99988 \nonumber\\
this_word & 0.99988 \nonumber\\
attune & 0.99988 \nonumber\\
chat & 0.99988 \nonumber\\
fall_to & 0.99988 \nonumber\\
argument_degrade & 0.99988 \nonumber\\
your_style & 0.99988 \nonumber\\
common_denominator & 0.99988 \nonumber\\
disputable & 0.99988 \nonumber\\
dispute_your & 0.99988 \nonumber\\
chat_room & 0.99988 \nonumber\\
that_form & 0.99988 \nonumber\\
check_them & 0.99988 \nonumber\\
disputable_. & 0.99988 \nonumber\\
think_yahoo & 0.99988 \nonumber\\
claim_from & 0.99988 \nonumber\\
the_lowest & 0.99988 \nonumber\\
._check & 0.99988 \nonumber\\
room_more & 0.99988 \nonumber\\
more_attune & 0.99988 \nonumber\\
denominator_. & 0.99988 \nonumber\\
development & 0.99988 \nonumber\\
include & 0.99988 \nonumber\\
idiotic & 0.99988 \nonumber\\
that_raffle & 0.99988 \nonumber\\
me_. & 0.99988 \nonumber\\
that_, & 0.99988 \nonumber\\
v. & 0.99988 \nonumber\\
entertainment & 0.99988 \nonumber\\
suppose_to & 0.99988 \nonumber\\
suppose & 0.99988 \nonumber\\
not_there & 0.99988 \nonumber\\
view_. & 0.99988 \nonumber\\
from_personal & 0.99988 \nonumber\\
the_human & 0.99988 \nonumber\\
crap_. & 0.99988 \nonumber\\
_pos_ngram_CARD_NN_V & 0.99989 \nonumber\\
william_have & 0.99989 \nonumber\\
_pos_ngram_ADJ_CONJ_NN & 0.99989 \nonumber\\
and_child & 0.99989 \nonumber\\
_pos_ngram_CARD_PR_V & 0.99989 \nonumber\\
_pos_ngram_CARD_PR & 0.99989 \nonumber\\
_pos_ngram_PP_PUNC_ADV & 0.99989 \nonumber\\
you_may & 0.99989 \nonumber\\
nature_be & 0.99989 \nonumber\\
that_will & 0.99989 \nonumber\\
word & 0.99989 \nonumber\\
be_less & 0.99989 \nonumber\\
ProductionRule_VP->VB,NP,PP,SBAR, & 0.99989 \nonumber\\
opponent & 0.99989 \nonumber\\
the_first & 0.99989 \nonumber\\
school_uniform & 0.99989 \nonumber\\
forever_. & 0.99989 \nonumber\\
death & 0.99989 \nonumber\\
_pos_ngram_PR_ART_ADJ & 0.99989 \nonumber\\
ProductionRule_S->NP,ADVP, & 0.99989 \nonumber\\
be_selfish & 0.99989 \nonumber\\
be_do & 0.99989 \nonumber\\
olden & 0.99989 \nonumber\\
such_a & 0.99989 \nonumber\\
_pos_ngram_PUNC_NN_ART & 0.99989 \nonumber\\
point_of & 0.99989 \nonumber\\
ProductionRule_ADVP->ADVP,PP, & 0.99989 \nonumber\\
it_make & 0.99989 \nonumber\\
n't_mean & 0.99989 \nonumber\\
gender & 0.99989 \nonumber\\
._one & 0.99989 \nonumber\\
,_who & 0.99989 \nonumber\\
sex & 0.99989 \nonumber\\
_pos_ngram_NN_CONJ_PP & 0.99989 \nonumber\\
one_thing & 0.99989 \nonumber\\
ProductionRule_S->PP,,,NP,VP,., & 0.99989 \nonumber\\
_pos_ngram_CONJ_ADJ_PP & 0.99989 \nonumber\\
person_and & 0.99989 \nonumber\\
would_probably & 0.99989 \nonumber\\
william & 0.99989 \nonumber\\
a_question & 0.99989 \nonumber\\
thing_to & 0.99989 \nonumber\\
,_corruption & 0.99989 \nonumber\\
_pos_ngram_O_PUNC_V & 0.99989 \nonumber\\
_pos_ngram_CONJ_CARD_PUNC & 0.99989 \nonumber\\
lot_of & 0.99989 \nonumber\\
_pos_ngram_NN_CONJ_CARD & 0.99989 \nonumber\\
his_life & 0.99989 \nonumber\\
rights_than & 0.99989 \nonumber\\
superior_and & 0.99989 \nonumber\\
_pos_ngram_V_ADV_O & 0.99989 \nonumber\\
_pos_ngram_V_PUNC_NN & 0.99989 \nonumber\\
it_would & 0.99989 \nonumber\\
_pos_ngram_ADV_V_ADJ & 0.99989 \nonumber\\
be_pro & 0.99989 \nonumber\\
farquhar & 0.99989 \nonumber\\
cool_and & 0.99989 \nonumber\\
_pos_ngram_O_PP_NN & 0.99989 \nonumber\\
_pos_ngram_CONJ_NN_O & 0.99989 \nonumber\\
n't_. & 0.99989 \nonumber\\
the_second & 0.99989 \nonumber\\
you_assume & 0.99989 \nonumber\\
and_will & 0.99989 \nonumber\\
try & 0.99989 \nonumber\\
be_suppose & 0.99989 \nonumber\\
intelligent & 0.99989 \nonumber\\
limit & 0.99989 \nonumber\\
program & 0.99989 \nonumber\\
much_more & 0.99989 \nonumber\\
_pos_ngram_ADV_PP_ADJ & 0.99989 \nonumber\\
if_she & 0.99989 \nonumber\\
look_at & 0.99989 \nonumber\\
be_really & 0.99989 \nonumber\\
they_want & 0.99989 \nonumber\\
different & 0.99989 \nonumber\\
think_of & 0.99989 \nonumber\\
ProductionRule_VP->VBP,PP, & 0.99989 \nonumber\\
have_some & 0.99989 \nonumber\\
ProductionRule_SBAR->SBAR,,,SBAR, & 0.99989 \nonumber\\
endeavor & 0.99989 \nonumber\\
true & 0.99989 \nonumber\\
_pos_ngram_ADJ_V_PUNC & 0.99989 \nonumber\\
_pos_ngram_ADJ_PP_NP & 0.99989 \nonumber\\
exact & 0.99989 \nonumber\\
society & 0.99989 \nonumber\\
be_try & 0.99989 \nonumber\\
who_want & 0.99989 \nonumber\\
_pos_ngram_ART_CARD_V & 0.99989 \nonumber\\
side_. & 0.99989 \nonumber\\
be_live & 0.99989 \nonumber\\
ProductionRule_ADVP->RB,RB, & 0.99989 \nonumber\\
who_do & 0.99989 \nonumber\\
book_take & 0.99989 \nonumber\\
can_get & 0.99989 \nonumber\\
life_, & 0.99989 \nonumber\\
a_big & 0.99989 \nonumber\\
again & 0.99989 \nonumber\\
faith & 0.99989 \nonumber\\
call & 0.99990 \nonumber\\
few & 0.99990 \nonumber\\
easy_to & 0.99990 \nonumber\\
ProductionRule_VP->VB,NP,NP, & 0.99990 \nonumber\\
get_marry & 0.99990 \nonumber\\
and_would & 0.99990 \nonumber\\
do_have & 0.99990 \nonumber\\
what_. & 0.99990 \nonumber\\
back_up & 0.99990 \nonumber\\
create & 0.99990 \nonumber\\
one_be & 0.99990 \nonumber\\
period_of & 0.99990 \nonumber\\
be_look & 0.99990 \nonumber\\
people_. & 0.99990 \nonumber\\
her_body & 0.99990 \nonumber\\
you_see & 0.99990 \nonumber\\
; & 0.99990 \nonumber\\
n't_know & 0.99990 \nonumber\\
to_. & 0.99990 \nonumber\\
you_. & 0.99990 \nonumber\\
soon & 0.99990 \nonumber\\
for_separate & 0.99990 \nonumber\\
with_civil & 0.99990 \nonumber\\
ProductionRule_NP->ADJP,NN,NN, & 0.99990 \nonumber\\
student_from & 0.99990 \nonumber\\
idea_for & 0.99990 \nonumber\\
for_harmonious & 0.99990 \nonumber\\
civil_. & 0.99990 \nonumber\\
garment_job & 0.99990 \nonumber\\
ProductionRule_ADJP->JJS,NN, & 0.99990 \nonumber\\
uniform_? & 0.99990 \nonumber\\
?_for & 0.99990 \nonumber\\
civil_and & 0.99990 \nonumber\\
garment & 0.99990 \nonumber\\
separate_student & 0.99990 \nonumber\\
increase_garment & 0.99990 \nonumber\\
from_civil & 0.99990 \nonumber\\
terrorist_not & 0.99990 \nonumber\\
attack_enemy & 0.99990 \nonumber\\
least_increase & 0.99990 \nonumber\\
ProductionRule_NP->NP,PP,PP,., & 0.99990 \nonumber\\
harmonious_with & 0.99990 \nonumber\\
from_other & 0.99990 \nonumber\\
use_soldier & 0.99990 \nonumber\\
soldier_uniform & 0.99990 \nonumber\\
harmonious & 0.99990 \nonumber\\
enemy & 0.99990 \nonumber\\
why_terrorist & 0.99990 \nonumber\\
enemy_. & 0.99990 \nonumber\\
ProductionRule_VP->VBP,ADVP,VP, & 0.99990 \nonumber\\
ProductionRule_S->S,,,CC,S, & 0.99990 \nonumber\\
find_a & 0.99990 \nonumber\\
ProductionRule_VP->VBD,PP,S, & 0.99990 \nonumber\\
bully & 0.99990 \nonumber\\
say_again & 0.99990 \nonumber\\
i_need & 0.99990 \nonumber\\
the_only & 0.99990 \nonumber\\
base & 0.99990 \nonumber\\
why_they & 0.99990 \nonumber\\
course_assume & 0.99990 \nonumber\\
way_) & 0.99990 \nonumber\\
show_have & 0.99990 \nonumber\\
family_therapy & 0.99990 \nonumber\\
abusive_in & 0.99990 \nonumber\\
therapy & 0.99990 \nonumber\\
ProductionRule_NP->NP,CC,RB, & 0.99990 \nonumber\\
physically_and & 0.99990 \nonumber\\
therapy_session & 0.99990 \nonumber\\
)_also & 0.99990 \nonumber\\
attend_to & 0.99990 \nonumber\\
to_progress & 0.99990 \nonumber\\
the_healthiest & 0.99990 \nonumber\\
healthiest & 0.99990 \nonumber\\
mentally_. & 0.99990 \nonumber\\
and_mentally & 0.99990 \nonumber\\
healthiest_way & 0.99990 \nonumber\\
that_show & 0.99990 \nonumber\\
session_you & 0.99990 \nonumber\\
lousy_forever & 0.99990 \nonumber\\
not_abusive & 0.99990 \nonumber\\
progress_physically & 0.99990 \nonumber\\
can_attend & 0.99990 \nonumber\\
be_family & 0.99990 \nonumber\\
people_change & 0.99990 \nonumber\\
(_that & 0.99990 \nonumber\\
be_scientific & 0.99990 \nonumber\\
_pos_ngram_ADV_NN_PUNC & 0.99990 \nonumber\\
than_be & 0.99990 \nonumber\\
be_happy & 0.99990 \nonumber\\
,_which & 0.99990 \nonumber\\
of_what & 0.99990 \nonumber\\
better_yourself & 0.99990 \nonumber\\
_pos_ngram_NP_ADV_PUNC & 0.99990 \nonumber\\
._your & 0.99990 \nonumber\\
than_no & 0.99990 \nonumber\\
corruption_, & 0.99990 \nonumber\\
the_opposite & 0.99990 \nonumber\\
child_can & 0.99990 \nonumber\\
n't_want & 0.99990 \nonumber\\
raffle & 0.99990 \nonumber\\
womb & 0.99990 \nonumber\\
_pos_ngram_NP_O_PUNC & 0.99990 \nonumber\\
ProductionRule_VP->VP,,,CC,VP, & 0.99990 \nonumber\\
bottle & 0.99990 \nonumber\\
they_might & 0.99990 \nonumber\\
example_of & 0.99990 \nonumber\\
that_they & 0.99990 \nonumber\\
tab & 0.99990 \nonumber\\
marry & 0.99990 \nonumber\\
further & 0.99990 \nonumber\\
them_and & 0.99990 \nonumber\\
know_. & 0.99990 \nonumber\\
argue_with & 0.99990 \nonumber\\
_pos_ngram_NN_PR_ADJ & 0.99990 \nonumber\\
read_this & 0.99990 \nonumber\\
save & 0.99990 \nonumber\\
evidence_that & 0.99990 \nonumber\\
_pos_ngram_ART_ADJ_PP & 0.99990 \nonumber\\
,_most & 0.99990 \nonumber\\
_pos_ngram_ART_ADJ_CARD & 0.99990 \nonumber\\
better_in & 0.99990 \nonumber\\
have_someone & 0.99990 \nonumber\\
ie & 0.99990 \nonumber\\
too_much & 0.99990 \nonumber\\
,_even & 0.99990 \nonumber\\
a_law & 0.99990 \nonumber\\
_pos_ngram_ADV_O_V & 0.99990 \nonumber\\
_pos_ngram_PUNC_NP_PUNC & 0.99990 \nonumber\\
kid_will & 0.99990 \nonumber\\
good_father & 0.99990 \nonumber\\
bully_because & 0.99990 \nonumber\\
be_bully & 0.99990 \nonumber\\
screw & 0.99990 \nonumber\\
_pos_ngram_V_CONJ_NN & 0.99990 \nonumber\\
we_do & 0.99990 \nonumber\\
singapore_as & 0.99990 \nonumber\\
._for & 0.99990 \nonumber\\
i_never & 0.99990 \nonumber\\
he_' & 0.99990 \nonumber\\
_pos_ngram_PP_O_PR & 0.99990 \nonumber\\
year_, & 0.99990 \nonumber\\
further_, & 0.99990 \nonumber\\
ProductionRule_S->S,VP,., & 0.99990 \nonumber\\
the_argument & 0.99990 \nonumber\\
sister & 0.99990 \nonumber\\
the_earth & 0.99990 \nonumber\\
be_, & 0.99990 \nonumber\\
can_be & 0.99990 \nonumber\\
ProductionRule_NP->DT,NNP,NNP,NNP, & 0.99990 \nonumber\\
be_use & 0.99990 \nonumber\\
job & 0.99990 \nonumber\\
self_defense & 0.99990 \nonumber\\
disaster & 0.99990 \nonumber\\
_pos_ngram_V_ADJ_NP & 0.99990 \nonumber\\
million & 0.99990 \nonumber\\
ProductionRule_S->PP,,,NP,VP, & 0.99990 \nonumber\\
singapore_be & 0.99990 \nonumber\\
?_what & 0.99990 \nonumber\\
_pos_ngram_NP_ADV_V & 0.99990 \nonumber\\
victim & 0.99990 \nonumber\\
prefer & 0.99990 \nonumber\\
ProductionRule_SBAR->ADVP,IN,S, & 0.99990 \nonumber\\
would_rather & 0.99990 \nonumber\\
her_in & 0.99990 \nonumber\\
turn_her & 0.99990 \nonumber\\
on_that & 0.99991 \nonumber\\
come_in & 0.99991 \nonumber\\
she_do & 0.99991 \nonumber\\
yes_, & 0.99991 \nonumber\\
_pos_ngram_PUNC_PP_O & 0.99991 \nonumber\\
_pos_ngram_V_V_CARD & 0.99991 \nonumber\\
ProductionRule_NP->CD,NN, & 0.99991 \nonumber\\
because_he & 0.99991 \nonumber\\
up_for & 0.99991 \nonumber\\
decide_to & 0.99991 \nonumber\\
_pos_ngram_ART_PUNC_ADV & 0.99991 \nonumber\\
of_how & 0.99991 \nonumber\\
beside_, & 0.99991 \nonumber\\
_pos_ngram_ADV_NP_ADV & 0.99991 \nonumber\\
and_easy & 0.99991 \nonumber\\
expect_it & 0.99991 \nonumber\\
should_n't & 0.99991 \nonumber\\
idiot & 0.99991 \nonumber\\
'd & 0.99991 \nonumber\\
_pos_ngram_V_O_V & 0.99991 \nonumber\\
"_choice & 0.99991 \nonumber\\
"_when & 0.99991 \nonumber\\
call_someone & 0.99991 \nonumber\\
not_choose & 0.99991 \nonumber\\
'_lifestyle & 0.99991 \nonumber\\
_pos_ngram_NN_ART_O & 0.99991 \nonumber\\
not_call & 0.99991 \nonumber\\
lifestyle_a & 0.99991 \nonumber\\
lifestyle_because & 0.99991 \nonumber\\
n't_agree & 0.99991 \nonumber\\
choose_someone & 0.99991 \nonumber\\
choice_" & 0.99991 \nonumber\\
mother_and & 0.99991 \nonumber\\
least_you & 0.99991 \nonumber\\
ProductionRule_ADJP->RB,JJR, & 0.99991 \nonumber\\
which_i & 0.99991 \nonumber\\
among & 0.99991 \nonumber\\
to_spend & 0.99991 \nonumber\\
_pos_ngram_PUNC_NP_O & 0.99991 \nonumber\\
mentally & 0.99991 \nonumber\\
ProductionRule_NP->DT,NN,NNS, & 0.99991 \nonumber\\
thing_happen & 0.99991 \nonumber\\
a_story & 0.99991 \nonumber\\
them_out & 0.99991 \nonumber\\
_pos_ngram_PR_PP_ART & 0.99991 \nonumber\\
_pos_ngram_PUNC_ADV_NN & 0.99991 \nonumber\\
give_you & 0.99991 \nonumber\\
_pos_ngram_ADV_NP_PUNC & 0.99991 \nonumber\\
help_yourself & 0.99991 \nonumber\\
_pos_ngram_V_CARD_PUNC & 0.99991 \nonumber\\
porn & 0.99991 \nonumber\\
ProductionRule_S->SBAR,,,NP,VP, & 0.99991 \nonumber\\
access_to & 0.99991 \nonumber\\
access & 0.99991 \nonumber\\
people_for & 0.99991 \nonumber\\
selfish_but & 0.99991 \nonumber\\
never_know & 0.99991 \nonumber\\
be_make & 0.99991 \nonumber\\
be_on & 0.99991 \nonumber\\
desire_to & 0.99991 \nonumber\\
use_constantly & 0.99991 \nonumber\\
_pos_ngram_O_PUNC_NP & 0.99991 \nonumber\\
fatherless_then & 0.99991 \nonumber\\
if_your & 0.99991 \nonumber\\
(_for & 0.99991 \nonumber\\
you_mean & 0.99991 \nonumber\\
specify & 0.99991 \nonumber\\
address & 0.99991 \nonumber\\
unfortunately_, & 0.99991 \nonumber\\
affect & 0.99991 \nonumber\\
ProductionRule_NP->JJ,JJ,NN, & 0.99991 \nonumber\\
kind_of & 0.99991 \nonumber\\
instance & 0.99991 \nonumber\\
_pos_ngram_PUNC_O_ART & 0.99991 \nonumber\\
a_red & 0.99991 \nonumber\\
red & 0.99991 \nonumber\\
will_find & 0.99991 \nonumber\\
anything_from & 0.99991 \nonumber\\
you_know & 0.99991 \nonumber\\
_pos_ngram_CONJ_NN_NN & 0.99991 \nonumber\\
issue_should & 0.99991 \nonumber\\
politician_and & 0.99991 \nonumber\\
and_lawmaker & 0.99991 \nonumber\\
n't_break & 0.99991 \nonumber\\
and_state & 0.99991 \nonumber\\
pass_a & 0.99991 \nonumber\\
maybe_, & 0.99991 \nonumber\\
to_pass & 0.99991 \nonumber\\
break_the & 0.99991 \nonumber\\
separation & 0.99991 \nonumber\\
to_allow & 0.99991 \nonumber\\
separation_between & 0.99991 \nonumber\\
legislation & 0.99991 \nonumber\\
state_rule & 0.99991 \nonumber\\
decide_, & 0.99991 \nonumber\\
no_power & 0.99991 \nonumber\\
force_religious & 0.99991 \nonumber\\
congress & 0.99991 \nonumber\\
congress_have & 0.99991 \nonumber\\
institution_about & 0.99991 \nonumber\\
marriage_issue & 0.99991 \nonumber\\
lawmaker_. & 0.99991 \nonumber\\
church_to & 0.99991 \nonumber\\
a_legislation & 0.99991 \nonumber\\
lawmaker & 0.99991 \nonumber\\
of_politician & 0.99991 \nonumber\\
allow_gay & 0.99991 \nonumber\\
,_congress & 0.99991 \nonumber\\
court_. & 0.99991 \nonumber\\
court_be & 0.99991 \nonumber\\
about_marriage & 0.99991 \nonumber\\
the_separation & 0.99991 \nonumber\\
the_court & 0.99991 \nonumber\\
between_church & 0.99991 \nonumber\\
alright_since & 0.99991 \nonumber\\
legislation_force & 0.99991 \nonumber\\
though_william & 0.99991 \nonumber\\
and_act & 0.99991 \nonumber\\
to_know & 0.99991 \nonumber\\
_pos_ngram_PP_ART_PR & 0.99991 \nonumber\\
_pos_ngram_PUNC_NN_ADV & 0.99991 \nonumber\\
we_will & 0.99991 \nonumber\\
know_it & 0.99991 \nonumber\\
help_. & 0.99991 \nonumber\\
some & 0.99991 \nonumber\\
defense & 0.99991 \nonumber\\
leader & 0.99991 \nonumber\\
other_out & 0.99991 \nonumber\\
ProductionRule_S->S,:,S,., & 0.99991 \nonumber\\
same_thing & 0.99991 \nonumber\\
say_be & 0.99991 \nonumber\\
company & 0.99991 \nonumber\\
sex_be & 0.99991 \nonumber\\
_pos_ngram_CONJ_NP_V & 0.99991 \nonumber\\
after & 0.99991 \nonumber\\
their_individuality & 0.99991 \nonumber\\
personally_, & 0.99991 \nonumber\\
sabrejimmy_say & 0.99991 \nonumber\\
but_this & 0.99991 \nonumber\\
he_continue & 0.99991 \nonumber\\
make_these & 0.99991 \nonumber\\
some_idiot & 0.99991 \nonumber\\
post_. & 0.99991 \nonumber\\
to_ignore & 0.99991 \nonumber\\
ask_ridiculous & 0.99991 \nonumber\\
pointless & 0.99991 \nonumber\\
intelligent_debate & 0.99991 \nonumber\\
pointless_. & 0.99991 \nonumber\\
satisfy_, & 0.99991 \nonumber\\
these_kind & 0.99991 \nonumber\\
ProductionRule_SINV->VBZ,NP, & 0.99991 \nonumber\\
n't_attempt & 0.99991 \nonumber\\
future_post & 0.99991 \nonumber\\
._intelligent & 0.99991 \nonumber\\
idiot_creationist & 0.99991 \nonumber\\
ridiculous_question & 0.99991 \nonumber\\
his_future & 0.99991 \nonumber\\
debate_pointless & 0.99991 \nonumber\\
._personally & 0.99991 \nonumber\\
about_science & 0.99991 \nonumber\\
ProductionRule_NP->WDT,NN, & 0.99991 \nonumber\\
sabrejimmy_have & 0.99991 \nonumber\\
ignore_his & 0.99991 \nonumber\\
creationist_, & 0.99991 \nonumber\\
what_sabrejimmy & 0.99991 \nonumber\\
._sabrejimmy & 0.99991 \nonumber\\
be_satisfy & 0.99991 \nonumber\\
or_a & 0.99991 \nonumber\\
have_alway & 0.99991 \nonumber\\
emergency & 0.99991 \nonumber\\
other_you & 0.99991 \nonumber\\
yet & 0.99991 \nonumber\\
._first & 0.99991 \nonumber\\
/ & 0.99991 \nonumber\\
plastic & 0.99991 \nonumber\\
public & 0.99991 \nonumber\\
mistake_. & 0.99991 \nonumber\\
anything_about & 0.99991 \nonumber\\
pretty & 0.99991 \nonumber\\
mistake_but & 0.99991 \nonumber\\
can_do & 0.99991 \nonumber\\
ProductionRule_VP->VB,NP,,,PP, & 0.99991 \nonumber\\
the_british & 0.99991 \nonumber\\
no_father & 0.99991 \nonumber\\
_pos_ngram_ADJ_PUNC_V & 0.99991 \nonumber\\
claim_that & 0.99991 \nonumber\\
clothe & 0.99991 \nonumber\\
most_people & 0.99991 \nonumber\\
remove & 0.99991 \nonumber\\
the_amount & 0.99991 \nonumber\\
that_school & 0.99991 \nonumber\\
to_avoid & 0.99991 \nonumber\\
amount_of & 0.99991 \nonumber\\
evolution_, & 0.99991 \nonumber\\
ProductionRule_NP->VBG,NNS, & 0.99991 \nonumber\\
_pos_ngram_ADJ_PUNC_PP & 0.99991 \nonumber\\
_pos_ngram_V_PUNC_V & 0.99991 \nonumber\\
here_be & 0.99991 \nonumber\\
_pos_ngram_ART_NN_NP & 0.99991 \nonumber\\
you_go & 0.99991 \nonumber\\
_pos_ngram_NP_V_ADJ & 0.99991 \nonumber\\
_pos_ngram_PP_CONJ_V & 0.99991 \nonumber\\
but_there & 0.99991 \nonumber\\
_pos_ngram_ADJ_PUNC_ART & 0.99991 \nonumber\\
_pos_ngram_ADV_O_O & 0.99991 \nonumber\\
be_already & 0.99991 \nonumber\\
all_over & 0.99991 \nonumber\\
%_of & 0.99991 \nonumber\\
the_plan & 0.99991 \nonumber\\
make_other & 0.99991 \nonumber\\
help_someone & 0.99991 \nonumber\\
_pos_ngram_NP_ART & 0.99991 \nonumber\\
_pos_ngram_NN_PP_O & 0.99991 \nonumber\\
that_indium & 0.99991 \nonumber\\
billion & 0.99991 \nonumber\\
_pos_ngram_ADV_CONJ_ART & 0.99991 \nonumber\\
ok_, & 0.99991 \nonumber\\
_pos_ngram_CONJ_PP_ART & 0.99991 \nonumber\\
species_. & 0.99991 \nonumber\\
amount & 0.99991 \nonumber\\
time_be & 0.99991 \nonumber\\
but_my & 0.99991 \nonumber\\
learn_anything & 0.99991 \nonumber\\
various & 0.99991 \nonumber\\
ProductionRule_VP->MD,ADVP,VP, & 0.99991 \nonumber\\
success_and & 0.99991 \nonumber\\
of_time & 0.99991 \nonumber\\
this_: & 0.99991 \nonumber\\
student_be & 0.99991 \nonumber\\
to_support & 0.99991 \nonumber\\
might_grow & 0.99991 \nonumber\\
them_so & 0.99991 \nonumber\\
_pos_ngram_NP_CARD & 0.99991 \nonumber\\
word_. & 0.99991 \nonumber\\
would_just & 0.99992 \nonumber\\
for_it & 0.99992 \nonumber\\
animal & 0.99992 \nonumber\\
think_you & 0.99992 \nonumber\\
_pos_ngram_PP_PUNC_ADJ & 0.99992 \nonumber\\
decide_what & 0.99992 \nonumber\\
assume & 0.99992 \nonumber\\
hold & 0.99992 \nonumber\\
say_they & 0.99992 \nonumber\\
unfortunately & 0.99992 \nonumber\\
._what & 0.99992 \nonumber\\
update & 0.99992 \nonumber\\
commitment_to & 0.99992 \nonumber\\
any_mistake & 0.99992 \nonumber\\
whit & 0.99992 \nonumber\\
greater_then & 0.99992 \nonumber\\
but_love & 0.99992 \nonumber\\
a_commitment & 0.99992 \nonumber\\
ProductionRule_ADJP->ADJP,ADVP, & 0.99992 \nonumber\\
whit_her & 0.99992 \nonumber\\
unforgivable & 0.99992 \nonumber\\
a_unforgivable & 0.99992 \nonumber\\
unforgivable_mistake & 0.99992 \nonumber\\
me_no & 0.99992 \nonumber\\
to_confide & 0.99992 \nonumber\\
much_greater & 0.99992 \nonumber\\
through_rough & 0.99992 \nonumber\\
wife_will & 0.99992 \nonumber\\
her_through & 0.99992 \nonumber\\
rough & 0.99992 \nonumber\\
go_wrong & 0.99992 \nonumber\\
know_thing & 0.99992 \nonumber\\
stay_whit & 0.99992 \nonumber\\
happen_but & 0.99992 \nonumber\\
rough_time & 0.99992 \nonumber\\
of_gay & 0.99992 \nonumber\\
british & 0.99992 \nonumber\\
_pos_ngram_PR_V_CARD & 0.99992 \nonumber\\
._that & 0.99992 \nonumber\\
rather & 0.99992 \nonumber\\
month & 0.99992 \nonumber\\
me_and & 0.99992 \nonumber\\
they_love & 0.99992 \nonumber\\
on_what & 0.99992 \nonumber\\
i_consider & 0.99992 \nonumber\\
why_would & 0.99992 \nonumber\\
_pos_ngram_O_CONJ & 0.99992 \nonumber\\
though & 0.99992 \nonumber\\
show_that & 0.99992 \nonumber\\
ProductionRule_NP->NP,,,VP, & 0.99992 \nonumber\\
healthy & 0.99992 \nonumber\\
ProductionRule_VP->VBD,NP,NP, & 0.99992 \nonumber\\
._plus & 0.99992 \nonumber\\
what_make & 0.99992 \nonumber\\
ProductionRule_VP->ADVP,VBN, & 0.99992 \nonumber\\
to_death & 0.99992 \nonumber\\
_pos_ngram_PR_CONJ_PR & 0.99992 \nonumber\\
,_all & 0.99992 \nonumber\\
you_dont & 0.99992 \nonumber\\
me_that & 0.99992 \nonumber\\
of_self & 0.99992 \nonumber\\
someone_be & 0.99992 \nonumber\\
be_alright & 0.99992 \nonumber\\
since_it & 0.99992 \nonumber\\
to_use & 0.99992 \nonumber\\
_pos_ngram_ART_O_V & 0.99992 \nonumber\\
then_any & 0.99992 \nonumber\\
back & 0.99992 \nonumber\\
do_a & 0.99992 \nonumber\\
you_find & 0.99992 \nonumber\\
a_spank & 0.99992 \nonumber\\
picture & 0.99992 \nonumber\\
._everyone & 0.99992 \nonumber\\
turn_in & 0.99992 \nonumber\\
separate_from & 0.99992 \nonumber\\
if_a & 0.99992 \nonumber\\
means & 0.99992 \nonumber\\
alway_be & 0.99992 \nonumber\\
ModalVerbMay & 0.99992 \nonumber\\
provider & 0.99992 \nonumber\\
singapore_. & 0.99992 \nonumber\\
however_i & 0.99992 \nonumber\\
course & 0.99992 \nonumber\\
of_course & 0.99992 \nonumber\\
basic & 0.99992 \nonumber\\
knowledge & 0.99992 \nonumber\\
ProductionRule_ADJP->ADVP,JJ,CC,JJ, & 0.99992 \nonumber\\
alone & 0.99992 \nonumber\\
_pos_ngram_V_CONJ_ADV & 0.99992 \nonumber\\
get_the & 0.99992 \nonumber\\
a_religious & 0.99992 \nonumber\\
happen_. & 0.99992 \nonumber\\
grow_up & 0.99992 \nonumber\\
_pos_ngram_NN_NN_CARD & 0.99992 \nonumber\\
right_? & 0.99992 \nonumber\\
'_be & 0.99992 \nonumber\\
success & 0.99992 \nonumber\\
the_supreme & 0.99992 \nonumber\\
supreme & 0.99992 \nonumber\\
he_would & 0.99992 \nonumber\\
evolution_to & 0.99992 \nonumber\\
he_have & 0.99992 \nonumber\\
significance & 0.99992 \nonumber\\
in_school & 0.99992 \nonumber\\
be_great & 0.99992 \nonumber\\
he_will & 0.99992 \nonumber\\
not_make & 0.99992 \nonumber\\
ProductionRule_ADJP->RBS,JJ, & 0.99992 \nonumber\\
_pos_ngram_ADV_NN_NN & 0.99992 \nonumber\\
._to & 0.99992 \nonumber\\
everybody & 0.99992 \nonumber\\
need_of & 0.99992 \nonumber\\
not_try & 0.99992 \nonumber\\
toward & 0.99992 \nonumber\\
_pos_ngram_CARD_NN_ADV & 0.99992 \nonumber\\
and_your & 0.99992 \nonumber\\
_pos_ngram_NN_PUNC_O & 0.99992 \nonumber\\
_pos_ngram_PP_PP_CARD & 0.99992 \nonumber\\
ProductionRule_ADJP->RBR,JJ, & 0.99992 \nonumber\\
have_do & 0.99992 \nonumber\\
avoid & 0.99992 \nonumber\\
family & 0.99992 \nonumber\\
"_what & 0.99992 \nonumber\\
your_own & 0.99992 \nonumber\\
marriage_, & 0.99992 \nonumber\\
want_him & 0.99992 \nonumber\\
everyone & 0.99992 \nonumber\\
_pos_ngram_CONJ_PP_PP & 0.99992 \nonumber\\
else_. & 0.99992 \nonumber\\
rigor & 0.99992 \nonumber\\
radiometric_date & 0.99992 \nonumber\\
radiometric & 0.99992 \nonumber\\
scientific_rigor & 0.99992 \nonumber\\
for_other & 0.99992 \nonumber\\
ProductionRule_VP->VBZ,RB,ADJP, & 0.99992 \nonumber\\
creature & 0.99992 \nonumber\\
_pos_ngram_V_PR_NP & 0.99992 \nonumber\\
just_like & 0.99992 \nonumber\\
well_, & 0.99992 \nonumber\\
pe_because & 0.99992 \nonumber\\
theory_of & 0.99992 \nonumber\\
the_theory & 0.99992 \nonumber\\
walk & 0.99992 \nonumber\\
question_. & 0.99992 \nonumber\\
have_that & 0.99992 \nonumber\\
_pos_ngram_ADV_PR_PUNC & 0.99992 \nonumber\\
your_mom & 0.99992 \nonumber\\
_pos_ngram_ART_PUNC_PP & 0.99992 \nonumber\\
illness & 0.99992 \nonumber\\
in_instance & 0.99992 \nonumber\\
illness_. & 0.99992 \nonumber\\
hold_validity & 0.99992 \nonumber\\
intervene & 0.99992 \nonumber\\
instance_of & 0.99992 \nonumber\\
mental_illness & 0.99992 \nonumber\\
validity & 0.99992 \nonumber\\
mental_stability & 0.99992 \nonumber\\
since_in & 0.99992 \nonumber\\
validity_since & 0.99992 \nonumber\\
intervene_in & 0.99992 \nonumber\\
stability_and & 0.99992 \nonumber\\
stability & 0.99992 \nonumber\\
._try & 0.99992 \nonumber\\
argument_do & 0.99992 \nonumber\\
you_site & 0.99992 \nonumber\\
to_reason & 0.99992 \nonumber\\
the_mental & 0.99992 \nonumber\\
compromise_. & 0.99992 \nonumber\\
case_in & 0.99992 \nonumber\\
will_need & 0.99992 \nonumber\\
compromise & 0.99992 \nonumber\\
state_intervene & 0.99992 \nonumber\\
completely_compromise & 0.99992 \nonumber\\
better_answer & 0.99992 \nonumber\\
of_mental & 0.99992 \nonumber\\
site_, & 0.99992 \nonumber\\
case_you & 0.99992 \nonumber\\
try_again & 0.99992 \nonumber\\
_pos_ngram_O_ART_V & 0.99992 \nonumber\\
prison & 0.99992 \nonumber\\
_pos_ngram_O_PUNC_PP & 0.99992 \nonumber\\
it_should & 0.99992 \nonumber\\
make_. & 0.99992 \nonumber\\
information_. & 0.99992 \nonumber\\
court & 0.99992 \nonumber\\
supreme_court & 0.99992 \nonumber\\
_pos_ngram_O_PP_NP & 0.99992 \nonumber\\
child_because & 0.99992 \nonumber\\
power & 0.99992 \nonumber\\
why_should & 0.99992 \nonumber\\
ability & 0.99992 \nonumber\\
._so & 0.99992 \nonumber\\
power_to & 0.99992 \nonumber\\
be_true & 0.99992 \nonumber\\
thousand_of & 0.99992 \nonumber\\
carry & 0.99992 \nonumber\\
ProductionRule_SBAR->SBAR,,,CC,SBAR, & 0.99992 \nonumber\\
it_could & 0.99992 \nonumber\\
by_society & 0.99992 \nonumber\\
process_. & 0.99992 \nonumber\\
never_be & 0.99992 \nonumber\\
ProductionRule_VP->VBP,NP,PP, & 0.99992 \nonumber\\
malacca & 0.99992 \nonumber\\
evolution & 0.99992 \nonumber\\
not_like & 0.99992 \nonumber\\
mean_that & 0.99992 \nonumber\\
a_healthy & 0.99992 \nonumber\\
firefox & 0.99992 \nonumber\\
his_mistake & 0.99992 \nonumber\\
opposite_gender & 0.99992 \nonumber\\
gender_. & 0.99992 \nonumber\\
and_know & 0.99992 \nonumber\\
obese & 0.99992 \nonumber\\
ProductionRule_SBARQ->WHADVP,SQ,., & 0.99992 \nonumber\\
_pos_ngram_CONJ_ART_ART & 0.99992 \nonumber\\
woman_can & 0.99992 \nonumber\\
would_not & 0.99992 \nonumber\\
lousy_. & 0.99992 \nonumber\\
you_wear & 0.99992 \nonumber\\
_pos_ngram_PUNC_CONJ_ADJ & 0.99992 \nonumber\\
a_parent & 0.99992 \nonumber\\
one_. & 0.99992 \nonumber\\
succeed & 0.99992 \nonumber\\
yourself_, & 0.99992 \nonumber\\
indium_have & 0.99992 \nonumber\\
_pos_ngram_NN_ADJ_O & 0.99992 \nonumber\\
cause & 0.99992 \nonumber\\
way_i & 0.99992 \nonumber\\
out & 0.99992 \nonumber\\
ProductionRule_NP->NP,CC,NP, & 0.99992 \nonumber\\
._murder & 0.99992 \nonumber\\
progress & 0.99992 \nonumber\\
prove_that & 0.99992 \nonumber\\
the_state & 0.99992 \nonumber\\
dangerous & 0.99993 \nonumber\\
balance & 0.99993 \nonumber\\
._both & 0.99993 \nonumber\\
mean_the & 0.99993 \nonumber\\
and_ability & 0.99993 \nonumber\\
due & 0.99993 \nonumber\\
with_your & 0.99993 \nonumber\\
hope_you & 0.99993 \nonumber\\
time_you & 0.99993 \nonumber\\
so_until & 0.99993 \nonumber\\
brainwash & 0.99993 \nonumber\\
pro_choice & 0.99993 \nonumber\\
do_this & 0.99993 \nonumber\\
they_commit & 0.99993 \nonumber\\
and_then & 0.99993 \nonumber\\
be_hard & 0.99993 \nonumber\\
to_other & 0.99993 \nonumber\\
about_, & 0.99993 \nonumber\\
have_help & 0.99993 \nonumber\\
crisp & 0.99993 \nonumber\\
crash & 0.99993 \nonumber\\
the_school & 0.99993 \nonumber\\
_pos_ngram_ADJ_PP_PUNC & 0.99993 \nonumber\\
due_to & 0.99993 \nonumber\\
and_murder & 0.99993 \nonumber\\
make_sure & 0.99993 \nonumber\\
in_a & 0.99993 \nonumber\\
you_point & 0.99993 \nonumber\\
_pos_ngram_CONJ_CONJ & 0.99993 \nonumber\\
better_way & 0.99993 \nonumber\\
anyone_who & 0.99993 \nonumber\\
make_any & 0.99993 \nonumber\\
_pos_ngram_V_ART_ADV & 0.99993 \nonumber\\
world_and & 0.99993 \nonumber\\
make_it & 0.99993 \nonumber\\
up_on & 0.99993 \nonumber\\
belief_. & 0.99993 \nonumber\\
benefit & 0.99993 \nonumber\\
ProductionRule_NP->JJ,NNP, & 0.99993 \nonumber\\
what_the & 0.99993 \nonumber\\
_pos_ngram_PR_NP_PUNC & 0.99993 \nonumber\\
i_wish & 0.99993 \nonumber\\
style & 0.99993 \nonumber\\
ProductionRule_NP->DT,JJ,JJ,NNS, & 0.99993 \nonumber\\
and_allow & 0.99993 \nonumber\\
should_hit & 0.99993 \nonumber\\
hit_you & 0.99993 \nonumber\\
steal_you & 0.99993 \nonumber\\
or_steal & 0.99993 \nonumber\\
your_car & 0.99993 \nonumber\\
like_crash & 0.99993 \nonumber\\
really_bid & 0.99993 \nonumber\\
crash_your & 0.99993 \nonumber\\
something_really & 0.99993 \nonumber\\
bid_like & 0.99993 \nonumber\\
car_or & 0.99993 \nonumber\\
_pos_ngram_V_NP_PUNC & 0.99993 \nonumber\\
_pos_ngram_V_CONJ_PP & 0.99993 \nonumber\\
_pos_ngram_PUNC_PUNC_O & 0.99993 \nonumber\\
avoid_something & 0.99993 \nonumber\\
such_assertion & 0.99993 \nonumber\\
,_back & 0.99993 \nonumber\\
evidence_, & 0.99993 \nonumber\\
cosmology & 0.99993 \nonumber\\
prove_anything & 0.99993 \nonumber\\
assertion_. & 0.99993 \nonumber\\
not_once & 0.99993 \nonumber\\
again_, & 0.99993 \nonumber\\
once_do & 0.99993 \nonumber\\
about_evolution & 0.99993 \nonumber\\
to_steer & 0.99993 \nonumber\\
cosmology_. & 0.99993 \nonumber\\
just_avoid & 0.99993 \nonumber\\
not_answer & 0.99993 \nonumber\\
ask_be & 0.99993 \nonumber\\
debate_away & 0.99993 \nonumber\\
any_such & 0.99993 \nonumber\\
not_cosmology & 0.99993 \nonumber\\
steer_the & 0.99993 \nonumber\\
credible_evidence & 0.99993 \nonumber\\
up_your & 0.99993 \nonumber\\
credible & 0.99993 \nonumber\\
assertion & 0.99993 \nonumber\\
evolve_with & 0.99993 \nonumber\\
not_back & 0.99993 \nonumber\\
sabrejimmy_, & 0.99993 \nonumber\\
steer & 0.99993 \nonumber\\
herring_, & 0.99993 \nonumber\\
with_credible & 0.99993 \nonumber\\
bang_be & 0.99993 \nonumber\\
i_ask & 0.99993 \nonumber\\
learn_to & 0.99993 \nonumber\\
of_us & 0.99993 \nonumber\\
or_hear & 0.99993 \nonumber\\
not_happen & 0.99993 \nonumber\\
as_be & 0.99993 \nonumber\\
day & 0.99993 \nonumber\\
do_learn & 0.99993 \nonumber\\
ProductionRule_ADJP->RB,JJ,PP, & 0.99993 \nonumber\\
_pos_ngram_ADJ_PR_PR & 0.99993 \nonumber\\
run & 0.99993 \nonumber\\
._life & 0.99993 \nonumber\\
economy & 0.99993 \nonumber\\
ProductionRule_VP->VBP,S,SBAR, & 0.99993 \nonumber\\
_pos_ngram_ADV_ART_V & 0.99993 \nonumber\\
_pos_ngram_PP_CONJ_PP & 0.99993 \nonumber\\
type & 0.99993 \nonumber\\
type_of & 0.99993 \nonumber\\
wholly & 0.99993 \nonumber\\
ProductionRule_VP->VBN,S, & 0.99993 \nonumber\\
reach_common & 0.99993 \nonumber\\
to_reach & 0.99993 \nonumber\\
cant_better & 0.99993 \nonumber\\
may_see & 0.99993 \nonumber\\
other_if & 0.99993 \nonumber\\
that_as & 0.99993 \nonumber\\
good_if & 0.99993 \nonumber\\
prove_to & 0.99993 \nonumber\\
ProductionRule_VP->VBZ,NP,ADVP, & 0.99993 \nonumber\\
you_never & 0.99993 \nonumber\\
major & 0.99993 \nonumber\\
spongebob & 0.99993 \nonumber\\
no_reason & 0.99993 \nonumber\\
book_, & 0.99993 \nonumber\\
_pos_ngram_CONJ_NP_O & 0.99993 \nonumber\\
time_, & 0.99993 \nonumber\\
_pos_ngram_NN_ART_CARD & 0.99993 \nonumber\\
pursuit_. & 0.99993 \nonumber\\
of_view & 0.99993 \nonumber\\
select_singapore & 0.99993 \nonumber\\
another_british & 0.99993 \nonumber\\
to_select & 0.99993 \nonumber\\
british_base & 0.99993 \nonumber\\
of_shape & 0.99993 \nonumber\\
we_should & 0.99993 \nonumber\\
never_do & 0.99993 \nonumber\\
ProductionRule_NP->DT,JJ,NN,CC,NN, & 0.99993 \nonumber\\
ProductionRule_NP->DT,JJ, & 0.99993 \nonumber\\
community_agree & 0.99993 \nonumber\\
entire_scientific & 0.99993 \nonumber\\
happen_and & 0.99993 \nonumber\\
still_happen & 0.99993 \nonumber\\
scientific_community & 0.99993 \nonumber\\
argument_need & 0.99993 \nonumber\\
entire & 0.99993 \nonumber\\
agree_: & 0.99993 \nonumber\\
the_entire & 0.99993 \nonumber\\
evolution_happen & 0.99993 \nonumber\\
should_have & 0.99993 \nonumber\\
_pos_ngram_PR_PUNC_ADV & 0.99993 \nonumber\\
herring & 0.99993 \nonumber\\
red_herring & 0.99993 \nonumber\\
spring & 0.99993 \nonumber\\
consistency & 0.99993 \nonumber\\
system_that & 0.99993 \nonumber\\
sip & 0.99993 \nonumber\\
federal_regulation & 0.99993 \nonumber\\
time_per & 0.99993 \nonumber\\
hygienically_design & 0.99993 \nonumber\\
we_test & 0.99993 \nonumber\\
we_employ & 0.99993 \nonumber\\
federal & 0.99993 \nonumber\\
carefully_control & 0.99993 \nonumber\\
poland_spring & 0.99993 \nonumber\\
possible_contaminants-far & 0.99993 \nonumber\\
freshness_and & 0.99993 \nonumber\\
say_http://delivery.polandspring.com/delivery/home/help/ourwater.aspx & 0.99993 \nonumber\\
require_. & 0.99993 \nonumber\\
carefully & 0.99993 \nonumber\\
to_maintain & 0.99993 \nonumber\\
the_purity & 0.99993 \nonumber\\
poland & 0.99993 \nonumber\\
bottle_process & 0.99993 \nonumber\\
200_possible & 0.99993 \nonumber\\
you_take & 0.99993 \nonumber\\
contaminants-far & 0.99993 \nonumber\\
will_enjoy & 0.99993 \nonumber\\
nuff_say & 0.99993 \nonumber\\
standard_help & 0.99993 \nonumber\\
design_line & 0.99993 \nonumber\\
in_hygienically & 0.99993 \nonumber\\
involve_carefully & 0.99993 \nonumber\\
a_comprehensive & 0.99993 \nonumber\\
we_screen & 0.99993 \nonumber\\
screen & 0.99993 \nonumber\\
for_over & 0.99993 \nonumber\\
regulation_require & 0.99993 \nonumber\\
at_poland & 0.99993 \nonumber\\
the_plant & 0.99993 \nonumber\\
-_nuff & 0.99993 \nonumber\\
disinfection_process & 0.99993 \nonumber\\
multi-barrier_filtration & 0.99993 \nonumber\\
disinfection & 0.99993 \nonumber\\
sip_. & 0.99993 \nonumber\\
at_every & 0.99993 \nonumber\\
consistency_several & 0.99993 \nonumber\\
rigorous_quality & 0.99993 \nonumber\\
consistency_go & 0.99993 \nonumber\\
than_state & 0.99993 \nonumber\\
multi-barrier & 0.99993 \nonumber\\
enjoy_the & 0.99993 \nonumber\\
delicious_water & 0.99993 \nonumber\\
delicious & 0.99993 \nonumber\\
that_involve & 0.99993 \nonumber\\
control_standard & 0.99993 \nonumber\\
our_rigorous & 0.99993 \nonumber\\
crisp_, & 0.99993 \nonumber\\
purity & 0.99993 \nonumber\\
contaminants-far_more & 0.99993 \nonumber\\
freshness & 0.99993 \nonumber\\
hour_at & 0.99993 \nonumber\\
that_freshness & 0.99993 \nonumber\\
employ & 0.99993 \nonumber\\
come_into & 0.99993 \nonumber\\
a_sip & 0.99993 \nonumber\\
continuously & 0.99993 \nonumber\\
and_continuously & 0.99993 \nonumber\\
rigorous & 0.99993 \nonumber\\
and_consistency & 0.99993 \nonumber\\
monitor & 0.99993 \nonumber\\
for_consistency & 0.99993 \nonumber\\
monitor_disinfection & 0.99993 \nonumber\\
plant_and & 0.99993 \nonumber\\
us_make & 0.99993 \nonumber\\
and_federal & 0.99993 \nonumber\\
,_multi-barrier & 0.99993 \nonumber\\
every_stage & 0.99993 \nonumber\\
over_200 & 0.99993 \nonumber\\
spring_, & 0.99993 \nonumber\\
employ_a & 0.99993 \nonumber\\
"_at & 0.99993 \nonumber\\
maintain_the & 0.99993 \nonumber\\
quality_control & 0.99993 \nonumber\\
same_crisp & 0.99993 \nonumber\\
state_and & 0.99993 \nonumber\\
,_delicious & 0.99993 \nonumber\\
control_and & 0.99993 \nonumber\\
filtration & 0.99993 \nonumber\\
test_our & 0.99993 \nonumber\\
comprehensive & 0.99993 \nonumber\\
nuff & 0.99993 \nonumber\\
hygienically & 0.99993 \nonumber\\
process_in & 0.99993 \nonumber\\
screen_for & 0.99993 \nonumber\\
per_hour & 0.99993 \nonumber\\
purity_of & 0.99993 \nonumber\\
filtration_system & 0.99993 \nonumber\\
continuously_monitor & 0.99993 \nonumber\\
comprehensive_, & 0.99993 \nonumber\\
rule_by & 0.99993 \nonumber\\
see_that & 0.99993 \nonumber\\
to_marry & 0.99993 \nonumber\\
ProductionRule_VP->VBP,ADVP,PP, & 0.99993 \nonumber\\
we_know & 0.99993 \nonumber\\
mean_be & 0.99993 \nonumber\\
story_, & 0.99993 \nonumber\\
ProductionRule_SBARQ->WHNP,SQ, & 0.99993 \nonumber\\
reason_to & 0.99993 \nonumber\\
will_turn & 0.99993 \nonumber\\
child_and & 0.99993 \nonumber\\
you_a & 0.99993 \nonumber\\
not_gay & 0.99993 \nonumber\\
learn_from & 0.99993 \nonumber\\
s & 0.99993 \nonumber\\
know_if & 0.99993 \nonumber\\
?_" & 0.99993 \nonumber\\
solve_the & 0.99993 \nonumber\\
._our & 0.99993 \nonumber\\
be_why & 0.99993 \nonumber\\
what_we & 0.99993 \nonumber\\
:_evolution & 0.99993 \nonumber\\
do_in & 0.99993 \nonumber\\
and_understand & 0.99993 \nonumber\\
should_do & 0.99993 \nonumber\\
punish & 0.99993 \nonumber\\
if_my & 0.99993 \nonumber\\
this_way & 0.99993 \nonumber\\
the_island & 0.99993 \nonumber\\
,_people & 0.99993 \nonumber\\
who_i & 0.99993 \nonumber\\
_pos_ngram_NP_PR & 0.99993 \nonumber\\
sister_and & 0.99993 \nonumber\\
_pos_ngram_O_V_PUNC & 0.99993 \nonumber\\
nor_be & 0.99993 \nonumber\\
hit_them & 0.99993 \nonumber\\
ProductionRule_ADJP->ADJP,CC,ADJP, & 0.99993 \nonumber\\
and_thus & 0.99993 \nonumber\\
together & 0.99993 \nonumber\\
i_want & 0.99993 \nonumber\\
charge & 0.99993 \nonumber\\
defense_for & 0.99993 \nonumber\\
hard_on & 0.99993 \nonumber\\
that_porn & 0.99993 \nonumber\\
surely & 0.99993 \nonumber\\
ProductionRule_PP->ADVP,IN,NP, & 0.99993 \nonumber\\
first_. & 0.99993 \nonumber\\
be_brainwash & 0.99993 \nonumber\\
copy & 0.99993 \nonumber\\
difference_? & 0.99993 \nonumber\\
you_kid & 0.99993 \nonumber\\
come_from & 0.99993 \nonumber\\
ProductionRule_ADVP->DT,RBR, & 0.99993 \nonumber\\
bully_. & 0.99993 \nonumber\\
to_this & 0.99993 \nonumber\\
and_more & 0.99993 \nonumber\\
there_to & 0.99993 \nonumber\\
,_feel & 0.99993 \nonumber\\
than_personal & 0.99993 \nonumber\\
this_restriction & 0.99993 \nonumber\\
length_for & 0.99993 \nonumber\\
and_discourse & 0.99993 \nonumber\\
can_keep & 0.99993 \nonumber\\
the_quality & 0.99993 \nonumber\\
length & 0.99993 \nonumber\\
dumb_joke & 0.99993 \nonumber\\
to_cut & 0.99993 \nonumber\\
cut_down & 0.99993 \nonumber\\
joke & 0.99993 \nonumber\\
joke_, & 0.99993 \nonumber\\
as_high & 0.99993 \nonumber\\
high_as & 0.99993 \nonumber\\
be_50 & 0.99993 \nonumber\\
restriction_be & 0.99993 \nonumber\\
minimum_length & 0.99993 \nonumber\\
50_character & 0.99993 \nonumber\\
character_. & 0.99993 \nonumber\\
discourse & 0.99993 \nonumber\\
of_dumb & 0.99993 \nonumber\\
discourse_as & 0.99993 \nonumber\\
minimum & 0.99993 \nonumber\\
down_on & 0.99993 \nonumber\\
health & 0.99993 \nonumber\\
i_mean & 0.99993 \nonumber\\
._with & 0.99993 \nonumber\\
ProductionRule_VP->VBD,ADJP,SBAR, & 0.99993 \nonumber\\
._1 & 0.99993 \nonumber\\
be_' & 0.99993 \nonumber\\
that_gay & 0.99993 \nonumber\\
_pos_ngram_NP_V_PR & 0.99993 \nonumber\\
._why & 0.99993 \nonumber\\
it_like & 0.99993 \nonumber\\
why_. & 0.99993 \nonumber\\
,_as & 0.99993 \nonumber\\
be_consider & 0.99993 \nonumber\\
part & 0.99993 \nonumber\\
feel_it & 0.99993 \nonumber\\
ProductionRule_VP->RB,VP, & 0.99993 \nonumber\\
case_gay & 0.99993 \nonumber\\
ProductionRule_VP->VBG,S, & 0.99993 \nonumber\\
ProductionRule_VP->VB,PRT, & 0.99993 \nonumber\\
sign & 0.99993 \nonumber\\
pretty_sure & 0.99993 \nonumber\\
_pos_ngram_ADJ_O_O & 0.99993 \nonumber\\
beside & 0.99993 \nonumber\\
_pos_ngram_ADJ_O_PUNC & 0.99993 \nonumber\\
_pos_ngram_ADJ_V_NN & 0.99993 \nonumber\\
into_the & 0.99993 \nonumber\\
wholly_believe & 0.99993 \nonumber\\
lucky_to & 0.99993 \nonumber\\
still_wholly & 0.99993 \nonumber\\
to_encounter & 0.99993 \nonumber\\
ProductionRule_NP->DT,NN,JJ, & 0.99993 \nonumber\\
encounter_a & 0.99993 \nonumber\\
_pos_ngram_CONJ_ADJ_PR & 0.99993 \nonumber\\
consider_myself & 0.99993 \nonumber\\
who_still & 0.99993 \nonumber\\
baptist_church & 0.99993 \nonumber\\
freewill & 0.99993 \nonumber\\
preach & 0.99993 \nonumber\\
not_religion & 0.99993 \nonumber\\
church_full & 0.99993 \nonumber\\
and_teaching & 0.99993 \nonumber\\
christian_, & 0.99993 \nonumber\\
they_preach & 0.99993 \nonumber\\
freewill_baptist & 0.99993 \nonumber\\
practice_what & 0.99993 \nonumber\\
preach_. & 0.99993 \nonumber\\
only_now & 0.99993 \nonumber\\
the_belief & 0.99993 \nonumber\\
encounter & 0.99993 \nonumber\\
baptist & 0.99993 \nonumber\\
a_freewill & 0.99993 \nonumber\\
kind_and & 0.99993 \nonumber\\
actually_kind & 0.99993 \nonumber\\
non-denominational_who & 0.99993 \nonumber\\
myself_a & 0.99993 \nonumber\\
a_church & 0.99993 \nonumber\\
non-denominational & 0.99993 \nonumber\\
a_non-denominational & 0.99993 \nonumber\\
illegal & 0.99993 \nonumber\\
plan_, & 0.99993 \nonumber\\
do_something & 0.99993 \nonumber\\
association & 0.99993 \nonumber\\
ProductionRule_NP->DT,NN,SBAR, & 0.99993 \nonumber\\
._because & 0.99993 \nonumber\\
way_. & 0.99993 \nonumber\\
._without & 0.99993 \nonumber\\
time_. & 0.99993 \nonumber\\
be_raise & 0.99993 \nonumber\\
poorly & 0.99993 \nonumber\\
a_specific & 0.99993 \nonumber\\
have_be & 0.99993 \nonumber\\
lose & 0.99993 \nonumber\\
_pos_ngram_NN_O_PR & 0.99993 \nonumber\\
brother_marriage & 0.99993 \nonumber\\
and_brother & 0.99993 \nonumber\\
too_? & 0.99993 \nonumber\\
brother_and & 0.99993 \nonumber\\
ok_... & 0.99993 \nonumber\\
and_sister & 0.99993 \nonumber\\
ok_too & 0.99993 \nonumber\\
why_gay & 0.99993 \nonumber\\
or_brother & 0.99993 \nonumber\\
..._right & 0.99993 \nonumber\\
then_sister & 0.99993 \nonumber\\
?_oh & 0.99993 \nonumber\\
if_gay & 0.99993 \nonumber\\
brother_be & 0.99993 \nonumber\\
oh_wait & 0.99993 \nonumber\\
marriage_could & 0.99993 \nonumber\\
wait_, & 0.99993 \nonumber\\
the_sex & 0.99993 \nonumber\\
difference_, & 0.99993 \nonumber\\
sister_or & 0.99993 \nonumber\\
so_sister & 0.99993 \nonumber\\
"_, & 0.99993 \nonumber\\
'd_have & 0.99993 \nonumber\\
an_alright & 0.99993 \nonumber\\
of_television & 0.99993 \nonumber\\
for_spongebob & 0.99993 \nonumber\\
except_for & 0.99993 \nonumber\\
be_awful & 0.99993 \nonumber\\
book_base & 0.99993 \nonumber\\
still_, & 0.99993 \nonumber\\
maybe_. & 0.99993 \nonumber\\
spongebob_maybe & 0.99993 \nonumber\\
awful_. & 0.99993 \nonumber\\
terrible_. & 0.99993 \nonumber\\
alright_show & 0.99993 \nonumber\\
show_. & 0.99993 \nonumber\\
._still & 0.99993 \nonumber\\
._except & 0.99993 \nonumber\\
this_can & 0.99993 \nonumber\\
ProductionRule_VP->VP,CC,VP,SBAR, & 0.99993 \nonumber\\
know_how & 0.99993 \nonumber\\
especially & 0.99993 \nonumber\\
be_be & 0.99993 \nonumber\\
only_care & 0.99993 \nonumber\\
more_and & 0.99993 \nonumber\\
company_be & 0.99993 \nonumber\\
to_love & 0.99993 \nonumber\\
._no & 0.99994 \nonumber\\
to_ask & 0.99994 \nonumber\\
founder_because & 0.99994 \nonumber\\
raffle_leave & 0.99994 \nonumber\\
with_me & 0.99994 \nonumber\\
indium & 0.99994 \nonumber\\
rather_than & 0.99994 \nonumber\\
be_terrible & 0.99994 \nonumber\\
ie_be & 0.99994 \nonumber\\
between_the & 0.99994 \nonumber\\
cause_the & 0.99994 \nonumber\\
upon & 0.99994 \nonumber\\
ProductionRule_S->SBAR,NP,VP,., & 0.99994 \nonumber\\
school_be & 0.99994 \nonumber\\
of_this & 0.99994 \nonumber\\
with_my & 0.99994 \nonumber\\
father_there & 0.99994 \nonumber\\
ability_to & 0.99994 \nonumber\\
parent_attitude & 0.99994 \nonumber\\
ProductionRule_NP->DT,NN,CC,NNS, & 0.99994 \nonumber\\
ProductionRule_VP->JJ,NP,NP, & 0.99994 \nonumber\\
can_pick & 0.99994 \nonumber\\
example_use & 0.99994 \nonumber\\
and_parent & 0.99994 \nonumber\\
might_effect & 0.99994 \nonumber\\
effect_the & 0.99994 \nonumber\\
attitude_act & 0.99994 \nonumber\\
pick_up & 0.99994 \nonumber\\
solve_problem & 0.99994 \nonumber\\
technique_. & 0.99994 \nonumber\\
spank_might & 0.99994 \nonumber\\
act_violent & 0.99994 \nonumber\\
relationship_between & 0.99994 \nonumber\\
violent_. & 0.99994 \nonumber\\
not_leave & 0.99994 \nonumber\\
ProductionRule_PP->IN,FRAG, & 0.99994 \nonumber\\
a_few & 0.99994 \nonumber\\
reality & 0.99994 \nonumber\\
figure & 0.99994 \nonumber\\
ProductionRule_NP->PDT,DT,NNS, & 0.99994 \nonumber\\
_pos_ngram_O_PUNC_ADV & 0.99994 \nonumber\\
bid_idea & 0.99994 \nonumber\\
'_the & 0.99994 \nonumber\\
ProductionRule_S->S,CC,S,., & 0.99994 \nonumber\\
be_human & 0.99994 \nonumber\\
why_do & 0.99994 \nonumber\\
'_something & 0.99994 \nonumber\\
ProductionRule_SQ->MD,NP,VP, & 0.99994 \nonumber\\
be_watch & 0.99994 \nonumber\\
the_sultan & 0.99994 \nonumber\\
'_an & 0.99994 \nonumber\\
impossible & 0.99994 \nonumber\\
better_because & 0.99994 \nonumber\\
system & 0.99994 \nonumber\\
_pos_ngram_PR_NN_ART & 0.99994 \nonumber\\
ProductionRule_NP->JJ,NN,NN,NN, & 0.99994 \nonumber\\
be_as & 0.99994 \nonumber\\
_pos_ngram_ADV_ADJ_CONJ & 0.99994 \nonumber\\
from_this & 0.99994 \nonumber\\
father_or & 0.99994 \nonumber\\
eat & 0.99994 \nonumber\\
._imagine & 0.99994 \nonumber\\
but_all & 0.99994 \nonumber\\
mean_it & 0.99994 \nonumber\\
kind & 0.99994 \nonumber\\
break & 0.99994 \nonumber\\
concept & 0.99994 \nonumber\\
a_low & 0.99994 \nonumber\\
._look & 0.99994 \nonumber\\
at_that & 0.99994 \nonumber\\
ProductionRule_SBAR->WHPP,S, & 0.99994 \nonumber\\
ProductionRule_WHPP->IN,WHNP, & 0.99994 \nonumber\\
each_other & 0.99994 \nonumber\\
ProductionRule_NP->NP,ADJP, & 0.99994 \nonumber\\
father_could & 0.99994 \nonumber\\
fatherless_than & 0.99994 \nonumber\\
world_because & 0.99994 \nonumber\\
know_? & 0.99994 \nonumber\\
of_other & 0.99994 \nonumber\\
_pos_ngram_CONJ_NN_PR & 0.99994 \nonumber\\
because_it & 0.99994 \nonumber\\
only_good & 0.99994 \nonumber\\
upon_their & 0.99994 \nonumber\\
bully_other & 0.99994 \nonumber\\
bully_under & 0.99994 \nonumber\\
of_bully & 0.99994 \nonumber\\
problem_concern & 0.99994 \nonumber\\
even_address & 0.99994 \nonumber\\
their_basic & 0.99994 \nonumber\\
the_in & 0.99994 \nonumber\\
of_or & 0.99994 \nonumber\\
bully_" & 0.99994 \nonumber\\
to_bully & 0.99994 \nonumber\\
reduce_bully & 0.99994 \nonumber\\
reduce_student & 0.99994 \nonumber\\
concern_bully & 0.99994 \nonumber\\
also_infringe & 0.99994 \nonumber\\
sweep & 0.99994 \nonumber\\
cousin_' & 0.99994 \nonumber\\
plus_the & 0.99994 \nonumber\\
be_individual & 0.99994 \nonumber\\
find_other & 0.99994 \nonumber\\
cousin & 0.99994 \nonumber\\
sweep_the & 0.99994 \nonumber\\
individual_and & 0.99994 \nonumber\\
my_cousin & 0.99994 \nonumber\\
or_reduce & 0.99994 \nonumber\\
clothe_label & 0.99994 \nonumber\\
mother_work & 0.99994 \nonumber\\
label_that & 0.99994 \nonumber\\
at_, & 0.99994 \nonumber\\
in_thing & 0.99994 \nonumber\\
,_plus & 0.99994 \nonumber\\
label & 0.99994 \nonumber\\
_pos_ngram_ART_CARD_ADJ & 0.99994 \nonumber\\
specific_clothe & 0.99994 \nonumber\\
dictate_be & 0.99994 \nonumber\\
utilize_school & 0.99994 \nonumber\\
other_reason & 0.99994 \nonumber\\
utilize & 0.99994 \nonumber\\
be_utilize & 0.99994 \nonumber\\
3_child & 0.99994 \nonumber\\
work_at & 0.99994 \nonumber\\
ProductionRule_NP->NP,CD,NNS, & 0.99994 \nonumber\\
infringe_upon & 0.99994 \nonumber\\
district_my & 0.99994 \nonumber\\
be_sweep & 0.99994 \nonumber\\
rug_. & 0.99994 \nonumber\\
they_dictate & 0.99994 \nonumber\\
infringe & 0.99994 \nonumber\\
address_the & 0.99994 \nonumber\\
rug & 0.99994 \nonumber\\
n't_wear & 0.99994 \nonumber\\
._while & 0.99994 \nonumber\\
basic_rights & 0.99994 \nonumber\\
the_rug & 0.99994 \nonumber\\
basic_type & 0.99994 \nonumber\\
good_it & 0.99994 \nonumber\\
all_it & 0.99994 \nonumber\\
'_3 & 0.99994 \nonumber\\
ProductionRule_NP->NP,,,CC,NP,,, & 0.99994 \nonumber\\
school_my & 0.99994 \nonumber\\
"_reduce & 0.99994 \nonumber\\
which_in & 0.99994 \nonumber\\
dictate & 0.99994 \nonumber\\
one_basic & 0.99994 \nonumber\\
reality_, & 0.99994 \nonumber\\
ProductionRule_NP->DT,JJ,CD,NNS, & 0.99994 \nonumber\\
_pos_ngram_PR_PUNC_V & 0.99994 \nonumber\\
_pos_ngram_ART_V_PP & 0.99994 \nonumber\\
perfectly & 0.99994 \nonumber\\
addition & 0.99994 \nonumber\\
in_addition & 0.99994 \nonumber\\
and_how & 0.99994 \nonumber\\
feel & 0.99994 \nonumber\\
student_should & 0.99994 \nonumber\\
single & 0.99994 \nonumber\\
_pos_ngram_O_NN_CONJ & 0.99994 \nonumber\\
love_you & 0.99994 \nonumber\\
then_not & 0.99994 \nonumber\\
be_argue & 0.99994 \nonumber\\
accomplish & 0.99994 \nonumber\\
select & 0.99994 \nonumber\\
you_then & 0.99994 \nonumber\\
british_. & 0.99994 \nonumber\\
awful & 0.99994 \nonumber\\
unhappy & 0.99994 \nonumber\\
monkey & 0.99994 \nonumber\\
for_their & 0.99994 \nonumber\\
obvious & 0.99994 \nonumber\\
_pos_ngram_CONJ_ADV_O & 0.99994 \nonumber\\
father_but & 0.99994 \nonumber\\
uniform_. & 0.99994 \nonumber\\
that_its & 0.99994 \nonumber\\
religion & 0.99994 \nonumber\\
other_technique & 0.99994 \nonumber\\
have_ever & 0.99994 \nonumber\\
several & 0.99994 \nonumber\\
that_for & 0.99994 \nonumber\\
like_to & 0.99994 \nonumber\\
_pos_ngram_ADV_ADV_NN & 0.99994 \nonumber\\
eventually & 0.99994 \nonumber\\
._much & 0.99994 \nonumber\\
let_you & 0.99994 \nonumber\\
out_his & 0.99994 \nonumber\\
or_it & 0.99994 \nonumber\\
other_around & 0.99994 \nonumber\\
but_man & 0.99994 \nonumber\\
that_do & 0.99994 \nonumber\\
,_only & 0.99994 \nonumber\\
except & 0.99994 \nonumber\\
team & 0.99994 \nonumber\\
_pos_ngram_PUNC_V_NP & 0.99994 \nonumber\\
a_school & 0.99994 \nonumber\\
rather_be & 0.99994 \nonumber\\
ProductionRule_QP->RB,CD, & 0.99994 \nonumber\\
people_you & 0.99994 \nonumber\\
prove & 0.99994 \nonumber\\
_pos_ngram_ART_CARD_PP & 0.99994 \nonumber\\
watch_. & 0.99994 \nonumber\\
ProductionRule_VP->VBD,RB,VP, & 0.99994 \nonumber\\
not_evolve & 0.99994 \nonumber\\
carry_out & 0.99994 \nonumber\\
in_need & 0.99994 \nonumber\\
the_people & 0.99994 \nonumber\\
strengthen_the & 0.99994 \nonumber\\
within_the & 0.99994 \nonumber\\
confide_in & 0.99994 \nonumber\\
ProductionRule_ADVP->IN,JJS, & 0.99994 \nonumber\\
key_component & 0.99994 \nonumber\\
hear_it & 0.99994 \nonumber\\
'_there & 0.99994 \nonumber\\
component_to & 0.99994 \nonumber\\
be_faith & 0.99994 \nonumber\\
gravity_, & 0.99994 \nonumber\\
gravity & 0.99994 \nonumber\\
._faith & 0.99994 \nonumber\\
faith_. & 0.99994 \nonumber\\
._gravity & 0.99994 \nonumber\\
to_christianity & 0.99994 \nonumber\\
component & 0.99994 \nonumber\\
_pos_ngram_ADV_PUNC_V & 0.99994 \nonumber\\
the_big & 0.99994 \nonumber\\
believe_the & 0.99994 \nonumber\\
an_example & 0.99994 \nonumber\\
why_not & 0.99994 \nonumber\\
such_as & 0.99994 \nonumber\\
selfish_and & 0.99994 \nonumber\\
everyone_should & 0.99994 \nonumber\\
counter & 0.99994 \nonumber\\
provide_the & 0.99994 \nonumber\\
involve_. & 0.99994 \nonumber\\
pregnant & 0.99994 \nonumber\\
restriction & 0.99994 \nonumber\\
._: & 0.99994 \nonumber\\
ProductionRule_VP->VBP,RB,ADJP, & 0.99994 \nonumber\\
think_its & 0.99994 \nonumber\\
hard & 0.99994 \nonumber\\
process_, & 0.99994 \nonumber\\
can_make & 0.99994 \nonumber\\
ProductionRule_VP->VB,ADVP,S, & 0.99994 \nonumber\\
indium_. & 0.99994 \nonumber\\
_pos_ngram_ADV_ADV_ADJ & 0.99994 \nonumber\\
to_worry & 0.99994 \nonumber\\
murder_be & 0.99994 \nonumber\\
good_at & 0.99994 \nonumber\\
rich & 0.99994 \nonumber\\
or_the & 0.99994 \nonumber\\
she_be & 0.99994 \nonumber\\
evolve_. & 0.99994 \nonumber\\
n't_expect & 0.99994 \nonumber\\
improve_. & 0.99994 \nonumber\\
other_improve & 0.99994 \nonumber\\
be_significant & 0.99994 \nonumber\\
significance_and & 0.99994 \nonumber\\
they_the & 0.99994 \nonumber\\
enviorment_around & 0.99994 \nonumber\\
good_there & 0.99994 \nonumber\\
the_goods & 0.99994 \nonumber\\
enviorment & 0.99994 \nonumber\\
ProductionRule_S->NP,DT,VP, & 0.99994 \nonumber\\
._personal & 0.99994 \nonumber\\
goods_help & 0.99994 \nonumber\\
different_nor & 0.99994 \nonumber\\
ProductionRule_VP->VBZ,ADVP,PP, & 0.99994 \nonumber\\
same_but & 0.99994 \nonumber\\
then_advance & 0.99994 \nonumber\\
honestly_i & 0.99994 \nonumber\\
balance_each & 0.99994 \nonumber\\
this_arguement & 0.99994 \nonumber\\
no_better & 0.99994 \nonumber\\
n't_perfect & 0.99994 \nonumber\\
significant_. & 0.99994 \nonumber\\
perfect_and & 0.99994 \nonumber\\
you_improve & 0.99994 \nonumber\\
they_both & 0.99994 \nonumber\\
they_balance & 0.99994 \nonumber\\
both_have & 0.99994 \nonumber\\
that_significance & 0.99994 \nonumber\\
arguement_, & 0.99994 \nonumber\\
self_for & 0.99994 \nonumber\\
the_enviorment & 0.99994 \nonumber\\
ProductionRule_VP->VBP,NP,PRT, & 0.99994 \nonumber\\
same_way & 0.99994 \nonumber\\
horrible & 0.99994 \nonumber\\
_pos_ngram_PP_NP_NP & 0.99994 \nonumber\\
fine & 0.99994 \nonumber\\
keep_the & 0.99994 \nonumber\\
our_water & 0.99994 \nonumber\\
a_baby & 0.99994 \nonumber\\
engineer & 0.99994 \nonumber\\
win & 0.99994 \nonumber\\
of_entertainment & 0.99994 \nonumber\\
the_minimum & 0.99994 \nonumber\\
protect & 0.99994 \nonumber\\
remind & 0.99994 \nonumber\\
debate_and & 0.99994 \nonumber\\
._every & 0.99994 \nonumber\\
ie_copy & 0.99994 \nonumber\\
7_.... & 0.99994 \nonumber\\
copy_in & 0.99994 \nonumber\\
that_close & 0.99994 \nonumber\\
be_tab & 0.99994 \nonumber\\
what_ie & 0.99994 \nonumber\\
look_what & 0.99994 \nonumber\\
version_7 & 0.99994 \nonumber\\
tab_... & 0.99994 \nonumber\\
deal_be & 0.99994 \nonumber\\
ProductionRule_NP->NN,CD,NN, & 0.99994 \nonumber\\
..._look & 0.99994 \nonumber\\
in_version & 0.99994 \nonumber\\
feature_that & 0.99994 \nonumber\\
ProductionRule_VP->VBZ,NP,:,FRAG, & 0.99994 \nonumber\\
one_feature & 0.99994 \nonumber\\
the_deal & 0.99994 \nonumber\\
pro_life & 0.99994 \nonumber\\
someone_who & 0.99994 \nonumber\\
_pos_ngram_PR_PUNC_O & 0.99994 \nonumber\\
_pos_ngram_O_PUNC_PUNC & 0.99994 \nonumber\\
secret & 0.99994 \nonumber\\
and_beside & 0.99994 \nonumber\\
plan & 0.99994 \nonumber\\
m & 0.99994 \nonumber\\
i_m & 0.99994 \nonumber\\
now_. & 0.99994 \nonumber\\
one_to & 0.99994 \nonumber\\
that_both & 0.99994 \nonumber\\
europe & 0.99994 \nonumber\\
wear & 0.99994 \nonumber\\
to_discipline & 0.99994 \nonumber\\
,_should & 0.99994 \nonumber\\
be_sure & 0.99994 \nonumber\\
n't_exist & 0.99994 \nonumber\\
confide & 0.99994 \nonumber\\
be_proclaim & 0.99994 \nonumber\\
although_farquhar & 0.99994 \nonumber\\
who_stay & 0.99994 \nonumber\\
strategize_, & 0.99994 \nonumber\\
singapore_support & 0.99994 \nonumber\\
ProductionRule_VP->VBG,NP,NP, & 0.99994 \nonumber\\
leave_of & 0.99994 \nonumber\\
its_development & 0.99994 \nonumber\\
strategize & 0.99994 \nonumber\\
singapore_under & 0.99994 \nonumber\\
as_another & 0.99994 \nonumber\\
the_order & 0.99994 \nonumber\\
grunt_work & 0.99994 \nonumber\\
the_supervisor & 0.99994 \nonumber\\
commission & 0.99994 \nonumber\\
give_early & 0.99994 \nonumber\\
work_" & 0.99994 \nonumber\\
support_its & 0.99994 \nonumber\\
ProductionRule_NP->NP,,,NP,,, & 0.99994 \nonumber\\
of_free & 0.99994 \nonumber\\
proclaim_the & 0.99994 \nonumber\\
most_commission & 0.99994 \nonumber\\
proclaim & 0.99994 \nonumber\\
a_construction & 0.99994 \nonumber\\
contractor_? & 0.99994 \nonumber\\
site_get & 0.99994 \nonumber\\
base_, & 0.99994 \nonumber\\
contractor & 0.99994 \nonumber\\
construction_site & 0.99994 \nonumber\\
"_grunt & 0.99994 \nonumber\\
raffle_provide & 0.99994 \nonumber\\
the_contractor & 0.99994 \nonumber\\
grunt & 0.99994 \nonumber\\
commission_, & 0.99994 \nonumber\\
free_will & 0.99994 \nonumber\\
if_william & 0.99994 \nonumber\\
the_strategize & 0.99994 \nonumber\\
early_singapore & 0.99994 \nonumber\\
supervisor_of & 0.99994 \nonumber\\
supervisor & 0.99994 \nonumber\\
the_law & 0.99994 \nonumber\\
us & 0.99994 \nonumber\\
study_. & 0.99994 \nonumber\\
because_no & 0.99994 \nonumber\\
purpose_of & 0.99994 \nonumber\\
the_purpose & 0.99994 \nonumber\\
student & 0.99994 \nonumber\\
spank_as & 0.99994 \nonumber\\
use_spank & 0.99994 \nonumber\\
for_any & 0.99994 \nonumber\\
ProductionRule_VP->VP,VP, & 0.99994 \nonumber\\
situation_. & 0.99994 \nonumber\\
have_nothing & 0.99994 \nonumber\\
_pos_ngram_ART_NP_PUNC & 0.99994 \nonumber\\
attitude & 0.99994 \nonumber\\
go_on & 0.99994 \nonumber\\
to_" & 0.99994 \nonumber\\
the_leader & 0.99994 \nonumber\\
poorly_develop & 0.99994 \nonumber\\
unhappy_. & 0.99994 \nonumber\\
responsibilily_and & 0.99994 \nonumber\\
murder_everywhere & 0.99994 \nonumber\\
leader_and & 0.99994 \nonumber\\
of_farquhar & 0.99994 \nonumber\\
be_unhappy & 0.99994 \nonumber\\
slave & 0.99994 \nonumber\\
everywhere_in & 0.99994 \nonumber\\
the_boss & 0.99994 \nonumber\\
so_poorly & 0.99994 \nonumber\\
more_rights & 0.99994 \nonumber\\
cockfight & 0.99994 \nonumber\\
duty_responsibilily & 0.99994 \nonumber\\
than_farquhar & 0.99994 \nonumber\\
sine_he & 0.99994 \nonumber\\
._singapore & 0.99994 \nonumber\\
cockfight_and & 0.99994 \nonumber\\
slave_, & 0.99994 \nonumber\\
allow_slave & 0.99994 \nonumber\\
sine & 0.99994 \nonumber\\
farquhar_and & 0.99994 \nonumber\\
,_cockfight & 0.99994 \nonumber\\
thus_should & 0.99994 \nonumber\\
responsibilily & 0.99994 \nonumber\\
singapore_sine & 0.99994 \nonumber\\
boss_of & 0.99994 \nonumber\\
not_carry & 0.99994 \nonumber\\
develop_that & 0.99994 \nonumber\\
his_duty & 0.99994 \nonumber\\
gay_people & 0.99994 \nonumber\\
_pos_ngram_ADV_PUNC_PUNC & 0.99994 \nonumber\\
order_of & 0.99994 \nonumber\\
support_the & 0.99994 \nonumber\\
far & 0.99994 \nonumber\\
island & 0.99994 \nonumber\\
_pos_ngram_PP_ADV_ART & 0.99994 \nonumber\\
institution_, & 0.99994 \nonumber\\
_pos_ngram_PP_PR_O & 0.99994 \nonumber\\
just_you & 0.99994 \nonumber\\
government & 0.99994 \nonumber\\
._have & 0.99994 \nonumber\\
see_. & 0.99994 \nonumber\\
class_. & 0.99994 \nonumber\\
promote & 0.99994 \nonumber\\
will_never & 0.99994 \nonumber\\
in_rape & 0.99994 \nonumber\\
ProductionRule_VP->VB,PP,ADVP, & 0.99994 \nonumber\\
support_of & 0.99994 \nonumber\\
two_be & 0.99994 \nonumber\\
_pos_ngram_CONJ_NN_ADV & 0.99994 \nonumber\\
ProductionRule_NP->DT,NNPS, & 0.99994 \nonumber\\
200 & 0.99994 \nonumber\\
example_. & 0.99994 \nonumber\\
'_over & 0.99994 \nonumber\\
fatherless_when & 0.99994 \nonumber\\
what_point & 0.99994 \nonumber\\
._father & 0.99994 \nonumber\\
alpha_male & 0.99994 \nonumber\\
ProductionRule_VP->VBG,ADJP,ADVP, & 0.99994 \nonumber\\
alpha & 0.99994 \nonumber\\
fact_of & 0.99994 \nonumber\\
male_but & 0.99994 \nonumber\\
because_his & 0.99994 \nonumber\\
_pos_ngram_PR_ADJ_ADV & 0.99994 \nonumber\\
action_they & 0.99994 \nonumber\\
hand_because & 0.99994 \nonumber\\
look_toward & 0.99994 \nonumber\\
the_provider & 0.99994 \nonumber\\
the_household & 0.99994 \nonumber\\
father_most & 0.99994 \nonumber\\
the_alpha & 0.99994 \nonumber\\
have_responsibility & 0.99994 \nonumber\\
provider_for & 0.99994 \nonumber\\
likely_be & 0.99994 \nonumber\\
household_and & 0.99994 \nonumber\\
responsibility_' & 0.99994 \nonumber\\
have_around & 0.99994 \nonumber\\
household & 0.99994 \nonumber\\
when_have & 0.99994 \nonumber\\
their_father & 0.99994 \nonumber\\
would_support & 0.99994 \nonumber\\
his_like & 0.99994 \nonumber\\
your_father & 0.99994 \nonumber\\
the_crime & 0.99994 \nonumber\\
._then & 0.99994 \nonumber\\
reduce & 0.99994 \nonumber\\
a_disease & 0.99994 \nonumber\\
._of & 0.99994 \nonumber\\
worth & 0.99994 \nonumber\\
right_of & 0.99994 \nonumber\\
_pos_ngram_V_ADJ_CARD & 0.99994 \nonumber\\
water_bottle & 0.99994 \nonumber\\
_pos_ngram_PUNC_CARD & 0.99994 \nonumber\\
quality_of & 0.99994 \nonumber\\
truth & 0.99994 \nonumber\\
_pos_ngram_CONJ_V_ADJ & 0.99994 \nonumber\\
game & 0.99994 \nonumber\\
year_. & 0.99994 \nonumber\\
ProductionRule_VP->VBP,ADJP,SBAR, & 0.99994 \nonumber\\
ProductionRule_VP->VBD,PP, & 0.99994 \nonumber\\
._another & 0.99994 \nonumber\\
resource & 0.99994 \nonumber\\
piss & 0.99994 \nonumber\\
that_way & 0.99994 \nonumber\\
._these & 0.99994 \nonumber\\
to_the & 0.99994 \nonumber\\
defend & 0.99994 \nonumber\\
about_me & 0.99995 \nonumber\\
fine_. & 0.99995 \nonumber\\
imagine & 0.99995 \nonumber\\
ProductionRule_CONJP->RB,IN, & 0.99995 \nonumber\\
first_i & 0.99995 \nonumber\\
imagine_just & 0.99995 \nonumber\\
interview_with & 0.99995 \nonumber\\
,_alabama & 0.99995 \nonumber\\
v._see & 0.99995 \nonumber\\
immediate & 0.99995 \nonumber\\
disaster_in & 0.99995 \nonumber\\
powerful_and & 0.99995 \nonumber\\
just_read & 0.99995 \nonumber\\
much_faster & 0.99995 \nonumber\\
the_recent & 0.99995 \nonumber\\
ProductionRule_NP->DT,CD,NNS, & 0.99995 \nonumber\\
worth_a & 0.99995 \nonumber\\
recent_disaster & 0.99995 \nonumber\\
see_and & 0.99995 \nonumber\\
._tv & 0.99995 \nonumber\\
with_survivor & 0.99995 \nonumber\\
and_missourus & 0.99995 \nonumber\\
and_immediate & 0.99995 \nonumber\\
survivor_. & 0.99995 \nonumber\\
survivor & 0.99995 \nonumber\\
tv_let & 0.99995 \nonumber\\
in_japan & 0.99995 \nonumber\\
and_hear & 0.99995 \nonumber\\
missourus_v. & 0.99995 \nonumber\\
missourus & 0.99995 \nonumber\\
the_info & 0.99995 \nonumber\\
alabama & 0.99995 \nonumber\\
alabama_and & 0.99995 \nonumber\\
or_information & 0.99995 \nonumber\\
see_interview & 0.99995 \nonumber\\
immediate_on & 0.99995 \nonumber\\
hear_a & 0.99995 \nonumber\\
a_thousand & 0.99995 \nonumber\\
a_picture & 0.99995 \nonumber\\
interview & 0.99995 \nonumber\\
picture_be & 0.99995 \nonumber\\
info & 0.99995 \nonumber\\
info_much & 0.99995 \nonumber\\
_pos_ngram_ADJ_ART_CARD & 0.99995 \nonumber\\
tv_give & 0.99995 \nonumber\\
thousand_word & 0.99995 \nonumber\\
western & 0.99995 \nonumber\\
aid & 0.99995 \nonumber\\
why_ca & 0.99995 \nonumber\\
lousy_then & 0.99995 \nonumber\\
your_a & 0.99995 \nonumber\\
n't_hold & 0.99995 \nonumber\\
that_come & 0.99995 \nonumber\\
_pos_ngram_O_PR_PP & 0.99995 \nonumber\\
cold & 0.99995 \nonumber\\
_pos_ngram_NP_CONJ_PR & 0.99995 \nonumber\\
weather & 0.99995 \nonumber\\
weather_it & 0.99995 \nonumber\\
father_, & 0.99995 \nonumber\\
when_people & 0.99995 \nonumber\\
anything_and & 0.99995 \nonumber\\
leave & 0.99995 \nonumber\\
plant & 0.99995 \nonumber\\
take_care & 0.99995 \nonumber\\
care_of & 0.99995 \nonumber\\
n't_help & 0.99995 \nonumber\\
n't_care & 0.99995 \nonumber\\
:_/ & 0.99995 \nonumber\\
wish_there & 0.99995 \nonumber\\
or_any & 0.99995 \nonumber\\
turn_it & 0.99995 \nonumber\\
to_bencoolen & 0.99995 \nonumber\\
cant_help & 0.99995 \nonumber\\
plz & 0.99995 \nonumber\\
request & 0.99995 \nonumber\\
when_i & 0.99995 \nonumber\\
god_be & 0.99995 \nonumber\\
thus & 0.99995 \nonumber\\
but_never & 0.99995 \nonumber\\
close_the & 0.99995 \nonumber\\
the_key & 0.99995 \nonumber\\
_pos_ngram_PR_O_ADV & 0.99995 \nonumber\\
oneself.i_need & 0.99995 \nonumber\\
ourself & 0.99995 \nonumber\\
before_think & 0.99995 \nonumber\\
oneself.i & 0.99995 \nonumber\\
ourself_first & 0.99995 \nonumber\\
human_nature.but & 0.99995 \nonumber\\
about_oneself.i & 0.99995 \nonumber\\
themselve_before & 0.99995 \nonumber\\
,_success & 0.99995 \nonumber\\
nature.but_personal & 0.99995 \nonumber\\
happy_to & 0.99995 \nonumber\\
me_happy & 0.99995 \nonumber\\
then_think & 0.99995 \nonumber\\
everyone_do & 0.99995 \nonumber\\
of_ourself & 0.99995 \nonumber\\
better_and & 0.99995 \nonumber\\
life_better & 0.99995 \nonumber\\
other_happy & 0.99995 \nonumber\\
be_who & 0.99995 \nonumber\\
persuit_because & 0.99995 \nonumber\\
nature.but & 0.99995 \nonumber\\
me_first & 0.99995 \nonumber\\
with_personal & 0.99995 \nonumber\\
,_raffle & 0.99995 \nonumber\\
construction & 0.99995 \nonumber\\
take_too & 0.99995 \nonumber\\
per & 0.99995 \nonumber\\
they_decide & 0.99995 \nonumber\\
be_very & 0.99995 \nonumber\\
join & 0.99995 \nonumber\\
there_' & 0.99995 \nonumber\\
leave_singapore & 0.99995 \nonumber\\
not_bid & 0.99995 \nonumber\\
ProductionRule_NP->DT,NNS,POS, & 0.99995 \nonumber\\
ProductionRule_VP->VBZ,RB, & 0.99995 \nonumber\\
that_feel & 0.99995 \nonumber\\
ProductionRule_NP->DT,NN,., & 0.99995 \nonumber\\
might_be & 0.99995 \nonumber\\
return & 0.99995 \nonumber\\
ProductionRule_NP->NP,CC,ADVP,NP, & 0.99995 \nonumber\\
people_' & 0.99995 \nonumber\\
problem_that & 0.99995 \nonumber\\
about_yourself & 0.99995 \nonumber\\
someone_then & 0.99995 \nonumber\\
PastVerbRatio & 0.99995 \nonumber\\
arguement & 0.99995 \nonumber\\
claim_. & 0.99995 \nonumber\\
7 & 0.99995 \nonumber\\
say_what & 0.99995 \nonumber\\
nothing_to & 0.99995 \nonumber\\
do_we & 0.99995 \nonumber\\
_pos_ngram_PUNC_O_O & 0.99995 \nonumber\\
thing_. & 0.99995 \nonumber\\
opinion_. & 0.99995 \nonumber\\
while_it & 0.99995 \nonumber\\
good_, & 0.99995 \nonumber\\
ProductionRule_NP->CD,NNS, & 0.99995 \nonumber\\
bear & 0.99995 \nonumber\\
_pos_ngram_NP_V_PUNC & 0.99995 \nonumber\\
go_and & 0.99995 \nonumber\\
up_with & 0.99995 \nonumber\\
tourism & 0.99995 \nonumber\\
_pos_ngram_NN_O_CONJ & 0.99995 \nonumber\\
be_marry & 0.99995 \nonumber\\
useless & 0.99995 \nonumber\\
that_this & 0.99995 \nonumber\\
rate & 0.99995 \nonumber\\
actually_be & 0.99995 \nonumber\\
make_your & 0.99995 \nonumber\\
chance_of & 0.99995 \nonumber\\
never_get & 0.99995 \nonumber\\
a_new & 0.99995 \nonumber\\
faith_to & 0.99995 \nonumber\\
problem_for & 0.99995 \nonumber\\
tv_. & 0.99995 \nonumber\\
disease & 0.99995 \nonumber\\
near & 0.99995 \nonumber\\
n't_live & 0.99995 \nonumber\\
anybody & 0.99995 \nonumber\\
moon & 0.99995 \nonumber\\
who_have & 0.99995 \nonumber\\
the_action & 0.99995 \nonumber\\
numerous & 0.99995 \nonumber\\
traumatize & 0.99995 \nonumber\\
old & 0.99995 \nonumber\\
not_mean & 0.99995 \nonumber\\
local & 0.99995 \nonumber\\
nor & 0.99995 \nonumber\\
,_terrorism & 0.99995 \nonumber\\
terrorism & 0.99995 \nonumber\\
wonderful & 0.99995 \nonumber\\
she_kill & 0.99995 \nonumber\\
spank_a & 0.99995 \nonumber\\
before_we & 0.99995 \nonumber\\
western_europe & 0.99995 \nonumber\\
wait_and & 0.99995 \nonumber\\
cant_prove & 0.99995 \nonumber\\
sultan & 0.99995 \nonumber\\
spank_, & 0.99995 \nonumber\\
_pos_ngram_NP_PUNC_NN & 0.99995 \nonumber\\
_pos_ngram_PP_PR_PR & 0.99995 \nonumber\\
solid & 0.99995 \nonumber\\
ProductionRule_VP->VB,PP,PP, & 0.99995 \nonumber\\
evolution_. & 0.99995 \nonumber\\
christianity_be & 0.99995 \nonumber\\
....._. & 0.99995 \nonumber\\
not_believe & 0.99995 \nonumber\\
planet & 0.99995 \nonumber\\
hus & 0.99995 \nonumber\\
ban & 0.99995 \nonumber\\
_pos_ngram_PP_NP_ART & 0.99995 \nonumber\\
so_a & 0.99995 \nonumber\\
it_in & 0.99995 \nonumber\\
_pos_ngram_NP_ART_V & 0.99995 \nonumber\\
weak & 0.99995 \nonumber\\
or_wrong & 0.99995 \nonumber\\
right_or & 0.99995 \nonumber\\
virgin & 0.99995 \nonumber\\
_pos_ngram_V_ADV_CARD & 0.99995 \nonumber\\
reason_that & 0.99995 \nonumber\\
very_much & 0.99995 \nonumber\\
me_soon & 0.99995 \nonumber\\
syona & 0.99995 \nonumber\\
and_he & 0.99995 \nonumber\\
not_that & 0.99995 \nonumber\\
at_my & 0.99995 \nonumber\\
kid_because & 0.99995 \nonumber\\
_pos_ngram_ADJ_V_PP & 0.99995 \nonumber\\
them_for & 0.99995 \nonumber\\
act_like & 0.99995 \nonumber\\
....._he & 0.99995 \nonumber\\
question_me & 0.99995 \nonumber\\
down_for & 0.99995 \nonumber\\
reason_plus & 0.99995 \nonumber\\
be_safe & 0.99995 \nonumber\\
about_anything & 0.99995 \nonumber\\
let_him & 0.99995 \nonumber\\
plus_his & 0.99995 \nonumber\\
me_... & 0.99995 \nonumber\\
anything_i & 0.99995 \nonumber\\
on_him & 0.99995 \nonumber\\
tell_on & 0.99995 \nonumber\\
come_question & 0.99995 \nonumber\\
him_down & 0.99995 \nonumber\\
for_self & 0.99995 \nonumber\\
secret_be & 0.99995 \nonumber\\
nothing_..... & 0.99995 \nonumber\\
my_trust & 0.99995 \nonumber\\
n't_let & 0.99995 \nonumber\\
reason_might & 0.99995 \nonumber\\
his_secret & 0.99995 \nonumber\\
safe_with & 0.99995 \nonumber\\
trust_and & 0.99995 \nonumber\\
ProductionRule_S->SBAR,S,CC,S, & 0.99995 \nonumber\\
you_love & 0.99995 \nonumber\\
_pos_ngram_ADJ_PP_PP & 0.99995 \nonumber\\
half & 0.99995 \nonumber\\
of_our & 0.99995 \nonumber\\
ProductionRule_VP->VP,,,NP, & 0.99995 \nonumber\\
rights_to & 0.99995 \nonumber\\
him_be & 0.99995 \nonumber\\
or_help & 0.99995 \nonumber\\
specific & 0.99995 \nonumber\\
i_must & 0.99995 \nonumber\\
% & 0.99995 \nonumber\\
build & 0.99995 \nonumber\\
_pos_ngram_ADV_PR_ADJ & 0.99995 \nonumber\\
pornography & 0.99995 \nonumber\\
so_, & 0.99995 \nonumber\\
ProductionRule_VP->VBP,ADVP, & 0.99995 \nonumber\\
then_what & 0.99995 \nonumber\\
just_a & 0.99995 \nonumber\\
now_i & 0.99995 \nonumber\\
live_, & 0.99995 \nonumber\\
you_because & 0.99995 \nonumber\\
the_porn & 0.99995 \nonumber\\
sex_. & 0.99995 \nonumber\\
a_fatherless & 0.99995 \nonumber\\
gender_either & 0.99995 \nonumber\\
culture_disallow & 0.99995 \nonumber\\
religion_or & 0.99995 \nonumber\\
culture_? & 0.99995 \nonumber\\
affect_your & 0.99995 \nonumber\\
either_, & 0.99995 \nonumber\\
,_lifestyle & 0.99995 \nonumber\\
your_marriage & 0.99995 \nonumber\\
same_gender & 0.99995 \nonumber\\
extend_to & 0.99995 \nonumber\\
people_marry & 0.99995 \nonumber\\
extend & 0.99995 \nonumber\\
it_extend & 0.99995 \nonumber\\
disallow & 0.99995 \nonumber\\
person_of & 0.99995 \nonumber\\
or_culture & 0.99995 \nonumber\\
should_it & 0.99995 \nonumber\\
disallow_gay & 0.99995 \nonumber\\
lifestyle_etc & 0.99995 \nonumber\\
way_affect & 0.99995 \nonumber\\
?_gay & 0.99995 \nonumber\\
they_simply & 0.99995 \nonumber\\
etc_be & 0.99995 \nonumber\\
marriage_to & 0.99995 \nonumber\\
marry_a & 0.99995 \nonumber\\
simply_get & 0.99995 \nonumber\\
_pos_ngram_PR_NP_NN & 0.99995 \nonumber\\
should_pay & 0.99995 \nonumber\\
_pos_ngram_PUNC_PUNC & 0.99995 \nonumber\\
,_someone & 0.99995 \nonumber\\
_pos_ngram_NN_V_NP & 0.99995 \nonumber\\
of_themselve & 0.99995 \nonumber\\
_pos_ngram_PP_ADJ_ADJ & 0.99995 \nonumber\\
_pos_ngram_V_CONJ_ADJ & 0.99995 \nonumber\\
man_' & 0.99995 \nonumber\\
kill_that & 0.99995 \nonumber\\
call_the & 0.99995 \nonumber\\
rid & 0.99995 \nonumber\\
_pos_ngram_PUNC_O_ADJ & 0.99995 \nonumber\\
whether & 0.99995 \nonumber\\
not_everyone & 0.99995 \nonumber\\
n't_use & 0.99995 \nonumber\\
design & 0.99995 \nonumber\\
can_bring & 0.99995 \nonumber\\
fatherless_because & 0.99995 \nonumber\\
equal & 0.99995 \nonumber\\
thing_it & 0.99995 \nonumber\\
ProductionRule_SBAR->ADVP,WHADVP,S, & 0.99995 \nonumber\\
they_think & 0.99995 \nonumber\\
not_argue & 0.99995 \nonumber\\
ProductionRule_ADJP->FW,FW, & 0.99995 \nonumber\\
because_we & 0.99995 \nonumber\\
world_' & 0.99995 \nonumber\\
his & 0.99995 \nonumber\\
those_who & 0.99995 \nonumber\\
father_i & 0.99995 \nonumber\\
person_in & 0.99995 \nonumber\\
fast & 0.99995 \nonumber\\
a_person & 0.99995 \nonumber\\
be_an & 0.99995 \nonumber\\
one_reason & 0.99995 \nonumber\\
'_impossible & 0.99995 \nonumber\\
load_of & 0.99995 \nonumber\\
be_difficult & 0.99995 \nonumber\\
scientific_evidence & 0.99995 \nonumber\\
n't_believe & 0.99995 \nonumber\\
in_favor & 0.99995 \nonumber\\
favor_of & 0.99995 \nonumber\\
option_. & 0.99995 \nonumber\\
EndingOus & 0.99995 \nonumber\\
be_right & 0.99995 \nonumber\\
her_child & 0.99995 \nonumber\\
and_moon & 0.99995 \nonumber\\
image_. & 0.99995 \nonumber\\
ever_see & 0.99995 \nonumber\\
debate_i & 0.99995 \nonumber\\
distinctively & 0.99995 \nonumber\\
moon_be & 0.99995 \nonumber\\
me_please & 0.99995 \nonumber\\
so_perfect & 0.99995 \nonumber\\
and_sun & 0.99995 \nonumber\\
cause_we & 0.99995 \nonumber\\
after_his & 0.99995 \nonumber\\
idiotic_debate & 0.99995 \nonumber\\
spot & 0.99995 \nonumber\\
spot_and & 0.99995 \nonumber\\
most_idiotic & 0.99995 \nonumber\\
hoe & 0.99995 \nonumber\\
please_hoe & 0.99995 \nonumber\\
perfectly_be & 0.99995 \nonumber\\
function & 0.99995 \nonumber\\
make_after & 0.99995 \nonumber\\
perfect_be & 0.99995 \nonumber\\
right_spot & 0.99995 \nonumber\\
function_perfectly & 0.99995 \nonumber\\
hand_make & 0.99995 \nonumber\\
._cause & 0.99995 \nonumber\\
body_function & 0.99995 \nonumber\\
distinctively_. & 0.99995 \nonumber\\
own_image & 0.99995 \nonumber\\
be_body & 0.99995 \nonumber\\
hoe_do & 0.99995 \nonumber\\
make_distinctively & 0.99995 \nonumber\\
sun_and & 0.99995 \nonumber\\
be_evolution & 0.99995 \nonumber\\
ProductionRule_ADVP->NP,JJR, & 0.99995 \nonumber\\
go_around & 0.99995 \nonumber\\
all_we & 0.99995 \nonumber\\
because_spank & 0.99995 \nonumber\\
be_help & 0.99995 \nonumber\\
for_all & 0.99995 \nonumber\\
also_help & 0.99995 \nonumber\\
question_of & 0.99995 \nonumber\\
EndingLess & 0.99995 \nonumber\\
ProductionRule_S->S,,,S,., & 0.99995 \nonumber\\
opponent_have & 0.99995 \nonumber\\
argument_any & 0.99995 \nonumber\\
be_accept & 0.99995 \nonumber\\
earth_and & 0.99995 \nonumber\\
when & 0.99995 \nonumber\\
it_look & 0.99995 \nonumber\\
over_again & 0.99995 \nonumber\\
then_you & 0.99995 \nonumber\\
ProductionRule_NP->NNP,NN, & 0.99995 \nonumber\\
image & 0.99995 \nonumber\\
japan & 0.99995 \nonumber\\
japan_, & 0.99995 \nonumber\\
have_her & 0.99995 \nonumber\\
ProductionRule_S->NP,NP, & 0.99995 \nonumber\\
choice_be & 0.99995 \nonumber\\
ProductionRule_VP->JJ,NP, & 0.99995 \nonumber\\
'_fine & 0.99995 \nonumber\\
skill & 0.99995 \nonumber\\
_ & 0.99995 \nonumber\\
__sex & 0.99995 \nonumber\\
spread_aid & 0.99995 \nonumber\\
__be & 0.99995 \nonumber\\
sex__ & 0.99995 \nonumber\\
aid_? & 0.99995 \nonumber\\
help_reduce & 0.99995 \nonumber\\
gay__ & 0.99995 \nonumber\\
help_spread & 0.99995 \nonumber\\
marriage_may & 0.99995 \nonumber\\
which_case & 0.99995 \nonumber\\
_pos_ngram_V_PR_O & 0.99995 \nonumber\\
will_. & 0.99995 \nonumber\\
people_come & 0.99995 \nonumber\\
notice_that & 0.99995 \nonumber\\
have_see & 0.99995 \nonumber\\
the_relationship & 0.99995 \nonumber\\
water_when & 0.99995 \nonumber\\
be_unable & 0.99995 \nonumber\\
unable_to & 0.99995 \nonumber\\
unable & 0.99995 \nonumber\\
abt_. & 0.99995 \nonumber\\
abt & 0.99995 \nonumber\\
n't_have & 0.99995 \nonumber\\
faster_. & 0.99995 \nonumber\\
sex_with & 0.99995 \nonumber\\
great & 0.99995 \nonumber\\
,_that & 0.99995 \nonumber\\
better_. & 0.99995 \nonumber\\
"_- & 0.99995 \nonumber\\
it_might & 0.99995 \nonumber\\
can_also & 0.99995 \nonumber\\
improve_your & 0.99995 \nonumber\\
ProductionRule_VP->VB,NP,S, & 0.99995 \nonumber\\
you_need & 0.99995 \nonumber\\
,_so & 0.99995 \nonumber\\
not_good & 0.99995 \nonumber\\
animal_, & 0.99995 \nonumber\\
ProductionRule_NP->DT,NN,S, & 0.99995 \nonumber\\
country_with & 0.99995 \nonumber\\
life_he & 0.99995 \nonumber\\
be_wear & 0.99995 \nonumber\\
and_watch & 0.99995 \nonumber\\
people_think & 0.99995 \nonumber\\
-_can & 0.99995 \nonumber\\
fact_- & 0.99995 \nonumber\\
point_me & 0.99995 \nonumber\\
know_fact & 0.99995 \nonumber\\
a_reference & 0.99995 \nonumber\\
ProductionRule_ADJP->RB,VBN, & 0.99995 \nonumber\\
reference & 0.99995 \nonumber\\
reference_? & 0.99995 \nonumber\\
commonly_know & 0.99995 \nonumber\\
ProductionRule_S->S,:,SQ,., & 0.99995 \nonumber\\
someone_else & 0.99995 \nonumber\\
last_option & 0.99995 \nonumber\\
one_who & 0.99995 \nonumber\\
deserve & 0.99995 \nonumber\\
your_self & 0.99995 \nonumber\\
stage_of & 0.99995 \nonumber\\
stage & 0.99995 \nonumber\\
totally_obvious & 0.99995 \nonumber\\
ProductionRule_S->IN,NP,VP,., & 0.99995 \nonumber\\
assume_have & 0.99995 \nonumber\\
other_involve & 0.99995 \nonumber\\
ProductionRule_NP->NNS,SBAR, & 0.99995 \nonumber\\
ProductionRule_VP->ADVP,VBN,PRT,PP, & 0.99995 \nonumber\\
obvious_, & 0.99995 \nonumber\\
would_assume & 0.99995 \nonumber\\
thoroughly & 0.99995 \nonumber\\
and_which & 0.99995 \nonumber\\
thoroughly_flesh & 0.99995 \nonumber\\
flesh_out & 0.99995 \nonumber\\
be_thoroughly & 0.99995 \nonumber\\
flesh & 0.99995 \nonumber\\
male & 0.99995 \nonumber\\
government_have & 0.99995 \nonumber\\
_pos_ngram_PUNC_NN_PR & 0.99995 \nonumber\\
say_book & 0.99995 \nonumber\\
not_around & 0.99995 \nonumber\\
feel_unlove & 0.99995 \nonumber\\
self_of & 0.99995 \nonumber\\
traumatize_and & 0.99995 \nonumber\\
low_self & 0.99995 \nonumber\\
lot_, & 0.99995 \nonumber\\
logically_. & 0.99995 \nonumber\\
logically & 0.99995 \nonumber\\
unlove & 0.99995 \nonumber\\
unlove_since & 0.99995 \nonumber\\
option_because & 0.99995 \nonumber\\
think_logically & 0.99995 \nonumber\\
also_spank & 0.99995 \nonumber\\
esteem & 0.99995 \nonumber\\
full_with & 0.99995 \nonumber\\
up_traumatize & 0.99995 \nonumber\\
moment_the & 0.99995 \nonumber\\
of_esteem & 0.99995 \nonumber\\
esteem_. & 0.99995 \nonumber\\
with_anger & 0.99995 \nonumber\\
around_you & 0.99995 \nonumber\\
the_internet & 0.99995 \nonumber\\
responsibility & 0.99995 \nonumber\\
later_on & 0.99995 \nonumber\\
continue_to & 0.99995 \nonumber\\
bid_at & 0.99995 \nonumber\\
go_hand & 0.99995 \nonumber\\
hand_in & 0.99995 \nonumber\\
just_get & 0.99995 \nonumber\\
to_focus & 0.99995 \nonumber\\
on_yourself & 0.99995 \nonumber\\
have_turn & 0.99995 \nonumber\\
it_so & 0.99995 \nonumber\\
have_legalize & 0.99995 \nonumber\\
singapore_can & 0.99995 \nonumber\\
can_prosper & 0.99995 \nonumber\\
singapore_alone & 0.99995 \nonumber\\
ProductionRule_S->SBAR,,,S,,,CC,S,., & 0.99995 \nonumber\\
ProductionRule_VP->VBN,NP,ADVP,,,S, & 0.99995 \nonumber\\
prosper & 0.99995 \nonumber\\
gamble_, & 0.99995 \nonumber\\
down_, & 0.99995 \nonumber\\
legalize_gamble & 0.99995 \nonumber\\
prosper_, & 0.99995 \nonumber\\
_pos_ngram_NN_ADJ_PR & 0.99995 \nonumber\\
rights_of & 0.99995 \nonumber\\
ProductionRule_NP->DT,JJ,NNP, & 0.99995 \nonumber\\
& & 0.99995 \nonumber\\
and_clean & 0.99995 \nonumber\\
clean_house & 0.99995 \nonumber\\
old_to & 0.99995 \nonumber\\
specify_who & 0.99995 \nonumber\\
too_old & 0.99995 \nonumber\\
maybe_she & 0.99995 \nonumber\\
cook & 0.99995 \nonumber\\
kill_or & 0.99995 \nonumber\\
cook_and & 0.99995 \nonumber\\
?_; & 0.99995 \nonumber\\
scene_all & 0.99995 \nonumber\\
or_why & 0.99995 \nonumber\\
everyone_deserve & 0.99995 \nonumber\\
date_scene & 0.99995 \nonumber\\
na_have & 0.99995 \nonumber\\
ProductionRule_SBAR->ADVP,WHNP,S,., & 0.99995 \nonumber\\
her_reason & 0.99995 \nonumber\\
'_gon & 0.99995 \nonumber\\
'_go & 0.99995 \nonumber\\
house_? & 0.99995 \nonumber\\
to_cook & 0.99995 \nonumber\\
n't_specify & 0.99995 \nonumber\\
live_the & 0.99995 \nonumber\\
liberal & 0.99995 \nonumber\\
look_and & 0.99995 \nonumber\\
or_what & 0.99995 \nonumber\\
atheist & 0.99995 \nonumber\\
_pos_ngram_PP_PUNC_ART & 0.99995 \nonumber\\
be_rape & 0.99995 \nonumber\\
possible_. & 0.99995 \nonumber\\
in_which & 0.99995 \nonumber\\
believe_abortion & 0.99995 \nonumber\\
ProductionRule_S->ADVP,,,NP,VP,., & 0.99995 \nonumber\\
then_it & 0.99995 \nonumber\\
_pos_ngram_ART_ADJ_NP & 0.99995 \nonumber\\
bid_. & 0.99995 \nonumber\\
and_it & 0.99995 \nonumber\\
ProductionRule_PP->VBG,PP, & 0.99995 \nonumber\\
buy & 0.99995 \nonumber\\
continue & 0.99995 \nonumber\\
damage & 0.99995 \nonumber\\
moral & 0.99995 \nonumber\\
might_feel & 0.99995 \nonumber\\
often & 0.99995 \nonumber\\
totally & 0.99995 \nonumber\\
be_totally & 0.99995 \nonumber\\
_pos_ngram_PP_NP_O & 0.99995 \nonumber\\
ProductionRule_VP->VB,NP,PP,PP, & 0.99995 \nonumber\\
for_an & 0.99995 \nonumber\\
ourselve & 0.99995 \nonumber\\
ProductionRule_NP->NN,JJ,NN, & 0.99995 \nonumber\\
talk_to & 0.99995 \nonumber\\
_pos_ngram_ADV_NP_NP & 0.99995 \nonumber\\
that_moment & 0.99995 \nonumber\\
them_think & 0.99995 \nonumber\\
people_may & 0.99995 \nonumber\\
as_" & 0.99995 \nonumber\\
out_by & 0.99995 \nonumber\\
she_commit & 0.99995 \nonumber\\
development_. & 0.99995 \nonumber\\
because_your & 0.99995 \nonumber\\
a_mere & 0.99995 \nonumber\\
mere & 0.99995 \nonumber\\
them_. & 0.99995 \nonumber\\
ProductionRule_VP->VB,CC,VB,NP, & 0.99995 \nonumber\\
him_because & 0.99995 \nonumber\\
to_solve & 0.99995 \nonumber\\
or_whatever & 0.99995 \nonumber\\
my_word & 0.99995 \nonumber\\
be_pretty & 0.99995 \nonumber\\
so_they & 0.99995 \nonumber\\
strengthen & 0.99995 \nonumber\\
only_have & 0.99995 \nonumber\\
could_have & 0.99995 \nonumber\\
since_they & 0.99995 \nonumber\\
student_of & 0.99995 \nonumber\\
_pos_ngram_ADJ_PP_ADV & 0.99995 \nonumber\\
yes_. & 0.99995 \nonumber\\
get_so & 0.99995 \nonumber\\
period & 0.99995 \nonumber\\
first_thing & 0.99995 \nonumber\\
confidence & 0.99996 \nonumber\\
about_you & 0.99996 \nonumber\\
because_most & 0.99996 \nonumber\\
husband & 0.99996 \nonumber\\
ProductionRule_PP->IN,IN,NP, & 0.99996 \nonumber\\
spouse_. & 0.99996 \nonumber\\
so_we & 0.99996 \nonumber\\
turn_out & 0.99996 \nonumber\\
by_other & 0.99996 \nonumber\\
go_through & 0.99996 \nonumber\\
_pos_ngram_O_PUNC_O & 0.99996 \nonumber\\
for_no & 0.99996 \nonumber\\
in_reality & 0.99996 \nonumber\\
homosexual & 0.99996 \nonumber\\
have_more & 0.99996 \nonumber\\
the_rights & 0.99996 \nonumber\\
happen_, & 0.99996 \nonumber\\
better_person & 0.99996 \nonumber\\
much_time & 0.99996 \nonumber\\
to_make & 0.99996 \nonumber\\
part_in & 0.99996 \nonumber\\
really_be & 0.99996 \nonumber\\
tv_you & 0.99996 \nonumber\\
over_the & 0.99996 \nonumber\\
because_how & 0.99996 \nonumber\\
necessary & 0.99996 \nonumber\\
the_difference & 0.99996 \nonumber\\
motivate_you & 0.99996 \nonumber\\
motivate & 0.99996 \nonumber\\
lower & 0.99996 \nonumber\\
in_every & 0.99996 \nonumber\\
that_all & 0.99996 \nonumber\\
,_be & 0.99996 \nonumber\\
occur & 0.99996 \nonumber\\
_pos_ngram_ADV_NN_PP & 0.99996 \nonumber\\
then_the & 0.99996 \nonumber\\
problem_. & 0.99996 \nonumber\\
father_that & 0.99996 \nonumber\\
ProductionRule_S->S,,,NP,VP,., & 0.99996 \nonumber\\
it_and & 0.99996 \nonumber\\
its_more & 0.99996 \nonumber\\
addition_, & 0.99996 \nonumber\\
express_their & 0.99996 \nonumber\\
district & 0.99996 \nonumber\\
school_district & 0.99996 \nonumber\\
as_he & 0.99996 \nonumber\\
earth & 0.99996 \nonumber\\
father_at & 0.99996 \nonumber\\
(_or & 0.99996 \nonumber\\
but_not & 0.99996 \nonumber\\
work_. & 0.99996 \nonumber\\
billion_of & 0.99996 \nonumber\\
as_possible & 0.99996 \nonumber\\
of_it & 0.99996 \nonumber\\
lot_more & 0.99996 \nonumber\\
match & 0.99996 \nonumber\\
the_feeling & 0.99996 \nonumber\\
be_worry & 0.99996 \nonumber\\
conscious_animal & 0.99996 \nonumber\\
about_protect & 0.99996 \nonumber\\
pregnancy_, & 0.99996 \nonumber\\
as_fully-develop & 0.99996 \nonumber\\
child_within & 0.99996 \nonumber\\
confuse_about & 0.99996 \nonumber\\
ProductionRule_ADJP->RB,RBR,JJ, & 0.99996 \nonumber\\
should_first & 0.99996 \nonumber\\
pro-life_point & 0.99996 \nonumber\\
of_pregnancy & 0.99996 \nonumber\\
its_be & 0.99996 \nonumber\\
primate_. & 0.99996 \nonumber\\
of_far & 0.99996 \nonumber\\
more_conscious & 0.99996 \nonumber\\
their_feeling & 0.99996 \nonumber\\
confuse & 0.99996 \nonumber\\
fully-develop & 0.99996 \nonumber\\
fully-develop_primate & 0.99996 \nonumber\\
surely_if & 0.99996 \nonumber\\
first_few & 0.99996 \nonumber\\
primate & 0.99996 \nonumber\\
feeling_of & 0.99996 \nonumber\\
month_of & 0.99996 \nonumber\\
feeling_we & 0.99996 \nonumber\\
guess_i & 0.99996 \nonumber\\
ProductionRule_FRAG->ADVP,SBAR,., & 0.99996 \nonumber\\
n't_their & 0.99996 \nonumber\\
very_confuse & 0.99996 \nonumber\\
of_unborn & 0.99996 \nonumber\\
conscious & 0.99996 \nonumber\\
few_month & 0.99996 \nonumber\\
first_be & 0.99996 \nonumber\\
should_stop & 0.99996 \nonumber\\
tell_us & 0.99996 \nonumber\\
believe_. & 0.99996 \nonumber\\
least_in & 0.99996 \nonumber\\
_pos_ngram_V_O_NN & 0.99996 \nonumber\\
first_, & 0.99996 \nonumber\\
least_a & 0.99996 \nonumber\\
favorite & 0.99996 \nonumber\\
you_kill & 0.99996 \nonumber\\
that_child & 0.99996 \nonumber\\
way_of & 0.99996 \nonumber\\
be_bear & 0.99996 \nonumber\\
put_on & 0.99996 \nonumber\\
ProductionRule_ADJP->RB,JJ,SBAR, & 0.99996 \nonumber\\
do_what & 0.99996 \nonumber\\
ProductionRule_ADJP->JJ,CC,JJ, & 0.99996 \nonumber\\
create_an & 0.99996 \nonumber\\
huge & 0.99996 \nonumber\\
so_what & 0.99996 \nonumber\\
._now & 0.99996 \nonumber\\
life_would & 0.99996 \nonumber\\
,_accord & 0.99996 \nonumber\\
it_up & 0.99996 \nonumber\\
but_then & 0.99996 \nonumber\\
im & 0.99996 \nonumber\\
and_actually & 0.99996 \nonumber\\
no_because & 0.99996 \nonumber\\
ProductionRule_S->SBAR,,,NP,ADVP,VP,., & 0.99996 \nonumber\\
for_normal & 0.99996 \nonumber\\
marriage_life & 0.99996 \nonumber\\
terrible_mistake & 0.99996 \nonumber\\
lot_better & 0.99996 \nonumber\\
commit_to & 0.99996 \nonumber\\
now_with & 0.99996 \nonumber\\
whole_lot & 0.99996 \nonumber\\
normal_marriage & 0.99996 \nonumber\\
promise & 0.99996 \nonumber\\
life_right & 0.99996 \nonumber\\
or_to & 0.99996 \nonumber\\
if_its & 0.99996 \nonumber\\
big_bang & 0.99996 \nonumber\\
bang & 0.99996 \nonumber\\
if_someone & 0.99996 \nonumber\\
the_pro-life & 0.99996 \nonumber\\
_pos_ngram_NN_ADV_NP & 0.99996 \nonumber\\
and_say & 0.99996 \nonumber\\
age & 0.99996 \nonumber\\
knowledge_people & 0.99996 \nonumber\\
too_curious & 0.99996 \nonumber\\
never_meet & 0.99996 \nonumber\\
than_know & 0.99996 \nonumber\\
could_of & 0.99996 \nonumber\\
my_knowledge & 0.99996 \nonumber\\
that_my & 0.99996 \nonumber\\
the_hope & 0.99996 \nonumber\\
meet_him & 0.99996 \nonumber\\
curious_as & 0.99996 \nonumber\\
,_in & 0.99996 \nonumber\\
get_an & 0.99996 \nonumber\\
into_an & 0.99996 \nonumber\\
place_. & 0.99996 \nonumber\\
the_fear & 0.99996 \nonumber\\
sentence & 0.99996 \nonumber\\
in_prison & 0.99996 \nonumber\\
therefore & 0.99996 \nonumber\\
state & 0.99996 \nonumber\\
ModalVerbMight & 0.99996 \nonumber\\
personally_how & 0.99996 \nonumber\\
say_advance & 0.99996 \nonumber\\
you_personally & 0.99996 \nonumber\\
cant_focus & 0.99996 \nonumber\\
ProductionRule_S->NP,ADVP,NP,VP, & 0.99996 \nonumber\\
you_focus & 0.99996 \nonumber\\
focus_or & 0.99996 \nonumber\\
mom & 0.99996 \nonumber\\
weight_and & 0.99996 \nonumber\\
._many & 0.99996 \nonumber\\
_pos_ngram_ART_PP_O & 0.99996 \nonumber\\
anger & 0.99996 \nonumber\\
anger_and & 0.99996 \nonumber\\
_pos_ngram_ADJ_ADJ_PUNC & 0.99996 \nonumber\\
ProductionRule_SBAR->SBAR,CC,SBAR, & 0.99996 \nonumber\\
he_care & 0.99996 \nonumber\\
and_concept & 0.99996 \nonumber\\
_pos_ngram_CONJ_NN_NP & 0.99996 \nonumber\\
concept_farquhar & 0.99996 \nonumber\\
he_change & 0.99996 \nonumber\\
back_after & 0.99996 \nonumber\\
rule_and & 0.99996 \nonumber\\
change_rule & 0.99996 \nonumber\\
set_accord & 0.99996 \nonumber\\
have_set & 0.99996 \nonumber\\
sometime & 0.99996 \nonumber\\
one_you & 0.99996 \nonumber\\
read_about & 0.99996 \nonumber\\
force & 0.99996 \nonumber\\
by_this & 0.99996 \nonumber\\
it_help & 0.99996 \nonumber\\
_pos_ngram_PR_PP_CONJ & 0.99996 \nonumber\\
human_have & 0.99996 \nonumber\\
consume & 0.99996 \nonumber\\
_pos_ngram_ART_ADV_PP & 0.99996 \nonumber\\
_pos_ngram_ART_PP_ADJ & 0.99996 \nonumber\\
a_huge & 0.99996 \nonumber\\
ProductionRule_PRN->,,S,,, & 0.99996 \nonumber\\
ProductionRule_VP->VB,NP,PRT,PP, & 0.99996 \nonumber\\
and_kill & 0.99996 \nonumber\\
_pos_ngram_O_CARD_PUNC & 0.99996 \nonumber\\
the_body & 0.99996 \nonumber\\
_pos_ngram_ART_ADV_PR & 0.99996 \nonumber\\
._marriage & 0.99996 \nonumber\\
that_time & 0.99996 \nonumber\\
_pos_ngram_PP_CARD_ADJ & 0.99996 \nonumber\\
ie7 & 0.99996 \nonumber\\
importance & 0.99996 \nonumber\\
christian_be & 0.99996 \nonumber\\
ProductionRule_VP->VBP,ADJP,,,SBAR, & 0.99996 \nonumber\\
ProductionRule_INTJ->UH,., & 0.99996 \nonumber\\
'_more & 0.99996 \nonumber\\
water_every & 0.99996 \nonumber\\
some_evidence & 0.99996 \nonumber\\
share & 0.99996 \nonumber\\
warning_or & 0.99996 \nonumber\\
emergency_warning & 0.99996 \nonumber\\
fit_all & 0.99996 \nonumber\\
without_tv & 0.99996 \nonumber\\
the_newspaper & 0.99996 \nonumber\\
and_newspaper & 0.99996 \nonumber\\
actors/actresses & 0.99996 \nonumber\\
actors/actresses_would & 0.99996 \nonumber\\
have_job & 0.99996 \nonumber\\
newspaper & 0.99996 \nonumber\\
you_emergency & 0.99996 \nonumber\\
newspaper_ca & 0.99996 \nonumber\\
warning & 0.99996 \nonumber\\
n't_fit & 0.99996 \nonumber\\
tv_actors/actresses & 0.99996 \nonumber\\
update_or & 0.99996 \nonumber\\
or_new & 0.99996 \nonumber\\
'_happen & 0.99996 \nonumber\\
or_update & 0.99996 \nonumber\\
book_and & 0.99996 \nonumber\\
happen_around & 0.99996 \nonumber\\
new_flash & 0.99996 \nonumber\\
kid_look & 0.99996 \nonumber\\
and_practice & 0.99996 \nonumber\\
until_you & 0.99996 \nonumber\\
stay_in & 0.99996 \nonumber\\
they_know & 0.99996 \nonumber\\
it_for & 0.99996 \nonumber\\
fit & 0.99996 \nonumber\\
come_together & 0.99996 \nonumber\\
of_be & 0.99996 \nonumber\\
knock & 0.99996 \nonumber\\
have_two & 0.99996 \nonumber\\
stop & 0.99996 \nonumber\\
other_but & 0.99996 \nonumber\\
move & 0.99996 \nonumber\\
each_day & 0.99996 \nonumber\\
_pos_ngram_CONJ_PP_V & 0.99996 \nonumber\\
"_; & 0.99996 \nonumber\\
_pos_ngram_ART_PP_V & 0.99996 \nonumber\\
the_effect & 0.99996 \nonumber\\
protect_the & 0.99996 \nonumber\\
only_be & 0.99996 \nonumber\\
various_religion & 0.99996 \nonumber\\
numerous_religion & 0.99996 \nonumber\\
between_various & 0.99996 \nonumber\\
corruption_in & 0.99996 \nonumber\\
,_fight & 0.99996 \nonumber\\
ProductionRule_NP->NP,,,NP,,,NP,,,NP,,,CC,ADVP,NP, & 0.99996 \nonumber\\
,_numerous & 0.99996 \nonumber\\
of_corruption & 0.99996 \nonumber\\
in_politician & 0.99996 \nonumber\\
ProductionRule_NP->NNP,NNP,NNP,NNP,NNP,NNP, & 0.99996 \nonumber\\
without_get & 0.99996 \nonumber\\
of_creatoinism & 0.99996 \nonumber\\
who_beleive & 0.99996 \nonumber\\
everybody_this & 0.99996 \nonumber\\
with_anyone & 0.99996 \nonumber\\
get_into & 0.99996 \nonumber\\
hint & 0.99996 \nonumber\\
hint_everybody & 0.99996 \nonumber\\
argument_because & 0.99996 \nonumber\\
in_creatoinism & 0.99996 \nonumber\\
think_take & 0.99996 \nonumber\\
be_moronic & 0.99996 \nonumber\\
moronic_!!!!!!!!!!!!!!!!!! & 0.99996 \nonumber\\
creatoinism_without & 0.99996 \nonumber\\
creatoinism_who & 0.99996 \nonumber\\
extreamly_dumb & 0.99996 \nonumber\\
extreamly & 0.99996 \nonumber\\
creatoinism & 0.99996 \nonumber\\
moronic & 0.99996 \nonumber\\
a_hint & 0.99996 \nonumber\\
anybody_who & 0.99996 \nonumber\\
dumb_argument & 0.99996 \nonumber\\
an_extreamly & 0.99996 \nonumber\\
because_anybody & 0.99996 \nonumber\\
n't_can & 0.99996 \nonumber\\
behavior & 0.99996 \nonumber\\
an_85 & 0.99996 \nonumber\\
85 & 0.99996 \nonumber\\
university_. & 0.99996 \nonumber\\
reason_there & 0.99996 \nonumber\\
last_25 & 0.99996 \nonumber\\
decline_in & 0.99996 \nonumber\\
rape_over & 0.99996 \nonumber\\
professor_at & 0.99996 \nonumber\\
decline & 0.99996 \nonumber\\
ProductionRule_NP->DT,CD,NN,NN, & 0.99996 \nonumber\\
northwestern_university & 0.99996 \nonumber\\
25 & 0.99996 \nonumber\\
professor & 0.99996 \nonumber\\
easy_access & 0.99996 \nonumber\\
law_professor & 0.99996 \nonumber\\
northwestern & 0.99996 \nonumber\\
85_percent & 0.99996 \nonumber\\
porn_may & 0.99996 \nonumber\\
25_year & 0.99996 \nonumber\\
at_northwestern & 0.99996 \nonumber\\
percent_decline & 0.99996 \nonumber\\
parent_would & 0.99996 \nonumber\\
because_that & 0.99996 \nonumber\\
difference & 0.99996 \nonumber\\
legal & 0.99996 \nonumber\\
just_say & 0.99996 \nonumber\\
us_be & 0.99996 \nonumber\\
favor & 0.99996 \nonumber\\
purchase & 0.99996 \nonumber\\
that_evolution & 0.99996 \nonumber\\
dog & 0.99996 \nonumber\\
if_student & 0.99996 \nonumber\\
to_farquhar & 0.99996 \nonumber\\
the_majority & 0.99996 \nonumber\\
n't_alway & 0.99996 \nonumber\\
_pos_ngram_CONJ_ART_PR & 0.99996 \nonumber\\
to_turn & 0.99996 \nonumber\\
ProductionRule_VP->VBZ,ADVP,VP, & 0.99996 \nonumber\\
_pos_ngram_PR_CONJ_NN & 0.99996 \nonumber\\
_pos_ngram_CONJ_ADJ_ART & 0.99996 \nonumber\\
me_? & 0.99996 \nonumber\\
because_sometime & 0.99996 \nonumber\\
another_reason & 0.99996 \nonumber\\
moral_and & 0.99996 \nonumber\\
and_solve & 0.99996 \nonumber\\
know_and & 0.99996 \nonumber\\
a_human & 0.99996 \nonumber\\
_pos_ngram_PUNC_ART_PP & 0.99996 \nonumber\\
water_, & 0.99996 \nonumber\\
deserve_to & 0.99996 \nonumber\\
non & 0.99996 \nonumber\\
combine & 0.99996 \nonumber\\
attention_to & 0.99996 \nonumber\\
difficult & 0.99996 \nonumber\\
ProductionRule_PP->RB,IN,S, & 0.99996 \nonumber\\
raise_in & 0.99996 \nonumber\\
human_race & 0.99996 \nonumber\\
employee & 0.99996 \nonumber\\
no_i & 0.99996 \nonumber\\
ProductionRule_NP->NP,,,ADVP,NP, & 0.99996 \nonumber\\
for_my & 0.99996 \nonumber\\
parent_. & 0.99996 \nonumber\\
._today & 0.99996 \nonumber\\
the_unborn & 0.99996 \nonumber\\
discipline & 0.99996 \nonumber\\
government_. & 0.99996 \nonumber\\
that_abortion & 0.99996 \nonumber\\
make_by & 0.99996 \nonumber\\
parent_of & 0.99996 \nonumber\\
personally_do & 0.99996 \nonumber\\
way_shape & 0.99996 \nonumber\\
a_debate & 0.99996 \nonumber\\
environment_. & 0.99996 \nonumber\\
activity & 0.99996 \nonumber\\
_pos_ngram_CARD_NN_ART & 0.99996 \nonumber\\
treaty_with & 0.99996 \nonumber\\
who_sign & 0.99996 \nonumber\\
_pos_ngram_NP_NN_PP & 0.99996 \nonumber\\
yourself_and & 0.99996 \nonumber\\
hole & 0.99996 \nonumber\\
bencoolen & 0.99996 \nonumber\\
my_spouse & 0.99996 \nonumber\\
science_, & 0.99996 \nonumber\\
_pos_ngram_NP_ADV_PR & 0.99996 \nonumber\\
about_ourselve & 0.99996 \nonumber\\
their_community & 0.99996 \nonumber\\
our_community & 0.99996 \nonumber\\
dangerous_place & 0.99996 \nonumber\\
everyone_try & 0.99996 \nonumber\\
than_just & 0.99996 \nonumber\\
community_first & 0.99996 \nonumber\\
ourselve_. & 0.99996 \nonumber\\
community_then & 0.99996 \nonumber\\
no_dangerous & 0.99996 \nonumber\\
tell_them & 0.99996 \nonumber\\
porn_, & 0.99996 \nonumber\\
qualify & 0.99996 \nonumber\\
thing_you & 0.99996 \nonumber\\
from_his & 0.99996 \nonumber\\
the_economy & 0.99996 \nonumber\\
a_period & 0.99996 \nonumber\\
on_in & 0.99996 \nonumber\\
than_we & 0.99996 \nonumber\\
tv_can & 0.99996 \nonumber\\
will_go & 0.99996 \nonumber\\
pest & 0.99996 \nonumber\\
of_you & 0.99996 \nonumber\\
course_, & 0.99996 \nonumber\\
do_, & 0.99996 \nonumber\\
mankind & 0.99996 \nonumber\\
_pos_ngram_ART_PUNC_V & 0.99996 \nonumber\\
EndingIble & 0.99996 \nonumber\\
make_my & 0.99996 \nonumber\\
that_advance & 0.99996 \nonumber\\
the_rest & 0.99996 \nonumber\\
rest_of & 0.99996 \nonumber\\
development_, & 0.99996 \nonumber\\
also_the & 0.99996 \nonumber\\
_pos_ngram_NP_CONJ_NP & 0.99996 \nonumber\\
._ofcourse & 0.99996 \nonumber\\
probably_leave & 0.99996 \nonumber\\
deed_instead & 0.99996 \nonumber\\
a_malicious & 0.99996 \nonumber\\
malicious_deed & 0.99996 \nonumber\\
ofcourse & 0.99996 \nonumber\\
the_severity & 0.99996 \nonumber\\
toward_my & 0.99996 \nonumber\\
ofcourse_i & 0.99996 \nonumber\\
want_nothong & 0.99996 \nonumber\\
him_free & 0.99996 \nonumber\\
belongings & 0.99996 \nonumber\\
his_family & 0.99996 \nonumber\\
nothong_to & 0.99996 \nonumber\\
or_belongings & 0.99996 \nonumber\\
to_defend & 0.99996 \nonumber\\
family_or & 0.99996 \nonumber\\
severity & 0.99996 \nonumber\\
empathetic & 0.99996 \nonumber\\
be_empathetic & 0.99996 \nonumber\\
free_, & 0.99996 \nonumber\\
empathetic_toward & 0.99996 \nonumber\\
malicious & 0.99996 \nonumber\\
nothong & 0.99996 \nonumber\\
defense_, & 0.99996 \nonumber\\
belongings_i & 0.99996 \nonumber\\
the_kill & 0.99996 \nonumber\\
defend_his & 0.99996 \nonumber\\
severity_of & 0.99996 \nonumber\\
_pos_ngram_CONJ_PP_PUNC & 0.99996 \nonumber\\
ProductionRule_VP->VBD,NP,ADVP, & 0.99996 \nonumber\\
pursuit_do & 0.99996 \nonumber\\
a_terrible & 0.99996 \nonumber\\
all_, & 0.99996 \nonumber\\
then_who & 0.99996 \nonumber\\
ProductionRule_FRAG->NP,SBAR, & 0.99996 \nonumber\\
a_christian & 0.99996 \nonumber\\
or_something & 0.99996 \nonumber\\
fight_and & 0.99996 \nonumber\\
ProductionRule_NP->DT,S, & 0.99996 \nonumber\\
beleive_in & 0.99996 \nonumber\\
their_personal & 0.99996 \nonumber\\
_pos_ngram_CARD_NN_CONJ & 0.99996 \nonumber\\
more_about & 0.99996 \nonumber\\
people_feel & 0.99996 \nonumber\\
of_" & 0.99996 \nonumber\\
ProductionRule_VP->ADVP,VBD,PP, & 0.99996 \nonumber\\
know_him & 0.99996 \nonumber\\
will_cause & 0.99996 \nonumber\\
go_with & 0.99996 \nonumber\\
kill_. & 0.99996 \nonumber\\
i_prefer & 0.99996 \nonumber\\
husband_, & 0.99996 \nonumber\\
child_to & 0.99996 \nonumber\\
and_wonder & 0.99996 \nonumber\\
basicly_. & 0.99996 \nonumber\\
a_horrible & 0.99996 \nonumber\\
horrible_crime & 0.99996 \nonumber\\
turn_yourself & 0.99996 \nonumber\\
law_basicly & 0.99996 \nonumber\\
wrong_no & 0.99996 \nonumber\\
difficult_for & 0.99996 \nonumber\\
of_wait & 0.99996 \nonumber\\
be_above & 0.99996 \nonumber\\
basicly & 0.99996 \nonumber\\
above_the & 0.99996 \nonumber\\
wife_, & 0.99996 \nonumber\\
at_him & 0.99996 \nonumber\\
life_in & 0.99996 \nonumber\\
than_anything & 0.99996 \nonumber\\
exact_answer & 0.99996 \nonumber\\
stronger_that & 0.99996 \nonumber\\
sentence_to & 0.99996 \nonumber\\
like_nothing & 0.99996 \nonumber\\
feel_be & 0.99996 \nonumber\\
my_exact & 0.99996 \nonumber\\
or_spend & 0.99996 \nonumber\\
probably_be & 0.99996 \nonumber\\
stronger_than & 0.99996 \nonumber\\
feeling_would & 0.99996 \nonumber\\
everyday_and & 0.99996 \nonumber\\
husband_have & 0.99996 \nonumber\\
prison_. & 0.99996 \nonumber\\
bid_husband & 0.99996 \nonumber\\
answer_but & 0.99996 \nonumber\\
nothing_happen & 0.99996 \nonumber\\
be_sentence & 0.99996 \nonumber\\
him_everyday & 0.99996 \nonumber\\
my_feeling & 0.99996 \nonumber\\
death_or & 0.99996 \nonumber\\
contribute & 0.99996 \nonumber\\
a_decision & 0.99996 \nonumber\\
clean_the & 0.99996 \nonumber\\
line_. & 0.99996 \nonumber\\
grade & 0.99996 \nonumber\\
optional & 0.99996 \nonumber\\
love_, & 0.99996 \nonumber\\
lucky & 0.99996 \nonumber\\
be_lucky & 0.99996 \nonumber\\
ProductionRule_WHADVP->RB,WRB, & 0.99996 \nonumber\\
_pos_ngram_NN_O_NN & 0.99996 \nonumber\\
every_single & 0.99996 \nonumber\\
condition_it & 0.99996 \nonumber\\
those_condition & 0.99996 \nonumber\\
disease_every & 0.99996 \nonumber\\
raffle_build & 0.99996 \nonumber\\
not_catch & 0.99996 \nonumber\\
help_on & 0.99996 \nonumber\\
the_live & 0.99996 \nonumber\\
olden_time & 0.99996 \nonumber\\
ProductionRule_NP->RB,CD,NN, & 0.99996 \nonumber\\
catch_a & 0.99996 \nonumber\\
thing_raffle & 0.99996 \nonumber\\
condition_be & 0.99996 \nonumber\\
reason_he & 0.99996 \nonumber\\
month_in & 0.99996 \nonumber\\
save_so & 0.99996 \nonumber\\
day.hospitals & 0.99996 \nonumber\\
one_month & 0.99996 \nonumber\\
day.hospitals_be & 0.99996 \nonumber\\
a_surprise & 0.99996 \nonumber\\
go_live & 0.99996 \nonumber\\
single_day.hospitals & 0.99996 \nonumber\\
condition_in & 0.99996 \nonumber\\
time_condition & 0.99996 \nonumber\\
have_save & 0.99996 \nonumber\\
live_there & 0.99996 \nonumber\\
be_condition & 0.99996 \nonumber\\
build_and & 0.99996 \nonumber\\
surprise_if & 0.99996 \nonumber\\
surprise & 0.99996 \nonumber\\
that_olden & 0.99996 \nonumber\\
can_look & 0.99996 \nonumber\\
personal_choice & 0.99996 \nonumber\\
do_for & 0.99996 \nonumber\\
the_life & 0.99996 \nonumber\\
._even & 0.99996 \nonumber\\
i_just & 0.99996 \nonumber\\
near_future & 0.99996 \nonumber\\
in_near & 0.99996 \nonumber\\
lot_go & 0.99996 \nonumber\\
grade_. & 0.99996 \nonumber\\
grade_student & 0.99996 \nonumber\\
beneficially & 0.99996 \nonumber\\
beneficially_by & 0.99996 \nonumber\\
in_8th & 0.99996 \nonumber\\
optional_in & 0.99996 \nonumber\\
student_want & 0.99996 \nonumber\\
time_may & 0.99996 \nonumber\\
8th_grade & 0.99996 \nonumber\\
8th & 0.99996 \nonumber\\
more_beneficially & 0.99996 \nonumber\\
be_optional & 0.99996 \nonumber\\
participate_, & 0.99996 \nonumber\\
p.e._should & 0.99996 \nonumber\\
by_study & 0.99996 \nonumber\\
to_participate & 0.99996 \nonumber\\
norm & 0.99996 \nonumber\\
moth & 0.99996 \nonumber\\
charge_of & 0.99996 \nonumber\\
_pos_ngram_V_O_PUNC & 0.99996 \nonumber\\
when_you & 0.99996 \nonumber\\
at_work & 0.99996 \nonumber\\
potato & 0.99996 \nonumber\\
regulation & 0.99996 \nonumber\\
ProductionRule_VP->VB,NP,,,SBAR, & 0.99996 \nonumber\\
physical_education & 0.99996 \nonumber\\
?_or & 0.99996 \nonumber\\
britain & 0.99996 \nonumber\\
legalize & 0.99996 \nonumber\\
be_become & 0.99996 \nonumber\\
wrong_with & 0.99996 \nonumber\\
clothe_. & 0.99996 \nonumber\\
time_and & 0.99996 \nonumber\\
that_decision & 0.99996 \nonumber\\
decision_. & 0.99996 \nonumber\\
but_do & 0.99996 \nonumber\\
who_my & 0.99996 \nonumber\\
steal & 0.99996 \nonumber\\
easy & 0.99996 \nonumber\\
ProductionRule_NP->DT,JJ,NN,NNS, & 0.99996 \nonumber\\
be_bid & 0.99996 \nonumber\\
_pos_ngram_O_ART_ADJ & 0.99996 \nonumber\\
_pos_ngram_PUNC_NP_CONJ & 0.99996 \nonumber\\
more_than & 0.99996 \nonumber\\
everything_. & 0.99996 \nonumber\\
father_he & 0.99996 \nonumber\\
_pos_ngram_ADJ_ADV_PUNC & 0.99996 \nonumber\\
ProductionRule_VP->VBN,NP,PP, & 0.99996 \nonumber\\
in_indium & 0.99996 \nonumber\\
ProductionRule_VP->VBN,NP,SBAR, & 0.99996 \nonumber\\
and_with & 0.99996 \nonumber\\
a_major & 0.99996 \nonumber\\
person_that & 0.99996 \nonumber\\
ProductionRule_VP->VBG,PP,SBAR, & 0.99996 \nonumber\\
what_kind & 0.99996 \nonumber\\
decision_to & 0.99996 \nonumber\\
those_time & 0.99996 \nonumber\\
it_to & 0.99996 \nonumber\\
EndingAble & 0.99996 \nonumber\\
side_of & 0.99996 \nonumber\\
fight_between & 0.99996 \nonumber\\
really_dont & 0.99996 \nonumber\\
a_father & 0.99996 \nonumber\\
happiness & 0.99996 \nonumber\\
._yes & 0.99996 \nonumber\\
certain & 0.99996 \nonumber\\
mistake_, & 0.99996 \nonumber\\
_pos_ngram_PR_O_PP & 0.99996 \nonumber\\
pro-life & 0.99996 \nonumber\\
_pos_ngram_CONJ_ART_PP & 0.99996 \nonumber\\
_pos_ngram_PR_CONJ_ADV & 0.99996 \nonumber\\
so_i & 0.99996 \nonumber\\
_pos_ngram_V_NN_ART & 0.99996 \nonumber\\
work_together & 0.99996 \nonumber\\
it_! & 0.99996 \nonumber\\
kid_. & 0.99996 \nonumber\\
a_god & 0.99996 \nonumber\\
above & 0.99996 \nonumber\\
worst & 0.99996 \nonumber\\
manage & 0.99996 \nonumber\\
indium_can & 0.99996 \nonumber\\
abuse & 0.99996 \nonumber\\
be_at & 0.99996 \nonumber\\
on_radiometric & 0.99996 \nonumber\\
over_40 & 0.99996 \nonumber\\
be_independent & 0.99996 \nonumber\\
falsifiable & 0.99996 \nonumber\\
different_technique & 0.99996 \nonumber\\
independent_, & 0.99996 \nonumber\\
and_falsifiable & 0.99996 \nonumber\\
independent & 0.99996 \nonumber\\
recommend_go & 0.99996 \nonumber\\
tohttp_: & 0.99996 \nonumber\\
tohttp & 0.99996 \nonumber\\
/_www.asa3.org/asa/resources/wiens.html & 0.99996 \nonumber\\
,_observable & 0.99996 \nonumber\\
today_there & 0.99996 \nonumber\\
date_can & 0.99996 \nonumber\\
date_. & 0.99996 \nonumber\\
fact_they & 0.99996 \nonumber\\
more_information & 0.99996 \nonumber\\
be_over & 0.99996 \nonumber\\
/_/ & 0.99996 \nonumber\\
ProductionRule_NP->JJ,VBG, & 0.99996 \nonumber\\
information_on & 0.99996 \nonumber\\
40_different & 0.99996 \nonumber\\
go_tohttp & 0.99996 \nonumber\\
rigor_. & 0.99996 \nonumber\\
www.asa3.org/asa/resources/wiens.html_for & 0.99996 \nonumber\\
it_scientific & 0.99996 \nonumber\\
observable & 0.99996 \nonumber\\
falsifiable_that & 0.99996 \nonumber\\
would_recommend & 0.99996 \nonumber\\
observable_, & 0.99996 \nonumber\\
recommend & 0.99996 \nonumber\\
www.asa3.org/asa/resources/wiens.html & 0.99996 \nonumber\\
_pos_ngram_ADJ_PUNC_PUNC & 0.99996 \nonumber\\
ProductionRule_VP->VB,PP,NP, & 0.99996 \nonumber\\
_pos_ngram_O_CONJ_NN & 0.99996 \nonumber\\
national & 0.99996 \nonumber\\
be_what & 0.99996 \nonumber\\
not_sure & 0.99996 \nonumber\\
the_population & 0.99996 \nonumber\\
society_, & 0.99996 \nonumber\\
kill_somebody & 0.99996 \nonumber\\
unfair & 0.99996 \nonumber\\
in_those & 0.99996 \nonumber\\
time_because & 0.99996 \nonumber\\
because_at & 0.99996 \nonumber\\
reduce_the & 0.99996 \nonumber\\
must_be & 0.99996 \nonumber\\
watch & 0.99996 \nonumber\\
the_development & 0.99996 \nonumber\\
remove_the & 0.99996 \nonumber\\
ProductionRule_S->CC,NP,VP, & 0.99996 \nonumber\\
to_attack & 0.99996 \nonumber\\
concern & 0.99996 \nonumber\\
think_they & 0.99996 \nonumber\\
ProductionRule_VP->VBG,ADJP, & 0.99996 \nonumber\\
a_right & 0.99996 \nonumber\\
this_one & 0.99996 \nonumber\\
ProductionRule_S->PP,VP, & 0.99996 \nonumber\\
say_some & 0.99996 \nonumber\\
debate_can & 0.99996 \nonumber\\
help_!!! & 0.99996 \nonumber\\
at_our & 0.99996 \nonumber\\
please_help & 0.99996 \nonumber\\
point_on & 0.99996 \nonumber\\
can_people & 0.99996 \nonumber\\
_pos_ngram_ADV_CONJ_PP & 0.99996 \nonumber\\
with_that & 0.99996 \nonumber\\
whom & 0.99996 \nonumber\\
father_who & 0.99996 \nonumber\\
to_buy & 0.99996 \nonumber\\
our_child & 0.99996 \nonumber\\
currently_not & 0.99996 \nonumber\\
be_currently & 0.99996 \nonumber\\
walk_on & 0.99996 \nonumber\\
evolution_beleiver & 0.99996 \nonumber\\
beleiver & 0.99996 \nonumber\\
to_walk & 0.99996 \nonumber\\
and_man & 0.99996 \nonumber\\
mankind_? & 0.99996 \nonumber\\
currently & 0.99996 \nonumber\\
banus_adam & 0.99996 \nonumber\\
_pos_ngram_O_ART_ADV & 0.99996 \nonumber\\
and_eve & 0.99996 \nonumber\\
of_mankind & 0.99996 \nonumber\\
banus & 0.99996 \nonumber\\
beleiver_... & 0.99996 \nonumber\\
the_tribe & 0.99996 \nonumber\\
man_kind & 0.99996 \nonumber\\
very_planet & 0.99996 \nonumber\\
parent_' & 0.99996 \nonumber\\
whom_have & 0.99996 \nonumber\\
of_adam & 0.99996 \nonumber\\
ProductionRule_VP->VBZ,ADVP,RB,VP, & 0.99996 \nonumber\\
this_evolution & 0.99996 \nonumber\\
have_religion & 0.99996 \nonumber\\
planet_, & 0.99996 \nonumber\\
..._how & 0.99996 \nonumber\\
in_arabic & 0.99996 \nonumber\\
adam_' & 0.99996 \nonumber\\
tribe_of & 0.99996 \nonumber\\
adam_... & 0.99996 \nonumber\\
'_banus & 0.99996 \nonumber\\
ProductionRule_NP->NP,:,SBARQ, & 0.99996 \nonumber\\
makind_be & 0.99996 \nonumber\\
literally_means & 0.99996 \nonumber\\
now_tell & 0.99996 \nonumber\\
kind_be & 0.99996 \nonumber\\
eve_be & 0.99996 \nonumber\\
eve & 0.99996 \nonumber\\
true_, & 0.99996 \nonumber\\
me_this & 0.99996 \nonumber\\
which_literally & 0.99996 \nonumber\\
_pos_ngram_NP_NN_O & 0.99996 \nonumber\\
'_parent & 0.99996 \nonumber\\
it_( & 0.99996 \nonumber\\
you_whom & 0.99996 \nonumber\\
makind & 0.99996 \nonumber\\
arabic_makind & 0.99996 \nonumber\\
'_which & 0.99996 \nonumber\\
_pos_ngram_PR_PR_NP & 0.99996 \nonumber\\
religion_) & 0.99996 \nonumber\\
that_adam & 0.99996 \nonumber\\
arabic & 0.99996 \nonumber\\
race_to & 0.99996 \nonumber\\
fear & 0.99996 \nonumber\\
be_my & 0.99996 \nonumber\\
brother & 0.99996 \nonumber\\
human_. & 0.99996 \nonumber\\
competition & 0.99996 \nonumber\\
r & 0.99996 \nonumber\\
ProductionRule_ADJP->VBN,PP, & 0.99996 \nonumber\\
loser & 0.99996 \nonumber\\
water_be & 0.99996 \nonumber\\
in_that & 0.99996 \nonumber\\
say_to & 0.99996 \nonumber\\
supportive_of & 0.99996 \nonumber\\
_pos_ngram_PR_NP_CONJ & 0.99996 \nonumber\\
be_eighteen & 0.99996 \nonumber\\
be_supportive & 0.99996 \nonumber\\
yet_not & 0.99996 \nonumber\\
supportive & 0.99996 \nonumber\\
year_since & 0.99996 \nonumber\\
_pos_ngram_ART_NP_PR & 0.99996 \nonumber\\
he_want & 0.99996 \nonumber\\
pay_attention & 0.99996 \nonumber\\
eighteen_year & 0.99996 \nonumber\\
should_i & 0.99996 \nonumber\\
eighteen & 0.99996 \nonumber\\
_pos_ngram_NP_CONJ_CONJ & 0.99996 \nonumber\\
care_then & 0.99996 \nonumber\\
but_yet & 0.99996 \nonumber\\
wish_i & 0.99996 \nonumber\\
see_my & 0.99996 \nonumber\\
opinion_to & 0.99996 \nonumber\\
through_it & 0.99996 \nonumber\\
_pos_ngram_NP_PR_PR & 0.99996 \nonumber\\
i_? & 0.99996 \nonumber\\
ProductionRule_VP->MD,CC,MD,RB,VP, & 0.99996 \nonumber\\
damn & 0.99996 \nonumber\\
every_way & 0.99996 \nonumber\\
every_person & 0.99996 \nonumber\\
get_rid & 0.99996 \nonumber\\
rid_of & 0.99996 \nonumber\\
a_commonly & 0.99996 \nonumber\\
commonly & 0.99996 \nonumber\\
spread & 0.99996 \nonumber\\
but_i & 0.99996 \nonumber\\
for_child & 0.99996 \nonumber\\
so_why & 0.99996 \nonumber\\
wonder_if & 0.99996 \nonumber\\
pollute & 0.99996 \nonumber\\
right_. & 0.99996 \nonumber\\
or_form & 0.99996 \nonumber\\
shape_or & 0.99996 \nonumber\\
form_. & 0.99996 \nonumber\\
p.e. & 0.99996 \nonumber\\
ProductionRule_S->INTJ,,,NP,VP,., & 0.99996 \nonumber\\
to_raise & 0.99996 \nonumber\\
and_cant & 0.99996 \nonumber\\
not_be & 0.99996 \nonumber\\
criminal & 0.99996 \nonumber\\
ProductionRule_VP->VBD,ADVP,PP, & 0.99996 \nonumber\\
_pos_ngram_PP_PUNC_V & 0.99996 \nonumber\\
people_should & 0.99996 \nonumber\\
_pos_ngram_CONJ_CONJ_ADV & 0.99996 \nonumber\\
ProductionRule_NP->FW,FW,FW, & 0.99996 \nonumber\\
so_therefore & 0.99996 \nonumber\\
will_also & 0.99996 \nonumber\\
people_do & 0.99996 \nonumber\\
be_more & 0.99996 \nonumber\\
your_dad & 0.99996 \nonumber\\
the_church & 0.99996 \nonumber\\
number & 0.99996 \nonumber\\
alway_go & 0.99996 \nonumber\\
obesity & 0.99996 \nonumber\\
._trust & 0.99996 \nonumber\\
set & 0.99996 \nonumber\\
around_the & 0.99996 \nonumber\\
reason_for & 0.99996 \nonumber\\
will_end & 0.99996 \nonumber\\
be_many & 0.99996 \nonumber\\
ProductionRule_VP->VB,ADJP,PP, & 0.99996 \nonumber\\
ProductionRule_RRC->ADVP,NP, & 0.99996 \nonumber\\
by_raffle & 0.99996 \nonumber\\
man_and & 0.99996 \nonumber\\
do_thing & 0.99996 \nonumber\\
somebody & 0.99996 \nonumber\\
and_because & 0.99996 \nonumber\\
mean_to & 0.99996 \nonumber\\
well_. & 0.99996 \nonumber\\
what_if & 0.99996 \nonumber\\
_pos_ngram_PP_ADJ_V & 0.99996 \nonumber\\
stupid & 0.99996 \nonumber\\
use_in & 0.99996 \nonumber\\
enjoy_help & 0.99996 \nonumber\\
that_would & 0.99996 \nonumber\\
we_just & 0.99996 \nonumber\\
_pos_ngram_PUNC_ADV_O & 0.99996 \nonumber\\
his_own & 0.99997 \nonumber\\
these_two & 0.99997 \nonumber\\
ProductionRule_FRAG->NP,,,SBAR,., & 0.99997 \nonumber\\
curious & 0.99997 \nonumber\\
load & 0.99997 \nonumber\\
if_not & 0.99997 \nonumber\\
,_what & 0.99997 \nonumber\\
be_also & 0.99997 \nonumber\\
advancement & 0.99997 \nonumber\\
ProductionRule_NP->PRP$,JJ, & 0.99997 \nonumber\\
option_to & 0.99997 \nonumber\\
not_your & 0.99997 \nonumber\\
private & 0.99997 \nonumber\\
tribe & 0.99997 \nonumber\\
be_important & 0.99997 \nonumber\\
ProductionRule_NP->NN,RB, & 0.99997 \nonumber\\
side_, & 0.99997 \nonumber\\
homosexuality_be & 0.99997 \nonumber\\
religion_and & 0.99997 \nonumber\\
yes_because & 0.99997 \nonumber\\
contribute_to & 0.99997 \nonumber\\
believe_it & 0.99997 \nonumber\\
industry & 0.99997 \nonumber\\
toward_their & 0.99997 \nonumber\\
six & 0.99997 \nonumber\\
ProductionRule_NP->DT,NNP,NNP, & 0.99997 \nonumber\\
there_when & 0.99997 \nonumber\\
,_etc & 0.99997 \nonumber\\
"_by & 0.99997 \nonumber\\
depression & 0.99997 \nonumber\\
genius & 0.99997 \nonumber\\
have_highest & 0.99997 \nonumber\\
indian_employee & 0.99997 \nonumber\\
do_most & 0.99997 \nonumber\\
cuz_we & 0.99997 \nonumber\\
surely_lead & 0.99997 \nonumber\\
intellectually & 0.99997 \nonumber\\
intellectually_superior.in & 0.99997 \nonumber\\
their_door & 0.99997 \nonumber\\
of_depression & 0.99997 \nonumber\\
genius_, & 0.99997 \nonumber\\
really_david & 0.99997 \nonumber\\
past_we & 0.99997 \nonumber\\
be_genius & 0.99997 \nonumber\\
_pos_ngram_ADJ_ART_PUNC & 0.99997 \nonumber\\
knock_their & 0.99997 \nonumber\\
depression_, & 0.99997 \nonumber\\
name_firm & 0.99997 \nonumber\\
ProductionRule_VP->VB,ADJP,,,SBAR, & 0.99997 \nonumber\\
have_lead & 0.99997 \nonumber\\
for_gain & 0.99997 \nonumber\\
will_surely & 0.99997 \nonumber\\
employee_cuz & 0.99997 \nonumber\\
ProductionRule_VP->ADVP,NP,SBAR, & 0.99997 \nonumber\\
again_in & 0.99997 \nonumber\\
world_again & 0.99997 \nonumber\\
your_country & 0.99997 \nonumber\\
gain_peace & 0.99997 \nonumber\\
indium_for & 0.99997 \nonumber\\
david_then & 0.99997 \nonumber\\
future_wait & 0.99997 \nonumber\\
door_in & 0.99997 \nonumber\\
of_indian & 0.99997 \nonumber\\
why_people & 0.99997 \nonumber\\
ProductionRule_NP->DT,VBN,NNS, & 0.99997 \nonumber\\
world_have & 0.99997 \nonumber\\
country_knock & 0.99997 \nonumber\\
ooooooooh & 0.99997 \nonumber\\
david & 0.99997 \nonumber\\
superior.in & 0.99997 \nonumber\\
superior.in_past & 0.99997 \nonumber\\
actually_intellectually & 0.99997 \nonumber\\
firm_of & 0.99997 \nonumber\\
highest_no & 0.99997 \nonumber\\
from_your & 0.99997 \nonumber\\
ooooooooh_really & 0.99997 \nonumber\\
country.because_a & 0.99997 \nonumber\\
glance_, & 0.99997 \nonumber\\
terrorism_and & 0.99997 \nonumber\\
can_remove & 0.99997 \nonumber\\
aware & 0.99997 \nonumber\\
progress_from & 0.99997 \nonumber\\
so_on.no & 0.99997 \nonumber\\
a_criminal & 0.99997 \nonumber\\
one_realize & 0.99997 \nonumber\\
to_specify & 0.99997 \nonumber\\
any_solid & 0.99997 \nonumber\\
glance & 0.99997 \nonumber\\
human.i & 0.99997 \nonumber\\
hurdle_in & 0.99997 \nonumber\\
which_we & 0.99997 \nonumber\\
of_problem & 0.99997 \nonumber\\
from_root.we & 0.99997 \nonumber\\
hurdle & 0.99997 \nonumber\\
another_human.i & 0.99997 \nonumber\\
our_progress & 0.99997 \nonumber\\
root.we & 0.99997 \nonumber\\
country.because & 0.99997 \nonumber\\
but_unable & 0.99997 \nonumber\\
give_solutions.they & 0.99997 \nonumber\\
role_for & 0.99997 \nonumber\\
root.we_all & 0.99997 \nonumber\\
the_hurdle & 0.99997 \nonumber\\
human.i_hope & 0.99997 \nonumber\\
if_look & 0.99997 \nonumber\\
why_a & 0.99997 \nonumber\\
think_my & 0.99997 \nonumber\\
and_reply & 0.99997 \nonumber\\
terrorist_, & 0.99997 \nonumber\\
reply_me & 0.99997 \nonumber\\
reply & 0.99997 \nonumber\\
much_aware & 0.99997 \nonumber\\
on.no & 0.99997 \nonumber\\
be_criticize & 0.99997 \nonumber\\
at_glance & 0.99997 \nonumber\\
problem_but & 0.99997 \nonumber\\
solutions.they & 0.99997 \nonumber\\
on.no_one & 0.99997 \nonumber\\
and_role & 0.99997 \nonumber\\
solutions.they_be & 0.99997 \nonumber\\
good_citizen & 0.99997 \nonumber\\
a_citizen & 0.99997 \nonumber\\
syona_if & 0.99997 \nonumber\\
create_problem & 0.99997 \nonumber\\
duty_? & 0.99997 \nonumber\\
government_, & 0.99997 \nonumber\\
by_which & 0.99997 \nonumber\\
my_view & 0.99997 \nonumber\\
understand_abt & 0.99997 \nonumber\\
ProductionRule_NP->RB,JJ,NN, & 0.99997 \nonumber\\
citizen_what & 0.99997 \nonumber\\
should_understand & 0.99997 \nonumber\\
aware_of & 0.99997 \nonumber\\
,_terrorist & 0.99997 \nonumber\\
importance_and & 0.99997 \nonumber\\
criticize & 0.99997 \nonumber\\
,_corrupt & 0.99997 \nonumber\\
corrupt_politician & 0.99997 \nonumber\\
ProductionRule_NP->NP,SBAR,PP, & 0.99997 \nonumber\\
criminal_, & 0.99997 \nonumber\\
our_duty & 0.99997 \nonumber\\
criticize_government & 0.99997 \nonumber\\
view_and & 0.99997 \nonumber\\
their_importance & 0.99997 \nonumber\\
solid_solution & 0.99997 \nonumber\\
solution_by & 0.99997 \nonumber\\
specify_any & 0.99997 \nonumber\\
ProductionRule_UCP->NP,CC,ADJP, & 0.99997 \nonumber\\
for_country.because & 0.99997 \nonumber\\
good_in & 0.99997 \nonumber\\
for_themselve & 0.99997 \nonumber\\
ProductionRule_VP->VBN,PP,SBAR, & 0.99997 \nonumber\\
_pos_ngram_ADJ_NN_ART & 0.99997 \nonumber\\
up_without & 0.99997 \nonumber\\
of_love & 0.99997 \nonumber\\
_pos_ngram_CONJ_V_NP & 0.99997 \nonumber\\
lol & 0.99997 \nonumber\\
some_point & 0.99997 \nonumber\\
constantly & 0.99997 \nonumber\\
be_raffle & 0.99997 \nonumber\\
whenever & 0.99997 \nonumber\\
religious_, & 0.99997 \nonumber\\
ProductionRule_NP->NP,SBAR,SBAR, & 0.99997 \nonumber\\
just_because & 0.99997 \nonumber\\
eh & 0.99997 \nonumber\\
ProductionRule_VP->VBP,RB,ADVP,VP, & 0.99997 \nonumber\\
be_against & 0.99997 \nonumber\\
ProductionRule_NP->NP,ADJP,POS, & 0.99997 \nonumber\\
because_people & 0.99997 \nonumber\\
face & 0.99997 \nonumber\\
_pos_ngram_O_CARD_V & 0.99997 \nonumber\\
soon_. & 0.99997 \nonumber\\
lesson & 0.99997 \nonumber\\
nerve & 0.99997 \nonumber\\
all_depend & 0.99997 \nonumber\\
should_not & 0.99997 \nonumber\\
illegal_. & 0.99997 \nonumber\\
some_choice & 0.99997 \nonumber\\
world_would & 0.99997 \nonumber\\
total_chaos & 0.99997 \nonumber\\
choice_in & 0.99997 \nonumber\\
in_charge & 0.99997 \nonumber\\
_pos_ngram_PP_ADV_CARD & 0.99997 \nonumber\\
minute & 0.99997 \nonumber\\
we_get & 0.99997 \nonumber\\
science & 0.99997 \nonumber\\
of_student & 0.99997 \nonumber\\
a_simple & 0.99997 \nonumber\\
all_that & 0.99997 \nonumber\\
_pos_ngram_V_NP_PR & 0.99997 \nonumber\\
school_and & 0.99997 \nonumber\\
ProductionRule_VP->VBZ,UCP, & 0.99997 \nonumber\\
have_them & 0.99997 \nonumber\\
leave_and & 0.99997 \nonumber\\
world_. & 0.99997 \nonumber\\
today_. & 0.99997 \nonumber\\
technique_to & 0.99997 \nonumber\\
ProductionRule_ADJP->JJR,PP, & 0.99997 \nonumber\\
so_many & 0.99997 \nonumber\\
no_different & 0.99997 \nonumber\\
file & 0.99997 \nonumber\\
this_person & 0.99997 \nonumber\\
only_when & 0.99997 \nonumber\\
peace_and & 0.99997 \nonumber\\
emerge & 0.99997 \nonumber\\
well_as & 0.99997 \nonumber\\
and_fight & 0.99997 \nonumber\\
_pos_ngram_CARD_PP_PR & 0.99997 \nonumber\\
then_its & 0.99997 \nonumber\\
ProductionRule_VP->VBD,ADVP,S, & 0.99997 \nonumber\\
you_learn & 0.99997 \nonumber\\
alone_with & 0.99997 \nonumber\\
really_care & 0.99997 \nonumber\\
get_a & 0.99997 \nonumber\\
its_the & 0.99997 \nonumber\\
would_help & 0.99997 \nonumber\\
for_every & 0.99997 \nonumber\\
_pos_ngram_ADV_PR_PR & 0.99997 \nonumber\\
the_right & 0.99997 \nonumber\\
ProductionRule_NP->JJ,NN,CC,NN, & 0.99997 \nonumber\\
_pos_ngram_PR_CONJ_ART & 0.99997 \nonumber\\
be_worth & 0.99997 \nonumber\\
way_, & 0.99997 \nonumber\\
40 & 0.99997 \nonumber\\
compare & 0.99997 \nonumber\\
in_sport & 0.99997 \nonumber\\
this_very & 0.99997 \nonumber\\
several_time & 0.99997 \nonumber\\
unbelievably_minute & 0.99997 \nonumber\\
)_exist & 0.99997 \nonumber\\
ProductionRule_VP->VBZ,ADJP,PP,PP,S, & 0.99997 \nonumber\\
the_unbelievably & 0.99997 \nonumber\\
breed_. & 0.99997 \nonumber\\
the_strong & 0.99997 \nonumber\\
the_species & 0.99997 \nonumber\\
this_strengthen & 0.99997 \nonumber\\
over_. & 0.99997 \nonumber\\
creationism_and & 0.99997 \nonumber\\
exclusionary_. & 0.99997 \nonumber\\
exclusionary & 0.99997 \nonumber\\
not_exclusionary & 0.99997 \nonumber\\
minute_chance & 0.99997 \nonumber\\
argument_over & 0.99997 \nonumber\\
unbelievably & 0.99997 \nonumber\\
to_breed & 0.99997 \nonumber\\
god_simply & 0.99997 \nonumber\\
impossible_for & 0.99997 \nonumber\\
strong_continue & 0.99997 \nonumber\\
._argument & 0.99997 \nonumber\\
god_( & 0.99997 \nonumber\\
god_) & 0.99997 \nonumber\\
the_weak & 0.99997 \nonumber\\
weak_die & 0.99997 \nonumber\\
use_more & 0.99997 \nonumber\\
for_me & 0.99997 \nonumber\\
the_date & 0.99997 \nonumber\\
and_only & 0.99997 \nonumber\\
of_these & 0.99997 \nonumber\\
turn_my & 0.99997 \nonumber\\
be_load & 0.99997 \nonumber\\
who_' & 0.99997 \nonumber\\
ProductionRule_VP->VBZ,NP,SBAR, & 0.99997 \nonumber\\
practice & 0.99997 \nonumber\\
twice_. & 0.99997 \nonumber\\
'_of & 0.99997 \nonumber\\
who_she & 0.99997 \nonumber\\
door & 0.99997 \nonumber\\
be_gon & 0.99997 \nonumber\\
share_and & 0.99997 \nonumber\\
he_pass & 0.99997 \nonumber\\
nerve_and & 0.99997 \nonumber\\
way_father & 0.99997 \nonumber\\
without_my & 0.99997 \nonumber\\
there_because & 0.99997 \nonumber\\
hey_that & 0.99997 \nonumber\\
n't_wan & 0.99997 \nonumber\\
dad_there & 0.99997 \nonumber\\
mom_without & 0.99997 \nonumber\\
father_' & 0.99997 \nonumber\\
pass_away & 0.99997 \nonumber\\
away_when & 0.99997 \nonumber\\
to_even & 0.99997 \nonumber\\
be_six & 0.99997 \nonumber\\
six_. & 0.99997 \nonumber\\
ProductionRule_NP->CC,NN, & 0.99997 \nonumber\\
a_favorite & 0.99997 \nonumber\\
favorite_side & 0.99997 \nonumber\\
have_other & 0.99997 \nonumber\\
your_nerve & 0.99997 \nonumber\\
sometime_they & 0.99997 \nonumber\\
be_christian & 0.99997 \nonumber\\
n't_do & 0.99997 \nonumber\\
than_have & 0.99997 \nonumber\\
no_match & 0.99997 \nonumber\\
my_use & 0.99997 \nonumber\\
match_. & 0.99997 \nonumber\\
every_year & 0.99997 \nonumber\\
supplies & 0.99997 \nonumber\\
happy_and & 0.99997 \nonumber\\
baby_up & 0.99997 \nonumber\\
doughter_to & 0.99997 \nonumber\\
guess_lousy & 0.99997 \nonumber\\
doughter & 0.99997 \nonumber\\
could_happen & 0.99997 \nonumber\\
or_doughter & 0.99997 \nonumber\\
love_their & 0.99997 \nonumber\\
as_perfect & 0.99997 \nonumber\\
on_anything & 0.99997 \nonumber\\
perfect_as & 0.99997 \nonumber\\
posible_. & 0.99997 \nonumber\\
wonderful_thing & 0.99997 \nonumber\\
their_son & 0.99997 \nonumber\\
posible & 0.99997 \nonumber\\
want_their & 0.99997 \nonumber\\
as_posible & 0.99997 \nonumber\\
need_someone & 0.99997 \nonumber\\
one_can & 0.99997 \nonumber\\
what_she & 0.99997 \nonumber\\
the_christian & 0.99997 \nonumber\\
_pos_ngram_PP_PUNC_NN & 0.99997 \nonumber\\
themselve_better & 0.99997 \nonumber\\
make_themselve & 0.99997 \nonumber\\
better_people & 0.99997 \nonumber\\
teaching_of & 0.99997 \nonumber\\
my_mom & 0.99997 \nonumber\\
i_get & 0.99997 \nonumber\\
hav_n't & 0.99997 \nonumber\\
hav & 0.99997 \nonumber\\
evidence_if & 0.99997 \nonumber\\
evolution_at & 0.99997 \nonumber\\
up_; & 0.99997 \nonumber\\
our_small & 0.99997 \nonumber\\
,_seemingly & 0.99997 \nonumber\\
,_simple & 0.99997 \nonumber\\
who_really & 0.99997 \nonumber\\
up_lose & 0.99997 \nonumber\\
lose_it & 0.99997 \nonumber\\
become_increasingly & 0.99997 \nonumber\\
look_this & 0.99997 \nonumber\\
;_every & 0.99997 \nonumber\\
be_evolve & 0.99997 \nonumber\\
generation_our & 0.99997 \nonumber\\
._eventually & 0.99997 \nonumber\\
increasingly_smaller & 0.99997 \nonumber\\
useless_appendage & 0.99997 \nonumber\\
small_toe & 0.99997 \nonumber\\
increasingly & 0.99997 \nonumber\\
small_, & 0.99997 \nonumber\\
toe_be & 0.99997 \nonumber\\
one_up & 0.99997 \nonumber\\
appendage & 0.99997 \nonumber\\
smaller & 0.99997 \nonumber\\
seemingly_useless & 0.99997 \nonumber\\
seemingly & 0.99997 \nonumber\\
toe & 0.99997 \nonumber\\
appendage_and & 0.99997 \nonumber\\
every_generation & 0.99997 \nonumber\\
and_who & 0.99997 \nonumber\\
eventually_, & 0.99997 \nonumber\\
smaller_. & 0.99997 \nonumber\\
her_and & 0.99997 \nonumber\\
have_commit & 0.99997 \nonumber\\
birth_to & 0.99997 \nonumber\\
give_birth & 0.99997 \nonumber\\
hole_in & 0.99997 \nonumber\\
more_violent & 0.99997 \nonumber\\
act_up & 0.99997 \nonumber\\
get_discipline & 0.99997 \nonumber\\
discipline_if & 0.99997 \nonumber\\
violent_and & 0.99997 \nonumber\\
be_acceptable & 0.99997 \nonumber\\
_pos_ngram_CONJ_ART_ADV & 0.99997 \nonumber\\
truly & 0.99997 \nonumber\\
advancement_of & 0.99997 \nonumber\\
_pos_ngram_NN_PP_PUNC & 0.99997 \nonumber\\
even_though & 0.99997 \nonumber\\
singapore_but & 0.99997 \nonumber\\
the_grind & 0.99997 \nonumber\\
ProductionRule_NP->PDT,DT,NN,NN, & 0.99997 \nonumber\\
grind_work & 0.99997 \nonumber\\
only_dream & 0.99997 \nonumber\\
improve_singapore & 0.99997 \nonumber\\
that_she & 0.99997 \nonumber\\
show & 0.99997 \nonumber\\
thing_and & 0.99997 \nonumber\\
fashion & 0.99997 \nonumber\\
to_act & 0.99997 \nonumber\\
himself & 0.99997 \nonumber\\
send & 0.99997 \nonumber\\
play_the & 0.99997 \nonumber\\
get_more & 0.99997 \nonumber\\
but_still & 0.99997 \nonumber\\
illogical & 0.99997 \nonumber\\
ProductionRule_S->``,NP,VP,.,'', & 0.99997 \nonumber\\
bid_as & 0.99997 \nonumber\\
on_my & 0.99997 \nonumber\\
simple & 0.99997 \nonumber\\
ProductionRule_S->NP,ADJP,SBAR, & 0.99997 \nonumber\\
wan_na & 0.99997 \nonumber\\
wan & 0.99997 \nonumber\\
feel_that & 0.99997 \nonumber\\
goods & 0.99997 \nonumber\\
from_right & 0.99997 \nonumber\\
,_such & 0.99997 \nonumber\\
to_see & 0.99997 \nonumber\\
pop & 0.99997 \nonumber\\
they_get & 0.99997 \nonumber\\
to_watch & 0.99997 \nonumber\\
do_think & 0.99997 \nonumber\\
browser & 0.99997 \nonumber\\
be_hand & 0.99997 \nonumber\\
'_mother & 0.99997 \nonumber\\
notice & 0.99997 \nonumber\\
centipede & 0.99997 \nonumber\\
the_city & 0.99997 \nonumber\\
thing_, & 0.99997 \nonumber\\
time_that & 0.99997 \nonumber\\
a_perfect & 0.99997 \nonumber\\
?_a & 0.99997 \nonumber\\
standard & 0.99997 \nonumber\\
bank & 0.99997 \nonumber\\
electrical_engineer & 0.99997 \nonumber\\
mechanical_and & 0.99997 \nonumber\\
mechanical & 0.99997 \nonumber\\
as_mechanical & 0.99997 \nonumber\\
food_process & 0.99997 \nonumber\\
fast_emerge & 0.99997 \nonumber\\
in_sector & 0.99997 \nonumber\\
multinational_company & 0.99997 \nonumber\\
have_provide & 0.99997 \nonumber\\
tourism_and & 0.99997 \nonumber\\
every_multinational & 0.99997 \nonumber\\
to_enhance & 0.99997 \nonumber\\
bank_among & 0.99997 \nonumber\\
multinational & 0.99997 \nonumber\\
electrical & 0.99997 \nonumber\\
among_other & 0.99997 \nonumber\\
,_tourism & 0.99997 \nonumber\\
enhance & 0.99997 \nonumber\\
enhance_trade & 0.99997 \nonumber\\
and_electrical & 0.99997 \nonumber\\
automotive & 0.99997 \nonumber\\
investment_in & 0.99997 \nonumber\\
be_focus & 0.99997 \nonumber\\
engineer_, & 0.99997 \nonumber\\
investment_. & 0.99997 \nonumber\\
a_hub & 0.99997 \nonumber\\
,_food & 0.99997 \nonumber\\
investment & 0.99997 \nonumber\\
and_investment & 0.99997 \nonumber\\
for_international & 0.99997 \nonumber\\
automotive_, & 0.99997 \nonumber\\
provide_a & 0.99997 \nonumber\\
and_bank & 0.99997 \nonumber\\
be_fast & 0.99997 \nonumber\\
,_automotive & 0.99997 \nonumber\\
emerge_as & 0.99997 \nonumber\\
on_indium & 0.99997 \nonumber\\
sector_such & 0.99997 \nonumber\\
hub_for & 0.99997 \nonumber\\
huge_opportunity & 0.99997 \nonumber\\
international_trade & 0.99997 \nonumber\\
its_not & 0.99997 \nonumber\\
parent_to & 0.99997 \nonumber\\
government_do & 0.99997 \nonumber\\
woman_what & 0.99997 \nonumber\\
the_marriage & 0.99997 \nonumber\\
across & 0.99997 \nonumber\\
involve & 0.99997 \nonumber\\
food & 0.99997 \nonumber\\
ProductionRule_SQ->VBP,NP,VP, & 0.99997 \nonumber\\
_pos_ngram_CARD_PUNC_ADJ & 0.99997 \nonumber\\
dont_wear & 0.99997 \nonumber\\
this_and & 0.99997 \nonumber\\
everyone_wear & 0.99997 \nonumber\\
drama & 0.99997 \nonumber\\
forever_try & 0.99997 \nonumber\\
of_oh & 0.99997 \nonumber\\
then_everyone & 0.99997 \nonumber\\
nicer & 0.99997 \nonumber\\
spend_forever & 0.99997 \nonumber\\
nicer_2 & 0.99997 \nonumber\\
drama_, & 0.99997 \nonumber\\
wear_that & 0.99997 \nonumber\\
uniform_there & 0.99997 \nonumber\\
wear_this & 0.99997 \nonumber\\
._less & 0.99997 \nonumber\\
and_3 & 0.99997 \nonumber\\
less_of & 0.99997 \nonumber\\
to_figure & 0.99997 \nonumber\\
and_1 & 0.99997 \nonumber\\
out_what & 0.99997 \nonumber\\
oh_you & 0.99997 \nonumber\\
wear_and & 0.99997 \nonumber\\
_pos_ngram_ART_CONJ_PR & 0.99997 \nonumber\\
look_nicer & 0.99997 \nonumber\\
less_drama & 0.99997 \nonumber\\
,_to & 0.99997 \nonumber\\
world_but & 0.99997 \nonumber\\
baby_that & 0.99997 \nonumber\\
counter_to & 0.99997 \nonumber\\
be_unprepare & 0.99997 \nonumber\\
common_argument & 0.99997 \nonumber\\
a_legendary & 0.99997 \nonumber\\
davincus_? & 0.99997 \nonumber\\
:_what & 0.99997 \nonumber\\
legendary_figure & 0.99997 \nonumber\\
het & 0.99997 \nonumber\\
het_pregnant & 0.99997 \nonumber\\
unprepare_for & 0.99997 \nonumber\\
unprepare & 0.99997 \nonumber\\
next_davincus & 0.99997 \nonumber\\
davincus & 0.99997 \nonumber\\
ProductionRule_WHNP->WHNP,ADJP, & 0.99997 \nonumber\\
legendary & 0.99997 \nonumber\\
pregnant_be & 0.99997 \nonumber\\
who_het & 0.99997 \nonumber\\
simple_counter & 0.99997 \nonumber\\
to_because & 0.99997 \nonumber\\
ProductionRule_VP->VBZ,,,``,SBAR, & 0.99997 \nonumber\\
an_image & 0.99997 \nonumber\\
_pos_ngram_NP_ADJ & 0.99997 \nonumber\\
think_your & 0.99997 \nonumber\\
your_opponent & 0.99997 \nonumber\\
ProductionRule_ADVP->DT,JJR, & 0.99997 \nonumber\\
any_stronger & 0.99997 \nonumber\\
brainwash_one & 0.99997 \nonumber\\
ProductionRule_FRAG->ADVP,SBAR, & 0.99997 \nonumber\\
way_or & 0.99997 \nonumber\\
the_good & 0.99997 \nonumber\\
of_your & 0.99997 \nonumber\\
me_about & 0.99997 \nonumber\\
yes_i & 0.99997 \nonumber\\
._they & 0.99997 \nonumber\\
wouldnt & 0.99997 \nonumber\\
not_create & 0.99997 \nonumber\\
the_whole & 0.99997 \nonumber\\
percent & 0.99997 \nonumber\\
for_reason & 0.99997 \nonumber\\
change_and & 0.99997 \nonumber\\
"_there & 0.99997 \nonumber\\
themselve_. & 0.99997 \nonumber\\
than_a & 0.99997 \nonumber\\
ProductionRule_NP->DT,ADJP,NNS, & 0.99997 \nonumber\\
rather_have & 0.99997 \nonumber\\
the_property & 0.99997 \nonumber\\
to_command & 0.99997 \nonumber\\
command_her & 0.99997 \nonumber\\
ProductionRule_PP->IN,``,SBARQ,'', & 0.99997 \nonumber\\
command & 0.99997 \nonumber\\
choose_, & 0.99997 \nonumber\\
you_choose & 0.99997 \nonumber\\
property_of & 0.99997 \nonumber\\
she_the & 0.99997 \nonumber\\
property_. & 0.99997 \nonumber\\
any_fetus & 0.99997 \nonumber\\
her_servitude & 0.99997 \nonumber\\
church_, & 0.99997 \nonumber\\
decide_" & 0.99997 \nonumber\\
your_property & 0.99997 \nonumber\\
servitude_. & 0.99997 \nonumber\\
servitude & 0.99997 \nonumber\\
._nor & 0.99997 \nonumber\\
your_church & 0.99997 \nonumber\\
who_decide & 0.99997 \nonumber\\
breed & 0.99997 \nonumber\\
close & 0.99997 \nonumber\\
._all & 0.99997 \nonumber\\
support & 0.99997 \nonumber\\
evolutionary & 0.99997 \nonumber\\
my_kid & 0.99997 \nonumber\\
creationist & 0.99997 \nonumber\\
so_be & 0.99997 \nonumber\\
ProductionRule_S->SBAR,,,NP,VP,., & 0.99997 \nonumber\\
special & 0.99997 \nonumber\\
some_of & 0.99997 \nonumber\\
ProductionRule_NP->NP,ADJP,., & 0.99997 \nonumber\\
baby_, & 0.99997 \nonumber\\
raise_a & 0.99997 \nonumber\\
habit & 0.99997 \nonumber\\
the_industrial & 0.99997 \nonumber\\
revolution & 0.99997 \nonumber\\
industrial_revolution & 0.99997 \nonumber\\
revolution_. & 0.99997 \nonumber\\
therefore_i & 0.99997 \nonumber\\
that_everyone & 0.99997 \nonumber\\
large & 0.99997 \nonumber\\
who_we & 0.99997 \nonumber\\
his_idea & 0.99997 \nonumber\\
to_learn & 0.99997 \nonumber\\
else_would & 0.99997 \nonumber\\
argument_could & 0.99997 \nonumber\\
n't_find & 0.99997 \nonumber\\
ProductionRule_NP->NP,UCP, & 0.99997 \nonumber\\
of_year & 0.99997 \nonumber\\
hour_. & 0.99997 \nonumber\\
fun & 0.99997 \nonumber\\
then_most & 0.99997 \nonumber\\
as_harry & 0.99997 \nonumber\\
tree_so & 0.99997 \nonumber\\
damage_to & 0.99997 \nonumber\\
potter_be & 0.99997 \nonumber\\
potter & 0.99997 \nonumber\\
of_tree & 0.99997 \nonumber\\
television_use & 0.99997 \nonumber\\
more_damage & 0.99997 \nonumber\\
book_such & 0.99997 \nonumber\\
electricity_and & 0.99997 \nonumber\\
make_of & 0.99997 \nonumber\\
harry_potter & 0.99997 \nonumber\\
harry & 0.99997 \nonumber\\
cause_more & 0.99997 \nonumber\\
because_be & 0.99997 \nonumber\\
strength_to & 0.99997 \nonumber\\
through_that & 0.99997 \nonumber\\
the_confidence & 0.99997 \nonumber\\
with_yourself & 0.99997 \nonumber\\
satisfy_yourself & 0.99997 \nonumber\\
happy_with & 0.99997 \nonumber\\
yoursel_first & 0.99997 \nonumber\\
yoursel & 0.99997 \nonumber\\
money_he & 0.99997 \nonumber\\
,_whenever & 0.99997 \nonumber\\
someone_want & 0.99997 \nonumber\\
and_enjoy & 0.99997 \nonumber\\
outside_world & 0.99997 \nonumber\\
goal_, & 0.99997 \nonumber\\
already_succesful & 0.99997 \nonumber\\
succesful_and & 0.99997 \nonumber\\
while_satisfy & 0.99997 \nonumber\\
succesful & 0.99997 \nonumber\\
succeed_in & 0.99997 \nonumber\\
help_yoursel & 0.99997 \nonumber\\
strength & 0.99997 \nonumber\\
and_through & 0.99997 \nonumber\\
to_succeed & 0.99997 \nonumber\\
achieve_his & 0.99997 \nonumber\\
whenever_he & 0.99997 \nonumber\\
the_outside & 0.99997 \nonumber\\
he_achieve & 0.99997 \nonumber\\
his_goal & 0.99997 \nonumber\\
with_money & 0.99997 \nonumber\\
and_strength & 0.99997 \nonumber\\
attack & 0.99997 \nonumber\\
wear_. & 0.99997 \nonumber\\
to_his & 0.99997 \nonumber\\
that_i & 0.99997 \nonumber\\
the_butt & 0.99997 \nonumber\\
would_spank & 0.99997 \nonumber\\
thing_twice & 0.99997 \nonumber\\
,_out & 0.99997 \nonumber\\
spank_my & 0.99997 \nonumber\\
butt_. & 0.99997 \nonumber\\
butt & 0.99997 \nonumber\\
after_i & 0.99997 \nonumber\\
shape_and & 0.99997 \nonumber\\
stress & 0.99997 \nonumber\\
take & 0.99997 \nonumber\\
bother & 0.99997 \nonumber\\
bother_me & 0.99997 \nonumber\\
have_pe & 0.99997 \nonumber\\
_pos_ngram_PP_PUNC_NP & 0.99997 \nonumber\\
so_much & 0.99997 \nonumber\\
eye & 0.99997 \nonumber\\
_pos_ngram_ART_PP_PP & 0.99997 \nonumber\\
consider_a & 0.99997 \nonumber\\
..._i & 0.99997 \nonumber\\
fatherless_so & 0.99997 \nonumber\\
correct_your & 0.99997 \nonumber\\
follow_your & 0.99997 \nonumber\\
or_fatherless & 0.99997 \nonumber\\
msitake_that & 0.99997 \nonumber\\
success_in & 0.99997 \nonumber\\
your_msitake & 0.99997 \nonumber\\
good_either & 0.99997 \nonumber\\
might_follow & 0.99997 \nonumber\\
msitake & 0.99997 \nonumber\\
to_success & 0.99997 \nonumber\\
can_encourage & 0.99997 \nonumber\\
you_correct & 0.99997 \nonumber\\
bid_influence & 0.99997 \nonumber\\
either_because & 0.99997 \nonumber\\
ok_but & 0.99997 \nonumber\\
you_bid & 0.99997 \nonumber\\
boss & 0.99997 \nonumber\\
again_to & 0.99997 \nonumber\\
ProductionRule_VP->VBD,NP,ADVP,S, & 0.99997 \nonumber\\
second_time & 0.99997 \nonumber\\
already_. & 0.99997 \nonumber\\
spank_i & 0.99997 \nonumber\\
punish_because & 0.99997 \nonumber\\
ProductionRule_VP->VBZ,ADVP,ADJP,SBAR, & 0.99997 \nonumber\\
worst_because & 0.99997 \nonumber\\
ProductionRule_VP->VBN,S,ADVP, & 0.99997 \nonumber\\
to_already & 0.99997 \nonumber\\
sure_i & 0.99997 \nonumber\\
avoid_be & 0.99997 \nonumber\\
alway_worst & 0.99997 \nonumber\\
_pos_ngram_PP_PUNC_O & 0.99997 \nonumber\\
because_only & 0.99997 \nonumber\\
find_also & 0.99997 \nonumber\\
'_educational & 0.99997 \nonumber\\
u_live & 0.99997 \nonumber\\
live_news & 0.99997 \nonumber\\
at_book & 0.99997 \nonumber\\
u_ca & 0.99997 \nonumber\\
news_at & 0.99997 \nonumber\\
only_tv & 0.99997 \nonumber\\
bring_u & 0.99997 \nonumber\\
book_u & 0.99997 \nonumber\\
gain & 0.99997 \nonumber\\
have_your & 0.99997 \nonumber\\
be_pay & 0.99997 \nonumber\\
participate & 0.99997 \nonumber\\
it_all & 0.99997 \nonumber\\
_pos_ngram_O_PR_ADV & 0.99997 \nonumber\\
influence & 0.99997 \nonumber\\
kid_, & 0.99997 \nonumber\\
school_, & 0.99997 \nonumber\\
back_to & 0.99997 \nonumber\\
pepper_moth & 0.99997 \nonumber\\
pepper & 0.99997 \nonumber\\
aint & 0.99997 \nonumber\\
'_why & 0.99997 \nonumber\\
lend & 0.99997 \nonumber\\
avoid_them & 0.99997 \nonumber\\
example_or & 0.99997 \nonumber\\
to_lend & 0.99997 \nonumber\\
at_his & 0.99997 \nonumber\\
and_avoid & 0.99997 \nonumber\\
a_hand & 0.99997 \nonumber\\
mom_. & 0.99997 \nonumber\\
need_help & 0.99997 \nonumber\\
any_kind & 0.99997 \nonumber\\
of_person & 0.99997 \nonumber\\
lend_you & 0.99997 \nonumber\\
no_example & 0.99997 \nonumber\\
people_in & 0.99997 \nonumber\\
(_i & 0.99997 \nonumber\\
the_water & 0.99997 \nonumber\\
you_should & 0.99997 \nonumber\\
ProductionRule_VP->VBZ,S,SBAR, & 0.99997 \nonumber\\
a_problem & 0.99997 \nonumber\\
me_what & 0.99997 \nonumber\\
issue_, & 0.99997 \nonumber\\
ProductionRule_NP->NN,CD, & 0.99997 \nonumber\\
choose_life & 0.99997 \nonumber\\
would_much & 0.99997 \nonumber\\
much_rather & 0.99997 \nonumber\\
_pos_ngram_ADJ_CONJ_NP & 0.99997 \nonumber\\
person_or & 0.99997 \nonumber\\
allow_to & 0.99997 \nonumber\\
turn_you & 0.99997 \nonumber\\
till & 0.99997 \nonumber\\
kill_me & 0.99997 \nonumber\\
source_of & 0.99997 \nonumber\\
ultimate & 0.99997 \nonumber\\
other_do & 0.99997 \nonumber\\
be_your & 0.99997 \nonumber\\
ProductionRule_VP->VBG,VP, & 0.99997 \nonumber\\
ProductionRule_UCP->NP,CC,PP, & 0.99997 \nonumber\\
your_religion & 0.99997 \nonumber\\
believe_there & 0.99997 \nonumber\\
._before & 0.99997 \nonumber\\
remember_about & 0.99997 \nonumber\\
about_those & 0.99997 \nonumber\\
within_yourself & 0.99997 \nonumber\\
truly_happy & 0.99997 \nonumber\\
fulfil_something & 0.99997 \nonumber\\
must_remember & 0.99997 \nonumber\\
fulfillment & 0.99997 \nonumber\\
to_fulfillment & 0.99997 \nonumber\\
where_one & 0.99997 \nonumber\\
fulfillment_where & 0.99997 \nonumber\\
endeavor_because & 0.99997 \nonumber\\
fulfil & 0.99997 \nonumber\\
before_help & 0.99997 \nonumber\\
._achieve & 0.99997 \nonumber\\
be_fulfil & 0.99997 \nonumber\\
be_truly & 0.99997 \nonumber\\
something_within & 0.99997 \nonumber\\
journey_to & 0.99997 \nonumber\\
achieve_a & 0.99997 \nonumber\\
really_in & 0.99997 \nonumber\\
say_the & 0.99997 \nonumber\\
_pos_ngram_ADV_ADV_ART & 0.99997 \nonumber\\
indian & 0.99997 \nonumber\\
news & 0.99997 \nonumber\\
less_likely & 0.99997 \nonumber\\
ProductionRule_NP->JJ,JJ,NNS, & 0.99997 \nonumber\\
wait & 0.99997 \nonumber\\
also_a & 0.99997 \nonumber\\
that_need & 0.99997 \nonumber\\
motivation & 0.99997 \nonumber\\
die & 0.99997 \nonumber\\
can_count & 0.99997 \nonumber\\
count_on & 0.99997 \nonumber\\
ProductionRule_S->SBAR,,,ADVP,NP,VP,., & 0.99997 \nonumber\\
night & 0.99997 \nonumber\\
if_this & 0.99997 \nonumber\\
n't_give & 0.99997 \nonumber\\
better_if & 0.99997 \nonumber\\
confidence_and & 0.99997 \nonumber\\
goal_be & 0.99997 \nonumber\\
plus_it & 0.99997 \nonumber\\
be_and & 0.99997 \nonumber\\
father_then & 0.99997 \nonumber\\
add-on & 0.99997 \nonumber\\
hey & 0.99997 \nonumber\\
about_love & 0.99997 \nonumber\\
generation_. & 0.99997 \nonumber\\
about_family & 0.99997 \nonumber\\
about_example & 0.99997 \nonumber\\
about_parental & 0.99997 \nonumber\\
about_legal & 0.99997 \nonumber\\
about_societal & 0.99997 \nonumber\\
only_about & 0.99997 \nonumber\\
about_" & 0.99997 \nonumber\\
about_tax & 0.99997 \nonumber\\
about_generation & 0.99997 \nonumber\\
role_. & 0.99997 \nonumber\\
about_commitment & 0.99997 \nonumber\\
local_middle-school & 0.99997 \nonumber\\
dog_and & 0.99997 \nonumber\\
ProductionRule_SQ->VBZ,NP,ADVP,.,'', & 0.99997 \nonumber\\
just_about & 0.99997 \nonumber\\
my_dog & 0.99997 \nonumber\\
norm_. & 0.99997 \nonumber\\
really_just & 0.99997 \nonumber\\
love_" & 0.99997 \nonumber\\
love_? & 0.99997 \nonumber\\
'_about & 0.99997 \nonumber\\
could_get & 0.99997 \nonumber\\
marry_as & 0.99997 \nonumber\\
could_marry & 0.99997 \nonumber\\
marriage_really & 0.99997 \nonumber\\
be_marriage & 0.99997 \nonumber\\
think_not & 0.99997 \nonumber\\
commitment_. & 0.99997 \nonumber\\
societal_norm & 0.99997 \nonumber\\
marry_my & 0.99997 \nonumber\\
middle-school & 0.99997 \nonumber\\
societal & 0.99997 \nonumber\\
middle-school_could & 0.99997 \nonumber\\
parental & 0.99997 \nonumber\\
kid_at & 0.99997 \nonumber\\
parental_role & 0.99997 \nonumber\\
legal_rights & 0.99997 \nonumber\\
two_kid & 0.99997 \nonumber\\
"_love & 0.99997 \nonumber\\
and_get & 0.99997 \nonumber\\
outfit & 0.99997 \nonumber\\
do_be & 0.99997 \nonumber\\
have_not & 0.99997 \nonumber\\
anyway & 0.99997 \nonumber\\
for_book & 0.99997 \nonumber\\
human_, & 0.99997 \nonumber\\
into & 0.99997 \nonumber\\
character & 0.99997 \nonumber\\
_pos_ngram_V_NP_ADV & 0.99997 \nonumber\\
mention & 0.99997 \nonumber\\
then_do & 0.99997 \nonumber\\
ProductionRule_SBAR->RB,IN,S, & 0.99997 \nonumber\\
everyone_who & 0.99997 \nonumber\\
ProductionRule_NP->JJ,NN,NN,NNS, & 0.99997 \nonumber\\
find_it & 0.99997 \nonumber\\
_pos_ngram_ADV_ART_ADV & 0.99997 \nonumber\\
he_could & 0.99997 \nonumber\\
in_just & 0.99997 \nonumber\\
ProductionRule_NP->PRP$,NP, & 0.99997 \nonumber\\
easier_than & 0.99997 \nonumber\\
forget_about & 0.99997 \nonumber\\
regard_to & 0.99997 \nonumber\\
and_gang & 0.99997 \nonumber\\
victimization & 0.99997 \nonumber\\
less_competition & 0.99997 \nonumber\\
gang_activity & 0.99997 \nonumber\\
ProductionRule_S->S,CC,S,,,SBAR,., & 0.99997 \nonumber\\
as_there & 0.99997 \nonumber\\
competition_in & 0.99997 \nonumber\\
victimization_be & 0.99997 \nonumber\\
be_decrease & 0.99997 \nonumber\\
student_victimization & 0.99997 \nonumber\\
lower_and & 0.99997 \nonumber\\
gang & 0.99997 \nonumber\\
be_lower & 0.99997 \nonumber\\
decrease & 0.99997 \nonumber\\
most_fashionable & 0.99997 \nonumber\\
activity_should & 0.99997 \nonumber\\
decrease_, & 0.99997 \nonumber\\
in_regard & 0.99997 \nonumber\\
fashionable_clothe & 0.99997 \nonumber\\
that_to & 0.99997 \nonumber\\
?_everyone & 0.99997 \nonumber\\
problem_in & 0.99997 \nonumber\\
that_give & 0.99997 \nonumber\\
what_it & 0.99997 \nonumber\\
_pos_ngram_ART_V_NP & 0.99997 \nonumber\\
decision & 0.99997 \nonumber\\
the_point & 0.99997 \nonumber\\
abortion_be & 0.99997 \nonumber\\
be_get & 0.99997 \nonumber\\
the_local & 0.99997 \nonumber\\
perfect_world & 0.99997 \nonumber\\
ProductionRule_WHNP->WHNP,PP, & 0.99997 \nonumber\\
who_in & 0.99997 \nonumber\\
girl_outfit & 0.99997 \nonumber\\
school_girl & 0.99997 \nonumber\\
catholic_school & 0.99997 \nonumber\\
outfit_? & 0.99997 \nonumber\\
of_catholic & 0.99997 \nonumber\\
right_mind & 0.99997 \nonumber\\
mind_want & 0.99997 \nonumber\\
their_right & 0.99997 \nonumber\\
,_no & 0.99997 \nonumber\\
reason_why & 0.99997 \nonumber\\
of_all & 0.99997 \nonumber\\
_pos_ngram_O_O_PR & 0.99997 \nonumber\\
of_man & 0.99997 \nonumber\\
na_be & 0.99997 \nonumber\\
up_these & 0.99997 \nonumber\\
sure_thousand & 0.99997 \nonumber\\
..._mean & 0.99997 \nonumber\\
record_human & 0.99997 \nonumber\\
only_till & 0.99997 \nonumber\\
piss_ant & 0.99997 \nonumber\\
history_have & 0.99997 \nonumber\\
6_people & 0.99997 \nonumber\\
its_never & 0.99997 \nonumber\\
society_only & 0.99997 \nonumber\\
be_homosexual & 0.99997 \nonumber\\
6 & 0.99997 \nonumber\\
its_unfair & 0.99997 \nonumber\\
some_piss & 0.99997 \nonumber\\
how_its & 0.99997 \nonumber\\
vent & 0.99997 \nonumber\\
...._heck & 0.99997 \nonumber\\
more_weight & 0.99997 \nonumber\\
vent_on & 0.99997 \nonumber\\
_pos_ngram_ADJ_ADV_CARD & 0.99997 \nonumber\\
little_more & 0.99997 \nonumber\\
ProductionRule_VP->VBD,ADJP,ADVP,NP, & 0.99997 \nonumber\\
accept_as & 0.99997 \nonumber\\
remake_would & 0.99997 \nonumber\\
earth_... & 0.99997 \nonumber\\
sarcastic_remake & 0.99997 \nonumber\\
the_front & 0.99997 \nonumber\\
if_homosexuality & 0.99997 \nonumber\\
mean_none & 0.99997 \nonumber\\
weight_than & 0.99997 \nonumber\\
front_part & 0.99997 \nonumber\\
ant_liberal & 0.99997 \nonumber\\
around_2 & 0.99997 \nonumber\\
be_possibly & 0.99997 \nonumber\\
around_.... & 0.99997 \nonumber\\
ant & 0.99997 \nonumber\\
than_some & 0.99997 \nonumber\\
the_butthole & 0.99997 \nonumber\\
remake & 0.99997 \nonumber\\
human_history & 0.99997 \nonumber\\
natural_then & 0.99997 \nonumber\\
butthole_would & 0.99997 \nonumber\\
butthole & 0.99997 \nonumber\\
liberal_vent & 0.99997 \nonumber\\
unfair_. & 0.99997 \nonumber\\
these_sarcastic & 0.99997 \nonumber\\
heck_i & 0.99997 \nonumber\\
"_natural & 0.99997 \nonumber\\
natural_" & 0.99997 \nonumber\\
till_now & 0.99997 \nonumber\\
possibly_6 & 0.99997 \nonumber\\
and_centipede & 0.99997 \nonumber\\
rat_and & 0.99997 \nonumber\\
here_so & 0.99997 \nonumber\\
sometime_i & 0.99997 \nonumber\\
ProductionRule_S->NP,,,NP,VP,., & 0.99997 \nonumber\\
,_creationism & 0.99997 \nonumber\\
_pos_ngram_CONJ_CONJ_PR & 0.99997 \nonumber\\
and_plus & 0.99997 \nonumber\\
beat & 0.99997 \nonumber\\
far_more & 0.99997 \nonumber\\
of_choice & 0.99997 \nonumber\\
what_most & 0.99997 \nonumber\\
abortion_, & 0.99997 \nonumber\\
what_matter & 0.99997 \nonumber\\
pregnant_mother & 0.99997 \nonumber\\
must_decide & 0.99997 \nonumber\\
she_must & 0.99997 \nonumber\\
mother_what & 0.99997 \nonumber\\
personally_against & 0.99997 \nonumber\\
think_or & 0.99997 \nonumber\\
be_personally & 0.99997 \nonumber\\
homosexuality & 0.99997 \nonumber\\
he_decide & 0.99997 \nonumber\\
_pos_ngram_NN_O_NP & 0.99997 \nonumber\\
treaty & 0.99997 \nonumber\\
adam & 0.99997 \nonumber\\
title & 0.99997 \nonumber\\
the_title & 0.99997 \nonumber\\
purpose & 0.99997 \nonumber\\
what_, & 0.99997 \nonumber\\
?_who & 0.99997 \nonumber\\
home & 0.99997 \nonumber\\
cost_effective & 0.99997 \nonumber\\
._bid & 0.99997 \nonumber\\
very_. & 0.99997 \nonumber\\
ProductionRule_SQ->VBZ,ADVP, & 0.99997 \nonumber\\
ProductionRule_ADVP->RB,., & 0.99997 \nonumber\\
and_use & 0.99997 \nonumber\\
opinion_because & 0.99997 \nonumber\\
of_' & 0.99997 \nonumber\\
more_..... & 0.99997 \nonumber\\
apart & 0.99997 \nonumber\\
be_someone & 0.99997 \nonumber\\
regard & 0.99997 \nonumber\\
use_as & 0.99997 \nonumber\\
all_other & 0.99997 \nonumber\\
murder_someone & 0.99997 \nonumber\\
default_browser & 0.99997 \nonumber\\
default & 0.99997 \nonumber\\
._as & 0.99997 \nonumber\\
during_the & 0.99997 \nonumber\\
and_bring & 0.99997 \nonumber\\
of_exercise & 0.99997 \nonumber\\
_pos_ngram_PUNC_ART_CARD & 0.99997 \nonumber\\
be_tell & 0.99997 \nonumber\\
message & 0.99997 \nonumber\\
god_make & 0.99997 \nonumber\\
i_choose & 0.99997 \nonumber\\
as_i & 0.99997 \nonumber\\
see_them & 0.99997 \nonumber\\
in_case & 0.99997 \nonumber\\
bright & 0.99997 \nonumber\\
greatest & 0.99997 \nonumber\\
the_greatest & 0.99997 \nonumber\\
his_promise & 0.99997 \nonumber\\
be_once & 0.99997 \nonumber\\
pocket_. & 0.99997 \nonumber\\
when_singapore & 0.99997 \nonumber\\
promise_. & 0.99997 \nonumber\\
this_solve & 0.99997 \nonumber\\
pest_they & 0.99997 \nonumber\\
with_coin & 0.99997 \nonumber\\
he_hold & 0.99997 \nonumber\\
once_infest & 0.99997 \nonumber\\
use_cash & 0.99997 \nonumber\\
they_catch & 0.99997 \nonumber\\
coin & 0.99997 \nonumber\\
coin_for & 0.99997 \nonumber\\
hold_to & 0.99997 \nonumber\\
problem_quickly & 0.99997 \nonumber\\
reward_the & 0.99997 \nonumber\\
cash_from & 0.99997 \nonumber\\
quickly_, & 0.99997 \nonumber\\
every_pest & 0.99997 \nonumber\\
centipede_, & 0.99997 \nonumber\\
faquhar_solve & 0.99997 \nonumber\\
cash & 0.99997 \nonumber\\
infest_with & 0.99997 \nonumber\\
faquhar & 0.99997 \nonumber\\
with_rat & 0.99997 \nonumber\\
farquhar_reward & 0.99997 \nonumber\\
infest & 0.99997 \nonumber\\
singapore_use & 0.99997 \nonumber\\
one_way & 0.99997 \nonumber\\
needless_to & 0.99997 \nonumber\\
him_abort & 0.99997 \nonumber\\
mother_want & 0.99997 \nonumber\\
hitler & 0.99997 \nonumber\\
hitler_' & 0.99997 \nonumber\\
abort_. & 0.99997 \nonumber\\
._needless & 0.99997 \nonumber\\
have_him & 0.99997 \nonumber\\
let_her & 0.99997 \nonumber\\
needless & 0.99997 \nonumber\\
have_let & 0.99997 \nonumber\\
make_you & 0.99997 \nonumber\\
discipline_a & 0.99997 \nonumber\\
beleive & 0.99997 \nonumber\\
of_know & 0.99997 \nonumber\\
no_way & 0.99997 \nonumber\\
rise & 0.99997 \nonumber\\
an_atheist & 0.99997 \nonumber\\
you_please & 0.99997 \nonumber\\
think_what & 0.99997 \nonumber\\
_pos_ngram_NP_PP_ADJ & 0.99997 \nonumber\\
scientologist & 0.99997 \nonumber\\
scientologist_be & 0.99997 \nonumber\\
now_those & 0.99997 \nonumber\\
fight_them & 0.99997 \nonumber\\
ProductionRule_VP->VBG,,,ADVP,FRAG, & 0.99997 \nonumber\\
fight_, & 0.99997 \nonumber\\
run_rampant & 0.99997 \nonumber\\
those_scientologist & 0.99997 \nonumber\\
we_fight & 0.99997 \nonumber\\
rampant & 0.99997 \nonumber\\
rampant_. & 0.99997 \nonumber\\
be_little & 0.99997 \nonumber\\
marriage_just & 0.99997 \nonumber\\
in_many & 0.99997 \nonumber\\
woman_be & 0.99997 \nonumber\\
up_, & 0.99997 \nonumber\\
harder & 0.99997 \nonumber\\
ProductionRule_NP->NP,,,PP, & 0.99997 \nonumber\\
all_be & 0.99997 \nonumber\\
ProductionRule_CONJP->IN,RB, & 0.99997 \nonumber\\
christ & 0.99997 \nonumber\\
._) & 0.99997 \nonumber\\
persue & 0.99997 \nonumber\\
ProductionRule_S->NP,ADJP,., & 0.99997 \nonumber\\
_pos_ngram_NP_O_V & 0.99997 \nonumber\\
and_on & 0.99997 \nonumber\\
ProductionRule_S->NP,,,VP,., & 0.99997 \nonumber\\
to_gain & 0.99997 \nonumber\\
that_in & 0.99997 \nonumber\\
_pos_ngram_PP_PP_ADV & 0.99997 \nonumber\\
_pos_ngram_CONJ_CARD_NN & 0.99997 \nonumber\\
my_husband & 0.99997 \nonumber\\
should_follow & 0.99997 \nonumber\\
you_still & 0.99997 \nonumber\\
be_because & 0.99997 \nonumber\\
teaching & 0.99997 \nonumber\\
with_uniform & 0.99997 \nonumber\\
ProductionRule_S->VP,VP, & 0.99997 \nonumber\\
can_believe & 0.99997 \nonumber\\
deal_with & 0.99997 \nonumber\\
_pos_ngram_CARD_CONJ & 0.99997 \nonumber\\
be_those & 0.99997 \nonumber\\
or_not & 0.99997 \nonumber\\
heck & 0.99997 \nonumber\\
simply_because & 0.99997 \nonumber\\
_pos_ngram_CARD_NN_PR & 0.99997 \nonumber\\
here_' & 0.99997 \nonumber\\
child_, & 0.99997 \nonumber\\
ProductionRule_PP->IN,ADJP, & 0.99997 \nonumber\\
ProductionRule_NP->JJS,NNS, & 0.99997 \nonumber\\
n't_make & 0.99997 \nonumber\\
be_either & 0.99997 \nonumber\\
journey & 0.99997 \nonumber\\
a_journey & 0.99997 \nonumber\\
mandatory & 0.99997 \nonumber\\
be_mandatory & 0.99997 \nonumber\\
indian_people & 0.99997 \nonumber\\
foreign & 0.99997 \nonumber\\
foreign_country & 0.99997 \nonumber\\
life_and & 0.99997 \nonumber\\
tweak & 0.99997 \nonumber\\
god_' & 0.99997 \nonumber\\
ProductionRule_NP->NP,,,SBAR, & 0.99997 \nonumber\\
ProductionRule_PP->IN,UCP, & 0.99997 \nonumber\\
because_she & 0.99997 \nonumber\\
._indium & 0.99997 \nonumber\\
son & 0.99997 \nonumber\\
a_whole & 0.99997 \nonumber\\
say_it & 0.99997 \nonumber\\
acceptable_. & 0.99997 \nonumber\\
and_feel & 0.99997 \nonumber\\
ProductionRule_SQ->VBZ,NP, & 0.99997 \nonumber\\
that_he & 0.99997 \nonumber\\
to_hard & 0.99997 \nonumber\\
college & 0.99997 \nonumber\\
_pos_ngram_NN_CARD_PP & 0.99997 \nonumber\\
he_make & 0.99997 \nonumber\\
fetus & 0.99997 \nonumber\\
just_not & 0.99997 \nonumber\\
solution & 0.99997 \nonumber\\
kid_that & 0.99997 \nonumber\\
bring_up & 0.99997 \nonumber\\
waste_and & 0.99997 \nonumber\\
those_of & 0.99997 \nonumber\\
water_would & 0.99997 \nonumber\\
ProductionRule_VP->VBP,RB,NP, & 0.99997 \nonumber\\
business & 0.99997 \nonumber\\
wonder_about & 0.99997 \nonumber\\
._mainly & 0.99997 \nonumber\\
about_your & 0.99997 \nonumber\\
everyday & 0.99997 \nonumber\\
ProductionRule_NP->NP,., & 0.99997 \nonumber\\
ProductionRule_ADVP->RBR,PP, & 0.99997 \nonumber\\
people_ca & 0.99997 \nonumber\\
_pos_ngram_O_NN_PUNC & 0.99997 \nonumber\\
creativity & 0.99997 \nonumber\\
bring_some & 0.99997 \nonumber\\
trader_in & 0.99997 \nonumber\\
the_trader & 0.99997 \nonumber\\
necessity & 0.99997 \nonumber\\
farquhar_order & 0.99997 \nonumber\\
malacca_and & 0.99997 \nonumber\\
singapore_also & 0.99997 \nonumber\\
to_malacca & 0.99997 \nonumber\\
some_food & 0.99997 \nonumber\\
the_necessity & 0.99997 \nonumber\\
also_bring & 0.99997 \nonumber\\
food_back & 0.99997 \nonumber\\
necessity_here & 0.99997 \nonumber\\
his_man & 0.99997 \nonumber\\
order_his & 0.99997 \nonumber\\
for_evolution & 0.99997 \nonumber\\
your_eye & 0.99997 \nonumber\\
to_develop & 0.99997 \nonumber\\
._like & 0.99997 \nonumber\\
_pos_ngram_ADV_CONJ_ADV & 0.99997 \nonumber\\
'_wrong & 0.99997 \nonumber\\
my_own & 0.99997 \nonumber\\
"_yes & 0.99997 \nonumber\\
theory_. & 0.99997 \nonumber\\
ProductionRule_VP->VBP,S,,,SBAR, & 0.99997 \nonumber\\
something_like & 0.99997 \nonumber\\
point_be & 0.99997 \nonumber\\
ProductionRule_VP->VB,NP,PP,,,SBAR, & 0.99997 \nonumber\\
the_government & 0.99997 \nonumber\\
figure_out & 0.99997 \nonumber\\
yourself_first & 0.99997 \nonumber\\
to_fight & 0.99997 \nonumber\\
spank_. & 0.99997 \nonumber\\
can_kill & 0.99997 \nonumber\\
an_opinion & 0.99997 \nonumber\\
own_, & 0.99997 \nonumber\\
come_people & 0.99997 \nonumber\\
n't_still & 0.99997 \nonumber\\
other_and & 0.99997 \nonumber\\
of_my & 0.99997 \nonumber\\
beyond & 0.99997 \nonumber\\
ProductionRule_NP->JJ,CC,JJ,NNS, & 0.99997 \nonumber\\
say_you & 0.99997 \nonumber\\
uniform_do & 0.99997 \nonumber\\
as_it & 0.99997 \nonumber\\
father_his & 0.99997 \nonumber\\
you_no & 0.99997 \nonumber\\
can_tell & 0.99997 \nonumber\\
tell_yourself & 0.99997 \nonumber\\
can_still & 0.99997 \nonumber\\
his_go & 0.99997 \nonumber\\
still_learn & 0.99997 \nonumber\\
better_" & 0.99997 \nonumber\\
maybe_you & 0.99997 \nonumber\\
_pos_ngram_PP_CARD_V & 0.99997 \nonumber\\
._how & 0.99997 \nonumber\\
than_the & 0.99997 \nonumber\\
faster & 0.99997 \nonumber\\
obviously & 0.99997 \nonumber\\
put_it & 0.99997 \nonumber\\
count & 0.99997 \nonumber\\
of_me & 0.99997 \nonumber\\
student_look & 0.99997 \nonumber\\
resource_, & 0.99997 \nonumber\\
do_so & 0.99997 \nonumber\\
h-school & 0.99997 \nonumber\\
petition & 0.99997 \nonumber\\
for_uniform & 0.99997 \nonumber\\
actually_this & 0.99997 \nonumber\\
sign_for & 0.99997 \nonumber\\
h-school_be & 0.99997 \nonumber\\
gay_! & 0.99997 \nonumber\\
my_h-school & 0.99997 \nonumber\\
just_experience & 0.99997 \nonumber\\
experience_... & 0.99997 \nonumber\\
their_gay & 0.99997 \nonumber\\
gay_but & 0.99997 \nonumber\\
petition_sign & 0.99997 \nonumber\\
a_petition & 0.99997 \nonumber\\
!_actually & 0.99997 \nonumber\\
beat_the & 0.99997 \nonumber\\
i_go & 0.99997 \nonumber\\
like_be & 0.99997 \nonumber\\
the_solution & 0.99997 \nonumber\\
use_electricity & 0.99997 \nonumber\\
peace & 0.99997 \nonumber\\
abuse_, & 0.99997 \nonumber\\
hand_, & 0.99997 \nonumber\\
student_to & 0.99997 \nonumber\\
individual & 0.99997 \nonumber\\
know_for & 0.99997 \nonumber\\
only_for & 0.99997 \nonumber\\
ProductionRule_VP->VP,CONJP,VP, & 0.99997 \nonumber\\
ProductionRule_NP->JJ,NN,SBAR, & 0.99997 \nonumber\\
_pos_ngram_ADJ_NN_NN & 0.99997 \nonumber\\
this_recession & 0.99997 \nonumber\\
culture_, & 0.99997 \nonumber\\
browser_. & 0.99997 \nonumber\\
disapointment_. & 0.99997 \nonumber\\
disapointment & 0.99997 \nonumber\\
personally_feel & 0.99997 \nonumber\\
personally_know & 0.99997 \nonumber\\
very_lousy & 0.99997 \nonumber\\
n't_bother & 0.99997 \nonumber\\
n't_hear & 0.99997 \nonumber\\
around_i & 0.99997 \nonumber\\
since_. & 0.99997 \nonumber\\
i_hav & 0.99997 \nonumber\\
him_since & 0.99997 \nonumber\\
thirteen_, & 0.99997 \nonumber\\
any_disapointment & 0.99997 \nonumber\\
be_thirteen & 0.99997 \nonumber\\
hear_from & 0.99997 \nonumber\\
never_set & 0.99997 \nonumber\\
twice & 0.99997 \nonumber\\
who_know & 0.99997 \nonumber\\
the_message & 0.99997 \nonumber\\
ProductionRule_ADVP->ADVP,S, & 0.99997 \nonumber\\
constantly_but & 0.99997 \nonumber\\
across_to & 0.99997 \nonumber\\
message_across & 0.99997 \nonumber\\
_pos_ngram_PP_ADV_ADJ & 0.99997 \nonumber\\
marry_in & 0.99997 \nonumber\\
_pos_ngram_CONJ_NN_ART & 0.99997 \nonumber\\
n't_a & 0.99997 \nonumber\\
be_degrade & 0.99997 \nonumber\\
have_sexual & 0.99998 \nonumber\\
sexual_desire & 0.99998 \nonumber\\
in_him & 0.99998 \nonumber\\
bright_and & 0.99998 \nonumber\\
a_lously & 0.99998 \nonumber\\
;_mean & 0.99998 \nonumber\\
ProductionRule_VP->VBG,PRT,S, & 0.99998 \nonumber\\
be_greatness & 0.99998 \nonumber\\
or_good & 0.99998 \nonumber\\
about_who & 0.99998 \nonumber\\
greatness & 0.99998 \nonumber\\
greatness_in & 0.99998 \nonumber\\
at_or & 0.99998 \nonumber\\
;_because & 0.99998 \nonumber\\
lousy_at & 0.99998 \nonumber\\
lously_father & 0.99998 \nonumber\\
up_be & 0.99998 \nonumber\\
lously & 0.99998 \nonumber\\
also_grow & 0.99998 \nonumber\\
,_wonder & 0.99998 \nonumber\\
the_son & 0.99998 \nonumber\\
father_; & 0.99998 \nonumber\\
and_better & 0.99998 \nonumber\\
at_. & 0.99998 \nonumber\\
_pos_ngram_PP_CONJ_ADJ & 0.99998 \nonumber\\
your_childhood.meaning & 0.99998 \nonumber\\
childhood.meaning & 0.99998 \nonumber\\
major_impact & 0.99998 \nonumber\\
him_; & 0.99998 \nonumber\\
who_your & 0.99998 \nonumber\\
childhood.meaning_, & 0.99998 \nonumber\\
ProductionRule_SBAR->SBAR,:,SBAR, & 0.99998 \nonumber\\
son_he & 0.99998 \nonumber\\
make_turn & 0.99998 \nonumber\\
because_grow & 0.99998 \nonumber\\
a_bright & 0.99998 \nonumber\\
"_how & 0.99998 \nonumber\\
me_not & 0.99998 \nonumber\\
_pos_ngram_NP_ADV_PP & 0.99998 \nonumber\\
child_their & 0.99998 \nonumber\\
their_gon & 0.99998 \nonumber\\
na_think & 0.99998 \nonumber\\
we_hit & 0.99998 \nonumber\\
hit_our & 0.99998 \nonumber\\
ProductionRule_S->NP,NP,S, & 0.99998 \nonumber\\
ProductionRule_ADVP->DT,PP, & 0.99998 \nonumber\\
love_them & 0.99998 \nonumber\\
bible_bullshit & 0.99998 \nonumber\\
one_gad & 0.99998 \nonumber\\
empirical & 0.99998 \nonumber\\
shred_of & 0.99998 \nonumber\\
priorus & 0.99998 \nonumber\\
bullshit_. & 0.99998 \nonumber\\
christianity_with & 0.99998 \nonumber\\
discredit & 0.99998 \nonumber\\
discredit_all & 0.99998 \nonumber\\
see_one & 0.99998 \nonumber\\
believe_christianity & 0.99998 \nonumber\\
priorus_argument & 0.99998 \nonumber\\
disprove_all & 0.99998 \nonumber\\
be_illogical & 0.99998 \nonumber\\
notmymuse & 0.99998 \nonumber\\
contrary_. & 0.99998 \nonumber\\
this_bible & 0.99998 \nonumber\\
contrary & 0.99998 \nonumber\\
evidence_against & 0.99998 \nonumber\\
evidence_for & 0.99998 \nonumber\\
argument_against & 0.99998 \nonumber\\
with_empirical & 0.99998 \nonumber\\
fact_( & 0.99998 \nonumber\\
one_logical & 0.99998 \nonumber\\
mountain & 0.99998 \nonumber\\
gad & 0.99998 \nonumber\\
gad_damn & 0.99998 \nonumber\\
see_mountain & 0.99998 \nonumber\\
solid_priorus & 0.99998 \nonumber\\
have_also & 0.99998 \nonumber\\
christianity_. & 0.99998 \nonumber\\
against_christianity & 0.99998 \nonumber\\
illogical_to & 0.99998 \nonumber\\
yet_to & 0.99998 \nonumber\\
mountain_of & 0.99998 \nonumber\\
until_such & 0.99998 \nonumber\\
have_discredit & 0.99998 \nonumber\\
,_create & 0.99998 \nonumber\\
argument_) & 0.99998 \nonumber\\
_pos_ngram_PR_CARD_ADJ & 0.99998 \nonumber\\
shred & 0.99998 \nonumber\\
a_damn & 0.99998 \nonumber\\
me_one & 0.99998 \nonumber\\
._- & 0.99998 \nonumber\\
,_disprove & 0.99998 \nonumber\\
the_contrary & 0.99998 \nonumber\\
notmymuse_, & 0.99998 \nonumber\\
once_you & 0.99998 \nonumber\\
logical_reason & 0.99998 \nonumber\\
logical_argument & 0.99998 \nonumber\\
-_until & 0.99998 \nonumber\\
damn_shred & 0.99998 \nonumber\\
damn_solid & 0.99998 \nonumber\\
all_logical & 0.99998 \nonumber\\
empirical_fact & 0.99998 \nonumber\\
make_decision & 0.99998 \nonumber\\
evolution_be & 0.99998 \nonumber\\
like_it & 0.99998 \nonumber\\
that_there & 0.99998 \nonumber\\
you_become & 0.99998 \nonumber\\
._would & 0.99998 \nonumber\\
with_their & 0.99998 \nonumber\\
be_she & 0.99998 \nonumber\\
simple_, & 0.99998 \nonumber\\
have_have & 0.99998 \nonumber\\
guideline & 0.99998 \nonumber\\
save_the & 0.99998 \nonumber\\
theist & 0.99998 \nonumber\\
container & 0.99998 \nonumber\\
ProductionRule_S->NP,NP,VP, & 0.99998 \nonumber\\
ed & 0.99998 \nonumber\\
phy & 0.99998 \nonumber\\
understand_they & 0.99998 \nonumber\\
likely_that & 0.99998 \nonumber\\
your_side & 0.99998 \nonumber\\
_pos_ngram_O_CONJ_ART & 0.99998 \nonumber\\
it_once & 0.99998 \nonumber\\
have_my & 0.99998 \nonumber\\
_pos_ngram_V_CONJ_O & 0.99998 \nonumber\\
ProductionRule_VP->VBD,ADJP,PP, & 0.99998 \nonumber\\
which_the & 0.99998 \nonumber\\
act_, & 0.99998 \nonumber\\
the_choice & 0.99998 \nonumber\\
almost_the & 0.99998 \nonumber\\
only_difference & 0.99998 \nonumber\\
as_book & 0.99998 \nonumber\\
actually_have & 0.99998 \nonumber\\
to_move & 0.99998 \nonumber\\
difference_be & 0.99998 \nonumber\\
move_your & 0.99998 \nonumber\\
eye_for & 0.99998 \nonumber\\
exact_same & 0.99998 \nonumber\\
ProductionRule_S->PRN,NP,ADVP,VP, & 0.99998 \nonumber\\
ProductionRule_VP->VBD,SBAR, & 0.99998 \nonumber\\
_pos_ngram_PUNC_O_PP & 0.99998 \nonumber\\
it_happen & 0.99998 \nonumber\\
farquhar_be & 0.99998 \nonumber\\
desire_, & 0.99998 \nonumber\\
water_for & 0.99998 \nonumber\\
but_raffle & 0.99998 \nonumber\\
be_come & 0.99998 \nonumber\\
means_the & 0.99998 \nonumber\\
_pos_ngram_CONJ_O_NN & 0.99998 \nonumber\\
disprove & 0.99998 \nonumber\\
should_use & 0.99998 \nonumber\\
as_equal & 0.99998 \nonumber\\
hit_me & 0.99998 \nonumber\\
treat_as & 0.99998 \nonumber\\
lol_i & 0.99998 \nonumber\\
my_child & 0.99998 \nonumber\\
equal_lol & 0.99998 \nonumber\\
_pos_ngram_ADV_PUNC_O & 0.99998 \nonumber\\
but_only & 0.99998 \nonumber\\
_pos_ngram_V_NP_CONJ & 0.99998 \nonumber\\
last_source & 0.99998 \nonumber\\
ProductionRule_VP->VBN,UCP, & 0.99998 \nonumber\\
hard_. & 0.99998 \nonumber\\
source_and & 0.99998 \nonumber\\
agree_but & 0.99998 \nonumber\\
ProductionRule_ADVP->RB,TO,RB, & 0.99998 \nonumber\\
and_of & 0.99998 \nonumber\\
ProductionRule_VP->PP,ADVP, & 0.99998 \nonumber\\
constantly_and & 0.99998 \nonumber\\
porn_and & 0.99998 \nonumber\\
n't_turn & 0.99998 \nonumber\\
_pos_ngram_V_O_CONJ & 0.99998 \nonumber\\
'_my & 0.99998 \nonumber\\
population & 0.99998 \nonumber\\
find_in & 0.99998 \nonumber\\
be_people & 0.99998 \nonumber\\
would_mean & 0.99998 \nonumber\\
spank_because & 0.99998 \nonumber\\
themselve & 0.99998 \nonumber\\
like_him & 0.99998 \nonumber\\
course_not & 0.99998 \nonumber\\
absence & 0.99998 \nonumber\\
circumstance & 0.99998 \nonumber\\
uniform_and & 0.99998 \nonumber\\
son_or & 0.99998 \nonumber\\
_pos_ngram_CONJ_ADV_ART & 0.99998 \nonumber\\
chaos & 0.99998 \nonumber\\
chaos_. & 0.99998 \nonumber\\
ProductionRule_NP->NN,., & 0.99998 \nonumber\\
ProductionRule_VP->VB,S,PP, & 0.99998 \nonumber\\
_pos_ngram_O_O_NN & 0.99998 \nonumber\\
unnatural & 0.99998 \nonumber\\
eat_too & 0.99998 \nonumber\\
kid_need & 0.99998 \nonumber\\
in_firefox & 0.99998 \nonumber\\
normal_. & 0.99998 \nonumber\\
ProductionRule_VP->VB,NP,,,UCP, & 0.99998 \nonumber\\
actually_, & 0.99998 \nonumber\\
._student & 0.99998 \nonumber\\
creature_mate & 0.99998 \nonumber\\
mate_with & 0.99998 \nonumber\\
just_unnatural & 0.99998 \nonumber\\
all_sexual & 0.99998 \nonumber\\
mate & 0.99998 \nonumber\\
unnatural_because & 0.99998 \nonumber\\
sexual_creature & 0.99998 \nonumber\\
because_all & 0.99998 \nonumber\\
opposite_sex & 0.99998 \nonumber\\
couple_in & 0.99998 \nonumber\\
desire_of & 0.99998 \nonumber\\
..._to & 0.99998 \nonumber\\
base_desire & 0.99998 \nonumber\\
evolve_because & 0.99998 \nonumber\\
right_be & 0.99998 \nonumber\\
of_moral & 0.99998 \nonumber\\
and_religious & 0.99998 \nonumber\\
state_... & 0.99998 \nonumber\\
debase_marriage & 0.99998 \nonumber\\
to_accomodate & 0.99998 \nonumber\\
debase & 0.99998 \nonumber\\
to_debase & 0.99998 \nonumber\\
disguise_if & 0.99998 \nonumber\\
stupid_... & 0.99998 \nonumber\\
grounds_rather & 0.99998 \nonumber\\
marriage_evolve & 0.99998 \nonumber\\
disguise & 0.99998 \nonumber\\
grounds & 0.99998 \nonumber\\
religious_grounds & 0.99998 \nonumber\\
union_approve & 0.99998 \nonumber\\
accomodate_base & 0.99998 \nonumber\\
simply_stupid & 0.99998 \nonumber\\
accomodate & 0.99998 \nonumber\\
mere_union & 0.99998 \nonumber\\
in_disguise & 0.99998 \nonumber\\
ProductionRule_VP->VBD,PP,:,S, & 0.99998 \nonumber\\
since_i & 0.99998 \nonumber\\
for_not & 0.99998 \nonumber\\
to_her & 0.99998 \nonumber\\
use_of & 0.99998 \nonumber\\
ProductionRule_S->INTJ,NP,VP, & 0.99998 \nonumber\\
rat & 0.99998 \nonumber\\
more_to & 0.99998 \nonumber\\
_pos_ngram_V_PR_CARD & 0.99998 \nonumber\\
dont_have & 0.99998 \nonumber\\
n't_love & 0.99998 \nonumber\\
opinion_, & 0.99998 \nonumber\\
ProductionRule_NP->PRP$,NN,POS, & 0.99998 \nonumber\\
wrong_but & 0.99998 \nonumber\\
ready_to & 0.99998 \nonumber\\
okay & 0.99998 \nonumber\\
to_come & 0.99998 \nonumber\\
crime_. & 0.99998 \nonumber\\
will_think & 0.99998 \nonumber\\
your_kid & 0.99998 \nonumber\\
_pos_ngram_V_CONJ_CARD & 0.99998 \nonumber\\
process & 0.99998 \nonumber\\
,_its & 0.99998 \nonumber\\
our_religion & 0.99998 \nonumber\\
risk & 0.99998 \nonumber\\
_pos_ngram_CONJ_NP_ADV & 0.99998 \nonumber\\
_pos_ngram_ART_ADV_NN & 0.99998 \nonumber\\
tap_water & 0.99998 \nonumber\\
tap & 0.99998 \nonumber\\
out_in & 0.99998 \nonumber\\
it_without & 0.99998 \nonumber\\
their_moral & 0.99998 \nonumber\\
argument_? & 0.99998 \nonumber\\
._can & 0.99998 \nonumber\\
a_profitable & 0.99998 \nonumber\\
entertainment_for & 0.99998 \nonumber\\
nobody_. & 0.99998 \nonumber\\
inject_their & 0.99998 \nonumber\\
inject & 0.99998 \nonumber\\
without_inject & 0.99998 \nonumber\\
moral_standard & 0.99998 \nonumber\\
really_tell & 0.99998 \nonumber\\
can_somebody & 0.99998 \nonumber\\
profitable_source & 0.99998 \nonumber\\
profitable & 0.99998 \nonumber\\
kill_nobody & 0.99998 \nonumber\\
somebody_really & 0.99998 \nonumber\\
porn_kill & 0.99998 \nonumber\\
some_. & 0.99998 \nonumber\\
standard_into & 0.99998 \nonumber\\
"_or & 0.99998 \nonumber\\
better_then & 0.99998 \nonumber\\
be_if & 0.99998 \nonumber\\
not_only & 0.99998 \nonumber\\
be_alone & 0.99998 \nonumber\\
as_they & 0.99998 \nonumber\\
care_what & 0.99998 \nonumber\\
fish & 0.99998 \nonumber\\
not_lead & 0.99998 \nonumber\\
christian_and & 0.99998 \nonumber\\
reagan & 0.99998 \nonumber\\
reagan_once & 0.99998 \nonumber\\
this_notice & 0.99998 \nonumber\\
once_say & 0.99998 \nonumber\\
choice_have & 0.99998 \nonumber\\
life_reagan & 0.99998 \nonumber\\
not_right & 0.99998 \nonumber\\
it_get & 0.99998 \nonumber\\
unless & 0.99998 \nonumber\\
,_however & 0.99998 \nonumber\\
help_, & 0.99998 \nonumber\\
be_likely & 0.99998 \nonumber\\
find_, & 0.99998 \nonumber\\
learn_lesson & 0.99998 \nonumber\\
them_!! & 0.99998 \nonumber\\
definitely_say & 0.99998 \nonumber\\
n't_spank & 0.99998 \nonumber\\
spank_when & 0.99998 \nonumber\\
though_with & 0.99998 \nonumber\\
with_whatever & 0.99998 \nonumber\\
kid_though & 0.99998 \nonumber\\
while_. & 0.99998 \nonumber\\
little_but & 0.99998 \nonumber\\
could_definitely & 0.99998 \nonumber\\
kill_them & 0.99998 \nonumber\\
should_make & 0.99998 \nonumber\\
ProductionRule_PP->IN,``,NP, & 0.99998 \nonumber\\
like_i & 0.99998 \nonumber\\
adult & 0.99998 \nonumber\\
illegal_to & 0.99998 \nonumber\\
but_also & 0.99998 \nonumber\\
"_. & 0.99998 \nonumber\\
ruin & 0.99998 \nonumber\\
agriculture & 0.99998 \nonumber\\
continent_have & 0.99998 \nonumber\\
industry_date & 0.99998 \nonumber\\
agriculture_and & 0.99998 \nonumber\\
continent & 0.99998 \nonumber\\
almost_50 & 0.99998 \nonumber\\
'_bottle & 0.99998 \nonumber\\
the_continent & 0.99998 \nonumber\\
water_due & 0.99998 \nonumber\\
pollute_water & 0.99998 \nonumber\\
many_claim & 0.99998 \nonumber\\
very_pollute & 0.99998 \nonumber\\
consume_almost & 0.99998 \nonumber\\
to_european & 0.99998 \nonumber\\
european & 0.99998 \nonumber\\
europe_consume & 0.99998 \nonumber\\
buy_help & 0.99998 \nonumber\\
bottle_they & 0.99998 \nonumber\\
they_buy & 0.99998 \nonumber\\
have_very & 0.99998 \nonumber\\
and_industry & 0.99998 \nonumber\\
european_culture & 0.99998 \nonumber\\
to_agriculture & 0.99998 \nonumber\\
date_back & 0.99998 \nonumber\\
help_you & 0.99998 \nonumber\\
and_woman & 0.99998 \nonumber\\
chance & 0.99998 \nonumber\\
remember & 0.99998 \nonumber\\
for_each & 0.99998 \nonumber\\
how_do & 0.99998 \nonumber\\
ask_you & 0.99998 \nonumber\\
a_common & 0.99998 \nonumber\\
a_kid & 0.99998 \nonumber\\
that_parent & 0.99998 \nonumber\\
be_simply & 0.99998 \nonumber\\
spank_should & 0.99998 \nonumber\\
who_kill & 0.99998 \nonumber\\
n't_work & 0.99998 \nonumber\\
ProductionRule_NP->FW,FW,FW,FW,FW, & 0.99998 \nonumber\\
back_. & 0.99998 \nonumber\\
a_pregnant & 0.99998 \nonumber\\
know_nothing & 0.99998 \nonumber\\
result & 0.99998 \nonumber\\
be_abuse & 0.99998 \nonumber\\
be_provide & 0.99998 \nonumber\\
individual_should & 0.99998 \nonumber\\
decision_of & 0.99998 \nonumber\\
what_an & 0.99998 \nonumber\\
_pos_ngram_O_O_ART & 0.99998 \nonumber\\
out_and & 0.99998 \nonumber\\
grammar & 0.99998 \nonumber\\
police_, & 0.99998 \nonumber\\
position & 0.99998 \nonumber\\
can_take & 0.99998 \nonumber\\
ProductionRule_UCP->VP,CC,ADJP, & 0.99998 \nonumber\\
to_porn & 0.99998 \nonumber\\
would_try & 0.99998 \nonumber\\
person_out & 0.99998 \nonumber\\
but_hey & 0.99998 \nonumber\\
with_atheism & 0.99998 \nonumber\\
and_very & 0.99998 \nonumber\\
the_description & 0.99998 \nonumber\\
the_qualify & 0.99998 \nonumber\\
qualify_factor & 0.99998 \nonumber\\
n't_christian & 0.99998 \nonumber\\
description & 0.99998 \nonumber\\
very_religious & 0.99998 \nonumber\\
description_of & 0.99998 \nonumber\\
and_tell & 0.99998 \nonumber\\
who_" & 0.99998 \nonumber\\
._since & 0.99998 \nonumber\\
they_look & 0.99998 \nonumber\\
feed & 0.99998 \nonumber\\
all_human & 0.99998 \nonumber\\
ProductionRule_S->NP,,,VP, & 0.99998 \nonumber\\
'_singapore & 0.99998 \nonumber\\
spare & 0.99998 \nonumber\\
singapura_, & 0.99998 \nonumber\\
majulah & 0.99998 \nonumber\\
should_he & 0.99998 \nonumber\\
spare_a & 0.99998 \nonumber\\
he_deserve & 0.99998 \nonumber\\
he_discover & 0.99998 \nonumber\\
'_founder & 0.99998 \nonumber\\
singapura & 0.99998 \nonumber\\
the_citizen & 0.99998 \nonumber\\
?_farquhar & 0.99998 \nonumber\\
why_in & 0.99998 \nonumber\\
a_think & 0.99998 \nonumber\\
idea_contribute & 0.99998 \nonumber\\
develop_the & 0.99998 \nonumber\\
founder_' & 0.99998 \nonumber\\
majulah_singapura & 0.99998 \nonumber\\
think_at & 0.99998 \nonumber\\
all_his & 0.99998 \nonumber\\
island_majulah & 0.99998 \nonumber\\
n't_spare & 0.99998 \nonumber\\
title_of & 0.99998 \nonumber\\
our_selfe & 0.99998 \nonumber\\
we_really & 0.99998 \nonumber\\
adult_be & 0.99998 \nonumber\\
a_stupid & 0.99998 \nonumber\\
stupid_uniform & 0.99998 \nonumber\\
._adult & 0.99998 \nonumber\\
selfe & 0.99998 \nonumber\\
school_!! & 0.99998 \nonumber\\
selfe_and & 0.99998 \nonumber\\
express_who & 0.99998 \nonumber\\
alway_tell & 0.99998 \nonumber\\
while_wear & 0.99998 \nonumber\\
cant_do & 0.99998 \nonumber\\
action_by & 0.99998 \nonumber\\
do_wrong & 0.99998 \nonumber\\
figure_in & 0.99998 \nonumber\\
_pos_ngram_ADJ_CONJ_CARD & 0.99998 \nonumber\\
attention & 0.99998 \nonumber\\
._an & 0.99998 \nonumber\\
of_do & 0.99998 \nonumber\\
_pos_ngram_ADJ_PP_CARD & 0.99998 \nonumber\\
must_have & 0.99998 \nonumber\\
_pos_ngram_PR_PR_PR & 0.99998 \nonumber\\
with_all & 0.99998 \nonumber\\
provide_. & 0.99998 \nonumber\\
ProductionRule_WHADVP->WRB,NP, & 0.99998 \nonumber\\
personal_relationship & 0.99998 \nonumber\\
christ_. & 0.99998 \nonumber\\
with_christ & 0.99998 \nonumber\\
unfit & 0.99998 \nonumber\\
body & 0.99998 \nonumber\\
._once & 0.99998 \nonumber\\
just_be & 0.99998 \nonumber\\
"_a & 0.99998 \nonumber\\
husband_murder & 0.99998 \nonumber\\
consequence_of & 0.99998 \nonumber\\
consequence_for & 0.99998 \nonumber\\
a_consequence & 0.99998 \nonumber\\
every_act & 0.99998 \nonumber\\
of_commit & 0.99998 \nonumber\\
the_girl & 0.99998 \nonumber\\
_pos_ngram_NP_NP_CONJ & 0.99998 \nonumber\\
someone_i & 0.99998 \nonumber\\
_pos_ngram_ART_ADJ_CONJ & 0.99998 \nonumber\\
of_record & 0.99998 \nonumber\\
it_down & 0.99998 \nonumber\\
have_actually & 0.99998 \nonumber\\
baby_. & 0.99998 \nonumber\\
strong & 0.99998 \nonumber\\
it_because & 0.99998 \nonumber\\
alway_better & 0.99998 \nonumber\\
firm & 0.99998 \nonumber\\
who_commit & 0.99998 \nonumber\\
him_and & 0.99998 \nonumber\\
"_then & 0.99998 \nonumber\\
do_occur & 0.99998 \nonumber\\
the_way & 0.99998 \nonumber\\
personal_goal & 0.99998 \nonumber\\
of_that & 0.99998 \nonumber\\
class & 0.99998 \nonumber\\
die_, & 0.99998 \nonumber\\
a_couch & 0.99998 \nonumber\\
know_should & 0.99998 \nonumber\\
content & 0.99998 \nonumber\\
in_pornographic & 0.99998 \nonumber\\
watch_you & 0.99998 \nonumber\\
even_know & 0.99998 \nonumber\\
content_. & 0.99998 \nonumber\\
pornographic_content & 0.99998 \nonumber\\
pornographic & 0.99998 \nonumber\\
mean_people & 0.99998 \nonumber\\
though_human & 0.99998 \nonumber\\
personally_i & 0.99998 \nonumber\\
would_give & 0.99998 \nonumber\\
majority_of & 0.99998 \nonumber\\
majority & 0.99998 \nonumber\\
our_school & 0.99998 \nonumber\\
opportunity & 0.99998 \nonumber\\
opportunity_to & 0.99998 \nonumber\\
in_it & 0.99998 \nonumber\\
industrial & 0.99998 \nonumber\\
throw & 0.99998 \nonumber\\
matter_of & 0.99998 \nonumber\\
a_matter & 0.99998 \nonumber\\
that_prove & 0.99998 \nonumber\\
exist_. & 0.99998 \nonumber\\
the_abortion & 0.99998 \nonumber\\
also_cost & 0.99998 \nonumber\\
_pos_ngram_O_NN_V & 0.99998 \nonumber\\
and_make & 0.99998 \nonumber\\
ProductionRule_VP->VB,S,SBAR, & 0.99998 \nonumber\\
other_people & 0.99998 \nonumber\\
discover_the & 0.99998 \nonumber\\
influence_. & 0.99998 \nonumber\\
ancient & 0.99998 \nonumber\\
feature & 0.99998 \nonumber\\
but_be & 0.99998 \nonumber\\
with_you & 0.99998 \nonumber\\
..._what & 0.99998 \nonumber\\
good_and & 0.99998 \nonumber\\
_pos_ngram_CARD_PUNC_V & 0.99998 \nonumber\\
have_yet & 0.99998 \nonumber\\
_pos_ngram_CONJ_NN_ADJ & 0.99998 \nonumber\\
and_see & 0.99998 \nonumber\\
use_their & 0.99998 \nonumber\\
fame & 0.99998 \nonumber\\
,_fame & 0.99998 \nonumber\\
._from & 0.99998 \nonumber\\
_pos_ngram_ART_PR_NN & 0.99998 \nonumber\\
,_the & 0.99998 \nonumber\\
honestly_, & 0.99998 \nonumber\\
them_, & 0.99998 \nonumber\\
while_i & 0.99998 \nonumber\\
let_them & 0.99998 \nonumber\\
_pos_ngram_NN_NP_V & 0.99998 \nonumber\\
_pos_ngram_PUNC_ADJ_ADJ & 0.99998 \nonumber\\
physical & 0.99998 \nonumber\\
my_point & 0.99998 \nonumber\\
with_. & 0.99998 \nonumber\\
n't_tell & 0.99998 \nonumber\\
satisfy & 0.99998 \nonumber\\
be_our & 0.99998 \nonumber\\
live_. & 0.99998 \nonumber\\
(_to & 0.99998 \nonumber\\
yourself_in & 0.99998 \nonumber\\
and_everyone & 0.99998 \nonumber\\
point_further & 0.99998 \nonumber\\
useful_' & 0.99998 \nonumber\\
raffle_all & 0.99998 \nonumber\\
up_badly & 0.99998 \nonumber\\
conquer & 0.99998 \nonumber\\
to_settle & 0.99998 \nonumber\\
all_end & 0.99998 \nonumber\\
ProductionRule_ADJP->JJ,'', & 0.99998 \nonumber\\
for_about & 0.99998 \nonumber\\
he_go & 0.99998 \nonumber\\
country_that & 0.99998 \nonumber\\
about_four & 0.99998 \nonumber\\
leave_all & 0.99998 \nonumber\\
raffle_neglect & 0.99998 \nonumber\\
'_country & 0.99998 \nonumber\\
four & 0.99998 \nonumber\\
developer_of & 0.99998 \nonumber\\
badly & 0.99998 \nonumber\\
ProductionRule_VP->VBD,NP,PP,,,S, & 0.99998 \nonumber\\
four_year & 0.99998 \nonumber\\
conquer_other & 0.99998 \nonumber\\
singapore_when & 0.99998 \nonumber\\
to_drive & 0.99998 \nonumber\\
run_by & 0.99998 \nonumber\\
drive_my & 0.99998 \nonumber\\
settle & 0.99998 \nonumber\\
settle_. & 0.99998 \nonumber\\
around_conquer & 0.99998 \nonumber\\
badly_. & 0.99998 \nonumber\\
world_while & 0.99998 \nonumber\\
tiny & 0.99998 \nonumber\\
_pos_ngram_PP_CARD_PR & 0.99998 \nonumber\\
ProductionRule_NP->DT,CD, & 0.99998 \nonumber\\
successful & 0.99998 \nonumber\\
orientation & 0.99998 \nonumber\\
sexual_orientation & 0.99998 \nonumber\\
any_money & 0.99998 \nonumber\\
how_porn & 0.99998 \nonumber\\
wrong_be & 0.99998 \nonumber\\
king_way & 0.99998 \nonumber\\
yous & 0.99998 \nonumber\\
yous_any & 0.99998 \nonumber\\
:_l & 0.99998 \nonumber\\
the_yes & 0.99998 \nonumber\\
money_that & 0.99998 \nonumber\\
a_f & 0.99998 \nonumber\\
whatever_? & 0.99998 \nonumber\\
yes_argument & 0.99998 \nonumber\\
virgin_: & 0.99998 \nonumber\\
be_virgin & 0.99998 \nonumber\\
bet_yous & 0.99998 \nonumber\\
?_porn & 0.99998 \nonumber\\
ProductionRule_FRAG->WHNP,., & 0.99998 \nonumber\\
friend & 0.99998 \nonumber\\
as_to & 0.99998 \nonumber\\
dad_be & 0.99998 \nonumber\\
the_bottle & 0.99998 \nonumber\\
ProductionRule_NP->PRP$,JJ,JJ,NN, & 0.99998 \nonumber\\
2006_, & 0.99998 \nonumber\\
2006 & 0.99998 \nonumber\\
in_2006 & 0.99998 \nonumber\\
follow_the & 0.99998 \nonumber\\
_pos_ngram_PR_PR_ADV & 0.99998 \nonumber\\
._which & 0.99998 \nonumber\\
ProductionRule_NP->NNP,NNS, & 0.99998 \nonumber\\
a_certain & 0.99998 \nonumber\\
really_know & 0.99998 \nonumber\\
which_one & 0.99998 \nonumber\\
at_the & 0.99998 \nonumber\\
key & 0.99998 \nonumber\\
like_physical & 0.99998 \nonumber\\
however_be & 0.99998 \nonumber\\
it_that & 0.99998 \nonumber\\
_pos_ngram_PUNC_ADV_ADJ & 0.99998 \nonumber\\
:_) & 0.99998 \nonumber\\
because_some & 0.99998 \nonumber\\
tease & 0.99998 \nonumber\\
all_out & 0.99998 \nonumber\\
get_your & 0.99998 \nonumber\\
exactly & 0.99998 \nonumber\\
browser_in & 0.99998 \nonumber\\
_pos_ngram_ADJ_PUNC_O & 0.99998 \nonumber\\
recognition & 0.99998 \nonumber\\
break_. & 0.99998 \nonumber\\
trend & 0.99998 \nonumber\\
island_, & 0.99998 \nonumber\\
people_of & 0.99998 \nonumber\\
i_bet & 0.99998 \nonumber\\
bet & 0.99998 \nonumber\\
lousy_one & 0.99998 \nonumber\\
_pos_ngram_ADJ_ADJ_PP & 0.99998 \nonumber\\
_pos_ngram_CONJ_NN_CONJ & 0.99998 \nonumber\\
_pos_ngram_PR_V_O & 0.99998 \nonumber\\
so_far & 0.99998 \nonumber\\
atheist_. & 0.99998 \nonumber\\
evolution_do & 0.99998 \nonumber\\
di & 0.99998 \nonumber\\
to_christian & 0.99998 \nonumber\\
:_if & 0.99998 \nonumber\\
consult & 0.99998 \nonumber\\
source & 0.99998 \nonumber\\
_pos_ngram_PR_O_NN & 0.99998 \nonumber\\
for_another & 0.99998 \nonumber\\
william_farquhar & 0.99998 \nonumber\\
we_r & 0.99998 \nonumber\\
_pos_ngram_ADJ_CONJ_V & 0.99998 \nonumber\\
ProductionRule_FRAG->NP,., & 0.99998 \nonumber\\
should_get & 0.99998 \nonumber\\
believe_they & 0.99998 \nonumber\\
that_singapore & 0.99998 \nonumber\\
many_bid & 0.99998 \nonumber\\
not_get & 0.99998 \nonumber\\
_pos_ngram_PP_PUNC_PR & 0.99998 \nonumber\\
use_for & 0.99998 \nonumber\\
book_you & 0.99998 \nonumber\\
ProductionRule_NP->NP,:,NP, & 0.99998 \nonumber\\
bite_. & 0.99998 \nonumber\\
!_and & 0.99998 \nonumber\\
only_a & 0.99998 \nonumber\\
recession & 0.99998 \nonumber\\
ProductionRule_VP->VB,ADJP,PP,SBAR, & 0.99998 \nonumber\\
though_your & 0.99998 \nonumber\\
give_me & 0.99998 \nonumber\\
stuff & 0.99998 \nonumber\\
have_grow & 0.99998 \nonumber\\
_pos_ngram_NN_PP_CONJ & 0.99998 \nonumber\\
pregnancy & 0.99998 \nonumber\\
higher & 0.99998 \nonumber\\
be_too & 0.99998 \nonumber\\
_pos_ngram_V_CONJ_ART & 0.99998 \nonumber\\
n't_confide & 0.99998 \nonumber\\
spouse_of & 0.99998 \nonumber\\
they_turn & 0.99998 \nonumber\\
take_them & 0.99998 \nonumber\\
,_take & 0.99998 \nonumber\\
"_do & 0.99998 \nonumber\\
out_before & 0.99998 \nonumber\\
somebody_; & 0.99998 \nonumber\\
!_" & 0.99998 \nonumber\\
spouse_and & 0.99998 \nonumber\\
the_spouse & 0.99998 \nonumber\\
;_they & 0.99998 \nonumber\\
debate_, & 0.99998 \nonumber\\
ProductionRule_S->NP,,,``,VP, & 0.99998 \nonumber\\
they_find & 0.99998 \nonumber\\
prove_the & 0.99998 \nonumber\\
own_personal & 0.99998 \nonumber\\
from_the & 0.99998 \nonumber\\
any_other & 0.99998 \nonumber\\
EndingFul & 0.99998 \nonumber\\
_pos_ngram_ADV_ART_PR & 0.99998 \nonumber\\
ProductionRule_NP->JJ,NN,NNS, & 0.99998 \nonumber\\
in_no & 0.99998 \nonumber\\
would_prefer & 0.99998 \nonumber\\
n't_get & 0.99998 \nonumber\\
student_can & 0.99998 \nonumber\\
fire & 0.99998 \nonumber\\
make_mistake & 0.99998 \nonumber\\
so_. & 0.99998 \nonumber\\
_pos_ngram_O_ADJ_V & 0.99998 \nonumber\\
marry_and & 0.99998 \nonumber\\
_pos_ngram_CONJ_NP_PUNC & 0.99998 \nonumber\\
female & 0.99998 \nonumber\\
bible_be & 0.99998 \nonumber\\
almost_every & 0.99998 \nonumber\\
all_make & 0.99998 \nonumber\\
not_use & 0.99998 \nonumber\\
and_become & 0.99998 \nonumber\\
to_back & 0.99998 \nonumber\\
god_exist & 0.99998 \nonumber\\
_pos_ngram_NP_CARD_PUNC & 0.99998 \nonumber\\
improve_our & 0.99998 \nonumber\\
school_( & 0.99998 \nonumber\\
but_, & 0.99998 \nonumber\\
later & 0.99998 \nonumber\\
to_, & 0.99998 \nonumber\\
!! & 0.99998 \nonumber\\
truth_. & 0.99998 \nonumber\\
in_3-d & 0.99998 \nonumber\\
be_hus & 0.99998 \nonumber\\
def & 0.99998 \nonumber\\
three_year & 0.99998 \nonumber\\
def_. & 0.99998 \nonumber\\
3-d_. & 0.99998 \nonumber\\
3-d & 0.99998 \nonumber\\
in_three & 0.99998 \nonumber\\
hus_def & 0.99998 \nonumber\\
it_right & 0.99998 \nonumber\\
request_u & 0.99998 \nonumber\\
nw & 0.99998 \nonumber\\
develop_den & 0.99998 \nonumber\\
the_loot & 0.99998 \nonumber\\
indium_..... & 0.99998 \nonumber\\
think_before & 0.99998 \nonumber\\
i_request & 0.99998 \nonumber\\
indium_" & 0.99998 \nonumber\\
topic_..... & 0.99998 \nonumber\\
ProductionRule_NP->ADJP,DT, & 0.99998 \nonumber\\
develop_..... & 0.99998 \nonumber\\
join_da & 0.99998 \nonumber\\
bcoz_the & 0.99998 \nonumber\\
di_be & 0.99998 \nonumber\\
di_topic & 0.99998 \nonumber\\
of_di & 0.99998 \nonumber\\
hus_all & 0.99998 \nonumber\\
thing_dat & 0.99998 \nonumber\\
4m & 0.99998 \nonumber\\
bcoz & 0.99998 \nonumber\\
argue_..... & 0.99998 \nonumber\\
den_us & 0.99998 \nonumber\\
enjoy_nw & 0.99998 \nonumber\\
di_argue & 0.99998 \nonumber\\
nw_be & 0.99998 \nonumber\\
be_enjoy & 0.99998 \nonumber\\
4m_indium & 0.99998 \nonumber\\
be_da & 0.99998 \nonumber\\
bcoz_it & 0.99998 \nonumber\\
in_oppose & 0.99998 \nonumber\\
may_i & 0.99998 \nonumber\\
prsn & 0.99998 \nonumber\\
new_gal & 0.99998 \nonumber\\
prsn_who & 0.99998 \nonumber\\
one_4m & 0.99998 \nonumber\\
brain_and & 0.99998 \nonumber\\
foreigner_be & 0.99998 \nonumber\\
foreigner & 0.99998 \nonumber\\
dat_plz & 0.99998 \nonumber\\
da_prsn & 0.99998 \nonumber\\
da_indian & 0.99998 \nonumber\\
wealth_which & 0.99998 \nonumber\\
of_u. & 0.99998 \nonumber\\
potential_bcoz & 0.99998 \nonumber\\
r_in & 0.99998 \nonumber\\
loot_one & 0.99998 \nonumber\\
loot & 0.99998 \nonumber\\
u. & 0.99998 \nonumber\\
before_u & 0.99998 \nonumber\\
who_r & 0.99998 \nonumber\\
....._may & 0.99998 \nonumber\\
u._..... & 0.99998 \nonumber\\
other_foreign & 0.99998 \nonumber\\
country_develop & 0.99998 \nonumber\\
u_tell & 0.99998 \nonumber\\
._di & 0.99998 \nonumber\\
s_potential & 0.99998 \nonumber\\
u_one & 0.99998 \nonumber\\
"_s & 0.99998 \nonumber\\
the_foreigner & 0.99998 \nonumber\\
plz_think & 0.99998 \nonumber\\
us_bcoz & 0.99998 \nonumber\\
about_indium & 0.99998 \nonumber\\
more_develop & 0.99998 \nonumber\\
tell_about & 0.99998 \nonumber\\
their_brain & 0.99998 \nonumber\\
oppose_of & 0.99998 \nonumber\\
gal & 0.99998 \nonumber\\
gal_join & 0.99998 \nonumber\\
the_foreign & 0.99998 \nonumber\\
_pos_ngram_NP_ADV_ADV & 0.99998 \nonumber\\
group & 0.99998 \nonumber\\
raffle_only & 0.99998 \nonumber\\
,_mormonism & 0.99998 \nonumber\\
,_norse & 0.99998 \nonumber\\
roman_mythology & 0.99998 \nonumber\\
sarcasm_feature & 0.99998 \nonumber\\
sarcasm & 0.99998 \nonumber\\
be_disappoint & 0.99998 \nonumber\\
,_roman & 0.99998 \nonumber\\
,_sikhism & 0.99998 \nonumber\\
,_jainism & 0.99998 \nonumber\\
sikhism_, & 0.99998 \nonumber\\
sikhism & 0.99998 \nonumber\\
with_islam & 0.99998 \nonumber\\
norse_mythology & 0.99998 \nonumber\\
norse & 0.99998 \nonumber\\
ProductionRule_S->ADVP,,,PP,,,NP,VP,., & 0.99998 \nonumber\\
pastafarian_, & 0.99998 \nonumber\\
feature_on & 0.99998 \nonumber\\
judaism_, & 0.99998 \nonumber\\
._along & 0.99998 \nonumber\\
recognition_of & 0.99998 \nonumber\\
jainism & 0.99998 \nonumber\\
mormonism & 0.99998 \nonumber\\
jainism_, & 0.99998 \nonumber\\
mormonism_, & 0.99998 \nonumber\\
an_active & 0.99998 \nonumber\\
,_greek & 0.99998 \nonumber\\
pastafarian & 0.99998 \nonumber\\
,_hinduism & 0.99998 \nonumber\\
disappoint_at & 0.99998 \nonumber\\
see_as & 0.99998 \nonumber\\
disappoint & 0.99998 \nonumber\\
of_recognition & 0.99998 \nonumber\\
but_see & 0.99998 \nonumber\\
and_buddhism & 0.99998 \nonumber\\
greek & 0.99998 \nonumber\\
you_wish & 0.99998 \nonumber\\
greek_mythology & 0.99998 \nonumber\\
internet_? & 0.99998 \nonumber\\
a_theist & 0.99998 \nonumber\\
active_pastafarian & 0.99998 \nonumber\\
roman & 0.99998 \nonumber\\
a_sarcasm & 0.99998 \nonumber\\
mythology_, & 0.99998 \nonumber\\
buddhism_. & 0.99998 \nonumber\\
,_egyptian & 0.99998 \nonumber\\
egyptian_mythology & 0.99998 \nonumber\\
egyptian & 0.99998 \nonumber\\
mythology & 0.99998 \nonumber\\
theist_, & 0.99998 \nonumber\\
would_think & 0.99998 \nonumber\\
after_you & 0.99998 \nonumber\\
goal_because & 0.99998 \nonumber\\
dont_help & 0.99998 \nonumber\\
accomplish_your & 0.99998 \nonumber\\
i_thing & 0.99998 \nonumber\\
._help & 0.99998 \nonumber\\
someone_if & 0.99998 \nonumber\\
your_goal & 0.99998 \nonumber\\
achieve_your & 0.99998 \nonumber\\
thing_personal & 0.99998 \nonumber\\
ProductionRule_PP->IN,SBARQ, & 0.99998 \nonumber\\
you_achieve & 0.99998 \nonumber\\
first_would & 0.99998 \nonumber\\
that_after & 0.99998 \nonumber\\
they_dont & 0.99998 \nonumber\\
_pos_ngram_CONJ_O_V & 0.99998 \nonumber\\
no_, & 0.99998 \nonumber\\
be_punish & 0.99998 \nonumber\\
kid_get & 0.99998 \nonumber\\
,_wherea & 0.99998 \nonumber\\
wherea_raffle & 0.99998 \nonumber\\
ignorant_and & 0.99998 \nonumber\\
invalid & 0.99998 \nonumber\\
invalid_. & 0.99998 \nonumber\\
other_argument & 0.99998 \nonumber\\
completely_invalid & 0.99998 \nonumber\\
and_idiotic & 0.99998 \nonumber\\
be_ignorant & 0.99998 \nonumber\\
choice_should & 0.99998 \nonumber\\
link & 0.99998 \nonumber\\
possibly & 0.99998 \nonumber\\
think_gay & 0.99998 \nonumber\\
to_improve & 0.99998 \nonumber\\
and_therefore & 0.99998 \nonumber\\
subordinate & 0.99998 \nonumber\\
that_while & 0.99998 \nonumber\\
_pos_ngram_ADJ_ADV_PP & 0.99998 \nonumber\\
prepare & 0.99998 \nonumber\\
ProductionRule_S->PP,:,NP,VP,., & 0.99998 \nonumber\\
"_i & 0.99998 \nonumber\\
house & 0.99998 \nonumber\\
ProductionRule_PP->NN,NP, & 0.99998 \nonumber\\
for_him & 0.99998 \nonumber\\
exact_yes & 0.99998 \nonumber\\
hand_and & 0.99998 \nonumber\\
man_that & 0.99998 \nonumber\\
be_him & 0.99998 \nonumber\\
crime_then & 0.99998 \nonumber\\
question_depend & 0.99998 \nonumber\\
of_hand & 0.99998 \nonumber\\
yes_or & 0.99998 \nonumber\\
evidence_and & 0.99998 \nonumber\\
convict & 0.99998 \nonumber\\
convict_the & 0.99998 \nonumber\\
its_him & 0.99998 \nonumber\\
and_witness & 0.99998 \nonumber\\
or_no & 0.99998 \nonumber\\
police_new & 0.99998 \nonumber\\
him_then & 0.99998 \nonumber\\
this_question & 0.99998 \nonumber\\
witness_that & 0.99998 \nonumber\\
him_that & 0.99998 \nonumber\\
answer_to & 0.99998 \nonumber\\
my_man & 0.99998 \nonumber\\
really_get & 0.99998 \nonumber\\
new_it & 0.99998 \nonumber\\
that_convict & 0.99998 \nonumber\\
no_answer & 0.99998 \nonumber\\
an_exact & 0.99998 \nonumber\\
the_evidence & 0.99998 \nonumber\\
water_and & 0.99998 \nonumber\\
and_my & 0.99998 \nonumber\\
moment & 0.99998 \nonumber\\
habitat & 0.99998 \nonumber\\
that_case & 0.99998 \nonumber\\
feel_about & 0.99998 \nonumber\\
university & 0.99998 \nonumber\\
watch_tv & 0.99998 \nonumber\\
download & 0.99998 \nonumber\\
many_people & 0.99998 \nonumber\\
family_. & 0.99998 \nonumber\\
out_to & 0.99998 \nonumber\\
the_wealth & 0.99998 \nonumber\\
also_see & 0.99998 \nonumber\\
ProductionRule_NP->DT,NN,CD, & 0.99998 \nonumber\\
themselve_, & 0.99998 \nonumber\\
to_persue & 0.99998 \nonumber\\
not_for & 0.99998 \nonumber\\
._human & 0.99998 \nonumber\\
persue_thing & 0.99998 \nonumber\\
persuit_. & 0.99998 \nonumber\\
what_circumstance & 0.99998 \nonumber\\
and_dont & 0.99998 \nonumber\\
can_never & 0.99998 \nonumber\\
college_, & 0.99998 \nonumber\\
ProductionRule_VP->VBN,ADVP,PP, & 0.99998 \nonumber\\
and_give & 0.99998 \nonumber\\
partner_. & 0.99998 \nonumber\\
achievement & 0.99998 \nonumber\\
wud & 0.99998 \nonumber\\
farquar & 0.99998 \nonumber\\
dont_know & 0.99998 \nonumber\\
ProductionRule_VP->VBN,PP,PP, & 0.99998 \nonumber\\
_pos_ngram_CONJ_V_ADV & 0.99998 \nonumber\\
be_due & 0.99998 \nonumber\\
i_support & 0.99998 \nonumber\\
._beside & 0.99998 \nonumber\\
that_people & 0.99998 \nonumber\\
from_monkey & 0.99998 \nonumber\\
_pos_ngram_NP_NP_NN & 0.99998 \nonumber\\
plus_, & 0.99998 \nonumber\\
all-powerful & 0.99998 \nonumber\\
cause_by & 0.99998 \nonumber\\
be_cause & 0.99998 \nonumber\\
evolve_to & 0.99998 \nonumber\\
ProductionRule_UCP->ADJP,CC,PP, & 0.99998 \nonumber\\
_pos_ngram_CONJ_ADV_PR & 0.99998 \nonumber\\
lesson_. & 0.99998 \nonumber\\
do_all & 0.99998 \nonumber\\
in_and & 0.99998 \nonumber\\
with_raffle & 0.99998 \nonumber\\
situation & 0.99998 \nonumber\\
._almost & 0.99998 \nonumber\\
no_problem & 0.99998 \nonumber\\
reproduce & 0.99998 \nonumber\\
_pos_ngram_CONJ_ADV_NN & 0.99998 \nonumber\\
_pos_ngram_ART_ADJ_O & 0.99998 \nonumber\\
before_i & 0.99998 \nonumber\\
you_actually & 0.99998 \nonumber\\
that_most & 0.99998 \nonumber\\
have_cause & 0.99998 \nonumber\\
actually_do & 0.99998 \nonumber\\
in_pe & 0.99998 \nonumber\\
and_than & 0.99998 \nonumber\\
mental & 0.99998 \nonumber\\
your_problem & 0.99998 \nonumber\\
_pos_ngram_ADV_CARD_CONJ & 0.99998 \nonumber\\
be_something & 0.99998 \nonumber\\
the_year & 0.99998 \nonumber\\
ever_be & 0.99998 \nonumber\\
spell_skill & 0.99998 \nonumber\\
anywhere_and & 0.99998 \nonumber\\
everywhere_without & 0.99998 \nonumber\\
with_grammar & 0.99998 \nonumber\\
offer_improvement & 0.99998 \nonumber\\
set_with & 0.99998 \nonumber\\
book_anywhere & 0.99998 \nonumber\\
little_creativity & 0.99998 \nonumber\\
with_book & 0.99998 \nonumber\\
and_everywhere & 0.99998 \nonumber\\
book_offer & 0.99998 \nonumber\\
disrupt_anyone & 0.99998 \nonumber\\
tv_everything & 0.99998 \nonumber\\
disrupt & 0.99998 \nonumber\\
imagine_the & 0.99998 \nonumber\\
take_book & 0.99998 \nonumber\\
own_little & 0.99998 \nonumber\\
ProductionRule_ADJP->NN,CC,NN, & 0.99998 \nonumber\\
the_set & 0.99998 \nonumber\\
and_spell & 0.99998 \nonumber\\
character_look & 0.99998 \nonumber\\
creative_. & 0.99998 \nonumber\\
skill_. & 0.99998 \nonumber\\
improvement & 0.99998 \nonumber\\
plus_you & 0.99998 \nonumber\\
more_creative & 0.99998 \nonumber\\
improvement_with & 0.99998 \nonumber\\
creativity_in & 0.99998 \nonumber\\
grammar_and & 0.99998 \nonumber\\
without_disrupt & 0.99998 \nonumber\\
it_will & 0.99998 \nonumber\\
monkey_or & 0.99998 \nonumber\\
man_have & 0.99998 \nonumber\\
not_deny & 0.99998 \nonumber\\
man_) & 0.99998 \nonumber\\
)_2 & 0.99998 \nonumber\\
really_human & 0.99998 \nonumber\\
those_thing & 0.99998 \nonumber\\
create_evolve & 0.99998 \nonumber\\
surroundings_. & 0.99998 \nonumber\\
proof_of & 0.99998 \nonumber\\
time_believe & 0.99998 \nonumber\\
and_ever & 0.99998 \nonumber\\
single_cell & 0.99998 \nonumber\\
maybe_single & 0.99998 \nonumber\\
their_surroundings & 0.99998 \nonumber\\
think_adam & 0.99998 \nonumber\\
(_there & 0.99998 \nonumber\\
cell_. & 0.99998 \nonumber\\
be_proof & 0.99998 \nonumber\\
creature_man & 0.99998 \nonumber\\
deny_this & 0.99998 \nonumber\\
first_creature & 0.99998 \nonumber\\
thing_god & 0.99998 \nonumber\\
thing_( & 0.99998 \nonumber\\
we_make & 0.99998 \nonumber\\
we_come & 0.99998 \nonumber\\
since_the & 0.99998 \nonumber\\
a_grow & 0.99998 \nonumber\\
father_on & 0.99998 \nonumber\\
to_manage & 0.99998 \nonumber\\
ProductionRule_NP->JJ,NN,NN, & 0.99998 \nonumber\\
true_. & 0.99998 \nonumber\\
all_those & 0.99998 \nonumber\\
_pos_ngram_CARD_PP_V & 0.99998 \nonumber\\
hence & 0.99998 \nonumber\\
how_to & 0.99998 \nonumber\\
deny & 0.99998 \nonumber\\
etc._. & 0.99998 \nonumber\\
word_: & 0.99998 \nonumber\\
can_learn & 0.99998 \nonumber\\
the_character & 0.99998 \nonumber\\
nobody_should & 0.99998 \nonumber\\
by_see & 0.99998 \nonumber\\
easier_by & 0.99998 \nonumber\\
not_read & 0.99998 \nonumber\\
learn_easier & 0.99998 \nonumber\\
see_not & 0.99998 \nonumber\\
wealth & 0.99998 \nonumber\\
_pos_ngram_ART_V_CARD & 0.99998 \nonumber\\
wrong_thing & 0.99998 \nonumber\\
agree_that & 0.99998 \nonumber\\
spend_the & 0.99998 \nonumber\\
that_. & 0.99998 \nonumber\\
raffle_come & 0.99998 \nonumber\\
year_of & 0.99998 \nonumber\\
pursue & 0.99998 \nonumber\\
heat & 0.99998 \nonumber\\
tat & 0.99998 \nonumber\\
wud_b & 0.99998 \nonumber\\
ter & 0.99998 \nonumber\\
howzz & 0.99998 \nonumber\\
b_a & 0.99998 \nonumber\\
u_wud & 0.99998 \nonumber\\
ter_then & 0.99998 \nonumber\\
couch_potato & 0.99998 \nonumber\\
!!!!!!!!!!!!!!!!_howzz & 0.99998 \nonumber\\
potato_!!!!!!!!!!!!!!!! & 0.99998 \nonumber\\
ProductionRule_NP->JJ,NNS,NN, & 0.99998 \nonumber\\
not_ter & 0.99998 \nonumber\\
then_u & 0.99998 \nonumber\\
education_r & 0.99998 \nonumber\\
howzz_tat & 0.99998 \nonumber\\
!!!!!!!!!!!!!!!! & 0.99998 \nonumber\\
if_physical & 0.99998 \nonumber\\
r_not & 0.99998 \nonumber\\
tat_??? & 0.99998 \nonumber\\
its_a & 0.99998 \nonumber\\
be_they & 0.99998 \nonumber\\
wherea & 0.99998 \nonumber\\
itt & 0.99998 \nonumber\\
atheism_. & 0.99998 \nonumber\\
you_help & 0.99998 \nonumber\\
no_argument & 0.99998 \nonumber\\
'_right & 0.99998 \nonumber\\
ProductionRule_S->NP,VP,.,'', & 0.99998 \nonumber\\
_pos_ngram_ADJ_ADV_ART & 0.99998 \nonumber\\
all_for & 0.99998 \nonumber\\
_pos_ngram_NP_ADJ_NN & 0.99998 \nonumber\\
population_of & 0.99998 \nonumber\\
want_my & 0.99998 \nonumber\\
from_that & 0.99998 \nonumber\\
ProductionRule_NP->DT,NN,NN,NN, & 0.99998 \nonumber\\
matter_to & 0.99998 \nonumber\\
,_when & 0.99998 \nonumber\\
accord_to & 0.99998 \nonumber\\
accord & 0.99998 \nonumber\\
than_simply & 0.99998 \nonumber\\
create_fallacy & 0.99998 \nonumber\\
fallacy_in & 0.99998 \nonumber\\
be_morally & 0.99998 \nonumber\\
foundation_on & 0.99998 \nonumber\\
determine_under & 0.99998 \nonumber\\
circumstance_may & 0.99998 \nonumber\\
your_etymology & 0.99998 \nonumber\\
to_brush & 0.99998 \nonumber\\
that_an & 0.99998 \nonumber\\
brush & 0.99998 \nonumber\\
under_what & 0.99998 \nonumber\\
brush_up & 0.99998 \nonumber\\
paraphrase_definition & 0.99998 \nonumber\\
on_which & 0.99998 \nonumber\\
the_legal & 0.99998 \nonumber\\
mix_topic & 0.99998 \nonumber\\
definition_that & 0.99998 \nonumber\\
etymology & 0.99998 \nonumber\\
paraphrase & 0.99998 \nonumber\\
source_rather & 0.99998 \nonumber\\
morally_acceptable & 0.99998 \nonumber\\
thereby & 0.99998 \nonumber\\
)_foundation & 0.99998 \nonumber\\
vary & 0.99998 \nonumber\\
say_moral & 0.99998 \nonumber\\
legal_( & 0.99998 \nonumber\\
simply_paraphrase & 0.99998 \nonumber\\
your_source & 0.99998 \nonumber\\
acceptable_, & 0.99998 \nonumber\\
topic_thereby & 0.99998 \nonumber\\
fit_your & 0.99998 \nonumber\\
to_determine & 0.99998 \nonumber\\
to_terminate & 0.99998 \nonumber\\
terminate & 0.99998 \nonumber\\
terminate_pregnancy & 0.99998 \nonumber\\
morally & 0.99998 \nonumber\\
(_some & 0.99998 \nonumber\\
and_vary & 0.99998 \nonumber\\
individual_have & 0.99998 \nonumber\\
etymology_and & 0.99998 \nonumber\\
may_want & 0.99998 \nonumber\\
vary_your & 0.99998 \nonumber\\
that_fit & 0.99998 \nonumber\\
rather_, & 0.99998 \nonumber\\
thereby_create & 0.99998 \nonumber\\
be_mix & 0.99998 \nonumber\\
can_state & 0.99998 \nonumber\\
may_murder & 0.99998 \nonumber\\
may_say & 0.99998 \nonumber\\
moral_) & 0.99998 \nonumber\\
help_in & 0.99998 \nonumber\\
,_right & 0.99998 \nonumber\\
murder_, & 0.99998 \nonumber\\
,_do & 0.99998 \nonumber\\
other_than & 0.99998 \nonumber\\
can_grow & 0.99998 \nonumber\\
slavery & 0.99998 \nonumber\\
who_care & 0.99998 \nonumber\\
any_more & 0.99998 \nonumber\\
and_want & 0.99998 \nonumber\\
good_health & 0.99998 \nonumber\\
vital & 0.99998 \nonumber\\
like_if & 0.99998 \nonumber\\
lose_. & 0.99998 \nonumber\\
be_run & 0.99998 \nonumber\\
and_two & 0.99998 \nonumber\\
person_. & 0.99998 \nonumber\\
offer & 0.99998 \nonumber\\
to_stop & 0.99998 \nonumber\\
_pos_ngram_NP_CONJ_PP & 0.99998 \nonumber\\
when_raffle & 0.99998 \nonumber\\
._i & 0.99998 \nonumber\\
for_your & 0.99998 \nonumber\\
much_better & 0.99998 \nonumber\\
health_. & 0.99998 \nonumber\\
ProductionRule_SBAR->NP,IN,S, & 0.99998 \nonumber\\
love_the & 0.99998 \nonumber\\
that_can & 0.99998 \nonumber\\
-_i & 0.99998 \nonumber\\
or_human & 0.99998 \nonumber\\
"_? & 0.99998 \nonumber\\
that_someone & 0.99998 \nonumber\\
ProductionRule_VP->VBN,SBAR, & 0.99998 \nonumber\\
be_stronger & 0.99998 \nonumber\\
neglect_singapore & 0.99998 \nonumber\\
neglect & 0.99998 \nonumber\\
of_abortion & 0.99998 \nonumber\\
first_to & 0.99998 \nonumber\\
many_country & 0.99998 \nonumber\\
christianity_, & 0.99998 \nonumber\\
before_they & 0.99998 \nonumber\\
homosexual_be & 0.99998 \nonumber\\
_pos_ngram_O_PP_V & 0.99998 \nonumber\\
cell & 0.99998 \nonumber\\
because_farquhar & 0.99998 \nonumber\\
yes_! & 0.99998 \nonumber\\
_pos_ngram_ADJ_O_ART & 0.99998 \nonumber\\
in_some & 0.99998 \nonumber\\
idea_and & 0.99998 \nonumber\\
feel_of & 0.99998 \nonumber\\
whatever_they & 0.99998 \nonumber\\
either_way & 0.99998 \nonumber\\
the_end & 0.99998 \nonumber\\
make_me & 0.99998 \nonumber\\
and_im & 0.99998 \nonumber\\
need_there & 0.99998 \nonumber\\
christianity_: & 0.99998 \nonumber\\
expect_physical & 0.99998 \nonumber\\
ProductionRule_S->ADVP,,,SBAR,VP,., & 0.99998 \nonumber\\
of_rich & 0.99998 \nonumber\\
especially_rich & 0.99998 \nonumber\\
rich_parent & 0.99998 \nonumber\\
anything_expect & 0.99998 \nonumber\\
rich_child & 0.99998 \nonumber\\
education_especially & 0.99998 \nonumber\\
fashionable & 0.99998 \nonumber\\
hve & 0.99998 \nonumber\\
mufti & 0.99998 \nonumber\\
hve_to & 0.99998 \nonumber\\
wear_! & 0.99998 \nonumber\\
!_less & 0.99998 \nonumber\\
wear_mufti & 0.99998 \nonumber\\
say_wear & 0.99998 \nonumber\\
you_hve & 0.99998 \nonumber\\
less_awkward & 0.99998 \nonumber\\
awkward & 0.99998 \nonumber\\
awkward_when & 0.99998 \nonumber\\
mufti_... & 0.99998 \nonumber\\
world_should & 0.99998 \nonumber\\
_pos_ngram_ART_V_CONJ & 0.99998 \nonumber\\
do_my & 0.99998 \nonumber\\
the_help & 0.99998 \nonumber\\
help_of & 0.99998 \nonumber\\
relationship_with & 0.99998 \nonumber\\
,_since & 0.99998 \nonumber\\
...._discovery & 0.99998 \nonumber\\
nalanda & 0.99998 \nonumber\\
nalanda_where & 0.99998 \nonumber\\
decimal & 0.99998 \nonumber\\
country_come & 0.99998 \nonumber\\
and_0 & 0.99998 \nonumber\\
come_for & 0.99998 \nonumber\\
of_decimal & 0.99998 \nonumber\\
where_student & 0.99998 \nonumber\\
international_institute & 0.99998 \nonumber\\
institute_like & 0.99998 \nonumber\\
ProductionRule_X->NP,SBAR, & 0.99998 \nonumber\\
like_nalanda & 0.99998 \nonumber\\
for_study & 0.99998 \nonumber\\
indium_international & 0.99998 \nonumber\\
study_..... & 0.99998 \nonumber\\
decimal_and & 0.99998 \nonumber\\
in_an & 0.99998 \nonumber\\
itself & 0.99998 \nonumber\\
dicipline & 0.99998 \nonumber\\
many_way & 0.99998 \nonumber\\
wo_n't & 0.99998 \nonumber\\
wo & 0.99998 \nonumber\\
a_time & 0.99998 \nonumber\\
to_behave & 0.99998 \nonumber\\
stop_, & 0.99998 \nonumber\\
those_no & 0.99998 \nonumber\\
behave_all & 0.99998 \nonumber\\
ProductionRule_S->SBAR,,,NP,,,S,,,ADVP,VP,., & 0.99998 \nonumber\\
ProductionRule_SBAR->ADVP,S, & 0.99998 \nonumber\\
,_stop & 0.99998 \nonumber\\
work_sometime & 0.99998 \nonumber\\
sometime_. & 0.99998 \nonumber\\
know_its & 0.99998 \nonumber\\
forget & 0.99998 \nonumber\\
spank_the & 0.99998 \nonumber\\
_pos_ngram_ART_CONJ & 0.99998 \nonumber\\
then_have & 0.99998 \nonumber\\
gallon_of & 0.99998 \nonumber\\
mean_, & 0.99998 \nonumber\\
deed & 0.99998 \nonumber\\
start_to & 0.99998 \nonumber\\
sense_into & 0.99998 \nonumber\\
into_him & 0.99998 \nonumber\\
some_sense & 0.99998 \nonumber\\
knock_some & 0.99998 \nonumber\\
bid_because & 0.99998 \nonumber\\
_pos_ngram_ADJ_PUNC_NP & 0.99998 \nonumber\\
her_, & 0.99998 \nonumber\\
in_return & 0.99998 \nonumber\\
sign_a & 0.99998 \nonumber\\
ProductionRule_ADVP->RB,S, & 0.99998 \nonumber\\
notice_if & 0.99998 \nonumber\\
sure_we & 0.99998 \nonumber\\
?_could & 0.99998 \nonumber\\
your_key & 0.99998 \nonumber\\
key_to & 0.99998 \nonumber\\
dont_say & 0.99998 \nonumber\\
prove_your & 0.99998 \nonumber\\
you_so & 0.99998 \nonumber\\
varifiable & 0.99998 \nonumber\\
so_sure & 0.99998 \nonumber\\
varifiable_evidence & 0.99998 \nonumber\\
show_some & 0.99998 \nonumber\\
could_you & 0.99998 \nonumber\\
solid_varifiable & 0.99998 \nonumber\\
._solid & 0.99998 \nonumber\\
please_show & 0.99998 \nonumber\\
would_notice & 0.99998 \nonumber\\
,_just & 0.99998 \nonumber\\
that_kind & 0.99998 \nonumber\\
at_a & 0.99998 \nonumber\\
_pos_ngram_CARD_PUNC_CONJ & 0.99998 \nonumber\\
ProductionRule_S->INTJ,,,NP,VP, & 0.99998 \nonumber\\
i_alway & 0.99998 \nonumber\\
ProductionRule_S->ADVP,,,S,,,CC,S,., & 0.99998 \nonumber\\
mom_about & 0.99998 \nonumber\\
raise_me & 0.99998 \nonumber\\
a_second & 0.99998 \nonumber\\
fix_if & 0.99998 \nonumber\\
that_care & 0.99998 \nonumber\\
to_when & 0.99998 \nonumber\\
mom_raise & 0.99998 \nonumber\\
n't_talk & 0.99998 \nonumber\\
second_parent & 0.99998 \nonumber\\
only_my & 0.99998 \nonumber\\
and_knock & 0.99998 \nonumber\\
and_love & 0.99998 \nonumber\\
can_fix & 0.99998 \nonumber\\
'_lousy & 0.99998 \nonumber\\
respectful & 0.99998 \nonumber\\
discovery & 0.99998 \nonumber\\
people_before & 0.99998 \nonumber\\
mere_belief & 0.99998 \nonumber\\
punish_them & 0.99998 \nonumber\\
my_big & 0.99998 \nonumber\\
be_believer & 0.99998 \nonumber\\
preposterous_, & 0.99998 \nonumber\\
ProductionRule_NP->NP,PP,:,SBARQ, & 0.99998 \nonumber\\
can_seal & 0.99998 \nonumber\\
the_nature & 0.99998 \nonumber\\
preposterous & 0.99998 \nonumber\\
atheist_and & 0.99998 \nonumber\\
madness_!! & 0.99998 \nonumber\\
do_great & 0.99998 \nonumber\\
???_i & 0.99998 \nonumber\\
be_atheist & 0.99998 \nonumber\\
:_why & 0.99998 \nonumber\\
wonderful_people & 0.99998 \nonumber\\
its_madness & 0.99998 \nonumber\\
be_??? & 0.99998 \nonumber\\
be_horrible & 0.99998 \nonumber\\
beyond_preposterous & 0.99998 \nonumber\\
difference_can & 0.99998 \nonumber\\
nature_od & 0.99998 \nonumber\\
it_about & 0.99998 \nonumber\\
belief_difference & 0.99998 \nonumber\\
believer & 0.99998 \nonumber\\
believer_. & 0.99998 \nonumber\\
madness & 0.99998 \nonumber\\
be_beyond & 0.99998 \nonumber\\
it_fair & 0.99998 \nonumber\\
reality_be & 0.99998 \nonumber\\
seal & 0.99998 \nonumber\\
about_belief & 0.99998 \nonumber\\
great_thing & 0.99998 \nonumber\\
about_wonderful & 0.99998 \nonumber\\
od & 0.99998 \nonumber\\
od_reality & 0.99998 \nonumber\\
with_christianity & 0.99998 \nonumber\\
idea_that & 0.99998 \nonumber\\
horrible_people & 0.99998 \nonumber\\
_pos_ngram_V_CARD_PR & 0.99998 \nonumber\\
ProductionRule_SQ->VBZ,NP,ADVP,NP, & 0.99998 \nonumber\\
seal_one & 0.99998 \nonumber\\
fate_be & 0.99998 \nonumber\\
one_fate & 0.99998 \nonumber\\
good_person & 0.99998 \nonumber\\
fair_to & 0.99998 \nonumber\\
anyhow & 0.99998 \nonumber\\
mainly & 0.99998 \nonumber\\
n't_express & 0.99998 \nonumber\\
thing_as & 0.99998 \nonumber\\
couch & 0.99998 \nonumber\\
this_thing & 0.99998 \nonumber\\
that_ok & 0.99998 \nonumber\\
psychology_book & 0.99998 \nonumber\\
not_normal & 0.99998 \nonumber\\
its_normal & 0.99998 \nonumber\\
abnormal & 0.99998 \nonumber\\
psychology & 0.99998 \nonumber\\
guess_that & 0.99998 \nonumber\\
a_abnormal & 0.99998 \nonumber\\
abnormal_psychology & 0.99998 \nonumber\\
means_they & 0.99998 \nonumber\\
i_read & 0.99998 \nonumber\\
ProductionRule_NP->NN,,,NP,NN, & 0.99998 \nonumber\\
a_disorder & 0.99998 \nonumber\\
._he & 0.99998 \nonumber\\
certainly & 0.99998 \nonumber\\
become_the & 0.99998 \nonumber\\
money_. & 0.99998 \nonumber\\
ur & 0.99998 \nonumber\\
,_with & 0.99998 \nonumber\\
will_know & 0.99998 \nonumber\\
the_correct & 0.99998 \nonumber\\
be_ridiculous & 0.99998 \nonumber\\
alone_. & 0.99998 \nonumber\\
they_would & 0.99998 \nonumber\\
watch_porn & 0.99998 \nonumber\\
sleep & 0.99998 \nonumber\\
miss & 0.99998 \nonumber\\
big_problem & 0.99998 \nonumber\\
the_answer & 0.99998 \nonumber\\
commit_suicide & 0.99998 \nonumber\\
suicide & 0.99998 \nonumber\\
only_in & 0.99998 \nonumber\\
_pos_ngram_ART_PUNC_O & 0.99998 \nonumber\\
that_go & 0.99998 \nonumber\\
_pos_ngram_ART_PP_PUNC & 0.99998 \nonumber\\
be_almost & 0.99998 \nonumber\\
think_both & 0.99998 \nonumber\\
now_, & 0.99998 \nonumber\\
magic & 0.99998 \nonumber\\
so_not & 0.99998 \nonumber\\
to_leave & 0.99998 \nonumber\\
government_for & 0.99998 \nonumber\\
bastion_that & 0.99998 \nonumber\\
free_people & 0.99998 \nonumber\\
support_pro & 0.99998 \nonumber\\
else_because & 0.99998 \nonumber\\
bastion & 0.99998 \nonumber\\
ProductionRule_VP->VBP,PRT,PP, & 0.99998 \nonumber\\
that_free & 0.99998 \nonumber\\
out_against & 0.99998 \nonumber\\
hold_out & 0.99998 \nonumber\\
last_bastion & 0.99998 \nonumber\\
people_hold & 0.99998 \nonumber\\
choice_if & 0.99998 \nonumber\\
come_to & 0.99998 \nonumber\\
man_evolve & 0.99998 \nonumber\\
there_a & 0.99998 \nonumber\\
ProductionRule_SQ->VBD,NP,NP,., & 0.99998 \nonumber\\
?_dang & 0.99998 \nonumber\\
a_historical & 0.99998 \nonumber\\
record_of & 0.99998 \nonumber\\
miss_it & 0.99998 \nonumber\\
dang & 0.99998 \nonumber\\
dang_, & 0.99998 \nonumber\\
have_miss & 0.99998 \nonumber\\
historical_record & 0.99998 \nonumber\\
occur_. & 0.99998 \nonumber\\
ProductionRule_NP->DT,ADJP,NN,NN, & 0.99998 \nonumber\\
mistake_that & 0.99998 \nonumber\\
_pos_ngram_NP_O_PP & 0.99998 \nonumber\\
help_people & 0.99998 \nonumber\\
,_at & 0.99998 \nonumber\\
be_it & 0.99998 \nonumber\\
1_word & 0.99998 \nonumber\\
_pos_ngram_CONJ_NP_CARD & 0.99998 \nonumber\\
:_corruption & 0.99998 \nonumber\\
ProductionRule_VP->TO,S, & 0.99998 \nonumber\\
corruption_..... & 0.99998 \nonumber\\
just_1 & 0.99998 \nonumber\\
corruption_& & 0.99998 \nonumber\\
but_just & 0.99998 \nonumber\\
ProductionRule_NP->NNP,,,NNP,CC,NNP, & 0.99998 \nonumber\\
&_corruption & 0.99998 \nonumber\\
be_place & 0.99998 \nonumber\\
to_hack & 0.99998 \nonumber\\
tell_woman & 0.99998 \nonumber\\
to_peice & 0.99998 \nonumber\\
ProductionRule_FRAG->ADVP,NP, & 0.99998 \nonumber\\
suicide_if & 0.99998 \nonumber\\
do_limit & 0.99998 \nonumber\\
catch_try & 0.99998 \nonumber\\
themselve_to & 0.99998 \nonumber\\
hack & 0.99998 \nonumber\\
institute_so & 0.99998 \nonumber\\
hack_themselve & 0.99998 \nonumber\\
peice_they & 0.99998 \nonumber\\
a_mental & 0.99998 \nonumber\\
government_actually & 0.99998 \nonumber\\
limit_what & 0.99998 \nonumber\\
peice & 0.99998 \nonumber\\
'_illegal & 0.99998 \nonumber\\
body_it & 0.99998 \nonumber\\
mental_institute & 0.99998 \nonumber\\
actually_the & 0.99998 \nonumber\\
be_kind & 0.99998 \nonumber\\
attack_her & 0.99998 \nonumber\\
be_accidental & 0.99998 \nonumber\\
kill_spree & 0.99998 \nonumber\\
case_she & 0.99998 \nonumber\\
i_wil & 0.99998 \nonumber\\
or_decide & 0.99998 \nonumber\\
trouble_, & 0.99998 \nonumber\\
another_kill & 0.99998 \nonumber\\
someone_try & 0.99998 \nonumber\\
get_you & 0.99998 \nonumber\\
accidental & 0.99998 \nonumber\\
she_tell & 0.99998 \nonumber\\
wil_call & 0.99998 \nonumber\\
accompalice & 0.99998 \nonumber\\
accompalice_. & 0.99998 \nonumber\\
spree_or & 0.99998 \nonumber\\
major_trouble & 0.99998 \nonumber\\
second_she & 0.99998 \nonumber\\
in_major & 0.99998 \nonumber\\
spree & 0.99998 \nonumber\\
there_could & 0.99998 \nonumber\\
an_accompalice & 0.99998 \nonumber\\
wil & 0.99998 \nonumber\\
either_go & 0.99998 \nonumber\\
she_either & 0.99998 \nonumber\\
accidental_, & 0.99998 \nonumber\\
and_eat & 0.99998 \nonumber\\
part_and & 0.99998 \nonumber\\
most_part & 0.99998 \nonumber\\
much_junk & 0.99998 \nonumber\\
so_out & 0.99998 \nonumber\\
shape_for & 0.99998 \nonumber\\
!_our & 0.99998 \nonumber\\
our_kid & 0.99998 \nonumber\\
the_risk & 0.99998 \nonumber\\
risk_of & 0.99998 \nonumber\\
the_site & 0.99998 \nonumber\\
current & 0.99998 \nonumber\\
thirteen & 0.99998 \nonumber\\
..._the & 0.99998 \nonumber\\
no_right & 0.99998 \nonumber\\
the_person & 0.99998 \nonumber\\
to_convince & 0.99998 \nonumber\\
s_why & 0.99998 \nonumber\\
plz.give & 0.99998 \nonumber\\
highly_oblige & 0.99998 \nonumber\\
'_s & 0.99998 \nonumber\\
of_class & 0.99998 \nonumber\\
11_. & 0.99998 \nonumber\\
why_ask & 0.99998 \nonumber\\
oblige_to & 0.99998 \nonumber\\
11 & 0.99998 \nonumber\\
plz.give_me & 0.99998 \nonumber\\
in_dbt & 0.99998 \nonumber\\
oblige & 0.99998 \nonumber\\
m_student & 0.99998 \nonumber\\
take_part & 0.99998 \nonumber\\
,_plz.give & 0.99998 \nonumber\\
more_datas.i & 0.99998 \nonumber\\
datas.i_will & 0.99998 \nonumber\\
class_11 & 0.99998 \nonumber\\
datas.i & 0.99998 \nonumber\\
dbt & 0.99998 \nonumber\\
me_more & 0.99998 \nonumber\\
dbt_. & 0.99998 \nonumber\\
also_think & 0.99998 \nonumber\\
no_place & 0.99998 \nonumber\\
book_make & 0.99998 \nonumber\\
also_say & 0.99998 \nonumber\\
more_intelligent & 0.99998 \nonumber\\
intelligent_. & 0.99998 \nonumber\\
encourage_you & 0.99998 \nonumber\\
country_be & 0.99998 \nonumber\\
humanity & 0.99998 \nonumber\\
those_big & 0.99998 \nonumber\\
their_parent & 0.99998 \nonumber\\
be_think & 0.99998 \nonumber\\
who_watch & 0.99998 \nonumber\\
_pos_ngram_CONJ_ADJ_CONJ & 0.99998 \nonumber\\
ProductionRule_VP->VP,NP, & 0.99998 \nonumber\\
really_? & 0.99998 \nonumber\\
status_of & 0.99998 \nonumber\\
so_there & 0.99998 \nonumber\\
bullshit & 0.99998 \nonumber\\
and_ca & 0.99998 \nonumber\\
of_marriage & 0.99998 \nonumber\\
the_browser & 0.99998 \nonumber\\
ProductionRule_VP->VBP,NP,NP, & 0.99998 \nonumber\\
raffle_to & 0.99998 \nonumber\\
country_for & 0.99998 \nonumber\\
approve_by & 0.99998 \nonumber\\
soldier_, & 0.99998 \nonumber\\
_pos_ngram_V_PUNC_CARD & 0.99998 \nonumber\\
he_know & 0.99998 \nonumber\\
water_on & 0.99998 \nonumber\\
._porn & 0.99998 \nonumber\\
force_. & 0.99998 \nonumber\\
police_force & 0.99998 \nonumber\\
people_from & 0.99998 \nonumber\\
_pos_ngram_PUNC_CARD_PUNC & 0.99998 \nonumber\\
this_show & 0.99998 \nonumber\\
that_spank & 0.99998 \nonumber\\
and_wrong & 0.99998 \nonumber\\
it_cause & 0.99998 \nonumber\\
._ff & 0.99998 \nonumber\\
my_school & 0.99998 \nonumber\\
he_should & 0.99998 \nonumber\\
farquhar_to & 0.99998 \nonumber\\
blame & 0.99998 \nonumber\\
ProductionRule_VP->VBZ,RB,NP,PP, & 0.99998 \nonumber\\
should_talk & 0.99998 \nonumber\\
understand_, & 0.99998 \nonumber\\
problem_... & 0.99998 \nonumber\\
kid_with & 0.99998 \nonumber\\
solution_to & 0.99998 \nonumber\\
u_should & 0.99998 \nonumber\\
with_love & 0.99998 \nonumber\\
good_thing & 0.99998 \nonumber\\
_pos_ngram_PUNC_PUNC_PP & 0.99998 \nonumber\\
show_their & 0.99998 \nonumber\\
their_color & 0.99998 \nonumber\\
kid_wo & 0.99998 \nonumber\\
color_. & 0.99998 \nonumber\\
economic & 0.99998 \nonumber\\
datum & 0.99998 \nonumber\\
the_pepper & 0.99998 \nonumber\\
ProductionRule_ADVP->FW,FW, & 0.99998 \nonumber\\
raffle_' & 0.99998 \nonumber\\
think_. & 0.99998 \nonumber\\
of_have & 0.99998 \nonumber\\
to_punish & 0.99998 \nonumber\\
argument_. & 0.99998 \nonumber\\
fear_of & 0.99998 \nonumber\\
fit_their & 0.99998 \nonumber\\
to_fit & 0.99998 \nonumber\\
,_while & 0.99998 \nonumber\\
serious & 0.99998 \nonumber\\
of_many & 0.99998 \nonumber\\
ProductionRule_X->ADVP,NP,., & 0.99998 \nonumber\\
witness & 0.99998 \nonumber\\
their_child & 0.99998 \nonumber\\
opinion_i & 0.99998 \nonumber\\
case_. & 0.99998 \nonumber\\
i_honestly & 0.99998 \nonumber\\
chance_to & 0.99998 \nonumber\\
would_only & 0.99998 \nonumber\\
speech & 0.99998 \nonumber\\
a_hole & 0.99998 \nonumber\\
anyway_, & 0.99998 \nonumber\\
_pos_ngram_V_ADV_NP & 0.99998 \nonumber\\
** & 0.99998 \nonumber\\
**_king & 0.99998 \nonumber\\
f & 0.99998 \nonumber\\
f_** & 0.99998 \nonumber\\
most_wonderful & 0.99998 \nonumber\\
with_tv & 0.99998 \nonumber\\
your_job & 0.99998 \nonumber\\
our_real & 0.99998 \nonumber\\
like_they & 0.99998 \nonumber\\
)_. & 0.99998 \nonumber\\
condition_and & 0.99998 \nonumber\\
quote_" & 0.99998 \nonumber\\
first_year & 0.99998 \nonumber\\
sport_athlete & 0.99998 \nonumber\\
school_combine & 0.99998 \nonumber\\
to_only & 0.99998 \nonumber\\
ProductionRule_NP->JJ,NN,ADJP,NN, & 0.99998 \nonumber\\
i_attend & 0.99998 \nonumber\\
hard_it & 0.99998 \nonumber\\
pe_for & 0.99998 \nonumber\\
school_i & 0.99998 \nonumber\\
sport_our & 0.99998 \nonumber\\
pe_condition & 0.99998 \nonumber\\
make_condition & 0.99998 \nonumber\\
not_high & 0.99998 \nonumber\\
condition_would & 0.99998 \nonumber\\
school_not & 0.99998 \nonumber\\
simple_" & 0.99998 \nonumber\\
school_many & 0.99998 \nonumber\\
middle_school & 0.99998 \nonumber\\
attend_only & 0.99998 \nonumber\\
middle_and & 0.99998 \nonumber\\
school_we & 0.99998 \nonumber\\
condition_simple & 0.99998 \nonumber\\
simple_pre & 0.99998 \nonumber\\
pre & 0.99998 \nonumber\\
perform_simple & 0.99998 \nonumber\\
a_middle & 0.99998 \nonumber\\
exercise_have & 0.99998 \nonumber\\
pre_season & 0.99998 \nonumber\\
only_3 & 0.99998 \nonumber\\
accomplish_only & 0.99998 \nonumber\\
they_quote & 0.99998 \nonumber\\
our_first & 0.99998 \nonumber\\
active_habit & 0.99998 \nonumber\\
season_condition & 0.99998 \nonumber\\
to_perform & 0.99998 \nonumber\\
for_middle & 0.99998 \nonumber\\
bid_non & 0.99998 \nonumber\\
push-up & 0.99998 \nonumber\\
push-up_! & 0.99998 \nonumber\\
only_accomplish & 0.99998 \nonumber\\
3_push-up & 0.99998 \nonumber\\
many_student & 0.99998 \nonumber\\
our_sport & 0.99998 \nonumber\\
combine_. & 0.99998 \nonumber\\
habit_and & 0.99998 \nonumber\\
our_high & 0.99998 \nonumber\\
non_active & 0.99998 \nonumber\\
season & 0.99998 \nonumber\\
athlete_have & 0.99998 \nonumber\\
how_hard & 0.99998 \nonumber\\
develop_many & 0.99998 \nonumber\\
year_in & 0.99998 \nonumber\\
education_in & 0.99998 \nonumber\\
act_of & 0.99998 \nonumber\\
victim_. & 0.99998 \nonumber\\
n't_see & 0.99998 \nonumber\\
catch_. & 0.99998 \nonumber\\
_pos_ngram_PP_ADJ_PR & 0.99998 \nonumber\\
what_you & 0.99998 \nonumber\\
live_a & 0.99998 \nonumber\\
they_kill & 0.99998 \nonumber\\
spank_and & 0.99998 \nonumber\\
past & 0.99998 \nonumber\\
time_out & 0.99998 \nonumber\\
9_time & 0.99998 \nonumber\\
9 & 0.99998 \nonumber\\
of_10 & 0.99998 \nonumber\\
and_grow & 0.99998 \nonumber\\
than_how & 0.99998 \nonumber\\
grow_leg & 0.99998 \nonumber\\
we_find & 0.99998 \nonumber\\
form_? & 0.99998 \nonumber\\
mysterious & 0.99998 \nonumber\\
mysterious_time & 0.99998 \nonumber\\
n't_? & 0.99998 \nonumber\\
make_much & 0.99998 \nonumber\\
today_? & 0.99998 \nonumber\\
much_sense & 0.99998 \nonumber\\
fish_with & 0.99998 \nonumber\\
come_its & 0.99998 \nonumber\\
with_leg & 0.99998 \nonumber\\
happen_today & 0.99998 \nonumber\\
a_mysterious & 0.99998 \nonumber\\
fish_jump & 0.99998 \nonumber\\
happen_for & 0.99998 \nonumber\\
n't_fish & 0.99998 \nonumber\\
happen_billion & 0.99998 \nonumber\\
of_thousand & 0.99998 \nonumber\\
psuedo-hybrid & 0.99998 \nonumber\\
leg_? & 0.99998 \nonumber\\
the_monkey & 0.99998 \nonumber\\
ago_than & 0.99998 \nonumber\\
jump & 0.99998 \nonumber\\
cause_evolution & 0.99998 \nonumber\\
jump_out & 0.99998 \nonumber\\
monkey_be & 0.99998 \nonumber\\
we_still & 0.99998 \nonumber\\
leg_form & 0.99998 \nonumber\\
psuedo-hybrid_fish & 0.99998 \nonumber\\
find_psuedo-hybrid & 0.99998 \nonumber\\
evolve_and & 0.99998 \nonumber\\
stop_happen & 0.99998 \nonumber\\
mad & 0.99998 \nonumber\\
some_child & 0.99998 \nonumber\\
raffle_and & 0.99998 \nonumber\\
sure_of & 0.99998 \nonumber\\
,_how & 0.99998 \nonumber\\
about_the & 0.99998 \nonumber\\
love_him & 0.99998 \nonumber\\
spank_once & 0.99998 \nonumber\\
cuz & 0.99998 \nonumber\\
on_with & 0.99998 \nonumber\\
different_. & 0.99998 \nonumber\\
increase_their & 0.99998 \nonumber\\
developer & 0.99998 \nonumber\\
bid_developer & 0.99998 \nonumber\\
be_warn & 0.99998 \nonumber\\
warn & 0.99998 \nonumber\\
child_deserve & 0.99998 \nonumber\\
behavior_that & 0.99998 \nonumber\\
after_several & 0.99998 \nonumber\\
n't_follow & 0.99998 \nonumber\\
correct_behavior & 0.99998 \nonumber\\
follow_after & 0.99998 \nonumber\\
discipline_only & 0.99998 \nonumber\\
deserve_a & 0.99998 \nonumber\\
warn_, & 0.99998 \nonumber\\
and_most & 0.99998 \nonumber\\
academic & 0.99998 \nonumber\\
their_academic & 0.99998 \nonumber\\
help_us & 0.99998 \nonumber\\
ProductionRule_VP->VBN,ADJP, & 0.99998 \nonumber\\
founder_be & 0.99998 \nonumber\\
would_n't & 0.99998 \nonumber\\
2000 & 0.99998 \nonumber\\
human_will & 0.99998 \nonumber\\
?_not & 0.99998 \nonumber\\
2000_? & 0.99998 \nonumber\\
anyhow_. & 0.99998 \nonumber\\
he_create & 0.99998 \nonumber\\
some_single-cell & 0.99998 \nonumber\\
these_tiny & 0.99998 \nonumber\\
then_? & 0.99998 \nonumber\\
create_some & 0.99998 \nonumber\\
set_this & 0.99998 \nonumber\\
judge_us & 0.99998 \nonumber\\
guy_be & 0.99998 \nonumber\\
organism & 0.99998 \nonumber\\
make_mary & 0.99998 \nonumber\\
mary & 0.99998 \nonumber\\
tweak_anyhow & 0.99998 \nonumber\\
-_be & 0.99998 \nonumber\\
would_god & 0.99998 \nonumber\\
tiny_organism & 0.99998 \nonumber\\
of_sense & 0.99998 \nonumber\\
ProductionRule_VP->VBG,PP,S, & 0.99998 \nonumber\\
organism_a & 0.99998 \nonumber\\
in_2000 & 0.99998 \nonumber\\
evolve_some & 0.99998 \nonumber\\
jesus_. & 0.99998 \nonumber\\
all-powerful_. & 0.99998 \nonumber\\
2100_to & 0.99998 \nonumber\\
ProductionRule_FRAG->X,:,VP,., & 0.99998 \nonumber\\
good_use & 0.99998 \nonumber\\
2100 & 0.99998 \nonumber\\
tweak_these & 0.99998 \nonumber\\
organism_billion & 0.99998 \nonumber\\
call_evolution & 0.99998 \nonumber\\
ago_, & 0.99998 \nonumber\\
mary_give & 0.99998 \nonumber\\
year_2100 & 0.99998 \nonumber\\
will_tweak & 0.99998 \nonumber\\
then_maybe & 0.99998 \nonumber\\
be_god & 0.99998 \nonumber\\
thing_call & 0.99998 \nonumber\\
himself_" & 0.99998 \nonumber\\
god_come & 0.99998 \nonumber\\
some_day & 0.99998 \nonumber\\
to_set & 0.99998 \nonumber\\
evolution_go & 0.99998 \nonumber\\
single-cell & 0.99998 \nonumber\\
single-cell_organism & 0.99998 \nonumber\\
to_tweak & 0.99998 \nonumber\\
what_- & 0.99998 \nonumber\\
'_time & 0.99998 \nonumber\\
maybe_human & 0.99998 \nonumber\\
then_say & 0.99998 \nonumber\\
be_all-powerful & 0.99998 \nonumber\\
to_himself & 0.99998 \nonumber\\
!!! & 0.99998 \nonumber\\
ProductionRule_NP->PDT,DT,NN, & 0.99998 \nonumber\\
leg & 0.99998 \nonumber\\
_pos_ngram_NP_PP_PP & 0.99998 \nonumber\\
occasional & 0.99998 \nonumber\\
ProductionRule_ADJP->RB,RB,JJ, & 0.99998 \nonumber\\
growth & 0.99998 \nonumber\\
i_try & 0.99998 \nonumber\\
help_singapore & 0.99998 \nonumber\\
work_to & 0.99998 \nonumber\\
goal_and & 0.99998 \nonumber\\
be_allow & 0.99998 \nonumber\\
of_independence & 0.99998 \nonumber\\
alway_about & 0.99998 \nonumber\\
and_success & 0.99998 \nonumber\\
it_start & 0.99998 \nonumber\\
needy & 0.99998 \nonumber\\
needy_or & 0.99998 \nonumber\\
that_money & 0.99998 \nonumber\\
happiness_, & 0.99998 \nonumber\\
your_desire & 0.99998 \nonumber\\
about_happiness & 0.99998 \nonumber\\
about_money & 0.99998 \nonumber\\
you_if & 0.99998 \nonumber\\
the_needy & 0.99998 \nonumber\\
also_about & 0.99998 \nonumber\\
money_but & 0.99998 \nonumber\\
success_. & 0.99998 \nonumber\\
money_for & 0.99998 \nonumber\\
god_and & 0.99998 \nonumber\\
ProductionRule_VP->VBZ,ADVP, & 0.99998 \nonumber\\
poverty & 0.99998 \nonumber\\
point_where & 0.99998 \nonumber\\
_pos_ngram_O_O_ADJ & 0.99998 \nonumber\\
be_teach & 0.99998 \nonumber\\
ProductionRule_VP->VBG,ADVP,PP, & 0.99998 \nonumber\\
virus & 0.99998 \nonumber\\
real_, & 0.99998 \nonumber\\
have_learn & 0.99998 \nonumber\\
meet & 0.99998 \nonumber\\
_pos_ngram_NP_NN_ADV & 0.99998 \nonumber\\
then_no & 0.99998 \nonumber\\
ProductionRule_S->S,IN,S, & 0.99998 \nonumber\\
drive & 0.99998 \nonumber\\
,_give & 0.99998 \nonumber\\
weak_, & 0.99998 \nonumber\\
plain_out & 0.99998 \nonumber\\
say_plain & 0.99998 \nonumber\\
._call & 0.99998 \nonumber\\
me_pathetic & 0.99998 \nonumber\\
pathetic_, & 0.99998 \nonumber\\
,_weak & 0.99998 \nonumber\\
only_truth & 0.99998 \nonumber\\
truth_, & 0.99998 \nonumber\\
for_sure & 0.99998 \nonumber\\
whole_truth & 0.99998 \nonumber\\
pathetic & 0.99998 \nonumber\\
call_me & 0.99998 \nonumber\\
pursuit_before & 0.99998 \nonumber\\
a_feel & 0.99998 \nonumber\\
of_pride & 0.99998 \nonumber\\
however_for & 0.99998 \nonumber\\
have_common & 0.99998 \nonumber\\
think_one & 0.99998 \nonumber\\
you_first & 0.99998 \nonumber\\
people_their & 0.99998 \nonumber\\
the_means & 0.99998 \nonumber\\
means_to & 0.99998 \nonumber\\
pride & 0.99998 \nonumber\\
other_person & 0.99998 \nonumber\\
pride_but & 0.99998 \nonumber\\
first_have & 0.99998 \nonumber\\
those_means & 0.99998 \nonumber\\
good_can & 0.99998 \nonumber\\
farquhar_develop & 0.99998 \nonumber\\
would_hurt & 0.99998 \nonumber\\
ProductionRule_NP->PRP$,NN,NN, & 0.99998 \nonumber\\
what_cause & 0.99998 \nonumber\\
problem_with & 0.99998 \nonumber\\
be_attempt & 0.99998 \nonumber\\
and_bid & 0.99998 \nonumber\\
mine & 0.99998 \nonumber\\
hope_that & 0.99998 \nonumber\\
goal_. & 0.99998 \nonumber\\
pursuit_its & 0.99998 \nonumber\\
all_on & 0.99998 \nonumber\\
someone_by & 0.99998 \nonumber\\
other_reach & 0.99998 \nonumber\\
succeed_their & 0.99998 \nonumber\\
not_alway & 0.99998 \nonumber\\
of_reach & 0.99998 \nonumber\\
their_goal & 0.99998 \nonumber\\
side_tell & 0.99998 \nonumber\\
their_succeed & 0.99998 \nonumber\\
reach_their & 0.99998 \nonumber\\
its_your & 0.99998 \nonumber\\
murder_. & 0.99998 \nonumber\\
thing_that & 0.99998 \nonumber\\
need_and & 0.99998 \nonumber\\
oh & 0.99998 \nonumber\\
guy & 0.99998 \nonumber\\
90 & 0.99998 \nonumber\\
90_% & 0.99998 \nonumber\\
surroundings & 0.99998 \nonumber\\
other_for & 0.99998 \nonumber\\
the_next & 0.99999 \nonumber\\
earth_. & 0.99999 \nonumber\\
its_also & 0.99999 \nonumber\\
would_make & 0.99999 \nonumber\\
worship & 0.99999 \nonumber\\
do_whatever & 0.99999 \nonumber\\
supress_free & 0.99999 \nonumber\\
free_speech & 0.99999 \nonumber\\
even_there & 0.99999 \nonumber\\
supress & 0.99999 \nonumber\\
in_private & 0.99999 \nonumber\\
voluntary & 0.99999 \nonumber\\
private_school & 0.99999 \nonumber\\
voluntary_association & 0.99999 \nonumber\\
association_. & 0.99999 \nonumber\\
see_i & 0.99999 \nonumber\\
uniform_supress & 0.99999 \nonumber\\
'_individuality & 0.99999 \nonumber\\
a_voluntary & 0.99999 \nonumber\\
only_agree & 0.99999 \nonumber\\
youth_' & 0.99999 \nonumber\\
a_youth & 0.99999 \nonumber\\
there_i & 0.99999 \nonumber\\
truthfully & 0.99999 \nonumber\\
about_another & 0.99999 \nonumber\\
"_illegal & 0.99999 \nonumber\\
really_wrong & 0.99999 \nonumber\\
porn_should & 0.99999 \nonumber\\
porn_supplies & 0.99999 \nonumber\\
illegal_" & 0.99999 \nonumber\\
erotic & 0.99999 \nonumber\\
erotic_" & 0.99999 \nonumber\\
then_porn & 0.99999 \nonumber\\
"_need & 0.99999 \nonumber\\
a_partner & 0.99999 \nonumber\\
supplies_the & 0.99999 \nonumber\\
"_erotic & 0.99999 \nonumber\\
_pos_ngram_NN_CONJ_NP & 0.99999 \nonumber\\
ProductionRule_VP->VBP,PP,SBAR, & 0.99999 \nonumber\\
in_one & 0.99999 \nonumber\\
kid_be & 0.99999 \nonumber\\
?_why & 0.99999 \nonumber\\
ProductionRule_SBAR->WHADVP,FRAG, & 0.99999 \nonumber\\
28 & 0.99999 \nonumber\\
the_blimem & 0.99999 \nonumber\\
blimem_olden & 0.99999 \nonumber\\
olden_day & 0.99999 \nonumber\\
blimem & 0.99999 \nonumber\\
book_from & 0.99999 \nonumber\\
than_read & 0.99999 \nonumber\\
an_excuse & 0.99999 \nonumber\\
more_useful & 0.99999 \nonumber\\
why_cant & 0.99999 \nonumber\\
b & 0.99999 \nonumber\\
just_go & 0.99999 \nonumber\\
some_may & 0.99999 \nonumber\\
rather_the & 0.99999 \nonumber\\
but_rather & 0.99999 \nonumber\\
become_degrade & 0.99999 \nonumber\\
an_actor & 0.99999 \nonumber\\
pornography_and & 0.99999 \nonumber\\
a_society & 0.99999 \nonumber\\
produce_the & 0.99999 \nonumber\\
actor_( & 0.99999 \nonumber\\
to_berate & 0.99999 \nonumber\\
actor_would & 0.99999 \nonumber\\
produce_it & 0.99999 \nonumber\\
movie_actor & 0.99999 \nonumber\\
._likewise & 0.99999 \nonumber\\
ProductionRule_ADJP->RB,VBN,PP, & 0.99999 \nonumber\\
society_we & 0.99999 \nonumber\\
degrade_. & 0.99999 \nonumber\\
porn_that & 0.99999 \nonumber\\
acceptance_of & 0.99999 \nonumber\\
berate_movie & 0.99999 \nonumber\\
if_, & 0.99999 \nonumber\\
the_acceptance & 0.99999 \nonumber\\
of_produce & 0.99999 \nonumber\\
likewise_, & 0.99999 \nonumber\\
if_pornography & 0.99999 \nonumber\\
likewise & 0.99999 \nonumber\\
berate & 0.99999 \nonumber\\
example_) & 0.99999 \nonumber\\
degrade_anyone & 0.99999 \nonumber\\
who_produce & 0.99999 \nonumber\\
athlete & 0.99999 \nonumber\\
positive_achievement & 0.99999 \nonumber\\
his_many & 0.99999 \nonumber\\
contribution_and & 0.99999 \nonumber\\
he_adopt & 0.99999 \nonumber\\
administration & 0.99999 \nonumber\\
which_conflict & 0.99999 \nonumber\\
achievement_in & 0.99999 \nonumber\\
sack_. & 0.99999 \nonumber\\
ignore_farquhar & 0.99999 \nonumber\\
his_administration & 0.99999 \nonumber\\
many_positive & 0.99999 \nonumber\\
the_formative & 0.99999 \nonumber\\
administration_which & 0.99999 \nonumber\\
and_credit & 0.99999 \nonumber\\
'_instruction & 0.99999 \nonumber\\
despite_his & 0.99999 \nonumber\\
credit_them & 0.99999 \nonumber\\
instruction & 0.99999 \nonumber\\
formative & 0.99999 \nonumber\\
instruction_, & 0.99999 \nonumber\\
formative_period & 0.99999 \nonumber\\
farquhar_' & 0.99999 \nonumber\\
measure_in & 0.99999 \nonumber\\
'_contribution & 0.99999 \nonumber\\
straight & 0.99999 \nonumber\\
_pos_ngram_ADV_NN_CONJ & 0.99999 \nonumber\\
the_past & 0.99999 \nonumber\\
year_ago & 0.99999 \nonumber\\
up_and & 0.99999 \nonumber\\
its_all & 0.99999 \nonumber\\
for_kill & 0.99999 \nonumber\\
be_well & 0.99999 \nonumber\\
kill_many & 0.99999 \nonumber\\
can_and & 0.99999 \nonumber\\
when_we & 0.99999 \nonumber\\
] & 0.99999 \nonumber\\
[ & 0.99999 \nonumber\\
to_and & 0.99999 \nonumber\\
minimal & 0.99999 \nonumber\\
by_a & 0.99999 \nonumber\\
another & 0.99999 \nonumber\\
have_good & 0.99999 \nonumber\\
microsot.com & 0.99999 \nonumber\\
prefer_firefox & 0.99999 \nonumber\\
just_some & 0.99999 \nonumber\\
you_visit & 0.99999 \nonumber\\
greasemonkey_, & 0.99999 \nonumber\\
visit_microsot.com & 0.99999 \nonumber\\
,_greasemonkey & 0.99999 \nonumber\\
,_webdeveloper & 0.99999 \nonumber\\
_pos_ngram_O_V_NP & 0.99999 \nonumber\\
webdeveloper_, & 0.99999 \nonumber\\
ProductionRule_NP->NP,,,NP,,,NP,,,NP,,,NP,,,NP,., & 0.99999 \nonumber\\
some_reason & 0.99999 \nonumber\\
faviconizetab_, & 0.99999 \nonumber\\
firebug & 0.99999 \nonumber\\
tabmix & 0.99999 \nonumber\\
greasemonkey & 0.99999 \nonumber\\
use_when & 0.99999 \nonumber\\
faviconizetab & 0.99999 \nonumber\\
,_tabmix & 0.99999 \nonumber\\
tabmix_, & 0.99999 \nonumber\\
ietab_( & 0.99999 \nonumber\\
firebug_, & 0.99999 \nonumber\\
microsot.com_) & 0.99999 \nonumber\\
ietab & 0.99999 \nonumber\\
,_ietab & 0.99999 \nonumber\\
,_faviconizetab & 0.99999 \nonumber\\
webdeveloper & 0.99999 \nonumber\\
get_all & 0.99999 \nonumber\\
_pos_ngram_PP_V_CONJ & 0.99999 \nonumber\\
care_for & 0.99999 \nonumber\\
the_indian & 0.99999 \nonumber\\
in_our & 0.99999 \nonumber\\
far_. & 0.99999 \nonumber\\
society_. & 0.99999 \nonumber\\
some_people & 0.99999 \nonumber\\
_pos_ngram_CARD_CONJ_PP & 0.99999 \nonumber\\
take_the & 0.99999 \nonumber\\
belief_and & 0.99999 \nonumber\\
student_who & 0.99999 \nonumber\\
the_knowledge & 0.99999 \nonumber\\
we_can & 0.99999 \nonumber\\
ProductionRule_S->``,PP,,,NP,VP,., & 0.99999 \nonumber\\
_pos_ngram_ADV_ADJ_ADV & 0.99999 \nonumber\\
time_of & 0.99999 \nonumber\\
_pos_ngram_ADJ_ART_V & 0.99999 \nonumber\\
ProductionRule_SBARQ->WHADVP,SQ, & 0.99999 \nonumber\\
innovation & 0.99999 \nonumber\\
_pos_ngram_V_NP_O & 0.99999 \nonumber\\
heat_like & 0.99999 \nonumber\\
cold_or & 0.99999 \nonumber\\
cant_save & 0.99999 \nonumber\\
of_cold & 0.99999 \nonumber\\
save_person & 0.99999 \nonumber\\
special_clothe & 0.99999 \nonumber\\
uniform_cant & 0.99999 \nonumber\\
or_heat & 0.99999 \nonumber\\
like_special & 0.99999 \nonumber\\
right_and & 0.99999 \nonumber\\
money_to & 0.99999 \nonumber\\
will_evolve & 0.99999 \nonumber\\
god_create & 0.99999 \nonumber\\
stuff_in & 0.99999 \nonumber\\
a_pain & 0.99999 \nonumber\\
its_too & 0.99999 \nonumber\\
the_mmorn & 0.99999 \nonumber\\
to_clean & 0.99999 \nonumber\\
much_work & 0.99999 \nonumber\\
pain_if & 0.99999 \nonumber\\
of_stuff & 0.99999 \nonumber\\
mix & 0.99999 \nonumber\\
make_them & 0.99999 \nonumber\\
set_of & 0.99999 \nonumber\\
version_of & 0.99999 \nonumber\\
ProductionRule_PRN->-LRB-,PP,-RRB-, & 0.99999 \nonumber\\
issue_in & 0.99999 \nonumber\\
rule & 0.99999 \nonumber\\
only_because & 0.99999 \nonumber\\
on_. & 0.99999 \nonumber\\
would_want & 0.99999 \nonumber\\
or_steve & 0.99999 \nonumber\\
fanboy_. & 0.99999 \nonumber\\
zealot & 0.99999 \nonumber\\
apple_or & 0.99999 \nonumber\\
zealot_fanboy & 0.99999 \nonumber\\
fanatical_zealot & 0.99999 \nonumber\\
with_apple & 0.99999 \nonumber\\
fanatical & 0.99999 \nonumber\\
'd_say & 0.99999 \nonumber\\
steve_job & 0.99999 \nonumber\\
the_fanatical & 0.99999 \nonumber\\
fanboy & 0.99999 \nonumber\\
be_hold & 0.99999 \nonumber\\
know_because & 0.99999 \nonumber\\
to_submit & 0.99999 \nonumber\\
wow_! & 0.99999 \nonumber\\
get_these & 0.99999 \nonumber\\
be_accurate?reply & 0.99999 \nonumber\\
n't_mind & 0.99999 \nonumber\\
these_plz & 0.99999 \nonumber\\
data_be & 0.99999 \nonumber\\
special_data & 0.99999 \nonumber\\
data_, & 0.99999 \nonumber\\
data & 0.99999 \nonumber\\
mind_my & 0.99999 \nonumber\\
submit & 0.99999 \nonumber\\
m_very & 0.99999 \nonumber\\
plz_. & 0.99999 \nonumber\\
soon_! & 0.99999 \nonumber\\
request_you & 0.99999 \nonumber\\
impress_by & 0.99999 \nonumber\\
impress & 0.99999 \nonumber\\
these_unique & 0.99999 \nonumber\\
pt & 0.99999 \nonumber\\
your_view & 0.99999 \nonumber\\
i_kindly & 0.99999 \nonumber\\
more_pt & 0.99999 \nonumber\\
pt_. & 0.99999 \nonumber\\
like_all & 0.99999 \nonumber\\
kindly & 0.99999 \nonumber\\
unique & 0.99999 \nonumber\\
these_special & 0.99999 \nonumber\\
syona_i & 0.99999 \nonumber\\
unique_data & 0.99999 \nonumber\\
kindly_request & 0.99999 \nonumber\\
word_syona & 0.99999 \nonumber\\
submit_more & 0.99999 \nonumber\\
syona_, & 0.99999 \nonumber\\
accurate?reply & 0.99999 \nonumber\\
!_syona & 0.99999 \nonumber\\
accurate?reply_me & 0.99999 \nonumber\\
much_impress & 0.99999 \nonumber\\
._2 & 0.99999 \nonumber\\
ProductionRule_VP->MD,NP,S, & 0.99999 \nonumber\\
topic_. & 0.99999 \nonumber\\
_pos_ngram_ADV_O_CONJ & 0.99999 \nonumber\\
him_around & 0.99999 \nonumber\\
?_which & 0.99999 \nonumber\\
^ & 0.99999 \nonumber\\
*_^ & 0.99999 \nonumber\\
!_firefox & 0.99999 \nonumber\\
advantage & 0.99999 \nonumber\\
speech_, & 0.99999 \nonumber\\
)_, & 0.99999 \nonumber\\
and_people & 0.99999 \nonumber\\
like_this & 0.99999 \nonumber\\
_pos_ngram_NN_O_ART & 0.99999 \nonumber\\
dont_let & 0.99999 \nonumber\\
must_know & 0.99999 \nonumber\\
he_do & 0.99999 \nonumber\\
that_means & 0.99999 \nonumber\\
likely_i & 0.99999 \nonumber\\
such_an & 0.99999 \nonumber\\
and_farquhar & 0.99999 \nonumber\\
and_in & 0.99999 \nonumber\\
not_an & 0.99999 \nonumber\\
country_and & 0.99999 \nonumber\\
therefore_the & 0.99999 \nonumber\\
a_man & 0.99999 \nonumber\\
failure & 0.99999 \nonumber\\
also_be & 0.99999 \nonumber\\
and_by & 0.99999 \nonumber\\
conflict_with & 0.99999 \nonumber\\
baby_be & 0.99999 \nonumber\\
then_that & 0.99999 \nonumber\\
life_could & 0.99999 \nonumber\\
though_sometime & 0.99999 \nonumber\\
but_even & 0.99999 \nonumber\\
be_ready & 0.99999 \nonumber\\
ProductionRule_NP->DT,NN,CC,NN,S, & 0.99999 \nonumber\\
_pos_ngram_PP_ADV_NP & 0.99999 \nonumber\\
become_harder & 0.99999 \nonumber\\
harder_or & 0.99999 \nonumber\\
or_person & 0.99999 \nonumber\\
see_thing & 0.99999 \nonumber\\
sometime_ill & 0.99999 \nonumber\\
ready_for & 0.99999 \nonumber\\
ill_rather & 0.99999 \nonumber\\
image_or & 0.99999 \nonumber\\
about_life & 0.99999 \nonumber\\
ill & 0.99999 \nonumber\\
could_become & 0.99999 \nonumber\\
fatherless_father & 0.99999 \nonumber\\
ProductionRule_NP->RB,NNP, & 0.99999 \nonumber\\
up_life & 0.99999 \nonumber\\
learn_about & 0.99999 \nonumber\\
in_both & 0.99999 \nonumber\\
or_more & 0.99999 \nonumber\\
classic & 0.99999 \nonumber\\
fallacy & 0.99999 \nonumber\\
in_magic & 0.99999 \nonumber\\
ProductionRule_NP->ADVP,NP,SBAR, & 0.99999 \nonumber\\
atheism_; & 0.99999 \nonumber\\
least_some & 0.99999 \nonumber\\
magic_. & 0.99999 \nonumber\\
evidence_before & 0.99999 \nonumber\\
._especially & 0.99999 \nonumber\\
marry_, & 0.99999 \nonumber\\
._second & 0.99999 \nonumber\\
least_have & 0.99999 \nonumber\\
life_with & 0.99999 \nonumber\\
think_have & 0.99999 \nonumber\\
_pos_ngram_CONJ_NP_NP & 0.99999 \nonumber\\
do_then & 0.99999 \nonumber\\
justice & 0.99999 \nonumber\\
justice_for & 0.99999 \nonumber\\
do_here & 0.99999 \nonumber\\
on_earth & 0.99999 \nonumber\\
christian_for & 0.99999 \nonumber\\
bid_deed & 0.99999 \nonumber\\
just_god & 0.99999 \nonumber\\
do_ultimate & 0.99999 \nonumber\\
ultimate_justice & 0.99999 \nonumber\\
for_i & 0.99999 \nonumber\\
_pos_ngram_ART_ADV_NP & 0.99999 \nonumber\\
a_just & 0.99999 \nonumber\\
god_who & 0.99999 \nonumber\\
ProductionRule_NP->DT,RRC, & 0.99999 \nonumber\\
here_on & 0.99999 \nonumber\\
deed_do & 0.99999 \nonumber\\
_pos_ngram_PUNC_ADJ_V & 0.99999 \nonumber\\
think_anybody & 0.99999 \nonumber\\
let_the & 0.99999 \nonumber\\
allow_homosexual & 0.99999 \nonumber\\
file_jointly & 0.99999 \nonumber\\
condone_homosexuality & 0.99999 \nonumber\\
completely_. & 0.99999 \nonumber\\
ProductionRule_S->SBAR,NP,ADVP,VP, & 0.99999 \nonumber\\
irk & 0.99999 \nonumber\\
to_condone & 0.99999 \nonumber\\
homosexuality_let & 0.99999 \nonumber\\
no_tax & 0.99999 \nonumber\\
eye_of & 0.99999 \nonumber\\
church_do & 0.99999 \nonumber\\
homosexual_clergy & 0.99999 \nonumber\\
particular & 0.99999 \nonumber\\
denomination_want & 0.99999 \nonumber\\
n't_support & 0.99999 \nonumber\\
church_perform & 0.99999 \nonumber\\
who_claim & 0.99999 \nonumber\\
denomination & 0.99999 \nonumber\\
against_their & 0.99999 \nonumber\\
no_marry & 0.99999 \nonumber\\
the_eye & 0.99999 \nonumber\\
;_nothing & 0.99999 \nonumber\\
or_incentive & 0.99999 \nonumber\\
deduction_, & 0.99999 \nonumber\\
deduction & 0.99999 \nonumber\\
out_completely & 0.99999 \nonumber\\
clergy & 0.99999 \nonumber\\
'_them & 0.99999 \nonumber\\
clergy_. & 0.99999 \nonumber\\
not_tax & 0.99999 \nonumber\\
jointly & 0.99999 \nonumber\\
any_incentive & 0.99999 \nonumber\\
break_or & 0.99999 \nonumber\\
irk_me & 0.99999 \nonumber\\
of_any & 0.99999 \nonumber\\
perform_marriage & 0.99999 \nonumber\\
politically & 0.99999 \nonumber\\
even_allow & 0.99999 \nonumber\\
it_irk & 0.99999 \nonumber\\
jointly_; & 0.99999 \nonumber\\
,_politically & 0.99999 \nonumber\\
a_particular & 0.99999 \nonumber\\
tax_deduction & 0.99999 \nonumber\\
incentive_to & 0.99999 \nonumber\\
politically_that & 0.99999 \nonumber\\
christian_support & 0.99999 \nonumber\\
particular_denomination & 0.99999 \nonumber\\
support_it & 0.99999 \nonumber\\
care_. & 0.99999 \nonumber\\
government_out & 0.99999 \nonumber\\
marry_file & 0.99999 \nonumber\\
my_church & 0.99999 \nonumber\\
the_guy & 0.99999 \nonumber\\
to_some & 0.99999 \nonumber\\
useful & 0.99999 \nonumber\\
birth & 0.99999 \nonumber\\
tree & 0.99999 \nonumber\\
this_because & 0.99999 \nonumber\\
ProductionRule_S->VP,., & 0.99999 \nonumber\\
vote_for & 0.99999 \nonumber\\
for_them & 0.99999 \nonumber\\
ProductionRule_VP->NP,ADVP, & 0.99999 \nonumber\\
somewhere & 0.99999 \nonumber\\
youth & 0.99999 \nonumber\\
please & 0.99999 \nonumber\\
be_young & 0.99999 \nonumber\\
each_child & 0.99999 \nonumber\\
evolve_? & 0.99999 \nonumber\\
of_happiness & 0.99999 \nonumber\\
religion_. & 0.99999 \nonumber\\
channel & 0.99999 \nonumber\\
school_because & 0.99999 \nonumber\\
state_that & 0.99999 \nonumber\\
can_help & 0.99999 \nonumber\\
before_you & 0.99999 \nonumber\\
a_nervous & 0.99999 \nonumber\\
a_cow & 0.99999 \nonumber\\
fetus_should & 0.99999 \nonumber\\
cow_. & 0.99999 \nonumber\\
cow & 0.99999 \nonumber\\
develop_than & 0.99999 \nonumber\\
think_a & 0.99999 \nonumber\\
cow_should & 0.99999 \nonumber\\
system_much & 0.99999 \nonumber\\
fetus_with & 0.99999 \nonumber\\
have_greater & 0.99999 \nonumber\\
think_she & 0.99999 \nonumber\\
nervous_system & 0.99999 \nonumber\\
nervous & 0.99999 \nonumber\\
of_whether & 0.99999 \nonumber\\
greater_rights & 0.99999 \nonumber\\
mother_should & 0.99999 \nonumber\\
less_develop & 0.99999 \nonumber\\
'_one & 0.99999 \nonumber\\
movie & 0.99999 \nonumber\\
us_then & 0.99999 \nonumber\\
im_a & 0.99999 \nonumber\\
farquer & 0.99999 \nonumber\\
therefore_he & 0.99999 \nonumber\\
outcome & 0.99999 \nonumber\\
area & 0.99999 \nonumber\\
ignorant & 0.99999 \nonumber\\
husband_and & 0.99999 \nonumber\\
help_with & 0.99999 \nonumber\\
see_him & 0.99999 \nonumber\\
proof & 0.99999 \nonumber\\
....._... & 0.99999 \nonumber\\
_pos_ngram_PUNC_PUNC_ART & 0.99999 \nonumber\\
all_these & 0.99999 \nonumber\\
present & 0.99999 \nonumber\\
raffle_do & 0.99999 \nonumber\\
none & 0.99999 \nonumber\\
to_relax & 0.99999 \nonumber\\
relax & 0.99999 \nonumber\\
_pos_ngram_PUNC_PUNC_PR & 0.99999 \nonumber\\
be_highly & 0.99999 \nonumber\\
curb & 0.99999 \nonumber\\
good_. & 0.99999 \nonumber\\
day_and & 0.99999 \nonumber\\
what_ever & 0.99999 \nonumber\\
strict & 0.99999 \nonumber\\
_pos_ngram_ADJ_ADV_NN & 0.99999 \nonumber\\
marriage_. & 0.99999 \nonumber\\
sexism_and & 0.99999 \nonumber\\
sexism & 0.99999 \nonumber\\
racism_, & 0.99999 \nonumber\\
,_sexism & 0.99999 \nonumber\\
racism & 0.99999 \nonumber\\
ProductionRule_NP->DT,VBG,NN, & 0.99999 \nonumber\\
still_have & 0.99999 \nonumber\\
incentive & 0.99999 \nonumber\\
a_negative & 0.99999 \nonumber\\
reason_. & 0.99999 \nonumber\\
ProductionRule_PP->LS,NP, & 0.99999 \nonumber\\
impact_on & 0.99999 \nonumber\\
the_cause & 0.99999 \nonumber\\
na_do & 0.99999 \nonumber\\
_pos_ngram_O_ADJ_PP & 0.99999 \nonumber\\
rights_. & 0.99999 \nonumber\\
not_even & 0.99999 \nonumber\\
lousy_you & 0.99999 \nonumber\\
world_power & 0.99999 \nonumber\\
button & 0.99999 \nonumber\\
property & 0.99999 \nonumber\\
bid_for & 0.99999 \nonumber\\
like_porn & 0.99999 \nonumber\\
how_be & 0.99999 \nonumber\\
class_then & 0.99999 \nonumber\\
good_to & 0.99999 \nonumber\\
be_sack & 0.99999 \nonumber\\
read_. & 0.99999 \nonumber\\
ProductionRule_ADJP->RB,JJ,CC,JJ, & 0.99999 \nonumber\\
kill_her & 0.99999 \nonumber\\
point_out & 0.99999 \nonumber\\
gay & 0.99999 \nonumber\\
deity & 0.99999 \nonumber\\
before_jesus & 0.99999 \nonumber\\
ProductionRule_S->SBAR,,,SBAR,NP,VP,., & 0.99999 \nonumber\\
say_exactly & 0.99999 \nonumber\\
exactly_what & 0.99999 \nonumber\\
year_before & 0.99999 \nonumber\\
send_by & 0.99999 \nonumber\\
write_thousand & 0.99999 \nonumber\\
,_send & 0.99999 \nonumber\\
of_prediction & 0.99999 \nonumber\\
ProductionRule_VP->VBN,NP,PP,VP, & 0.99999 \nonumber\\
by_god & 0.99999 \nonumber\\
come_there & 0.99999 \nonumber\\
prediction_, & 0.99999 \nonumber\\
ProductionRule_NP->NP,,,VP,,,VP, & 0.99999 \nonumber\\
ProductionRule_WHNP->RB,WP, & 0.99999 \nonumber\\
prediction & 0.99999 \nonumber\\
jesus_say & 0.99999 \nonumber\\
jesus_? & 0.99999 \nonumber\\
_pos_ngram_PP_V_O & 0.99999 \nonumber\\
that_should & 0.99999 \nonumber\\
literally & 0.99999 \nonumber\\
not_forget & 0.99999 \nonumber\\
wave & 0.99999 \nonumber\\
child_have & 0.99999 \nonumber\\
limit_. & 0.99999 \nonumber\\
lollollollollollollollollollollollollollollollol_lollollollollollollollollollollollollollollollol & 0.99999 \nonumber\\
_pos_ngram_NP_PR_O & 0.99999 \nonumber\\
it_iz & 0.99999 \nonumber\\
spell_lollollollollollollollollollollollollollollollol & 0.99999 \nonumber\\
ProductionRule_FRAG->NP,NP, & 0.99999 \nonumber\\
harder_to & 0.99999 \nonumber\\
_pos_ngram_PR_O_ADJ & 0.99999 \nonumber\\
suck_because & 0.99999 \nonumber\\
ProductionRule_S->NP,ADJP,S, & 0.99999 \nonumber\\
lollollollollollollollollollollollollollollollol & 0.99999 \nonumber\\
bookz & 0.99999 \nonumber\\
iz & 0.99999 \nonumber\\
bookz_suck & 0.99999 \nonumber\\
iz_harder & 0.99999 \nonumber\\
to_spell & 0.99999 \nonumber\\
ProductionRule_NP->NN,NN,NN,NN, & 0.99999 \nonumber\\
ProductionRule_NP->PRP$,ADJP,NN, & 0.99999 \nonumber\\
who_will & 0.99999 \nonumber\\
_pos_ngram_O_ADJ_PUNC & 0.99999 \nonumber\\
road & 0.99999 \nonumber\\
ProductionRule_NP->RB,NN, & 0.99999 \nonumber\\
hurt_me & 0.99999 \nonumber\\
the_benefit & 0.99999 \nonumber\\
could_go & 0.99999 \nonumber\\
_pos_ngram_O_CONJ_O & 0.99999 \nonumber\\
country_to & 0.99999 \nonumber\\
gallon & 0.99999 \nonumber\\
once_that & 0.99999 \nonumber\\
be_recycle & 0.99999 \nonumber\\
parent_need & 0.99999 \nonumber\\
end_of & 0.99999 \nonumber\\
out_how & 0.99999 \nonumber\\
once_they & 0.99999 \nonumber\\
excuse & 0.99999 \nonumber\\
wow & 0.99999 \nonumber\\
....._.... & 0.99999 \nonumber\\
anywhere & 0.99999 \nonumber\\
when_he & 0.99999 \nonumber\\
and_from & 0.99999 \nonumber\\
_pos_ngram_PR_ART_PP & 0.99999 \nonumber\\
for_christianity & 0.99999 \nonumber\\
argument_for & 0.99999 \nonumber\\
be_responsible & 0.99999 \nonumber\\
friend_. & 0.99999 \nonumber\\
"_who & 0.99999 \nonumber\\
place_in & 0.99999 \nonumber\\
_pos_ngram_NP_ADV_CARD & 0.99999 \nonumber\\
my_mother & 0.99999 \nonumber\\
be_sad & 0.99999 \nonumber\\
attract & 0.99999 \nonumber\\
_pos_ngram_V_O_PP & 0.99999 \nonumber\\
sure_do & 0.99999 \nonumber\\
i_remember & 0.99999 \nonumber\\
ProductionRule_S->SBAR,VP,., & 0.99999 \nonumber\\
on_another & 0.99999 \nonumber\\
no_authority & 0.99999 \nonumber\\
authority_to & 0.99999 \nonumber\\
should_we & 0.99999 \nonumber\\
who_put & 0.99999 \nonumber\\
it_life & 0.99999 \nonumber\\
do_such & 0.99999 \nonumber\\
_pos_ngram_O_PR_PUNC & 0.99999 \nonumber\\
read & 0.99999 \nonumber\\
you_more & 0.99999 \nonumber\\
._spank & 0.99999 \nonumber\\
indian_government & 0.99999 \nonumber\\
and_as & 0.99999 \nonumber\\
let & 0.99999 \nonumber\\
this_prove & 0.99999 \nonumber\\
atheism_be & 0.99999 \nonumber\\
._apart & 0.99999 \nonumber\\
apart_from & 0.99999 \nonumber\\
best_they & 0.99999 \nonumber\\
which_by & 0.99999 \nonumber\\
ProductionRule_SBAR->S,CC,S, & 0.99999 \nonumber\\
winner_" & 0.99999 \nonumber\\
"_winner & 0.99999 \nonumber\\
this_happen & 0.99999 \nonumber\\
top_. & 0.99999 \nonumber\\
the_top & 0.99999 \nonumber\\
be_personal & 0.99999 \nonumber\\
loser_. & 0.99999 \nonumber\\
a_loser & 0.99999 \nonumber\\
someone_have & 0.99999 \nonumber\\
happen_it & 0.99999 \nonumber\\
help_out & 0.99999 \nonumber\\
can_have & 0.99999 \nonumber\\
contribution & 0.99999 \nonumber\\
._god & 0.99999 \nonumber\\
yeah_, & 0.99999 \nonumber\\
year_? & 0.99999 \nonumber\\
,_everyone & 0.99999 \nonumber\\
murder_should & 0.99999 \nonumber\\
dangerous_to & 0.99999 \nonumber\\
ProductionRule_VP->ADVP,VBD,NP,SBAR, & 0.99999 \nonumber\\
that_commit & 0.99999 \nonumber\\
ProductionRule_PP->IN,RB, & 0.99999 \nonumber\\
in_even & 0.99999 \nonumber\\
life_i & 0.99999 \nonumber\\
dont_turn & 0.99999 \nonumber\\
the_enviroment & 0.99999 \nonumber\\
it_dangerous & 0.99999 \nonumber\\
in_how & 0.99999 \nonumber\\
ProductionRule_SBAR->PP,IN,S, & 0.99999 \nonumber\\
again_so & 0.99999 \nonumber\\
that_later & 0.99999 \nonumber\\
a_victim & 0.99999 \nonumber\\
hurst_me & 0.99999 \nonumber\\
definately_turn & 0.99999 \nonumber\\
would_definately & 0.99999 \nonumber\\
hurst & 0.99999 \nonumber\\
it_hurst & 0.99999 \nonumber\\
any_person & 0.99999 \nonumber\\
become_better & 0.99999 \nonumber\\
pass & 0.99999 \nonumber\\
ProductionRule_NP->DT,JJ,NN,SBAR, & 0.99999 \nonumber\\
who_not & 0.99999 \nonumber\\
beleave & 0.99999 \nonumber\\
because_im & 0.99999 \nonumber\\
beleif_because & 0.99999 \nonumber\\
beleif & 0.99999 \nonumber\\
im_christian & 0.99999 \nonumber\\
be_completly & 0.99999 \nonumber\\
your_beleif & 0.99999 \nonumber\\
someone_ele & 0.99999 \nonumber\\
be_but & 0.99999 \nonumber\\
beleave_it & 0.99999 \nonumber\\
ProductionRule_ADJP->RB,PP, & 0.99999 \nonumber\\
christian_i & 0.99999 \nonumber\\
completly_ok & 0.99999 \nonumber\\
ele & 0.99999 \nonumber\\
completly & 0.99999 \nonumber\\
christian_it & 0.99999 \nonumber\\
i_beleave & 0.99999 \nonumber\\
not_christian & 0.99999 \nonumber\\
ProductionRule_PP->CC,PP, & 0.99999 \nonumber\\
ele_who & 0.99999 \nonumber\\
be_compulsaryy & 0.99999 \nonumber\\
day_in & 0.99999 \nonumber\\
wrong_! & 0.99999 \nonumber\\
team_be & 0.99999 \nonumber\\
!!!!!!!!!!!!!!! & 0.99999 \nonumber\\
victim_each & 0.99999 \nonumber\\
!_bully & 0.99999 \nonumber\\
pick_there & 0.99999 \nonumber\\
man_kid & 0.99999 \nonumber\\
fatter_then & 0.99999 \nonumber\\
be_fatter & 0.99999 \nonumber\\
the_affirmative & 0.99999 \nonumber\\
so_man & 0.99999 \nonumber\\
unfit_! & 0.99999 \nonumber\\
!!!!!!!!!!!!!!!_so & 0.99999 \nonumber\\
so_all & 0.99999 \nonumber\\
bully_in & 0.99999 \nonumber\\
guy_on & 0.99999 \nonumber\\
there_victim & 0.99999 \nonumber\\
more_unfit & 0.99999 \nonumber\\
sport_should & 0.99999 \nonumber\\
all_u & 0.99999 \nonumber\\
compulsaryy & 0.99999 \nonumber\\
affirmative_team & 0.99999 \nonumber\\
compulsaryy_!!!!!!!!!!!!!!! & 0.99999 \nonumber\\
affirmative & 0.99999 \nonumber\\
u_guy & 0.99999 \nonumber\\
other_or & 0.99999 \nonumber\\
pe_so & 0.99999 \nonumber\\
bully_pick & 0.99999 \nonumber\\
be_by & 0.99999 \nonumber\\
trust_me & 0.99999 \nonumber\\
grind & 0.99999 \nonumber\\
ff_be & 0.99999 \nonumber\\
develop_country & 0.99999 \nonumber\\
ProductionRule_PP->RB,IN,NP, & 0.99999 \nonumber\\
._those & 0.99999 \nonumber\\
ProductionRule_VP->VBN,ADJP,SBAR, & 0.99999 \nonumber\\
be_kill & 0.99999 \nonumber\\
wear_school & 0.99999 \nonumber\\
if_god & 0.99999 \nonumber\\
obesity_. & 0.99999 \nonumber\\
stranger & 0.99999 \nonumber\\
have_lot & 0.99999 \nonumber\\
post_a & 0.99999 \nonumber\\
this_or & 0.99999 \nonumber\\
alway_baffle & 0.99999 \nonumber\\
who_post & 0.99999 \nonumber\\
people_take & 0.99999 \nonumber\\
"_button & 0.99999 \nonumber\\
..._people & 0.99999 \nonumber\\
button_be & 0.99999 \nonumber\\
button_. & 0.99999 \nonumber\\
see_people & 0.99999 \nonumber\\
one_say & 0.99999 \nonumber\\
and_another & 0.99999 \nonumber\\
a_comment & 0.99999 \nonumber\\
stop_talk & 0.99999 \nonumber\\
or_vote & 0.99999 \nonumber\\
thing_... & 0.99999 \nonumber\\
or_post & 0.99999 \nonumber\\
post_comment & 0.99999 \nonumber\\
care_and & 0.99999 \nonumber\\
comment_to & 0.99999 \nonumber\\
comment_like & 0.99999 \nonumber\\
a_crap & 0.99999 \nonumber\\
vote_on & 0.99999 \nonumber\\
back_button & 0.99999 \nonumber\\
like_mine & 0.99999 \nonumber\\
ProductionRule_SBAR->``,WHNP,S, & 0.99999 \nonumber\\
crap_" & 0.99999 \nonumber\\
browser_' & 0.99999 \nonumber\\
baffle_me & 0.99999 \nonumber\\
baffle & 0.99999 \nonumber\\
mine_make & 0.99999 \nonumber\\
ProductionRule_NP->DT,NN,'',NN, & 0.99999 \nonumber\\
we_cant & 0.99999 \nonumber\\
ProductionRule_S->S,,,S,,,SBAR,., & 0.99999 \nonumber\\
woman_and & 0.99999 \nonumber\\
mainly_because & 0.99999 \nonumber\\
separate_way & 0.99999 \nonumber\\
go_our & 0.99999 \nonumber\\
truthfully_i & 0.99999 \nonumber\\
in_i & 0.99999 \nonumber\\
know_part & 0.99999 \nonumber\\
our_separate & 0.99999 \nonumber\\
know_in & 0.99999 \nonumber\\
but_truthfully & 0.99999 \nonumber\\
have_know & 0.99999 \nonumber\\
no_. & 0.99999 \nonumber\\
over_it & 0.99999 \nonumber\\
drop & 0.99999 \nonumber\\
etc. & 0.99999 \nonumber\\
people_, & 0.99999 \nonumber\\
'_what & 0.99999 \nonumber\\
advantage_. & 0.99999 \nonumber\\
to_drink & 0.99999 \nonumber\\
race & 0.99999 \nonumber\\
assistant_" & 0.99999 \nonumber\\
assistant & 0.99999 \nonumber\\
work_but & 0.99999 \nonumber\\
even_do & 0.99999 \nonumber\\
singapore_therefore & 0.99999 \nonumber\\
this_help & 0.99999 \nonumber\\
island_first & 0.99999 \nonumber\\
ProductionRule_NP->``,NNS,'', & 0.99999 \nonumber\\
consult_raffle & 0.99999 \nonumber\\
but_let & 0.99999 \nonumber\\
prince & 0.99999 \nonumber\\
very_involve & 0.99999 \nonumber\\
give_credit & 0.99999 \nonumber\\
authority_over & 0.99999 \nonumber\\
"_assistant & 0.99999 \nonumber\\
singapore_! & 0.99999 \nonumber\\
institution_" & 0.99999 \nonumber\\
prince_sanilum & 0.99999 \nonumber\\
do_know & 0.99999 \nonumber\\
"_discover & 0.99999 \nonumber\\
"_he & 0.99999 \nonumber\\
ask_u & 0.99999 \nonumber\\
some_who & 0.99999 \nonumber\\
ProductionRule_SBAR->IN,RB,S, & 0.99999 \nonumber\\
farquer_have & 0.99999 \nonumber\\
utama & 0.99999 \nonumber\\
that_farquer & 0.99999 \nonumber\\
all_authority & 0.99999 \nonumber\\
sanilum & 0.99999 \nonumber\\
sanilum_utama & 0.99999 \nonumber\\
credit_. & 0.99999 \nonumber\\
question_why & 0.99999 \nonumber\\
place_if & 0.99999 \nonumber\\
clinic & 0.99999 \nonumber\\
clinic_" & 0.99999 \nonumber\\
sometime_even & 0.99999 \nonumber\\
_pos_ngram_NN_PR_O & 0.99999 \nonumber\\
(_this & 0.99999 \nonumber\\
first_) & 0.99999 \nonumber\\
the_prince & 0.99999 \nonumber\\
utama_be & 0.99999 \nonumber\\
raffle_hospital & 0.99999 \nonumber\\
over_singapore & 0.99999 \nonumber\\
_pos_ngram_O_ART_PP & 0.99999 \nonumber\\
say_farquhar & 0.99999 \nonumber\\
"_raffle & 0.99999 \nonumber\\
discover_" & 0.99999 \nonumber\\
why_then & 0.99999 \nonumber\\
u_a & 0.99999 \nonumber\\
me_remind & 0.99999 \nonumber\\
he_still & 0.99999 \nonumber\\
to_consult & 0.99999 \nonumber\\
medical_clinic & 0.99999 \nonumber\\
raffle_" & 0.99999 \nonumber\\
hospital_" & 0.99999 \nonumber\\
name_" & 0.99999 \nonumber\\
raffle_medical & 0.99999 \nonumber\\
farquhar_see & 0.99999 \nonumber\\
ship & 0.99999 \nonumber\\
so_people & 0.99999 \nonumber\\
to_post & 0.99999 \nonumber\\
be_say & 0.99999 \nonumber\\
d_hub & 0.99999 \nonumber\\
uk & 0.99999 \nonumber\\
,_uk & 0.99999 \nonumber\\
_pos_ngram_NP_CONJ_ADJ & 0.99999 \nonumber\\
weapon_do & 0.99999 \nonumber\\
d_potential & 0.99999 \nonumber\\
more_strong.it & 0.99999 \nonumber\\
company_. & 0.99999 \nonumber\\
or_such & 0.99999 \nonumber\\
economically_more & 0.99999 \nonumber\\
such_other & 0.99999 \nonumber\\
_pos_ngram_O_ADV_NP & 0.99999 \nonumber\\
weapon & 0.99999 \nonumber\\
d_world & 0.99999 \nonumber\\
....._maybe & 0.99999 \nonumber\\
contry & 0.99999 \nonumber\\
certainly_have & 0.99999 \nonumber\\
other_company & 0.99999 \nonumber\\
and_weapon & 0.99999 \nonumber\\
strong.it_be & 0.99999 \nonumber\\
strong.it & 0.99999 \nonumber\\
hub_4 & 0.99999 \nonumber\\
have_d & 0.99999 \nonumber\\
other_contry & 0.99999 \nonumber\\
be_d & 0.99999 \nonumber\\
be_economically & 0.99999 \nonumber\\
more_maybe & 0.99999 \nonumber\\
maybe_..... & 0.99999 \nonumber\\
maybe_usa & 0.99999 \nonumber\\
_pos_ngram_CARD_ADJ_ADJ & 0.99999 \nonumber\\
but_indium & 0.99999 \nonumber\\
4_many & 0.99999 \nonumber\\
2_lead & 0.99999 \nonumber\\
potential_2 & 0.99999 \nonumber\\
work_any & 0.99999 \nonumber\\
lead_d & 0.99999 \nonumber\\
uk_or & 0.99999 \nonumber\\
contry_be & 0.99999 \nonumber\\
powerful_but & 0.99999 \nonumber\\
indium_certainly & 0.99999 \nonumber\\
will_alway & 0.99999 \nonumber\\
install & 0.99999 \nonumber\\
ProductionRule_NP->NNP,NNP,NNP, & 0.99999 \nonumber\\
_pos_ngram_NP_V_O & 0.99999 \nonumber\\
,_leave & 0.99999 \nonumber\\
relationship & 0.99999 \nonumber\\
_pos_ngram_ART_PUNC_ART & 0.99999 \nonumber\\
100 & 0.99999 \nonumber\\
because_what & 0.99999 \nonumber\\
indium_will & 0.99999 \nonumber\\
than_yourself & 0.99999 \nonumber\\
approve & 0.99999 \nonumber\\
an_individual & 0.99999 \nonumber\\
._gene & 0.99999 \nonumber\\
accept_to & 0.99999 \nonumber\\
many_option & 0.99999 \nonumber\\
mouth_to & 0.99999 \nonumber\\
option_that & 0.99999 \nonumber\\
speak_and & 0.99999 \nonumber\\
parent_can & 0.99999 \nonumber\\
wrong_from & 0.99999 \nonumber\\
a_mouth & 0.99999 \nonumber\\
how_would & 0.99999 \nonumber\\
and_what & 0.99999 \nonumber\\
invest & 0.99999 \nonumber\\
position_to & 0.99999 \nonumber\\
like_rob & 0.99999 \nonumber\\
small_police & 0.99999 \nonumber\\
rob & 0.99999 \nonumber\\
ProductionRule_UCP->PP,CC,VP, & 0.99999 \nonumber\\
rob_and & 0.99999 \nonumber\\
fight_often & 0.99999 \nonumber\\
crime_like & 0.99999 \nonumber\\
farquhar_set & 0.99999 \nonumber\\
science_. & 0.99999 \nonumber\\
young_they & 0.99999 \nonumber\\
what_wrong & 0.99999 \nonumber\\
teach_the & 0.99999 \nonumber\\
right_the & 0.99999 \nonumber\\
child_from & 0.99999 \nonumber\\
do_tell & 0.99999 \nonumber\\
wear_what & 0.99999 \nonumber\\
them_that & 0.99999 \nonumber\\
more_likely & 0.99999 \nonumber\\
a_funny & 0.99999 \nonumber\\
can_switch & 0.99999 \nonumber\\
and_ready & 0.99999 \nonumber\\
think_tv & 0.99999 \nonumber\\
learn_and & 0.99999 \nonumber\\
informational & 0.99999 \nonumber\\
relax_you & 0.99999 \nonumber\\
an_informational & 0.99999 \nonumber\\
documentary_on & 0.99999 \nonumber\\
different_informational & 0.99999 \nonumber\\
different_subject & 0.99999 \nonumber\\
watch_an & 0.99999 \nonumber\\
channel_and & 0.99999 \nonumber\\
an_search & 0.99999 \nonumber\\
informational_channel & 0.99999 \nonumber\\
channel_an & 0.99999 \nonumber\\
ever_you & 0.99999 \nonumber\\
subject_and & 0.99999 \nonumber\\
search_documentary & 0.99999 \nonumber\\
funny_show & 0.99999 \nonumber\\
that_so & 0.99999 \nonumber\\
bedroom & 0.99999 \nonumber\\
the_bedroom & 0.99999 \nonumber\\
beverage & 0.99999 \nonumber\\
should_spank & 0.99999 \nonumber\\
they_cant & 0.99999 \nonumber\\
physical_exercise & 0.99999 \nonumber\\
fish_be & 0.99999 \nonumber\\
status & 0.99999 \nonumber\\
to_deal & 0.99999 \nonumber\\
by_day & 0.99999 \nonumber\\
day_by & 0.99999 \nonumber\\
,_gay & 0.99999 \nonumber\\
empire & 0.99999 \nonumber\\
islam & 0.99999 \nonumber\\
,_judaism & 0.99999 \nonumber\\
islam_, & 0.99999 \nonumber\\
hinduism & 0.99999 \nonumber\\
buddhism & 0.99999 \nonumber\\
hinduism_, & 0.99999 \nonumber\\
daughter_. & 0.99999 \nonumber\\
plastic_bottle & 0.99999 \nonumber\\
_pos_ngram_PUNC_PR_NN & 0.99999 \nonumber\\
_pos_ngram_NN_NP_ADV & 0.99999 \nonumber\\
where_do & 0.99999 \nonumber\\
apple & 0.99999 \nonumber\\
have_personal & 0.99999 \nonumber\\
a_schoolgirl & 0.99999 \nonumber\\
schoolgirl & 0.99999 \nonumber\\
maintain_that & 0.99999 \nonumber\\
schoolgirl_, & 0.99999 \nonumber\\
and_respectful & 0.99999 \nonumber\\
alway_like & 0.99999 \nonumber\\
the_status & 0.99999 \nonumber\\
very_nice & 0.99999 \nonumber\\
alway_maintain & 0.99999 \nonumber\\
uniform_at & 0.99999 \nonumber\\
respectful_. & 0.99999 \nonumber\\
adopt & 0.99999 \nonumber\\
be_catch & 0.99999 \nonumber\\
' & 0.99999 \nonumber\\
alway_look & 0.99999 \nonumber\\
n't_allow & 0.99999 \nonumber\\
bible & 0.99999 \nonumber\\
it_can & 0.99999 \nonumber\\
be_obese & 0.99999 \nonumber\\
spank_your & 0.99999 \nonumber\\
winner & 0.99999 \nonumber\\
be_female & 0.99999 \nonumber\\
to_rest & 0.99999 \nonumber\\
about_than & 0.99999 \nonumber\\
kill_him/her & 0.99999 \nonumber\\
my_self & 0.99999 \nonumber\\
allow_my & 0.99999 \nonumber\\
by_accident & 0.99999 \nonumber\\
that_out & 0.99999 \nonumber\\
murder_your & 0.99999 \nonumber\\
on_purpose & 0.99999 \nonumber\\
figure_that & 0.99999 \nonumber\\
police_will & 0.99999 \nonumber\\
self_to & 0.99999 \nonumber\\
spouse_murder & 0.99999 \nonumber\\
life_their & 0.99999 \nonumber\\
until_i & 0.99999 \nonumber\\
accident_than & 0.99999 \nonumber\\
would_, & 0.99999 \nonumber\\
._weather & 0.99999 \nonumber\\
him/her & 0.99999 \nonumber\\
will_figure & 0.99999 \nonumber\\
or_on & 0.99999 \nonumber\\
him/her_? & 0.99999 \nonumber\\
they_tell & 0.99999 \nonumber\\
purpose_. & 0.99999 \nonumber\\
rest_until & 0.99999 \nonumber\\
actor & 0.99999 \nonumber\\
fate & 0.99999 \nonumber\\
hell & 0.99999 \nonumber\\
to_call & 0.99999 \nonumber\\
ProductionRule_VP->VP,CC,ADVP,VP, & 0.99999 \nonumber\\
hard_time & 0.99999 \nonumber\\
50 & 0.99999 \nonumber\\
it_feel & 0.99999 \nonumber\\
afraid & 0.99999 \nonumber\\
personal_opinion & 0.99999 \nonumber\\
quote & 0.99999 \nonumber\\
_pos_ngram_ADV_CONJ_PR & 0.99999 \nonumber\\
be_base & 0.99999 \nonumber\\
be_successful & 0.99999 \nonumber\\
therefore_should & 0.99999 \nonumber\\
ProductionRule_VP->ADVP,MD,RB,VP, & 0.99999 \nonumber\\
waste_of & 0.99999 \nonumber\\
._however & 0.99999 \nonumber\\
our_world & 0.99999 \nonumber\\
ProductionRule_NP->NNS,CC,NNS, & 0.99999 \nonumber\\
god_have & 0.99999 \nonumber\\
matter_how & 0.99999 \nonumber\\
_pos_ngram_ADV_NP_PR & 0.99999 \nonumber\\
get_lay & 0.99999 \nonumber\\
first_of & 0.99999 \nonumber\\
until_the & 0.99999 \nonumber\\
ProductionRule_NP->CD,JJ,NN, & 0.99999 \nonumber\\
ProductionRule_QP->RB,DT, & 0.99999 \nonumber\\
reside & 0.99999 \nonumber\\
reside_here & 0.99999 \nonumber\\
of_world & 0.99999 \nonumber\\
easily_lead & 0.99999 \nonumber\\
secular_state.people & 0.99999 \nonumber\\
a_secular & 0.99999 \nonumber\\
create_any & 0.99999 \nonumber\\
among_anyone & 0.99999 \nonumber\\
lead_all & 0.99999 \nonumber\\
any_nuissance & 0.99999 \nonumber\\
all_country & 0.99999 \nonumber\\
so_indium & 0.99999 \nonumber\\
all_community & 0.99999 \nonumber\\
state.people_of & 0.99999 \nonumber\\
of_almost & 0.99999 \nonumber\\
state.people & 0.99999 \nonumber\\
they_live & 0.99999 \nonumber\\
world_without & 0.99999 \nonumber\\
almost_all & 0.99999 \nonumber\\
nuissance & 0.99999 \nonumber\\
community_reside & 0.99999 \nonumber\\
nuissance_among & 0.99999 \nonumber\\
without_create & 0.99999 \nonumber\\
by_say & 0.99999 \nonumber\\
lightly & 0.99999 \nonumber\\
admit_it & 0.99999 \nonumber\\
14 & 0.99999 \nonumber\\
be_14 & 0.99999 \nonumber\\
14_year & 0.99999 \nonumber\\
before & 0.99999 \nonumber\\
._television & 0.99999 \nonumber\\
mention_that & 0.99999 \nonumber\\
a_place & 0.99999 \nonumber\\
documentary & 0.99999 \nonumber\\
to_them & 0.99999 \nonumber\\
father_would & 0.99999 \nonumber\\
play & 0.99999 \nonumber\\
power_and & 0.99999 \nonumber\\
ProductionRule_NP->NNP,NNP,NNP,NNP, & 0.99999 \nonumber\\
,_spank & 0.99999 \nonumber\\
be_never & 0.99999 \nonumber\\
ProductionRule_NP->CD,NN,NNS, & 0.99999 \nonumber\\
"_and & 0.99999 \nonumber\\
this_, & 0.99999 \nonumber\\
fix & 0.99999 \nonumber\\
use_firefox & 0.99999 \nonumber\\
mistake_in & 0.99999 \nonumber\\
_pos_ngram_ADJ_O_ADJ & 0.99999 \nonumber\\
be_from & 0.99999 \nonumber\\
science_be & 0.99999 \nonumber\\
show_how & 0.99999 \nonumber\\
browser_with & 0.99999 \nonumber\\
world_could & 0.99999 \nonumber\\
exceedingly_likely & 0.99999 \nonumber\\
exceedingly & 0.99999 \nonumber\\
giant & 0.99999 \nonumber\\
a_giant & 0.99999 \nonumber\\
http://www.newscientist.com/article/mg20126911.300-our-world-may-be-a-giant-hologram.html & 0.99999 \nonumber\\
http://www.newscientist.com/article/mg20126911.300-our-world-may-be-a-giant-hologram.html_it & 0.99999 \nonumber\\
hologram_http://www.newscientist.com/article/mg20126911.300-our-world-may-be-a-giant-hologram.html & 0.99999 \nonumber\\
simulate & 0.99999 \nonumber\\
hologram & 0.99999 \nonumber\\
giant_hologram & 0.99999 \nonumber\\
simulate_universe & 0.99999 \nonumber\\
be_exceedingly & 0.99999 \nonumber\\
a_simulate & 0.99999 \nonumber\\
against_it & 0.99999 \nonumber\\
ProductionRule_S->S,,,S,CC,S, & 0.99999 \nonumber\\
call_" & 0.99999 \nonumber\\
invent & 0.99999 \nonumber\\
fire_. & 0.99999 \nonumber\\
throw_my & 0.99999 \nonumber\\
the_sink & 0.99999 \nonumber\\
your_stuff & 0.99999 \nonumber\\
much_that & 0.99999 \nonumber\\
and_search & 0.99999 \nonumber\\
n't_pry & 0.99999 \nonumber\\
'_actually & 0.99999 \nonumber\\
my_backpack & 0.99999 \nonumber\\
n't_clean & 0.99999 \nonumber\\
care_so & 0.99999 \nonumber\\
room_and & 0.99999 \nonumber\\
or_i & 0.99999 \nonumber\\
after_breakfast & 0.99999 \nonumber\\
forget_my & 0.99999 \nonumber\\
hate_you & 0.99999 \nonumber\\
my_computer & 0.99999 \nonumber\\
doesnt_think & 0.99999 \nonumber\\
a_wall & 0.99999 \nonumber\\
will_tell & 0.99999 \nonumber\\
backpack & 0.99999 \nonumber\\
every_mistake & 0.99999 \nonumber\\
and_throw & 0.99999 \nonumber\\
it_at & 0.99999 \nonumber\\
he_wo & 0.99999 \nonumber\\
mistake_you & 0.99999 \nonumber\\
he_wouldnt & 0.99999 \nonumber\\
need_it & 0.99999 \nonumber\\
i_forget & 0.99999 \nonumber\\
piss_and & 0.99999 \nonumber\\
practical & 0.99999 \nonumber\\
computer_in & 0.99999 \nonumber\\
blame_every & 0.99999 \nonumber\\
father_for & 0.99999 \nonumber\\
sink_after & 0.99999 \nonumber\\
get_piss & 0.99999 \nonumber\\
into_your & 0.99999 \nonumber\\
business_and & 0.99999 \nonumber\\
i_ruin & 0.99999 \nonumber\\
search_your & 0.99999 \nonumber\\
practical_reason & 0.99999 \nonumber\\
can_blame & 0.99999 \nonumber\\
backpack_with & 0.99999 \nonumber\\
actually_an & 0.99999 \nonumber\\
still_lousy & 0.99999 \nonumber\\
wall_put & 0.99999 \nonumber\\
for_practical & 0.99999 \nonumber\\
pry_into & 0.99999 \nonumber\\
pry & 0.99999 \nonumber\\
wouldnt_care & 0.99999 \nonumber\\
my_key & 0.99999 \nonumber\\
breakfast_or & 0.99999 \nonumber\\
your_room & 0.99999 \nonumber\\
make_on & 0.99999 \nonumber\\
breakfast & 0.99999 \nonumber\\
key_. & 0.99999 \nonumber\\
your_business & 0.99999 \nonumber\\
ruin_his & 0.99999 \nonumber\\
stuff_because & 0.99999 \nonumber\\
he_doesnt & 0.99999 \nonumber\\
fetus_be & 0.99999 \nonumber\\
series_of & 0.99999 \nonumber\\
series & 0.99999 \nonumber\\
trust & 0.99999 \nonumber\\
bigote & 0.99999 \nonumber\\
not_worship & 0.99999 \nonumber\\
narcissistic & 0.99999 \nonumber\\
biggot_plain & 0.99999 \nonumber\\
narcissistic_, & 0.99999 \nonumber\\
totally_bigote & 0.99999 \nonumber\\
biggot & 0.99999 \nonumber\\
bigote_and & 0.99999 \nonumber\\
and_intolerant & 0.99999 \nonumber\\
,_narcissistic & 0.99999 \nonumber\\
worship_as & 0.99999 \nonumber\\
atheist_who & 0.99999 \nonumber\\
cant_leave & 0.99999 \nonumber\\
ProductionRule_UCP->ADJP,,,VP,CC,RB,NP, & 0.99999 \nonumber\\
to_worship & 0.99999 \nonumber\\
athieist & 0.99999 \nonumber\\
ProductionRule_VP->VBD,PRT, & 0.99999 \nonumber\\
people_belief & 0.99999 \nonumber\\
leave_people & 0.99999 \nonumber\\
concede & 0.99999 \nonumber\\
concede_, & 0.99999 \nonumber\\
worship_or & 0.99999 \nonumber\\
prove_be & 0.99999 \nonumber\\
intolerant_of & 0.99999 \nonumber\\
,_stick & 0.99999 \nonumber\\
ProductionRule_S->S,,,S,,,S, & 0.99999 \nonumber\\
of_concede & 0.99999 \nonumber\\
intolerant & 0.99999 \nonumber\\
debate_prove & 0.99999 \nonumber\\
,_atheist & 0.99999 \nonumber\\
athieist_be & 0.99999 \nonumber\\
people_alone & 0.99999 \nonumber\\
choose_athieist & 0.99999 \nonumber\\
be_biggot & 0.99999 \nonumber\\
alone_to & 0.99999 \nonumber\\
ProductionRule_NP->JJ,NNS,NNS, & 0.99999 \nonumber\\
ProductionRule_NP->NP,NP,., & 0.99999 \nonumber\\
unity & 0.99999 \nonumber\\
raffle_have & 0.99999 \nonumber\\
still_if & 0.99999 \nonumber\\
way_better & 0.99999 \nonumber\\
along & 0.99999 \nonumber\\
n't_around & 0.99999 \nonumber\\
_pos_ngram_PP_ADJ_PP & 0.99999 \nonumber\\
one_ever & 0.99999 \nonumber\\
rate_? & 0.99999 \nonumber\\
this_up & 0.99999 \nonumber\\
everyone_have & 0.99999 \nonumber\\
both_the & 0.99999 \nonumber\\
with_everything & 0.99999 \nonumber\\
significantly & 0.99999 \nonumber\\
it_on & 0.99999 \nonumber\\
up_the & 0.99999 \nonumber\\
switch_to & 0.99999 \nonumber\\
switch & 0.99999 \nonumber\\
and_never & 0.99999 \nonumber\\
and_abuse & 0.99999 \nonumber\\
school_work & 0.99999 \nonumber\\
much_less & 0.99999 \nonumber\\
research_behind & 0.99999 \nonumber\\
5_on & 0.99999 \nonumber\\
be_# & 0.99999 \nonumber\\
wing/conservative_group & 0.99999 \nonumber\\
i_recall & 0.99999 \nonumber\\
especially_against & 0.99999 \nonumber\\
those_three & 0.99999 \nonumber\\
your_link & 0.99999 \nonumber\\
your_list & 0.99999 \nonumber\\
site_to & 0.99999 \nonumber\\
bar_on & 0.99999 \nonumber\\
try_' & 0.99999 \nonumber\\
a_poll & 0.99999 \nonumber\\
three_be & 0.99999 \nonumber\\
three_of & 0.99999 \nonumber\\
at_hand & 0.99999 \nonumber\\
argument_at & 0.99999 \nonumber\\
right_wing/conservative & 0.99999 \nonumber\\
recall_and & 0.99999 \nonumber\\
their_writings & 0.99999 \nonumber\\
'_try & 0.99999 \nonumber\\
wing/conservative & 0.99999 \nonumber\\
#_5 & 0.99999 \nonumber\\
recall & 0.99999 \nonumber\\
writings_. & 0.99999 \nonumber\\
write_intelligently & 0.99999 \nonumber\\
3_, & 0.99999 \nonumber\\
and_# & 0.99999 \nonumber\\
and_' & 0.99999 \nonumber\\
bias & 0.99999 \nonumber\\
1_have & 0.99999 \nonumber\\
bias_. & 0.99999 \nonumber\\
real_bar & 0.99999 \nonumber\\
link_be & 0.99999 \nonumber\\
poll_company & 0.99999 \nonumber\\
extremely_bias & 0.99999 \nonumber\\
2_be & 0.99999 \nonumber\\
list_. & 0.99999 \nonumber\\
have_research & 0.99999 \nonumber\\
writings & 0.99999 \nonumber\\
behind_their & 0.99999 \nonumber\\
2_, & 0.99999 \nonumber\\
poll & 0.99999 \nonumber\\
company_, & 0.99999 \nonumber\\
he_hate & 0.99999 \nonumber\\
would_become & 0.99999 \nonumber\\
your_brain & 0.99999 \nonumber\\
discovery_of & 0.99999 \nonumber\\
a_waste & 0.99999 \nonumber\\
subject_. & 0.99999 \nonumber\\
love_we & 0.99999 \nonumber\\
_pos_ngram_PP_ADJ_NP & 0.99999 \nonumber\\
n't_that & 0.99999 \nonumber\\
to_me & 0.99999 \nonumber\\
_pos_ngram_ADJ_ART_ADJ & 0.99999 \nonumber\\
be_natural & 0.99999 \nonumber\\
;_the & 0.99999 \nonumber\\
!_people & 0.99999 \nonumber\\
the_chance & 0.99999 \nonumber\\
and_she & 0.99999 \nonumber\\
big_question & 0.99999 \nonumber\\
time_didnt & 0.99999 \nonumber\\
excuse_make & 0.99999 \nonumber\\
science_have & 0.99999 \nonumber\\
no_god & 0.99999 \nonumber\\
on_those & 0.99999 \nonumber\\
from_simplier & 0.99999 \nonumber\\
didnt & 0.99999 \nonumber\\
think_to & 0.99999 \nonumber\\
up_so & 0.99999 \nonumber\\
didnt_have & 0.99999 \nonumber\\
simplier & 0.99999 \nonumber\\
simplier_time & 0.99999 \nonumber\\
,_along & 0.99999 \nonumber\\
wall & 0.99999 \nonumber\\
idea_. & 0.99999 \nonumber\\
than_that & 0.99999 \nonumber\\
a_million & 0.99999 \nonumber\\
million_people & 0.99999 \nonumber\\
_pos_ngram_NP_NP_PP & 0.99999 \nonumber\\
bt & 0.99999 \nonumber\\
way_! & 0.99999 \nonumber\\
that_book & 0.99999 \nonumber\\
go_out & 0.99999 \nonumber\\
but_the & 0.99999 \nonumber\\
really_have & 0.99999 \nonumber\\
good_! & 0.99999 \nonumber\\
ProductionRule_NP->NP,,,RB,NP, & 0.99999 \nonumber\\
just_raffle & 0.99999 \nonumber\\
subordinate_. & 0.99999 \nonumber\\
not_farquhar & 0.99999 \nonumber\\
the_treaty & 0.99999 \nonumber\\
raffle_subordinate & 0.99999 \nonumber\\
raffle_who & 0.99999 \nonumber\\
hussein_, & 0.99999 \nonumber\\
sign_the & 0.99999 \nonumber\\
bear_with & 0.99999 \nonumber\\
property_" & 0.99999 \nonumber\\
ProductionRule_NP->NP,:,``,SBAR, & 0.99999 \nonumber\\
species_have & 0.99999 \nonumber\\
magically_grow & 0.99999 \nonumber\\
n't_bear & 0.99999 \nonumber\\
point_- & 0.99999 \nonumber\\
you_prove & 0.99999 \nonumber\\
everything_... & 0.99999 \nonumber\\
it_magically & 0.99999 \nonumber\\
ProductionRule_ADVP->RB,'', & 0.99999 \nonumber\\
characteristic_randomly & 0.99999 \nonumber\\
characteristic_and & 0.99999 \nonumber\\
"_species & 0.99999 \nonumber\\
animal_aquire & 0.99999 \nonumber\\
hard_and & 0.99999 \nonumber\\
you_talk & 0.99999 \nonumber\\
outside_my & 0.99999 \nonumber\\
prove_my & 0.99999 \nonumber\\
certain_characteristic & 0.99999 \nonumber\\
their_characteristic & 0.99999 \nonumber\\
sure_squirrel & 0.99999 \nonumber\\
an_animal & 0.99999 \nonumber\\
and_property & 0.99999 \nonumber\\
i_notice & 0.99999 \nonumber\\
a_curious & 0.99999 \nonumber\\
do_an & 0.99999 \nonumber\\
person_... & 0.99999 \nonumber\\
a_trait & 0.99999 \nonumber\\
n't_mention & 0.99999 \nonumber\\
have_look & 0.99999 \nonumber\\
insect & 0.99999 \nonumber\\
trait_that & 0.99999 \nonumber\\
trait & 0.99999 \nonumber\\
randomly_change & 0.99999 \nonumber\\
curious_person & 0.99999 \nonumber\\
randomly & 0.99999 \nonumber\\
just_wonder & 0.99999 \nonumber\\
aquire & 0.99999 \nonumber\\
aquire_a & 0.99999 \nonumber\\
really_hard & 0.99999 \nonumber\\
your_best & 0.99999 \nonumber\\
window_evolve & 0.99999 \nonumber\\
argument_- & 0.99999 \nonumber\\
notice_you & 0.99999 \nonumber\\
grow_? & 0.99999 \nonumber\\
same_for & 0.99999 \nonumber\\
squirrel_outside & 0.99999 \nonumber\\
squirrel_have & 0.99999 \nonumber\\
squirrel & 0.99999 \nonumber\\
wonder_because & 0.99999 \nonumber\\
my_window & 0.99999 \nonumber\\
-_" & 0.99999 \nonumber\\
wish_for & 0.99999 \nonumber\\
just_wish & 0.99999 \nonumber\\
insect_be & 0.99999 \nonumber\\
n't_" & 0.99999 \nonumber\\
best_argument & 0.99999 \nonumber\\
with_? & 0.99999 \nonumber\\
what_insect & 0.99999 \nonumber\\
act_the & 0.99999 \nonumber\\
have_certain & 0.99999 \nonumber\\
the_squirrel & 0.99999 \nonumber\\
about_? & 0.99999 \nonumber\\
an_option & 0.99999 \nonumber\\
_pos_ngram_CONJ_O_O & 0.99999 \nonumber\\
really_it & 0.99999 \nonumber\\
magically & 0.99999 \nonumber\\
to_pay & 0.99999 \nonumber\\
not_help & 0.99999 \nonumber\\
embryo_be & 0.99999 \nonumber\\
gain_one & 0.99999 \nonumber\\
embryo & 0.99999 \nonumber\\
the_heartbeat & 0.99999 \nonumber\\
your_rape & 0.99999 \nonumber\\
._around & 0.99999 \nonumber\\
human_with & 0.99999 \nonumber\\
rape_. & 0.99999 \nonumber\\
as_early & 0.99999 \nonumber\\
adoption_instead & 0.99999 \nonumber\\
rape_do & 0.99999 \nonumber\\
21st_day & 0.99999 \nonumber\\
marry_woman & 0.99999 \nonumber\\
instead_, & 0.99999 \nonumber\\
60_% & 0.99999 \nonumber\\
60 & 0.99999 \nonumber\\
form_, & 0.99999 \nonumber\\
grow_embryo & 0.99999 \nonumber\\
as_21st & 0.99999 \nonumber\\
on_never & 0.99999 \nonumber\\
conception_. & 0.99999 \nonumber\\
ProductionRule_VP->VBN,ADJP,PP, & 0.99999 \nonumber\\
around_60 & 0.99999 \nonumber\\
woman_give & 0.99999 \nonumber\\
n't_woman & 0.99999 \nonumber\\
heartbeat_initiate & 0.99999 \nonumber\\
initiate_as & 0.99999 \nonumber\\
heartbeat & 0.99999 \nonumber\\
human_form & 0.99999 \nonumber\\
be_perform & 0.99999 \nonumber\\
someone_? & 0.99999 \nonumber\\
early_as & 0.99999 \nonumber\\
initiate & 0.99999 \nonumber\\
perform_on & 0.99999 \nonumber\\
never_marry & 0.99999 \nonumber\\
of_conception & 0.99999 \nonumber\\
unprotect & 0.99999 \nonumber\\
say_i & 0.99999 \nonumber\\
right_in & 0.99999 \nonumber\\
form_of & 0.99999 \nonumber\\
vote & 0.99999 \nonumber\\
me_sick & 0.99999 \nonumber\\
sick_. & 0.99999 \nonumber\\
despite & 0.99999 \nonumber\\
all_day & 0.99999 \nonumber\\
and_book & 0.99999 \nonumber\\
of_indium & 0.99999 \nonumber\\
personality & 0.99999 \nonumber\\
than_spend & 0.99999 \nonumber\\
wonder_who & 0.99999 \nonumber\\
up_fatherless & 0.99999 \nonumber\\
tranquility & 0.99999 \nonumber\\
fatherless_i & 0.99999 \nonumber\\
spend_my & 0.99999 \nonumber\\
emptiness & 0.99999 \nonumber\\
life_wonder & 0.99999 \nonumber\\
emptiness_in & 0.99999 \nonumber\\
be_than & 0.99999 \nonumber\\
an_emptiness & 0.99999 \nonumber\\
tranquility_of & 0.99999 \nonumber\\
the_tranquility & 0.99999 \nonumber\\
mistake_than & 0.99999 \nonumber\\
would_grow & 0.99999 \nonumber\\
grow_with & 0.99999 \nonumber\\
and_learn & 0.99999 \nonumber\\
my_whole & 0.99999 \nonumber\\
with_an & 0.99999 \nonumber\\
prefer_grow & 0.99999 \nonumber\\
would_at & 0.99999 \nonumber\\
to_anything & 0.99999 \nonumber\\
dad_, & 0.99999 \nonumber\\
see_the & 0.99999 \nonumber\\
whether_a & 0.99999 \nonumber\\
set_up & 0.99999 \nonumber\\
food_source & 0.99999 \nonumber\\
bird_which & 0.99999 \nonumber\\
of_fish & 0.99999 \nonumber\\
for_bird & 0.99999 \nonumber\\
therfore & 0.99999 \nonumber\\
which_eat & 0.99999 \nonumber\\
vital_to & 0.99999 \nonumber\\
26 & 0.99999 \nonumber\\
be_extremly & 0.99999 \nonumber\\
26_piece & 0.99999 \nonumber\\
piece_of & 0.99999 \nonumber\\
fish_. & 0.99999 \nonumber\\
fish_find & 0.99999 \nonumber\\
bug_therfore & 0.99999 \nonumber\\
source_for & 0.99999 \nonumber\\
fish_species & 0.99999 \nonumber\\
extremly & 0.99999 \nonumber\\
extremly_vital & 0.99999 \nonumber\\
a_food & 0.99999 \nonumber\\
bug & 0.99999 \nonumber\\
one_single & 0.99999 \nonumber\\
eat_bug & 0.99999 \nonumber\\
bird & 0.99999 \nonumber\\
the_cycle & 0.99999 \nonumber\\
cycle_of & 0.99999 \nonumber\\
._fish & 0.99999 \nonumber\\
therfore_the & 0.99999 \nonumber\\
plastic_can & 0.99999 \nonumber\\
single_fish & 0.99999 \nonumber\\
cycle & 0.99999 \nonumber\\
be_26 & 0.99999 \nonumber\\
in_fact & 0.99999 \nonumber\\
i_help & 0.99999 \nonumber\\
layer & 0.99999 \nonumber\\
take_. & 0.99999 \nonumber\\
for_us & 0.99999 \nonumber\\
record & 0.99999 \nonumber\\
or_god & 0.99999 \nonumber\\
be_legal & 0.99999 \nonumber\\
scientist & 0.99999 \nonumber\\
._despite & 0.99999 \nonumber\\
alway & 0.99999 \nonumber\\
reward & 0.99999 \nonumber\\
over_a & 0.99999 \nonumber\\
ProductionRule_NP->RB,DT, & 0.99999 \nonumber\\
!_i & 0.99999 \nonumber\\
remain & 0.99999 \nonumber\\
world_, & 0.99999 \nonumber\\
with_better & 0.99999 \nonumber\\
can_easily & 0.99999 \nonumber\\
show_the & 0.99999 \nonumber\\
_pos_ngram_ADJ_NP_V & 0.99999 \nonumber\\
entertainment_. & 0.99999 \nonumber\\
ok_. & 0.99999 \nonumber\\
a_bite & 0.99999 \nonumber\\
the_indium & 0.99999 \nonumber\\
can_give & 0.99999 \nonumber\\
it_say & 0.99999 \nonumber\\
office & 0.99999 \nonumber\\
gay_, & 0.99999 \nonumber\\
atheism_should & 0.99999 \nonumber\\
the_absence & 0.99999 \nonumber\\
atheist_be & 0.99999 \nonumber\\
but_religious & 0.99999 \nonumber\\
faith_should & 0.99999 \nonumber\\
faith_be & 0.99999 \nonumber\\
think_atheist & 0.99999 \nonumber\\
person_just & 0.99999 \nonumber\\
besause & 0.99999 \nonumber\\
atheist_can & 0.99999 \nonumber\\
besause_everyone & 0.99999 \nonumber\\
hear_besause & 0.99999 \nonumber\\
but_faith & 0.99999 \nonumber\\
to_hear & 0.99999 \nonumber\\
absence_of & 0.99999 \nonumber\\
can_stand & 0.99999 \nonumber\\
be_indepent & 0.99999 \nonumber\\
stand_to & 0.99999 \nonumber\\
constantly_feed & 0.99999 \nonumber\\
indepent & 0.99999 \nonumber\\
religious_person & 0.99999 \nonumber\\
feed_, & 0.99999 \nonumber\\
have_his & 0.99999 \nonumber\\
just_believe & 0.99999 \nonumber\\
on_science & 0.99999 \nonumber\\
indepent_and & 0.99999 \nonumber\\
own_opinion & 0.99999 \nonumber\\
by_number & 0.99999 \nonumber\\
container_in & 0.99999 \nonumber\\
container_resource & 0.99999 \nonumber\\
economy_com & 0.99999 \nonumber\\
national_association & 0.99999 \nonumber\\
kid_of & 0.99999 \nonumber\\
number_! & 0.99999 \nonumber\\
by_weight & 0.99999 \nonumber\\
pet_water & 0.99999 \nonumber\\
most_recycle & 0.99999 \nonumber\\
also_only & 0.99999 \nonumber\\
in_curb & 0.99999 \nonumber\\
pet_container & 0.99999 \nonumber\\
1_& & 0.99999 \nonumber\\
recession_we & 0.99999 \nonumber\\
program_by & 0.99999 \nonumber\\
day_which & 0.99999 \nonumber\\
count_! & 0.99999 \nonumber\\
!_bottle & 0.99999 \nonumber\\
association_for & 0.99999 \nonumber\\
!_http://www.nestlewaterscorporate.com/bottled & 0.99999 \nonumber\\
pet & 0.99999 \nonumber\\
water_also & 0.99999 \nonumber\\
the_national & 0.99999 \nonumber\\
only_make & 0.99999 \nonumber\\
,_pet & 0.99999 \nonumber\\
purchase_bottle & 0.99999 \nonumber\\
no_the & 0.99999 \nonumber\\
very_moment & 0.99999 \nonumber\\
com_out & 0.99999 \nonumber\\
com & 0.99999 \nonumber\\
!_accord & 0.99999 \nonumber\\
for_pet & 0.99999 \nonumber\\
recycle_! & 0.99999 \nonumber\\
of_help & 0.99999 \nonumber\\
_pos_ngram_CARD_CONJ_NN & 0.99999 \nonumber\\
moment_. & 0.99999 \nonumber\\
world_waste & 0.99999 \nonumber\\
make_less & 0.99999 \nonumber\\
recycle_container & 0.99999 \nonumber\\
#xof & 0.99999 \nonumber\\
big_way & 0.99999 \nonumber\\
huge_mistake & 0.99999 \nonumber\\
help_count & 0.99999 \nonumber\\
less_then & 0.99999 \nonumber\\
side_program & 0.99999 \nonumber\\
&_#xof & 0.99999 \nonumber\\
._more & 0.99999 \nonumber\\
curb_side & 0.99999 \nonumber\\
ban_plastic & 0.99999 \nonumber\\
_pos_ngram_NP_NN_ADJ & 0.99999 \nonumber\\
#xof_; & 0.99999 \nonumber\\
state_purchase & 0.99999 \nonumber\\
point_you & 0.99999 \nonumber\\
lightly_spank & 0.99999 \nonumber\\
never_to & 0.99999 \nonumber\\
be_beat & 0.99999 \nonumber\\
certain_point & 0.99999 \nonumber\\
can_lightly & 0.99999 \nonumber\\
anal & 0.99999 \nonumber\\
unprotect_anal & 0.99999 \nonumber\\
people_involve & 0.99999 \nonumber\\
sex_' & 0.99999 \nonumber\\
anal_sex & 0.99999 \nonumber\\
of_aid & 0.99999 \nonumber\\
'_gay & 0.99999 \nonumber\\
a_wild & 0.99999 \nonumber\\
the_liklihood & 0.99999 \nonumber\\
make_be & 0.99999 \nonumber\\
liklihood_of & 0.99999 \nonumber\\
liklihood & 0.99999 \nonumber\\
the_original & 0.99999 \nonumber\\
transmission & 0.99999 \nonumber\\
transmission_. & 0.99999 \nonumber\\
sex_can & 0.99999 \nonumber\\
)_that & 0.99999 \nonumber\\
aid_transmission & 0.99999 \nonumber\\
that_unprotect & 0.99999 \nonumber\\
guess_) & 0.99999 \nonumber\\
_pos_ngram_O_CONJ_V & 0.99999 \nonumber\\
original_argument & 0.99999 \nonumber\\
orientation_of & 0.99999 \nonumber\\
that_might & 0.99999 \nonumber\\
wild & 0.99999 \nonumber\\
the_sexual & 0.99999 \nonumber\\
wild_guess & 0.99999 \nonumber\\
argument_the & 0.99999 \nonumber\\
can_increase & 0.99999 \nonumber\\
gay_sex & 0.99999 \nonumber\\
think_( & 0.99999 \nonumber\\
safety & 0.99999 \nonumber\\
for_everything & 0.99999 \nonumber\\
uniform_the & 0.99999 \nonumber\\
_pos_ngram_O_ADV_ADV & 0.99999 \nonumber\\
and_work & 0.99999 \nonumber\\
_pos_ngram_ADV_PP_ADV & 0.99999 \nonumber\\
afraid_of & 0.99999 \nonumber\\
at_them & 0.99999 \nonumber\\
how_gay & 0.99999 \nonumber\\
show_about & 0.99999 \nonumber\\
have_watch & 0.99999 \nonumber\\
watch_show & 0.99999 \nonumber\\
stop_be & 0.99999 \nonumber\\
see_how & 0.99999 \nonumber\\
them_feel & 0.99999 \nonumber\\
really_see & 0.99999 \nonumber\\
help_it & 0.99999 \nonumber\\
gay_friend & 0.99999 \nonumber\\
can_really & 0.99999 \nonumber\\
so_against & 0.99999 \nonumber\\
me_mad & 0.99999 \nonumber\\
harm_habitat & 0.99999 \nonumber\\
pollute_in & 0.99999 \nonumber\\
disaster_. & 0.99999 \nonumber\\
by_dump & 0.99999 \nonumber\\
environment_and & 0.99999 \nonumber\\
decompose_so & 0.99999 \nonumber\\
dump_in & 0.99999 \nonumber\\
dump & 0.99999 \nonumber\\
case_do & 0.99999 \nonumber\\
and_harm & 0.99999 \nonumber\\
for_emergency & 0.99999 \nonumber\\
or_in & 0.99999 \nonumber\\
n't_decompose & 0.99999 \nonumber\\
use_on & 0.99999 \nonumber\\
on_for & 0.99999 \nonumber\\
ProductionRule_VP->VB,ADVP,VP, & 0.99999 \nonumber\\
emergency_weather & 0.99999 \nonumber\\
human_disaster & 0.99999 \nonumber\\
ocean_or & 0.99999 \nonumber\\
landfill_. & 0.99999 \nonumber\\
only_use & 0.99999 \nonumber\\
natural_or & 0.99999 \nonumber\\
not_pollute & 0.99999 \nonumber\\
habitat_by & 0.99999 \nonumber\\
water_should & 0.99999 \nonumber\\
plastic_do & 0.99999 \nonumber\\
??? & 0.99999 \nonumber\\
educational & 0.99999 \nonumber\\
trade_and & 0.99999 \nonumber\\
connection_with & 0.99999 \nonumber\\
ProductionRule_NP->DT,JJ,NP, & 0.99999 \nonumber\\
that_question & 0.99999 \nonumber\\
characteristic & 0.99999 \nonumber\\
girl_that & 0.99999 \nonumber\\
terrible_person & 0.99999 \nonumber\\
someone_do & 0.99999 \nonumber\\
marry_kill & 0.99999 \nonumber\\
i_marry & 0.99999 \nonumber\\
game_when & 0.99999 \nonumber\\
effort & 0.99999 \nonumber\\
_pos_ngram_ART_NN_CARD & 0.99999 \nonumber\\
away_from & 0.99999 \nonumber\\
small & 0.99999 \nonumber\\
real_world & 0.99999 \nonumber\\
point_. & 0.99999 \nonumber\\
_pos_ngram_ART_PUNC_NN & 0.99999 \nonumber\\
"_because & 0.99999 \nonumber\\
quickly & 0.99999 \nonumber\\
persuit & 0.99999 \nonumber\\
personal_persuit & 0.99999 \nonumber\\
all_virgin & 0.99999 \nonumber\\
virgin_or & 0.99999 \nonumber\\
ProductionRule_SINV->ADVP,,,VP,NP, & 0.99999 \nonumber\\
,_yess & 0.99999 \nonumber\\
ProductionRule_NP->NP,CC,S, & 0.99999 \nonumber\\
cant_have & 0.99999 \nonumber\\
yess & 0.99999 \nonumber\\
porn_lol & 0.99999 \nonumber\\
hmm & 0.99999 \nonumber\\
hmm_, & 0.99999 \nonumber\\
or_still & 0.99999 \nonumber\\
yess_there & 0.99999 \nonumber\\
there_mother & 0.99999 \nonumber\\
have_porn & 0.99999 \nonumber\\
either_all & 0.99999 \nonumber\\
there_either & 0.99999 \nonumber\\
!_) & 0.99999 \nonumber\\
earn & 0.99999 \nonumber\\
student_have & 0.99999 \nonumber\\
extension & 0.99999 \nonumber\\
make_sense & 0.99999 \nonumber\\
where_the & 0.99999 \nonumber\\
first_it & 0.99999 \nonumber\\
feel_happy & 0.99999 \nonumber\\
term & 0.99999 \nonumber\\
very_quickly & 0.99999 \nonumber\\
and_let & 0.99999 \nonumber\\
both_be & 0.99999 \nonumber\\
_pos_ngram_PUNC_PR_PP & 0.99999 \nonumber\\
_pos_ngram_ADJ_O_V & 0.99999 \nonumber\\
motivation_to & 0.99999 \nonumber\\
their_body & 0.99999 \nonumber\\
stick_up & 0.99999 \nonumber\\
necessary_to & 0.99999 \nonumber\\
benefit_of & 0.99999 \nonumber\\
it_take & 0.99999 \nonumber\\
parent_that & 0.99999 \nonumber\\
what_do & 0.99999 \nonumber\\
_pos_ngram_PP_PR_NP & 0.99999 \nonumber\\
she_would & 0.99999 \nonumber\\
look_for & 0.99999 \nonumber\\
might_not & 0.99999 \nonumber\\
,_write & 0.99999 \nonumber\\
me_because & 0.99999 \nonumber\\
be_best & 0.99999 \nonumber\\
have_prove & 0.99999 \nonumber\\
say_" & 0.99999 \nonumber\\
ProductionRule_NP->DT,NP,CC,NP, & 0.99999 \nonumber\\
up_in & 0.99999 \nonumber\\
you_ever & 0.99999 \nonumber\\
your_not & 0.99999 \nonumber\\
obese_child & 0.99999 \nonumber\\
consider_human & 0.99999 \nonumber\\
piece & 0.99999 \nonumber\\
test & 0.99999 \nonumber\\
_pos_ngram_PR_O_PR & 0.99999 \nonumber\\
leave_with & 0.99999 \nonumber\\
ProductionRule_S->S,NP,VP, & 0.99999 \nonumber\\
husband_in & 0.99999 \nonumber\\
school_should & 0.99999 \nonumber\\
21st & 0.99999 \nonumber\\
not_compare & 0.99999 \nonumber\\
contribution_to & 0.99999 \nonumber\\
,_know & 0.99999 \nonumber\\
in_evolutionary & 0.99999 \nonumber\\
be_calibrate & 0.99999 \nonumber\\
match_the & 0.99999 \nonumber\\
a_logical & 0.99999 \nonumber\\
the_1900 & 0.99999 \nonumber\\
1900_. & 0.99999 \nonumber\\
1900 & 0.99999 \nonumber\\
not_present & 0.99999 \nonumber\\
lyell & 0.99999 \nonumber\\
date_that & 0.99999 \nonumber\\
the_rock & 0.99999 \nonumber\\
that_lyell & 0.99999 \nonumber\\
with_date & 0.99999 \nonumber\\
1800 & 0.99999 \nonumber\\
to_match & 0.99999 \nonumber\\
like_true & 0.99999 \nonumber\\
calibrate & 0.99999 \nonumber\\
stratum_. & 0.99999 \nonumber\\
calibrate_to & 0.99999 \nonumber\\
you_mention & 0.99999 \nonumber\\
true_scientific & 0.99999 \nonumber\\
the_technique & 0.99999 \nonumber\\
1800_, & 0.99999 \nonumber\\
evolutionary_theory & 0.99999 \nonumber\\
date_for & 0.99999 \nonumber\\
rigor_to & 0.99999 \nonumber\\
be_invent & 0.99999 \nonumber\\
technique_be & 0.99999 \nonumber\\
it_sure & 0.99999 \nonumber\\
charle & 0.99999 \nonumber\\
fallacy_, & 0.99999 \nonumber\\
,_charle & 0.99999 \nonumber\\
:_in & 0.99999 \nonumber\\
rigor_you & 0.99999 \nonumber\\
mention_be & 0.99999 \nonumber\\
date_be & 0.99999 \nonumber\\
the_1800 & 0.99999 \nonumber\\
logical_fallacy & 0.99999 \nonumber\\
charle_lyell & 0.99999 \nonumber\\
example_: & 0.99999 \nonumber\\
invent_until & 0.99999 \nonumber\\
sound_like & 0.99999 \nonumber\\
lyell_and & 0.99999 \nonumber\\
invent_, & 0.99999 \nonumber\\
n't_sound & 0.99999 \nonumber\\
date_lyell & 0.99999 \nonumber\\
present_in & 0.99999 \nonumber\\
one_example & 0.99999 \nonumber\\
._radiometric & 0.99999 \nonumber\\
n't_invent & 0.99999 \nonumber\\
other_come & 0.99999 \nonumber\\
lyell_come & 0.99999 \nonumber\\
would_get & 0.99999 \nonumber\\
firefox_have & 0.99999 \nonumber\\
in_if & 0.99999 \nonumber\\
you_look & 0.99999 \nonumber\\
"_if & 0.99999 \nonumber\\
to_grow & 0.99999 \nonumber\\
._at & 0.99999 \nonumber\\
they_need & 0.99999 \nonumber\\
why_it & 0.99999 \nonumber\\
mean_you & 0.99999 \nonumber\\
the_settlement & 0.99999 \nonumber\\
cause_a & 0.99999 \nonumber\\
u.s._, & 0.99999 \nonumber\\
the_u.s. & 0.99999 \nonumber\\
die_in & 0.99999 \nonumber\\
at_school & 0.99999 \nonumber\\
about_what & 0.99999 \nonumber\\
i_start & 0.99999 \nonumber\\
n't_watch & 0.99999 \nonumber\\
_pos_ngram_O_ADJ_NN & 0.99999 \nonumber\\
_pos_ngram_NP_CONJ_V & 0.99999 \nonumber\\
ounce & 0.99999 \nonumber\\
but_to & 0.99999 \nonumber\\
as_our & 0.99999 \nonumber\\
a_high & 0.99999 \nonumber\\
plain_and & 0.99999 \nonumber\\
and_simple & 0.99999 \nonumber\\
king & 0.99999 \nonumber\\
want_, & 0.99999 \nonumber\\
get_bully & 0.99999 \nonumber\\
fatter & 0.99999 \nonumber\\
ProductionRule_VP->VBN,PP,,,NP, & 0.99999 \nonumber\\
last_comment & 0.99999 \nonumber\\
my_bid & 0.99999 \nonumber\\
comment_be & 0.99999 \nonumber\\
wrong_side & 0.99999 \nonumber\\
ProductionRule_NP->S,CC,NP, & 0.99999 \nonumber\\
2day & 0.99999 \nonumber\\
newborn & 0.99999 \nonumber\\
2day_bt & 0.99999 \nonumber\\
rise_indium & 0.99999 \nonumber\\
r_so & 0.99999 \nonumber\\
better_day & 0.99999 \nonumber\\
newborn_child & 0.99999 \nonumber\\
a_newborn & 0.99999 \nonumber\\
say_indium & 0.99999 \nonumber\\
r_get & 0.99999 \nonumber\\
_pos_ngram_O_PR_NN & 0.99999 \nonumber\\
face_2day & 0.99999 \nonumber\\
the_rise & 0.99999 \nonumber\\
there_r & 0.99999 \nonumber\\
get_better & 0.99999 \nonumber\\
walk_!!! & 0.99999 \nonumber\\
bt_we & 0.99999 \nonumber\\
never_walk & 0.99999 \nonumber\\
scene & 0.99999 \nonumber\\
but_she & 0.99999 \nonumber\\
you_of & 0.99999 \nonumber\\
in_! & 0.99999 \nonumber\\
legacy & 0.99999 \nonumber\\
moth_be & 0.99999 \nonumber\\
death_, & 0.99999 \nonumber\\
ridiculous_and & 0.99999 \nonumber\\
give_us & 0.99999 \nonumber\\
more_on & 0.99999 \nonumber\\
an_accident & 0.99999 \nonumber\\
angry & 0.99999 \nonumber\\
which_country & 0.99999 \nonumber\\
you_not & 0.99999 \nonumber\\
should_never & 0.99999 \nonumber\\
be_school & 0.99999 \nonumber\\
still_need & 0.99999 \nonumber\\
remind_you & 0.99999 \nonumber\\
_pos_ngram_O_NP_PR & 0.99999 \nonumber\\
_pos_ngram_V_PR_CONJ & 0.99999 \nonumber\\
do_he & 0.99999 \nonumber\\
the_act & 0.99999 \nonumber\\
blind & 0.99999 \nonumber\\
or_if & 0.99999 \nonumber\\
you_the & 0.99999 \nonumber\\
high & 0.99999 \nonumber\\
penalty & 0.99999 \nonumber\\
what_about & 0.99999 \nonumber\\
they_like & 0.99999 \nonumber\\
be_post & 0.99999 \nonumber\\
invention_would & 0.99999 \nonumber\\
as_soon & 0.99999 \nonumber\\
obviously_everybody & 0.99999 \nonumber\\
good_all & 0.99999 \nonumber\\
now_be & 0.99999 \nonumber\\
world_or & 0.99999 \nonumber\\
city_, & 0.99999 \nonumber\\
post_under & 0.99999 \nonumber\\
small_percent & 0.99999 \nonumber\\
help_mankind & 0.99999 \nonumber\\
_pos_ngram_ADJ_ADJ_ART & 0.99999 \nonumber\\
car_and & 0.99999 \nonumber\\
ProductionRule_NP->RB,DT,JJ,NN, & 0.99999 \nonumber\\
and_factory & 0.99999 \nonumber\\
these_situation & 0.99999 \nonumber\\
economical_car & 0.99999 \nonumber\\
._anyway & 0.99999 \nonumber\\
economical & 0.99999 \nonumber\\
everybody_want & 0.99999 \nonumber\\
warm_come & 0.99999 \nonumber\\
would_actually & 0.99999 \nonumber\\
these_invention & 0.99999 \nonumber\\
factory & 0.99999 \nonumber\\
factory_would & 0.99999 \nonumber\\
just_now & 0.99999 \nonumber\\
mankind_, & 0.99999 \nonumber\\
honestly_would & 0.99999 \nonumber\\
under_personal & 0.99999 \nonumber\\
to_save & 0.99999 \nonumber\\
soon_as & 0.99999 \nonumber\\
_pos_ngram_ADJ_ART_PP & 0.99999 \nonumber\\
or_save & 0.99999 \nonumber\\
the_economical & 0.99999 \nonumber\\
to_life & 0.99999 \nonumber\\
abuse_. & 0.99999 \nonumber\\
against_woman & 0.99999 \nonumber\\
the_fashion & 0.99999 \nonumber\\
singapore.he_also & 0.99999 \nonumber\\
of_singapore.he & 0.99999 \nonumber\\
malay_, & 0.99999 \nonumber\\
farquar_deal & 0.99999 \nonumber\\
problem_during & 0.99999 \nonumber\\
ProductionRule_VP->VBD,S,,,SBAR, & 0.99999 \nonumber\\
also_attempt & 0.99999 \nonumber\\
early_year & 0.99999 \nonumber\\
day_problem & 0.99999 \nonumber\\
raffle_hardly & 0.99999 \nonumber\\
with_every & 0.99999 \nonumber\\
the_early & 0.99999 \nonumber\\
understand_malay & 0.99999 \nonumber\\
hardly_communicate & 0.99999 \nonumber\\
a_sense & 0.99999 \nonumber\\
universal_! & 0.99999 \nonumber\\
typical & 0.99999 \nonumber\\
typical_computer & 0.99999 \nonumber\\
or_install & 0.99999 \nonumber\\
download_or & 0.99999 \nonumber\\
there_since & 0.99999 \nonumber\\
universal & 0.99999 \nonumber\\
since_then & 0.99999 \nonumber\\
already_install & 0.99999 \nonumber\\
install_. & 0.99999 \nonumber\\
a_typical & 0.99999 \nonumber\\
install_in & 0.99999 \nonumber\\
firefox_still & 0.99999 \nonumber\\
be_universal & 0.99999 \nonumber\\
then_and & 0.99999 \nonumber\\
_pos_ngram_PP_ADV_CONJ & 0.99999 \nonumber\\
accident_or & 0.99999 \nonumber\\
n't_the & 0.99999 \nonumber\\
be_real & 0.99999 \nonumber\\
common_sense & 0.99999 \nonumber\\
work_on & 0.99999 \nonumber\\
ProductionRule_NP->NP,``,NP,'', & 0.99999 \nonumber\\
a_track & 0.99999 \nonumber\\
education_. & 0.99999 \nonumber\\
as_fast & 0.99999 \nonumber\\
20_push & 0.99999 \nonumber\\
teach_student & 0.99999 \nonumber\\
fast_as & 0.99999 \nonumber\\
eat_right & 0.99999 \nonumber\\
education_which & 0.99999 \nonumber\\
education_could & 0.99999 \nonumber\\
bid_if & 0.99999 \nonumber\\
run_as & 0.99999 \nonumber\\
ProductionRule_NP->JJ,DT, & 0.99999 \nonumber\\
lap & 0.99999 \nonumber\\
10_lap & 0.99999 \nonumber\\
around_a & 0.99999 \nonumber\\
ProductionRule_VP->VBG,NP,S,SBAR, & 0.99999 \nonumber\\
p.e_should & 0.99999 \nonumber\\
that_eat & 0.99999 \nonumber\\
a_5k & 0.99999 \nonumber\\
_pos_ngram_ADJ_ART_CONJ & 0.99999 \nonumber\\
lap_around & 0.99999 \nonumber\\
style_not & 0.99999 \nonumber\\
track_but & 0.99999 \nonumber\\
track & 0.99999 \nonumber\\
run_10 & 0.99999 \nonumber\\
a_fat & 0.99999 \nonumber\\
student_how & 0.99999 \nonumber\\
ProductionRule_ADVP->NP,IN,NP, & 0.99999 \nonumber\\
what_physical & 0.99999 \nonumber\\
life_style & 0.99999 \nonumber\\
real_education & 0.99999 \nonumber\\
fun_not & 0.99999 \nonumber\\
ok_no & 0.99999 \nonumber\\
5k & 0.99999 \nonumber\\
5k_or & 0.99999 \nonumber\\
exercise_can & 0.99999 \nonumber\\
think_p.e & 0.99999 \nonumber\\
push_up & 0.99999 \nonumber\\
be_education & 0.99999 \nonumber\\
an_obese & 0.99999 \nonumber\\
healthy_life & 0.99999 \nonumber\\
n't_run & 0.99999 \nonumber\\
_pos_ngram_ART_CONJ_ADV & 0.99999 \nonumber\\
kid_run & 0.99999 \nonumber\\
ProductionRule_NP->NP,CC,RB,NP, & 0.99999 \nonumber\\
but_show & 0.99999 \nonumber\\
do_20 & 0.99999 \nonumber\\
spouse_be & 0.99999 \nonumber\\
responsible_for & 0.99999 \nonumber\\
bottle_, & 0.99999 \nonumber\\
prettiest & 0.99999 \nonumber\\
other_about & 0.99999 \nonumber\\
fashion_issue & 0.99999 \nonumber\\
prettiest_and & 0.99999 \nonumber\\
coolest & 0.99999 \nonumber\\
coolest_and & 0.99999 \nonumber\\
expensive_cloth & 0.99999 \nonumber\\
equal_which & 0.99999 \nonumber\\
look_the & 0.99999 \nonumber\\
work_since & 0.99999 \nonumber\\
tease_each & 0.99999 \nonumber\\
feel_equal & 0.99999 \nonumber\\
issue_and & 0.99999 \nonumber\\
on_school & 0.99999 \nonumber\\
not_tease & 0.99999 \nonumber\\
the_coolest & 0.99999 \nonumber\\
most_expensive & 0.99999 \nonumber\\
the_prettiest & 0.99999 \nonumber\\
way_all & 0.99999 \nonumber\\
girl_out & 0.99999 \nonumber\\
make_all & 0.99999 \nonumber\\
about_fashion & 0.99999 \nonumber\\
cloth_be & 0.99999 \nonumber\\
which_increase & 0.99999 \nonumber\\
attention_on & 0.99999 \nonumber\\
have_make & 0.99999 \nonumber\\
fame_, & 0.99999 \nonumber\\
_pos_ngram_CONJ_PUNC_V & 0.99999 \nonumber\\
gay_. & 0.99999 \nonumber\\
little_daughter & 0.99999 \nonumber\\
record_- & 0.99999 \nonumber\\
:) & 0.99999 \nonumber\\
line & 0.99999 \nonumber\\
sport_, & 0.99999 \nonumber\\
find_any & 0.99999 \nonumber\\
d & 0.99999 \nonumber\\
dasanus & 0.99999 \nonumber\\
n't_like & 0.99999 \nonumber\\
citizen_, & 0.99999 \nonumber\\
total & 0.99999 \nonumber\\
in_total & 0.99999 \nonumber\\
grow_significantly & 0.99999 \nonumber\\
we_now & 0.99999 \nonumber\\
earthquake & 0.99999 \nonumber\\
understand_of & 0.99999 \nonumber\\
earthquake_be & 0.99999 \nonumber\\
from_billion & 0.99999 \nonumber\\
'_understand & 0.99999 \nonumber\\
an_angry & 0.99999 \nonumber\\
humanity_back & 0.99999 \nonumber\\
by_tectonic & 0.99999 \nonumber\\
"_early & 0.99999 \nonumber\\
ProductionRule_NP->DT,``,NNP, & 0.99999 \nonumber\\
let_religion & 0.99999 \nonumber\\
of_earthquake & 0.99999 \nonumber\\
hold_humanity & 0.99999 \nonumber\\
deity_seem & 0.99999 \nonumber\\
._support & 0.99999 \nonumber\\
that_earthquake & 0.99999 \nonumber\\
logical_, & 0.99999 \nonumber\\
universe_have & 0.99999 \nonumber\\
religion_fade & 0.99999 \nonumber\\
work_of & 0.99999 \nonumber\\
shift_. & 0.99999 \nonumber\\
that_creationist & 0.99999 \nonumber\\
that_current & 0.99999 \nonumber\\
shift & 0.99999 \nonumber\\
angry_deity & 0.99999 \nonumber\\
god_that & 0.99999 \nonumber\\
support_creationism & 0.99999 \nonumber\\
god_of & 0.99999 \nonumber\\
i_call & 0.99999 \nonumber\\
plate & 0.99999 \nonumber\\
significantly_. & 0.99999 \nonumber\\
plate_shift & 0.99999 \nonumber\\
tectonic_plate & 0.99999 \nonumber\\
gap_. & 0.99999 \nonumber\\
seem_logical & 0.99999 \nonumber\\
extremely_limit & 0.99999 \nonumber\\
accept_the & 0.99999 \nonumber\\
early_man & 0.99999 \nonumber\\
fade_away & 0.99999 \nonumber\\
tectonic & 0.99999 \nonumber\\
fade & 0.99999 \nonumber\\
current_species & 0.99999 \nonumber\\
creationist_believe & 0.99999 \nonumber\\
usa_, & 0.99999 \nonumber\\
love_her & 0.99999 \nonumber\\
reality_. & 0.99999 \nonumber\\
age_and & 0.99999 \nonumber\\
_pos_ngram_PUNC_PP_ADV & 0.99999 \nonumber\\
ProductionRule_NP->CD,NN,NN, & 0.99999 \nonumber\\
"_" & 0.99999 \nonumber\\
definately & 0.99999 \nonumber\\
increase & 0.99999 \nonumber\\
child_in & 0.99999 \nonumber\\
helpful & 0.99999 \nonumber\\
:_" & 0.99999 \nonumber\\
invention & 0.99999 \nonumber\\
,_get & 0.99999 \nonumber\\
earn_money & 0.99999 \nonumber\\
run_a & 0.99999 \nonumber\\
show_be & 0.99999 \nonumber\\
twist & 0.99999 \nonumber\\
my_religion & 0.99999 \nonumber\\
universe & 0.99999 \nonumber\\
remodel & 0.99999 \nonumber\\
think_be & 0.99999 \nonumber\\
their_action & 0.99999 \nonumber\\
"_into & 0.99999 \nonumber\\
book_because & 0.99999 \nonumber\\
her_because & 0.99999 \nonumber\\
step & 0.99999 \nonumber\\
context_that & 0.99999 \nonumber\\
be_internet & 0.99999 \nonumber\\
context & 0.99999 \nonumber\\
have_minimal & 0.99999 \nonumber\\
and_private & 0.99999 \nonumber\\
private_information & 0.99999 \nonumber\\
vista_support & 0.99999 \nonumber\\
a_security & 0.99999 \nonumber\\
both_firefox & 0.99999 \nonumber\\
security_architecture & 0.99999 \nonumber\\
security_context & 0.99999 \nonumber\\
app_with & 0.99999 \nonumber\\
internet_face & 0.99999 \nonumber\\
security_issue & 0.99999 \nonumber\\
ie7_on & 0.99999 \nonumber\\
and_ie & 0.99999 \nonumber\\
architecture & 0.99999 \nonumber\\
architecture_. & 0.99999 \nonumber\\
vista & 0.99999 \nonumber\\
mode_which & 0.99999 \nonumber\\
which_run & 0.99999 \nonumber\\
with_occasional & 0.99999 \nonumber\\
on_vista & 0.99999 \nonumber\\
protect_mode & 0.99999 \nonumber\\
ProductionRule_NP->PRP$,NN,CC,JJ,NN, & 0.99999 \nonumber\\
occasional_security & 0.99999 \nonumber\\
computer_and & 0.99999 \nonumber\\
prefer_the & 0.99999 \nonumber\\
run_the & 0.99999 \nonumber\\
minimal_access & 0.99999 \nonumber\\
face_app & 0.99999 \nonumber\\
mode & 0.99999 \nonumber\\
support_protect & 0.99999 \nonumber\\
better_security & 0.99999 \nonumber\\
shall_be & 0.99999 \nonumber\\
shall & 0.99999 \nonumber\\
the_environment & 0.99999 \nonumber\\
then_they & 0.99999 \nonumber\\
any_wed & 0.99999 \nonumber\\
that_another & 0.99999 \nonumber\\
institution_be & 0.99999 \nonumber\\
would_certainley & 0.99999 \nonumber\\
holy_matrimony & 0.99999 \nonumber\\
ProductionRule_VP->VP,CC,VP,,,ADVP,VP, & 0.99999 \nonumber\\
wholly_irrelevant & 0.99999 \nonumber\\
attend_. & 0.99999 \nonumber\\
debate_entirely & 0.99999 \nonumber\\
an_institution & 0.99999 \nonumber\\
wish_to & 0.99999 \nonumber\\
._far & 0.99999 \nonumber\\
need_n't & 0.99999 \nonumber\\
to_join & 0.99999 \nonumber\\
start_by & 0.99999 \nonumber\\
join_in & 0.99999 \nonumber\\
._hell & 0.99999 \nonumber\\
who_wish & 0.99999 \nonumber\\
entertain & 0.99999 \nonumber\\
entirely_. & 0.99999 \nonumber\\
entertain_ceremony & 0.99999 \nonumber\\
in_holy & 0.99999 \nonumber\\
entirely & 0.99999 \nonumber\\
another_debate & 0.99999 \nonumber\\
certainley & 0.99999 \nonumber\\
however_that & 0.99999 \nonumber\\
wed & 0.99999 \nonumber\\
think_animal & 0.99999 \nonumber\\
me_who & 0.99999 \nonumber\\
hell_i & 0.99999 \nonumber\\
animal_should & 0.99999 \nonumber\\
marry_be & 0.99999 \nonumber\\
an_entertain & 0.99999 \nonumber\\
irrelevant & 0.99999 \nonumber\\
me_start & 0.99999 \nonumber\\
irrelevant_. & 0.99999 \nonumber\\
matrimony & 0.99999 \nonumber\\
matrimony_as & 0.99999 \nonumber\\
ceremony_. & 0.99999 \nonumber\\
and_need & 0.99999 \nonumber\\
more_so & 0.99999 \nonumber\\
be_wholly & 0.99999 \nonumber\\
ever_attend & 0.99999 \nonumber\\
certainley_be & 0.99999 \nonumber\\
feel_marriage & 0.99999 \nonumber\\
wed_i & 0.99999 \nonumber\\
_pos_ngram_NN_CONJ_O & 0.99999 \nonumber\\
an_unborn & 0.99999 \nonumber\\
tv_show & 0.99999 \nonumber\\
that_what & 0.99999 \nonumber\\
people_say & 0.99999 \nonumber\\
no_porn & 0.99999 \nonumber\\
also_come & 0.99999 \nonumber\\
sex_, & 0.99999 \nonumber\\
school_or & 0.99999 \nonumber\\
the_thing & 0.99999 \nonumber\\
there_should & 0.99999 \nonumber\\
crazy_and & 0.99999 \nonumber\\
get_catch & 0.99999 \nonumber\\
:_d & 0.99999 \nonumber\\
just_as & 0.99999 \nonumber\\
ProductionRule_NP->DT,NP, & 0.99999 \nonumber\\
porn_be & 0.99999 \nonumber\\
_pos_ngram_ADJ_NP_PP & 0.99999 \nonumber\\
flipppin_real & 0.99999 \nonumber\\
ProductionRule_SINV->ADJP,,,ADVP,VP,NP, & 0.99999 \nonumber\\
god_aint & 0.99999 \nonumber\\
it_u & 0.99999 \nonumber\\
so_get & 0.99999 \nonumber\\
dumb_beliver & 0.99999 \nonumber\\
aint_flipppin & 0.99999 \nonumber\\
beliver_of & 0.99999 \nonumber\\
u_dumb & 0.99999 \nonumber\\
beliver & 0.99999 \nonumber\\
flipppin & 0.99999 \nonumber\\
jerk & 0.99999 \nonumber\\
happiness_. & 0.99999 \nonumber\\
argue_for & 0.99999 \nonumber\\
?_do & 0.99999 \nonumber\\
garden & 0.99999 \nonumber\\
_pos_ngram_ART_O_PR & 0.99999 \nonumber\\
not_in & 0.99999 \nonumber\\
ProductionRule_ADVP->RB,JJR, & 0.99999 \nonumber\\
selfish_person & 0.99999 \nonumber\\
actual & 0.99999 \nonumber\\
_pos_ngram_PUNC_NP_PR & 0.99999 \nonumber\\
pain & 0.99999 \nonumber\\
the_least & 0.99999 \nonumber\\
_pos_ngram_PR_ADJ_ADJ & 0.99999 \nonumber\\
child_of & 0.99999 \nonumber\\
partner & 0.99999 \nonumber\\
fair & 0.99999 \nonumber\\
exercise & 0.99999 \nonumber\\
bid_but & 0.99999 \nonumber\\
money_, & 0.99999 \nonumber\\
be_necessary & 0.99999 \nonumber\\
top & 0.99999 \nonumber\\
like_your & 0.99999 \nonumber\\
therefore_, & 0.99999 \nonumber\\
on_both & 0.99999 \nonumber\\
where_you & 0.99999 \nonumber\\
ProductionRule_S->SBAR,NP,VP, & 0.99999 \nonumber\\
'_to & 0.99999 \nonumber\\
._only & 0.99999 \nonumber\\
ProductionRule_VP->VBP,RB, & 0.99999 \nonumber\\
4_. & 0.99999 \nonumber\\
5_. & 0.99999 \nonumber\\
more_powerful & 0.99999 \nonumber\\
soul & 0.99999 \nonumber\\
dealer & 0.99999 \nonumber\\
drug_dealer & 0.99999 \nonumber\\
a_reason & 0.99999 \nonumber\\
security & 0.99999 \nonumber\\
because_my & 0.99999 \nonumber\\
addiction & 0.99999 \nonumber\\
book_r & 0.99999 \nonumber\\
both_way & 0.99999 \nonumber\\
in_ie & 0.99999 \nonumber\\
and_can & 0.99999 \nonumber\\
lifestyle_. & 0.99999 \nonumber\\
force_to & 0.99999 \nonumber\\
be_force & 0.99999 \nonumber\\
to_give & 0.99999 \nonumber\\
my_life & 0.99999 \nonumber\\
,_in-fact & 0.99999 \nonumber\\
an_better & 0.99999 \nonumber\\
kinda_get & 0.99999 \nonumber\\
also_kinda & 0.99999 \nonumber\\
in-fact_that & 0.99999 \nonumber\\
in-fact & 0.99999 \nonumber\\
a_least & 0.99999 \nonumber\\
greatest_father & 0.99999 \nonumber\\
an_lousy & 0.99999 \nonumber\\
an_father & 0.99999 \nonumber\\
go_up & 0.99999 \nonumber\\
idea_on & 0.99999 \nonumber\\
an_idea & 0.99999 \nonumber\\
be_motivation & 0.99999 \nonumber\\
should_motivate & 0.99999 \nonumber\\
and_where & 0.99999 \nonumber\\
motivation_that & 0.99999 \nonumber\\
ProductionRule_VP->VBZ,ADVP,ADJP,S, & 0.99999 \nonumber\\
uncomfortable & 0.99999 \nonumber\\
of_tab & 0.99999 \nonumber\\
ProductionRule_NP->PRP$,JJ,NN,NN, & 0.99999 \nonumber\\
u_forget & 0.99999 \nonumber\\
its_ancient & 0.99999 \nonumber\\
ndian & 0.99999 \nonumber\\
ancient_glory & 0.99999 \nonumber\\
glory_history & 0.99999 \nonumber\\
about_its & 0.99999 \nonumber\\
be_powerful & 0.99999 \nonumber\\
glory & 0.99999 \nonumber\\
ndian_have & 0.99999 \nonumber\\
r_u & 0.99999 \nonumber\\
powerful_why & 0.99999 \nonumber\\
why_r & 0.99999 \nonumber\\
like_you & 0.99999 \nonumber\\
._their & 0.99999 \nonumber\\
wife_. & 0.99999 \nonumber\\
ProductionRule_PP->VBN,PP, & 0.99999 \nonumber\\
recently & 0.99999 \nonumber\\
dissapoint & 0.99999 \nonumber\\
wouldnt_know & 0.99999 \nonumber\\
dissapoint_by & 0.99999 \nonumber\\
friend_that & 0.99999 \nonumber\\
feel_to & 0.99999 \nonumber\\
they_wish & 0.99999 \nonumber\\
alway_drink & 0.99999 \nonumber\\
be_dissapoint & 0.99999 \nonumber\\
same_because & 0.99999 \nonumber\\
you_wouldnt & 0.99999 \nonumber\\
there_father & 0.99999 \nonumber\\
now_if & 0.99999 \nonumber\\
sometime_tell & 0.99999 \nonumber\\
have_friend & 0.99999 \nonumber\\
they_sometime & 0.99999 \nonumber\\
least_by & 0.99999 \nonumber\\
drink_and & 0.99999 \nonumber\\
there_dad & 0.99999 \nonumber\\
creationism & 0.99999 \nonumber\\
emergency_. & 0.99999 \nonumber\\
landfill & 0.99999 \nonumber\\
in_landfill & 0.99999 \nonumber\\
and_exercise & 0.99999 \nonumber\\
ProductionRule_PP->IN,'',NP, & 0.99999 \nonumber\\
a_country & 0.99999 \nonumber\\
ProductionRule_ADJP->ADVP,JJR, & 0.99999 \nonumber\\
because_so & 0.99999 \nonumber\\
ProductionRule_ADVP->RB,JJ, & 0.99999 \nonumber\\
side_now & 0.99999 \nonumber\\
people_agree & 0.99999 \nonumber\\
would_we & 0.99999 \nonumber\\
most_school & 0.99999 \nonumber\\
a_twist & 0.99999 \nonumber\\
give_strict & 0.99999 \nonumber\\
then_give & 0.99999 \nonumber\\
be_then & 0.99999 \nonumber\\
"_casual & 0.99999 \nonumber\\
"_uniform & 0.99999 \nonumber\\
"_causal & 0.99999 \nonumber\\
their_casual & 0.99999 \nonumber\\
be_effectively & 0.99999 \nonumber\\
casual_clothe & 0.99999 \nonumber\\
causal_" & 0.99999 \nonumber\\
that_destruction & 0.99999 \nonumber\\
effectively & 0.99999 \nonumber\\
guideline_as & 0.99999 \nonumber\\
destruction_. & 0.99999 \nonumber\\
destruction & 0.99999 \nonumber\\
destroy_creativity & 0.99999 \nonumber\\
effectively_turn & 0.99999 \nonumber\\
turn_" & 0.99999 \nonumber\\
classic_example & 0.99999 \nonumber\\
the_occasional & 0.99999 \nonumber\\
causal & 0.99999 \nonumber\\
how_school & 0.99999 \nonumber\\
strict_guideline & 0.99999 \nonumber\\
clothe_" & 0.99999 \nonumber\\
school_destroy & 0.99999 \nonumber\\
a_classic & 0.99999 \nonumber\\
and_uniform & 0.99999 \nonumber\\
twist_" & 0.99999 \nonumber\\
occasional_day & 0.99999 \nonumber\\
we_talk & 0.99999 \nonumber\\
creativity_and & 0.99999 \nonumber\\
ProductionRule_SINV->S,VP,NP, & 0.99999 \nonumber\\
ProductionRule_VP->VBG,ADVP, & 0.99999 \nonumber\\
spend & 0.99999 \nonumber\\
ProductionRule_S->SBAR,VP, & 0.99999 \nonumber\\
a_balance & 0.99999 \nonumber\\
ProductionRule_VP->VBZ,RB,ADJP,PP, & 0.99999 \nonumber\\
let_me & 0.99999 \nonumber\\
have_take & 0.99999 \nonumber\\
education & 0.99999 \nonumber\\
maybe_have & 0.99999 \nonumber\\
ProductionRule_S->ADVP,VP, & 0.99999 \nonumber\\
in_most & 0.99999 \nonumber\\
ProductionRule_FRAG->NP,:,S,., & 0.99999 \nonumber\\
one_fly & 0.99999 \nonumber\\
,_nabokov & 0.99999 \nonumber\\
,_martian & 0.99999 \nonumber\\
,_east & 0.99999 \nonumber\\
cuckoo_nest & 0.99999 \nonumber\\
the_cuckoo & 0.99999 \nonumber\\
cuckoo & 0.99999 \nonumber\\
real_. & 0.99999 \nonumber\\
fly_over & 0.99999 \nonumber\\
world_describe & 0.99999 \nonumber\\
lolita & 0.99999 \nonumber\\
nest_, & 0.99999 \nonumber\\
nabokov & 0.99999 \nonumber\\
martian & 0.99999 \nonumber\\
nabokov_' & 0.99999 \nonumber\\
that_beat & 0.99999 \nonumber\\
,_1984 & 0.99999 \nonumber\\
martian_chronicle & 0.99999 \nonumber\\
little_that & 0.99999 \nonumber\\
for_real & 0.99999 \nonumber\\
east_of & 0.99999 \nonumber\\
'_lolita & 0.99999 \nonumber\\
describe_in & 0.99999 \nonumber\\
1984 & 0.99999 \nonumber\\
nest & 0.99999 \nonumber\\
lolita_, & 0.99999 \nonumber\\
ProductionRule_ADVP->IN,CC,IN, & 0.99999 \nonumber\\
1984_, & 0.99999 \nonumber\\
chronicle & 0.99999 \nonumber\\
eden_, & 0.99999 \nonumber\\
chronicle_- & 0.99999 \nonumber\\
live_at & 0.99999 \nonumber\\
still_live & 0.99999 \nonumber\\
home_with & 0.99999 \nonumber\\
of_malacca & 0.99999 \nonumber\\
strait & 0.99999 \nonumber\\
the_strait & 0.99999 \nonumber\\
strait_of & 0.99999 \nonumber\\
excite_and & 0.99999 \nonumber\\
we_enjoy & 0.99999 \nonumber\\
the_love & 0.99999 \nonumber\\
wife_share & 0.99999 \nonumber\\
excite & 0.99999 \nonumber\\
and_passionate & 0.99999 \nonumber\\
enjoy_together & 0.99999 \nonumber\\
love_life & 0.99999 \nonumber\\
and_expand & 0.99999 \nonumber\\
the_room & 0.99999 \nonumber\\
so_as & 0.99999 \nonumber\\
of_age & 0.99999 \nonumber\\
age_then & 0.99999 \nonumber\\
an_excite & 0.99999 \nonumber\\
pop_it & 0.99999 \nonumber\\
together_in & 0.99999 \nonumber\\
bedroom_. & 0.99999 \nonumber\\
legal_and & 0.99999 \nonumber\\
notch_. & 0.99999 \nonumber\\
notch & 0.99999 \nonumber\\
room_on & 0.99999 \nonumber\\
kick_it & 0.99999 \nonumber\\
kick & 0.99999 \nonumber\\
passionate_love & 0.99999 \nonumber\\
._set & 0.99999 \nonumber\\
on_fire & 0.99999 \nonumber\\
expand_the & 0.99999 \nonumber\\
to_kick & 0.99999 \nonumber\\
we_pop & 0.99999 \nonumber\\
passionate & 0.99999 \nonumber\\
share_an & 0.99999 \nonumber\\
a_notch & 0.99999 \nonumber\\
us_itt & 0.99999 \nonumber\\
itt_be & 0.99999 \nonumber\\
user_from & 0.99999 \nonumber\\
avaible_in & 0.99999 \nonumber\\
also_now & 0.99999 \nonumber\\
ie7_have & 0.99999 \nonumber\\
avaible & 0.99999 \nonumber\\
begin_, & 0.99999 \nonumber\\
but_recently & 0.99999 \nonumber\\
firefox_which & 0.99999 \nonumber\\
other_significant & 0.99999 \nonumber\\
feature_include & 0.99999 \nonumber\\
think_ie & 0.99999 \nonumber\\
to_provide & 0.99999 \nonumber\\
obvious_difference & 0.99999 \nonumber\\
provide_different & 0.99999 \nonumber\\
a_ie & 0.99999 \nonumber\\
start_use & 0.99999 \nonumber\\
ie_i & 0.99999 \nonumber\\
availability & 0.99999 \nonumber\\
not_avaible & 0.99999 \nonumber\\
in_use & 0.99999 \nonumber\\
the_obvious & 0.99999 \nonumber\\
with_add-on & 0.99999 \nonumber\\
recently_i & 0.99999 \nonumber\\
difference_like & 0.99999 \nonumber\\
tab_feature & 0.99999 \nonumber\\
now_ie7 & 0.99999 \nonumber\\
functionality_. & 0.99999 \nonumber\\
advantage_in & 0.99999 \nonumber\\
significant_advantage & 0.99999 \nonumber\\
tab_in & 0.99999 \nonumber\\
like_availability & 0.99999 \nonumber\\
different_functionality & 0.99999 \nonumber\\
availability_of & 0.99999 \nonumber\\
add-on_to & 0.99999 \nonumber\\
include_, & 0.99999 \nonumber\\
older & 0.99999 \nonumber\\
the_student & 0.99999 \nonumber\\
good_reason & 0.99999 \nonumber\\
ProductionRule_NP->JJ,NNS,CC,NNS, & 0.99999 \nonumber\\
around_them & 0.99999 \nonumber\\
you_try & 0.99999 \nonumber\\
be_face & 0.99999 \nonumber\\
_pos_ngram_PUNC_PR_NP & 0.99999 \nonumber\\
own_clothe & 0.99999 \nonumber\\
out_for & 0.99999 \nonumber\\
immune & 0.99999 \nonumber\\
ProductionRule_VP->VBN,PP,ADVP, & 0.99999 \nonumber\\
head & 0.99999 \nonumber\\
the_head & 0.99999 \nonumber\\
alright & 0.99999 \nonumber\\
u.s. & 0.99999 \nonumber\\
to_accomplish & 0.99999 \nonumber\\
however_, & 0.99999 \nonumber\\
lousy_, & 0.99999 \nonumber\\
_pos_ngram_PUNC_O_ADV & 0.99999 \nonumber\\
think_there & 0.99999 \nonumber\\
fatherless_. & 0.99999 \nonumber\\
relationship_. & 0.99999 \nonumber\\
and_personality & 0.99999 \nonumber\\
watch_it & 0.99999 \nonumber\\
that_motivate & 0.99999 \nonumber\\
,_dad & 0.99999 \nonumber\\
._dad & 0.99999 \nonumber\\
can_sometime & 0.99999 \nonumber\\
to_guide & 0.99999 \nonumber\\
icon & 0.99999 \nonumber\\
how_tall & 0.99999 \nonumber\\
through_their & 0.99999 \nonumber\\
icon_that & 0.99999 \nonumber\\
surpass_them & 0.99999 \nonumber\\
guide & 0.99999 \nonumber\\
most_, & 0.99999 \nonumber\\
sometime_be & 0.99999 \nonumber\\
family_without & 0.99999 \nonumber\\
better_parent & 0.99999 \nonumber\\
their_mistake & 0.99999 \nonumber\\
tall_you & 0.99999 \nonumber\\
tall & 0.99999 \nonumber\\
two_parent & 0.99999 \nonumber\\
that_icon & 0.99999 \nonumber\\
without_have & 0.99999 \nonumber\\
guide_you & 0.99999 \nonumber\\
healthy_family & 0.99999 \nonumber\\
be_through & 0.99999 \nonumber\\
proud & 0.99999 \nonumber\\
ProductionRule_NP->NN,JJ, & 0.99999 \nonumber\\
ProductionRule_VP->VP,,,SBAR, & 0.99999 \nonumber\\
_pos_ngram_ART_PUNC_ADJ & 0.99999 \nonumber\\
be_mean & 0.99999 \nonumber\\
ProductionRule_VP->VB,ADJP,ADVP, & 0.99999 \nonumber\\
student_. & 0.99999 \nonumber\\
get_over & 0.99999 \nonumber\\
the_community & 0.99999 \nonumber\\
important & 0.99999 \nonumber\\
apology_. & 0.99999 \nonumber\\
creationist_version & 0.99999 \nonumber\\
apology & 0.99999 \nonumber\\
oop & 0.99999 \nonumber\\
say_creationist & 0.99999 \nonumber\\
my_apology & 0.99999 \nonumber\\
oop_, & 0.99999 \nonumber\\
location & 0.99999 \nonumber\\
finish_. & 0.99999 \nonumber\\
also_student & 0.99999 \nonumber\\
like_cancer & 0.99999 \nonumber\\
wave_. & 0.99999 \nonumber\\
because_today & 0.99999 \nonumber\\
electromagnetic_wave & 0.99999 \nonumber\\
electromagnetic & 0.99999 \nonumber\\
because_computer & 0.99999 \nonumber\\
health_and & 0.99999 \nonumber\\
serious_diease & 0.99999 \nonumber\\
computer_game & 0.99999 \nonumber\\
be_play & 0.99999 \nonumber\\
student_ca & 0.99999 \nonumber\\
than_student & 0.99999 \nonumber\\
get_good & 0.99999 \nonumber\\
computer_have & 0.99999 \nonumber\\
true_because & 0.99999 \nonumber\\
today_lot & 0.99999 \nonumber\\
cancer_because & 0.99999 \nonumber\\
get_serious & 0.99999 \nonumber\\
of_electromagnetic & 0.99999 \nonumber\\
play_computer & 0.99999 \nonumber\\
diease_like & 0.99999 \nonumber\\
diease & 0.99999 \nonumber\\
school_finish & 0.99999 \nonumber\\
clothe_but & 0.99999 \nonumber\\
._make & 0.99999 \nonumber\\
many_type & 0.99999 \nonumber\\
guy_. & 0.99999 \nonumber\\
to_teach & 0.99999 \nonumber\\
ProductionRule_SBAR->WHADVP,S,., & 0.99999 \nonumber\\
argument_which & 0.99999 \nonumber\\
behave & 0.99999 \nonumber\\
by_your & 0.99999 \nonumber\\
come_if & 0.99999 \nonumber\\
mabye_some & 0.99999 \nonumber\\
._come & 0.99999 \nonumber\\
if_their & 0.99999 \nonumber\\
people_thing & 0.99999 \nonumber\\
mabye & 0.99999 \nonumber\\
have_baby & 0.99999 \nonumber\\
._mabye & 0.99999 \nonumber\\
sex_how & 0.99999 \nonumber\\
but_really & 0.99999 \nonumber\\
and_sex & 0.99999 \nonumber\\
singapore.he & 0.99999 \nonumber\\
take_all & 0.99999 \nonumber\\
system_. & 0.99999 \nonumber\\
human_be & 0.99999 \nonumber\\
but_they & 0.99999 \nonumber\\
bulk & 0.99999 \nonumber\\
from_single & 0.99999 \nonumber\\
bulk_storage & 0.99999 \nonumber\\
storage & 0.99999 \nonumber\\
ProductionRule_ADJP->RB,RBR,JJ,S, & 0.99999 \nonumber\\
single_12-20 & 0.99999 \nonumber\\
_pos_ngram_PP_ADJ_CARD & 0.99999 \nonumber\\
from_large & 0.99999 \nonumber\\
where_public & 0.99999 \nonumber\\
likely_than & 0.99999 \nonumber\\
storage_container & 0.99999 \nonumber\\
government_program & 0.99999 \nonumber\\
various_reason & 0.99999 \nonumber\\
storage_of & 0.99999 \nonumber\\
12-20 & 0.99999 \nonumber\\
contamination_from & 0.99999 \nonumber\\
contamination & 0.99999 \nonumber\\
large_bulk & 0.99999 \nonumber\\
12-20_ounce & 0.99999 \nonumber\\
container_be & 0.99999 \nonumber\\
large_water & 0.99999 \nonumber\\
safe_to & 0.99999 \nonumber\\
water_storage & 0.99999 \nonumber\\
for_various & 0.99999 \nonumber\\
public_water & 0.99999 \nonumber\\
somewhat & 0.99999 \nonumber\\
program_regularly & 0.99999 \nonumber\\
somewhat_less & 0.99999 \nonumber\\
ounce_bottle & 0.99999 \nonumber\\
distribute_small & 0.99999 \nonumber\\
be_somewhat & 0.99999 \nonumber\\
distribute_large & 0.99999 \nonumber\\
disperse_bottle & 0.99999 \nonumber\\
disperse & 0.99999 \nonumber\\
be_least & 0.99999 \nonumber\\
regularly_disperse & 0.99999 \nonumber\\
than_from & 0.99999 \nonumber\\
also_contamination & 0.99999 \nonumber\\
than_distribute & 0.99999 \nonumber\\
least_safe & 0.99999 \nonumber\\
,_where & 0.99999 \nonumber\\
drink_. & 0.99999 \nonumber\\
._distribute & 0.99999 \nonumber\\
small_bottle & 0.99999 \nonumber\\
many_government & 0.99999 \nonumber\\
condone & 0.99999 \nonumber\\
many_problem & 0.99999 \nonumber\\
of_eden & 0.99999 \nonumber\\
eden & 0.99999 \nonumber\\
student_so & 0.99999 \nonumber\\
?_because & 0.99999 \nonumber\\
choice_of & 0.99999 \nonumber\\
a_pretty & 0.99999 \nonumber\\
my_logic & 0.99999 \nonumber\\
eh_, & 0.99999 \nonumber\\
of_anything & 0.99999 \nonumber\\
logic_work & 0.99999 \nonumber\\
pretty_cool & 0.99999 \nonumber\\
cool_guy & 0.99999 \nonumber\\
n't_afraid & 0.99999 \nonumber\\
have_child & 0.99999 \nonumber\\
ProductionRule_VP->VBZ,ADJP,S, & 0.99999 \nonumber\\
_pos_ngram_PP_ART_CONJ & 0.99999 \nonumber\\
for_this & 0.99999 \nonumber\\
the_datum & 0.99999 \nonumber\\
insufficient & 0.99999 \nonumber\\
but_evolution & 0.99999 \nonumber\\
phro_and & 0.99999 \nonumber\\
insufficient_, & 0.99999 \nonumber\\
evidence_of & 0.99999 \nonumber\\
datum_may & 0.99999 \nonumber\\
allele_be & 0.99999 \nonumber\\
to_external & 0.99999 \nonumber\\
phro & 0.99999 \nonumber\\
show_evidence & 0.99999 \nonumber\\
contradict_phro & 0.99999 \nonumber\\
to_contradict & 0.99999 \nonumber\\
do_show & 0.99999 \nonumber\\
allele & 0.99999 \nonumber\\
different_allele & 0.99999 \nonumber\\
be_insufficient & 0.99999 \nonumber\\
express_due & 0.99999 \nonumber\\
moth_do & 0.99999 \nonumber\\
when_different & 0.99999 \nonumber\\
external_factor & 0.99999 \nonumber\\
external & 0.99999 \nonumber\\
be_express & 0.99999 \nonumber\\
site_be & 0.99999 \nonumber\\
ProductionRule_S->S,,,IN,S,., & 0.99999 \nonumber\\
go_for & 0.99999 \nonumber\\
ProductionRule_ADJP->JJ,RB,SBAR, & 0.99999 \nonumber\\
avoid_do & 0.99999 \nonumber\\
enough_for & 0.99999 \nonumber\\
painful_enough & 0.99999 \nonumber\\
painful & 0.99999 \nonumber\\
spanking_be & 0.99999 \nonumber\\
be_painful & 0.99999 \nonumber\\
the_spanking & 0.99999 \nonumber\\
strongly_agree & 0.99999 \nonumber\\
spanking & 0.99999 \nonumber\\
potential & 0.99999 \nonumber\\
hospital & 0.99999 \nonumber\\
ever_kill & 0.99999 \nonumber\\
,_vishvamitr & 0.99999 \nonumber\\
ProductionRule_NP->ADJP,,,NN,,,NN,NN, & 0.99999 \nonumber\\
forget_lord & 0.99999 \nonumber\\
vishvguru_in & 0.99999 \nonumber\\
rama & 0.99999 \nonumber\\
in_future & 0.99999 \nonumber\\
,_krishna & 0.99999 \nonumber\\
far_view & 0.99999 \nonumber\\
which_give & 0.99999 \nonumber\\
krishna & 0.99999 \nonumber\\
etc_which & 0.99999 \nonumber\\
vishvguru & 0.99999 \nonumber\\
krishna_, & 0.99999 \nonumber\\
rama_, & 0.99999 \nonumber\\
vishvamitr & 0.99999 \nonumber\\
vishvamitr_etc & 0.99999 \nonumber\\
lord_rama & 0.99999 \nonumber\\
give_far & 0.99999 \nonumber\\
the_vishvguru & 0.99999 \nonumber\\
be_normal & 0.99999 \nonumber\\
whether_you & 0.99999 \nonumber\\
fetus_. & 0.99999 \nonumber\\
ProductionRule_VP->ADVP,VBP,SBAR, & 0.99999 \nonumber\\
support_a & 0.99999 \nonumber\\
)_she & 0.99999 \nonumber\\
most_responsible & 0.99999 \nonumber\\
make_such & 0.99999 \nonumber\\
and_maturity & 0.99999 \nonumber\\
,_physically & 0.99999 \nonumber\\
financially_) & 0.99999 \nonumber\\
physically_, & 0.99999 \nonumber\\
important_decision & 0.99999 \nonumber\\
financially & 0.99999 \nonumber\\
or_financially & 0.99999 \nonumber\\
make_in & 0.99999 \nonumber\\
maturity_it & 0.99999 \nonumber\\
in_her & 0.99999 \nonumber\\
(_either & 0.99999 \nonumber\\
decision_a & 0.99999 \nonumber\\
the_responsibility & 0.99999 \nonumber\\
take_to & 0.99999 \nonumber\\
_pos_ngram_ADV_O_PR & 0.99999 \nonumber\\
you_any & 0.99999 \nonumber\\
not_support & 0.99999 \nonumber\\
any_idea & 0.99999 \nonumber\\
responsible_decision & 0.99999 \nonumber\\
have_right & 0.99999 \nonumber\\
_pos_ngram_O_NP_ADV & 0.99999 \nonumber\\
an_important & 0.99999 \nonumber\\
child_( & 0.99999 \nonumber\\
either_emotionally & 0.99999 \nonumber\\
responsibility_and & 0.99999 \nonumber\\
away_. & 0.99999 \nonumber\\
pay_for & 0.99999 \nonumber\\
n't_we & 0.99999 \nonumber\\
yeah & 0.99999 \nonumber\\
will_help & 0.99999 \nonumber\\
_pos_ngram_NN_CARD_NN & 0.99999 \nonumber\\
important_to & 0.99999 \nonumber\\
job_to & 0.99999 \nonumber\\
pe_, & 0.99999 \nonumber\\
together_as & 0.99999 \nonumber\\
alway_happen & 0.99999 \nonumber\\
habit_later & 0.99999 \nonumber\\
other_class & 0.99999 \nonumber\\
in_other & 0.99999 \nonumber\\
good_habit & 0.99999 \nonumber\\
,_help & 0.99999 \nonumber\\
get_involve & 0.99999 \nonumber\\
ProductionRule_NP->S,,,RRC,,, & 0.99999 \nonumber\\
team_that & 0.99999 \nonumber\\
be_active & 0.99999 \nonumber\\
of_work & 0.99999 \nonumber\\
ProductionRule_RRC->ADVP,PP, & 0.99999 \nonumber\\
active_and & 0.99999 \nonumber\\
even_through & 0.99999 \nonumber\\
develop_good & 0.99999 \nonumber\\
through_pe & 0.99999 \nonumber\\
help_child & 0.99999 \nonumber\\
my_opponent & 0.99999 \nonumber\\
i_my & 0.99999 \nonumber\\
and_indoctrinate & 0.99999 \nonumber\\
weaker_? & 0.99999 \nonumber\\
indoctrinate & 0.99999 \nonumber\\
would_that & 0.99999 \nonumber\\
since_birth & 0.99999 \nonumber\\
brainwash_and & 0.99999 \nonumber\\
any_weaker & 0.99999 \nonumber\\
birth_? & 0.99999 \nonumber\\
indoctrinate_since & 0.99999 \nonumber\\
whole_life & 0.99999 \nonumber\\
it_improve & 0.99999 \nonumber\\
there_next & 0.99999 \nonumber\\
with_each & 0.99999 \nonumber\\
give_your & 0.99999 \nonumber\\
to_show & 0.99999 \nonumber\\
at_home & 0.99999 \nonumber\\
ago & 0.99999 \nonumber\\
us_what & 0.99999 \nonumber\\
means_that & 0.99999 \nonumber\\
tend_to & 0.99999 \nonumber\\
tend & 0.99999 \nonumber\\
acceptance & 0.99999 \nonumber\\
he_come & 0.99999 \nonumber\\
be_for & 0.99999 \nonumber\\
_pos_ngram_PP_ADJ_ART & 0.99999 \nonumber\\
ProductionRule_NP->DT,NN,JJ,NNS, & 0.99999 \nonumber\\
up_that & 0.99999 \nonumber\\
give_up & 0.99999 \nonumber\\
fact_and & 0.99999 \nonumber\\
you_move & 0.99999 \nonumber\\
singapore_and & 0.99999 \nonumber\\
become_an & 0.99999 \nonumber\\
not_? & 0.99999 \nonumber\\
bore & 0.99999 \nonumber\\
healthy_for & 0.99999 \nonumber\\
make_physical & 0.99999 \nonumber\\
healthy_person & 0.99999 \nonumber\\
ProductionRule_NP->JJ,NN,S, & 0.99999 \nonumber\\
be_healthy & 0.99999 \nonumber\\
mandatory_in & 0.99999 \nonumber\\
of_obesity & 0.99999 \nonumber\\
dream_about & 0.99999 \nonumber\\
be_fun & 0.99999 \nonumber\\
action & 0.99999 \nonumber\\
in_all & 0.99999 \nonumber\\
good_or & 0.99999 \nonumber\\
line_of & 0.99999 \nonumber\\
_pos_ngram_O_ART_NP & 0.99999 \nonumber\\
to_jail & 0.99999 \nonumber\\
that_shall & 0.99999 \nonumber\\
also_go & 0.99999 \nonumber\\
jail_for & 0.99999 \nonumber\\
punish_for & 0.99999 \nonumber\\
whoever_would & 0.99999 \nonumber\\
crime_as & 0.99999 \nonumber\\
?_whoever & 0.99999 \nonumber\\
somebody_? & 0.99999 \nonumber\\
their_crime & 0.99999 \nonumber\\
just_crazy & 0.99999 \nonumber\\
care_who & 0.99999 \nonumber\\
think_he & 0.99999 \nonumber\\
_pos_ngram_PP_ADJ_ADV & 0.99999 \nonumber\\
all_this & 0.99999 \nonumber\\
functionality & 0.99999 \nonumber\\
regularly & 0.99999 \nonumber\\
relationship_and & 0.99999 \nonumber\\
song & 0.99999 \nonumber\\
prove_it & 0.99999 \nonumber\\
'_back & 0.99999 \nonumber\\
dominate & 0.99999 \nonumber\\
of_father & 0.99999 \nonumber\\
say_but & 0.99999 \nonumber\\
ProductionRule_VP->VB,ADVP,NP, & 0.99999 \nonumber\\
of_an & 0.99999 \nonumber\\
pursuit_can & 0.99999 \nonumber\\
for_anyone & 0.99999 \nonumber\\
we_live & 0.99999 \nonumber\\
sick & 0.99999 \nonumber\\
stutter_. & 0.99999 \nonumber\\
to_fear & 0.99999 \nonumber\\
physical_abuse & 0.99999 \nonumber\\
abuse_toward & 0.99999 \nonumber\\
fear_their & 0.99999 \nonumber\\
may_cause & 0.99999 \nonumber\\
child_cause & 0.99999 \nonumber\\
a_stutter & 0.99999 \nonumber\\
stutter & 0.99999 \nonumber\\
toward_child & 0.99999 \nonumber\\
_pos_ngram_ADV_V_CARD & 0.99999 \nonumber\\
rights_and & 0.99999 \nonumber\\
middle & 0.99999 \nonumber\\
ProductionRule_NP->PRP$,NNP, & 0.99999 \nonumber\\
people_with & 0.99999 \nonumber\\
without_the & 0.99999 \nonumber\\
some_other & 0.99999 \nonumber\\
ProductionRule_PRN->-LRB-,SBAR,-RRB-, & 0.99999 \nonumber\\
lay_out & 0.99999 \nonumber\\
,_also & 0.99999 \nonumber\\
not_william & 0.99999 \nonumber\\
that_remain & 0.99999 \nonumber\\
founder_. & 0.99999 \nonumber\\
who_lay & 0.99999 \nonumber\\
foundation_of & 0.99999 \nonumber\\
it_further & 0.99999 \nonumber\\
ProductionRule_NP->NP,,,CC,RB,NP, & 0.99999 \nonumber\\
hussien & 0.99999 \nonumber\\
give_him & 0.99999 \nonumber\\
sultan_hussien & 0.99999 \nonumber\\
a_treaty & 0.99999 \nonumber\\
and_return & 0.99999 \nonumber\\
develop_it & 0.99999 \nonumber\\
that_william & 0.99999 \nonumber\\
the_foundation & 0.99999 \nonumber\\
temenggong_and & 0.99999 \nonumber\\
hussien_, & 0.99999 \nonumber\\
also_develop & 0.99999 \nonumber\\
bencoolen_, & 0.99999 \nonumber\\
remain_in & 0.99999 \nonumber\\
position_because & 0.99999 \nonumber\\
no_physical & 0.99999 \nonumber\\
._exercise & 0.99999 \nonumber\\
sit_where & 0.99999 \nonumber\\
show_on & 0.99999 \nonumber\\
so_tv & 0.99999 \nonumber\\
book_!!!!!!! & 0.99999 \nonumber\\
so_no & 0.99999 \nonumber\\
move_. & 0.99999 \nonumber\\
one_sit & 0.99999 \nonumber\\
exercise_will & 0.99999 \nonumber\\
tv_in & 0.99999 \nonumber\\
where_as & 0.99999 \nonumber\\
then_book & 0.99999 \nonumber\\
get_do & 0.99999 \nonumber\\
tv_make & 0.99999 \nonumber\\
exercise_show & 0.99999 \nonumber\\
do_read & 0.99999 \nonumber\\
feel_bid & 0.99999 \nonumber\\
that_your & 0.99999 \nonumber\\
your_computer & 0.99999 \nonumber\\
can_imagine & 0.99999 \nonumber\\
dead & 0.99999 \nonumber\\
prejudice & 0.99999 \nonumber\\
prejudice_. & 0.99999 \nonumber\\
wrong_when & 0.99999 \nonumber\\
outside & 0.99999 \nonumber\\
mozillum_firefox & 0.99999 \nonumber\\
mozillum & 0.99999 \nonumber\\
grow_economy & 0.99999 \nonumber\\
girl_be & 0.99999 \nonumber\\
bible_say & 0.99999 \nonumber\\
as_one & 0.99999 \nonumber\\
_pos_ngram_CONJ_O_CARD & 0.99999 \nonumber\\
bag_jeans & 0.99999 \nonumber\\
the_legacy & 0.99999 \nonumber\\
more_concern & 0.99999 \nonumber\\
academic_success & 0.99999 \nonumber\\
ProductionRule_NP->NP,,,IN,NP, & 0.99999 \nonumber\\
school_today & 0.99999 \nonumber\\
legacy_educational & 0.99999 \nonumber\\
classroom_and & 0.99999 \nonumber\\
trend_change & 0.99999 \nonumber\\
and_safety & 0.99999 \nonumber\\
hallway_of & 0.99999 \nonumber\\
,_large & 0.99999 \nonumber\\
hallway & 0.99999 \nonumber\\
to_behavior & 0.99999 \nonumber\\
of_low & 0.99999 \nonumber\\
the_classroom & 0.99999 \nonumber\\
the_hallway & 0.99999 \nonumber\\
,_bag & 0.99999 \nonumber\\
fashion_of & 0.99999 \nonumber\\
educational_resource & 0.99999 \nonumber\\
how_they & 0.99999 \nonumber\\
ProductionRule_NP->NN,CC,NNS,NN, & 0.99999 \nonumber\\
ProductionRule_NP->PRP$,JJ,NN,CC,NN, & 0.99999 \nonumber\\
as_fashion & 0.99999 \nonumber\\
jeans_, & 0.99999 \nonumber\\
,_low & 0.99999 \nonumber\\
and_achievement & 0.99999 \nonumber\\
and_trend & 0.99999 \nonumber\\
concern_with & 0.99999 \nonumber\\
be_perceive & 0.99999 \nonumber\\
rise_jeans & 0.99999 \nonumber\\
perceive_than & 0.99999 \nonumber\\
cut_shirt & 0.99999 \nonumber\\
large_trench & 0.99999 \nonumber\\
behavior_problem & 0.99999 \nonumber\\
with_how & 0.99999 \nonumber\\
bag & 0.99999 \nonumber\\
trench & 0.99999 \nonumber\\
fashion_and & 0.99999 \nonumber\\
safety_issue & 0.99999 \nonumber\\
trench_coat & 0.99999 \nonumber\\
achievement_. & 0.99999 \nonumber\\
low_rise & 0.99999 \nonumber\\
low_cut & 0.99999 \nonumber\\
coat_, & 0.99999 \nonumber\\
other_contribute & 0.99999 \nonumber\\
that_christianity & 0.99999 \nonumber\\
mouth & 0.99999 \nonumber\\
system_and & 0.99999 \nonumber\\
authority & 0.99999 \nonumber\\
ProductionRule_VP->VB,ADJP,,,S, & 0.99999 \nonumber\\
to_imagine & 0.99999 \nonumber\\
you_make & 0.99999 \nonumber\\
ProductionRule_VP->VBG,S,SBAR, & 0.99999 \nonumber\\
ProductionRule_PRN->,,S, & 0.99999 \nonumber\\
on_one & 0.99999 \nonumber\\
for_someone & 0.99999 \nonumber\\
ProductionRule_SBARQ->WHNP,SQ,., & 0.99999 \nonumber\\
ditrabution_. & 0.99999 \nonumber\\
for_ditrabution & 0.99999 \nonumber\\
ditrabution & 0.99999 \nonumber\\
good_light & 0.99999 \nonumber\\
light_weight & 0.99999 \nonumber\\
tax_break & 0.99999 \nonumber\\
indium_in & 0.99999 \nonumber\\
factor_, & 0.99999 \nonumber\\
factor & 0.99999 \nonumber\\
these_thing & 0.99999 \nonumber\\
with_many & 0.99999 \nonumber\\
_pos_ngram_NN_O_ADJ & 0.99999 \nonumber\\
when_they & 0.99999 \nonumber\\
mankind_. & 0.99999 \nonumber\\
a_book & 0.99999 \nonumber\\
perceive & 0.99999 \nonumber\\
_pos_ngram_PP_PP_PP & 0.99999 \nonumber\\
to_believe & 0.99999 \nonumber\\
all_evidence & 0.99999 \nonumber\\
ProductionRule_FRAG->X,VP,., & 0.99999 \nonumber\\
student_go & 0.99999 \nonumber\\
learn_at & 0.99999 \nonumber\\
(_student & 0.99999 \nonumber\\
uniform_) & 0.99999 \nonumber\\
n_school & 0.99999 \nonumber\\
wear_n & 0.99999 \nonumber\\
connection_between & 0.99999 \nonumber\\
uniform_wear & 0.99999 \nonumber\\
uniform_suck & 0.99999 \nonumber\\
no_connection & 0.99999 \nonumber\\
result_... & 0.99999 \nonumber\\
._wear & 0.99999 \nonumber\\
to_prepare & 0.99999 \nonumber\\
to_waste & 0.99999 \nonumber\\
mean_better & 0.99999 \nonumber\\
their_future & 0.99999 \nonumber\\
buy_uniform & 0.99999 \nonumber\\
between_uniform & 0.99999 \nonumber\\
better_learn & 0.99999 \nonumber\\
waste_money & 0.99999 \nonumber\\
school_result & 0.99999 \nonumber\\
wold_and & 0.99999 \nonumber\\
put_you & 0.99999 \nonumber\\
wold & 0.99999 \nonumber\\
norther & 0.99999 \nonumber\\
i_thick & 0.99999 \nonumber\\
be_educational & 0.99999 \nonumber\\
better_i & 0.99999 \nonumber\\
whole_norther & 0.99999 \nonumber\\
norther_wold & 0.99999 \nonumber\\
thick_that & 0.99999 \nonumber\\
to_advance & 0.99999 \nonumber\\
be_today & 0.99999 \nonumber\\
without_a & 0.99999 \nonumber\\
_pos_ngram_ADJ_ADJ_ADJ & 0.99999 \nonumber\\
imagination & 0.99999 \nonumber\\
at_least & 0.99999 \nonumber\\
father_can & 0.99999 \nonumber\\
work_and & 0.99999 \nonumber\\
the_actual & 0.99999 \nonumber\\
heart & 0.99999 \nonumber\\
man_. & 0.99999 \nonumber\\
5 & 0.99999 \nonumber\\
ProductionRule_S->``,NP,VP,., & 0.99999 \nonumber\\
abort & 0.99999 \nonumber\\
._hence & 0.99999 \nonumber\\
_pos_ngram_PR_O_O & 0.99999 \nonumber\\
coat & 0.99999 \nonumber\\
without_be & 0.99999 \nonumber\\
our_country & 0.99999 \nonumber\\
ProductionRule_NP->NP,PRN,SBAR, & 0.99999 \nonumber\\
level_. & 0.99999 \nonumber\\
._nobody & 0.99999 \nonumber\\
we_dont & 0.99999 \nonumber\\
the_light & 0.99999 \nonumber\\
understand_why & 0.99999 \nonumber\\
perform & 0.99999 \nonumber\\
football & 0.99999 \nonumber\\
than_internet & 0.99999 \nonumber\\
'_need & 0.99999 \nonumber\\
_pos_ngram_CONJ_PR_PR & 0.99999 \nonumber\\
you_from & 0.99999 \nonumber\\
,_jerk & 0.99999 \nonumber\\
off_be & 0.99999 \nonumber\\
up_way & 0.99999 \nonumber\\
justify & 0.99999 \nonumber\\
2gb & 0.99999 \nonumber\\
one_program & 0.99999 \nonumber\\
_pos_ngram_ART_CARD_CONJ & 0.99999 \nonumber\\
2gb_of & 0.99999 \nonumber\\
a_firefox & 0.99999 \nonumber\\
of_ram & 0.99999 \nonumber\\
ram & 0.99999 \nonumber\\
ram_on & 0.99999 \nonumber\\
two_advantage & 0.99999 \nonumber\\
suck_up & 0.99999 \nonumber\\
have_2gb & 0.99999 \nonumber\\
to_justify & 0.99999 \nonumber\\
justify_the & 0.99999 \nonumber\\
firefox_suck & 0.99999 \nonumber\\
program_at & 0.99999 \nonumber\\
way_too & 0.99999 \nonumber\\
learn_mistake & 0.99999 \nonumber\\
you_motivation & 0.99999 \nonumber\\
do_better & 0.99999 \nonumber\\
from_and & 0.99999 \nonumber\\
your_mind & 0.99999 \nonumber\\
question_in & 0.99999 \nonumber\\
mistake_from & 0.99999 \nonumber\\
view_that & 0.99999 \nonumber\\
something_be & 0.99999 \nonumber\\
and_agree & 0.99999 \nonumber\\
contain & 0.99999 \nonumber\\
percent_of & 0.99999 \nonumber\\
even_have & 0.99999 \nonumber\\
..._but & 0.99999 \nonumber\\
it_then & 0.99999 \nonumber\\
and_all & 0.99999 \nonumber\\
watch_the & 0.99999 \nonumber\\
also_have & 0.99999 \nonumber\\
ProductionRule_VP->VBP,ADVP,NP, & 0.99999 \nonumber\\
price & 0.99999 \nonumber\\
wrong_and & 0.99999 \nonumber\\
unite & 0.99999 \nonumber\\
keep & 0.99999 \nonumber\\
have_develop & 0.99999 \nonumber\\
ProductionRule_VP->VB,ADJP,SBAR, & 0.99999 \nonumber\\
look_very & 0.99999 \nonumber\\
original & 0.99999 \nonumber\\
a_week & 0.99999 \nonumber\\
annoy & 0.99999 \nonumber\\
disput & 0.99999 \nonumber\\
how_few & 0.99999 \nonumber\\
its_up & 0.99999 \nonumber\\
christian_side & 0.99999 \nonumber\\
ProductionRule_NP->JJ,VBN,NNS, & 0.99999 \nonumber\\
'd_like & 0.99999 \nonumber\\
ProductionRule_NP->JJ,POS, & 0.99999 \nonumber\\
make_our & 0.99999 \nonumber\\
disput_there & 0.99999 \nonumber\\
cuz_free & 0.99999 \nonumber\\
ProductionRule_VP->VB,PRT,SBAR, & 0.99999 \nonumber\\
'_cuz & 0.99999 \nonumber\\
people_dont & 0.99999 \nonumber\\
convince_other & 0.99999 \nonumber\\
mind_people & 0.99999 \nonumber\\
few_disput & 0.99999 \nonumber\\
bite & 0.99999 \nonumber\\
ensure & 0.99999 \nonumber\\
ensure_that & 0.99999 \nonumber\\
another_. & 0.99999 \nonumber\\
sick_in & 0.99999 \nonumber\\
than_firefox & 0.99999 \nonumber\\
?_woman & 0.99999 \nonumber\\
problem_and & 0.99999 \nonumber\\
would_like & 0.99999 \nonumber\\
to_share & 0.99999 \nonumber\\
exile & 0.99999 \nonumber\\
exile_by & 0.99999 \nonumber\\
raffle_even & 0.99999 \nonumber\\
ProductionRule_VP->ADVP,VBN,PP,SBAR, & 0.99999 \nonumber\\
unjustly_exile & 0.99999 \nonumber\\
surpass & 0.99999 \nonumber\\
to_surpass & 0.99999 \nonumber\\
_pos_ngram_ADV_ADJ_O & 0.99999 \nonumber\\
remains & 0.99999 \nonumber\\
after_a & 0.99999 \nonumber\\
distribute & 0.99999 \nonumber\\
rajasthan & 0.99999 \nonumber\\
government_can & 0.99999 \nonumber\\
of_astronomy & 0.99999 \nonumber\\
geographical_and & 0.99999 \nonumber\\
rajasthan_. & 0.99999 \nonumber\\
._eg & 0.99999 \nonumber\\
geographical & 0.99999 \nonumber\\
scarcity_in & 0.99999 \nonumber\\
heavy_rainfall & 0.99999 \nonumber\\
language_, & 0.99999 \nonumber\\
discover_water & 0.99999 \nonumber\\
28_way & 0.99999 \nonumber\\
can_certainly & 0.99999 \nonumber\\
,_aryabhatta & 0.99999 \nonumber\\
indium_discover & 0.99999 \nonumber\\
28_state & 0.99999 \nonumber\\
low_. & 0.99999 \nonumber\\
with_28 & 0.99999 \nonumber\\
rainfall_in & 0.99999 \nonumber\\
._economically & 0.99999 \nonumber\\
aryabhatta & 0.99999 \nonumber\\
say_about & 0.99999 \nonumber\\
moon_. & 0.99999 \nonumber\\
aryabhatta_be & 0.99999 \nonumber\\
that_low & 0.99999 \nonumber\\
father_of & 0.99999 \nonumber\\
certainly_can & 0.99999 \nonumber\\
from_indium & 0.99999 \nonumber\\
of_28 & 0.99999 \nonumber\\
economically_also & 0.99999 \nonumber\\
on_moon & 0.99999 \nonumber\\
water_scarcity & 0.99999 \nonumber\\
eg_: & 0.99999 \nonumber\\
scarcity & 0.99999 \nonumber\\
chandrayaan & 0.99999 \nonumber\\
chandrayaan_from & 0.99999 \nonumber\\
in_rajasthan & 0.99999 \nonumber\\
look_after & 0.99999 \nonumber\\
rainfall & 0.99999 \nonumber\\
be_heavy & 0.99999 \nonumber\\
manipur_, & 0.99999 \nonumber\\
in_manipur & 0.99999 \nonumber\\
astronomy_, & 0.99999 \nonumber\\
astronomy & 0.99999 \nonumber\\
,_culture & 0.99999 \nonumber\\
wonderful_technological & 0.99999 \nonumber\\
:_chandrayaan & 0.99999 \nonumber\\
manipur & 0.99999 \nonumber\\
u_say & 0.99999 \nonumber\\
also_indium & 0.99999 \nonumber\\
,_geographical & 0.99999 \nonumber\\
go_against & 0.99999 \nonumber\\
dictionary_, & 0.99999 \nonumber\\
someone_murder & 0.99999 \nonumber\\
charge_for & 0.99999 \nonumber\\
dictionary & 0.99999 \nonumber\\
excuss & 0.99999 \nonumber\\
the_chil & 0.99999 \nonumber\\
pregnant_woman & 0.99999 \nonumber\\
unborn_baby & 0.99999 \nonumber\\
chil & 0.99999 \nonumber\\
chil_, & 0.99999 \nonumber\\
woman_get & 0.99999 \nonumber\\
the_fetus & 0.99999 \nonumber\\
stupid_excuss & 0.99999 \nonumber\\
the_stupid & 0.99999 \nonumber\\
the_dictionary & 0.99999 \nonumber\\
excuss_that & 0.99999 \nonumber\\
murder_a & 0.99999 \nonumber\\
should_put & 0.99999 \nonumber\\
get_charge & 0.99999 \nonumber\\
look_it & 0.99999 \nonumber\\
a_limit & 0.99999 \nonumber\\
love_and & 0.99999 \nonumber\\
also_some & 0.99999 \nonumber\\
_pos_ngram_NN_ART_ADV & 0.99999 \nonumber\\
have_any & 0.99999 \nonumber\\
nothing_. & 0.99999 \nonumber\\
which_lead & 0.99999 \nonumber\\
"_it & 0.99999 \nonumber\\
of_her & 0.99999 \nonumber\\
send_off & 0.99999 \nonumber\\
to_him & 0.99999 \nonumber\\
you_even & 0.99999 \nonumber\\
least & 0.99999 \nonumber\\
of_his & 0.99999 \nonumber\\
the_purist & 0.99999 \nonumber\\
liberty & 0.99999 \nonumber\\
liberty_and & 0.99999 \nonumber\\
independence_that & 0.99999 \nonumber\\
declaration & 0.99999 \nonumber\\
ProductionRule_VP->VB,RB,ADVP,VP, & 0.99999 \nonumber\\
dose_n't & 0.99999 \nonumber\\
purist_of & 0.99999 \nonumber\\
the_declaration & 0.99999 \nonumber\\
life_liberty & 0.99999 \nonumber\\
declaration_of & 0.99999 \nonumber\\
purist & 0.99999 \nonumber\\
next & 0.99999 \nonumber\\
by_my & 0.99999 \nonumber\\
wear_uniform & 0.99999 \nonumber\\
teamwork & 0.99999 \nonumber\\
ProductionRule_WHNP->WHNP,NP, & 0.99999 \nonumber\\
?_be & 0.99999 \nonumber\\
school_to & 0.99999 \nonumber\\
-_if & 0.99999 \nonumber\\
just_would & 0.99999 \nonumber\\
maturity & 0.99999 \nonumber\\
not_feel & 0.99999 \nonumber\\
they_choose & 0.99999 \nonumber\\
existence & 0.99999 \nonumber\\
many_other & 0.99999 \nonumber\\
if_so & 0.99999 \nonumber\\
there_, & 0.99999 \nonumber\\
judaism & 0.99999 \nonumber\\
virus_study & 0.99999 \nonumber\\
make_use & 0.99999 \nonumber\\
straw_man & 0.99999 \nonumber\\
biotic_? & 0.99999 \nonumber\\
use_evolution & 0.99999 \nonumber\\
they_evolve & 0.99999 \nonumber\\
experiment_and & 0.99999 \nonumber\\
moth_experiment & 0.99999 \nonumber\\
other_experiments/observations & 0.99999 \nonumber\\
record_carbon & 0.99999 \nonumber\\
virus_reproduce & 0.99999 \nonumber\\
_pos_ngram_NP_NN_NP & 0.99999 \nonumber\\
evolve_, & 0.99999 \nonumber\\
virus_. & 0.99999 \nonumber\\
experiments/observations_do & 0.99999 \nonumber\\
ultimate_straw & 0.99999 \nonumber\\
how_strain & 0.99999 \nonumber\\
experiments/observations & 0.99999 \nonumber\\
experiment_be & 0.99999 \nonumber\\
study_ohh & 0.99999 \nonumber\\
biotic & 0.99999 \nonumber\\
virus_become & 0.99999 \nonumber\\
time_period & 0.99999 \nonumber\\
show_evolution & 0.99999 \nonumber\\
evolve_over & 0.99999 \nonumber\\
anti_biotic & 0.99999 \nonumber\\
observe & 0.99999 \nonumber\\
strain & 0.99999 \nonumber\\
injection_be & 0.99999 \nonumber\\
carbon_date & 0.99999 \nonumber\\
gene_fossil & 0.99999 \nonumber\\
strain_of & 0.99999 \nonumber\\
_pos_ngram_NN_NP_NN & 0.99999 \nonumber\\
fossil_record & 0.99999 \nonumber\\
ohh_yeah & 0.99999 \nonumber\\
because_virus & 0.99999 \nonumber\\
fossil & 0.99999 \nonumber\\
of_virus & 0.99999 \nonumber\\
shorter_time & 0.99999 \nonumber\\
to_anti & 0.99999 \nonumber\\
become_immune & 0.99999 \nonumber\\
injection & 0.99999 \nonumber\\
shorter & 0.99999 \nonumber\\
flu & 0.99999 \nonumber\\
anti & 0.99999 \nonumber\\
that_other & 0.99999 \nonumber\\
be_observe & 0.99999 \nonumber\\
carbon & 0.99999 \nonumber\\
datum_virus & 0.99999 \nonumber\\
reproduce_very & 0.99999 \nonumber\\
bid_experiment & 0.99999 \nonumber\\
by_human & 0.99999 \nonumber\\
quickly_they & 0.99999 \nonumber\\
immune_to & 0.99999 \nonumber\\
n't_show & 0.99999 \nonumber\\
straw & 0.99999 \nonumber\\
how_ever & 0.99999 \nonumber\\
a_shorter & 0.99999 \nonumber\\
,_virus & 0.99999 \nonumber\\
observe_by & 0.99999 \nonumber\\
ohh & 0.99999 \nonumber\\
evolution_science & 0.99999 \nonumber\\
geological & 0.99999 \nonumber\\
geological_datum & 0.99999 \nonumber\\
flu_injection & 0.99999 \nonumber\\
date_geological & 0.99999 \nonumber\\
_pos_ngram_PUNC_NN_NP & 0.99999 \nonumber\\
your_flu & 0.99999 \nonumber\\
period_and & 0.99999 \nonumber\\
n't_look & 0.99999 \nonumber\\
people_and & 0.99999 \nonumber\\
hit_. & 0.99999 \nonumber\\
there_child & 0.99999 \nonumber\\
_pos_ngram_ADV_PP_CARD & 0.99999 \nonumber\\
it_tv & 0.99999 \nonumber\\
brain_. & 0.99999 \nonumber\\
kid_there & 0.99999 \nonumber\\
ProductionRule_S->S,CC,S,,,S,,,S,CC,S, & 0.99999 \nonumber\\
play_for & 0.99999 \nonumber\\
suck_at & 0.99999 \nonumber\\
class_i & 0.99999 \nonumber\\
example_i & 0.99999 \nonumber\\
kid_unhappy & 0.99999 \nonumber\\
n't_play & 0.99999 \nonumber\\
the_team & 0.99999 \nonumber\\
ProductionRule_NP->DT,JJ,S, & 0.99999 \nonumber\\
last_, & 0.99999 \nonumber\\
i_suck & 0.99999 \nonumber\\
ProductionRule_VP->VBZ,RB,ADVP,NP, & 0.99999 \nonumber\\
do_p.e. & 0.99999 \nonumber\\
last_to & 0.99999 \nonumber\\
ProductionRule_VP->RB,VBN,PP, & 0.99999 \nonumber\\
in_anything & 0.99999 \nonumber\\
p.e._class & 0.99999 \nonumber\\
adult_who & 0.99999 \nonumber\\
hate_i & 0.99999 \nonumber\\
choose_for & 0.99999 \nonumber\\
be_choose & 0.99999 \nonumber\\
make_kid & 0.99999 \nonumber\\
alway_the & 0.99999 \nonumber\\
obese_adult & 0.99999 \nonumber\\
at_p.e. & 0.99999 \nonumber\\
p.e._and & 0.99999 \nonumber\\
choose_last & 0.99999 \nonumber\\
unhappy_, & 0.99999 \nonumber\\
get_sad & 0.99999 \nonumber\\
just_obese & 0.99999 \nonumber\\
many_obese & 0.99999 \nonumber\\
p.e._just & 0.99999 \nonumber\\
team_and & 0.99999 \nonumber\\
not_cool & 0.99999 \nonumber\\
and_p.e. & 0.99999 \nonumber\\
life_be & 0.99999 \nonumber\\
them_no & 0.99999 \nonumber\\
state_, & 0.99999 \nonumber\\
!_they & 0.99999 \nonumber\\
basis & 0.99999 \nonumber\\
universe_be & 0.99999 \nonumber\\
law_be & 0.99999 \nonumber\\
accident & 0.99999 \nonumber\\
better_that & 0.99999 \nonumber\\
evolution_? & 0.99999 \nonumber\\
every_day & 0.99999 \nonumber\\
explain & 0.99999 \nonumber\\
so_who & 0.99999 \nonumber\\
,_student & 0.99999 \nonumber\\
ProductionRule_VP->VBZ,ADJP,S,NP, & 0.99999 \nonumber\\
,_lut457 & 0.99999 \nonumber\\
sfjiiytg & 0.99999 \nonumber\\
ProductionRule_NP->FW,FW,FW,FW,FW,FW,FW, & 0.99999 \nonumber\\
;_o & 0.99999 \nonumber\\
;_l & 0.99999 \nonumber\\
ProductionRule_NP->NP,:,NP,:, & 0.99999 \nonumber\\
ProductionRule_NP->NP,,,NP,-RRB-, & 0.99999 \nonumber\\
ProductionRule_NP->NN,NN,-LRB-, & 0.99999 \nonumber\\
xtklp09 & 0.99999 \nonumber\\
dh_, & 0.99999 \nonumber\\
ihfej_tijkjdrk & 0.99999 \nonumber\\
ihfej & 0.99999 \nonumber\\
xtklp09_guil09 & 0.99999 \nonumber\\
dh & 0.99999 \nonumber\\
sfjiiytg_dh & 0.99999 \nonumber\\
lut457_p & 0.99999 \nonumber\\
o & 0.99999 \nonumber\\
lut457 & 0.99999 \nonumber\\
o_; & 0.99999 \nonumber\\
guil09_sfjiiytg & 0.99999 \nonumber\\
guil09 & 0.99999 \nonumber\\
p & 0.99999 \nonumber\\
book_dathu & 0.99999 \nonumber\\
[_] & 0.99999 \nonumber\\
p_[ & 0.99999 \nonumber\\
]_; & 0.99999 \nonumber\\
dathu_ihfej & 0.99999 \nonumber\\
dathu & 0.99999 \nonumber\\
tijkjdrk & 0.99999 \nonumber\\
tijkjdrk_xtklp09 & 0.99999 \nonumber\\
in_their & 0.99999 \nonumber\\
_pos_ngram_CONJ_ADV_NP & 0.99999 \nonumber\\
child_could & 0.99999 \nonumber\\
of_life & 0.99999 \nonumber\\
_pos_ngram_NP_CONJ_O & 0.99999 \nonumber\\
take_your & 0.99999 \nonumber\\
pro-life_, & 0.99999 \nonumber\\
..._u & 0.99999 \nonumber\\
multiple & 0.99999 \nonumber\\
secular & 0.99999 \nonumber\\
give_a & 0.99999 \nonumber\\
,_rather & 0.99999 \nonumber\\
and_porn & 0.99999 \nonumber\\
britisher & 0.99999 \nonumber\\
fiction & 0.99999 \nonumber\\
ProductionRule_ADJP->NP,RBR, & 0.99999 \nonumber\\
orginal & 0.99999 \nonumber\\
orginal_english & 0.99999 \nonumber\\
grammatical & 0.99999 \nonumber\\
grammatical_mistake & 0.99999 \nonumber\\
fiction_" & 0.99999 \nonumber\\
!!!!_" & 0.99999 \nonumber\\
stranger_than & 0.99999 \nonumber\\
britisher_and & 0.99999 \nonumber\\
of_grammatical & 0.99999 \nonumber\\
indian_!!!! & 0.99999 \nonumber\\
can_speak & 0.99999 \nonumber\\
english_man & 0.99999 \nonumber\\
than_fiction & 0.99999 \nonumber\\
be_stranger & 0.99999 \nonumber\\
"_truth & 0.99999 \nonumber\\
english_better & 0.99999 \nonumber\\
...._indian & 0.99999 \nonumber\\
include_a & 0.99999 \nonumber\\
better_.... & 0.99999 \nonumber\\
and_american & 0.99999 \nonumber\\
than_orginal & 0.99999 \nonumber\\
"_..... & 0.99999 \nonumber\\
american_speech & 0.99999 \nonumber\\
speech_include & 0.99999 \nonumber\\
._britisher & 0.99999 \nonumber\\
speak_english & 0.99999 \nonumber\\
and_some & 0.99999 \nonumber\\
here_. & 0.99999 \nonumber\\
even_better & 0.99999 \nonumber\\
enviroment_. & 0.99999 \nonumber\\
enviroment & 0.99999 \nonumber\\
ProductionRule_NP->PRP$,NN,NNS, & 0.99999 \nonumber\\
of_reason & 0.99999 \nonumber\\
feel_good & 0.99999 \nonumber\\
,_child & 0.99999 \nonumber\\
probably_would & 0.99999 \nonumber\\
ask_yourself & 0.99999 \nonumber\\
_pos_ngram_PUNC_O_NN & 0.99999 \nonumber\\
in_thier & 0.99999 \nonumber\\
sector & 0.99999 \nonumber\\
jesus & 0.99999 \nonumber\\
for_life & 0.99999 \nonumber\\
:_porn & 0.99999 \nonumber\\
pocket & 0.99999 \nonumber\\
a_world & 0.99999 \nonumber\\
to_ruin & 0.99999 \nonumber\\
world_! & 0.99999 \nonumber\\
ruin_the & 0.99999 \nonumber\\
us_will & 0.99999 \nonumber\\
,_us & 0.99999 \nonumber\\
off_! & 0.99999 \nonumber\\
screw_off & 0.99999 \nonumber\\
!_screw & 0.99999 \nonumber\\
dominate_, & 0.99999 \nonumber\\
china_will & 0.99999 \nonumber\\
will_dominate & 0.99999 \nonumber\\
!_china & 0.99999 \nonumber\\
ProductionRule_VP->VBG,NP,ADVP, & 0.99999 \nonumber\\
average & 0.99999 \nonumber\\
material & 0.99999 \nonumber\\
care_, & 0.99999 \nonumber\\
to_answer & 0.99999 \nonumber\\
wrong_!!!! & 0.99999 \nonumber\\
_pos_ngram_O_O_CONJ & 0.99999 \nonumber\\
then_so & 0.99999 \nonumber\\
thing_like & 0.99999 \nonumber\\
effect_on & 0.99999 \nonumber\\
severely & 0.99999 \nonumber\\
_pos_ngram_NN_ART_PP & 0.99999 \nonumber\\
very_little & 0.99999 \nonumber\\
irresponsible & 0.99999 \nonumber\\
be_irresponsible & 0.99999 \nonumber\\
n't_you & 0.99999 \nonumber\\
._atheism & 0.99999 \nonumber\\
if_his & 0.99999 \nonumber\\
mess_up & 0.99999 \nonumber\\
obviously_he & 0.99999 \nonumber\\
he_commit & 0.99999 \nonumber\\
be_mess & 0.99999 \nonumber\\
._obviously & 0.99999 \nonumber\\
ProductionRule_VP->VBZ,RB,SBAR, & 0.99999 \nonumber\\
attack_will & 0.99999 \nonumber\\
head_if & 0.99999 \nonumber\\
murderer_be & 0.99999 \nonumber\\
next_attack & 0.99999 \nonumber\\
his_next & 0.99999 \nonumber\\
not_who & 0.99999 \nonumber\\
marry_. & 0.99999 \nonumber\\
ProductionRule_NP->DT,CD,NN, & 0.99999 \nonumber\\
_pos_ngram_PUNC_PUNC_NN & 0.99999 \nonumber\\
as_many & 0.99999 \nonumber\\
be_afraid & 0.99999 \nonumber\\
put_them & 0.99999 \nonumber\\
_pos_ngram_ADJ_O_PP & 0.99999 \nonumber\\
nobody & 0.99999 \nonumber\\
_pos_ngram_PR_PUNC_NP & 0.99999 \nonumber\\
freak & 0.99999 \nonumber\\
jerk_off & 0.99999 \nonumber\\
to_promote & 0.99999 \nonumber\\
_pos_ngram_PUNC_NP_PP & 0.99999 \nonumber\\
ProductionRule_VP->VB,ADJP,S, & 0.99999 \nonumber\\
what_people & 0.99999 \nonumber\\
help_a & 0.99999 \nonumber\\
ProductionRule_FRAG->ADVP,., & 0.99999 \nonumber\\
future_, & 0.99999 \nonumber\\
false & 0.99999 \nonumber\\
truth_be & 0.99999 \nonumber\\
and_think & 0.99999 \nonumber\\
more_like & 0.99999 \nonumber\\
donot & 0.99999 \nonumber\\
donot_have & 0.99999 \nonumber\\
_pos_ngram_O_V_O & 0.99999 \nonumber\\
everything_be & 0.99999 \nonumber\\
merely & 0.99999 \nonumber\\
can_we & 0.99999 \nonumber\\
_pos_ngram_NN_CARD_ADJ & 0.99999 \nonumber\\
definition_of & 0.99999 \nonumber\\
him_for & 0.99999 \nonumber\\
recent & 0.99999 \nonumber\\
in_movie & 0.99999 \nonumber\\
word_in & 0.99999 \nonumber\\
in_song & 0.99999 \nonumber\\
evil_to & 0.99999 \nonumber\\
or_tv & 0.99999 \nonumber\\
song_, & 0.99999 \nonumber\\
movie_or & 0.99999 \nonumber\\
scene_in & 0.99999 \nonumber\\
illegal_? & 0.99999 \nonumber\\
?_nope & 0.99999 \nonumber\\
your_right & 0.99999 \nonumber\\
have_swear & 0.99999 \nonumber\\
be_entertainment & 0.99999 \nonumber\\
and_evil & 0.99999 \nonumber\\
sex_scene & 0.99999 \nonumber\\
should_sex & 0.99999 \nonumber\\
swear & 0.99999 \nonumber\\
?_of & 0.99999 \nonumber\\
swear_word & 0.99999 \nonumber\\
tire_to & 0.99999 \nonumber\\
something_with & 0.99999 \nonumber\\
food_on & 0.99999 \nonumber\\
._id & 0.99999 \nonumber\\
put_food & 0.99999 \nonumber\\
to_but & 0.99999 \nonumber\\
table & 0.99999 \nonumber\\
the_table & 0.99999 \nonumber\\
mother_who & 0.99999 \nonumber\\
everyday_to & 0.99999 \nonumber\\
id_rather & 0.99999 \nonumber\\
table_. & 0.99999 \nonumber\\
work_everyday & 0.99999 \nonumber\\
raise_by & 0.99999 \nonumber\\
mad_. & 0.99999 \nonumber\\
who_tire & 0.99999 \nonumber\\
be_care & 0.99999 \nonumber\\
could_not & 0.99999 \nonumber\\
straight_be & 0.99999 \nonumber\\
ProductionRule_FRAG->SBAR,,,WHADVP,., & 0.99999 \nonumber\\
cant_gay & 0.99999 \nonumber\\
if_straight & 0.99999 \nonumber\\
time_a & 0.99999 \nonumber\\
even_cancer & 0.99999 \nonumber\\
certain_type & 0.99999 \nonumber\\
of_disease & 0.99999 \nonumber\\
cancer_. & 0.99999 \nonumber\\
be_direct & 0.99999 \nonumber\\
direct & 0.99999 \nonumber\\
and_certain & 0.99999 \nonumber\\
link_to & 0.99999 \nonumber\\
disease_, & 0.99999 \nonumber\\
direct_link & 0.99999 \nonumber\\
people_that & 0.99999 \nonumber\\
her_: & 0.99999 \nonumber\\
shit_. & 0.99999 \nonumber\\
"_me & 0.99999 \nonumber\\
"_hope & 0.99999 \nonumber\\
ProductionRule_NP->PDT,PRP$,NN, & 0.99999 \nonumber\\
shit & 0.99999 \nonumber\\
ProductionRule_S->S,:,``,S,.,'', & 0.99999 \nonumber\\
#h_" & 0.99999 \nonumber\\
leave_you & 0.99999 \nonumber\\
^_#h & 0.99999 \nonumber\\
take_half & 0.99999 \nonumber\\
me_: & 0.99999 \nonumber\\
prenup & 0.99999 \nonumber\\
prison_b & 0.99999 \nonumber\\
#h & 0.99999 \nonumber\\
b_* & 0.99999 \nonumber\\
a_prenup & 0.99999 \nonumber\\
your_shit & 0.99999 \nonumber\\
prenup_:) & 0.99999 \nonumber\\
:)_her & 0.99999 \nonumber\\
like_prison & 0.99999 \nonumber\\
half_your & 0.99999 \nonumber\\
_pos_ngram_NP_PR_PP & 0.99999 \nonumber\\
can_lead & 0.99999 \nonumber\\
that_how & 0.99999 \nonumber\\
be_remove & 0.99999 \nonumber\\
face_by & 0.99999 \nonumber\\
people_well & 0.99999 \nonumber\\
ProductionRule_ADJP->RB,RB,PP, & 0.99999 \nonumber\\
position_by & 0.99999 \nonumber\\
help_farquhar & 0.99999 \nonumber\\
problem_face & 0.99999 \nonumber\\
grow_too & 0.99999 \nonumber\\
remove_from & 0.99999 \nonumber\\
raffle_because & 0.99999 \nonumber\\
farquhar_solve & 0.99999 \nonumber\\
ProductionRule_NP->PRP,DT, & 0.99999 \nonumber\\
adam_and & 0.99999 \nonumber\\
my_system & 0.99999 \nonumber\\
memory_to & 0.99999 \nonumber\\
you_that & 0.99999 \nonumber\\
their_religion & 0.99999 \nonumber\\
ie_user & 0.99999 \nonumber\\
ProductionRule_NP->NNS,NNS, & 0.99999 \nonumber\\
may_also & 0.99999 \nonumber\\
will_not & 0.99999 \nonumber\\
day_to & 0.99999 \nonumber\\
student_become & 0.99999 \nonumber\\
grow_. & 0.99999 \nonumber\\
sit_on & 0.99999 \nonumber\\
out_on & 0.99999 \nonumber\\
to_different & 0.99999 \nonumber\\
app & 0.99999 \nonumber\\
life_you & 0.99999 \nonumber\\
reason_, & 0.99999 \nonumber\\
nerd & 0.99999 \nonumber\\
get_me & 0.99999 \nonumber\\
on_me & 0.99999 \nonumber\\
ProductionRule_NP->RB,DT,NN, & 0.99999 \nonumber\\
someone_there & 0.99999 \nonumber\\
species_come & 0.99999 \nonumber\\
._action & 0.99999 \nonumber\\
right_cold & 0.99999 \nonumber\\
blood_murder & 0.99999 \nonumber\\
bind_us & 0.99999 \nonumber\\
down_right & 0.99999 \nonumber\\
love_that & 0.99999 \nonumber\\
us_together & 0.99999 \nonumber\\
than_likely & 0.99999 \nonumber\\
flip_side & 0.99999 \nonumber\\
flip & 0.99999 \nonumber\\
the_flip & 0.99999 \nonumber\\
ProductionRule_S->ADJP,NP,VP,., & 0.99999 \nonumber\\
but_on & 0.99999 \nonumber\\
just_down & 0.99999 \nonumber\\
cold_blood & 0.99999 \nonumber\\
that_love & 0.99999 \nonumber\\
that_bind & 0.99999 \nonumber\\
ProductionRule_S->NP,,,NP,VP, & 0.99999 \nonumber\\
do_u & 0.99999 \nonumber\\
set_the & 0.99999 \nonumber\\
make_out & 0.99999 \nonumber\\
respect_by & 0.99999 \nonumber\\
well_respect & 0.99999 \nonumber\\
computer_. & 0.99999 \nonumber\\
rightful & 0.99999 \nonumber\\
rightful_founder & 0.99999 \nonumber\\
the_rightful & 0.99999 \nonumber\\
headgear & 0.99999 \nonumber\\
headgear_. & 0.99999 \nonumber\\
!_usa & 0.99999 \nonumber\\
for_scrub & 0.99999 \nonumber\\
nope_last & 0.99999 \nonumber\\
rag & 0.99999 \nonumber\\
rag_be & 0.99999 \nonumber\\
whooo & 0.99999 \nonumber\\
not_fricken & 0.99999 \nonumber\\
scrub & 0.99999 \nonumber\\
scrub_toilet & 0.99999 \nonumber\\
whooo_! & 0.99999 \nonumber\\
toilet & 0.99999 \nonumber\\
fricken & 0.99999 \nonumber\\
fricken_headgear & 0.99999 \nonumber\\
toilet_not & 0.99999 \nonumber\\
._whooo & 0.99999 \nonumber\\
ProductionRule_PP->RB,NP, & 0.99999 \nonumber\\
check_rag & 0.99999 \nonumber\\
learn_that & 0.99999 \nonumber\\
bull & 0.99999 \nonumber\\
the_dutch & 0.99999 \nonumber\\
abortion_or & 0.99999 \nonumber\\
itt_its & 0.99999 \nonumber\\
should_all & 0.99999 \nonumber\\
not_disease & 0.99999 \nonumber\\
with_itt & 0.99999 \nonumber\\
disease_we & 0.99999 \nonumber\\
business_!!! & 0.99999 \nonumber\\
our_business & 0.99999 \nonumber\\
their_attention & 0.99999 \nonumber\\
she_will & 0.99999 \nonumber\\
ago_. & 0.99999 \nonumber\\
word_" & 0.99999 \nonumber\\
have_one & 0.99999 \nonumber\\
._third & 0.99999 \nonumber\\
government_would & 0.99999 \nonumber\\
the_equal & 0.99999 \nonumber\\
be_non & 0.99999 \nonumber\\
fundamental_right & 0.99999 \nonumber\\
still_part & 0.99999 \nonumber\\
gender_to & 0.99999 \nonumber\\
gay_have & 0.99999 \nonumber\\
existent & 0.99999 \nonumber\\
image_if & 0.99999 \nonumber\\
the_fundamental & 0.99999 \nonumber\\
third_of & 0.99999 \nonumber\\
third_gender & 0.99999 \nonumber\\
non_existent & 0.99999 \nonumber\\
fundamental & 0.99999 \nonumber\\
of_equal & 0.99999 \nonumber\\
that_racism & 0.99999 \nonumber\\
and_hatr & 0.99999 \nonumber\\
better_image & 0.99999 \nonumber\\
it_only & 0.99999 \nonumber\\
allow_the & 0.99999 \nonumber\\
equal_right & 0.99999 \nonumber\\
the_third & 0.99999 \nonumber\\
equal_happiness & 0.99999 \nonumber\\
we_allow & 0.99999 \nonumber\\
of_society & 0.99999 \nonumber\\
hatr_be & 0.99999 \nonumber\\
hatr & 0.99999 \nonumber\\
second_of & 0.99999 \nonumber\\
existent_. & 0.99999 \nonumber\\
heavy & 0.99999 \nonumber\\
._moreover & 0.99999 \nonumber\\
jail & 0.99999 \nonumber\\
jail_. & 0.99999 \nonumber\\
your_hand & 0.99999 \nonumber\\
sort & 0.99999 \nonumber\\
me_by & 0.99999 \nonumber\\
in_becuase & 0.99999 \nonumber\\
by_tell & 0.99999 \nonumber\\
becuase & 0.99999 \nonumber\\
becuase_she & 0.99999 \nonumber\\
,_ironic & 0.99999 \nonumber\\
ProductionRule_S->S,IN,S,., & 0.99999 \nonumber\\
ProductionRule_ADJP->ADJP,FRAG, & 0.99999 \nonumber\\
pro-lifer & 0.99999 \nonumber\\
ironic_eh & 0.99999 \nonumber\\
pro-lifer_want & 0.99999 \nonumber\\
live_baby & 0.99999 \nonumber\\
be_dead & 0.99999 \nonumber\\
want_live & 0.99999 \nonumber\\
baby_so & 0.99999 \nonumber\\
ProductionRule_VP->VP,,,ADJP, & 0.99999 \nonumber\\
they_bring & 0.99999 \nonumber\\
dead_soldier & 0.99999 \nonumber\\
bring_into & 0.99999 \nonumber\\
people_too & 0.99999 \nonumber\\
please_. & 0.99999 \nonumber\\
not_tell & 0.99999 \nonumber\\
othere_remains & 0.99999 \nonumber\\
dinosaur_and & 0.99999 \nonumber\\
dinosaur & 0.99999 \nonumber\\
._dinosaur & 0.99999 \nonumber\\
all_othere & 0.99999 \nonumber\\
noah & 0.99999 \nonumber\\
rock_but & 0.99999 \nonumber\\
layer_of & 0.99999 \nonumber\\
othere & 0.99999 \nonumber\\
animal_and & 0.99999 \nonumber\\
people_all & 0.99999 \nonumber\\
same_layer & 0.99999 \nonumber\\
remains_in & 0.99999 \nonumber\\
find_dinosaur & 0.99999 \nonumber\\
remains_of & 0.99999 \nonumber\\
._think & 0.99999 \nonumber\\
flood_of & 0.99999 \nonumber\\
different_layer & 0.99999 \nonumber\\
at_different & 0.99999 \nonumber\\
the_remains & 0.99999 \nonumber\\
find_this & 0.99999 \nonumber\\
dinosaur_bone & 0.99999 \nonumber\\
dont_. & 0.99999 \nonumber\\
flood_have & 0.99999 \nonumber\\
not_find & 0.99999 \nonumber\\
different_depths & 0.99999 \nonumber\\
flood & 0.99999 \nonumber\\
noah_happen & 0.99999 \nonumber\\
of_rock & 0.99999 \nonumber\\
bone & 0.99999 \nonumber\\
several_different & 0.99999 \nonumber\\
in_several & 0.99999 \nonumber\\
long_dead & 0.99999 \nonumber\\
depths_. & 0.99999 \nonumber\\
depths & 0.99999 \nonumber\\
this_at & 0.99999 \nonumber\\
have_scientific & 0.99999 \nonumber\\
bone_be & 0.99999 \nonumber\\
of_noah & 0.99999 \nonumber\\
about_this & 0.99999 \nonumber\\
should_expect & 0.99999 \nonumber\\
stratum_, & 0.99999 \nonumber\\
of_long & 0.99999 \nonumber\\
dead_animal & 0.99999 \nonumber\\
noah_could & 0.99999 \nonumber\\
the_flood & 0.99999 \nonumber\\
healthier & 0.99999 \nonumber\\
spank_to & 0.99999 \nonumber\\
in_his & 0.99999 \nonumber\\
elective_subject & 0.99999 \nonumber\\
an_elective & 0.99999 \nonumber\\
ProductionRule_S->S,,,ADVP,,,S,., & 0.99999 \nonumber\\
elective & 0.99999 \nonumber\\
be_put & 0.99999 \nonumber\\
side_and & 0.99999 \nonumber\\
be_free & 0.99999 \nonumber\\
reason_be & 0.99999 \nonumber\\
be_download & 0.99999 \nonumber\\
soul_. & 0.99999 \nonumber\\
the_soul & 0.99999 \nonumber\\
abstract & 0.99999 \nonumber\\
an_abstract & 0.99999 \nonumber\\
best_friend & 0.99999 \nonumber\\
female_and & 0.99999 \nonumber\\
like_people & 0.99999 \nonumber\\
gay_they & 0.99999 \nonumber\\
have_every & 0.99999 \nonumber\\
straight_. & 0.99999 \nonumber\\
friend_who & 0.99999 \nonumber\\
two_best & 0.99999 \nonumber\\
as_when & 0.99999 \nonumber\\
husband_. & 0.99999 \nonumber\\
every_right & 0.99999 \nonumber\\
_pos_ngram_PUNC_CARD_V & 0.99999 \nonumber\\
male_. & 0.99999 \nonumber\\
love_who & 0.99999 \nonumber\\
their_partner & 0.99999 \nonumber\\
marry_just & 0.99999 \nonumber\\
be_male & 0.99999 \nonumber\\
nice & 0.99999 \nonumber\\
ProductionRule_VP->VBG,NP,S, & 0.99999 \nonumber\\
ProductionRule_SQ->VBZ,NP,VP, & 0.99999 \nonumber\\
great_, & 0.99999 \nonumber\\
can_see & 0.99999 \nonumber\\
convince & 0.99999 \nonumber\\
the_mother & 0.99999 \nonumber\\
they_could & 0.99999 \nonumber\\
eh_? & 0.99999 \nonumber\\
)_i & 0.99999 \nonumber\\
pollution_. & 0.99999 \nonumber\\
ProductionRule_VP->MD,RB,ADVP,VP, & 0.99999 \nonumber\\
ProductionRule_NP->NP,PP,VP, & 0.99999 \nonumber\\
though_raffle & 0.99999 \nonumber\\
find_that & 0.99999 \nonumber\\
work_as & 0.99999 \nonumber\\
for_people & 0.99999 \nonumber\\
a_stop & 0.99999 \nonumber\\
_pos_ngram_CARD_ART_PUNC & 0.99999 \nonumber\\
encourage_racism & 0.99999 \nonumber\\
one_another & 0.99999 \nonumber\\
us_prejudice & 0.99999 \nonumber\\
and_homophobia & 0.99999 \nonumber\\
many_war & 0.99999 \nonumber\\
stop_to & 0.99999 \nonumber\\
homophobia & 0.99999 \nonumber\\
past_have & 0.99999 \nonumber\\
it_encourage & 0.99999 \nonumber\\
_pos_ngram_V_CARD_ART & 0.99999 \nonumber\\
homophobia_. & 0.99999 \nonumber\\
us_hate & 0.99999 \nonumber\\
war_. & 0.99999 \nonumber\\
religion_in & 0.99999 \nonumber\\
ProductionRule_VP->NNP,PP, & 0.99999 \nonumber\\
hate_one & 0.99999 \nonumber\\
we_ca & 0.99999 \nonumber\\
measure & 0.99999 \nonumber\\
adopt_measure & 0.99999 \nonumber\\
atla & 0.99999 \nonumber\\
to_shake & 0.99999 \nonumber\\
would_drop & 0.99999 \nonumber\\
atla_would & 0.99999 \nonumber\\
level_think & 0.99999 \nonumber\\
shake_his & 0.99999 \nonumber\\
._atla & 0.99999 \nonumber\\
drop_the & 0.99999 \nonumber\\
world_for & 0.99999 \nonumber\\
shake & 0.99999 \nonumber\\
his_hand & 0.99999 \nonumber\\
he_just & 0.99999 \nonumber\\
religion_be & 0.99999 \nonumber\\
._sometime & 0.99999 \nonumber\\
you_and & 0.99999 \nonumber\\
evidence_to & 0.99999 \nonumber\\
the_ocean & 0.99999 \nonumber\\
ocean & 0.99999 \nonumber\\
a_crime & 0.99999 \nonumber\\
follow_so & 0.99999 \nonumber\\
curriculum_that & 0.99999 \nonumber\\
curriculum & 0.99999 \nonumber\\
require_to & 0.99999 \nonumber\\
obese_. & 0.99999 \nonumber\\
stricter_curriculum & 0.99999 \nonumber\\
say_her & 0.99999 \nonumber\\
should_learn & 0.99999 \nonumber\\
so_less & 0.99999 \nonumber\\
be_require & 0.99999 \nonumber\\
everything_say & 0.99999 \nonumber\\
less_people & 0.99999 \nonumber\\
healthy_lifestyle & 0.99999 \nonumber\\
ProductionRule_ADVP->RB,VP, & 0.99999 \nonumber\\
profit_on & 0.99999 \nonumber\\
so_make & 0.99999 \nonumber\\
a_profit & 0.99999 \nonumber\\
'_genius & 0.99999 \nonumber\\
ProductionRule_VP->VBZ,NP,,,ADVP, & 0.99999 \nonumber\\
any_of & 0.99999 \nonumber\\
while_there & 0.99999 \nonumber\\
classroom & 0.99999 \nonumber\\
out_as & 0.99999 \nonumber\\
idea_you & 0.99999 \nonumber\\
_pos_ngram_V_CARD_V & 0.99999 \nonumber\\
,_other & 0.99999 \nonumber\\
the_doubt & 0.99999 \nonumber\\
doubt_of & 0.99999 \nonumber\\
how_could & 0.99999 \nonumber\\
or_with & 0.99999 \nonumber\\
could_it & 0.99999 \nonumber\\
ProductionRule_ADJP->IN,JJ, & 0.99999 \nonumber\\
than_live & 0.99999 \nonumber\\
_pos_ngram_V_CARD_CONJ & 0.99999 \nonumber\\
put_a & 0.99999 \nonumber\\
free_mind & 0.99999 \nonumber\\
come_up & 0.99999 \nonumber\\
._by & 0.99999 \nonumber\\
the_matter & 0.99999 \nonumber\\
port & 0.99999 \nonumber\\
trade_port & 0.99999 \nonumber\\
that_bid & 0.99999 \nonumber\\
:_theworlddebating.com & 0.99999 \nonumber\\
website_but & 0.99999 \nonumber\\
this_website & 0.99999 \nonumber\\
very_clear & 0.99999 \nonumber\\
better_: & 0.99999 \nonumber\\
it_very & 0.99999 \nonumber\\
expect_to & 0.99999 \nonumber\\
and_help & 0.99999 \nonumber\\
_pos_ngram_PR_CONJ_PP & 0.99999 \nonumber\\
million_gallon & 0.99999 \nonumber\\
ProductionRule_VP->NN,NP,PP, & 0.99999 \nonumber\\
would_he & 0.99999 \nonumber\\
good_time & 0.99999 \nonumber\\
off_during & 0.99999 \nonumber\\
be_manage & 0.99999 \nonumber\\
time_raffle & 0.99999 \nonumber\\
respect_farquhar & 0.99999 \nonumber\\
when_william & 0.99999 \nonumber\\
three_time & 0.99999 \nonumber\\
good_leader & 0.99999 \nonumber\\
a_leader & 0.99999 \nonumber\\
send_raffle & 0.99999 \nonumber\\
leader_. & 0.99999 \nonumber\\
raffle_off & 0.99999 \nonumber\\
leader_, & 0.99999 \nonumber\\
founder_would & 0.99999 \nonumber\\
to_britain & 0.99999 \nonumber\\
the_organisation/group & 0.99999 \nonumber\\
manage_. & 0.99999 \nonumber\\
singapore_respect & 0.99999 \nonumber\\
the_combine & 0.99999 \nonumber\\
organisation/group_he & 0.99999 \nonumber\\
organisation/group & 0.99999 \nonumber\\
that_send & 0.99999 \nonumber\\
both_raffle & 0.99999 \nonumber\\
the_three & 0.99999 \nonumber\\
combine_number & 0.99999 \nonumber\\
competent_leader & 0.99999 \nonumber\\
be_send & 0.99999 \nonumber\\
more_competent & 0.99999 \nonumber\\
britain_, & 0.99999 \nonumber\\
farquhar_more & 0.99999 \nonumber\\
competent & 0.99999 \nonumber\\
life_at & 0.99999 \nonumber\\
insolence & 0.99999 \nonumber\\
teamwork_, & 0.99999 \nonumber\\
situational & 0.99999 \nonumber\\
greater_respect & 0.99999 \nonumber\\
drop_and & 0.99999 \nonumber\\
few_. & 0.99999 \nonumber\\
twenty_for & 0.99999 \nonumber\\
the_outdoors & 0.99999 \nonumber\\
,_reflexive & 0.99999 \nonumber\\
me_twenty & 0.99999 \nonumber\\
benefit_, & 0.99999 \nonumber\\
twenty & 0.99999 \nonumber\\
to_name & 0.99999 \nonumber\\
insolence_! & 0.99999 \nonumber\\
_pos_ngram_PR_CARD_PP & 0.99999 \nonumber\\
now_drop & 0.99999 \nonumber\\
the_greater & 0.99999 \nonumber\\
ProductionRule_FRAG->RB,PP,., & 0.99999 \nonumber\\
situational_calculation & 0.99999 \nonumber\\
camaraderie & 0.99999 \nonumber\\
outdoors & 0.99999 \nonumber\\
your_insolence & 0.99999 \nonumber\\
yes_of & 0.99999 \nonumber\\
reflexive_situational & 0.99999 \nonumber\\
name_but & 0.99999 \nonumber\\
,_teamwork & 0.99999 \nonumber\\
sport_camaraderie & 0.99999 \nonumber\\
,_sport & 0.99999 \nonumber\\
outdoors_, & 0.99999 \nonumber\\
calculation & 0.99999 \nonumber\\
health_benefit & 0.99999 \nonumber\\
calculation_to & 0.99999 \nonumber\\
camaraderie_, & 0.99999 \nonumber\\
reflexive & 0.99999 \nonumber\\
struggle & 0.99999 \nonumber\\
clear_. & 0.99999 \nonumber\\
ProductionRule_VP->VBZ,PP,ADVP, & 0.99999 \nonumber\\
great_idea & 0.99999 \nonumber\\
if_those & 0.99999 \nonumber\\
life_than & 0.99999 \nonumber\\
high_school & 0.99999 \nonumber\\
people_go & 0.99999 \nonumber\\
yea & 0.99999 \nonumber\\
even_as & 0.99999 \nonumber\\
provide_chance & 0.99999 \nonumber\\
pe_lesson & 0.99999 \nonumber\\
be_productive & 0.99999 \nonumber\\
ProductionRule_VP->VBG,ADJP,PP, & 0.99999 \nonumber\\
lesson_provide & 0.99999 \nonumber\\
ProductionRule_VP->VBP,NP,PP,S, & 0.99999 \nonumber\\
self-esteem & 0.99999 \nonumber\\
to_realize & 0.99999 \nonumber\\
self-esteem_lead & 0.99999 \nonumber\\
productive_in & 0.99999 \nonumber\\
productive & 0.99999 \nonumber\\
the_self-esteem & 0.99999 \nonumber\\
will_strengthen & 0.99999 \nonumber\\
real_pe & 0.99999 \nonumber\\
realize_on & 0.99999 \nonumber\\
because_real & 0.99999 \nonumber\\
their_society & 0.99999 \nonumber\\
eg & 0.99999 \nonumber\\
hurt & 0.99999 \nonumber\\
argument_of & 0.99999 \nonumber\\
realistic & 0.99999 \nonumber\\
to_it & 0.99999 \nonumber\\
and_student & 0.99999 \nonumber\\
,_atheism & 0.99999 \nonumber\\
ban_. & 0.99999 \nonumber\\
bible_etc. & 0.99999 \nonumber\\
its_time & 0.99999 \nonumber\\
be_see & 0.99999 \nonumber\\
offspring & 0.99999 \nonumber\\
see_to & 0.99999 \nonumber\\
bear_no & 0.99999 \nonumber\\
no_offspring & 0.99999 \nonumber\\
to_weaken & 0.99999 \nonumber\\
be_ban & 0.99999 \nonumber\\
change_... & 0.99999 \nonumber\\
relationship_bear & 0.99999 \nonumber\\
offspring_which & 0.99999 \nonumber\\
gay_relationship & 0.99999 \nonumber\\
the_teaching & 0.99999 \nonumber\\
weaken_the & 0.99999 \nonumber\\
accept_. & 0.99999 \nonumber\\
weaken & 0.99999 \nonumber\\
return_to & 0.99999 \nonumber\\
it_run & 0.99999 \nonumber\\
obama & 0.99999 \nonumber\\
ProductionRule_QP->JJR,IN,CD, & 0.99999 \nonumber\\
ProductionRule_NP->DT,JJ,CD, & 0.99999 \nonumber\\
and_increase & 0.99999 \nonumber\\
and_innovation & 0.99999 \nonumber\\
enthusiastic & 0.99999 \nonumber\\
skill_of & 0.99999 \nonumber\\
child_enthusiastic & 0.99999 \nonumber\\
improve_their & 0.99999 \nonumber\\
make_child & 0.99999 \nonumber\\
improve_academic & 0.99999 \nonumber\\
television_have & 0.99999 \nonumber\\
innovation_!!! & 0.99999 \nonumber\\
confident & 0.99999 \nonumber\\
enthusiastic_and & 0.99999 \nonumber\\
child_improve & 0.99999 \nonumber\\
their_idea & 0.99999 \nonumber\\
._child & 0.99999 \nonumber\\
academic_skill & 0.99999 \nonumber\\
and_confident & 0.99999 \nonumber\\
academic_and & 0.99999 \nonumber\\
confident_. & 0.99999 \nonumber\\
_pos_ngram_PUNC_V_CONJ & 0.99999 \nonumber\\
communication_. & 0.99999 \nonumber\\
to_cross & 0.99999 \nonumber\\
charector_limit & 0.99999 \nonumber\\
for_communication & 0.99999 \nonumber\\
the_charector & 0.99999 \nonumber\\
communication & 0.99999 \nonumber\\
charector & 0.99999 \nonumber\\
cross_the & 0.99999 \nonumber\\
the_bible & 0.99999 \nonumber\\
pregnancy_. & 0.99999 \nonumber\\
theyre & 0.99999 \nonumber\\
the_exact & 0.99999 \nonumber\\
be_treat & 0.99999 \nonumber\\
maybe_not & 0.99999 \nonumber\\
other_will & 0.99999 \nonumber\\
community_to & 0.99999 \nonumber\\
ProductionRule_VP->VB,NP,S,,,S, & 0.99999 \nonumber\\
it_safe & 0.99999 \nonumber\\
their_dream & 0.99999 \nonumber\\
society_to & 0.99999 \nonumber\\
to.everyone_in & 0.99999 \nonumber\\
better.to & 0.99999 \nonumber\\
of.but & 0.99999 \nonumber\\
ProductionRule_ADJP->ADJP,S,SBAR, & 0.99999 \nonumber\\
in_themself & 0.99999 \nonumber\\
and_better.to & 0.99999 \nonumber\\
safe_and & 0.99999 \nonumber\\
wealthy & 0.99999 \nonumber\\
alone_pursue & 0.99999 \nonumber\\
them_what & 0.99999 \nonumber\\
thing_way & 0.99999 \nonumber\\
better.to_teach & 0.99999 \nonumber\\
but_some & 0.99999 \nonumber\\
endeavor_be & 0.99999 \nonumber\\
pursue_their & 0.99999 \nonumber\\
wealthy_people & 0.99999 \nonumber\\
both_endeavor & 0.99999 \nonumber\\
world_know & 0.99999 \nonumber\\
part_of.but & 0.99999 \nonumber\\
become_unpetty & 0.99999 \nonumber\\
thing_wealthy & 0.99999 \nonumber\\
individual_i & 0.99999 \nonumber\\
to.everyone & 0.99999 \nonumber\\
this_society & 0.99999 \nonumber\\
dream_without & 0.99999 \nonumber\\
ProductionRule_NP->NN,NN,CD, & 0.99999 \nonumber\\
to_beleive & 0.99999 \nonumber\\
use_to.everyone & 0.99999 \nonumber\\
themself_that & 0.99999 \nonumber\\
of.but_i & 0.99999 \nonumber\\
themself & 0.99999 \nonumber\\
they_use & 0.99999 \nonumber\\
unpetty & 0.99999 \nonumber\\
i_as & 0.99999 \nonumber\\
unpetty_with & 0.99999 \nonumber\\
own_pocket & 0.99999 \nonumber\\
another_thing & 0.99999 \nonumber\\
significant_result & 0.99999 \nonumber\\
be_bottle & 0.99999 \nonumber\\
guideline_. & 0.99999 \nonumber\\
pediatrician_and & 0.99999 \nonumber\\
pediatrician & 0.99999 \nonumber\\
highest_support & 0.99999 \nonumber\\
58_% & 0.99999 \nonumber\\
inception_there & 0.99999 \nonumber\\
illustrate_the & 0.99999 \nonumber\\
(_http://www.nikawater.org/bottled-water/ & 0.99999 \nonumber\\
a_survey & 0.99999 \nonumber\\
of_national & 0.99999 \nonumber\\
._further & 0.99999 \nonumber\\
contain_in & 0.99999 \nonumber\\
by_beverage & 0.99999 \nonumber\\
program_and & 0.99999 \nonumber\\
thus_far & 0.99999 \nonumber\\
the_program & 0.99999 \nonumber\\
58 & 0.99999 \nonumber\\
article_illustrate & 0.99999 \nonumber\\
illustrate & 0.99999 \nonumber\\
association_work & 0.99999 \nonumber\\
school_beverage & 0.99999 \nonumber\\
a_healthier & 0.99999 \nonumber\\
a_set & 0.99999 \nonumber\\
each_group & 0.99999 \nonumber\\
all_beverage & 0.99999 \nonumber\\
and_significant & 0.99999 \nonumber\\
school_by & 0.99999 \nonumber\\
develop_a & 0.99999 \nonumber\\
promote_healthier & 0.99999 \nonumber\\
to_reduce & 0.99999 \nonumber\\
the_alliance & 0.99999 \nonumber\\
generation_and & 0.99999 \nonumber\\
the_article & 0.99999 \nonumber\\
calorie & 0.99999 \nonumber\\
calorie_deliver & 0.99999 \nonumber\\
american_beverage & 0.99999 \nonumber\\
group_be & 0.99999 \nonumber\\
calorie_contain & 0.99999 \nonumber\\
physician & 0.99999 \nonumber\\
school_choice & 0.99999 \nonumber\\
physician_. & 0.99999 \nonumber\\
deliver_to & 0.99999 \nonumber\\
deliver & 0.99999 \nonumber\\
national_school & 0.99999 \nonumber\\
inception & 0.99999 \nonumber\\
beverage_company & 0.99999 \nonumber\\
its_inception & 0.99999 \nonumber\\
beverage_ship & 0.99999 \nonumber\\
since_its & 0.99999 \nonumber\\
beverage_guideline & 0.99999 \nonumber\\
cut_in & 0.99999 \nonumber\\
company_and & 0.99999 \nonumber\\
healthier_generation & 0.99999 \nonumber\\
beverage_association & 0.99999 \nonumber\\
alliance & 0.99999 \nonumber\\
alliance_for & 0.99999 \nonumber\\
,_pediatrician & 0.99999 \nonumber\\
the_calorie & 0.99999 \nonumber\\
%_cut & 0.99999 \nonumber\\
take_of & 0.99999 \nonumber\\
http://www.nikawater.org/bottled-water/_) & 0.99999 \nonumber\\
ship_to & 0.99999 \nonumber\\
http://www.nikawater.org/bottled-water/ & 0.99999 \nonumber\\
and_family & 0.99999 \nonumber\\
family_physician & 0.99999 \nonumber\\
article & 0.99999 \nonumber\\
survey_be & 0.99999 \nonumber\\
the_highest & 0.99999 \nonumber\\
a_58 & 0.99999 \nonumber\\
healthier_school & 0.99999 \nonumber\\
total_calorie & 0.99999 \nonumber\\
"_( & 0.99999 \nonumber\\
result_thus & 0.99999 \nonumber\\
prepare_to & 0.99999 \nonumber\\
support_choice & 0.99999 \nonumber\\
return_promote & 0.99999 \nonumber\\
_pos_ngram_ADV_ART_PP & 0.99999 \nonumber\\
not_murder & 0.99999 \nonumber\\
(_homosapien & 0.99999 \nonumber\\
homosapien_) & 0.99999 \nonumber\\
have_both & 0.99999 \nonumber\\
homosapien & 0.99999 \nonumber\\
follow_criterion & 0.99999 \nonumber\\
(_imo & 0.99999 \nonumber\\
,_abortion & 0.99999 \nonumber\\
criterion_( & 0.99999 \nonumber\\
criterion & 0.99999 \nonumber\\
this_criterium & 0.99999 \nonumber\\
criterium & 0.99999 \nonumber\\
to_contribute & 0.99999 \nonumber\\
imo & 0.99999 \nonumber\\
criterium_, & 0.99999 \nonumber\\
human_( & 0.99999 \nonumber\\
fetus_can & 0.99999 \nonumber\\
imo_) & 0.99999 \nonumber\\
ok_because & 0.99999 \nonumber\\
can_put & 0.99999 \nonumber\\
be_prepare & 0.99999 \nonumber\\
n't_concern & 0.99999 \nonumber\\
say_fatherless & 0.99999 \nonumber\\
because_both & 0.99999 \nonumber\\
same_to & 0.99999 \nonumber\\
much_as & 0.99999 \nonumber\\
figure_or & 0.99999 \nonumber\\
easy_question & 0.99999 \nonumber\\
ProductionRule_VP->VBZ,RB,NP,S, & 0.99999 \nonumber\\
no_man & 0.99999 \nonumber\\
somebody_that & 0.99999 \nonumber\\
model_. & 0.99999 \nonumber\\
question_to & 0.99999 \nonumber\\
a_male & 0.99999 \nonumber\\
answer_because & 0.99999 \nonumber\\
an_easy & 0.99999 \nonumber\\
find_another & 0.99999 \nonumber\\
man_in & 0.99999 \nonumber\\
alway_find & 0.99999 \nonumber\\
another_father & 0.99999 \nonumber\\
ton & 0.99999 \nonumber\\
ton_of & 0.99999 \nonumber\\
and_still & 0.99999 \nonumber\\
bid_, & 0.99999 \nonumber\\
young & 0.99999 \nonumber\\
other_be & 0.99999 \nonumber\\
some_plan & 0.99999 \nonumber\\
marriage_" & 0.99999 \nonumber\\
with_his & 0.99999 \nonumber\\
would_say & 0.99999 \nonumber\\
she_trust & 0.99999 \nonumber\\
physical_activity & 0.99999 \nonumber\\
career & 0.99999 \nonumber\\
it_much & 0.99999 \nonumber\\
be_different & 0.99999 \nonumber\\
or_even & 0.99999 \nonumber\\
singapore_would & 0.99999 \nonumber\\
_pos_ngram_ADV_CARD_O & 0.99999 \nonumber\\
your_child & 0.99999 \nonumber\\
_pos_ngram_O_NP_NP & 0.99999 \nonumber\\
know_your & 0.99999 \nonumber\\
it_never & 0.99999 \nonumber\\
not_they & 0.99999 \nonumber\\
how_about & 0.99999 \nonumber\\
thick & 0.99999 \nonumber\\
some_would & 0.99999 \nonumber\\
important_for & 0.99999 \nonumber\\
live_and & 0.99999 \nonumber\\
ProductionRule_NP->NP,:,SQ, & 0.99999 \nonumber\\
question_for & 0.99999 \nonumber\\
ProductionRule_NP->NNP,,, & 0.99999 \nonumber\\
stomach_live & 0.99999 \nonumber\\
ProductionRule_UCP->S,CC,SBAR, & 0.99999 \nonumber\\
,_here & 0.99999 \nonumber\\
stomach & 0.99999 \nonumber\\
pro-choice_: & 0.99999 \nonumber\\
ProductionRule_VP->VBP,UCP, & 0.99999 \nonumber\\
ProductionRule_NP->NP,NN,NN, & 0.99999 \nonumber\\
'_stomach & 0.99999 \nonumber\\
:_be & 0.99999 \nonumber\\
help_her & 0.99999 \nonumber\\
pupil & 0.99999 \nonumber\\
figure_, & 0.99999 \nonumber\\
too_, & 0.99999 \nonumber\\
the_margin & 0.99999 \nonumber\\
undoubtedly & 0.99999 \nonumber\\
dutch_colonial & 0.99999 \nonumber\\
and_vision & 0.99999 \nonumber\\
to_search & 0.99999 \nonumber\\
without_raffle & 0.99999 \nonumber\\
undoubtedly_raffle & 0.99999 \nonumber\\
lead_him & 0.99999 \nonumber\\
ambition & 0.99999 \nonumber\\
have_remain & 0.99999 \nonumber\\
'_ambition & 0.99999 \nonumber\\
strategic & 0.99999 \nonumber\\
strategic_objective & 0.99999 \nonumber\\
economic_and & 0.99999 \nonumber\\
_pos_ngram_ADV_NP_O & 0.99999 \nonumber\\
and_strategic & 0.99999 \nonumber\\
colonial_empire & 0.99999 \nonumber\\
colonial & 0.99999 \nonumber\\
british_economic & 0.99999 \nonumber\\
east_indy & 0.99999 \nonumber\\
empire_in & 0.99999 \nonumber\\
ambition_and & 0.99999 \nonumber\\
ProductionRule_VP->VBD,ADVP,NP, & 0.99999 \nonumber\\
best_location & 0.99999 \nonumber\\
a_sparsely & 0.99999 \nonumber\\
inhabit_island & 0.99999 \nonumber\\
the_east & 0.99999 \nonumber\\
search_for & 0.99999 \nonumber\\
sparsely & 0.99999 \nonumber\\
margin_of & 0.99999 \nonumber\\
inhabit & 0.99999 \nonumber\\
malacca_, & 0.99999 \nonumber\\
be_undoubtedly & 0.99999 \nonumber\\
achieve_british & 0.99999 \nonumber\\
,_on & 0.99999 \nonumber\\
region_. & 0.99999 \nonumber\\
sparsely_inhabit & 0.99999 \nonumber\\
margin & 0.99999 \nonumber\\
remain_a & 0.99999 \nonumber\\
ProductionRule_NP->NP,NN,CC,NN, & 0.99999 \nonumber\\
base_in & 0.99999 \nonumber\\
objective & 0.99999 \nonumber\\
location_to & 0.99999 \nonumber\\
ProductionRule_NP->JJ,JJ,CC,JJ,NNS, & 0.99999 \nonumber\\
indy_. & 0.99999 \nonumber\\
indy & 0.99999 \nonumber\\
vision_which & 0.99999 \nonumber\\
objective_in & 0.99999 \nonumber\\
reason_i & 0.99999 \nonumber\\
n't_wrong & 0.99999 \nonumber\\
may_start & 0.99999 \nonumber\\
good_but & 0.99999 \nonumber\\
own_need & 0.99999 \nonumber\\
even_want & 0.99999 \nonumber\\
to_forget & 0.99999 \nonumber\\
balance_of & 0.99999 \nonumber\\
alway_put & 0.99999 \nonumber\\
before_yourself & 0.99999 \nonumber\\
want_in & 0.99999 \nonumber\\
to_want & 0.99999 \nonumber\\
whose & 0.99999 \nonumber\\
security_council & 0.99999 \nonumber\\
partical & 0.99999 \nonumber\\
sixty_year & 0.99999 \nonumber\\
council_of & 0.99999 \nonumber\\
council & 0.99999 \nonumber\\
sixty & 0.99999 \nonumber\\
fear_alexander & 0.99999 \nonumber\\
matter_come & 0.99999 \nonumber\\
by_whose & 0.99999 \nonumber\\
of_security & 0.99999 \nonumber\\
partical_then & 0.99999 \nonumber\\
afraid_it & 0.99999 \nonumber\\
un_and & 0.99999 \nonumber\\
sixth_member & 0.99999 \nonumber\\
sixth & 0.99999 \nonumber\\
development_rate & 0.99999 \nonumber\\
contribution_of & 0.99999 \nonumber\\
just_sixty & 0.99999 \nonumber\\
remember_the & 0.99999 \nonumber\\
the_pottential & 0.99999 \nonumber\\
after_just & 0.99999 \nonumber\\
ProductionRule_VP->VBN,PP,S, & 0.99999 \nonumber\\
the_sixth & 0.99999 \nonumber\\
then_from & 0.99999 \nonumber\\
country_by & 0.99999 \nonumber\\
the_discovery & 0.99999 \nonumber\\
whose_fear & 0.99999 \nonumber\\
indium_after & 0.99999 \nonumber\\
independence_indium & 0.99999 \nonumber\\
ProductionRule_NP->RB,CD,NNS, & 0.99999 \nonumber\\
be_unknown & 0.99999 \nonumber\\
ProductionRule_WHNP->WP$,NP, & 0.99999 \nonumber\\
be_indium & 0.99999 \nonumber\\
ProductionRule_ADJP->JJ,ADVP,PP,PP, & 0.99999 \nonumber\\
of_un & 0.99999 \nonumber\\
god_partical & 0.99999 \nonumber\\
great_contribution & 0.99999 \nonumber\\
great_development & 0.99999 \nonumber\\
member_of & 0.99999 \nonumber\\
alexander & 0.99999 \nonumber\\
rate_and & 0.99999 \nonumber\\
army_be & 0.99999 \nonumber\\
'_army & 0.99999 \nonumber\\
look_as & 0.99999 \nonumber\\
unknown_to & 0.99999 \nonumber\\
only_country & 0.99999 \nonumber\\
the_great & 0.99999 \nonumber\\
unknown & 0.99999 \nonumber\\
that_none & 0.99999 \nonumber\\
alexander_' & 0.99999 \nonumber\\
?! & 0.99999 \nonumber\\
pill & 0.99999 \nonumber\\
pill_, & 0.99999 \nonumber\\
more_of & 0.99999 \nonumber\\
ProductionRule_VP->VBZ,:,SBARQ, & 0.99999 \nonumber\\
_pos_ngram_CONJ_PUNC_NN & 0.99999 \nonumber\\
thought_. & 0.99999 \nonumber\\
and_study & 0.99999 \nonumber\\
http://www.dinosauria.com/jdp/evol/lizard.html & 0.99999 \nonumber\\
document_, & 0.99999 \nonumber\\
document & 0.99999 \nonumber\\
http://www.dinosauria.com/jdp/evol/lizard.html_and & 0.99999 \nonumber\\
._thanks & 0.99999 \nonumber\\
i_invite & 0.99999 \nonumber\\
:_http://www.dinosauria.com/jdp/evol/lizard.html & 0.99999 \nonumber\\
occur_and & 0.99999 \nonumber\\
you_your & 0.99999 \nonumber\\
invite_you & 0.99999 \nonumber\\
ProductionRule_VP->VBN,,,CC,VBN, & 0.99999 \nonumber\\
be_document & 0.99999 \nonumber\\
by_not & 0.99999 \nonumber\\
atmosphere & 0.99999 \nonumber\\
lousy_because & 0.99999 \nonumber\\
child_life & 0.99999 \nonumber\\
,_well & 0.99999 \nonumber\\
_pos_ngram_O_CONJ_PR & 0.99999 \nonumber\\
them_a & 0.99999 \nonumber\\
have_it & 0.99999 \nonumber\\
3rd & 0.99999 \nonumber\\
a_selfish & 0.99999 \nonumber\\
the_brain & 0.99999 \nonumber\\
their_pants & 0.99999 \nonumber\\
everyone_equal & 0.99999 \nonumber\\
look_school & 0.99999 \nonumber\\
hr & 0.99999 \nonumber\\
level_it & 0.99999 \nonumber\\
take_less & 0.99999 \nonumber\\
find_their & 0.99999 \nonumber\\
hr_just & 0.99999 \nonumber\\
tease_and & 0.99999 \nonumber\\
._okay & 0.99999 \nonumber\\
about_1 & 0.99999 \nonumber\\
peer_around & 0.99999 \nonumber\\
uniform_take & 0.99999 \nonumber\\
can_wear & 0.99999 \nonumber\\
uniform_2 & 0.99999 \nonumber\\
or_shirt & 0.99999 \nonumber\\
like_about & 0.99999 \nonumber\\
feel_less & 0.99999 \nonumber\\
??_when & 0.99999 \nonumber\\
want_some & 0.99999 \nonumber\\
mean_really & 0.99999 \nonumber\\
pants_or & 0.99999 \nonumber\\
v._uniform & 0.99999 \nonumber\\
less_equal & 0.99999 \nonumber\\
but_maybe & 0.99999 \nonumber\\
10_min & 0.99999 \nonumber\\
equal_- & 0.99999 \nonumber\\
dress_but & 0.99999 \nonumber\\
take_like & 0.99999 \nonumber\\
if_child & 0.99999 \nonumber\\
equal_to & 0.99999 \nonumber\\
them_v. & 0.99999 \nonumber\\
okay_look & 0.99999 \nonumber\\
min & 0.99999 \nonumber\\
matter_and & 0.99999 \nonumber\\
some_level & 0.99999 \nonumber\\
will_tease & 0.99999 \nonumber\\
and_dress & 0.99999 \nonumber\\
shirt_i & 0.99999 \nonumber\\
1_hr & 0.99999 \nonumber\\
have_uniform & 0.99999 \nonumber\\
really_?? & 0.99999 \nonumber\\
min_just & 0.99999 \nonumber\\
uniform_it & 0.99999 \nonumber\\
these_argument & 0.99999 \nonumber\\
'_so & 1.00000 \nonumber\\
will_teach & 1.00000 \nonumber\\
ground_them & 1.00000 \nonumber\\
will_work & 1.00000 \nonumber\\
child_respond & 1.00000 \nonumber\\
respond_differently & 1.00000 \nonumber\\
while_one & 1.00000 \nonumber\\
use_if & 1.00000 \nonumber\\
run_but & 1.00000 \nonumber\\
punishment_while & 1.00000 \nonumber\\
_pos_ngram_PR_ART_CONJ & 1.00000 \nonumber\\
but_each & 1.00000 \nonumber\\
them_will & 1.00000 \nonumber\\
thee & 1.00000 \nonumber\\
ground & 1.00000 \nonumber\\
teach_thee & 1.00000 \nonumber\\
differently_to & 1.00000 \nonumber\\
differently & 1.00000 \nonumber\\
thee_child & 1.00000 \nonumber\\
may_take & 1.00000 \nonumber\\
ProductionRule_VP->VB,NP,NP,PP, & 1.00000 \nonumber\\
one_child & 1.00000 \nonumber\\
just_tell & 1.00000 \nonumber\\
or_ground & 1.00000 \nonumber\\
another_child & 1.00000 \nonumber\\
ProductionRule_VP->ADVP,VP,CC,VP, & 1.00000 \nonumber\\
no_or & 1.00000 \nonumber\\
and_raffle & 1.00000 \nonumber\\
other_' & 1.00000 \nonumber\\
i_check & 1.00000 \nonumber\\
a_hard & 1.00000 \nonumber\\
alway_a & 1.00000 \nonumber\\
they_also & 1.00000 \nonumber\\
(_and & 1.00000 \nonumber\\
behind & 1.00000 \nonumber\\
whether_they & 1.00000 \nonumber\\
economically & 1.00000 \nonumber\\
sad_because & 1.00000 \nonumber\\
be_water & 1.00000 \nonumber\\
like_. & 1.00000 \nonumber\\
be_unjustly & 1.00000 \nonumber\\
unjustly & 1.00000 \nonumber\\
understand_what & 1.00000 \nonumber\\
day_he & 1.00000 \nonumber\\
to_finish & 1.00000 \nonumber\\
personal_belief & 1.00000 \nonumber\\
down_with & 1.00000 \nonumber\\
likley_i & 1.00000 \nonumber\\
though_if & 1.00000 \nonumber\\
you_promise & 1.00000 \nonumber\\
wrong_though & 1.00000 \nonumber\\
through_worse & 1.00000 \nonumber\\
leave_them & 1.00000 \nonumber\\
ProductionRule_UCP->PP,CC,ADVP,ADJP, & 1.00000 \nonumber\\
for_eachother & 1.00000 \nonumber\\
would_anything & 1.00000 \nonumber\\
her_but & 1.00000 \nonumber\\
ProductionRule_S->S,CC,S,CC,,,S,., & 1.00000 \nonumber\\
catch_i & 1.00000 \nonumber\\
_pos_ngram_PR_CONJ_PUNC & 1.00000 \nonumber\\
go_down & 1.00000 \nonumber\\
ProductionRule_VP->VB,PRT,PP,PP, & 1.00000 \nonumber\\
marry_you & 1.00000 \nonumber\\
eachother & 1.00000 \nonumber\\
for_anything & 1.00000 \nonumber\\
eachother_through & 1.00000 \nonumber\\
or_through & 1.00000 \nonumber\\
ProductionRule_NP->JJS,NN, & 1.00000 \nonumber\\
ProductionRule_VP->VB,ADVP,UCP, & 1.00000 \nonumber\\
through_good & 1.00000 \nonumber\\
spouse_because & 1.00000 \nonumber\\
worse_and & 1.00000 \nonumber\\
family_to & 1.00000 \nonumber\\
of_and & 1.00000 \nonumber\\
bottle_. & 1.00000 \nonumber\\
of_sexual & 1.00000 \nonumber\\
a_relationship & 1.00000 \nonumber\\
split & 1.00000 \nonumber\\
about_how & 1.00000 \nonumber\\
many_exclamation & 1.00000 \nonumber\\
that_clearly & 1.00000 \nonumber\\
exclamation_mark & 1.00000 \nonumber\\
who_just & 1.00000 \nonumber\\
rot_the & 1.00000 \nonumber\\
in_capital & 1.00000 \nonumber\\
say_tv & 1.00000 \nonumber\\
mark & 1.00000 \nonumber\\
capital & 1.00000 \nonumber\\
awesome_with & 1.00000 \nonumber\\
have_terrible & 1.00000 \nonumber\\
rot & 1.00000 \nonumber\\
you_notice & 1.00000 \nonumber\\
mark_and & 1.00000 \nonumber\\
exclamation & 1.00000 \nonumber\\
capital_. & 1.00000 \nonumber\\
clearly_prove & 1.00000 \nonumber\\
against_book & 1.00000 \nonumber\\
terrible_argument & 1.00000 \nonumber\\
tv_rot & 1.00000 \nonumber\\
that_those & 1.00000 \nonumber\\
girl_it & 1.00000 \nonumber\\
you_problem & 1.00000 \nonumber\\
ProductionRule_NP->NP,ADJP,SBAR, & 1.00000 \nonumber\\
maybe_its & 1.00000 \nonumber\\
bring_you & 1.00000 \nonumber\\
sound_bid & 1.00000 \nonumber\\
less_it & 1.00000 \nonumber\\
same_if & 1.00000 \nonumber\\
would_love & 1.00000 \nonumber\\
bid_father & 1.00000 \nonumber\\
dad_but & 1.00000 \nonumber\\
might_sound & 1.00000 \nonumber\\
love_my & 1.00000 \nonumber\\
be_father & 1.00000 \nonumber\\
keep_bring & 1.00000 \nonumber\\
father_less & 1.00000 \nonumber\\
be_girl & 1.00000 \nonumber\\
it_i & 1.00000 \nonumber\\
'_alway & 1.00000 \nonumber\\
street & 1.00000 \nonumber\\
money_as & 1.00000 \nonumber\\
kill_one & 1.00000 \nonumber\\
them_the & 1.00000 \nonumber\\
person_what & 1.00000 \nonumber\\
what_say & 1.00000 \nonumber\\
tell_what & 1.00000 \nonumber\\
wrong_for & 1.00000 \nonumber\\
peace_that & 1.00000 \nonumber\\
not_kill & 1.00000 \nonumber\\
any_reason & 1.00000 \nonumber\\
the_peace & 1.00000 \nonumber\\
worth_the & 1.00000 \nonumber\\
in_becasue & 1.00000 \nonumber\\
._ie & 1.00000 \nonumber\\
smart & 1.00000 \nonumber\\
a_family & 1.00000 \nonumber\\
yea_, & 1.00000 \nonumber\\
only_way & 1.00000 \nonumber\\
evil & 1.00000 \nonumber\\
,_go & 1.00000 \nonumber\\
ceremony & 1.00000 \nonumber\\
ProductionRule_VP->VB,NP,ADVP,PP, & 1.00000 \nonumber\\
tell_me & 1.00000 \nonumber\\
pick_have & 1.00000 \nonumber\\
him_no & 1.00000 \nonumber\\
help_but & 1.00000 \nonumber\\
need_his & 1.00000 \nonumber\\
his_help & 1.00000 \nonumber\\
time_where & 1.00000 \nonumber\\
all_because & 1.00000 \nonumber\\
dumbest & 1.00000 \nonumber\\
again_there & 1.00000 \nonumber\\
mad_, & 1.00000 \nonumber\\
the_dumbest & 1.00000 \nonumber\\
dumbest_thing & 1.00000 \nonumber\\
be_time & 1.00000 \nonumber\\
laugh & 1.00000 \nonumber\\
laugh_. & 1.00000 \nonumber\\
to_pick & 1.00000 \nonumber\\
me_laugh & 1.00000 \nonumber\\
ProductionRule_NP->NP,ADVP,NP, & 1.00000 \nonumber\\
still_love & 1.00000 \nonumber\\
secure & 1.00000 \nonumber\\
window & 1.00000 \nonumber\\
come_around & 1.00000 \nonumber\\
of_bottle & 1.00000 \nonumber\\
about_crime & 1.00000 \nonumber\\
commit_these & 1.00000 \nonumber\\
will_in & 1.00000 \nonumber\\
disrespect_and & 1.00000 \nonumber\\
affect_how & 1.00000 \nonumber\\
woman_which & 1.00000 \nonumber\\
that_woman & 1.00000 \nonumber\\
how_woman & 1.00000 \nonumber\\
sense_that & 1.00000 \nonumber\\
treat_in & 1.00000 \nonumber\\
these_grave & 1.00000 \nonumber\\
how_man & 1.00000 \nonumber\\
this_not & 1.00000 \nonumber\\
woman_empowerment & 1.00000 \nonumber\\
perceive_woman & 1.00000 \nonumber\\
common_: & 1.00000 \nonumber\\
,_rape & 1.00000 \nonumber\\
society_today & 1.00000 \nonumber\\
disrespect & 1.00000 \nonumber\\
degrade_morality & 1.00000 \nonumber\\
as_sex & 1.00000 \nonumber\\
and_false & 1.00000 \nonumber\\
ProductionRule_VP->VBN,PP,NP, & 1.00000 \nonumber\\
sex_toy & 1.00000 \nonumber\\
view_merely & 1.00000 \nonumber\\
and_sexual & 1.00000 \nonumber\\
also_affect & 1.00000 \nonumber\\
?_murder & 1.00000 \nonumber\\
empowerment_in & 1.00000 \nonumber\\
in_common & 1.00000 \nonumber\\
sexual_abuse & 1.00000 \nonumber\\
empowerment & 1.00000 \nonumber\\
crime_all & 1.00000 \nonumber\\
of_disrespect & 1.00000 \nonumber\\
grave_crime & 1.00000 \nonumber\\
false_perception & 1.00000 \nonumber\\
crime_rate & 1.00000 \nonumber\\
be_view & 1.00000 \nonumber\\
turn_lead & 1.00000 \nonumber\\
which_at & 1.00000 \nonumber\\
day_affect & 1.00000 \nonumber\\
merely_as & 1.00000 \nonumber\\
man_perceive & 1.00000 \nonumber\\
n't_just & 1.00000 \nonumber\\
already_know & 1.00000 \nonumber\\
you_already & 1.00000 \nonumber\\
n't_they & 1.00000 \nonumber\\
,_man & 1.00000 \nonumber\\
pregnant_, & 1.00000 \nonumber\\
man_who & 1.00000 \nonumber\\
ironic & 1.00000 \nonumber\\
pe_class & 1.00000 \nonumber\\
sometime_in & 1.00000 \nonumber\\
who_they & 1.00000 \nonumber\\
begin & 1.00000 \nonumber\\
ProductionRule_VP->VBP,ADJP,PP, & 1.00000 \nonumber\\
as & 1.00000 \nonumber\\
it_wrong & 1.00000 \nonumber\\
and_society & 1.00000 \nonumber\\
the_wear & 1.00000 \nonumber\\
unity_and & 1.00000 \nonumber\\
equal_( & 1.00000 \nonumber\\
_pos_ngram_O_PP_ADJ & 1.00000 \nonumber\\
remind_each & 1.00000 \nonumber\\
wear_of & 1.00000 \nonumber\\
(_at & 1.00000 \nonumber\\
be_encourage & 1.00000 \nonumber\\
child_feel & 1.00000 \nonumber\\
school_) & 1.00000 \nonumber\\
ProductionRule_VP->VBP,ADJP,PRN, & 1.00000 \nonumber\\
show_unity & 1.00000 \nonumber\\
it_remind & 1.00000 \nonumber\\
team_. & 1.00000 \nonumber\\
uniform_should & 1.00000 \nonumber\\
include_and & 1.00000 \nonumber\\
encourage_because & 1.00000 \nonumber\\
also_show & 1.00000 \nonumber\\
feel_include & 1.00000 \nonumber\\
impact & 1.00000 \nonumber\\
for_indium & 1.00000 \nonumber\\
tell & 1.00000 \nonumber\\
ProductionRule_NP->NP,,,CC,NP, & 1.00000 \nonumber\\
level & 1.00000 \nonumber\\
_pos_ngram_ADV_ADV_NP & 1.00000 \nonumber\\
only_reason & 1.00000 \nonumber\\
better_! & 1.00000 \nonumber\\
,_tv & 1.00000 \nonumber\\
weirdo & 1.00000 \nonumber\\
cool_! & 1.00000 \nonumber\\
weirdo_, & 1.00000 \nonumber\\
rofl & 1.00000 \nonumber\\
op_be & 1.00000 \nonumber\\
rofl_! & 1.00000 \nonumber\\
ProductionRule_VP->NN,PP, & 1.00000 \nonumber\\
like_cool & 1.00000 \nonumber\\
for_weirdo & 1.00000 \nonumber\\
ProductionRule_PP->IN,NN, & 1.00000 \nonumber\\
r_like & 1.00000 \nonumber\\
op & 1.00000 \nonumber\\
!_tv & 1.00000 \nonumber\\
black_op & 1.00000 \nonumber\\
!_book & 1.00000 \nonumber\\
think_black & 1.00000 \nonumber\\
for_nerd & 1.00000 \nonumber\\
!_rofl & 1.00000 \nonumber\\
nerd_, & 1.00000 \nonumber\\
on_there & 1.00000 \nonumber\\
so_fat & 1.00000 \nonumber\\
fat_stop & 1.00000 \nonumber\\
not_fat & 1.00000 \nonumber\\
fuck_exercise & 1.00000 \nonumber\\
football_or & 1.00000 \nonumber\\
out_asshole & 1.00000 \nonumber\\
there_ass & 1.00000 \nonumber\\
peace_out & 1.00000 \nonumber\\
video_game & 1.00000 \nonumber\\
and_these & 1.00000 \nonumber\\
ProductionRule_VP->VBP,ADVP,S, & 1.00000 \nonumber\\
your_energy & 1.00000 \nonumber\\
fat_people & 1.00000 \nonumber\\
"_peace & 1.00000 \nonumber\\
there_fuck & 1.00000 \nonumber\\
and_go & 1.00000 \nonumber\\
stop_play & 1.00000 \nonumber\\
day_play & 1.00000 \nonumber\\
energy_back & 1.00000 \nonumber\\
out_side & 1.00000 \nonumber\\
play_video & 1.00000 \nonumber\\
fuck & 1.00000 \nonumber\\
play_football & 1.00000 \nonumber\\
game_and & 1.00000 \nonumber\\
ass_all & 1.00000 \nonumber\\
be_constantly & 1.00000 \nonumber\\
and_those & 1.00000 \nonumber\\
be_clear & 1.00000 \nonumber\\
redefine & 1.00000 \nonumber\\
the_street & 1.00000 \nonumber\\
create_the & 1.00000 \nonumber\\
obese_kid & 1.00000 \nonumber\\
._should & 1.00000 \nonumber\\
finish & 1.00000 \nonumber\\
great_boyfriend & 1.00000 \nonumber\\
be_annoy & 1.00000 \nonumber\\
once_or & 1.00000 \nonumber\\
thing_up & 1.00000 \nonumber\\
)_time & 1.00000 \nonumber\\
_pos_ngram_O_ADV_CARD & 1.00000 \nonumber\\
separate_fantasy & 1.00000 \nonumber\\
addiction_, & 1.00000 \nonumber\\
porn_hardly & 1.00000 \nonumber\\
addiction_be & 1.00000 \nonumber\\
(_sometime & 1.00000 \nonumber\\
porn_once & 1.00000 \nonumber\\
issue_or & 1.00000 \nonumber\\
from_reality & 1.00000 \nonumber\\
annoy_me & 1.00000 \nonumber\\
or_find & 1.00000 \nonumber\\
-_-_. & 1.00000 \nonumber\\
health_issue & 1.00000 \nonumber\\
-_- & 1.00000 \nonumber\\
porn_to & 1.00000 \nonumber\\
not_idiot & 1.00000 \nonumber\\
spice_thing & 1.00000 \nonumber\\
desire_that & 1.00000 \nonumber\\
own_but & 1.00000 \nonumber\\
idiot_, & 1.00000 \nonumber\\
or_attachment & 1.00000 \nonumber\\
bedroom_but & 1.00000 \nonumber\\
spice & 1.00000 \nonumber\\
meet_! & 1.00000 \nonumber\\
in_weak & 1.00000 \nonumber\\
porn_lead & 1.00000 \nonumber\\
maybe_who & 1.00000 \nonumber\\
me_now & 1.00000 \nonumber\\
sex_once & 1.00000 \nonumber\\
now_-_- & 1.00000 \nonumber\\
lucky_! & 1.00000 \nonumber\\
to_spice & 1.00000 \nonumber\\
weak_people & 1.00000 \nonumber\\
it_hard & 1.00000 \nonumber\\
or_twice & 1.00000 \nonumber\\
boyfriend_and & 1.00000 \nonumber\\
to_separate & 1.00000 \nonumber\\
have_desire & 1.00000 \nonumber\\
hardly_ever & 1.00000 \nonumber\\
have_mental & 1.00000 \nonumber\\
all_fantasy & 1.00000 \nonumber\\
fantasy_, & 1.00000 \nonumber\\
fantasy & 1.00000 \nonumber\\
twice_( & 1.00000 \nonumber\\
_pos_ngram_PR_ADV_CARD & 1.00000 \nonumber\\
ProductionRule_SBAR->TO,S, & 1.00000 \nonumber\\
be_meet & 1.00000 \nonumber\\
use_porn & 1.00000 \nonumber\\
argument_about & 1.00000 \nonumber\\
fantasy_from & 1.00000 \nonumber\\
twice_a & 1.00000 \nonumber\\
sometime_three & 1.00000 \nonumber\\
attachment & 1.00000 \nonumber\\
attachment_issue & 1.00000 \nonumber\\
ProductionRule_NP->DT,DT,NNS, & 1.00000 \nonumber\\
to_addiction & 1.00000 \nonumber\\
mental_health & 1.00000 \nonumber\\
_pos_ngram_ADV_NP_NN & 1.00000 \nonumber\\
we_love & 1.00000 \nonumber\\
._here & 1.00000 \nonumber\\
change_, & 1.00000 \nonumber\\
him_to & 1.00000 \nonumber\\
all_! & 1.00000 \nonumber\\
this_country & 1.00000 \nonumber\\
go_cry & 1.00000 \nonumber\\
cry & 1.00000 \nonumber\\
evolve_since & 1.00000 \nonumber\\
would_all & 1.00000 \nonumber\\
_pos_ngram_ADV_O_ADV & 1.00000 \nonumber\\
city_to & 1.00000 \nonumber\\
of_turn & 1.00000 \nonumber\\
normal_that & 1.00000 \nonumber\\
a_subordinate & 1.00000 \nonumber\\
a_successful & 1.00000 \nonumber\\
successful_city & 1.00000 \nonumber\\
leave_the & 1.00000 \nonumber\\
to_handle & 1.00000 \nonumber\\
turn_singapore & 1.00000 \nonumber\\
he_duty & 1.00000 \nonumber\\
handle_. & 1.00000 \nonumber\\
handle & 1.00000 \nonumber\\
subordinate_for & 1.00000 \nonumber\\
duty_of & 1.00000 \nonumber\\
give_he & 1.00000 \nonumber\\
raffle_found & 1.00000 \nonumber\\
raffle_give & 1.00000 \nonumber\\
city_and & 1.00000 \nonumber\\
sink & 1.00000 \nonumber\\
his_position & 1.00000 \nonumber\\
too_close & 1.00000 \nonumber\\
ProductionRule_NP->NP,,,NP,,,NP,CC,NP, & 1.00000 \nonumber\\
be_child & 1.00000 \nonumber\\
from_where & 1.00000 \nonumber\\
would_ever & 1.00000 \nonumber\\
farquhar_so & 1.00000 \nonumber\\
basis_for & 1.00000 \nonumber\\
be_summon & 1.00000 \nonumber\\
found_of & 1.00000 \nonumber\\
much_contribution & 1.00000 \nonumber\\
bencoolen_by & 1.00000 \nonumber\\
found_but & 1.00000 \nonumber\\
the_basis & 1.00000 \nonumber\\
have_much & 1.00000 \nonumber\\
believe_he & 1.00000 \nonumber\\
_pos_ngram_NP_ADV_O & 1.00000 \nonumber\\
'_idea & 1.00000 \nonumber\\
that_stamford & 1.00000 \nonumber\\
the_found & 1.00000 \nonumber\\
by_his & 1.00000 \nonumber\\
clear_that & 1.00000 \nonumber\\
summon_to & 1.00000 \nonumber\\
the_implementation & 1.00000 \nonumber\\
'_before & 1.00000 \nonumber\\
summon & 1.00000 \nonumber\\
implementation & 1.00000 \nonumber\\
idea_but & 1.00000 \nonumber\\
stamford_raffle & 1.00000 \nonumber\\
stamford & 1.00000 \nonumber\\
implementation_be & 1.00000 \nonumber\\
it_alway & 1.00000 \nonumber\\
proud_of & 1.00000 \nonumber\\
ProductionRule_NP->NP,ADJP,PP, & 1.00000 \nonumber\\
ProductionRule_ADJP->JJ,CC,NN, & 1.00000 \nonumber\\
make_somebody & 1.00000 \nonumber\\
doesnt_means & 1.00000 \nonumber\\
best_and & 1.00000 \nonumber\\
other_that & 1.00000 \nonumber\\
somebody_happy & 1.00000 \nonumber\\
and_proud & 1.00000 \nonumber\\
that_doesnt & 1.00000 \nonumber\\
of_feel & 1.00000 \nonumber\\
happy_help & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,S,,,S, & 1.00000 \nonumber\\
diffenrent_way & 1.00000 \nonumber\\
diffenrent & 1.00000 \nonumber\\
be_diffenrent & 1.00000 \nonumber\\
means_i & 1.00000 \nonumber\\
and_good & 1.00000 \nonumber\\
ProductionRule_VP->VBP,,,S, & 1.00000 \nonumber\\
i_wouldnt & 1.00000 \nonumber\\
the_real & 1.00000 \nonumber\\
day_or & 1.00000 \nonumber\\
realistic_? & 1.00000 \nonumber\\
be_process & 1.00000 \nonumber\\
outcome_which & 1.00000 \nonumber\\
happen_? & 1.00000 \nonumber\\
more_realistic & 1.00000 \nonumber\\
magically_create & 1.00000 \nonumber\\
we_magically & 1.00000 \nonumber\\
throughout_billion & 1.00000 \nonumber\\
ProductionRule_ADJP->RB,SBAR, & 1.00000 \nonumber\\
ProductionRule_SQ->VBD,NP,ADJP,., & 1.00000 \nonumber\\
an_outcome & 1.00000 \nonumber\\
process_throughout & 1.00000 \nonumber\\
raffle_, & 1.00000 \nonumber\\
knowledge_of & 1.00000 \nonumber\\
feel_, & 1.00000 \nonumber\\
fact_, & 1.00000 \nonumber\\
_pos_ngram_NN_PR_ADV & 1.00000 \nonumber\\
in_mind & 1.00000 \nonumber\\
(_in & 1.00000 \nonumber\\
_pos_ngram_ART_PP_NP & 1.00000 \nonumber\\
1819 & 1.00000 \nonumber\\
_pos_ngram_CARD_NP_CARD & 1.00000 \nonumber\\
february & 1.00000 \nonumber\\
_pos_ngram_PP_CARD_NP & 1.00000 \nonumber\\
february_1819 & 1.00000 \nonumber\\
record_history & 1.00000 \nonumber\\
his_or & 1.00000 \nonumber\\
remember_, & 1.00000 \nonumber\\
or_her & 1.00000 \nonumber\\
_pos_ngram_CONJ_PR_ART & 1.00000 \nonumber\\
concept_be & 1.00000 \nonumber\\
show_or & 1.00000 \nonumber\\
on_different & 1.00000 \nonumber\\
_pos_ngram_PP_O_ADJ & 1.00000 \nonumber\\
this_idea & 1.00000 \nonumber\\
idea_be & 1.00000 \nonumber\\
well_" & 1.00000 \nonumber\\
the_champ & 1.00000 \nonumber\\
life_die & 1.00000 \nonumber\\
let_a & 1.00000 \nonumber\\
'_body & 1.00000 \nonumber\\
body_we & 1.00000 \nonumber\\
die_for & 1.00000 \nonumber\\
_pos_ngram_NP_O_PR & 1.00000 \nonumber\\
champ_" & 1.00000 \nonumber\\
irresponsible_dont & 1.00000 \nonumber\\
a_position & 1.00000 \nonumber\\
have_you & 1.00000 \nonumber\\
under_age & 1.00000 \nonumber\\
masturbate & 1.00000 \nonumber\\
get_it & 1.00000 \nonumber\\
,_masturbate & 1.00000 \nonumber\\
'_also & 1.00000 \nonumber\\
would_film & 1.00000 \nonumber\\
freak_would & 1.00000 \nonumber\\
masturbate_or & 1.00000 \nonumber\\
so_good & 1.00000 \nonumber\\
really_sick & 1.00000 \nonumber\\
sex_?! & 1.00000 \nonumber\\
?!_i & 1.00000 \nonumber\\
those_girl & 1.00000 \nonumber\\
woman_rights & 1.00000 \nonumber\\
be_under & 1.00000 \nonumber\\
ProductionRule_NP->JJ,CC,JJ, & 1.00000 \nonumber\\
what_freak & 1.00000 \nonumber\\
good_about & 1.00000 \nonumber\\
film_people & 1.00000 \nonumber\\
entertainment_, & 1.00000 \nonumber\\
sexual_entertainment & 1.00000 \nonumber\\
want_sexual & 1.00000 \nonumber\\
also_really & 1.00000 \nonumber\\
cant_read & 1.00000 \nonumber\\
word_for & 1.00000 \nonumber\\
20 & 1.00000 \nonumber\\
we_all & 1.00000 \nonumber\\
contradict & 1.00000 \nonumber\\
will_understand & 1.00000 \nonumber\\
_pos_ngram_PP_PP_CONJ & 1.00000 \nonumber\\
muscle & 1.00000 \nonumber\\
ProductionRule_NP->NP,RRC, & 1.00000 \nonumber\\
._internet & 1.00000 \nonumber\\
but_we & 1.00000 \nonumber\\
pro-choice_be & 1.00000 \nonumber\\
past_, & 1.00000 \nonumber\\
million_of & 1.00000 \nonumber\\
trader & 1.00000 \nonumber\\
_pos_ngram_NN_ADJ_CONJ & 1.00000 \nonumber\\
hell_, & 1.00000 \nonumber\\
relatively_easier & 1.00000 \nonumber\\
internet_relatively & 1.00000 \nonumber\\
explore_. & 1.00000 \nonumber\\
internet_explore & 1.00000 \nonumber\\
plus_firefox & 1.00000 \nonumber\\
use_internet & 1.00000 \nonumber\\
search_the & 1.00000 \nonumber\\
than_use & 1.00000 \nonumber\\
make_search & 1.00000 \nonumber\\
firefox_make & 1.00000 \nonumber\\
firefox_right & 1.00000 \nonumber\\
research & 1.00000 \nonumber\\
community_service & 1.00000 \nonumber\\
service & 1.00000 \nonumber\\
sack & 1.00000 \nonumber\\
or_other & 1.00000 \nonumber\\
the_plastic & 1.00000 \nonumber\\
spank_be & 1.00000 \nonumber\\
_pos_ngram_O_ADJ_CONJ & 1.00000 \nonumber\\
overpopulation & 1.00000 \nonumber\\
supply_, & 1.00000 \nonumber\\
ProductionRule_CONJP->RB,RB,IN, & 1.00000 \nonumber\\
overpopulation_be & 1.00000 \nonumber\\
crack-addicted/poverty_ride & 1.00000 \nonumber\\
crack-addicted/poverty & 1.00000 \nonumber\\
directly & 1.00000 \nonumber\\
ProductionRule_NP->NP,,,CONJP,NP, & 1.00000 \nonumber\\
ProductionRule_NP->JJ,ADJP,JJ,NNS, & 1.00000 \nonumber\\
directly_supply & 1.00000 \nonumber\\
supply & 1.00000 \nonumber\\
of_overpopulation & 1.00000 \nonumber\\
be_directly & 1.00000 \nonumber\\
._pro-choice & 1.00000 \nonumber\\
pro-life_means & 1.00000 \nonumber\\
ride_baby & 1.00000 \nonumber\\
pro-choice_ftw & 1.00000 \nonumber\\
ride & 1.00000 \nonumber\\
more_crack-addicted/poverty & 1.00000 \nonumber\\
_pos_ngram_ADJ_ADV_ADJ & 1.00000 \nonumber\\
your_spouse & 1.00000 \nonumber\\
even_more & 1.00000 \nonumber\\
the_situation & 1.00000 \nonumber\\
wrong_? & 1.00000 \nonumber\\
few_day & 1.00000 \nonumber\\
ProductionRule_ADVP->RB,PP, & 1.00000 \nonumber\\
my_family & 1.00000 \nonumber\\
be_break & 1.00000 \nonumber\\
_pos_ngram_V_CARD_ADJ & 1.00000 \nonumber\\
well_? & 1.00000 \nonumber\\
person_involve & 1.00000 \nonumber\\
not_yours & 1.00000 \nonumber\\
to_whether & 1.00000 \nonumber\\
'_decision & 1.00000 \nonumber\\
ridiculous_, & 1.00000 \nonumber\\
'_ridiculous & 1.00000 \nonumber\\
,_nor & 1.00000 \nonumber\\
overblow & 1.00000 \nonumber\\
decision_as & 1.00000 \nonumber\\
'_but & 1.00000 \nonumber\\
issue_that & 1.00000 \nonumber\\
involve_' & 1.00000 \nonumber\\
leave_alone & 1.00000 \nonumber\\
--_it & 1.00000 \nonumber\\
kill_over & 1.00000 \nonumber\\
ProductionRule_NP->NN,RB,POS, & 1.00000 \nonumber\\
it_-- & 1.00000 \nonumber\\
overblow_issue & 1.00000 \nonumber\\
nor_anyone & 1.00000 \nonumber\\
an_overblow & 1.00000 \nonumber\\
this_need & 1.00000 \nonumber\\
sometime_that & 1.00000 \nonumber\\
one_person & 1.00000 \nonumber\\
_pos_ngram_ART_NP_O & 1.00000 \nonumber\\
dose & 1.00000 \nonumber\\
:_the & 1.00000 \nonumber\\
yourself_you & 1.00000 \nonumber\\
have_get & 1.00000 \nonumber\\
god_do & 1.00000 \nonumber\\
2007_07:09 & 1.00000 \nonumber\\
be_delete & 1.00000 \nonumber\\
delete & 1.00000 \nonumber\\
by_chasba & 1.00000 \nonumber\\
feb_07 & 1.00000 \nonumber\\
07:09 & 1.00000 \nonumber\\
feb & 1.00000 \nonumber\\
chasba_. & 1.00000 \nonumber\\
rebuttal_, & 1.00000 \nonumber\\
,_2007 & 1.00000 \nonumber\\
_pos_ngram_CARD_PUNC_CARD & 1.00000 \nonumber\\
07 & 1.00000 \nonumber\\
thread_of & 1.00000 \nonumber\\
07:09_have & 1.00000 \nonumber\\
ProductionRule_NP->NNP,CD,,,CD, & 1.00000 \nonumber\\
presumably_by & 1.00000 \nonumber\\
presumably & 1.00000 \nonumber\\
the_argument/rebuttal & 1.00000 \nonumber\\
thread & 1.00000 \nonumber\\
i_rebut & 1.00000 \nonumber\\
on_feb & 1.00000 \nonumber\\
follow_these & 1.00000 \nonumber\\
07_, & 1.00000 \nonumber\\
ProductionRule_VP->VBD,PP,,,PP, & 1.00000 \nonumber\\
chasba_' & 1.00000 \nonumber\\
_pos_ngram_CARD_CARD_V & 1.00000 \nonumber\\
rebut_on & 1.00000 \nonumber\\
argument/rebuttal & 1.00000 \nonumber\\
2007 & 1.00000 \nonumber\\
chasba & 1.00000 \nonumber\\
these_thread & 1.00000 \nonumber\\
delete_, & 1.00000 \nonumber\\
and_rebuttal & 1.00000 \nonumber\\
,_presumably & 1.00000 \nonumber\\
wish_the & 1.00000 \nonumber\\
system_on & 1.00000 \nonumber\\
like_chasba & 1.00000 \nonumber\\
who_try & 1.00000 \nonumber\\
_pos_ngram_NN_ART_PR & 1.00000 \nonumber\\
argument/rebuttal_system & 1.00000 \nonumber\\
there_exercise & 1.00000 \nonumber\\
get_physical & 1.00000 \nonumber\\
burn_as & 1.00000 \nonumber\\
sexist & 1.00000 \nonumber\\
sexist_, & 1.00000 \nonumber\\
those_class & 1.00000 \nonumber\\
just_mostly & 1.00000 \nonumber\\
education_because & 1.00000 \nonumber\\
they_accumulate & 1.00000 \nonumber\\
get_move & 1.00000 \nonumber\\
people_need & 1.00000 \nonumber\\
fat_as & 1.00000 \nonumber\\
everyone_active & 1.00000 \nonumber\\
burn & 1.00000 \nonumber\\
much_fat & 1.00000 \nonumber\\
activity_they & 1.00000 \nonumber\\
people_mostly & 1.00000 \nonumber\\
health_! & 1.00000 \nonumber\\
exercise_be & 1.00000 \nonumber\\
time_people & 1.00000 \nonumber\\
girl_and & 1.00000 \nonumber\\
wont_burn & 1.00000 \nonumber\\
chubbier_. & 1.00000 \nonumber\\
least_exercise & 1.00000 \nonumber\\
chubbier & 1.00000 \nonumber\\
mostly_just & 1.00000 \nonumber\\
mostly_stand & 1.00000 \nonumber\\
get_chubbier & 1.00000 \nonumber\\
keep_everyone & 1.00000 \nonumber\\
they_just & 1.00000 \nonumber\\
accumulate_thus & 1.00000 \nonumber\\
seem_sexist & 1.00000 \nonumber\\
stand_around & 1.00000 \nonumber\\
and_socialize & 1.00000 \nonumber\\
accumulate & 1.00000 \nonumber\\
active_, & 1.00000 \nonumber\\
to_seem & 1.00000 \nonumber\\
there_health & 1.00000 \nonumber\\
stricter_during & 1.00000 \nonumber\\
need_this & 1.00000 \nonumber\\
just_stand & 1.00000 \nonumber\\
stand_there & 1.00000 \nonumber\\
thus_will & 1.00000 \nonumber\\
move_! & 1.00000 \nonumber\\
socialize & 1.00000 \nonumber\\
socialize_. & 1.00000 \nonumber\\
interface & 1.00000 \nonumber\\
take_it & 1.00000 \nonumber\\
._my & 1.00000 \nonumber\\
than_10 & 1.00000 \nonumber\\
from_a & 1.00000 \nonumber\\
have_create & 1.00000 \nonumber\\
addition_to & 1.00000 \nonumber\\
anything_with & 1.00000 \nonumber\\
seek & 1.00000 \nonumber\\
to_eat & 1.00000 \nonumber\\
independence & 1.00000 \nonumber\\
_pos_ngram_PUNC_NP_CARD & 1.00000 \nonumber\\
._therefore & 1.00000 \nonumber\\
problem_be & 1.00000 \nonumber\\
the_uniform & 1.00000 \nonumber\\
just_sit & 1.00000 \nonumber\\
on_every & 1.00000 \nonumber\\
me_wrong & 1.00000 \nonumber\\
tire & 1.00000 \nonumber\\
ProductionRule_ADVP->RB,NP, & 1.00000 \nonumber\\
water_from & 1.00000 \nonumber\\
._# & 1.00000 \nonumber\\
#_3 & 1.00000 \nonumber\\
,_# & 1.00000 \nonumber\\
#_1 & 1.00000 \nonumber\\
# & 1.00000 \nonumber\\
_pos_ngram_O_CARD_PP & 1.00000 \nonumber\\
#_2 & 1.00000 \nonumber\\
be_basically & 1.00000 \nonumber\\
few_year & 1.00000 \nonumber\\
the_scientific & 1.00000 \nonumber\\
how_you & 1.00000 \nonumber\\
idiotic_to & 1.00000 \nonumber\\
plastic_be & 1.00000 \nonumber\\
father_and & 1.00000 \nonumber\\
different_punishment & 1.00000 \nonumber\\
way_but & 1.00000 \nonumber\\
thier & 1.00000 \nonumber\\
_pos_ngram_CONJ_ART_NP & 1.00000 \nonumber\\
these_be & 1.00000 \nonumber\\
will_look & 1.00000 \nonumber\\
ProductionRule_VP->VB,ADJP,PP,S, & 1.00000 \nonumber\\
fine_with & 1.00000 \nonumber\\
to_talk & 1.00000 \nonumber\\
diverse & 1.00000 \nonumber\\
a_different & 1.00000 \nonumber\\
n't_it & 1.00000 \nonumber\\
_pos_ngram_NN_CARD_V & 1.00000 \nonumber\\
ProductionRule_NP->DT,NNP,POS, & 1.00000 \nonumber\\
'd_love & 1.00000 \nonumber\\
major_fact & 1.00000 \nonumber\\
too_stupid & 1.00000 \nonumber\\
who_ca & 1.00000 \nonumber\\
birth_control & 1.00000 \nonumber\\
control_. & 1.00000 \nonumber\\
of_birth & 1.00000 \nonumber\\
just_give & 1.00000 \nonumber\\
minute_form & 1.00000 \nonumber\\
pro-life_base & 1.00000 \nonumber\\
wear_protection & 1.00000 \nonumber\\
...._abortion & 1.00000 \nonumber\\
one_major & 1.00000 \nonumber\\
protection_, & 1.00000 \nonumber\\
the_pill & 1.00000 \nonumber\\
love_to & 1.00000 \nonumber\\
fact_.... & 1.00000 \nonumber\\
who_'d & 1.00000 \nonumber\\
stupid_to & 1.00000 \nonumber\\
last_minute & 1.00000 \nonumber\\
!!!!_and & 1.00000 \nonumber\\
ProductionRule_FRAG->WHADVP,VP, & 1.00000 \nonumber\\
,_bottle & 1.00000 \nonumber\\
child_it & 1.00000 \nonumber\\
after_the & 1.00000 \nonumber\\
ProductionRule_VP->RB,VBG,NP, & 1.00000 \nonumber\\
whether_it & 1.00000 \nonumber\\
ProductionRule_VP->VB,PP,,,SBAR, & 1.00000 \nonumber\\
conception & 1.00000 \nonumber\\
ProductionRule_NP->NP,NNP, & 1.00000 \nonumber\\
ProductionRule_NP->NNP,POS, & 1.00000 \nonumber\\
ProductionRule_VP->VBD,ADVP,,,PP, & 1.00000 \nonumber\\
no_debate & 1.00000 \nonumber\\
actually_read & 1.00000 \nonumber\\
really_no & 1.00000 \nonumber\\
say_in & 1.00000 \nonumber\\
do_gay & 1.00000 \nonumber\\
to_raffle & 1.00000 \nonumber\\
_pos_ngram_PP_O_ADV & 1.00000 \nonumber\\
only_prove & 1.00000 \nonumber\\
firefox_and & 1.00000 \nonumber\\
and_yes & 1.00000 \nonumber\\
just_in & 1.00000 \nonumber\\
sale & 1.00000 \nonumber\\
the_market & 1.00000 \nonumber\\
big_business & 1.00000 \nonumber\\
century & 1.00000 \nonumber\\
_pos_ngram_O_PR_V & 1.00000 \nonumber\\
wont_kill & 1.00000 \nonumber\\
brain_because & 1.00000 \nonumber\\
blow_out & 1.00000 \nonumber\\
kill_again & 1.00000 \nonumber\\
n't_there & 1.00000 \nonumber\\
might_just & 1.00000 \nonumber\\
kill_once & 1.00000 \nonumber\\
paranoia_make & 1.00000 \nonumber\\
paranoia & 1.00000 \nonumber\\
about_be & 1.00000 \nonumber\\
paranoid & 1.00000 \nonumber\\
safety_. & 1.00000 \nonumber\\
paranoid_about & 1.00000 \nonumber\\
target_. & 1.00000 \nonumber\\
just_blow & 1.00000 \nonumber\\
next_target & 1.00000 \nonumber\\
because_paranoia & 1.00000 \nonumber\\
ever_become & 1.00000 \nonumber\\
spouse_but & 1.00000 \nonumber\\
deep_connection & 1.00000 \nonumber\\
become_paranoid & 1.00000 \nonumber\\
crazy_thing & 1.00000 \nonumber\\
target & 1.00000 \nonumber\\
out_your & 1.00000 \nonumber\\
a_deep & 1.00000 \nonumber\\
own_safety & 1.00000 \nonumber\\
catch_they & 1.00000 \nonumber\\
do_crazy & 1.00000 \nonumber\\
door_to & 1.00000 \nonumber\\
_pos_ngram_CONJ_PR_ADV & 1.00000 \nonumber\\
just_know & 1.00000 \nonumber\\
out_within & 1.00000 \nonumber\\
within_100 & 1.00000 \nonumber\\
create_and & 1.00000 \nonumber\\
100_year & 1.00000 \nonumber\\
ProductionRule_NP->NP,'',VP, & 1.00000 \nonumber\\
tweak_vium & 1.00000 \nonumber\\
then_tweak & 1.00000 \nonumber\\
'_god & 1.00000 \nonumber\\
k_, & 1.00000 \nonumber\\
year_anyway & 1.00000 \nonumber\\
vium & 1.00000 \nonumber\\
'_create & 1.00000 \nonumber\\
k & 1.00000 \nonumber\\
vium_evolution & 1.00000 \nonumber\\
all_find & 1.00000 \nonumber\\
anyway_.... & 1.00000 \nonumber\\
expensive & 1.00000 \nonumber\\
something_good & 1.00000 \nonumber\\
a_provider & 1.00000 \nonumber\\
a_protector & 1.00000 \nonumber\\
father_think & 1.00000 \nonumber\\
because_; & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,ADJP,S,PP, & 1.00000 \nonumber\\
they_go & 1.00000 \nonumber\\
provider_but & 1.00000 \nonumber\\
protector_. & 1.00000 \nonumber\\
work_without & 1.00000 \nonumber\\
child_grow & 1.00000 \nonumber\\
without_give & 1.00000 \nonumber\\
protector & 1.00000 \nonumber\\
;_when & 1.00000 \nonumber\\
give_much & 1.00000 \nonumber\\
ProductionRule_NP->RB,NP,CC,ADVP,NP, & 1.00000 \nonumber\\
any_shape & 1.00000 \nonumber\\
spouse_like & 1.00000 \nonumber\\
imagine_turn & 1.00000 \nonumber\\
say_a & 1.00000 \nonumber\\
right_there & 1.00000 \nonumber\\
someone_it & 1.00000 \nonumber\\
plus_if & 1.00000 \nonumber\\
a_word & 1.00000 \nonumber\\
business_. & 1.00000 \nonumber\\
theory & 1.00000 \nonumber\\
put_other & 1.00000 \nonumber\\
sacrifice & 1.00000 \nonumber\\
because_... & 1.00000 \nonumber\\
could_come & 1.00000 \nonumber\\
be_enough & 1.00000 \nonumber\\
never_exist & 1.00000 \nonumber\\
way_he & 1.00000 \nonumber\\
walk_out & 1.00000 \nonumber\\
rather_him & 1.00000 \nonumber\\
an_absence & 1.00000 \nonumber\\
because_either & 1.00000 \nonumber\\
enough_. & 1.00000 \nonumber\\
trust_, & 1.00000 \nonumber\\
you_nothing & 1.00000 \nonumber\\
have_from & 1.00000 \nonumber\\
than_come & 1.00000 \nonumber\\
heartache & 1.00000 \nonumber\\
your_trust & 1.00000 \nonumber\\
absence_because & 1.00000 \nonumber\\
about_him & 1.00000 \nonumber\\
his_absence & 1.00000 \nonumber\\
him_never & 1.00000 \nonumber\\
and_out & 1.00000 \nonumber\\
and_walk & 1.00000 \nonumber\\
itself_an & 1.00000 \nonumber\\
only_heartache & 1.00000 \nonumber\\
would_ensure & 1.00000 \nonumber\\
be_his & 1.00000 \nonumber\\
absence_, & 1.00000 \nonumber\\
in_gain & 1.00000 \nonumber\\
heartache_you & 1.00000 \nonumber\\
gain_your & 1.00000 \nonumber\\
exist_than & 1.00000 \nonumber\\
in_itself & 1.00000 \nonumber\\
your_browser & 1.00000 \nonumber\\
teach_you & 1.00000 \nonumber\\
..._game & 1.00000 \nonumber\\
2500 & 1.00000 \nonumber\\
%_more & 1.00000 \nonumber\\
2500_% & 1.00000 \nonumber\\
cry_about & 1.00000 \nonumber\\
sorry_firefox & 1.00000 \nonumber\\
lay_2500 & 1.00000 \nonumber\\
^_( & 1.00000 \nonumber\\
8 & 1.00000 \nonumber\\
match_go & 1.00000 \nonumber\\
ie_somewhere & 1.00000 \nonumber\\
else_8 & 1.00000 \nonumber\\
firefox_loser & 1.00000 \nonumber\\
the_average & 1.00000 \nonumber\\
game_set & 1.00000 \nonumber\\
loser_... & 1.00000 \nonumber\\
set_match & 1.00000 \nonumber\\
user_get & 1.00000 \nonumber\\
its_an & 1.00000 \nonumber\\
average_firefox & 1.00000 \nonumber\\
user_. & 1.00000 \nonumber\\
indisputable_fact & 1.00000 \nonumber\\
average_ie & 1.00000 \nonumber\\
_pos_ngram_CARD_O_O & 1.00000 \nonumber\\
somewhere_else & 1.00000 \nonumber\\
8_* & 1.00000 \nonumber\\
about_ie & 1.00000 \nonumber\\
an_indisputable & 1.00000 \nonumber\\
actual_evidence & 1.00000 \nonumber\\
evolution_!! & 1.00000 \nonumber\\
ProductionRule_NP->DT,FW, & 1.00000 \nonumber\\
say_on & 1.00000 \nonumber\\
be_actual & 1.00000 \nonumber\\
candy_store & 1.00000 \nonumber\\
child_pornographor & 1.00000 \nonumber\\
open_the & 1.00000 \nonumber\\
they_please & 1.00000 \nonumber\\
the_candy & 1.00000 \nonumber\\
predator & 1.00000 \nonumber\\
the_door & 1.00000 \nonumber\\
sexual_predator & 1.00000 \nonumber\\
have_open & 1.00000 \nonumber\\
pornographor_, & 1.00000 \nonumber\\
ProductionRule_UCP->S,CC,PP, & 1.00000 \nonumber\\
,_sexual & 1.00000 \nonumber\\
store & 1.00000 \nonumber\\
could_walk & 1.00000 \nonumber\\
to_new & 1.00000 \nonumber\\
store_, & 1.00000 \nonumber\\
online_. & 1.00000 \nonumber\\
pornographor & 1.00000 \nonumber\\
ProductionRule_VP->VBD,,,PP,,,UCP, & 1.00000 \nonumber\\
online & 1.00000 \nonumber\\
now_there & 1.00000 \nonumber\\
new_crime & 1.00000 \nonumber\\
around_as & 1.00000 \nonumber\\
ProductionRule_PP->TO,CC,IN,NP, & 1.00000 \nonumber\\
predator_online & 1.00000 \nonumber\\
as_other & 1.00000 \nonumber\\
_pos_ngram_ADV_ADV_PR & 1.00000 \nonumber\\
he_can & 1.00000 \nonumber\\
._well & 1.00000 \nonumber\\
._generally & 1.00000 \nonumber\\
general_, & 1.00000 \nonumber\\
generally & 1.00000 \nonumber\\
supposedly_unsophisticate & 1.00000 \nonumber\\
generally_, & 1.00000 \nonumber\\
transform & 1.00000 \nonumber\\
create_me & 1.00000 \nonumber\\
adam_where & 1.00000 \nonumber\\
ape & 1.00000 \nonumber\\
concrete_one & 1.00000 \nonumber\\
ape_concept & 1.00000 \nonumber\\
unsophisticate & 1.00000 \nonumber\\
be_abstract & 1.00000 \nonumber\\
ancient_would & 1.00000 \nonumber\\
a_concrete & 1.00000 \nonumber\\
all_choose & 1.00000 \nonumber\\
you_ask & 1.00000 \nonumber\\
unsophisticate_ancient & 1.00000 \nonumber\\
concept_rather & 1.00000 \nonumber\\
hand_around & 1.00000 \nonumber\\
general & 1.00000 \nonumber\\
ask_adam & 1.00000 \nonumber\\
concrete_. & 1.00000 \nonumber\\
pretty_hard & 1.00000 \nonumber\\
ape_be & 1.00000 \nonumber\\
ape_over & 1.00000 \nonumber\\
those_ape & 1.00000 \nonumber\\
'_funny & 1.00000 \nonumber\\
abstract_concept & 1.00000 \nonumber\\
._ape & 1.00000 \nonumber\\
be_magically & 1.00000 \nonumber\\
be_concrete & 1.00000 \nonumber\\
funny_that & 1.00000 \nonumber\\
abstract_. & 1.00000 \nonumber\\
"_instead & 1.00000 \nonumber\\
garden_" & 1.00000 \nonumber\\
whole_ape & 1.00000 \nonumber\\
the_garden & 1.00000 \nonumber\\
there_" & 1.00000 \nonumber\\
often_show & 1.00000 \nonumber\\
over_there & 1.00000 \nonumber\\
show_himself & 1.00000 \nonumber\\
god_must & 1.00000 \nonumber\\
supposedly & 1.00000 \nonumber\\
the_supposedly & 1.00000 \nonumber\\
transform_from & 1.00000 \nonumber\\
magically_transform & 1.00000 \nonumber\\
from_one & 1.00000 \nonumber\\
he_say & 1.00000 \nonumber\\
n't_often & 1.00000 \nonumber\\
in_general & 1.00000 \nonumber\\
the_line & 1.00000 \nonumber\\
,_especially & 1.00000 \nonumber\\
_pos_ngram_NP_ART_ADJ & 1.00000 \nonumber\\
their_choice & 1.00000 \nonumber\\
life_decision & 1.00000 \nonumber\\
happen_) & 1.00000 \nonumber\\
will_die & 1.00000 \nonumber\\
position_, & 1.00000 \nonumber\\
establish_, & 1.00000 \nonumber\\
14_, & 1.00000 \nonumber\\
which_, & 1.00000 \nonumber\\
ProductionRule_S->S,,,CC,S,,,CC,S, & 1.00000 \nonumber\\
ProductionRule_VP->LS,ADVP,PP, & 1.00000 \nonumber\\
officially_have & 1.00000 \nonumber\\
abortion_? & 1.00000 \nonumber\\
someone_on & 1.00000 \nonumber\\
officially & 1.00000 \nonumber\\
then_pro-life & 1.00000 \nonumber\\
rape_( & 1.00000 \nonumber\\
ProductionRule_PP->RB,ADJP, & 1.00000 \nonumber\\
an_answer & 1.00000 \nonumber\\
pro-life_to & 1.00000 \nonumber\\
know_: & 1.00000 \nonumber\\
_pos_ngram_O_ART_PUNC & 1.00000 \nonumber\\
from_someone & 1.00000 \nonumber\\
side_to & 1.00000 \nonumber\\
she_then & 1.00000 \nonumber\\
honestly_just & 1.00000 \nonumber\\
want_someone & 1.00000 \nonumber\\
die_if & 1.00000 \nonumber\\
,_happen & 1.00000 \nonumber\\
i_officially & 1.00000 \nonumber\\
answer_from & 1.00000 \nonumber\\
a_14 & 1.00000 \nonumber\\
answer_this & 1.00000 \nonumber\\
ProductionRule_VP->VBP,S,PRN, & 1.00000 \nonumber\\
the_pro & 1.00000 \nonumber\\
have_establish & 1.00000 \nonumber\\
old_be & 1.00000 \nonumber\\
ProductionRule_S->PRN,VP, & 1.00000 \nonumber\\
ProductionRule_VP->VBP,:,SBAR, & 1.00000 \nonumber\\
version_to & 1.00000 \nonumber\\
behalf & 1.00000 \nonumber\\
bear_. & 1.00000 \nonumber\\
as_bid & 1.00000 \nonumber\\
_pos_ngram_ART_PR_CONJ & 1.00000 \nonumber\\
by_her & 1.00000 \nonumber\\
in_poverty & 1.00000 \nonumber\\
step_dad & 1.00000 \nonumber\\
devout & 1.00000 \nonumber\\
life_actually & 1.00000 \nonumber\\
devout_catholic & 1.00000 \nonumber\\
_pos_ngram_CONJ_PR_CARD & 1.00000 \nonumber\\
rape_by & 1.00000 \nonumber\\
ProductionRule_NP->DT,JJ,NNS,RB, & 1.00000 \nonumber\\
a_nine & 1.00000 \nonumber\\
what_life & 1.00000 \nonumber\\
america_be & 1.00000 \nonumber\\
in_south & 1.00000 \nonumber\\
three_life & 1.00000 \nonumber\\
twin & 1.00000 \nonumber\\
two_child & 1.00000 \nonumber\\
childbirth_, & 1.00000 \nonumber\\
nine_year & 1.00000 \nonumber\\
twin_. & 1.00000 \nonumber\\
those_life & 1.00000 \nonumber\\
girl_live & 1.00000 \nonumber\\
year_back & 1.00000 \nonumber\\
childbirth & 1.00000 \nonumber\\
be_devout & 1.00000 \nonumber\\
with_twin & 1.00000 \nonumber\\
south_america & 1.00000 \nonumber\\
pregnant_with & 1.00000 \nonumber\\
._her & 1.00000 \nonumber\\
life_lose & 1.00000 \nonumber\\
in_childbirth & 1.00000 \nonumber\\
old_girl & 1.00000 \nonumber\\
poverty_in & 1.00000 \nonumber\\
child_die & 1.00000 \nonumber\\
story_for & 1.00000 \nonumber\\
catholic_. & 1.00000 \nonumber\\
'_three & 1.00000 \nonumber\\
her_family & 1.00000 \nonumber\\
her_step & 1.00000 \nonumber\\
her_two & 1.00000 \nonumber\\
actually_know & 1.00000 \nonumber\\
would_die & 1.00000 \nonumber\\
south & 1.00000 \nonumber\\
_pos_ngram_PUNC_CARD_PP & 1.00000 \nonumber\\
family_know & 1.00000 \nonumber\\
both_her & 1.00000 \nonumber\\
abortion_because & 1.00000 \nonumber\\
help_every & 1.00000 \nonumber\\
e & 1.00000 \nonumber\\
be_pro-choice & 1.00000 \nonumber\\
wrong_it & 1.00000 \nonumber\\
that_single & 1.00000 \nonumber\\
reason_more & 1.00000 \nonumber\\
be_becuse & 1.00000 \nonumber\\
becuse_it & 1.00000 \nonumber\\
the_default & 1.00000 \nonumber\\
becuse & 1.00000 \nonumber\\
single_browser & 1.00000 \nonumber\\
most_comp & 1.00000 \nonumber\\
browser_for & 1.00000 \nonumber\\
only_know & 1.00000 \nonumber\\
for_most & 1.00000 \nonumber\\
comp_. & 1.00000 \nonumber\\
comp & 1.00000 \nonumber\\
have_only & 1.00000 \nonumber\\
people_use & 1.00000 \nonumber\\
!_the & 1.00000 \nonumber\\
use_ie & 1.00000 \nonumber\\
bet_90 & 1.00000 \nonumber\\
ie_supporter & 1.00000 \nonumber\\
the_ie & 1.00000 \nonumber\\
best_! & 1.00000 \nonumber\\
supporter_have & 1.00000 \nonumber\\
say_obama & 1.00000 \nonumber\\
could_do & 1.00000 \nonumber\\
and_effort & 1.00000 \nonumber\\
a_succeful & 1.00000 \nonumber\\
in_good & 1.00000 \nonumber\\
succeful_trade & 1.00000 \nonumber\\
founder_! & 1.00000 \nonumber\\
founder_" & 1.00000 \nonumber\\
health_reform & 1.00000 \nonumber\\
he_invest & 1.00000 \nonumber\\
our_founder & 1.00000 \nonumber\\
credit_him & 1.00000 \nonumber\\
why_because & 1.00000 \nonumber\\
obama_be & 1.00000 \nonumber\\
founder_and & 1.00000 \nonumber\\
therefore_credit & 1.00000 \nonumber\\
reform_why & 1.00000 \nonumber\\
"_of & 1.00000 \nonumber\\
good_position & 1.00000 \nonumber\\
good_contact & 1.00000 \nonumber\\
him_we & 1.00000 \nonumber\\
a_project & 1.00000 \nonumber\\
in_such & 1.00000 \nonumber\\
port_you & 1.00000 \nonumber\\
succeful & 1.00000 \nonumber\\
invest_a & 1.00000 \nonumber\\
port_at & 1.00000 \nonumber\\
position_and & 1.00000 \nonumber\\
"_founder & 1.00000 \nonumber\\
high_position & 1.00000 \nonumber\\
invest_money & 1.00000 \nonumber\\
contact & 1.00000 \nonumber\\
lot_and & 1.00000 \nonumber\\
effort_in & 1.00000 \nonumber\\
we_therefore & 1.00000 \nonumber\\
contact_with & 1.00000 \nonumber\\
contact_without & 1.00000 \nonumber\\
the_important & 1.00000 \nonumber\\
we_say & 1.00000 \nonumber\\
like_invest & 1.00000 \nonumber\\
of_health & 1.00000 \nonumber\\
those_contact & 1.00000 \nonumber\\
money_time & 1.00000 \nonumber\\
important_quality & 1.00000 \nonumber\\
one_i & 1.00000 \nonumber\\
stand_for & 1.00000 \nonumber\\
say_science & 1.00000 \nonumber\\
really_stand & 1.00000 \nonumber\\
just_what & 1.00000 \nonumber\\
difference_between & 1.00000 \nonumber\\
be_perfect & 1.00000 \nonumber\\
dogmatic_enough & 1.00000 \nonumber\\
,_science & 1.00000 \nonumber\\
even_recognise & 1.00000 \nonumber\\
what_truth & 1.00000 \nonumber\\
perfect_. & 1.00000 \nonumber\\
recognise_fact & 1.00000 \nonumber\\
ever_say & 1.00000 \nonumber\\
between_religion & 1.00000 \nonumber\\
while_religion & 1.00000 \nonumber\\
recognise & 1.00000 \nonumber\\
answer_while & 1.00000 \nonumber\\
truth_really & 1.00000 \nonumber\\
and_science & 1.00000 \nonumber\\
so_dogmatic & 1.00000 \nonumber\\
even_just & 1.00000 \nonumber\\
science_admit & 1.00000 \nonumber\\
dogmatic & 1.00000 \nonumber\\
fact_. & 1.00000 \nonumber\\
ProductionRule_VP->VBD,``,VP, & 1.00000 \nonumber\\
be_corrupt & 1.00000 \nonumber\\
a_biological & 1.00000 \nonumber\\
engineer_" & 1.00000 \nonumber\\
"_engineer & 1.00000 \nonumber\\
society_of & 1.00000 \nonumber\\
biological_standpoint & 1.00000 \nonumber\\
ProductionRule_VP->VBN,'',S, & 1.00000 \nonumber\\
our_time & 1.00000 \nonumber\\
corrupt_by & 1.00000 \nonumber\\
logical & 1.00000 \nonumber\\
you_who & 1.00000 \nonumber\\
no_choice & 1.00000 \nonumber\\
it_matter & 1.00000 \nonumber\\
cop & 1.00000 \nonumber\\
_pos_ngram_PP_CARD_CONJ & 1.00000 \nonumber\\
energy & 1.00000 \nonumber\\
have_somebody & 1.00000 \nonumber\\
consequence_, & 1.00000 \nonumber\\
citizen & 1.00000 \nonumber\\
of_bull & 1.00000 \nonumber\\
the_firefox & 1.00000 \nonumber\\
religious_thing & 1.00000 \nonumber\\
,_religious & 1.00000 \nonumber\\
not_mix & 1.00000 \nonumber\\
real_issue & 1.00000 \nonumber\\
be_separate & 1.00000 \nonumber\\
institution_and & 1.00000 \nonumber\\
all_? & 1.00000 \nonumber\\
personal_, & 1.00000 \nonumber\\
from_government & 1.00000 \nonumber\\
be_- & 1.00000 \nonumber\\
government_should & 1.00000 \nonumber\\
government_regulation & 1.00000 \nonumber\\
government_involve & 1.00000 \nonumber\\
to_redefine & 1.00000 \nonumber\\
government_come & 1.00000 \nonumber\\
thing_should & 1.00000 \nonumber\\
that_solve & 1.00000 \nonumber\\
issue_at & 1.00000 \nonumber\\
problem_" & 1.00000 \nonumber\\
a_political & 1.00000 \nonumber\\
we_take & 1.00000 \nonumber\\
mix_. & 1.00000 \nonumber\\
political & 1.00000 \nonumber\\
regulate_it & 1.00000 \nonumber\\
"_problem & 1.00000 \nonumber\\
and_regulate & 1.00000 \nonumber\\
regulation_. & 1.00000 \nonumber\\
political_issue & 1.00000 \nonumber\\
redefine_it & 1.00000 \nonumber\\
_pos_ngram_PUNC_V_V & 1.00000 \nonumber\\
visually & 1.00000 \nonumber\\
more_secure & 1.00000 \nonumber\\
secure_as & 1.00000 \nonumber\\
visually_please & 1.00000 \nonumber\\
use_. & 1.00000 \nonumber\\
ProductionRule_ADJP->RB,JJR,SBAR, & 1.00000 \nonumber\\
more_visually & 1.00000 \nonumber\\
emotionally_, & 1.00000 \nonumber\\
video & 1.00000 \nonumber\\
read_it & 1.00000 \nonumber\\
invite_the & 1.00000 \nonumber\\
often_occur & 1.00000 \nonumber\\
_pos_ngram_ADV_O_NN & 1.00000 \nonumber\\
be_neither & 1.00000 \nonumber\\
be_callad & 1.00000 \nonumber\\
despite_i & 1.00000 \nonumber\\
nor_atheist & 1.00000 \nonumber\\
neither_christian & 1.00000 \nonumber\\
callad_as & 1.00000 \nonumber\\
atheist_, & 1.00000 \nonumber\\
place_for & 1.00000 \nonumber\\
callad & 1.00000 \nonumber\\
but_despite & 1.00000 \nonumber\\
god_in & 1.00000 \nonumber\\
atheism.if_there & 1.00000 \nonumber\\
christian_nor & 1.00000 \nonumber\\
atheism.if & 1.00000 \nonumber\\
for_god & 1.00000 \nonumber\\
than_atheism.if & 1.00000 \nonumber\\
an_addiction & 1.00000 \nonumber\\
effective & 1.00000 \nonumber\\
'_even & 1.00000 \nonumber\\
its_help & 1.00000 \nonumber\\
not_work & 1.00000 \nonumber\\
it_work & 1.00000 \nonumber\\
exist_, & 1.00000 \nonumber\\
reform & 1.00000 \nonumber\\
production & 1.00000 \nonumber\\
people_get & 1.00000 \nonumber\\
my_country & 1.00000 \nonumber\\
potential_. & 1.00000 \nonumber\\
need_. & 1.00000 \nonumber\\
everyone_want & 1.00000 \nonumber\\
then_get & 1.00000 \nonumber\\
good_would & 1.00000 \nonumber\\
school_? & 1.00000 \nonumber\\
role_in & 1.00000 \nonumber\\
play_a & 1.00000 \nonumber\\
may_have & 1.00000 \nonumber\\
that_because & 1.00000 \nonumber\\
wont & 1.00000 \nonumber\\
ever_. & 1.00000 \nonumber\\
ProductionRule_VP->VBP,PP,ADVP, & 1.00000 \nonumber\\
._accord & 1.00000 \nonumber\\
then_other & 1.00000 \nonumber\\
?? & 1.00000 \nonumber\\
make_everyone & 1.00000 \nonumber\\
reproduce_. & 1.00000 \nonumber\\
pro-life_i & 1.00000 \nonumber\\
pro-choice_because & 1.00000 \nonumber\\
choose_pro-choice & 1.00000 \nonumber\\
the_option & 1.00000 \nonumber\\
simple_choice & 1.00000 \nonumber\\
choose_pro & 1.00000 \nonumber\\
choose_pro-life & 1.00000 \nonumber\\
a_rather & 1.00000 \nonumber\\
rather_simple & 1.00000 \nonumber\\
read_and & 1.00000 \nonumber\\
expose_hole & 1.00000 \nonumber\\
ProductionRule_S->``,NP,'', & 1.00000 \nonumber\\
ProductionRule_S->S,RB,,,S,CC,S, & 1.00000 \nonumber\\
my_question & 1.00000 \nonumber\\
actually_you & 1.00000 \nonumber\\
cross_examine & 1.00000 \nonumber\\
opponent_' & 1.00000 \nonumber\\
about_debate & 1.00000 \nonumber\\
question_and & 1.00000 \nonumber\\
answer_my & 1.00000 \nonumber\\
position_also & 1.00000 \nonumber\\
common_tactic & 1.00000 \nonumber\\
an_opponent & 1.00000 \nonumber\\
debate_you & 1.00000 \nonumber\\
for_expose & 1.00000 \nonumber\\
ProductionRule_S->S,NP,ADVP,VP, & 1.00000 \nonumber\\
"_cross & 1.00000 \nonumber\\
examine & 1.00000 \nonumber\\
frustrate_for & 1.00000 \nonumber\\
be_frustrate & 1.00000 \nonumber\\
call_name & 1.00000 \nonumber\\
win_a & 1.00000 \nonumber\\
debate_because & 1.00000 \nonumber\\
tactic & 1.00000 \nonumber\\
tactic_for & 1.00000 \nonumber\\
,_call & 1.00000 \nonumber\\
'_position & 1.00000 \nonumber\\
never_win & 1.00000 \nonumber\\
n't_answer & 1.00000 \nonumber\\
very_common & 1.00000 \nonumber\\
name_never & 1.00000 \nonumber\\
examine_" & 1.00000 \nonumber\\
ProductionRule_S->NP,``,ADJP,'', & 1.00000 \nonumber\\
father_to & 1.00000 \nonumber\\
reality_that & 1.00000 \nonumber\\
porn_star & 1.00000 \nonumber\\
addict_turn & 1.00000 \nonumber\\
it_tend & 1.00000 \nonumber\\
view_woman & 1.00000 \nonumber\\
and_mistreat & 1.00000 \nonumber\\
and_view & 1.00000 \nonumber\\
be_addict & 1.00000 \nonumber\\
what_sex & 1.00000 \nonumber\\
in_moderation & 1.00000 \nonumber\\
porn_addict & 1.00000 \nonumber\\
all_woman & 1.00000 \nonumber\\
up_their & 1.00000 \nonumber\\
expect_all & 1.00000 \nonumber\\
,_expect & 1.00000 \nonumber\\
negative_manner & 1.00000 \nonumber\\
addict & 1.00000 \nonumber\\
about_... & 1.00000 \nonumber\\
not_what & 1.00000 \nonumber\\
star_and & 1.00000 \nonumber\\
intimacy & 1.00000 \nonumber\\
star_, & 1.00000 \nonumber\\
mistreat_and & 1.00000 \nonumber\\
moderation & 1.00000 \nonumber\\
intimacy_issue & 1.00000 \nonumber\\
also_people & 1.00000 \nonumber\\
mistreat & 1.00000 \nonumber\\
their_relationship & 1.00000 \nonumber\\
moderation_. & 1.00000 \nonumber\\
screw_up & 1.00000 \nonumber\\
their_reality & 1.00000 \nonumber\\
to_screw & 1.00000 \nonumber\\
addict_to & 1.00000 \nonumber\\
have_intimacy & 1.00000 \nonumber\\
star & 1.00000 \nonumber\\
nothing_about & 1.00000 \nonumber\\
parent_, & 1.00000 \nonumber\\
walk_around & 1.00000 \nonumber\\
ProductionRule_VP->ADVP,VBN,PP, & 1.00000 \nonumber\\
job_and & 1.00000 \nonumber\\
see_any & 1.00000 \nonumber\\
love_plastic & 1.00000 \nonumber\\
cant_argue & 1.00000 \nonumber\\
that_logic & 1.00000 \nonumber\\
jesus_love & 1.00000 \nonumber\\
and_live & 1.00000 \nonumber\\
they_will & 1.00000 \nonumber\\
n & 1.00000 \nonumber\\
introduce_opium & 1.00000 \nonumber\\
raise_the & 1.00000 \nonumber\\
raise_more & 1.00000 \nonumber\\
city_of & 1.00000 \nonumber\\
opium_sell & 1.00000 \nonumber\\
singapore_in & 1.00000 \nonumber\\
also_introduce & 1.00000 \nonumber\\
ProductionRule_S->SBAR,,,NP,ADVP,VP, & 1.00000 \nonumber\\
to_build & 1.00000 \nonumber\\
sell_into & 1.00000 \nonumber\\
build_singapore & 1.00000 \nonumber\\
into_singapore & 1.00000 \nonumber\\
raffle_find & 1.00000 \nonumber\\
he_also & 1.00000 \nonumber\\
of_raise & 1.00000 \nonumber\\
opium & 1.00000 \nonumber\\
bid_job & 1.00000 \nonumber\\
all_different & 1.00000 \nonumber\\
make_up & 1.00000 \nonumber\\
concrete & 1.00000 \nonumber\\
latest & 1.00000 \nonumber\\
we_only & 1.00000 \nonumber\\
my_parent & 1.00000 \nonumber\\
_pos_ngram_CARD_PUNC_ART & 1.00000 \nonumber\\
be_fire & 1.00000 \nonumber\\
of_parent & 1.00000 \nonumber\\
most_likley & 1.00000 \nonumber\\
likley & 1.00000 \nonumber\\
ban_their & 1.00000 \nonumber\\
record_than & 1.00000 \nonumber\\
detriment & 1.00000 \nonumber\\
advertise_on & 1.00000 \nonumber\\
onto & 1.00000 \nonumber\\
,_these & 1.00000 \nonumber\\
._ban & 1.00000 \nonumber\\
spend_billion & 1.00000 \nonumber\\
actual_sale & 1.00000 \nonumber\\
the_advertise & 1.00000 \nonumber\\
detriment_. & 1.00000 \nonumber\\
advertise & 1.00000 \nonumber\\
onto_the & 1.00000 \nonumber\\
(_http://www.cdc.gov/healthywater/drinking/bottled/ & 1.00000 \nonumber\\
http://www.cdc.gov/healthywater/drinking/bottled/_) & 1.00000 \nonumber\\
(_http://www.friendsjournal.org/bottled-water & 1.00000 \nonumber\\
http://www.friendsjournal.org/bottled-water & 1.00000 \nonumber\\
greatly_hurt & 1.00000 \nonumber\\
greatly & 1.00000 \nonumber\\
american_spend & 1.00000 \nonumber\\
use_instead & 1.00000 \nonumber\\
an_already & 1.00000 \nonumber\\
http://www.cdc.gov/healthywater/drinking/bottled/ & 1.00000 \nonumber\\
water_not & 1.00000 \nonumber\\
package_be & 1.00000 \nonumber\\
trace & 1.00000 \nonumber\\
trace_when & 1.00000 \nonumber\\
,_compostable & 1.00000 \nonumber\\
these_can & 1.00000 \nonumber\\
a_potential & 1.00000 \nonumber\\
http://www.friendsjournal.org/bottled-water_) & 1.00000 \nonumber\\
health_risk & 1.00000 \nonumber\\
that_detriment & 1.00000 \nonumber\\
cleaner & 1.00000 \nonumber\\
cleaner_safety & 1.00000 \nonumber\\
than_municipal & 1.00000 \nonumber\\
potential_health & 1.00000 \nonumber\\
their_sale & 1.00000 \nonumber\\
bottle_and & 1.00000 \nonumber\\
struggle_economy & 1.00000 \nonumber\\
on_bottle & 1.00000 \nonumber\\
come_onto & 1.00000 \nonumber\\
billion_on & 1.00000 \nonumber\\
a_cleaner & 1.00000 \nonumber\\
compostable & 1.00000 \nonumber\\
compostable_water & 1.00000 \nonumber\\
risk_do & 1.00000 \nonumber\\
eliminate_that & 1.00000 \nonumber\\
safety_record & 1.00000 \nonumber\\
sale_of & 1.00000 \nonumber\\
hurt_an & 1.00000 \nonumber\\
and_package & 1.00000 \nonumber\\
plastic_that & 1.00000 \nonumber\\
when_a & 1.00000 \nonumber\\
already_struggle & 1.00000 \nonumber\\
would_greatly & 1.00000 \nonumber\\
moreover_, & 1.00000 \nonumber\\
also_big & 1.00000 \nonumber\\
plastic_to & 1.00000 \nonumber\\
sale_would & 1.00000 \nonumber\\
to_trace & 1.00000 \nonumber\\
bottle_until & 1.00000 \nonumber\\
to_ban & 1.00000 \nonumber\\
ban_water & 1.00000 \nonumber\\
recession_! & 1.00000 \nonumber\\
until_we & 1.00000 \nonumber\\
its_only & 1.00000 \nonumber\\
only_do & 1.00000 \nonumber\\
expose & 1.00000 \nonumber\\
?_would & 1.00000 \nonumber\\
every_kid & 1.00000 \nonumber\\
because_child & 1.00000 \nonumber\\
have_bid & 1.00000 \nonumber\\
a_team & 1.00000 \nonumber\\
ProductionRule_NP->PRP$,JJS,NN, & 1.00000 \nonumber\\
would_. & 1.00000 \nonumber\\
not_say & 1.00000 \nonumber\\
nicotine_. & 1.00000 \nonumber\\
to_mystical & 1.00000 \nonumber\\
relativity & 1.00000 \nonumber\\
nicotine & 1.00000 \nonumber\\
of_relativity & 1.00000 \nonumber\\
kitchen & 1.00000 \nonumber\\
throw_the & 1.00000 \nonumber\\
often_give & 1.00000 \nonumber\\
fahrenheit & 1.00000 \nonumber\\
mind_into & 1.00000 \nonumber\\
fahrenheit_451 & 1.00000 \nonumber\\
circus & 1.00000 \nonumber\\
circus_, & 1.00000 \nonumber\\
book_throw & 1.00000 \nonumber\\
_pos_ngram_PUNC_NN_CARD & 1.00000 \nonumber\\
book_enlighten & 1.00000 \nonumber\\
paradise_, & 1.00000 \nonumber\\
451_, & 1.00000 \nonumber\\
451 & 1.00000 \nonumber\\
of_child & 1.00000 \nonumber\\
enlighten_the & 1.00000 \nonumber\\
enlighten & 1.00000 \nonumber\\
night_circus & 1.00000 \nonumber\\
._fahrenheit & 1.00000 \nonumber\\
garden_, & 1.00000 \nonumber\\
paradise & 1.00000 \nonumber\\
kitchen_sink & 1.00000 \nonumber\\
'_as & 1.00000 \nonumber\\
inkheart & 1.00000 \nonumber\\
on_life & 1.00000 \nonumber\\
question_, & 1.00000 \nonumber\\
perspective_on & 1.00000 \nonumber\\
,_inkheart & 1.00000 \nonumber\\
and_often & 1.00000 \nonumber\\
moral_of & 1.00000 \nonumber\\
as_nicotine & 1.00000 \nonumber\\
explain_. & 1.00000 \nonumber\\
the_reader & 1.00000 \nonumber\\
n't_destroy & 1.00000 \nonumber\\
change_your & 1.00000 \nonumber\\
drug_. & 1.00000 \nonumber\\
even_the & 1.00000 \nonumber\\
of_question & 1.00000 \nonumber\\
the_night & 1.00000 \nonumber\\
place_, & 1.00000 \nonumber\\
mystical_place & 1.00000 \nonumber\\
reader & 1.00000 \nonumber\\
mystical & 1.00000 \nonumber\\
inkheart_... & 1.00000 \nonumber\\
they_change & 1.00000 \nonumber\\
secret_garden & 1.00000 \nonumber\\
,_paradise & 1.00000 \nonumber\\
your_perspective & 1.00000 \nonumber\\
to_further & 1.00000 \nonumber\\
further_explain & 1.00000 \nonumber\\
the_kitchen & 1.00000 \nonumber\\
._? & 1.00000 \nonumber\\
reader_to & 1.00000 \nonumber\\
reader_a & 1.00000 \nonumber\\
relativity_. & 1.00000 \nonumber\\
river & 1.00000 \nonumber\\
rebut & 1.00000 \nonumber\\
smoke & 1.00000 \nonumber\\
should_watch & 1.00000 \nonumber\\
show_them & 1.00000 \nonumber\\
relatively & 1.00000 \nonumber\\
_pos_ngram_ADJ_ADV_ADV & 1.00000 \nonumber\\
be_ashame & 1.00000 \nonumber\\
easier_for & 1.00000 \nonumber\\
ProductionRule_VP->LS,VP, & 1.00000 \nonumber\\
_pos_ngram_NP_CONJ_ADV & 1.00000 \nonumber\\
._christianity & 1.00000 \nonumber\\
_pos_ngram_NN_ADV_ART & 1.00000 \nonumber\\
anytime & 1.00000 \nonumber\\
mandatory_, & 1.00000 \nonumber\\
activity_to & 1.00000 \nonumber\\
good_game & 1.00000 \nonumber\\
them_game & 1.00000 \nonumber\\
you_consider & 1.00000 \nonumber\\
a_requirement & 1.00000 \nonumber\\
not_more & 1.00000 \nonumber\\
with_girl & 1.00000 \nonumber\\
more_often & 1.00000 \nonumber\\
thing_with & 1.00000 \nonumber\\
girl_idea & 1.00000 \nonumber\\
so_well & 1.00000 \nonumber\\
assign & 1.00000 \nonumber\\
assign_some & 1.00000 \nonumber\\
for_girl & 1.00000 \nonumber\\
game_for & 1.00000 \nonumber\\
game_of & 1.00000 \nonumber\\
if_possible & 1.00000 \nonumber\\
for_boy & 1.00000 \nonumber\\
from_girl & 1.00000 \nonumber\\
requirement_but & 1.00000 \nonumber\\
consider_pe & 1.00000 \nonumber\\
pe_if & 1.00000 \nonumber\\
boy_assign & 1.00000 \nonumber\\
separate_boy & 1.00000 \nonumber\\
education_activity & 1.00000 \nonumber\\
possible_separate & 1.00000 \nonumber\\
boy_from & 1.00000 \nonumber\\
ProductionRule_NP->ADVP,NP,CC,RB,NP, & 1.00000 \nonumber\\
some_good & 1.00000 \nonumber\\
question_that & 1.00000 \nonumber\\
that_farquhar & 1.00000 \nonumber\\
even_imagine & 1.00000 \nonumber\\
a_safe & 1.00000 \nonumber\\
turn_to & 1.00000 \nonumber\\
shell & 1.00000 \nonumber\\
everything_! & 1.00000 \nonumber\\
engine & 1.00000 \nonumber\\
firefox_can & 1.00000 \nonumber\\
firefox_shell & 1.00000 \nonumber\\
firefox_year & 1.00000 \nonumber\\
engine_in & 1.00000 \nonumber\\
the_innovation & 1.00000 \nonumber\\
in_e & 1.00000 \nonumber\\
plugin & 1.00000 \nonumber\\
nice_feature & 1.00000 \nonumber\\
plugin_so & 1.00000 \nonumber\\
also_plugin & 1.00000 \nonumber\\
more_plugin & 1.00000 \nonumber\\
e_7.0 & 1.00000 \nonumber\\
theme_be & 1.00000 \nonumber\\
theme & 1.00000 \nonumber\\
innovation_in & 1.00000 \nonumber\\
7.0 & 1.00000 \nonumber\\
the_theme & 1.00000 \nonumber\\
a_nice & 1.00000 \nonumber\\
explorer_engine & 1.00000 \nonumber\\
shell_. & 1.00000 \nonumber\\
plugin_and & 1.00000 \nonumber\\
7.0_be & 1.00000 \nonumber\\
be_garentee & 1.00000 \nonumber\\
garentee & 1.00000 \nonumber\\
garentee_safety & 1.00000 \nonumber\\
safe_source & 1.00000 \nonumber\\
be_easy & 1.00000 \nonumber\\
to_singapore & 1.00000 \nonumber\\
get_out & 1.00000 \nonumber\\
person_be & 1.00000 \nonumber\\
film & 1.00000 \nonumber\\
opinion_it & 1.00000 \nonumber\\
sport_. & 1.00000 \nonumber\\
without_him & 1.00000 \nonumber\\
,_rss & 1.00000 \nonumber\\
interface_, & 1.00000 \nonumber\\
still_catch & 1.00000 \nonumber\\
rss_support & 1.00000 \nonumber\\
firefox_imho & 1.00000 \nonumber\\
work_better & 1.00000 \nonumber\\
of_activex & 1.00000 \nonumber\\
rss & 1.00000 \nonumber\\
firefox_just & 1.00000 \nonumber\\
imho_. & 1.00000 \nonumber\\
to_still & 1.00000 \nonumber\\
ProductionRule_S->ADVP,,,NP,ADVP,VP,., & 1.00000 \nonumber\\
just_work & 1.00000 \nonumber\\
activex_, & 1.00000 \nonumber\\
catch_up & 1.00000 \nonumber\\
imho & 1.00000 \nonumber\\
tab_interface & 1.00000 \nonumber\\
idea_man & 1.00000 \nonumber\\
vision & 1.00000 \nonumber\\
wear_a & 1.00000 \nonumber\\
can_understand & 1.00000 \nonumber\\
ProductionRule_UCP->PP,CC,RB,SBAR, & 1.00000 \nonumber\\
_pos_ngram_O_NN_PR & 1.00000 \nonumber\\
(_it & 1.00000 \nonumber\\
champ & 1.00000 \nonumber\\
_pos_ngram_PR_PUNC_ADJ & 1.00000 \nonumber\\
to_happen & 1.00000 \nonumber\\
emotionally & 1.00000 \nonumber\\
whatever_work & 1.00000 \nonumber\\
ProductionRule_SBAR->WHNP,S,,, & 1.00000 \nonumber\\
that_whatever & 1.00000 \nonumber\\
when_, & 1.00000 \nonumber\\
n't_too & 1.00000 \nonumber\\
person_individually & 1.00000 \nonumber\\
definately_superior & 1.00000 \nonumber\\
be_definately & 1.00000 \nonumber\\
superior_to & 1.00000 \nonumber\\
about_: & 1.00000 \nonumber\\
laughable_7 & 1.00000 \nonumber\\
on_someone & 1.00000 \nonumber\\
many_good & 1.00000 \nonumber\\
would_i & 1.00000 \nonumber\\
update_. & 1.00000 \nonumber\\
someone_els & 1.00000 \nonumber\\
the_laughable & 1.00000 \nonumber\\
time_better & 1.00000 \nonumber\\
experience_it & 1.00000 \nonumber\\
;_d & 1.00000 \nonumber\\
multiple_time & 1.00000 \nonumber\\
explorer_. & 1.00000 \nonumber\\
the_config & 1.00000 \nonumber\\
extension_. & 1.00000 \nonumber\\
7_update & 1.00000 \nonumber\\
have_work & 1.00000 \nonumber\\
too_bid & 1.00000 \nonumber\\
especially_after & 1.00000 \nonumber\\
though_not & 1.00000 \nonumber\\
my_experience & 1.00000 \nonumber\\
els_computer & 1.00000 \nonumber\\
els & 1.00000 \nonumber\\
computer_? & 1.00000 \nonumber\\
config & 1.00000 \nonumber\\
config_be & 1.00000 \nonumber\\
config_know & 1.00000 \nonumber\\
best_, & 1.00000 \nonumber\\
laughable & 1.00000 \nonumber\\
good_extension & 1.00000 \nonumber\\
tab_be & 1.00000 \nonumber\\
:_config & 1.00000 \nonumber\\
individually_, & 1.00000 \nonumber\\
to_internet & 1.00000 \nonumber\\
._; & 1.00000 \nonumber\\
individually & 1.00000 \nonumber\\
work_for & 1.00000 \nonumber\\
work_multiple & 1.00000 \nonumber\\
would_muder & 1.00000 \nonumber\\
'_beside & 1.00000 \nonumber\\
muder_anyone & 1.00000 \nonumber\\
sombody_that & 1.00000 \nonumber\\
ever_marrie & 1.00000 \nonumber\\
muder & 1.00000 \nonumber\\
sombody & 1.00000 \nonumber\\
marrie_sombody & 1.00000 \nonumber\\
marrie & 1.00000 \nonumber\\
minister & 1.00000 \nonumber\\
wrong_, & 1.00000 \nonumber\\
a_drug & 1.00000 \nonumber\\
politician_, & 1.00000 \nonumber\\
strongly & 1.00000 \nonumber\\
i_strongly & 1.00000 \nonumber\\
-_why & 1.00000 \nonumber\\
new_life & 1.00000 \nonumber\\
alone_, & 1.00000 \nonumber\\
_pos_ngram_NP_PP_CARD & 1.00000 \nonumber\\
in_from & 1.00000 \nonumber\\
estimate_3,800 & 1.00000 \nonumber\\
atmosphere_. & 1.00000 \nonumber\\
in_californium & 1.00000 \nonumber\\
18_million & 1.00000 \nonumber\\
new_york & 1.00000 \nonumber\\
ProductionRule_NP->DT,VBN,CD,NNS, & 1.00000 \nonumber\\
york_city & 1.00000 \nonumber\\
release_an & 1.00000 \nonumber\\
york & 1.00000 \nonumber\\
warm_pollution & 1.00000 \nonumber\\
be_ship & 1.00000 \nonumber\\
city_alone & 1.00000 \nonumber\\
2,500_ton & 1.00000 \nonumber\\
in_new & 1.00000 \nonumber\\
the_atmosphere & 1.00000 \nonumber\\
from_fijus & 1.00000 \nonumber\\
,_18 & 1.00000 \nonumber\\
3,800 & 1.00000 \nonumber\\
fijus_in & 1.00000 \nonumber\\
3,800_ton & 1.00000 \nonumber\\
ship_in & 1.00000 \nonumber\\
transportation & 1.00000 \nonumber\\
from_western & 1.00000 \nonumber\\
californium_, & 1.00000 \nonumber\\
fijus & 1.00000 \nonumber\\
californium & 1.00000 \nonumber\\
about_2,500 & 1.00000 \nonumber\\
transportation_of & 1.00000 \nonumber\\
europe_release & 1.00000 \nonumber\\
an_estimate & 1.00000 \nonumber\\
2,500 & 1.00000 \nonumber\\
18 & 1.00000 \nonumber\\
produce_about & 1.00000 \nonumber\\
the_transportation & 1.00000 \nonumber\\
pollution_into & 1.00000 \nonumber\\
,_produce & 1.00000 \nonumber\\
mess & 1.00000 \nonumber\\
activex & 1.00000 \nonumber\\
not_disprove & 1.00000 \nonumber\\
religious_people & 1.00000 \nonumber\\
prove_something & 1.00000 \nonumber\\
!!!!_you & 1.00000 \nonumber\\
negative_. & 1.00000 \nonumber\\
alway_use & 1.00000 \nonumber\\
argument_: & 1.00000 \nonumber\\
disprove_a & 1.00000 \nonumber\\
exist_!!!! & 1.00000 \nonumber\\
prove_he & 1.00000 \nonumber\\
._mean & 1.00000 \nonumber\\
same_argument & 1.00000 \nonumber\\
_pos_ngram_NN_PR_NP & 1.00000 \nonumber\\
which_already & 1.00000 \nonumber\\
ProductionRule_NP->DT,VBG, & 1.00000 \nonumber\\
globally & 1.00000 \nonumber\\
water_industry & 1.00000 \nonumber\\
industry_have & 1.00000 \nonumber\\
clearly & 1.00000 \nonumber\\
no_and & 1.00000 \nonumber\\
both_side & 1.00000 \nonumber\\
morality & 1.00000 \nonumber\\
lie & 1.00000 \nonumber\\
could_give & 1.00000 \nonumber\\
mother_' & 1.00000 \nonumber\\
._3 & 1.00000 \nonumber\\
-_they & 1.00000 \nonumber\\
benefit_. & 1.00000 \nonumber\\
their_peer & 1.00000 \nonumber\\
peer & 1.00000 \nonumber\\
that_class & 1.00000 \nonumber\\
it_by & 1.00000 \nonumber\\
so_to & 1.00000 \nonumber\\
like_do & 1.00000 \nonumber\\
anit-abortionist & 1.00000 \nonumber\\
be_pro-death & 1.00000 \nonumber\\
most_anit-abortionist & 1.00000 \nonumber\\
anit-abortionist_be & 1.00000 \nonumber\\
law_for & 1.00000 \nonumber\\
older_white & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,NP,,,PP, & 1.00000 \nonumber\\
penalty_? & 1.00000 \nonumber\\
determine_if & 1.00000 \nonumber\\
she_want & 1.00000 \nonumber\\
anti-abortion & 1.00000 \nonumber\\
anti-abortion_law & 1.00000 \nonumber\\
white_man & 1.00000 \nonumber\\
mostly_older & 1.00000 \nonumber\\
who_should & 1.00000 \nonumber\\
pro-death & 1.00000 \nonumber\\
she_alone & 1.00000 \nonumber\\
jon & 1.00000 \nonumber\\
jon_jax & 1.00000 \nonumber\\
for_woman & 1.00000 \nonumber\\
to_establish & 1.00000 \nonumber\\
jax_71 & 1.00000 \nonumber\\
woman_? & 1.00000 \nonumber\\
any_stage & 1.00000 \nonumber\\
her_pregnancy & 1.00000 \nonumber\\
jax & 1.00000 \nonumber\\
ProductionRule_SBAR->IN,S,CC,RB, & 1.00000 \nonumber\\
pro-death_penalty & 1.00000 \nonumber\\
at_any & 1.00000 \nonumber\\
should_determine & 1.00000 \nonumber\\
?_jon & 1.00000 \nonumber\\
establish_anti-abortion & 1.00000 \nonumber\\
alone_be & 1.00000 \nonumber\\
ProductionRule_NP->NP,NNS, & 1.00000 \nonumber\\
course_. & 1.00000 \nonumber\\
class_be & 1.00000 \nonumber\\
profit & 1.00000 \nonumber\\
_pos_ngram_ART_CONJ_V & 1.00000 \nonumber\\
there_and & 1.00000 \nonumber\\
woman_it & 1.00000 \nonumber\\
realistically & 1.00000 \nonumber\\
base_the & 1.00000 \nonumber\\
bible_it & 1.00000 \nonumber\\
and_realistically & 1.00000 \nonumber\\
of_say & 1.00000 \nonumber\\
'_definitely & 1.00000 \nonumber\\
realistically_marriage & 1.00000 \nonumber\\
intend & 1.00000 \nonumber\\
intend_for & 1.00000 \nonumber\\
be_intend & 1.00000 \nonumber\\
develop_singapore & 1.00000 \nonumber\\
or_an & 1.00000 \nonumber\\
blow & 1.00000 \nonumber\\
destroy_the & 1.00000 \nonumber\\
of_which & 1.00000 \nonumber\\
blind_. & 1.00000 \nonumber\\
neighbor & 1.00000 \nonumber\\
from_these & 1.00000 \nonumber\\
theory_be & 1.00000 \nonumber\\
also_you & 1.00000 \nonumber\\
how_it & 1.00000 \nonumber\\
ProductionRule_VP->RB,S, & 1.00000 \nonumber\\
"_law & 1.00000 \nonumber\\
a_man/woman & 1.00000 \nonumber\\
public_accomodation & 1.00000 \nonumber\\
to_isolate & 1.00000 \nonumber\\
"_distinct & 1.00000 \nonumber\\
isolate & 1.00000 \nonumber\\
isolate_them & 1.00000 \nonumber\\
contemplate & 1.00000 \nonumber\\
contemplate_man/woman & 1.00000 \nonumber\\
homosexual_people & 1.00000 \nonumber\\
law_define & 1.00000 \nonumber\\
very_different & 1.00000 \nonumber\\
accomodation & 1.00000 \nonumber\\
accomodation_for & 1.00000 \nonumber\\
relationship_intelligently & 1.00000 \nonumber\\
relationship_do & 1.00000 \nonumber\\
law_require & 1.00000 \nonumber\\
separate_school & 1.00000 \nonumber\\
of_implication & 1.00000 \nonumber\\
require_separate & 1.00000 \nonumber\\
and_public & 1.00000 \nonumber\\
relationship_, & 1.00000 \nonumber\\
the_aggregate & 1.00000 \nonumber\\
aggregate_, & 1.00000 \nonumber\\
to_contemplate & 1.00000 \nonumber\\
"_separate & 1.00000 \nonumber\\
violate_" & 1.00000 \nonumber\\
man/woman_relationship & 1.00000 \nonumber\\
man/woman & 1.00000 \nonumber\\
propose_" & 1.00000 \nonumber\\
implication & 1.00000 \nonumber\\
woman/woman & 1.00000 \nonumber\\
ProductionRule_ADJP->``,JJ,CC,JJ, & 1.00000 \nonumber\\
would_violate & 1.00000 \nonumber\\
implication_than & 1.00000 \nonumber\\
distinct & 1.00000 \nonumber\\
define_marriage & 1.00000 \nonumber\\
equal_. & 1.00000 \nonumber\\
i_propose & 1.00000 \nonumber\\
but_equal & 1.00000 \nonumber\\
"_man/woman & 1.00000 \nonumber\\
different_set & 1.00000 \nonumber\\
aggregate & 1.00000 \nonumber\\
man/man & 1.00000 \nonumber\\
than_man/man & 1.00000 \nonumber\\
distinct_and & 1.00000 \nonumber\\
and_woman/woman & 1.00000 \nonumber\\
and_different & 1.00000 \nonumber\\
woman/woman_relationship & 1.00000 \nonumber\\
man/man_and & 1.00000 \nonumber\\
master & 1.00000 \nonumber\\
russell_peter & 1.00000 \nonumber\\
master_at & 1.00000 \nonumber\\
russell & 1.00000 \nonumber\\
fun_of & 1.00000 \nonumber\\
peter_be & 1.00000 \nonumber\\
peter & 1.00000 \nonumber\\
a_master & 1.00000 \nonumber\\
at_make & 1.00000 \nonumber\\
make_fun & 1.00000 \nonumber\\
_pos_ngram_NN_ADJ_ADV & 1.00000 \nonumber\\
nestle & 1.00000 \nonumber\\
better_, & 1.00000 \nonumber\\
see_singapore & 1.00000 \nonumber\\
his_visit & 1.00000 \nonumber\\
visit_to & 1.00000 \nonumber\\
to_singapore.this & 1.00000 \nonumber\\
before_farquhar & 1.00000 \nonumber\\
singapore_before & 1.00000 \nonumber\\
during_his & 1.00000 \nonumber\\
by_farquhar & 1.00000 \nonumber\\
be_follow & 1.00000 \nonumber\\
farquhar_make & 1.00000 \nonumber\\
farquhar_during & 1.00000 \nonumber\\
singapore.this_show & 1.00000 \nonumber\\
an_acomplice & 1.00000 \nonumber\\
ProductionRule_NP->NP,CC,CC,S, & 1.00000 \nonumber\\
would_break & 1.00000 \nonumber\\
acomplice_and & 1.00000 \nonumber\\
acomplice_be & 1.00000 \nonumber\\
the_murderer & 1.00000 \nonumber\\
_pos_ngram_CONJ_CONJ_V & 1.00000 \nonumber\\
murderer_and & 1.00000 \nonumber\\
many_episode & 1.00000 \nonumber\\
file_; & 1.00000 \nonumber\\
crazy_for & 1.00000 \nonumber\\
alway_involve & 1.00000 \nonumber\\
and_cold & 1.00000 \nonumber\\
alway_catch & 1.00000 \nonumber\\
the_acomplice & 1.00000 \nonumber\\
episode & 1.00000 \nonumber\\
episode_of & 1.00000 \nonumber\\
case_file & 1.00000 \nonumber\\
watch_many & 1.00000 \nonumber\\
acomplice & 1.00000 \nonumber\\
of_cop & 1.00000 \nonumber\\
cold_case & 1.00000 \nonumber\\
individual_that & 1.00000 \nonumber\\
me_so & 1.00000 \nonumber\\
cop_and & 1.00000 \nonumber\\
too_crazy & 1.00000 \nonumber\\
break_up & 1.00000 \nonumber\\
after_watch & 1.00000 \nonumber\\
ProductionRule_ADJP->RB,VBG, & 1.00000 \nonumber\\
rapidly & 1.00000 \nonumber\\
economy_indium & 1.00000 \nonumber\\
rapidly_grow & 1.00000 \nonumber\\
ProductionRule_FRAG->NP,S, & 1.00000 \nonumber\\
grow_population & 1.00000 \nonumber\\
china_to & 1.00000 \nonumber\\
in_line & 1.00000 \nonumber\\
power_of & 1.00000 \nonumber\\
greatest_economic & 1.00000 \nonumber\\
a_rapidly & 1.00000 \nonumber\\
ProductionRule_NP->DT,JJS,JJ,NNS, & 1.00000 \nonumber\\
line_with & 1.00000 \nonumber\\
economic_power & 1.00000 \nonumber\\
_pos_ngram_CARD_O_ART & 1.00000 \nonumber\\
to_spank & 1.00000 \nonumber\\
much_memory & 1.00000 \nonumber\\
i_wont & 1.00000 \nonumber\\
any_case & 1.00000 \nonumber\\
me_they & 1.00000 \nonumber\\
more_money & 1.00000 \nonumber\\
the_definition & 1.00000 \nonumber\\
mother_be & 1.00000 \nonumber\\
their_kid & 1.00000 \nonumber\\
think_common & 1.00000 \nonumber\\
decompose & 1.00000 \nonumber\\
that_pe & 1.00000 \nonumber\\
more_recent & 1.00000 \nonumber\\
the_old & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,RB,ADJP,SBAR, & 1.00000 \nonumber\\
and_also & 1.00000 \nonumber\\
of_defense & 1.00000 \nonumber\\
someone_or & 1.00000 \nonumber\\
some_circumstance & 1.00000 \nonumber\\
ProductionRule_VP->VB,UCP, & 1.00000 \nonumber\\
yes_but & 1.00000 \nonumber\\
pure_dislike & 1.00000 \nonumber\\
i_that & 1.00000 \nonumber\\
could_kill & 1.00000 \nonumber\\
dislike_or & 1.00000 \nonumber\\
ProductionRule_VP->VB,INTJ,PP, & 1.00000 \nonumber\\
that_cold & 1.00000 \nonumber\\
object_and & 1.00000 \nonumber\\
pure & 1.00000 \nonumber\\
circumstance_would & 1.00000 \nonumber\\
or_out & 1.00000 \nonumber\\
cold_could & 1.00000 \nonumber\\
a_pure & 1.00000 \nonumber\\
person_then & 1.00000 \nonumber\\
heartedly & 1.00000 \nonumber\\
heartedly_like & 1.00000 \nonumber\\
cold_heartedly & 1.00000 \nonumber\\
circumstance_i & 1.00000 \nonumber\\
ProductionRule_NP->DT,DT, & 1.00000 \nonumber\\
like_rape & 1.00000 \nonumber\\
another_circumstance & 1.00000 \nonumber\\
defense_or & 1.00000 \nonumber\\
'_that & 1.00000 \nonumber\\
a_no & 1.00000 \nonumber\\
kill_cold & 1.00000 \nonumber\\
for_money & 1.00000 \nonumber\\
,_object & 1.00000 \nonumber\\
because_someone & 1.00000 \nonumber\\
person_for & 1.00000 \nonumber\\
_pos_ngram_O_PP_CARD & 1.00000 \nonumber\\
exercise_. & 1.00000 \nonumber\\
during_those & 1.00000 \nonumber\\
market & 1.00000 \nonumber\\
ProductionRule_QP->IN,CD, & 1.00000 \nonumber\\
sometime_it & 1.00000 \nonumber\\
_pos_ngram_ADJ_PR_O & 1.00000 \nonumber\\
._religion & 1.00000 \nonumber\\
ProductionRule_VP->VBP,ADVP,ADVP, & 1.00000 \nonumber\\
yourself_be & 1.00000 \nonumber\\
for_more & 1.00000 \nonumber\\
treat & 1.00000 \nonumber\\
bottle_for & 1.00000 \nonumber\\
its_good & 1.00000 \nonumber\\
create_water & 1.00000 \nonumber\\
william_be & 1.00000 \nonumber\\
because_william & 1.00000 \nonumber\\
singapore_continue & 1.00000 \nonumber\\
to_govern & 1.00000 \nonumber\\
perish & 1.00000 \nonumber\\
without_william & 1.00000 \nonumber\\
perish_. & 1.00000 \nonumber\\
farquhar_singapore & 1.00000 \nonumber\\
,_singapore & 1.00000 \nonumber\\
govern_the & 1.00000 \nonumber\\
have_perish & 1.00000 \nonumber\\
govern_another & 1.00000 \nonumber\\
govern & 1.00000 \nonumber\\
than_tv & 1.00000 \nonumber\\
promise_to & 1.00000 \nonumber\\
suitable & 1.00000 \nonumber\\
da & 1.00000 \nonumber\\
odds & 1.00000 \nonumber\\
next_level & 1.00000 \nonumber\\
the_individual & 1.00000 \nonumber\\
line_anyway & 1.00000 \nonumber\\
dad_that & 1.00000 \nonumber\\
the_outcome & 1.00000 \nonumber\\
year_down & 1.00000 \nonumber\\
arent_go & 1.00000 \nonumber\\
because_odds & 1.00000 \nonumber\\
try_and & 1.00000 \nonumber\\
him_arent & 1.00000 \nonumber\\
and_him & 1.00000 \nonumber\\
a_dad & 1.00000 \nonumber\\
out_if & 1.00000 \nonumber\\
why_try & 1.00000 \nonumber\\
ProductionRule_VP->VBG,ADVP,S,,,ADVP,FRAG, & 1.00000 \nonumber\\
ProductionRule_VP->VB,CC,VB,S,SBAR, & 1.00000 \nonumber\\
outcome_be & 1.00000 \nonumber\\
arent & 1.00000 \nonumber\\
ProductionRule_VP->VBD,NP,NP,SBAR, & 1.00000 \nonumber\\
odds_be & 1.00000 \nonumber\\
around_because & 1.00000 \nonumber\\
talk_5 & 1.00000 \nonumber\\
ProductionRule_NP->PRP$,JJ,NNS, & 1.00000 \nonumber\\
be_most & 1.00000 \nonumber\\
unhealthy & 1.00000 \nonumber\\
finish_his & 1.00000 \nonumber\\
himself_when & 1.00000 \nonumber\\
he_provide & 1.00000 \nonumber\\
closely_with & 1.00000 \nonumber\\
provide_plan & 1.00000 \nonumber\\
when_his & 1.00000 \nonumber\\
,_idea & 1.00000 \nonumber\\
his_subordinate & 1.00000 \nonumber\\
ProductionRule_VP->VB,NP,PP,PP,SBAR, & 1.00000 \nonumber\\
in_action & 1.00000 \nonumber\\
population_to & 1.00000 \nonumber\\
subordinate_to & 1.00000 \nonumber\\
order_him & 1.00000 \nonumber\\
ProductionRule_VP->VB,ADVP,PP,S, & 1.00000 \nonumber\\
work_closely & 1.00000 \nonumber\\
hence_it & 1.00000 \nonumber\\
be_common & 1.00000 \nonumber\\
though_it & 1.00000 \nonumber\\
superior_order & 1.00000 \nonumber\\
closely & 1.00000 \nonumber\\
leave_his & 1.00000 \nonumber\\
by_himself & 1.00000 \nonumber\\
sense_for & 1.00000 \nonumber\\
beside_the & 1.00000 \nonumber\\
class_that & 1.00000 \nonumber\\
_pos_ngram_PUNC_ADJ_O & 1.00000 \nonumber\\
come_and & 1.00000 \nonumber\\
understand_that & 1.00000 \nonumber\\
no_child & 1.00000 \nonumber\\
other_as & 1.00000 \nonumber\\
mind_. & 1.00000 \nonumber\\
white & 1.00000 \nonumber\\
tool & 1.00000 \nonumber\\
_pos_ngram_PUNC_V_O & 1.00000 \nonumber\\
introduce & 1.00000 \nonumber\\
it_ca & 1.00000 \nonumber\\
difference_in & 1.00000 \nonumber\\
?_they & 1.00000 \nonumber\\
,_marriage & 1.00000 \nonumber\\
amendment & 1.00000 \nonumber\\
the_wrong & 1.00000 \nonumber\\
neither & 1.00000 \nonumber\\
care_if & 1.00000 \nonumber\\
stop_them & 1.00000 \nonumber\\
but_tv & 1.00000 \nonumber\\
_pos_ngram_CARD_PUNC_O & 1.00000 \nonumber\\
plastic_water & 1.00000 \nonumber\\
harmful_, & 1.00000 \nonumber\\
the_excess & 1.00000 \nonumber\\
helpful_. & 1.00000 \nonumber\\
and_50 & 1.00000 \nonumber\\
normal_person & 1.00000 \nonumber\\
could_understand & 1.00000 \nonumber\\
imagine_so & 1.00000 \nonumber\\
survey_have & 1.00000 \nonumber\\
person_can & 1.00000 \nonumber\\
or_spore & 1.00000 \nonumber\\
helpful_as & 1.00000 \nonumber\\
can_remember & 1.00000 \nonumber\\
be_harmful & 1.00000 \nonumber\\
spore_formation & 1.00000 \nonumber\\
eye_, & 1.00000 \nonumber\\
spore & 1.00000 \nonumber\\
mind_, & 1.00000 \nonumber\\
limit_or & 1.00000 \nonumber\\
have_read & 1.00000 \nonumber\\
or_harm & 1.00000 \nonumber\\
formation & 1.00000 \nonumber\\
formation_we & 1.00000 \nonumber\\
to_something & 1.00000 \nonumber\\
have_listen & 1.00000 \nonumber\\
listen_and & 1.00000 \nonumber\\
more_helpful & 1.00000 \nonumber\\
t.v._in & 1.00000 \nonumber\\
remember_10 & 1.00000 \nonumber\\
have_find & 1.00000 \nonumber\\
read_of & 1.00000 \nonumber\\
t.v._be & 1.00000 \nonumber\\
image_about & 1.00000 \nonumber\\
our_eye & 1.00000 \nonumber\\
of_bud & 1.00000 \nonumber\\
be_helpful & 1.00000 \nonumber\\
10_% & 1.00000 \nonumber\\
ProductionRule_VP->VB,RBR, & 1.00000 \nonumber\\
think_t.v. & 1.00000 \nonumber\\
explain_like & 1.00000 \nonumber\\
excess & 1.00000 \nonumber\\
the_animation & 1.00000 \nonumber\\
bud & 1.00000 \nonumber\\
bud_or & 1.00000 \nonumber\\
we_read & 1.00000 \nonumber\\
of_everything & 1.00000 \nonumber\\
bud_then & 1.00000 \nonumber\\
animation & 1.00000 \nonumber\\
the_you & 1.00000 \nonumber\\
as_concern & 1.00000 \nonumber\\
time_limit & 1.00000 \nonumber\\
so_t.v. & 1.00000 \nonumber\\
a_normal & 1.00000 \nonumber\\
concern_the & 1.00000 \nonumber\\
understand_better & 1.00000 \nonumber\\
animation_of & 1.00000 \nonumber\\
even_read & 1.00000 \nonumber\\
watch_t.v. & 1.00000 \nonumber\\
about_bud & 1.00000 \nonumber\\
excess_of & 1.00000 \nonumber\\
._survey & 1.00000 \nonumber\\
limit_, & 1.00000 \nonumber\\
same_mistake & 1.00000 \nonumber\\
'_all & 1.00000 \nonumber\\
ashame & 1.00000 \nonumber\\
more_. & 1.00000 \nonumber\\
have_ie & 1.00000 \nonumber\\
to_us & 1.00000 \nonumber\\
ProductionRule_FRAG->ADJP,:, & 1.00000 \nonumber\\
ProductionRule_PRN->NP,-RRB-, & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,NP,PRN, & 1.00000 \nonumber\\
entertainment_also & 1.00000 \nonumber\\
a_source & 1.00000 \nonumber\\
ProductionRule_ADJP->JJ,NN, & 1.00000 \nonumber\\
also_its & 1.00000 \nonumber\\
,_same & 1.00000 \nonumber\\
boyfriend & 1.00000 \nonumber\\
internet_explorer & 1.00000 \nonumber\\
explorer & 1.00000 \nonumber\\
respect_. & 1.00000 \nonumber\\
bottle_be & 1.00000 \nonumber\\
the_so-call & 1.00000 \nonumber\\
so-call & 1.00000 \nonumber\\
between_a & 1.00000 \nonumber\\
office_. & 1.00000 \nonumber\\
a_office & 1.00000 \nonumber\\
ProductionRule_S->NP,,,PP, & 1.00000 \nonumber\\
yr_own & 1.00000 \nonumber\\
yr_out & 1.00000 \nonumber\\
choose_yr & 1.00000 \nonumber\\
when_yr & 1.00000 \nonumber\\
or_high & 1.00000 \nonumber\\
college_or & 1.00000 \nonumber\\
of_college & 1.00000 \nonumber\\
want_the & 1.00000 \nonumber\\
explore & 1.00000 \nonumber\\
be_even & 1.00000 \nonumber\\
ok_for & 1.00000 \nonumber\\
only_come & 1.00000 \nonumber\\
main_reason & 1.00000 \nonumber\\
main & 1.00000 \nonumber\\
help_and & 1.00000 \nonumber\\
ProductionRule_NP->NNP,NNP,NNP,NNP,NNP, & 1.00000 \nonumber\\
growth_in & 1.00000 \nonumber\\
water_shortage & 1.00000 \nonumber\\
ProductionRule_VP->VBN,NP,PP,,,S, & 1.00000 \nonumber\\
consumer & 1.00000 \nonumber\\
farmer & 1.00000 \nonumber\\
farmer_. & 1.00000 \nonumber\\
every_gallon & 1.00000 \nonumber\\
the_growth & 1.00000 \nonumber\\
area_near & 1.00000 \nonumber\\
go_into & 1.00000 \nonumber\\
extraction_in & 1.00000 \nonumber\\
water_production & 1.00000 \nonumber\\
bottle_plant & 1.00000 \nonumber\\
purification & 1.00000 \nonumber\\
consumer_and & 1.00000 \nonumber\\
purification_process & 1.00000 \nonumber\\
have_increase & 1.00000 \nonumber\\
and_farmer & 1.00000 \nonumber\\
extraction & 1.00000 \nonumber\\
water_extraction & 1.00000 \nonumber\\
in_bottle & 1.00000 \nonumber\\
two_gallon & 1.00000 \nonumber\\
waste_in & 1.00000 \nonumber\\
shortage_that & 1.00000 \nonumber\\
plastic-make & 1.00000 \nonumber\\
plastic-make_process & 1.00000 \nonumber\\
nearby_consumer & 1.00000 \nonumber\\
the_plastic-make & 1.00000 \nonumber\\
the_million & 1.00000 \nonumber\\
the_purification & 1.00000 \nonumber\\
production_have & 1.00000 \nonumber\\
of_gallon & 1.00000 \nonumber\\
,_lead & 1.00000 \nonumber\\
,_two & 1.00000 \nonumber\\
near_bottle & 1.00000 \nonumber\\
to_water & 1.00000 \nonumber\\
that_affect & 1.00000 \nonumber\\
gallon_that & 1.00000 \nonumber\\
plant_, & 1.00000 \nonumber\\
affect_nearby & 1.00000 \nonumber\\
shortage & 1.00000 \nonumber\\
process_for & 1.00000 \nonumber\\
increase_water & 1.00000 \nonumber\\
yourself_" & 1.00000 \nonumber\\
ahead_in & 1.00000 \nonumber\\
be_river & 1.00000 \nonumber\\
be_same & 1.00000 \nonumber\\
ProductionRule_S->S,:,CC,S,., & 1.00000 \nonumber\\
prise & 1.00000 \nonumber\\
ProductionRule_VP->VBG,NP,ADVP,PP, & 1.00000 \nonumber\\
the_3rd & 1.00000 \nonumber\\
doctor & 1.00000 \nonumber\\
compare_my & 1.00000 \nonumber\\
lead_power & 1.00000 \nonumber\\
count_in & 1.00000 \nonumber\\
insult_yourself & 1.00000 \nonumber\\
the_lead & 1.00000 \nonumber\\
doctor_and & 1.00000 \nonumber\\
believe_anyone & 1.00000 \nonumber\\
compare_yourself & 1.00000 \nonumber\\
it_bring & 1.00000 \nonumber\\
but_time & 1.00000 \nonumber\\
yes_we & 1.00000 \nonumber\\
(_count & 1.00000 \nonumber\\
move_a & 1.00000 \nonumber\\
own_country & 1.00000 \nonumber\\
in_become & 1.00000 \nonumber\\
we_produce & 1.00000 \nonumber\\
concern_show & 1.00000 \nonumber\\
to_prise & 1.00000 \nonumber\\
bring_change & 1.00000 \nonumber\\
)_but & 1.00000 \nonumber\\
"_compare & 1.00000 \nonumber\\
or_weaker & 1.00000 \nonumber\\
most_no & 1.00000 \nonumber\\
than_us & 1.00000 \nonumber\\
as_napoleon & 1.00000 \nonumber\\
ourselve_because & 1.00000 \nonumber\\
and_engineer & 1.00000 \nonumber\\
a_step & 1.00000 \nonumber\\
namaste_!!!! & 1.00000 \nonumber\\
yourself_with & 1.00000 \nonumber\\
internal_problem & 1.00000 \nonumber\\
stronger_or & 1.00000 \nonumber\\
as_insult & 1.00000 \nonumber\\
namaste & 1.00000 \nonumber\\
everyday_.... & 1.00000 \nonumber\\
napoleon & 1.00000 \nonumber\\
napoleon_say & 1.00000 \nonumber\\
weaker_than & 1.00000 \nonumber\\
produce_most & 1.00000 \nonumber\\
!!!!!_namaste & 1.00000 \nonumber\\
problem_which & 1.00000 \nonumber\\
us_.... & 1.00000 \nonumber\\
prise_ourselve & 1.00000 \nonumber\\
show_by & 1.00000 \nonumber\\
of_doctor & 1.00000 \nonumber\\
anyone_be & 1.00000 \nonumber\\
we_grow & 1.00000 \nonumber\\
indium_move & 1.00000 \nonumber\\
still_we & 1.00000 \nonumber\\
...._!!!!! & 1.00000 \nonumber\\
engineer_every & 1.00000 \nonumber\\
country_) & 1.00000 \nonumber\\
all_..... & 1.00000 \nonumber\\
country_say & 1.00000 \nonumber\\
year_( & 1.00000 \nonumber\\
country_do & 1.00000 \nonumber\\
...._concern & 1.00000 \nonumber\\
some_internal & 1.00000 \nonumber\\
power_... & 1.00000 \nonumber\\
step_ahead & 1.00000 \nonumber\\
power_everyday & 1.00000 \nonumber\\
3rd_largest & 1.00000 \nonumber\\
river_water & 1.00000 \nonumber\\
"_we & 1.00000 \nonumber\\
moreover_we & 1.00000 \nonumber\\
watch_television & 1.00000 \nonumber\\
no_human & 1.00000 \nonumber\\
a_make & 1.00000 \nonumber\\
dark & 1.00000 \nonumber\\
believe_situation & 1.00000 \nonumber\\
dark_. & 1.00000 \nonumber\\
view_tv & 1.00000 \nonumber\\
television_in & 1.00000 \nonumber\\
or_book & 1.00000 \nonumber\\
be_can & 1.00000 \nonumber\\
any_medium & 1.00000 \nonumber\\
use_no & 1.00000 \nonumber\\
by_watch & 1.00000 \nonumber\\
can_create & 1.00000 \nonumber\\
waste_electricity & 1.00000 \nonumber\\
light_on & 1.00000 \nonumber\\
medium_. & 1.00000 \nonumber\\
medium & 1.00000 \nonumber\\
the_television & 1.00000 \nonumber\\
brain_be & 1.00000 \nonumber\\
which_also & 1.00000 \nonumber\\
tv_require & 1.00000 \nonumber\\
require_brain & 1.00000 \nonumber\\
need_the & 1.00000 \nonumber\\
save_, & 1.00000 \nonumber\\
the_dark & 1.00000 \nonumber\\
unless_the & 1.00000 \nonumber\\
they_? & 1.00000 \nonumber\\
understand_any & 1.00000 \nonumber\\
television_people & 1.00000 \nonumber\\
would_go & 1.00000 \nonumber\\
even_view & 1.00000 \nonumber\\
tv_or & 1.00000 \nonumber\\
"_even & 1.00000 \nonumber\\
make_believe & 1.00000 \nonumber\\
be_save & 1.00000 \nonumber\\
also_waste & 1.00000 \nonumber\\
leave_? & 1.00000 \nonumber\\
go_leave & 1.00000 \nonumber\\
and_moreover & 1.00000 \nonumber\\
other_feel & 1.00000 \nonumber\\
_pos_ngram_PP_PR_CARD & 1.00000 \nonumber\\
with_someone & 1.00000 \nonumber\\
market_, & 1.00000 \nonumber\\
feel_the & 1.00000 \nonumber\\
anything_else & 1.00000 \nonumber\\
situation_and & 1.00000 \nonumber\\
but_he & 1.00000 \nonumber\\
not_do & 1.00000 \nonumber\\
gay_couple & 1.00000 \nonumber\\
one_number & 1.00000 \nonumber\\
a_crazy & 1.00000 \nonumber\\
sleep_or & 1.00000 \nonumber\\
relieve_to & 1.00000 \nonumber\\
month_, & 1.00000 \nonumber\\
house_or & 1.00000 \nonumber\\
crazy_woman & 1.00000 \nonumber\\
number_one & 1.00000 \nonumber\\
and_relieve & 1.00000 \nonumber\\
for_murder & 1.00000 \nonumber\\
crime_in & 1.00000 \nonumber\\
or_think & 1.00000 \nonumber\\
relieve & 1.00000 \nonumber\\
or_sleep & 1.00000 \nonumber\\
think_right & 1.00000 \nonumber\\
safe_if & 1.00000 \nonumber\\
maybe_year & 1.00000 \nonumber\\
one_crime & 1.00000 \nonumber\\
._kill & 1.00000 \nonumber\\
stay_marry & 1.00000 \nonumber\\
feel_safe & 1.00000 \nonumber\\
for_month & 1.00000 \nonumber\\
wear_? & 1.00000 \nonumber\\
somebody_have & 1.00000 \nonumber\\
rare_. & 1.00000 \nonumber\\
smart_. & 1.00000 \nonumber\\
own_uniform & 1.00000 \nonumber\\
remember_every & 1.00000 \nonumber\\
same_and & 1.00000 \nonumber\\
follow_it & 1.00000 \nonumber\\
skirt_or & 1.00000 \nonumber\\
and_everybody & 1.00000 \nonumber\\
spend_quiet & 1.00000 \nonumber\\
everyone_think & 1.00000 \nonumber\\
i_though & 1.00000 \nonumber\\
morn_i & 1.00000 \nonumber\\
or_jeans & 1.00000 \nonumber\\
be_happen & 1.00000 \nonumber\\
have_really & 1.00000 \nonumber\\
though_what & 1.00000 \nonumber\\
have_own & 1.00000 \nonumber\\
,_smart & 1.00000 \nonumber\\
quiet_a & 1.00000 \nonumber\\
really_problem & 1.00000 \nonumber\\
quiet & 1.00000 \nonumber\\
really_nice & 1.00000 \nonumber\\
think_as & 1.00000 \nonumber\\
every_pupil & 1.00000 \nonumber\\
'_really & 1.00000 \nonumber\\
new_clothe & 1.00000 \nonumber\\
ask_my & 1.00000 \nonumber\\
envy_that & 1.00000 \nonumber\\
buy_new & 1.00000 \nonumber\\
nice_skirt & 1.00000 \nonumber\\
that_somebody & 1.00000 \nonumber\\
no_envy & 1.00000 \nonumber\\
jeans_. & 1.00000 \nonumber\\
school_have & 1.00000 \nonumber\\
happen_not & 1.00000 \nonumber\\
secondly_there & 1.00000 \nonumber\\
thing_!! & 1.00000 \nonumber\\
guilt & 1.00000 \nonumber\\
weird & 1.00000 \nonumber\\
corrupt & 1.00000 \nonumber\\
a_day & 1.00000 \nonumber\\
a_possibility & 1.00000 \nonumber\\
possibility & 1.00000 \nonumber\\
not_turn & 1.00000 \nonumber\\
the_ultimate & 1.00000 \nonumber\\
the_secret & 1.00000 \nonumber\\
not_see & 1.00000 \nonumber\\
economy_severely & 1.00000 \nonumber\\
and_nestle & 1.00000 \nonumber\\
ProductionRule_NP->VBG,JJ,NN, & 1.00000 \nonumber\\
and_purchase & 1.00000 \nonumber\\
would_leave & 1.00000 \nonumber\\
of_dollar & 1.00000 \nonumber\\
dasanus_and & 1.00000 \nonumber\\
american_use & 1.00000 \nonumber\\
,_ban & 1.00000 \nonumber\\
leave_hundred & 1.00000 \nonumber\\
use_and & 1.00000 \nonumber\\
severely_. & 1.00000 \nonumber\\
._million & 1.00000 \nonumber\\
purchase_water & 1.00000 \nonumber\\
corporation_like & 1.00000 \nonumber\\
loose_million & 1.00000 \nonumber\\
hurt_the & 1.00000 \nonumber\\
hurt_big & 1.00000 \nonumber\\
loose & 1.00000 \nonumber\\
without_job & 1.00000 \nonumber\\
of_american & 1.00000 \nonumber\\
like_dasanus & 1.00000 \nonumber\\
bottle_everyday & 1.00000 \nonumber\\
everyday_so & 1.00000 \nonumber\\
ban_them & 1.00000 \nonumber\\
big_corporation & 1.00000 \nonumber\\
people_without & 1.00000 \nonumber\\
._http://www.nestlewaterscorporate.com/bottled & 1.00000 \nonumber\\
economy_because & 1.00000 \nonumber\\
nestle_would & 1.00000 \nonumber\\
would_loose & 1.00000 \nonumber\\
corporation_. & 1.00000 \nonumber\\
only_hurt & 1.00000 \nonumber\\
dollar_. & 1.00000 \nonumber\\
ban_bottle & 1.00000 \nonumber\\
_pos_ngram_O_O_NP & 1.00000 \nonumber\\
scare_of & 1.00000 \nonumber\\
much_the & 1.00000 \nonumber\\
the_truth & 1.00000 \nonumber\\
them_which & 1.00000 \nonumber\\
your_point & 1.00000 \nonumber\\
dealer_all & 1.00000 \nonumber\\
frankly_, & 1.00000 \nonumber\\
home_and & 1.00000 \nonumber\\
a_fashion & 1.00000 \nonumber\\
go_? & 1.00000 \nonumber\\
from_go & 1.00000 \nonumber\\
kid_go & 1.00000 \nonumber\\
if_kid & 1.00000 \nonumber\\
district_have & 1.00000 \nonumber\\
frankly & 1.00000 \nonumber\\
of_individuality & 1.00000 \nonumber\\
and_drug & 1.00000 \nonumber\\
individuality_... & 1.00000 \nonumber\\
care_? & 1.00000 \nonumber\\
bull_. & 1.00000 \nonumber\\
after_school & 1.00000 \nonumber\\
ProductionRule_NP->NNS,CC,NN,NNS, & 1.00000 \nonumber\\
like_whore & 1.00000 \nonumber\\
them_from & 1.00000 \nonumber\\
place_these & 1.00000 \nonumber\\
..._who & 1.00000 \nonumber\\
go_home & 1.00000 \nonumber\\
learn_environment & 1.00000 \nonumber\\
a_night & 1.00000 \nonumber\\
night_club & 1.00000 \nonumber\\
whore & 1.00000 \nonumber\\
clothe_after & 1.00000 \nonumber\\
club_. & 1.00000 \nonumber\\
school_the & 1.00000 \nonumber\\
only_place & 1.00000 \nonumber\\
school_job & 1.00000 \nonumber\\
since_a & 1.00000 \nonumber\\
these_kid & 1.00000 \nonumber\\
"_express & 1.00000 \nonumber\\
to_such & 1.00000 \nonumber\\
whore_and & 1.00000 \nonumber\\
"_school & 1.00000 \nonumber\\
dress_like & 1.00000 \nonumber\\
time_then & 1.00000 \nonumber\\
different_clothe & 1.00000 \nonumber\\
be_stop & 1.00000 \nonumber\\
fashion_show & 1.00000 \nonumber\\
club & 1.00000 \nonumber\\
n't_dress & 1.00000 \nonumber\\
_pos_ngram_NP_NP_CARD & 1.00000 \nonumber\\
for_thousand & 1.00000 \nonumber\\
nothing_for & 1.00000 \nonumber\\
as_their & 1.00000 \nonumber\\
to_admit & 1.00000 \nonumber\\
observation & 1.00000 \nonumber\\
kill_you & 1.00000 \nonumber\\
to_prove & 1.00000 \nonumber\\
school_day & 1.00000 \nonumber\\
school_' & 1.00000 \nonumber\\
with_other & 1.00000 \nonumber\\
have_fun & 1.00000 \nonumber\\
there_will & 1.00000 \nonumber\\
pray & 1.00000 \nonumber\\
and_indium & 1.00000 \nonumber\\
ProductionRule_ADVP->NP,IN, & 1.00000 \nonumber\\
money_case & 1.00000 \nonumber\\
be_involve & 1.00000 \nonumber\\
e.g. & 1.00000 \nonumber\\
in_black & 1.00000 \nonumber\\
the_politian & 1.00000 \nonumber\\
useless_topic & 1.00000 \nonumber\\
gain_or & 1.00000 \nonumber\\
._e.g. & 1.00000 \nonumber\\
e.g._, & 1.00000 \nonumber\\
politian_of & 1.00000 \nonumber\\
or_earn & 1.00000 \nonumber\\
politian_say & 1.00000 \nonumber\\
they_alway & 1.00000 \nonumber\\
something_about & 1.00000 \nonumber\\
not_ready & 1.00000 \nonumber\\
politian_, & 1.00000 \nonumber\\
of_useless & 1.00000 \nonumber\\
)_the & 1.00000 \nonumber\\
a_politian & 1.00000 \nonumber\\
big_issue & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,RB,ADJP,S, & 1.00000 \nonumber\\
black_money & 1.00000 \nonumber\\
politian & 1.00000 \nonumber\\
issue_of & 1.00000 \nonumber\\
many_reason & 1.00000 \nonumber\\
alway_try & 1.00000 \nonumber\\
)_they & 1.00000 \nonumber\\
another_politian & 1.00000 \nonumber\\
a_chance & 1.00000 \nonumber\\
to_firefox & 1.00000 \nonumber\\
_pos_ngram_NP_ART_NN & 1.00000 \nonumber\\
i_thank & 1.00000 \nonumber\\
the_tv & 1.00000 \nonumber\\
watch_add & 1.00000 \nonumber\\
more_from & 1.00000 \nonumber\\
influence_to & 1.00000 \nonumber\\
from_book & 1.00000 \nonumber\\
parent_do & 1.00000 \nonumber\\
thank & 1.00000 \nonumber\\
tv_kid & 1.00000 \nonumber\\
thank_book & 1.00000 \nonumber\\
what_there & 1.00000 \nonumber\\
child_watch & 1.00000 \nonumber\\
most_parent & 1.00000 \nonumber\\
add_influence & 1.00000 \nonumber\\
kid_watch & 1.00000 \nonumber\\
grave & 1.00000 \nonumber\\
ProductionRule_VP->ADVP,VBD,NP,PRT, & 1.00000 \nonumber\\
live_scare & 1.00000 \nonumber\\
too_because & 1.00000 \nonumber\\
anyone_, & 1.00000 \nonumber\\
or_kill & 1.00000 \nonumber\\
_pos_ngram_PUNC_CONJ_CONJ & 1.00000 \nonumber\\
of_not & 1.00000 \nonumber\\
never_tell & 1.00000 \nonumber\\
should_commit & 1.00000 \nonumber\\
plus_she & 1.00000 \nonumber\\
tell_. & 1.00000 \nonumber\\
definetly_turn & 1.00000 \nonumber\\
be_arrest & 1.00000 \nonumber\\
would_find & 1.00000 \nonumber\\
scare_in & 1.00000 \nonumber\\
eventually_would & 1.00000 \nonumber\\
out_about & 1.00000 \nonumber\\
would_definetly & 1.00000 \nonumber\\
arrest_too & 1.00000 \nonumber\\
own_house & 1.00000 \nonumber\\
her_never & 1.00000 \nonumber\\
life_easier & 1.00000 \nonumber\\
rather_preffer & 1.00000 \nonumber\\
someone_eventually & 1.00000 \nonumber\\
preffer_her & 1.00000 \nonumber\\
her_kill & 1.00000 \nonumber\\
she_might & 1.00000 \nonumber\\
preffer & 1.00000 \nonumber\\
have_their & 1.00000 \nonumber\\
can_talk & 1.00000 \nonumber\\
because_their & 1.00000 \nonumber\\
pass_my & 1.00000 \nonumber\\
the_ppl & 1.00000 \nonumber\\
den_b & 1.00000 \nonumber\\
ProductionRule_ADJP->NN,RB, & 1.00000 \nonumber\\
dem_bt & 1.00000 \nonumber\\
dem & 1.00000 \nonumber\\
ppl_cant & 1.00000 \nonumber\\
school_textbook & 1.00000 \nonumber\\
ProductionRule_WHNP->NP,PP, & 1.00000 \nonumber\\
who_cant & 1.00000 \nonumber\\
b_for & 1.00000 \nonumber\\
actually_sometime & 1.00000 \nonumber\\
nd_even & 1.00000 \nonumber\\
away_frm & 1.00000 \nonumber\\
speak_skill & 1.00000 \nonumber\\
book_all & 1.00000 \nonumber\\
a_chapter & 1.00000 \nonumber\\
by_read & 1.00000 \nonumber\\
tv_nd & 1.00000 \nonumber\\
frm_dem & 1.00000 \nonumber\\
frm_any & 1.00000 \nonumber\\
read_wud & 1.00000 \nonumber\\
textbook & 1.00000 \nonumber\\
frm & 1.00000 \nonumber\\
textbook_nd & 1.00000 \nonumber\\
2_news & 1.00000 \nonumber\\
wud_alway & 1.00000 \nonumber\\
nd_at & 1.00000 \nonumber\\
read_be & 1.00000 \nonumber\\
channel_hence & 1.00000 \nonumber\\
ProductionRule_VP->VB,NP,ADVP,ADVP, & 1.00000 \nonumber\\
chapter & 1.00000 \nonumber\\
chapter_frm & 1.00000 \nonumber\\
my_time & 1.00000 \nonumber\\
improve_my & 1.00000 \nonumber\\
for_best & 1.00000 \nonumber\\
hence_by & 1.00000 \nonumber\\
nd_b & 1.00000 \nonumber\\
bore_( & 1.00000 \nonumber\\
day_become & 1.00000 \nonumber\\
day_bt & 1.00000 \nonumber\\
my_speak & 1.00000 \nonumber\\
feel_read & 1.00000 \nonumber\\
best_i & 1.00000 \nonumber\\
even_pass & 1.00000 \nonumber\\
home_novel & 1.00000 \nonumber\\
best_so & 1.00000 \nonumber\\
only_sometime & 1.00000 \nonumber\\
bt_even & 1.00000 \nonumber\\
alway_run & 1.00000 \nonumber\\
become_bore & 1.00000 \nonumber\\
ProductionRule_NP->SQ,VP, & 1.00000 \nonumber\\
some_ppl & 1.00000 \nonumber\\
da_best & 1.00000 \nonumber\\
nd_dat & 1.00000 \nonumber\\
time_nd & 1.00000 \nonumber\\
cant_sleep & 1.00000 \nonumber\\
novel_each & 1.00000 \nonumber\\
novel_) & 1.00000 \nonumber\\
absolutely_idiotic & 1.00000 \nonumber\\
dat_2 & 1.00000 \nonumber\\
novel & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,NP,ADVP,ADVP, & 1.00000 \nonumber\\
be_absolutely & 1.00000 \nonumber\\
bt_actually & 1.00000 \nonumber\\
sleep_if & 1.00000 \nonumber\\
ProductionRule_VP->VBP,NP,PP,SBAR, & 1.00000 \nonumber\\
ProductionRule_SQ->VP,NP,NP, & 1.00000 \nonumber\\
book_i & 1.00000 \nonumber\\
book_nd & 1.00000 \nonumber\\
r_da & 1.00000 \nonumber\\
any_novel & 1.00000 \nonumber\\
news_channel & 1.00000 \nonumber\\
so_only & 1.00000 \nonumber\\
even_den & 1.00000 \nonumber\\
even_improve & 1.00000 \nonumber\\
wont_read & 1.00000 \nonumber\\
ppl_who & 1.00000 \nonumber\\
nake & 1.00000 \nonumber\\
me_when & 1.00000 \nonumber\\
ProductionRule_VP->NN,NP, & 1.00000 \nonumber\\
_pos_ngram_PUNC_CARD_CARD & 1.00000 \nonumber\\
day_they & 1.00000 \nonumber\\
possibility_that & 1.00000 \nonumber\\
no_need & 1.00000 \nonumber\\
have_too & 1.00000 \nonumber\\
you_what & 1.00000 \nonumber\\
everyone_else & 1.00000 \nonumber\\
but_what & 1.00000 \nonumber\\
stronger_and & 1.00000 \nonumber\\
affection & 1.00000 \nonumber\\
doesnt_want & 1.00000 \nonumber\\
decent_. & 1.00000 \nonumber\\
body_that & 1.00000 \nonumber\\
will_cover & 1.00000 \nonumber\\
decent & 1.00000 \nonumber\\
be_decent & 1.00000 \nonumber\\
uniform_will & 1.00000 \nonumber\\
cover_every & 1.00000 \nonumber\\
every_part & 1.00000 \nonumber\\
for_wear & 1.00000 \nonumber\\
cauntious_about & 1.00000 \nonumber\\
school_doesnt & 1.00000 \nonumber\\
show_and & 1.00000 \nonumber\\
student_would & 1.00000 \nonumber\\
cauntious & 1.00000 \nonumber\\
be_cauntious & 1.00000 \nonumber\\
of_7 & 1.00000 \nonumber\\
speak & 1.00000 \nonumber\\
it_easier & 1.00000 \nonumber\\
singapore_after & 1.00000 \nonumber\\
fire_? & 1.00000 \nonumber\\
certain_position & 1.00000 \nonumber\\
,_effort & 1.00000 \nonumber\\
about_do & 1.00000 \nonumber\\
after_he & 1.00000 \nonumber\\
as_time & 1.00000 \nonumber\\
if_then & 1.00000 \nonumber\\
)_he & 1.00000 \nonumber\\
else_if & 1.00000 \nonumber\\
invest_. & 1.00000 \nonumber\\
a_boss & 1.00000 \nonumber\\
all_invest & 1.00000 \nonumber\\
,_money & 1.00000 \nonumber\\
raffle_) & 1.00000 \nonumber\\
go_about & 1.00000 \nonumber\\
farquhar_help & 1.00000 \nonumber\\
follow_raffle & 1.00000 \nonumber\\
effort_be & 1.00000 \nonumber\\
again_you & 1.00000 \nonumber\\
(_raffle & 1.00000 \nonumber\\
founder_as & 1.00000 \nonumber\\
cant_farquhar & 1.00000 \nonumber\\
boss_! & 1.00000 \nonumber\\
know_people & 1.00000 \nonumber\\
cause_many & 1.00000 \nonumber\\
with_no & 1.00000 \nonumber\\
sometime_you & 1.00000 \nonumber\\
alway_think & 1.00000 \nonumber\\
he_invite & 1.00000 \nonumber\\
john & 1.00000 \nonumber\\
ProductionRule_NP->NNP,NNP,POS, & 1.00000 \nonumber\\
malacca_to & 1.00000 \nonumber\\
st._john & 1.00000 \nonumber\\
by_about & 1.00000 \nonumber\\
the_trade & 1.00000 \nonumber\\
'_island & 1.00000 \nonumber\\
inform_the & 1.00000 \nonumber\\
office_at & 1.00000 \nonumber\\
immigrant & 1.00000 \nonumber\\
island_to & 1.00000 \nonumber\\
inform & 1.00000 \nonumber\\
trade_ship & 1.00000 \nonumber\\
the_immigrant & 1.00000 \nonumber\\
settlement_in & 1.00000 \nonumber\\
from_malacca & 1.00000 \nonumber\\
pass_by & 1.00000 \nonumber\\
to_inform & 1.00000 \nonumber\\
john_' & 1.00000 \nonumber\\
st. & 1.00000 \nonumber\\
ship_pass & 1.00000 \nonumber\\
at_st. & 1.00000 \nonumber\\
station & 1.00000 \nonumber\\
and_station & 1.00000 \nonumber\\
immigrant_from & 1.00000 \nonumber\\
station_an & 1.00000 \nonumber\\
and_trade & 1.00000 \nonumber\\
an_office & 1.00000 \nonumber\\
firefox_be & 1.00000 \nonumber\\
wife_be & 1.00000 \nonumber\\
found_singapore & 1.00000 \nonumber\\
selfish & 1.00000 \nonumber\\
environment_, & 1.00000 \nonumber\\
adjust & 1.00000 \nonumber\\
road_with & 1.00000 \nonumber\\
share_, & 1.00000 \nonumber\\
._ask & 1.00000 \nonumber\\
ask_a & 1.00000 \nonumber\\
christianity_however & 1.00000 \nonumber\\
different_kind & 1.00000 \nonumber\\
adjust_their & 1.00000 \nonumber\\
force_or & 1.00000 \nonumber\\
i_compare & 1.00000 \nonumber\\
compare_it & 1.00000 \nonumber\\
solidarity_. & 1.00000 \nonumber\\
pretty_clear & 1.00000 \nonumber\\
find_one & 1.00000 \nonumber\\
religion_to & 1.00000 \nonumber\\
christian_share & 1.00000 \nonumber\\
more_scientific & 1.00000 \nonumber\\
not_one & 1.00000 \nonumber\\
atheïsm & 1.00000 \nonumber\\
sideway_to & 1.00000 \nonumber\\
scientific_, & 1.00000 \nonumber\\
firstly_because & 1.00000 \nonumber\\
higher_force & 1.00000 \nonumber\\
it_lack & 1.00000 \nonumber\\
question_about & 1.00000 \nonumber\\
with_atheïsm & 1.00000 \nonumber\\
about_religion & 1.00000 \nonumber\\
lack_solidarity & 1.00000 \nonumber\\
a_higher & 1.00000 \nonumber\\
belief_that & 1.00000 \nonumber\\
atheïsm_, & 1.00000 \nonumber\\
solidarity & 1.00000 \nonumber\\
know_exactly & 1.00000 \nonumber\\
exactly_if & 1.00000 \nonumber\\
of_sideway & 1.00000 \nonumber\\
the_concept & 1.00000 \nonumber\\
to_adjust & 1.00000 \nonumber\\
sideway & 1.00000 \nonumber\\
those_sideway & 1.00000 \nonumber\\
sideway_. & 1.00000 \nonumber\\
and_lot & 1.00000 \nonumber\\
every_christian & 1.00000 \nonumber\\
one_belief & 1.00000 \nonumber\\
_pos_ngram_NP_PUNC_PUNC & 1.00000 \nonumber\\
to_send & 1.00000 \nonumber\\
off_than & 1.00000 \nonumber\\
think_parent & 1.00000 \nonumber\\
choose_atheism & 1.00000 \nonumber\\
to_soothe & 1.00000 \nonumber\\
soothe_my & 1.00000 \nonumber\\
atheism_over & 1.00000 \nonumber\\
never_answer & 1.00000 \nonumber\\
soothe & 1.00000 \nonumber\\
not_enough & 1.00000 \nonumber\\
enough_evidence & 1.00000 \nonumber\\
respect_and & 1.00000 \nonumber\\
curiosity & 1.00000 \nonumber\\
this_turn & 1.00000 \nonumber\\
curiosity_. & 1.00000 \nonumber\\
much_spam & 1.00000 \nonumber\\
ProductionRule_VP->VBP,ADJP,S, & 1.00000 \nonumber\\
my_curiosity & 1.00000 \nonumber\\
many_question & 1.00000 \nonumber\\
christianity_raise & 1.00000 \nonumber\\
little_respect & 1.00000 \nonumber\\
spam_. & 1.00000 \nonumber\\
raise_too & 1.00000 \nonumber\\
sad_to & 1.00000 \nonumber\\
so_little & 1.00000 \nonumber\\
although_, & 1.00000 \nonumber\\
abortion_in & 1.00000 \nonumber\\
of_convenience & 1.00000 \nonumber\\
behind_me & 1.00000 \nonumber\\
n't_kid & 1.00000 \nonumber\\
trail & 1.00000 \nonumber\\
leave_a & 1.00000 \nonumber\\
convenience_. & 1.00000 \nonumber\\
kid_yourself & 1.00000 \nonumber\\
convenience & 1.00000 \nonumber\\
trail_of & 1.00000 \nonumber\\
someone_anytime & 1.00000 \nonumber\\
be_inconvenient & 1.00000 \nonumber\\
vast & 1.00000 \nonumber\\
body_behind & 1.00000 \nonumber\\
walk_down & 1.00000 \nonumber\\
i_walk & 1.00000 \nonumber\\
inconvenient & 1.00000 \nonumber\\
anytime_they & 1.00000 \nonumber\\
the_vast & 1.00000 \nonumber\\
inconvenient_to & 1.00000 \nonumber\\
of_body & 1.00000 \nonumber\\
street_. & 1.00000 \nonumber\\
a_trail & 1.00000 \nonumber\\
reason_of & 1.00000 \nonumber\\
vast_majority & 1.00000 \nonumber\\
yourself_: & 1.00000 \nonumber\\
ProductionRule_NP->PRP,:,SBAR, & 1.00000 \nonumber\\
one_and & 1.00000 \nonumber\\
choice_to & 1.00000 \nonumber\\
their_clothe & 1.00000 \nonumber\\
house_, & 1.00000 \nonumber\\
id & 1.00000 \nonumber\\
east_indium & 1.00000 \nonumber\\
on_february & 1.00000 \nonumber\\
southern & 1.00000 \nonumber\\
behalf_of & 1.00000 \nonumber\\
agreement_with & 1.00000 \nonumber\\
sultan_of & 1.00000 \nonumber\\
indium_company & 1.00000 \nonumber\\
he_sign & 1.00000 \nonumber\\
location_of & 1.00000 \nonumber\\
1819_to & 1.00000 \nonumber\\
on_behalf & 1.00000 \nonumber\\
good_location & 1.00000 \nonumber\\
on_28 & 1.00000 \nonumber\\
january & 1.00000 \nonumber\\
january_1819 & 1.00000 \nonumber\\
a_agreement & 1.00000 \nonumber\\
post_and & 1.00000 \nonumber\\
trade_post & 1.00000 \nonumber\\
_pos_ngram_NP_CARD_PP & 1.00000 \nonumber\\
southern_part & 1.00000 \nonumber\\
and_settlement & 1.00000 \nonumber\\
the_southern & 1.00000 \nonumber\\
british_east & 1.00000 \nonumber\\
british_trade & 1.00000 \nonumber\\
agreement & 1.00000 \nonumber\\
johor & 1.00000 \nonumber\\
of_johor & 1.00000 \nonumber\\
28_january & 1.00000 \nonumber\\
johor_on & 1.00000 \nonumber\\
1819_, & 1.00000 \nonumber\\
company_on & 1.00000 \nonumber\\
economic_policy & 1.00000 \nonumber\\
investor & 1.00000 \nonumber\\
economic_agenda & 1.00000 \nonumber\\
print_san & 1.00000 \nonumber\\
print & 1.00000 \nonumber\\
regards & 1.00000 \nonumber\\
poster & 1.00000 \nonumber\\
poster_print & 1.00000 \nonumber\\
effective_economic & 1.00000 \nonumber\\
policy_to & 1.00000 \nonumber\\
regards_, & 1.00000 \nonumber\\
agenda & 1.00000 \nonumber\\
and_effective & 1.00000 \nonumber\\
jerwin & 1.00000 \nonumber\\
agenda_. & 1.00000 \nonumber\\
._regards & 1.00000 \nonumber\\
consultant & 1.00000 \nonumber\\
consultant_of & 1.00000 \nonumber\\
san_francisco & 1.00000 \nonumber\\
francisco & 1.00000 \nonumber\\
their_economic & 1.00000 \nonumber\\
san & 1.00000 \nonumber\\
manage_the & 1.00000 \nonumber\\
"_consultant & 1.00000 \nonumber\\
positive_and & 1.00000 \nonumber\\
promote_their & 1.00000 \nonumber\\
their_tourism & 1.00000 \nonumber\\
,_jerwin & 1.00000 \nonumber\\
francisco_" & 1.00000 \nonumber\\
true_if & 1.00000 \nonumber\\
the_positive & 1.00000 \nonumber\\
to_every & 1.00000 \nonumber\\
of_poster & 1.00000 \nonumber\\
investor_and & 1.00000 \nonumber\\
they_continue & 1.00000 \nonumber\\
every_investor & 1.00000 \nonumber\\
jerwin_" & 1.00000 \nonumber\\
tourism_. & 1.00000 \nonumber\\
throughout & 1.00000 \nonumber\\
for_raffle & 1.00000 \nonumber\\
be_mostly & 1.00000 \nonumber\\
could_probably & 1.00000 \nonumber\\
faster_if & 1.00000 \nonumber\\
person_rather & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,ADJP,PP,,,SBAR, & 1.00000 \nonumber\\
deep_into & 1.00000 \nonumber\\
just_mean & 1.00000 \nonumber\\
hard_as & 1.00000 \nonumber\\
but_stand & 1.00000 \nonumber\\
dig_yourself & 1.00000 \nonumber\\
dig_faster & 1.00000 \nonumber\\
hole_as & 1.00000 \nonumber\\
._advance & 1.00000 \nonumber\\
many_, & 1.00000 \nonumber\\
as_hard & 1.00000 \nonumber\\
stand_as & 1.00000 \nonumber\\
than_many & 1.00000 \nonumber\\
probably_dig & 1.00000 \nonumber\\
to_dig & 1.00000 \nonumber\\
be_inequal & 1.00000 \nonumber\\
inequal_. & 1.00000 \nonumber\\
own_action & 1.00000 \nonumber\\
inequal & 1.00000 \nonumber\\
would_for & 1.00000 \nonumber\\
as_deep & 1.00000 \nonumber\\
them_right & 1.00000 \nonumber\\
job_for & 1.00000 \nonumber\\
be_call & 1.00000 \nonumber\\
because_every & 1.00000 \nonumber\\
other_it & 1.00000 \nonumber\\
catch_for & 1.00000 \nonumber\\
murderer_. & 1.00000 \nonumber\\
get_hit & 1.00000 \nonumber\\
punishment_you & 1.00000 \nonumber\\
at_something & 1.00000 \nonumber\\
something_, & 1.00000 \nonumber\\
unless_they & 1.00000 \nonumber\\
some_sort & 1.00000 \nonumber\\
,_material & 1.00000 \nonumber\\
ask_someone & 1.00000 \nonumber\\
service_hour & 1.00000 \nonumber\\
get_some & 1.00000 \nonumber\\
they_community & 1.00000 \nonumber\\
a_venture & 1.00000 \nonumber\\
people_unless & 1.00000 \nonumber\\
hour_, & 1.00000 \nonumber\\
something_along & 1.00000 \nonumber\\
people_around & 1.00000 \nonumber\\
when_ask & 1.00000 \nonumber\\
importance_. & 1.00000 \nonumber\\
along_the & 1.00000 \nonumber\\
ultimately_, & 1.00000 \nonumber\\
ultimately & 1.00000 \nonumber\\
ProductionRule_VP->VBP,PP,ADVP,PP, & 1.00000 \nonumber\\
satisfaction & 1.00000 \nonumber\\
someone_why & 1.00000 \nonumber\\
purely_for & 1.00000 \nonumber\\
it_whether & 1.00000 \nonumber\\
out_other & 1.00000 \nonumber\\
reward_, & 1.00000 \nonumber\\
yourself_or & 1.00000 \nonumber\\
material_reward & 1.00000 \nonumber\\
"_ultimately & 1.00000 \nonumber\\
venture & 1.00000 \nonumber\\
venture_purely & 1.00000 \nonumber\\
up_affect & 1.00000 \nonumber\\
out_people & 1.00000 \nonumber\\
have_importance & 1.00000 \nonumber\\
satisfaction_out & 1.00000 \nonumber\\
the_response & 1.00000 \nonumber\\
satisfaction_of & 1.00000 \nonumber\\
of_satisfaction & 1.00000 \nonumber\\
good_as & 1.00000 \nonumber\\
the_satisfaction & 1.00000 \nonumber\\
affect_the & 1.00000 \nonumber\\
response & 1.00000 \nonumber\\
still_end & 1.00000 \nonumber\\
sort_of & 1.00000 \nonumber\\
response_would & 1.00000 \nonumber\\
_pos_ngram_PR_NP_V & 1.00000 \nonumber\\
logo & 1.00000 \nonumber\\
an_emergency & 1.00000 \nonumber\\
education_should & 1.00000 \nonumber\\
grow_exponentially & 1.00000 \nonumber\\
ten & 1.00000 \nonumber\\
create_its & 1.00000 \nonumber\\
growth_have & 1.00000 \nonumber\\
consumption_have & 1.00000 \nonumber\\
exponentially & 1.00000 \nonumber\\
exponentially_over & 1.00000 \nonumber\\
globally_, & 1.00000 \nonumber\\
_pos_ngram_ADJ_CARD_PP & 1.00000 \nonumber\\
water_consumption & 1.00000 \nonumber\\
american_industry & 1.00000 \nonumber\\
water_culture & 1.00000 \nonumber\\
past_ten & 1.00000 \nonumber\\
own_water & 1.00000 \nonumber\\
its_own & 1.00000 \nonumber\\
fifteen & 1.00000 \nonumber\\
culture_which & 1.00000 \nonumber\\
fifteen_year & 1.00000 \nonumber\\
to_fifteen & 1.00000 \nonumber\\
europe_and & 1.00000 \nonumber\\
north_america & 1.00000 \nonumber\\
industry_. & 1.00000 \nonumber\\
but_particularly & 1.00000 \nonumber\\
literally_create & 1.00000 \nonumber\\
north & 1.00000 \nonumber\\
have_literally & 1.00000 \nonumber\\
for_american & 1.00000 \nonumber\\
this_growth & 1.00000 \nonumber\\
take_place & 1.00000 \nonumber\\
place_globally & 1.00000 \nonumber\\
and_north & 1.00000 \nonumber\\
ten_to & 1.00000 \nonumber\\
particularly & 1.00000 \nonumber\\
ProductionRule_VP->VBN,ADVP,PP,PP, & 1.00000 \nonumber\\
particularly_in & 1.00000 \nonumber\\
it_really & 1.00000 \nonumber\\
ModalVerbShall & 1.00000 \nonumber\\
a_road & 1.00000 \nonumber\\
barely_grow & 1.00000 \nonumber\\
still_try & 1.00000 \nonumber\\
really_understand & 1.00000 \nonumber\\
do_since & 1.00000 \nonumber\\
for_. & 1.00000 \nonumber\\
take_you & 1.00000 \nonumber\\
might_break & 1.00000 \nonumber\\
cop_might & 1.00000 \nonumber\\
affiliate & 1.00000 \nonumber\\
affiliate_with & 1.00000 \nonumber\\
for_affiliate & 1.00000 \nonumber\\
these_reason & 1.00000 \nonumber\\
stress_about & 1.00000 \nonumber\\
murderer_as & 1.00000 \nonumber\\
happiest & 1.00000 \nonumber\\
happiest_life & 1.00000 \nonumber\\
so_from & 1.00000 \nonumber\\
crime_scene & 1.00000 \nonumber\\
that_everyday & 1.00000 \nonumber\\
wife_would & 1.00000 \nonumber\\
a_spouse & 1.00000 \nonumber\\
much_stress & 1.00000 \nonumber\\
the_happiest & 1.00000 \nonumber\\
in_danger & 1.00000 \nonumber\\
everyday_you & 1.00000 \nonumber\\
about_when & 1.00000 \nonumber\\
danger & 1.00000 \nonumber\\
danger_. & 1.00000 \nonumber\\
bring_upon & 1.00000 \nonumber\\
own_life & 1.00000 \nonumber\\
upon_your & 1.00000 \nonumber\\
the_cop & 1.00000 \nonumber\\
scene_or & 1.00000 \nonumber\\
be_okay & 1.00000 \nonumber\\
from_, & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,PP,S, & 1.00000 \nonumber\\
considerate_act & 1.00000 \nonumber\\
really_" & 1.00000 \nonumber\\
gave-up_to & 1.00000 \nonumber\\
gave-up & 1.00000 \nonumber\\
less-difficult & 1.00000 \nonumber\\
less-difficult_time & 1.00000 \nonumber\\
??_no & 1.00000 \nonumber\\
ProductionRule_S->S,-LRB-,CC,-RRB-,S, & 1.00000 \nonumber\\
beem & 1.00000 \nonumber\\
_pos_ngram_CONJ_O_ART & 1.00000 \nonumber\\
goal_or & 1.00000 \nonumber\\
and_barrier & 1.00000 \nonumber\\
allow_door & 1.00000 \nonumber\\
sacrifice_] & 1.00000 \nonumber\\
sacrifice_" & 1.00000 \nonumber\\
beem_from & 1.00000 \nonumber\\
open_and & 1.00000 \nonumber\\
be_[ & 1.00000 \nonumber\\
neighbor_without & 1.00000 \nonumber\\
seek_to & 1.00000 \nonumber\\
"_goal & 1.00000 \nonumber\\
write_seek & 1.00000 \nonumber\\
an_less-difficult & 1.00000 \nonumber\\
thier_life & 1.00000 \nonumber\\
her_neighbor & 1.00000 \nonumber\\
"_personal & 1.00000 \nonumber\\
time_persue & 1.00000 \nonumber\\
much_would & 1.00000 \nonumber\\
and_after & 1.00000 \nonumber\\
ProductionRule_NP->DT,``,NNP,'',NN, & 1.00000 \nonumber\\
good_allow & 1.00000 \nonumber\\
considerate & 1.00000 \nonumber\\
blind_by & 1.00000 \nonumber\\
would_a & 1.00000 \nonumber\\
ProductionRule_S->ADVP,S,VP, & 1.00000 \nonumber\\
)_what & 1.00000 \nonumber\\
act_one & 1.00000 \nonumber\\
there_! & 1.00000 \nonumber\\
persue_a & 1.00000 \nonumber\\
barrier_to & 1.00000 \nonumber\\
barrier & 1.00000 \nonumber\\
for_his & 1.00000 \nonumber\\
journey_( & 1.00000 \nonumber\\
personal_" & 1.00000 \nonumber\\
or_) & 1.00000 \nonumber\\
...._remember & 1.00000 \nonumber\\
)_series & 1.00000 \nonumber\\
[_sacrifice & 1.00000 \nonumber\\
or_lifestyle & 1.00000 \nonumber\\
selfishness_?? & 1.00000 \nonumber\\
selfishness & 1.00000 \nonumber\\
]_how & 1.00000 \nonumber\\
of_considerate & 1.00000 \nonumber\\
light_beem & 1.00000 \nonumber\\
simply_write & 1.00000 \nonumber\\
life_.... & 1.00000 \nonumber\\
do_( & 1.00000 \nonumber\\
from_selfishness & 1.00000 \nonumber\\
"_sacrifice & 1.00000 \nonumber\\
break_, & 1.00000 \nonumber\\
where_a & 1.00000 \nonumber\\
they_gave-up & 1.00000 \nonumber\\
person_really & 1.00000 \nonumber\\
"_marriage & 1.00000 \nonumber\\
!!_maybe & 1.00000 \nonumber\\
na_watch & 1.00000 \nonumber\\
yur_self & 1.00000 \nonumber\\
yur & 1.00000 \nonumber\\
and_doin & 1.00000 \nonumber\\
yu_wan & 1.00000 \nonumber\\
wrong_why & 1.00000 \nonumber\\
here_r & 1.00000 \nonumber\\
at_yur & 1.00000 \nonumber\\
watchin_it & 1.00000 \nonumber\\
watchin & 1.00000 \nonumber\\
thing_! & 1.00000 \nonumber\\
cuz_kid & 1.00000 \nonumber\\
watch_people & 1.00000 \nonumber\\
sex_get & 1.00000 \nonumber\\
different_but & 1.00000 \nonumber\\
mirror & 1.00000 \nonumber\\
everyone_feel & 1.00000 \nonumber\\
mirror_and & 1.00000 \nonumber\\
doin_the & 1.00000 \nonumber\\
sex_!! & 1.00000 \nonumber\\
doin & 1.00000 \nonumber\\
..._cuz & 1.00000 \nonumber\\
kid_out & 1.00000 \nonumber\\
_pos_ngram_NP_ADV_NP & 1.00000 \nonumber\\
and_look & 1.00000 \nonumber\\
r_watchin & 1.00000 \nonumber\\
a_mirror & 1.00000 \nonumber\\
out_here & 1.00000 \nonumber\\
self_... & 1.00000 \nonumber\\
maybe_everyone & 1.00000 \nonumber\\
feel_different & 1.00000 \nonumber\\
if_yu & 1.00000 \nonumber\\
before_the & 1.00000 \nonumber\\
do_school & 1.00000 \nonumber\\
_pos_ngram_CARD_V_PP & 1.00000 \nonumber\\
to_point & 1.00000 \nonumber\\
bacterium_in & 1.00000 \nonumber\\
on_be & 1.00000 \nonumber\\
contaminant_in & 1.00000 \nonumber\\
sell_water & 1.00000 \nonumber\\
system_be & 1.00000 \nonumber\\
and_remains & 1.00000 \nonumber\\
cause_pollution & 1.00000 \nonumber\\
contaminant & 1.00000 \nonumber\\
water_battle & 1.00000 \nonumber\\
be_age & 1.00000 \nonumber\\
battle_that & 1.00000 \nonumber\\
than_tap & 1.00000 \nonumber\\
cost_more & 1.00000 \nonumber\\
of_chemical & 1.00000 \nonumber\\
chemical_contaminant & 1.00000 \nonumber\\
remains_hundred & 1.00000 \nonumber\\
people_sell & 1.00000 \nonumber\\
china_. & 1.00000 \nonumber\\
indium_? & 1.00000 \nonumber\\
th & 1.00000 \nonumber\\
in_china & 1.00000 \nonumber\\
spiritual_people & 1.00000 \nonumber\\
china_be & 1.00000 \nonumber\\
not_indium & 1.00000 \nonumber\\
hey_, & 1.00000 \nonumber\\
with_diverse & 1.00000 \nonumber\\
,_poverty & 1.00000 \nonumber\\
highly_spiritual & 1.00000 \nonumber\\
flourish & 1.00000 \nonumber\\
government_seem & 1.00000 \nonumber\\
to_flourish & 1.00000 \nonumber\\
flourish_. & 1.00000 \nonumber\\
tounge & 1.00000 \nonumber\\
and_race & 1.00000 \nonumber\\
poverty_still & 1.00000 \nonumber\\
corrupt_and & 1.00000 \nonumber\\
and_poverty & 1.00000 \nonumber\\
seem_pretty & 1.00000 \nonumber\\
poverty_be & 1.00000 \nonumber\\
ignore_the & 1.00000 \nonumber\\
still_exist & 1.00000 \nonumber\\
of_natural & 1.00000 \nonumber\\
race_. & 1.00000 \nonumber\\
pretty_corrupt & 1.00000 \nonumber\\
._full & 1.00000 \nonumber\\
th_potential & 1.00000 \nonumber\\
not_ignore & 1.00000 \nonumber\\
diverse_tounge & 1.00000 \nonumber\\
have_th & 1.00000 \nonumber\\
with_highly & 1.00000 \nonumber\\
,_china & 1.00000 \nonumber\\
tounge_and & 1.00000 \nonumber\\
spiritual & 1.00000 \nonumber\\
communist & 1.00000 \nonumber\\
and_country & 1.00000 \nonumber\\
be_communist & 1.00000 \nonumber\\
natural_resource & 1.00000 \nonumber\\
communist_, & 1.00000 \nonumber\\
,_fill & 1.00000 \nonumber\\
how_lousy & 1.00000 \nonumber\\
lousy_he & 1.00000 \nonumber\\
be_open & 1.00000 \nonumber\\
first_... & 1.00000 \nonumber\\
because_when & 1.00000 \nonumber\\
choice & 1.00000 \nonumber\\
perception & 1.00000 \nonumber\\
perception_. & 1.00000 \nonumber\\
off_to & 1.00000 \nonumber\\
school_that & 1.00000 \nonumber\\
name_of & 1.00000 \nonumber\\
a_war & 1.00000 \nonumber\\
war_in & 1.00000 \nonumber\\
wage & 1.00000 \nonumber\\
wage_a & 1.00000 \nonumber\\
ever_wage & 1.00000 \nonumber\\
._civil & 1.00000 \nonumber\\
too_. & 1.00000 \nonumber\\
ProductionRule_FRAG->ADVP,PP, & 1.00000 \nonumber\\
without_plastic & 1.00000 \nonumber\\
sunshine & 1.00000 \nonumber\\
only_darkness & 1.00000 \nonumber\\
aint_no & 1.00000 \nonumber\\
no_sunshine & 1.00000 \nonumber\\
there_aint & 1.00000 \nonumber\\
sunshine_without & 1.00000 \nonumber\\
everyday_. & 1.00000 \nonumber\\
darkness_everyday & 1.00000 \nonumber\\
nation & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,NP,ADVP,SBAR, & 1.00000 \nonumber\\
site_? & 1.00000 \nonumber\\
everybody_try & 1.00000 \nonumber\\
why_everybody & 1.00000 \nonumber\\
compatible_site & 1.00000 \nonumber\\
best_then & 1.00000 \nonumber\\
ie_compatible & 1.00000 \nonumber\\
ed_to & 1.00000 \nonumber\\
to_graduate & 1.00000 \nonumber\\
we_shouldnt & 1.00000 \nonumber\\
graduate_school & 1.00000 \nonumber\\
need_phy & 1.00000 \nonumber\\
graduate & 1.00000 \nonumber\\
physical_ed & 1.00000 \nonumber\\
ed_cause & 1.00000 \nonumber\\
shouldnt_need & 1.00000 \nonumber\\
when_everyone & 1.00000 \nonumber\\
merica_be & 1.00000 \nonumber\\
have_education & 1.00000 \nonumber\\
an_american & 1.00000 \nonumber\\
competitive & 1.00000 \nonumber\\
our_lifetime & 1.00000 \nonumber\\
merica & 1.00000 \nonumber\\
america_and & 1.00000 \nonumber\\
competitive_in & 1.00000 \nonumber\\
british_come & 1.00000 \nonumber\\
american_, & 1.00000 \nonumber\\
excel & 1.00000 \nonumber\\
develop_quickly & 1.00000 \nonumber\\
everything_away & 1.00000 \nonumber\\
excel_. & 1.00000 \nonumber\\
leave_in & 1.00000 \nonumber\\
slavery_and & 1.00000 \nonumber\\
rich_due & 1.00000 \nonumber\\
admit_" & 1.00000 \nonumber\\
in_education & 1.00000 \nonumber\\
_pos_ngram_NP_V_CONJ & 1.00000 \nonumber\\
start_develop & 1.00000 \nonumber\\
rich_until & 1.00000 \nonumber\\
more_competitive & 1.00000 \nonumber\\
than_america & 1.00000 \nonumber\\
will_excel & 1.00000 \nonumber\\
"_merica & 1.00000 \nonumber\\
ProductionRule_S->``,NP,VP, & 1.00000 \nonumber\\
soon_when & 1.00000 \nonumber\\
bid_state & 1.00000 \nonumber\\
have_slavery & 1.00000 \nonumber\\
to_slavery & 1.00000 \nonumber\\
take_everything & 1.00000 \nonumber\\
but_start & 1.00000 \nonumber\\
lifetime_) & 1.00000 \nonumber\\
will_happen & 1.00000 \nonumber\\
lifetime & 1.00000 \nonumber\\
indium_never & 1.00000 \nonumber\\
)_indium & 1.00000 \nonumber\\
slavery_. & 1.00000 \nonumber\\
education_( & 1.00000 \nonumber\\
and_soon & 1.00000 \nonumber\\
_pos_ngram_ART_PR_ADJ & 1.00000 \nonumber\\
,_think & 1.00000 \nonumber\\
ass & 1.00000 \nonumber\\
grow_a & 1.00000 \nonumber\\
christian_home & 1.00000 \nonumber\\
sandal_wear & 1.00000 \nonumber\\
assume_everyone & 1.00000 \nonumber\\
home_, & 1.00000 \nonumber\\
cultist & 1.00000 \nonumber\\
cultist_. & 1.00000 \nonumber\\
worship_a & 1.00000 \nonumber\\
ProductionRule_VP->VP,,,VP,,,SBAR, & 1.00000 \nonumber\\
pair_and & 1.00000 \nonumber\\
ProductionRule_VP->NN,NP,S, & 1.00000 \nonumber\\
sandal & 1.00000 \nonumber\\
and_ask & 1.00000 \nonumber\\
everyone_on & 1.00000 \nonumber\\
a_scruffy & 1.00000 \nonumber\\
wear_cultist & 1.00000 \nonumber\\
scruffy & 1.00000 \nonumber\\
i_worship & 1.00000 \nonumber\\
scruffy_sandal & 1.00000 \nonumber\\
a_pair & 1.00000 \nonumber\\
sunday_school & 1.00000 \nonumber\\
_pos_ngram_CARD_ADV_PR & 1.00000 \nonumber\\
brainwash_. & 1.00000 \nonumber\\
pray_before & 1.00000 \nonumber\\
prayer & 1.00000 \nonumber\\
prayer_( & 1.00000 \nonumber\\
prayer_in & 1.00000 \nonumber\\
?_pray & 1.00000 \nonumber\\
thankfully & 1.00000 \nonumber\\
remember_at & 1.00000 \nonumber\\
?_sunday & 1.00000 \nonumber\\
system_stop & 1.00000 \nonumber\\
i_stop & 1.00000 \nonumber\\
you_bring & 1.00000 \nonumber\\
pray_at & 1.00000 \nonumber\\
and_god & 1.00000 \nonumber\\
'_prayer & 1.00000 \nonumber\\
(_thankfully & 1.00000 \nonumber\\
question_the & 1.00000 \nonumber\\
stop_assume & 1.00000 \nonumber\\
church_? & 1.00000 \nonumber\\
age_of & 1.00000 \nonumber\\
_pos_ngram_PP_CARD_ADV & 1.00000 \nonumber\\
start_question & 1.00000 \nonumber\\
lord_' & 1.00000 \nonumber\\
so_please & 1.00000 \nonumber\\
can_that & 1.00000 \nonumber\\
up_? & 1.00000 \nonumber\\
and_stop & 1.00000 \nonumber\\
before_meal & 1.00000 \nonumber\\
7_when & 1.00000 \nonumber\\
night_? & 1.00000 \nonumber\\
stop_say & 1.00000 \nonumber\\
that_practice & 1.00000 \nonumber\\
public_school & 1.00000 \nonumber\\
school_system & 1.00000 \nonumber\\
at_night & 1.00000 \nonumber\\
thankfully_my & 1.00000 \nonumber\\
stop_that & 1.00000 \nonumber\\
meal_? & 1.00000 \nonumber\\
me_where & 1.00000 \nonumber\\
please_tell & 1.00000 \nonumber\\
practice_) & 1.00000 \nonumber\\
meal & 1.00000 \nonumber\\
assume_god & 1.00000 \nonumber\\
where_i & 1.00000 \nonumber\\
three_, & 1.00000 \nonumber\\
us_and & 1.00000 \nonumber\\
and_language & 1.00000 \nonumber\\
the_fat & 1.00000 \nonumber\\
of_gold & 1.00000 \nonumber\\
thirsty & 1.00000 \nonumber\\
thirsty_man & 1.00000 \nonumber\\
worth_more & 1.00000 \nonumber\\
ProductionRule_ADJP->JJ,ADVP,PP, & 1.00000 \nonumber\\
a_sack & 1.00000 \nonumber\\
a_thirsty & 1.00000 \nonumber\\
sack_of & 1.00000 \nonumber\\
gold_to & 1.00000 \nonumber\\
drop_of & 1.00000 \nonumber\\
a_drop & 1.00000 \nonumber\\
another_person & 1.00000 \nonumber\\
and_policy & 1.00000 \nonumber\\
plan_and & 1.00000 \nonumber\\
policy_that & 1.00000 \nonumber\\
leave_some & 1.00000 \nonumber\\
do_leave & 1.00000 \nonumber\\
before_leave & 1.00000 \nonumber\\
murder_in & 1.00000 \nonumber\\
plus_i & 1.00000 \nonumber\\
him_first & 1.00000 \nonumber\\
worng & 1.00000 \nonumber\\
n't_happen & 1.00000 \nonumber\\
turn_himself & 1.00000 \nonumber\\
in_but & 1.00000 \nonumber\\
persuade & 1.00000 \nonumber\\
worng_i & 1.00000 \nonumber\\
he_truly & 1.00000 \nonumber\\
of_alway & 1.00000 \nonumber\\
he_murder & 1.00000 \nonumber\\
take_reponsiblity & 1.00000 \nonumber\\
happen_i & 1.00000 \nonumber\\
persuade_him & 1.00000 \nonumber\\
himself_in & 1.00000 \nonumber\\
alway_know & 1.00000 \nonumber\\
love_me & 1.00000 \nonumber\\
to_persuade & 1.00000 \nonumber\\
me_worng & 1.00000 \nonumber\\
turn_that & 1.00000 \nonumber\\
reponsiblity & 1.00000 \nonumber\\
reponsiblity_for & 1.00000 \nonumber\\
be_definitely & 1.00000 \nonumber\\
?_how & 1.00000 \nonumber\\
estimate & 1.00000 \nonumber\\
nine & 1.00000 \nonumber\\
male_role & 1.00000 \nonumber\\
indian_citizen & 1.00000 \nonumber\\
year_..... & 1.00000 \nonumber\\
increase_in & 1.00000 \nonumber\\
the_gdp & 1.00000 \nonumber\\
gdp & 1.00000 \nonumber\\
fund_to & 1.00000 \nonumber\\
...._because & 1.00000 \nonumber\\
we_even & 1.00000 \nonumber\\
will_increase & 1.00000 \nonumber\\
soooo_even & 1.00000 \nonumber\\
gdp_of & 1.00000 \nonumber\\
unemployment & 1.00000 \nonumber\\
next_5 & 1.00000 \nonumber\\
soo & 1.00000 \nonumber\\
imagine_them & 1.00000 \nonumber\\
fund & 1.00000 \nonumber\\
much_unemployment & 1.00000 \nonumber\\
enough_fund & 1.00000 \nonumber\\
ProductionRule_NP->NP,VP,NP,., & 1.00000 \nonumber\\
unemployment_i & 1.00000 \nonumber\\
dont_even & 1.00000 \nonumber\\
soo_much & 1.00000 \nonumber\\
think_soooo & 1.00000 \nonumber\\
of_soo & 1.00000 \nonumber\\
citizen_..... & 1.00000 \nonumber\\
feed_all & 1.00000 \nonumber\\
father_. & 1.00000 \nonumber\\
_pos_ngram_O_CONJ_ADV & 1.00000 \nonumber\\
hundred & 1.00000 \nonumber\\
hundred_of & 1.00000 \nonumber\\
ProductionRule_VP->VBD,PRT,S, & 1.00000 \nonumber\\
can_alway & 1.00000 \nonumber\\
ProductionRule_PP->IN,:,S, & 1.00000 \nonumber\\
again_and & 1.00000 \nonumber\\
spank_teach & 1.00000 \nonumber\\
good_daughter & 1.00000 \nonumber\\
ProductionRule_S->RB,NP,VP,., & 1.00000 \nonumber\\
really_, & 1.00000 \nonumber\\
release & 1.00000 \nonumber\\
big_mess & 1.00000 \nonumber\\
anything_he & 1.00000 \nonumber\\
research_about & 1.00000 \nonumber\\
you_research & 1.00000 \nonumber\\
and_gamble & 1.00000 \nonumber\\
about_farquhar.he & 1.00000 \nonumber\\
den_carry & 1.00000 \nonumber\\
farquhar.he_do & 1.00000 \nonumber\\
mess_and & 1.00000 \nonumber\\
no.if_you & 1.00000 \nonumber\\
gamble_den & 1.00000 \nonumber\\
like_vice & 1.00000 \nonumber\\
vice_, & 1.00000 \nonumber\\
vice & 1.00000 \nonumber\\
allow_thing & 1.00000 \nonumber\\
,_crime & 1.00000 \nonumber\\
carry_on & 1.00000 \nonumber\\
no.if & 1.00000 \nonumber\\
farquhar.he & 1.00000 \nonumber\\
away_, & 1.00000 \nonumber\\
at_first & 1.00000 \nonumber\\
shirt & 1.00000 \nonumber\\
gratification & 1.00000 \nonumber\\
for_there & 1.00000 \nonumber\\
about_later & 1.00000 \nonumber\\
and_tap & 1.00000 \nonumber\\
about_now & 1.00000 \nonumber\\
even_need & 1.00000 \nonumber\\
price_and & 1.00000 \nonumber\\
bottle_water-have & 1.00000 \nonumber\\
water-have_all & 1.00000 \nonumber\\
more_waste & 1.00000 \nonumber\\
bottle_except & 1.00000 \nonumber\\
water-have_more & 1.00000 \nonumber\\
ProductionRule_ADVP->IN,RB, & 1.00000 \nonumber\\
n't_save & 1.00000 \nonumber\\
water-have & 1.00000 \nonumber\\
._tap & 1.00000 \nonumber\\
tap_water-have & 1.00000 \nonumber\\
emergency_you & 1.00000 \nonumber\\
later_you & 1.00000 \nonumber\\
except_no & 1.00000 \nonumber\\
no_price & 1.00000 \nonumber\\
no_waste & 1.00000 \nonumber\\
as_bottle & 1.00000 \nonumber\\
ProductionRule_NP->UCP,NNS, & 1.00000 \nonumber\\
hussein & 1.00000 \nonumber\\
sultan_hussein & 1.00000 \nonumber\\
abortion_. & 1.00000 \nonumber\\
not_necessary & 1.00000 \nonumber\\
only_degrade & 1.00000 \nonumber\\
day_one & 1.00000 \nonumber\\
may_need & 1.00000 \nonumber\\
day_, & 1.00000 \nonumber\\
be_blind & 1.00000 \nonumber\\
to_work & 1.00000 \nonumber\\
display & 1.00000 \nonumber\\
_pos_ngram_PP_NP_NN & 1.00000 \nonumber\\
ashame_to & 1.00000 \nonumber\\
the_lack & 1.00000 \nonumber\\
_pos_ngram_CARD_V_PUNC & 1.00000 \nonumber\\
!_that & 1.00000 \nonumber\\
only_post & 1.00000 \nonumber\\
lyric & 1.00000 \nonumber\\
song_lyric & 1.00000 \nonumber\\
post_song & 1.00000 \nonumber\\
water_! & 1.00000 \nonumber\\
lyric_! & 1.00000 \nonumber\\
in_area & 1.00000 \nonumber\\
product & 1.00000 \nonumber\\
development_of & 1.00000 \nonumber\\
?_we & 1.00000 \nonumber\\
teacher_say & 1.00000 \nonumber\\
love_get & 1.00000 \nonumber\\
so_my & 1.00000 \nonumber\\
say_:p & 1.00000 \nonumber\\
:p & 1.00000 \nonumber\\
also_improve & 1.00000 \nonumber\\
in_them & 1.00000 \nonumber\\
english_teacher & 1.00000 \nonumber\\
your_literature & 1.00000 \nonumber\\
(_so & 1.00000 \nonumber\\
get_lose & 1.00000 \nonumber\\
my_english & 1.00000 \nonumber\\
literature_( & 1.00000 \nonumber\\
love_book & 1.00000 \nonumber\\
:p_) & 1.00000 \nonumber\\
literature & 1.00000 \nonumber\\
choose_no & 1.00000 \nonumber\\
fatherly_figure & 1.00000 \nonumber\\
stain_in & 1.00000 \nonumber\\
a_uncare & 1.00000 \nonumber\\
ProductionRule_VP->TO,PRN,VP, & 1.00000 \nonumber\\
ProductionRule_NP->DT,JJ,CC,JJ,NN, & 1.00000 \nonumber\\
rather_choose & 1.00000 \nonumber\\
figure_i & 1.00000 \nonumber\\
a_stain & 1.00000 \nonumber\\
stain & 1.00000 \nonumber\\
uncare & 1.00000 \nonumber\\
necessarily_have & 1.00000 \nonumber\\
and_lousy & 1.00000 \nonumber\\
n't_necessarily & 1.00000 \nonumber\\
uncare_and & 1.00000 \nonumber\\
ahead & 1.00000 \nonumber\\
latest_version & 1.00000 \nonumber\\
the_older & 1.00000 \nonumber\\
download_very & 1.00000 \nonumber\\
the_latest & 1.00000 \nonumber\\
ProductionRule_VP->VBN,NP,ADVP, & 1.00000 \nonumber\\
google_toolbar & 1.00000 \nonumber\\
pop-up_and & 1.00000 \nonumber\\
ProductionRule_UCP->NP,CC,RRC, & 1.00000 \nonumber\\
have_block & 1.00000 \nonumber\\
it_download & 1.00000 \nonumber\\
version_along & 1.00000 \nonumber\\
it_alert & 1.00000 \nonumber\\
update_the & 1.00000 \nonumber\\
explorer_because & 1.00000 \nonumber\\
a_google & 1.00000 \nonumber\\
block_pop-up & 1.00000 \nonumber\\
automatically & 1.00000 \nonumber\\
older_version & 1.00000 \nonumber\\
and_automatically & 1.00000 \nonumber\\
alert_you & 1.00000 \nonumber\\
automatically_update & 1.00000 \nonumber\\
alert & 1.00000 \nonumber\\
case_kill & 1.00000 \nonumber\\
ProductionRule_NP->DT,JJ,NN,NN,NNS, & 1.00000 \nonumber\\
water_like & 1.00000 \nonumber\\
lake & 1.00000 \nonumber\\
platypus & 1.00000 \nonumber\\
platypus_. & 1.00000 \nonumber\\
that_like & 1.00000 \nonumber\\
kill_off & 1.00000 \nonumber\\
major_water & 1.00000 \nonumber\\
ProductionRule_VP->VBG,PRT,NP,PP, & 1.00000 \nonumber\\
our_lake & 1.00000 \nonumber\\
ProductionRule_VP->VBG,NP,PP,S, & 1.00000 \nonumber\\
the_major & 1.00000 \nonumber\\
from_our & 1.00000 \nonumber\\
like_platypus & 1.00000 \nonumber\\
like_water & 1.00000 \nonumber\\
producee & 1.00000 \nonumber\\
for_criter & 1.00000 \nonumber\\
water_producee & 1.00000 \nonumber\\
off_habitat & 1.00000 \nonumber\\
be_steal & 1.00000 \nonumber\\
criter_that & 1.00000 \nonumber\\
criter & 1.00000 \nonumber\\
producee_company & 1.00000 \nonumber\\
lake_in & 1.00000 \nonumber\\
steal_water & 1.00000 \nonumber\\
habitat_for & 1.00000 \nonumber\\
communicate_with & 1.00000 \nonumber\\
communicate & 1.00000 \nonumber\\
_pos_ngram_NP_NP_O & 1.00000 \nonumber\\
..._2nd & 1.00000 \nonumber\\
weight_!!!! & 1.00000 \nonumber\\
_pos_ngram_CONJ_PUNC_ADJ & 1.00000 \nonumber\\
a_proble & 1.00000 \nonumber\\
ProductionRule_NP->NP,,,ADVP, & 1.00000 \nonumber\\
..._now & 1.00000 \nonumber\\
ProductionRule_S->PP,,,S,:,VP, & 1.00000 \nonumber\\
the_weight & 1.00000 \nonumber\\
activity_of & 1.00000 \nonumber\\
our_excerse & 1.00000 \nonumber\\
a_moment & 1.00000 \nonumber\\
..._1st & 1.00000 \nonumber\\
!!_... & 1.00000 \nonumber\\
fake_lunch & 1.00000 \nonumber\\
weight_we & 1.00000 \nonumber\\
ProductionRule_FRAG->:,ADVP,NP, & 1.00000 \nonumber\\
certainly_a & 1.00000 \nonumber\\
some_weight & 1.00000 \nonumber\\
!_3rd & 1.00000 \nonumber\\
lose_some & 1.00000 \nonumber\\
1st_, & 1.00000 \nonumber\\
do_our & 1.00000 \nonumber\\
fat_when & 1.00000 \nonumber\\
do_!! & 1.00000 \nonumber\\
we_sweat & 1.00000 \nonumber\\
lunch_, & 1.00000 \nonumber\\
eat_the & 1.00000 \nonumber\\
proble_in & 1.00000 \nonumber\\
then_lose & 1.00000 \nonumber\\
2nd_, & 1.00000 \nonumber\\
help_! & 1.00000 \nonumber\\
proble & 1.00000 \nonumber\\
but_... & 1.00000 \nonumber\\
!_..... & 1.00000 \nonumber\\
sweat & 1.00000 \nonumber\\
fun_activity & 1.00000 \nonumber\\
lose_the & 1.00000 \nonumber\\
fun_, & 1.00000 \nonumber\\
be_certainly & 1.00000 \nonumber\\
'_fake & 1.00000 \nonumber\\
_pos_ngram_PP_PUNC_CARD & 1.00000 \nonumber\\
a_fun & 1.00000 \nonumber\\
obesity_be & 1.00000 \nonumber\\
excerse & 1.00000 \nonumber\\
excerse_-- & 1.00000 \nonumber\\
will_eat & 1.00000 \nonumber\\
now_go & 1.00000 \nonumber\\
be_gain & 1.00000 \nonumber\\
ProductionRule_S->ADVP,,,SBAR,,,NP,VP, & 1.00000 \nonumber\\
--_lose & 1.00000 \nonumber\\
gain_, & 1.00000 \nonumber\\
moment_that & 1.00000 \nonumber\\
sweat_! & 1.00000 \nonumber\\
,_obesity & 1.00000 \nonumber\\
1st & 1.00000 \nonumber\\
go_get & 1.00000 \nonumber\\
lunch & 1.00000 \nonumber\\
or_unborn & 1.00000 \nonumber\\
okay_. & 1.00000 \nonumber\\
but_necessary & 1.00000 \nonumber\\
attempt_it & 1.00000 \nonumber\\
,_bear & 1.00000 \nonumber\\
might_kill & 1.00000 \nonumber\\
unborn_. & 1.00000 \nonumber\\
bear_or & 1.00000 \nonumber\\
one_situation & 1.00000 \nonumber\\
otherwise_, & 1.00000 \nonumber\\
sad_, & 1.00000 \nonumber\\
of_give & 1.00000 \nonumber\\
and_attempt & 1.00000 \nonumber\\
medical & 1.00000 \nonumber\\
!!!_i & 1.00000 \nonumber\\
whatever_, & 1.00000 \nonumber\\
the_advancement & 1.00000 \nonumber\\
n't_inherently & 1.00000 \nonumber\\
harm_anyone & 1.00000 \nonumber\\
choice.it & 1.00000 \nonumber\\
substantially & 1.00000 \nonumber\\
n't_substantially & 1.00000 \nonumber\\
inherently & 1.00000 \nonumber\\
inherently_wrong & 1.00000 \nonumber\\
as_simple & 1.00000 \nonumber\\
substantially_harm & 1.00000 \nonumber\\
by_choice.it & 1.00000 \nonumber\\
n't_involve & 1.00000 \nonumber\\
choice.it_really & 1.00000 \nonumber\\
simple_as & 1.00000 \nonumber\\
it_allow & 1.00000 \nonumber\\
himself_. & 1.00000 \nonumber\\
that_murder & 1.00000 \nonumber\\
will_continue & 1.00000 \nonumber\\
,_make & 1.00000 \nonumber\\
how_that & 1.00000 \nonumber\\
sure_how & 1.00000 \nonumber\\
the_follow & 1.00000 \nonumber\\
_pos_ngram_CARD_V_ADJ & 1.00000 \nonumber\\
so_book & 1.00000 \nonumber\\
even_it & 1.00000 \nonumber\\
..._child & 1.00000 \nonumber\\
something_new & 1.00000 \nonumber\\
compare_clothe & 1.00000 \nonumber\\
buy_it & 1.00000 \nonumber\\
necessary_... & 1.00000 \nonumber\\
other_... & 1.00000 \nonumber\\
classmate & 1.00000 \nonumber\\
they_see & 1.00000 \nonumber\\
of_each & 1.00000 \nonumber\\
from_their & 1.00000 \nonumber\\
..._if & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,NP,:,S, & 1.00000 \nonumber\\
equal_, & 1.00000 \nonumber\\
classmate_, & 1.00000 \nonumber\\
clothe_of & 1.00000 \nonumber\\
idea_... & 1.00000 \nonumber\\
their_classmate & 1.00000 \nonumber\\
new_from & 1.00000 \nonumber\\
dont_think & 1.00000 \nonumber\\
hopefully & 1.00000 \nonumber\\
father_have & 1.00000 \nonumber\\
certain_connection & 1.00000 \nonumber\\
alway_there & 1.00000 \nonumber\\
daughter_character & 1.00000 \nonumber\\
father_might & 1.00000 \nonumber\\
major_role & 1.00000 \nonumber\\
character_and & 1.00000 \nonumber\\
lousy_they & 1.00000 \nonumber\\
our_kin & 1.00000 \nonumber\\
or_alway & 1.00000 \nonumber\\
determine_who & 1.00000 \nonumber\\
parent_play & 1.00000 \nonumber\\
still_your & 1.00000 \nonumber\\
you_he & 1.00000 \nonumber\\
kin & 1.00000 \nonumber\\
still_our & 1.00000 \nonumber\\
what_shape & 1.00000 \nonumber\\
kin_. & 1.00000 \nonumber\\
believe_our & 1.00000 \nonumber\\
best_or & 1.00000 \nonumber\\
or_daughter & 1.00000 \nonumber\\
personality_. & 1.00000 \nonumber\\
mold_a & 1.00000 \nonumber\\
in_determine & 1.00000 \nonumber\\
be_alway & 1.00000 \nonumber\\
state_of & 1.00000 \nonumber\\
have_enough & 1.00000 \nonumber\\
gay_? & 1.00000 \nonumber\\
just_make & 1.00000 \nonumber\\
with_water & 1.00000 \nonumber\\
china & 1.00000 \nonumber\\
someone_for & 1.00000 \nonumber\\
another_country & 1.00000 \nonumber\\
_pos_ngram_CARD_PUNC_NP & 1.00000 \nonumber\\
_pos_ngram_V_NP_ADJ & 1.00000 \nonumber\\
_pos_ngram_NP_ADJ_PP & 1.00000 \nonumber\\
the_page & 1.00000 \nonumber\\
nope_. & 1.00000 \nonumber\\
that_im & 1.00000 \nonumber\\
_pos_ngram_ADJ_ADV_O & 1.00000 \nonumber\\
im_do & 1.00000 \nonumber\\
people_because & 1.00000 \nonumber\\
happy_that & 1.00000 \nonumber\\
me_feel & 1.00000 \nonumber\\
be_murder & 1.00000 \nonumber\\
every_morn & 1.00000 \nonumber\\
with_there & 1.00000 \nonumber\\
_pos_ngram_ADJ_NP_PUNC & 1.00000 \nonumber\\
curse & 1.00000 \nonumber\\
pe_have & 1.00000 \nonumber\\
dislike & 1.00000 \nonumber\\
)_you & 1.00000 \nonumber\\
ever_do & 1.00000 \nonumber\\
weight & 1.00000 \nonumber\\
_pos_ngram_PUNC_ART_ART & 1.00000 \nonumber\\
object & 1.00000 \nonumber\\
with_bottle & 1.00000 \nonumber\\
take_seriously & 1.00000 \nonumber\\
hypocryte_with & 1.00000 \nonumber\\
hypocryte & 1.00000 \nonumber\\
craig_be & 1.00000 \nonumber\\
a_hypocryte & 1.00000 \nonumber\\
craig & 1.00000 \nonumber\\
be_correct & 1.00000 \nonumber\\
for_debate & 1.00000 \nonumber\\
me_people & 1.00000 \nonumber\\
that_fine & 1.00000 \nonumber\\
scientifically_prove & 1.00000 \nonumber\\
fine_by & 1.00000 \nonumber\\
religious_belief & 1.00000 \nonumber\\
be_judge & 1.00000 \nonumber\\
'_scientifically & 1.00000 \nonumber\\
debate_? & 1.00000 \nonumber\\
scientifically & 1.00000 \nonumber\\
ProductionRule_NP->ADVP,PP, & 1.00000 \nonumber\\
move_they & 1.00000 \nonumber\\
stuff_, & 1.00000 \nonumber\\
they_without & 1.00000 \nonumber\\
by_me & 1.00000 \nonumber\\
point_? & 1.00000 \nonumber\\
have_religious & 1.00000 \nonumber\\
judge_on & 1.00000 \nonumber\\
every_move & 1.00000 \nonumber\\
and_stuff & 1.00000 \nonumber\\
not_display & 1.00000 \nonumber\\
body_to & 1.00000 \nonumber\\
drug_into & 1.00000 \nonumber\\
use_her & 1.00000 \nonumber\\
3_) & 1.00000 \nonumber\\
legally_prostitute & 1.00000 \nonumber\\
2_) & 1.00000 \nonumber\\
4_) & 1.00000 \nonumber\\
state_2 & 1.00000 \nonumber\\
to_steal & 1.00000 \nonumber\\
_pos_ngram_V_CARD_O & 1.00000 \nonumber\\
nake_body & 1.00000 \nonumber\\
illicit & 1.00000 \nonumber\\
she_can & 1.00000 \nonumber\\
_pos_ngram_NN_CARD_O & 1.00000 \nonumber\\
other_4 & 1.00000 \nonumber\\
)_a & 1.00000 \nonumber\\
also_not & 1.00000 \nonumber\\
steal_5 & 1.00000 \nonumber\\
her_own & 1.00000 \nonumber\\
5_) & 1.00000 \nonumber\\
her_nake & 1.00000 \nonumber\\
display_her & 1.00000 \nonumber\\
1_) & 1.00000 \nonumber\\
._man & 1.00000 \nonumber\\
,_ever & 1.00000 \nonumber\\
murder_other & 1.00000 \nonumber\\
into_her & 1.00000 \nonumber\\
body_in & 1.00000 \nonumber\\
body_3 & 1.00000 \nonumber\\
illicit_drug & 1.00000 \nonumber\\
man_can & 1.00000 \nonumber\\
government_tell & 1.00000 \nonumber\\
public_there & 1.00000 \nonumber\\
in_public & 1.00000 \nonumber\\
prostitute_herself & 1.00000 \nonumber\\
ProductionRule_VP->VB,NP,PP,,,ADVP, & 1.00000 \nonumber\\
body_all & 1.00000 \nonumber\\
not_legally & 1.00000 \nonumber\\
do_these & 1.00000 \nonumber\\
prostitute & 1.00000 \nonumber\\
take_illicit & 1.00000 \nonumber\\
many_state & 1.00000 \nonumber\\
own_body & 1.00000 \nonumber\\
me_" & 1.00000 \nonumber\\
you_might & 1.00000 \nonumber\\
self-defense & 1.00000 \nonumber\\
they_may & 1.00000 \nonumber\\
pleasure & 1.00000 \nonumber\\
must_not & 1.00000 \nonumber\\
our_parent & 1.00000 \nonumber\\
recycle & 1.00000 \nonumber\\
by_pornography & 1.00000 \nonumber\\
this_will & 1.00000 \nonumber\\
evolution_... & 1.00000 \nonumber\\
superpower & 1.00000 \nonumber\\
good_you & 1.00000 \nonumber\\
soooo & 1.00000 \nonumber\\
,_book & 1.00000 \nonumber\\
disgust & 1.00000 \nonumber\\
she_murder & 1.00000 \nonumber\\
defense_then & 1.00000 \nonumber\\
tell_the & 1.00000 \nonumber\\
go_crazy & 1.00000 \nonumber\\
on_who & 1.00000 \nonumber\\
be_self & 1.00000 \nonumber\\
corporation & 1.00000 \nonumber\\
dollar & 1.00000 \nonumber\\
plain & 1.00000 \nonumber\\
and_affection & 1.00000 \nonumber\\
sometime_abuse & 1.00000 \nonumber\\
numerous_crime & 1.00000 \nonumber\\
an_unhealthy & 1.00000 \nonumber\\
promote_the & 1.00000 \nonumber\\
image_of & 1.00000 \nonumber\\
people_which & 1.00000 \nonumber\\
inspire_numerous & 1.00000 \nonumber\\
porn_give & 1.00000 \nonumber\\
porn_inspire & 1.00000 \nonumber\\
porn_promote & 1.00000 \nonumber\\
inspire & 1.00000 \nonumber\\
also_. & 1.00000 \nonumber\\
pleasure_, & 1.00000 \nonumber\\
guilt_and & 1.00000 \nonumber\\
virginity & 1.00000 \nonumber\\
unhealthy_image & 1.00000 \nonumber\\
that_sometime & 1.00000 \nonumber\\
of_real & 1.00000 \nonumber\\
affection_also & 1.00000 \nonumber\\
and_lust & 1.00000 \nonumber\\
on_pleasure & 1.00000 \nonumber\\
real_sex & 1.00000 \nonumber\\
abuse_the & 1.00000 \nonumber\\
like_an & 1.00000 \nonumber\\
addiction_to & 1.00000 \nonumber\\
to_guilt & 1.00000 \nonumber\\
totally_base & 1.00000 \nonumber\\
virginity_of & 1.00000 \nonumber\\
unhealthy_and & 1.00000 \nonumber\\
actually_base & 1.00000 \nonumber\\
lust & 1.00000 \nonumber\\
on_love & 1.00000 \nonumber\\
lust_. & 1.00000 \nonumber\\
and_virginity & 1.00000 \nonumber\\
that_sex & 1.00000 \nonumber\\
be_unhealthy & 1.00000 \nonumber\\
louder_than & 1.00000 \nonumber\\
than_word & 1.00000 \nonumber\\
believe_you & 1.00000 \nonumber\\
child_only & 1.00000 \nonumber\\
more_if & 1.00000 \nonumber\\
action_speak & 1.00000 \nonumber\\
louder & 1.00000 \nonumber\\
speak_louder & 1.00000 \nonumber\\
know_they & 1.00000 \nonumber\\
understand_more & 1.00000 \nonumber\\
scare_to & 1.00000 \nonumber\\
even_be & 1.00000 \nonumber\\
technically & 1.00000 \nonumber\\
be_lie & 1.00000 \nonumber\\
_pos_ngram_PUNC_PP_CONJ & 1.00000 \nonumber\\
ProductionRule_ADJP->RBR,JJ,PP, & 1.00000 \nonumber\\
own_self & 1.00000 \nonumber\\
nothing_be & 1.00000 \nonumber\\
much_grind & 1.00000 \nonumber\\
to_conclude & 1.00000 \nonumber\\
;_as & 1.00000 \nonumber\\
to_conceal & 1.00000 \nonumber\\
have_heat & 1.00000 \nonumber\\
anomalous & 1.00000 \nonumber\\
anomalous_to & 1.00000 \nonumber\\
norm_of & 1.00000 \nonumber\\
support_atheism & 1.00000 \nonumber\\
say_we & 1.00000 \nonumber\\
heat_up & 1.00000 \nonumber\\
conceal_our & 1.00000 \nonumber\\
conceal & 1.00000 \nonumber\\
conclude & 1.00000 \nonumber\\
be_anomalous & 1.00000 \nonumber\\
conclude_that & 1.00000 \nonumber\\
well_though & 1.00000 \nonumber\\
argument_have & 1.00000 \nonumber\\
n't_forget & 1.00000 \nonumber\\
trend_of & 1.00000 \nonumber\\
christianity_; & 1.00000 \nonumber\\
we_support & 1.00000 \nonumber\\
the_principle & 1.00000 \nonumber\\
as_this & 1.00000 \nonumber\\
and_norm & 1.00000 \nonumber\\
forget_the & 1.00000 \nonumber\\
ProductionRule_S->SBAR,,,S,CC,S, & 1.00000 \nonumber\\
certainly_i & 1.00000 \nonumber\\
gain_that & 1.00000 \nonumber\\
principle_and & 1.00000 \nonumber\\
atheist_certainly & 1.00000 \nonumber\\
ProductionRule_NP->DT,NNS,CC,NNS, & 1.00000 \nonumber\\
this_trend & 1.00000 \nonumber\\
ProductionRule_VP->VBN,PRT, & 1.00000 \nonumber\\
behave_as & 1.00000 \nonumber\\
i_behave & 1.00000 \nonumber\\
of_christianity & 1.00000 \nonumber\\
atheism_have & 1.00000 \nonumber\\
principle & 1.00000 \nonumber\\
really_gain & 1.00000 \nonumber\\
grind_and & 1.00000 \nonumber\\
indium_lead & 1.00000 \nonumber\\
tomorrow_. & 1.00000 \nonumber\\
???!!!_kill & 1.00000 \nonumber\\
world_???!!! & 1.00000 \nonumber\\
???!!! & 1.00000 \nonumber\\
develop_tomorrow & 1.00000 \nonumber\\
tomorrow & 1.00000 \nonumber\\
kill_all & 1.00000 \nonumber\\
the_politician & 1.00000 \nonumber\\
politician_first & 1.00000 \nonumber\\
be_develop & 1.00000 \nonumber\\
should_indium & 1.00000 \nonumber\\
ProductionRule_NP->DT,NNS,NN, & 1.00000 \nonumber\\
hahaha & 1.00000 \nonumber\\
?_this & 1.00000 \nonumber\\
a_3rd & 1.00000 \nonumber\\
hahaha_really & 1.00000 \nonumber\\
practically_a & 1.00000 \nonumber\\
ridiculous_. & 1.00000 \nonumber\\
no_they & 1.00000 \nonumber\\
be_practically & 1.00000 \nonumber\\
3rd_world & 1.00000 \nonumber\\
that_of & 1.00000 \nonumber\\
really_ca & 1.00000 \nonumber\\
an_avid & 1.00000 \nonumber\\
avid & 1.00000 \nonumber\\
task & 1.00000 \nonumber\\
see_in & 1.00000 \nonumber\\
whatever_you & 1.00000 \nonumber\\
dat & 1.00000 \nonumber\\
say_he & 1.00000 \nonumber\\
just_keep & 1.00000 \nonumber\\
quickly_. & 1.00000 \nonumber\\
blessing & 1.00000 \nonumber\\
and_provide & 1.00000 \nonumber\\
extent_it & 1.00000 \nonumber\\
successful_and & 1.00000 \nonumber\\
blessing_. & 1.00000 \nonumber\\
your_blessing & 1.00000 \nonumber\\
survive_and & 1.00000 \nonumber\\
middle_because & 1.00000 \nonumber\\
certain_extent & 1.00000 \nonumber\\
of_in & 1.00000 \nonumber\\
extent & 1.00000 \nonumber\\
can_survive & 1.00000 \nonumber\\
too_help & 1.00000 \nonumber\\
also_sometime & 1.00000 \nonumber\\
pop-up & 1.00000 \nonumber\\
the_record & 1.00000 \nonumber\\
unwant & 1.00000 \nonumber\\
understand_the & 1.00000 \nonumber\\
same_in & 1.00000 \nonumber\\
it_dosent & 1.00000 \nonumber\\
dosent_matter & 1.00000 \nonumber\\
dosent & 1.00000 \nonumber\\
expirence & 1.00000 \nonumber\\
theyre_all & 1.00000 \nonumber\\
class_if & 1.00000 \nonumber\\
the_nerd & 1.00000 \nonumber\\
a_jock & 1.00000 \nonumber\\
sometime_there & 1.00000 \nonumber\\
underneath & 1.00000 \nonumber\\
class_do & 1.00000 \nonumber\\
underneath_the & 1.00000 \nonumber\\
nerd_or & 1.00000 \nonumber\\
then_theyre & 1.00000 \nonumber\\
expirence_sometime & 1.00000 \nonumber\\
pass_that & 1.00000 \nonumber\\
only_pass & 1.00000 \nonumber\\
nerd_outside & 1.00000 \nonumber\\
thing_then & 1.00000 \nonumber\\
personal_expirence & 1.00000 \nonumber\\
so_stupid & 1.00000 \nonumber\\
aspect_that & 1.00000 \nonumber\\
effort_. & 1.00000 \nonumber\\
forth_effort & 1.00000 \nonumber\\
ProductionRule_FRAG->NP,ADJP,., & 1.00000 \nonumber\\
put_forth & 1.00000 \nonumber\\
forth & 1.00000 \nonumber\\
a_nerd & 1.00000 \nonumber\\
the_aspect & 1.00000 \nonumber\\
jock_underneath & 1.00000 \nonumber\\
stupid_. & 1.00000 \nonumber\\
they_put & 1.00000 \nonumber\\
education_teach & 1.00000 \nonumber\\
teach_kid & 1.00000 \nonumber\\
jock & 1.00000 \nonumber\\
if_theyre & 1.00000 \nonumber\\
jock_because & 1.00000 \nonumber\\
same_class & 1.00000 \nonumber\\
of_clue & 1.00000 \nonumber\\
night_that & 1.00000 \nonumber\\
it_they & 1.00000 \nonumber\\
mind_that & 1.00000 \nonumber\\
just_incase & 1.00000 \nonumber\\
clue_even & 1.00000 \nonumber\\
incase & 1.00000 \nonumber\\
clue & 1.00000 \nonumber\\
incase_they & 1.00000 \nonumber\\
cant_get & 1.00000 \nonumber\\
will_try & 1.00000 \nonumber\\
all_type & 1.00000 \nonumber\\
because_who & 1.00000 \nonumber\\
you_less & 1.00000 \nonumber\\
love_just & 1.00000 \nonumber\\
its_on & 1.00000 \nonumber\\
one_night & 1.00000 \nonumber\\
ProductionRule_VP->VB,PP,NP,SBAR, & 1.00000 \nonumber\\
less_expect & 1.00000 \nonumber\\
ProductionRule_PP->PP,CC,PP, & 1.00000 \nonumber\\
truth_cant & 1.00000 \nonumber\\
truth_and & 1.00000 \nonumber\\
those_they & 1.00000 \nonumber\\
even_of & 1.00000 \nonumber\\
_pos_ngram_CONJ_PP_CARD & 1.00000 \nonumber\\
thing_because & 1.00000 \nonumber\\
situation_in & 1.00000 \nonumber\\
right_for & 1.00000 \nonumber\\
_pos_ngram_O_V_CONJ & 1.00000 \nonumber\\
2011_so & 1.00000 \nonumber\\
year_2011 & 1.00000 \nonumber\\
activity_and & 1.00000 \nonumber\\
_pos_ngram_CARD_ADV_ADV & 1.00000 \nonumber\\
'_because & 1.00000 \nonumber\\
far_and & 1.00000 \nonumber\\
become_obese & 1.00000 \nonumber\\
_pos_ngram_NN_CARD_ADV & 1.00000 \nonumber\\
2011 & 1.00000 \nonumber\\
mandatory_cuhz & 1.00000 \nonumber\\
112,000 & 1.00000 \nonumber\\
cuhz & 1.00000 \nonumber\\
112,000_people & 1.00000 \nonumber\\
obese_!!!! & 1.00000 \nonumber\\
cuhz_112,000 & 1.00000 \nonumber\\
have_die & 1.00000 \nonumber\\
ProductionRule_S->RB,VP, & 1.00000 \nonumber\\
know_he & 1.00000 \nonumber\\
propose & 1.00000 \nonumber\\
not_propose & 1.00000 \nonumber\\
separate_but & 1.00000 \nonumber\\
for_homosexual & 1.00000 \nonumber\\
ProductionRule_VP->NP,S, & 1.00000 \nonumber\\
same_as & 1.00000 \nonumber\\
within & 1.00000 \nonumber\\
most_interest & 1.00000 \nonumber\\
not_drink & 1.00000 \nonumber\\
interest_man & 1.00000 \nonumber\\
he_drink & 1.00000 \nonumber\\
drink_do & 1.00000 \nonumber\\
do_equi & 1.00000 \nonumber\\
man_on & 1.00000 \nonumber\\
equi & 1.00000 \nonumber\\
equi_, & 1.00000 \nonumber\\
settlement & 1.00000 \nonumber\\
do_nothing & 1.00000 \nonumber\\
ProductionRule_UCP->FRAG,CC,SBAR, & 1.00000 \nonumber\\
pest_at & 1.00000 \nonumber\\
around_, & 1.00000 \nonumber\\
of_pest & 1.00000 \nonumber\\
and_william & 1.00000 \nonumber\\
suffer_from & 1.00000 \nonumber\\
be_suffer & 1.00000 \nonumber\\
solution_himself & 1.00000 \nonumber\\
_pos_ngram_PP_ADV_NN & 1.00000 \nonumber\\
i_probably & 1.00000 \nonumber\\
you_really & 1.00000 \nonumber\\
same_right & 1.00000 \nonumber\\
i_argue & 1.00000 \nonumber\\
ProductionRule_NP->NP,PP,,,SBAR, & 1.00000 \nonumber\\
who_deserve & 1.00000 \nonumber\\
life_as & 1.00000 \nonumber\\
them_would & 1.00000 \nonumber\\
ProductionRule_VP->ADVP,VB,NP, & 1.00000 \nonumber\\
for_man & 1.00000 \nonumber\\
ff_ie & 1.00000 \nonumber\\
on_why & 1.00000 \nonumber\\
the_number & 1.00000 \nonumber\\
listless & 1.00000 \nonumber\\
ProductionRule_NP->JJ,-LRB-, & 1.00000 \nonumber\\
why_ff & 1.00000 \nonumber\\
be_listless & 1.00000 \nonumber\\
listless_( & 1.00000 \nonumber\\
reason_on & 1.00000 \nonumber\\
(_: & 1.00000 \nonumber\\
of_book & 1.00000 \nonumber\\
one_woman & 1.00000 \nonumber\\
they_probably & 1.00000 \nonumber\\
ProductionRule_NP->NP,PP,ADVP,NP, & 1.00000 \nonumber\\
happen_in & 1.00000 \nonumber\\
resort_. & 1.00000 \nonumber\\
misbehave & 1.00000 \nonumber\\
be_misbehave & 1.00000 \nonumber\\
child_when & 1.00000 \nonumber\\
on_spank & 1.00000 \nonumber\\
misbehave_. & 1.00000 \nonumber\\
seem_necessary & 1.00000 \nonumber\\
not_rely & 1.00000 \nonumber\\
sometime_seem & 1.00000 \nonumber\\
may_sometime & 1.00000 \nonumber\\
ProductionRule_PP->PP,NP, & 1.00000 \nonumber\\
none_of & 1.00000 \nonumber\\
of_plastic & 1.00000 \nonumber\\
rare_and & 1.00000 \nonumber\\
be_counter & 1.00000 \nonumber\\
drug_if & 1.00000 \nonumber\\
seek_medical & 1.00000 \nonumber\\
counter_with & 1.00000 \nonumber\\
the_assault & 1.00000 \nonumber\\
medical_attention & 1.00000 \nonumber\\
very_rare & 1.00000 \nonumber\\
contraceptive_drug & 1.00000 \nonumber\\
contraceptive & 1.00000 \nonumber\\
situation_be & 1.00000 \nonumber\\
attention_after & 1.00000 \nonumber\\
usually_be & 1.00000 \nonumber\\
a_contraceptive & 1.00000 \nonumber\\
can_usually & 1.00000 \nonumber\\
woman_seek & 1.00000 \nonumber\\
that_situation & 1.00000 \nonumber\\
ur_health & 1.00000 \nonumber\\
_pos_ngram_ADV_CONJ_ADJ & 1.00000 \nonumber\\
smoke_but & 1.00000 \nonumber\\
later_tho & 1.00000 \nonumber\\
smoke_100 & 1.00000 \nonumber\\
they_smoke & 1.00000 \nonumber\\
it_isnot & 1.00000 \nonumber\\
._somker & 1.00000 \nonumber\\
facr_both & 1.00000 \nonumber\\
no_it & 1.00000 \nonumber\\
health_as & 1.00000 \nonumber\\
smoke_be & 1.00000 \nonumber\\
isnot_opponent & 1.00000 \nonumber\\
health_? & 1.00000 \nonumber\\
._somke & 1.00000 \nonumber\\
can_damage & 1.00000 \nonumber\\
serious_effect & 1.00000 \nonumber\\
health_slowly & 1.00000 \nonumber\\
opponent_say & 1.00000 \nonumber\\
slowly_especially & 1.00000 \nonumber\\
doont_have & 1.00000 \nonumber\\
slowly & 1.00000 \nonumber\\
sooner & 1.00000 \nonumber\\
than_porn & 1.00000 \nonumber\\
_pos_ngram_PUNC_ADV_CONJ & 1.00000 \nonumber\\
sooner_or & 1.00000 \nonumber\\
health_i & 1.00000 \nonumber\\
on_health & 1.00000 \nonumber\\
ur_immune & 1.00000 \nonumber\\
especially_ur & 1.00000 \nonumber\\
relationship_definitely & 1.00000 \nonumber\\
same_influence & 1.00000 \nonumber\\
key_question & 1.00000 \nonumber\\
damage_ur & 1.00000 \nonumber\\
isnot & 1.00000 \nonumber\\
facr & 1.00000 \nonumber\\
somker & 1.00000 \nonumber\\
a_serious & 1.00000 \nonumber\\
practice_it & 1.00000 \nonumber\\
tho_who & 1.00000 \nonumber\\
death_and & 1.00000 \nonumber\\
porn_good & 1.00000 \nonumber\\
definitely_they & 1.00000 \nonumber\\
tho & 1.00000 \nonumber\\
that_smoke & 1.00000 \nonumber\\
porn_doont & 1.00000 \nonumber\\
for_ur & 1.00000 \nonumber\\
%_lead & 1.00000 \nonumber\\
a_key & 1.00000 \nonumber\\
to_thier & 1.00000 \nonumber\\
both_of & 1.00000 \nonumber\\
or_later & 1.00000 \nonumber\\
however_study & 1.00000 \nonumber\\
immune_system & 1.00000 \nonumber\\
but_smoke & 1.00000 \nonumber\\
extremely_bid & 1.00000 \nonumber\\
somker_feel & 1.00000 \nonumber\\
influence_on & 1.00000 \nonumber\\
in_facr & 1.00000 \nonumber\\
porn_in & 1.00000 \nonumber\\
u_. & 1.00000 \nonumber\\
._sooner & 1.00000 \nonumber\\
they_donot & 1.00000 \nonumber\\
do_porn & 1.00000 \nonumber\\
somke & 1.00000 \nonumber\\
doont & 1.00000 \nonumber\\
somke_be & 1.00000 \nonumber\\
thier_death & 1.00000 \nonumber\\
for_u & 1.00000 \nonumber\\
thier_relationship & 1.00000 \nonumber\\
dan_oxígeno & 1.00000 \nonumber\\
,_meno & 1.00000 \nonumber\\
una & 1.00000 \nonumber\\
una_planta & 1.00000 \nonumber\\
oxígeno & 1.00000 \nonumber\\
ahora_en & 1.00000 \nonumber\\
niega_que & 1.00000 \nonumber\\
un_" & 1.00000 \nonumber\\
no_e & 1.00000 \nonumber\\
eso & 1.00000 \nonumber\\
al_igual & 1.00000 \nonumber\\
al & 1.00000 \nonumber\\
,_pero & 1.00000 \nonumber\\
que & 1.00000 \nonumber\\
ProductionRule_NP->NP,,,NP,,,NP, & 1.00000 \nonumber\\
me_atrevería & 1.00000 \nonumber\\
vida_, & 1.00000 \nonumber\\
,_al & 1.00000 \nonumber\\
una_vida & 1.00000 \nonumber\\
dan & 1.00000 \nonumber\\
planta_, & 1.00000 \nonumber\\
vida & 1.00000 \nonumber\\
eso_a & 1.00000 \nonumber\\
ProductionRule_NP->NN,FW,FW, & 1.00000 \nonumber\\
que_hace & 1.00000 \nonumber\\
más & 1.00000 \nonumber\\
,_lo & 1.00000 \nonumber\\
un_parásito & 1.00000 \nonumber\\
ProductionRule_NP->DT,FW,FW,FW,FW,FW, & 1.00000 \nonumber\\
,_aunque & 1.00000 \nonumber\\
un_ser & 1.00000 \nonumber\\
ProductionRule_NP->FW,FW,FW,FW,FW,FW,FW,FW,FW, & 1.00000 \nonumber\\
ProductionRule_NP->DT,FW,FW,FW,FW,FW,FW,FW,FW, & 1.00000 \nonumber\\
animale_el & 1.00000 \nonumber\\
niega & 1.00000 \nonumber\\
ProductionRule_NP->FW,FW,FW,FW,FW,FW,FW,FW, & 1.00000 \nonumber\\
planta_no & 1.00000 \nonumber\\
bebé_, & 1.00000 \nonumber\\
querido_idioma & 1.00000 \nonumber\\
ProductionRule_NP->DT,FW,FW,NNP, & 1.00000 \nonumber\\
ProductionRule_NP->FW,FW,FW,FW,FW,FW, & 1.00000 \nonumber\\
más_que & 1.00000 \nonumber\\
oxígeno_... & 1.00000 \nonumber\\
en & 1.00000 \nonumber\\
querido & 1.00000 \nonumber\\
que_una & 1.00000 \nonumber\\
que_suelen & 1.00000 \nonumber\\
que_e & 1.00000 \nonumber\\
ahora & 1.00000 \nonumber\\
más_a & 1.00000 \nonumber\\
matar & 1.00000 \nonumber\\
no_puede & 1.00000 \nonumber\\
no_dan & 1.00000 \nonumber\\
,_que & 1.00000 \nonumber\\
que_la & 1.00000 \nonumber\\
que_a & 1.00000 \nonumber\\
ProductionRule_NP->JJ,,,JJ,NN,NN, & 1.00000 \nonumber\\
matar_a & 1.00000 \nonumber\\
que_llaman & 1.00000 \nonumber\\
,_un & 1.00000 \nonumber\\
planta & 1.00000 \nonumber\\
en_mi & 1.00000 \nonumber\\
que_sea & 1.00000 \nonumber\\
la_planta & 1.00000 \nonumber\\
la & 1.00000 \nonumber\\
bebé & 1.00000 \nonumber\\
animale & 1.00000 \nonumber\\
único_que & 1.00000 \nonumber\\
e_chupar & 1.00000 \nonumber\\
chupar_recurso & 1.00000 \nonumber\\
mi & 1.00000 \nonumber\\
pero_no & 1.00000 \nonumber\\
aborto & 1.00000 \nonumber\\
único & 1.00000 \nonumber\\
a_un & 1.00000 \nonumber\\
"_bebé & 1.00000 \nonumber\\
"_no & 1.00000 \nonumber\\
suelen_decir & 1.00000 \nonumber\\
sea & 1.00000 \nonumber\\
suelen & 1.00000 \nonumber\\
sea_una & 1.00000 \nonumber\\
aunque & 1.00000 \nonumber\\
humano_que & 1.00000 \nonumber\\
decir & 1.00000 \nonumber\\
humano_" & 1.00000 \nonumber\\
humano & 1.00000 \nonumber\\
sentir & 1.00000 \nonumber\\
decir_lo & 1.00000 \nonumber\\
sentir_nus & 1.00000 \nonumber\\
nadie & 1.00000 \nonumber\\
idioma_, & 1.00000 \nonumber\\
idioma & 1.00000 \nonumber\\
puede & 1.00000 \nonumber\\
a_decir & 1.00000 \nonumber\\
meno & 1.00000 \nonumber\\
_pos_ngram_O_ART_O & 1.00000 \nonumber\\
pensar_, & 1.00000 \nonumber\\
mi_querido & 1.00000 \nonumber\\
meno_, & 1.00000 \nonumber\\
aunque_la & 1.00000 \nonumber\\
a_lo & 1.00000 \nonumber\\
decir_que & 1.00000 \nonumber\\
chupar & 1.00000 \nonumber\\
nus_pensar & 1.00000 \nonumber\\
diré & 1.00000 \nonumber\\
lo_único & 1.00000 \nonumber\\
ser & 1.00000 \nonumber\\
ser_humano & 1.00000 \nonumber\\
e_más & 1.00000 \nonumber\\
atrevería_a & 1.00000 \nonumber\\
diré_eso & 1.00000 \nonumber\\
lo_diré & 1.00000 \nonumber\\
el_aborto & 1.00000 \nonumber\\
lo_humano & 1.00000 \nonumber\\
e_matar & 1.00000 \nonumber\\
lo_que & 1.00000 \nonumber\\
atrevería & 1.00000 \nonumber\\
e_lo & 1.00000 \nonumber\\
el & 1.00000 \nonumber\\
nus & 1.00000 \nonumber\\
lo_animale & 1.00000 \nonumber\\
..._nadie & 1.00000 \nonumber\\
llaman & 1.00000 \nonumber\\
pensar & 1.00000 \nonumber\\
aborto_e & 1.00000 \nonumber\\
recurso & 1.00000 \nonumber\\
recurso_, & 1.00000 \nonumber\\
llaman_un & 1.00000 \nonumber\\
pero & 1.00000 \nonumber\\
nadie_niega & 1.00000 \nonumber\\
hace_e & 1.00000 \nonumber\\
hace_más & 1.00000 \nonumber\\
igual & 1.00000 \nonumber\\
igual_que & 1.00000 \nonumber\\
lo & 1.00000 \nonumber\\
puede_sentir & 1.00000 \nonumber\\
hace & 1.00000 \nonumber\\
experiment & 1.00000 \nonumber\\
it_out & 1.00000 \nonumber\\
the_time & 1.00000 \nonumber\\
as_we & 1.00000 \nonumber\\
electricity_. & 1.00000 \nonumber\\
google & 1.00000 \nonumber\\
,_shinto & 1.00000 \nonumber\\
,_buddhism & 1.00000 \nonumber\\
?_also & 1.00000 \nonumber\\
judaism_one & 1.00000 \nonumber\\
you_forget & 1.00000 \nonumber\\
question_? & 1.00000 \nonumber\\
buddhism_, & 1.00000 \nonumber\\
forget_all & 1.00000 \nonumber\\
_pos_ngram_NP_CARD_CONJ & 1.00000 \nonumber\\
._hinduism & 1.00000 \nonumber\\
,_islam & 1.00000 \nonumber\\
n't_stand & 1.00000 \nonumber\\
stand_that & 1.00000 \nonumber\\
shinto_, & 1.00000 \nonumber\\
shinto & 1.00000 \nonumber\\
please_, & 1.00000 \nonumber\\
_pos_ngram_ADJ_NN_CARD & 1.00000 \nonumber\\
very_good & 1.00000 \nonumber\\
so-call_plan & 1.00000 \nonumber\\
since_raffle & 1.00000 \nonumber\\
make_some & 1.00000 \nonumber\\
do_make & 1.00000 \nonumber\\
plan_of & 1.00000 \nonumber\\
leave_for & 1.00000 \nonumber\\
,_too & 1.00000 \nonumber\\
ProductionRule_NP->PDT,DT,JJ,NN, & 1.00000 \nonumber\\
ProductionRule_VP->VB,NP,,,ADVP,,,SBAR, & 1.00000 \nonumber\\
to_plan & 1.00000 \nonumber\\
for_bencoolen & 1.00000 \nonumber\\
this_means & 1.00000 \nonumber\\
in_love & 1.00000 \nonumber\\
to_exist & 1.00000 \nonumber\\
fat_kid & 1.00000 \nonumber\\
p.e & 1.00000 \nonumber\\
rare & 1.00000 \nonumber\\
stamen & 1.00000 \nonumber\\
lesser_stamen & 1.00000 \nonumber\\
lesser & 1.00000 \nonumber\\
ProductionRule_NP->NNP,NNP,NNP,., & 1.00000 \nonumber\\
well_well & 1.00000 \nonumber\\
suitable_for & 1.00000 \nonumber\\
stamen_and & 1.00000 \nonumber\\
less_intensive & 1.00000 \nonumber\\
muscle_cramp & 1.00000 \nonumber\\
._really & 1.00000 \nonumber\\
for_less & 1.00000 \nonumber\\
intensive & 1.00000 \nonumber\\
for_long & 1.00000 \nonumber\\
intensive_exercise & 1.00000 \nonumber\\
contrast_, & 1.00000 \nonumber\\
contrast & 1.00000 \nonumber\\
same_? & 1.00000 \nonumber\\
distance_run & 1.00000 \nonumber\\
force_everyone & 1.00000 \nonumber\\
do_intensive & 1.00000 \nonumber\\
long_distance & 1.00000 \nonumber\\
some_maybe & 1.00000 \nonumber\\
everyone_to & 1.00000 \nonumber\\
have_longer & 1.00000 \nonumber\\
have_lesser & 1.00000 \nonumber\\
exercise_like & 1.00000 \nonumber\\
be_suitable & 1.00000 \nonumber\\
only_suitable & 1.00000 \nonumber\\
have_muscle & 1.00000 \nonumber\\
more_intensive & 1.00000 \nonumber\\
over_when & 1.00000 \nonumber\\
cramp_all & 1.00000 \nonumber\\
cramp & 1.00000 \nonumber\\
why_force & 1.00000 \nonumber\\
in_contrast & 1.00000 \nonumber\\
distance & 1.00000 \nonumber\\
_pos_ngram_ART_PP_ADV & 1.00000 \nonumber\\
longer_stamen & 1.00000 \nonumber\\
make_different & 1.00000 \nonumber\\
mandatory_because & 1.00000 \nonumber\\
this_world & 1.00000 \nonumber\\
the_true & 1.00000 \nonumber\\
neither_. & 1.00000 \nonumber\\
n't_- & 1.00000 \nonumber\\
prove_this & 1.00000 \nonumber\\
true_answer & 1.00000 \nonumber\\
personally_believe & 1.00000 \nonumber\\
this_definitely & 1.00000 \nonumber\\
definitely_. & 1.00000 \nonumber\\
._agnostic & 1.00000 \nonumber\\
-_but & 1.00000 \nonumber\\
never_prove & 1.00000 \nonumber\\
god_but & 1.00000 \nonumber\\
agnostic_be & 1.00000 \nonumber\\
board & 1.00000 \nonumber\\
over_board & 1.00000 \nonumber\\
go_over & 1.00000 \nonumber\\
only_spank & 1.00000 \nonumber\\
keep_hit & 1.00000 \nonumber\\
spank_then & 1.00000 \nonumber\\
board_and & 1.00000 \nonumber\\
your_too & 1.00000 \nonumber\\
degrade_by & 1.00000 \nonumber\\
crazy_. & 1.00000 \nonumber\\
fit_and & 1.00000 \nonumber\\
meg_of & 1.00000 \nonumber\\
one_week & 1.00000 \nonumber\\
under_task & 1.00000 \nonumber\\
a_sieve & 1.00000 \nonumber\\
meg & 1.00000 \nonumber\\
use_250 & 1.00000 \nonumber\\
leak_memory & 1.00000 \nonumber\\
,_three & 1.00000 \nonumber\\
ProductionRule_NP->NP,-LRB-,CC,NP,-RRB-, & 1.00000 \nonumber\\
firefox_( & 1.00000 \nonumber\\
)_leak & 1.00000 \nonumber\\
firefox_2.0.0.1 & 1.00000 \nonumber\\
the_extension & 1.00000 \nonumber\\
three_tab & 1.00000 \nonumber\\
open_session & 1.00000 \nonumber\\
manager & 1.00000 \nonumber\\
250 & 1.00000 \nonumber\\
extension_) & 1.00000 \nonumber\\
manager_on & 1.00000 \nonumber\\
an_open & 1.00000 \nonumber\\
,_use & 1.00000 \nonumber\\
session_of & 1.00000 \nonumber\\
2.0.0.1_, & 1.00000 \nonumber\\
_pos_ngram_O_PUNC_CARD & 1.00000 \nonumber\\
memory_under & 1.00000 \nonumber\\
sieve_. & 1.00000 \nonumber\\
2.0.0.1 & 1.00000 \nonumber\\
_pos_ngram_PUNC_V_CARD & 1.00000 \nonumber\\
memory_like & 1.00000 \nonumber\\
on_window & 1.00000 \nonumber\\
sieve & 1.00000 \nonumber\\
250_meg & 1.00000 \nonumber\\
task_manager & 1.00000 \nonumber\\
thing_so & 1.00000 \nonumber\\
around_come & 1.00000 \nonumber\\
alot_of & 1.00000 \nonumber\\
lookin & 1.00000 \nonumber\\
than_look & 1.00000 \nonumber\\
lookin_out & 1.00000 \nonumber\\
please_yourself & 1.00000 \nonumber\\
i_fall & 1.00000 \nonumber\\
other_wo & 1.00000 \nonumber\\
like_advance & 1.00000 \nonumber\\
themselve_rather & 1.00000 \nonumber\\
to_please & 1.00000 \nonumber\\
fall_like & 1.00000 \nonumber\\
before_lookin & 1.00000 \nonumber\\
goods_be & 1.00000 \nonumber\\
of_good & 1.00000 \nonumber\\
around_thing & 1.00000 \nonumber\\
but_something & 1.00000 \nonumber\\
good_will & 1.00000 \nonumber\\
common_goods & 1.00000 \nonumber\\
_pos_ngram_ADJ_PR_PUNC & 1.00000 \nonumber\\
do_alot & 1.00000 \nonumber\\
the_what & 1.00000 \nonumber\\
the_classic & 1.00000 \nonumber\\
familiar_with & 1.00000 \nonumber\\
process_both & 1.00000 \nonumber\\
a_diet & 1.00000 \nonumber\\
diet_plan & 1.00000 \nonumber\\
evolution_- & 1.00000 \nonumber\\
evolutionary_process & 1.00000 \nonumber\\
not_evolution & 1.00000 \nonumber\\
ProductionRule_NP->DT,JJ,JJ,NN,NN, & 1.00000 \nonumber\\
moth_argument & 1.00000 \nonumber\\
prey_to & 1.00000 \nonumber\\
very_familiar & 1.00000 \nonumber\\
familiar & 1.00000 \nonumber\\
ProductionRule_FRAG->NP,NP,PP,S,., & 1.00000 \nonumber\\
there_its & 1.00000 \nonumber\\
moth_color & 1.00000 \nonumber\\
prey & 1.00000 \nonumber\\
color_have & 1.00000 \nonumber\\
-_that & 1.00000 \nonumber\\
argument_i & 1.00000 \nonumber\\
ah_yes & 1.00000 \nonumber\\
classic_pepper & 1.00000 \nonumber\\
the_evolutionary & 1.00000 \nonumber\\
their_prey & 1.00000 \nonumber\\
allow_your & 1.00000 \nonumber\\
than_do & 1.00000 \nonumber\\
you_write & 1.00000 \nonumber\\
book_teach & 1.00000 \nonumber\\
n't_ruin & 1.00000 \nonumber\\
book_a & 1.00000 \nonumber\\
write_better & 1.00000 \nonumber\\
brain_to & 1.00000 \nonumber\\
with_spell & 1.00000 \nonumber\\
imagine_rather & 1.00000 \nonumber\\
spell_. & 1.00000 \nonumber\\
ruin_your & 1.00000 \nonumber\\
book_allow & 1.00000 \nonumber\\
eye_like & 1.00000 \nonumber\\
._watch & 1.00000 \nonumber\\
._5 & 1.00000 \nonumber\\
you_with & 1.00000 \nonumber\\
lot_can & 1.00000 \nonumber\\
highest & 1.00000 \nonumber\\
ProductionRule_VP->VBP,ADVP,PP,SBAR, & 1.00000 \nonumber\\
feel_secure & 1.00000 \nonumber\\
get_older & 1.00000 \nonumber\\
then_fatherless & 1.00000 \nonumber\\
without_. & 1.00000 \nonumber\\
secure_in & 1.00000 \nonumber\\
'_who & 1.00000 \nonumber\\
in_another & 1.00000 \nonumber\\
,_mother & 1.00000 \nonumber\\
careless_then & 1.00000 \nonumber\\
which_should & 1.00000 \nonumber\\
older_. & 1.00000 \nonumber\\
careless & 1.00000 \nonumber\\
responsiblity & 1.00000 \nonumber\\
._boy & 1.00000 \nonumber\\
responsiblity_as & 1.00000 \nonumber\\
boy_, & 1.00000 \nonumber\\
have_father & 1.00000 \nonumber\\
but_father & 1.00000 \nonumber\\
see_girl & 1.00000 \nonumber\\
girl_for & 1.00000 \nonumber\\
girl_without & 1.00000 \nonumber\\
girl_who & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,ADJP,S,,,SBAR, & 1.00000 \nonumber\\
give_that & 1.00000 \nonumber\\
huge_impact & 1.00000 \nonumber\\
certain_sense & 1.00000 \nonumber\\
hard_life & 1.00000 \nonumber\\
father_just & 1.00000 \nonumber\\
ProductionRule_VP->ADVP,VBG,PP, & 1.00000 \nonumber\\
father_give & 1.00000 \nonumber\\
then_girl & 1.00000 \nonumber\\
another_way & 1.00000 \nonumber\\
ProductionRule_VP->ADVP,VBZ, & 1.00000 \nonumber\\
mother_give & 1.00000 \nonumber\\
probably_feel & 1.00000 \nonumber\\
,_girl & 1.00000 \nonumber\\
fatherly_responsiblity & 1.00000 \nonumber\\
less_careless & 1.00000 \nonumber\\
the_new & 1.00000 \nonumber\\
think_advance & 1.00000 \nonumber\\
like_me & 1.00000 \nonumber\\
break_in & 1.00000 \nonumber\\
child_get & 1.00000 \nonumber\\
explorer_7 & 1.00000 \nonumber\\
barely & 1.00000 \nonumber\\
and_no & 1.00000 \nonumber\\
cause_them & 1.00000 \nonumber\\
really_depend & 1.00000 \nonumber\\
close_to & 1.00000 \nonumber\\
significant & 1.00000 \nonumber\\
_pos_ngram_ADV_PR_ART & 1.00000 \nonumber\\
happen_when & 1.00000 \nonumber\\
acceptable & 1.00000 \nonumber\\
barrel_of & 1.00000 \nonumber\\
include_the & 1.00000 \nonumber\\
year-and & 1.00000 \nonumber\\
'_enough & 1.00000 \nonumber\\
100,000_automobile & 1.00000 \nonumber\\
year-and_that & 1.00000 \nonumber\\
to_power & 1.00000 \nonumber\\
_pos_ngram_ART_NP_ADJ & 1.00000 \nonumber\\
over_1.5 & 1.00000 \nonumber\\
power_100,000 & 1.00000 \nonumber\\
petroleum & 1.00000 \nonumber\\
petroleum_to & 1.00000 \nonumber\\
bottle_consume & 1.00000 \nonumber\\
last_year-and & 1.00000 \nonumber\\
automobile_for & 1.00000 \nonumber\\
consume_in & 1.00000 \nonumber\\
petroleum_use & 1.00000 \nonumber\\
the_petroleum & 1.00000 \nonumber\\
automobile & 1.00000 \nonumber\\
enough_petroleum & 1.00000 \nonumber\\
us_last & 1.00000 \nonumber\\
to_transport & 1.00000 \nonumber\\
ProductionRule_NP->DT,NNP,JJ,NN, & 1.00000 \nonumber\\
barrel & 1.00000 \nonumber\\
oil_be & 1.00000 \nonumber\\
the_us & 1.00000 \nonumber\\
a_year & 1.00000 \nonumber\\
ProductionRule_NP->CD,CD, & 1.00000 \nonumber\\
n't_include & 1.00000 \nonumber\\
transport_them & 1.00000 \nonumber\\
100,000 & 1.00000 \nonumber\\
million_barrel & 1.00000 \nonumber\\
1.5 & 1.00000 \nonumber\\
1.5_million & 1.00000 \nonumber\\
of_oil & 1.00000 \nonumber\\
violate & 1.00000 \nonumber\\
not_alone & 1.00000 \nonumber\\
drown & 1.00000 \nonumber\\
u_be & 1.00000 \nonumber\\
be_drown & 1.00000 \nonumber\\
n't_worryz & 1.00000 \nonumber\\
worryz & 1.00000 \nonumber\\
worryz_potato & 1.00000 \nonumber\\
drown_, & 1.00000 \nonumber\\
drown_. & 1.00000 \nonumber\\
potato_u & 1.00000 \nonumber\\
the_fish & 1.00000 \nonumber\\
as_guideline & 1.00000 \nonumber\\
other_fellow & 1.00000 \nonumber\\
be_lose & 1.00000 \nonumber\\
fellow & 1.00000 \nonumber\\
against_human & 1.00000 \nonumber\\
ProductionRule_VP->VBP,``,NP, & 1.00000 \nonumber\\
religion_from & 1.00000 \nonumber\\
have_faith & 1.00000 \nonumber\\
vote_" & 1.00000 \nonumber\\
guideline_to & 1.00000 \nonumber\\
fellow_voter & 1.00000 \nonumber\\
act_as & 1.00000 \nonumber\\
voter & 1.00000 \nonumber\\
faith_or & 1.00000 \nonumber\\
n't_exclude & 1.00000 \nonumber\\
nature_and & 1.00000 \nonumber\\
"_wrong & 1.00000 \nonumber\\
mention_, & 1.00000 \nonumber\\
exclude & 1.00000 \nonumber\\
or_belief & 1.00000 \nonumber\\
any_religion & 1.00000 \nonumber\\
have_mention & 1.00000 \nonumber\\
exclude_religion & 1.00000 \nonumber\\
voter_have & 1.00000 \nonumber\\
without_it & 1.00000 \nonumber\\
outlaw_pornography & 1.00000 \nonumber\\
the_question & 1.00000 \nonumber\\
would_there & 1.00000 \nonumber\\
you_? & 1.00000 \nonumber\\
europe_, & 1.00000 \nonumber\\
to_prohibit & 1.00000 \nonumber\\
press & 1.00000 \nonumber\\
question_be & 1.00000 \nonumber\\
europe_- & 1.00000 \nonumber\\
?_look & 1.00000 \nonumber\\
depravity & 1.00000 \nonumber\\
press_need & 1.00000 \nonumber\\
?_government & 1.00000 \nonumber\\
depravity_in & 1.00000 \nonumber\\
any_moral & 1.00000 \nonumber\\
any_press & 1.00000 \nonumber\\
state_to & 1.00000 \nonumber\\
prohibit_it & 1.00000 \nonumber\\
prohibit & 1.00000 \nonumber\\
cool_with & 1.00000 \nonumber\\
outlaw & 1.00000 \nonumber\\
:_who & 1.00000 \nonumber\\
much_everything & 1.00000 \nonumber\\
pornography_? & 1.00000 \nonumber\\
to_outlaw & 1.00000 \nonumber\\
be_: & 1.00000 \nonumber\\
moral_depravity & 1.00000 \nonumber\\
with_pretty & 1.00000 \nonumber\\
government_? & 1.00000 \nonumber\\
at_europe & 1.00000 \nonumber\\
her_next & 1.00000 \nonumber\\
ProductionRule_VP->ADVP,VBD,NP, & 1.00000 \nonumber\\
impossible_to & 1.00000 \nonumber\\
my_belief & 1.00000 \nonumber\\
seek_the & 1.00000 \nonumber\\
find_more & 1.00000 \nonumber\\
lord_until & 1.00000 \nonumber\\
more_peace & 1.00000 \nonumber\\
peace_in & 1.00000 \nonumber\\
i_die & 1.00000 \nonumber\\
to_seek & 1.00000 \nonumber\\
to_prevent & 1.00000 \nonumber\\
snitch & 1.00000 \nonumber\\
or_who & 1.00000 \nonumber\\
look_nice & 1.00000 \nonumber\\
'_make & 1.00000 \nonumber\\
tidy & 1.00000 \nonumber\\
that_who & 1.00000 \nonumber\\
spend_to & 1.00000 \nonumber\\
finally_it & 1.00000 \nonumber\\
tidy_. & 1.00000 \nonumber\\
clothe_to & 1.00000 \nonumber\\
convenient_because & 1.00000 \nonumber\\
and_finally & 1.00000 \nonumber\\
can_know & 1.00000 \nonumber\\
and_tidy & 1.00000 \nonumber\\
same_school & 1.00000 \nonumber\\
second_we & 1.00000 \nonumber\\
'_convenient & 1.00000 \nonumber\\
a_same & 1.00000 \nonumber\\
which_school & 1.00000 \nonumber\\
with_us & 1.00000 \nonumber\\
for_learn & 1.00000 \nonumber\\
gay_be & 1.00000 \nonumber\\
you_say & 1.00000 \nonumber\\
be_odd & 1.00000 \nonumber\\
odd & 1.00000 \nonumber\\
this_site & 1.00000 \nonumber\\
ProductionRule_NP->NP,CC,SBAR, & 1.00000 \nonumber\\
ProductionRule_SINV->PP,VP,SBAR,., & 1.00000 \nonumber\\
defend_it & 1.00000 \nonumber\\
and_defend & 1.00000 \nonumber\\
odd_be & 1.00000 \nonumber\\
start_with & 1.00000 \nonumber\\
it_? & 1.00000 \nonumber\\
damage_then & 1.00000 \nonumber\\
relationship_be & 1.00000 \nonumber\\
damage_as & 1.00000 \nonumber\\
;_mom & 1.00000 \nonumber\\
affect_their & 1.00000 \nonumber\\
damage_of & 1.00000 \nonumber\\
far_greater & 1.00000 \nonumber\\
and_dad & 1.00000 \nonumber\\
'_character & 1.00000 \nonumber\\
that_relationship & 1.00000 \nonumber\\
personality_far & 1.00000 \nonumber\\
parent_affect & 1.00000 \nonumber\\
two_role & 1.00000 \nonumber\\
behavior_and & 1.00000 \nonumber\\
be_damage & 1.00000 \nonumber\\
my_personality & 1.00000 \nonumber\\
model_; & 1.00000 \nonumber\\
greater_than & 1.00000 \nonumber\\
mom_and & 1.00000 \nonumber\\
would_scar & 1.00000 \nonumber\\
character_can & 1.00000 \nonumber\\
personality_so & 1.00000 \nonumber\\
scar_my & 1.00000 \nonumber\\
prime_minister & 1.00000 \nonumber\\
,_like & 1.00000 \nonumber\\
ProductionRule_WHNP->WDT,NN, & 1.00000 \nonumber\\
,_his & 1.00000 \nonumber\\
guilt_of & 1.00000 \nonumber\\
cut & 1.00000 \nonumber\\
know_many & 1.00000 \nonumber\\
many_child & 1.00000 \nonumber\\
,_adoption & 1.00000 \nonumber\\
ProductionRule_VP->,,S, & 1.00000 \nonumber\\
decide_one & 1.00000 \nonumber\\
guess_. & 1.00000 \nonumber\\
but_who & 1.00000 \nonumber\\
them_suffer & 1.00000 \nonumber\\
abortion_to & 1.00000 \nonumber\\
woman_pregnancy & 1.00000 \nonumber\\
suffer_. & 1.00000 \nonumber\\
n't_and & 1.00000 \nonumber\\
adopt_but & 1.00000 \nonumber\\
get_adopt & 1.00000 \nonumber\\
only_other & 1.00000 \nonumber\\
or_keep & 1.00000 \nonumber\\
better_off & 1.00000 \nonumber\\
to_let & 1.00000 \nonumber\\
chance_they & 1.00000 \nonumber\\
many_do & 1.00000 \nonumber\\
but_many & 1.00000 \nonumber\\
caste & 1.00000 \nonumber\\
be_together & 1.00000 \nonumber\\
other_what & 1.00000 \nonumber\\
tv_help & 1.00000 \nonumber\\
interaction_with & 1.00000 \nonumber\\
through_interaction & 1.00000 \nonumber\\
learn_english & 1.00000 \nonumber\\
native & 1.00000 \nonumber\\
speaker & 1.00000 \nonumber\\
._technically & 1.00000 \nonumber\\
speaker_, & 1.00000 \nonumber\\
through_tv & 1.00000 \nonumber\\
technically_, & 1.00000 \nonumber\\
english_through & 1.00000 \nonumber\\
i_learn & 1.00000 \nonumber\\
native_speaker & 1.00000 \nonumber\\
with_native & 1.00000 \nonumber\\
because_tv & 1.00000 \nonumber\\
with_this & 1.00000 \nonumber\\
or_man & 1.00000 \nonumber\\
gratification_other & 1.00000 \nonumber\\
their_spouse & 1.00000 \nonumber\\
disgust_. & 1.00000 \nonumber\\
not_realistic & 1.00000 \nonumber\\
yes_porn & 1.00000 \nonumber\\
man_be & 1.00000 \nonumber\\
up_relationship & 1.00000 \nonumber\\
only_hope & 1.00000 \nonumber\\
need_any & 1.00000 \nonumber\\
be_disgust & 1.00000 \nonumber\\
sexual_gratification & 1.00000 \nonumber\\
to_influence & 1.00000 \nonumber\\
woman_or & 1.00000 \nonumber\\
can_split & 1.00000 \nonumber\\
relationship_then & 1.00000 \nonumber\\
split_up & 1.00000 \nonumber\\
seriously_. & 1.00000 \nonumber\\
._seriously & 1.00000 \nonumber\\
exploit_man & 1.00000 \nonumber\\
exploit & 1.00000 \nonumber\\
realistic_and & 1.00000 \nonumber\\
it_exploit & 1.00000 \nonumber\\
._out & 1.00000 \nonumber\\
than_their & 1.00000 \nonumber\\
hope_to & 1.00000 \nonumber\\
regulate_while & 1.00000 \nonumber\\
strictly_regulate & 1.00000 \nonumber\\
idea_what & 1.00000 \nonumber\\
no_idea & 1.00000 \nonumber\\
while_tap & 1.00000 \nonumber\\
you_drink & 1.00000 \nonumber\\
strictly & 1.00000 \nonumber\\
not_strictly & 1.00000 \nonumber\\
drink_when & 1.00000 \nonumber\\
_pos_ngram_ART_ART_PR & 1.00000 \nonumber\\
the_begin & 1.00000 \nonumber\\
have_none & 1.00000 \nonumber\\
learn_how & 1.00000 \nonumber\\
ProductionRule_NP->NP,,,ADJP, & 1.00000 \nonumber\\
ProductionRule_S->ADVP,NP,ADVP,VP, & 1.00000 \nonumber\\
a_bond/partnership & 1.00000 \nonumber\\
eye_) & 1.00000 \nonumber\\
police_a & 1.00000 \nonumber\\
but_remember & 1.00000 \nonumber\\
bond/partnership_. & 1.00000 \nonumber\\
offense & 1.00000 \nonumber\\
basically_invite & 1.00000 \nonumber\\
5th_amendment & 1.00000 \nonumber\\
bond/partnership & 1.00000 \nonumber\\
my_eye & 1.00000 \nonumber\\
5th & 1.00000 \nonumber\\
ProductionRule_S->NP,,,NP,PRN,VP,., & 1.00000 \nonumber\\
flex_the & 1.00000 \nonumber\\
to_flex & 1.00000 \nonumber\\
flex & 1.00000 \nonumber\\
marry_into & 1.00000 \nonumber\\
still_divorce & 1.00000 \nonumber\\
rat_, & 1.00000 \nonumber\\
her_spouse & 1.00000 \nonumber\\
offense_but & 1.00000 \nonumber\\
amendment_! & 1.00000 \nonumber\\
hesitate & 1.00000 \nonumber\\
wife_where & 1.00000 \nonumber\\
!_murder & 1.00000 \nonumber\\
crazy_chick & 1.00000 \nonumber\\
heavy_offense & 1.00000 \nonumber\\
kudos & 1.00000 \nonumber\\
chick_though & 1.00000 \nonumber\\
,_join & 1.00000 \nonumber\\
the_crazy & 1.00000 \nonumber\\
marriage_( & 1.00000 \nonumber\\
a_rat & 1.00000 \nonumber\\
"_snitch & 1.00000 \nonumber\\
divorce_the & 1.00000 \nonumber\\
a_heavy & 1.00000 \nonumber\\
so_ask & 1.00000 \nonumber\\
??_if & 1.00000 \nonumber\\
though_! & 1.00000 \nonumber\\
snitch_" & 1.00000 \nonumber\\
wouldnt_hesitate & 1.00000 \nonumber\\
you_turn & 1.00000 \nonumber\\
call_anyone & 1.00000 \nonumber\\
,_' & 1.00000 \nonumber\\
hesitate_to & 1.00000 \nonumber\\
to_police & 1.00000 \nonumber\\
join_the & 1.00000 \nonumber\\
family_?? & 1.00000 \nonumber\\
in_family & 1.00000 \nonumber\\
the_5th & 1.00000 \nonumber\\
,_kudos & 1.00000 \nonumber\\
yourself_... & 1.00000 \nonumber\\
kudos_! & 1.00000 \nonumber\\
'_i & 1.00000 \nonumber\\
chick & 1.00000 \nonumber\\
definetly & 1.00000 \nonumber\\
accuse_him & 1.00000 \nonumber\\
accuse & 1.00000 \nonumber\\
him_of & 1.00000 \nonumber\\
negative & 1.00000 \nonumber\\
im_not & 1.00000 \nonumber\\
with_china & 1.00000 \nonumber\\
costly & 1.00000 \nonumber\\
technological & 1.00000 \nonumber\\
technological_development & 1.00000 \nonumber\\
plan_on & 1.00000 \nonumber\\
way_and & 1.00000 \nonumber\\
a_girl & 1.00000 \nonumber\\
eye_on & 1.00000 \nonumber\\
keep_an & 1.00000 \nonumber\\
century_. & 1.00000 \nonumber\\
for_superpower & 1.00000 \nonumber\\
thirty_year & 1.00000 \nonumber\\
next_thirty & 1.00000 \nonumber\\
an_eye & 1.00000 \nonumber\\
ProductionRule_NP->IN,NP, & 1.00000 \nonumber\\
contender & 1.00000 \nonumber\\
status_before & 1.00000 \nonumber\\
on_over & 1.00000 \nonumber\\
personal_list & 1.00000 \nonumber\\
good_contender & 1.00000 \nonumber\\
list_of & 1.00000 \nonumber\\
thirty & 1.00000 \nonumber\\
contender_for & 1.00000 \nonumber\\
superpower_status & 1.00000 \nonumber\\
this_century & 1.00000 \nonumber\\
of_country & 1.00000 \nonumber\\
a_point & 1.00000 \nonumber\\
i_disagree & 1.00000 \nonumber\\
use_spake & 1.00000 \nonumber\\
also_because & 1.00000 \nonumber\\
spake & 1.00000 \nonumber\\
your_children & 1.00000 \nonumber\\
the_children & 1.00000 \nonumber\\
to_dicipline & 1.00000 \nonumber\\
be_learn & 1.00000 \nonumber\\
parent_use & 1.00000 \nonumber\\
disagree & 1.00000 \nonumber\\
dicipline_because & 1.00000 \nonumber\\
spake_as & 1.00000 \nonumber\\
disagree_on & 1.00000 \nonumber\\
children_be & 1.00000 \nonumber\\
learn_what & 1.00000 \nonumber\\
parent_show & 1.00000 \nonumber\\
_pos_ngram_NP_PP_ADV & 1.00000 \nonumber\\
capable_of & 1.00000 \nonumber\\
capable & 1.00000 \nonumber\\
be_capable & 1.00000 \nonumber\\
action_, & 1.00000 \nonumber\\
ha & 1.00000 \nonumber\\
you_prefer & 1.00000 \nonumber\\
other_empire & 1.00000 \nonumber\\
empire_, & 1.00000 \nonumber\\
ProductionRule_FRAG->ADVP,,,ADVP,., & 1.00000 \nonumber\\
ha_, & 1.00000 \nonumber\\
ha_ha & 1.00000 \nonumber\\
even_lead & 1.00000 \nonumber\\
most_successful & 1.00000 \nonumber\\
lead_themselve & 1.00000 \nonumber\\
successful_when & 1.00000 \nonumber\\
_pos_ngram_ART_PUNC_NP & 1.00000 \nonumber\\
by_2013 & 1.00000 \nonumber\\
be_gallop & 1.00000 \nonumber\\
2013_, & 1.00000 \nonumber\\
2013 & 1.00000 \nonumber\\
2018 & 1.00000 \nonumber\\
crisis & 1.00000 \nonumber\\
by_2018 & 1.00000 \nonumber\\
high_growth & 1.00000 \nonumber\\
'_fastest & 1.00000 \nonumber\\
by_myriad & 1.00000 \nonumber\\
long_time & 1.00000 \nonumber\\
magazine & 1.00000 \nonumber\\
sustain_its & 1.00000 \nonumber\\
magazine_. & 1.00000 \nonumber\\
and_might & 1.00000 \nonumber\\
speed_and & 1.00000 \nonumber\\
2018_, & 1.00000 \nonumber\\
enviable & 1.00000 \nonumber\\
pranab & 1.00000 \nonumber\\
crisis_so & 1.00000 \nonumber\\
breakneck_speed & 1.00000 \nonumber\\
feel_finance & 1.00000 \nonumber\\
unit_, & 1.00000 \nonumber\\
plague & 1.00000 \nonumber\\
economist & 1.00000 \nonumber\\
resilient_to & 1.00000 \nonumber\\
economist_agree & 1.00000 \nonumber\\
myriad_problem & 1.00000 \nonumber\\
many_economist & 1.00000 \nonumber\\
a_breakneck & 1.00000 \nonumber\\
mukherjee_and & 1.00000 \nonumber\\
resilient & 1.00000 \nonumber\\
minister_pranab & 1.00000 \nonumber\\
indium_enjoy & 1.00000 \nonumber\\
mukherjee & 1.00000 \nonumber\\
to_economist & 1.00000 \nonumber\\
indium_growth & 1.00000 \nonumber\\
enjoy_could & 1.00000 \nonumber\\
arm_of & 1.00000 \nonumber\\
growth_rate & 1.00000 \nonumber\\
demographic & 1.00000 \nonumber\\
any_global & 1.00000 \nonumber\\
demographic_dividend & 1.00000 \nonumber\\
might_even & 1.00000 \nonumber\\
be_expect & 1.00000 \nonumber\\
finance_minister & 1.00000 \nonumber\\
finance & 1.00000 \nonumber\\
growth_story & 1.00000 \nonumber\\
double-digit_growth & 1.00000 \nonumber\\
global_crisis & 1.00000 \nonumber\\
breakneck & 1.00000 \nonumber\\
the_economist & 1.00000 \nonumber\\
the_demographic & 1.00000 \nonumber\\
intelligence_unit & 1.00000 \nonumber\\
intelligence & 1.00000 \nonumber\\
growth_by & 1.00000 \nonumber\\
double-digit & 1.00000 \nonumber\\
pranab_mukherjee & 1.00000 \nonumber\\
economist_intelligence & 1.00000 \nonumber\\
to_any & 1.00000 \nonumber\\
indeed_enviable & 1.00000 \nonumber\\
indeed & 1.00000 \nonumber\\
be_plague & 1.00000 \nonumber\\
country_sustain & 1.00000 \nonumber\\
its_high & 1.00000 \nonumber\\
emerge_stronger & 1.00000 \nonumber\\
commerce_minister & 1.00000 \nonumber\\
a_research & 1.00000 \nonumber\\
commerce & 1.00000 \nonumber\\
be_indeed & 1.00000 \nonumber\\
dividend_that & 1.00000 \nonumber\\
dividend & 1.00000 \nonumber\\
gallop_at & 1.00000 \nonumber\\
gallop & 1.00000 \nonumber\\
enviable_. & 1.00000 \nonumber\\
reach_double-digit & 1.00000 \nonumber\\
plague_by & 1.00000 \nonumber\\
economist_magazine & 1.00000 \nonumber\\
sharma_. & 1.00000 \nonumber\\
rate_for & 1.00000 \nonumber\\
sharma & 1.00000 \nonumber\\
fastest_grow & 1.00000 \nonumber\\
even_reach & 1.00000 \nonumber\\
economy_be & 1.00000 \nonumber\\
economy_by & 1.00000 \nonumber\\
minister_anand & 1.00000 \nonumber\\
anand & 1.00000 \nonumber\\
anand_sharma & 1.00000 \nonumber\\
have_emerge & 1.00000 \nonumber\\
ProductionRule_SINV->S,,,VP,NP,., & 1.00000 \nonumber\\
myriad & 1.00000 \nonumber\\
unit & 1.00000 \nonumber\\
could_see & 1.00000 \nonumber\\
research_arm & 1.00000 \nonumber\\
indian_economy & 1.00000 \nonumber\\
more_resilient & 1.00000 \nonumber\\
and_commerce & 1.00000 \nonumber\\
despite_be & 1.00000 \nonumber\\
believe_google & 1.00000 \nonumber\\
chrome & 1.00000 \nonumber\\
the_s & 1.00000 \nonumber\\
chrome_be & 1.00000 \nonumber\\
firefox_crash & 1.00000 \nonumber\\
crash_every & 1.00000 \nonumber\\
s_*** & 1.00000 \nonumber\\
but_firefox & 1.00000 \nonumber\\
*** & 1.00000 \nonumber\\
***_but & 1.00000 \nonumber\\
google_chrome & 1.00000 \nonumber\\
should_only & 1.00000 \nonumber\\
can_prove & 1.00000 \nonumber\\
wasteful & 1.00000 \nonumber\\
idea_because & 1.00000 \nonumber\\
the_project & 1.00000 \nonumber\\
ethnic_group & 1.00000 \nonumber\\
town & 1.00000 \nonumber\\
town_plan & 1.00000 \nonumber\\
1822_, & 1.00000 \nonumber\\
remodel_singapore & 1.00000 \nonumber\\
plan_committee & 1.00000 \nonumber\\
plan_consist & 1.00000 \nonumber\\
be_form & 1.00000 \nonumber\\
as_road & 1.00000 \nonumber\\
area_for & 1.00000 \nonumber\\
land_for & 1.00000 \nonumber\\
plan_to & 1.00000 \nonumber\\
ethnic & 1.00000 \nonumber\\
1822 & 1.00000 \nonumber\\
different_ethnic & 1.00000 \nonumber\\
modern_city & 1.00000 \nonumber\\
october_1822 & 1.00000 \nonumber\\
form_by & 1.00000 \nonumber\\
a_modern & 1.00000 \nonumber\\
government_building & 1.00000 \nonumber\\
and_land & 1.00000 \nonumber\\
other_facility & 1.00000 \nonumber\\
separate_area & 1.00000 \nonumber\\
of_separate & 1.00000 \nonumber\\
committee & 1.00000 \nonumber\\
building & 1.00000 \nonumber\\
in_october & 1.00000 \nonumber\\
to_remodel & 1.00000 \nonumber\\
facility & 1.00000 \nonumber\\
facility_such & 1.00000 \nonumber\\
road_, & 1.00000 \nonumber\\
a_town & 1.00000 \nonumber\\
to_oversee & 1.00000 \nonumber\\
city_. & 1.00000 \nonumber\\
provision & 1.00000 \nonumber\\
consist_of & 1.00000 \nonumber\\
provision_of & 1.00000 \nonumber\\
committee_be & 1.00000 \nonumber\\
conceive_a & 1.00000 \nonumber\\
for_different & 1.00000 \nonumber\\
oversee_the & 1.00000 \nonumber\\
oversee & 1.00000 \nonumber\\
consist & 1.00000 \nonumber\\
for_government & 1.00000 \nonumber\\
ProductionRule_NP->DT,NN,NN,S, & 1.00000 \nonumber\\
raffle_conceive & 1.00000 \nonumber\\
building_. & 1.00000 \nonumber\\
october & 1.00000 \nonumber\\
and_provision & 1.00000 \nonumber\\
group_and & 1.00000 \nonumber\\
for_firefox & 1.00000 \nonumber\\
wife_in & 1.00000 \nonumber\\
not_worth & 1.00000 \nonumber\\
which_complete & 1.00000 \nonumber\\
1837 & 1.00000 \nonumber\\
year_1837 & 1.00000 \nonumber\\
1837_. & 1.00000 \nonumber\\
establish_the & 1.00000 \nonumber\\
its_construction & 1.00000 \nonumber\\
(_now & 1.00000 \nonumber\\
institution_) & 1.00000 \nonumber\\
construction_on & 1.00000 \nonumber\\
singapore_institution & 1.00000 \nonumber\\
complete & 1.00000 \nonumber\\
complete_its & 1.00000 \nonumber\\
institution_( & 1.00000 \nonumber\\
_pos_ngram_NP_O_ADV & 1.00000 \nonumber\\
know_as & 1.00000 \nonumber\\
school_raffle & 1.00000 \nonumber\\
the_police & 1.00000 \nonumber\\
trouble & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,ADVP,ADJP, & 1.00000 \nonumber\\
as_raffle & 1.00000 \nonumber\\
porn_have & 1.00000 \nonumber\\
of_atheism & 1.00000 \nonumber\\
tab_. & 1.00000 \nonumber\\
a_copycat & 1.00000 \nonumber\\
7_, & 1.00000 \nonumber\\
like_internet & 1.00000 \nonumber\\
ProductionRule_NP->NP,NP,,,SBAR, & 1.00000 \nonumber\\
least_firefox & 1.00000 \nonumber\\
copy_firefox & 1.00000 \nonumber\\
copycat & 1.00000 \nonumber\\
firefox_on & 1.00000 \nonumber\\
who_copy & 1.00000 \nonumber\\
copycat_like & 1.00000 \nonumber\\
superior_due & 1.00000 \nonumber\\
far_superior & 1.00000 \nonumber\\
ProductionRule_UCP->ADJP,CC,ADVP, & 1.00000 \nonumber\\
a_smart & 1.00000 \nonumber\\
phone & 1.00000 \nonumber\\
phone_witch & 1.00000 \nonumber\\
to_its & 1.00000 \nonumber\\
incontinent & 1.00000 \nonumber\\
witch & 1.00000 \nonumber\\
witch_be & 1.00000 \nonumber\\
ProductionRule_NP->PRP$,JJR,NN, & 1.00000 \nonumber\\
be_incontinent & 1.00000 \nonumber\\
incontinent_but & 1.00000 \nonumber\\
its_wider & 1.00000 \nonumber\\
wider_variety & 1.00000 \nonumber\\
wider & 1.00000 \nonumber\\
smart_phone & 1.00000 \nonumber\\
tv_on & 1.00000 \nonumber\\
but_now & 1.00000 \nonumber\\
very_convenient & 1.00000 \nonumber\\
do_" & 1.00000 \nonumber\\
husband_kill & 1.00000 \nonumber\\
ProductionRule_ADJP->CD,NN, & 1.00000 \nonumber\\
and_listen & 1.00000 \nonumber\\
so_let & 1.00000 \nonumber\\
ProductionRule_SINV->S,VP,NP,., & 1.00000 \nonumber\\
necessary_. & 1.00000 \nonumber\\
think_and & 1.00000 \nonumber\\
german & 1.00000 \nonumber\\
give_high & 1.00000 \nonumber\\
in_spanish & 1.00000 \nonumber\\
godfather_he & 1.00000 \nonumber\\
fives & 1.00000 \nonumber\\
the_godfather & 1.00000 \nonumber\\
fives_; & 1.00000 \nonumber\\
ProductionRule_NP->RB,JJ,NNS, & 1.00000 \nonumber\\
german_shepherd & 1.00000 \nonumber\\
godfather_' & 1.00000 \nonumber\\
only_high & 1.00000 \nonumber\\
six_he & 1.00000 \nonumber\\
godfather & 1.00000 \nonumber\\
once_teach & 1.00000 \nonumber\\
'_godfather & 1.00000 \nonumber\\
spanish & 1.00000 \nonumber\\
_pos_ngram_NP_PR_ADV & 1.00000 \nonumber\\
to_bark & 1.00000 \nonumber\\
high_fives & 1.00000 \nonumber\\
;_only & 1.00000 \nonumber\\
high_six & 1.00000 \nonumber\\
teach_a & 1.00000 \nonumber\\
bark & 1.00000 \nonumber\\
bark_in & 1.00000 \nonumber\\
spanish_. & 1.00000 \nonumber\\
he_once & 1.00000 \nonumber\\
shepherd_to & 1.00000 \nonumber\\
shepherd & 1.00000 \nonumber\\
a_german & 1.00000 \nonumber\\
child_develop & 1.00000 \nonumber\\
of_express & 1.00000 \nonumber\\
polish_shoe & 1.00000 \nonumber\\
polish & 1.00000 \nonumber\\
neatly & 1.00000 \nonumber\\
oneself & 1.00000 \nonumber\\
oneself_imagine & 1.00000 \nonumber\\
neatly_iron & 1.00000 \nonumber\\
all_neatly & 1.00000 \nonumber\\
shoe_wont & 1.00000 \nonumber\\
emotion_now & 1.00000 \nonumber\\
ProductionRule_NP->NNS,NN,NNS, & 1.00000 \nonumber\\
express_oneself & 1.00000 \nonumber\\
of_ur & 1.00000 \nonumber\\
now_as & 1.00000 \nonumber\\
life_emotion & 1.00000 \nonumber\\
wont_he & 1.00000 \nonumber\\
ur_interveiw & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,NP,PP,ADVP,SBAR, & 1.00000 \nonumber\\
and_well & 1.00000 \nonumber\\
as_for & 1.00000 \nonumber\\
look_good.remember & 1.00000 \nonumber\\
bully_wear & 1.00000 \nonumber\\
no_harm & 1.00000 \nonumber\\
iron_and & 1.00000 \nonumber\\
ProductionRule_VP->RB,ADVP,VBN, & 1.00000 \nonumber\\
iron & 1.00000 \nonumber\\
dress_sense & 1.00000 \nonumber\\
,_pant & 1.00000 \nonumber\\
tie & 1.00000 \nonumber\\
one_bully & 1.00000 \nonumber\\
good.remember_dress & 1.00000 \nonumber\\
good.remember & 1.00000 \nonumber\\
well_polish & 1.00000 \nonumber\\
tie_, & 1.00000 \nonumber\\
pant & 1.00000 \nonumber\\
wear_shirt & 1.00000 \nonumber\\
sense_also & 1.00000 \nonumber\\
pant_all & 1.00000 \nonumber\\
imagine_one & 1.00000 \nonumber\\
student_life & 1.00000 \nonumber\\
,_tie & 1.00000 \nonumber\\
a_part & 1.00000 \nonumber\\
_pos_ngram_CONJ_PUNC_PP & 1.00000 \nonumber\\
to_people & 1.00000 \nonumber\\
emotion & 1.00000 \nonumber\\
bite_of & 1.00000 \nonumber\\
learn_more & 1.00000 \nonumber\\
father_figure & 1.00000 \nonumber\\
about_. & 1.00000 \nonumber\\
shouldnt & 1.00000 \nonumber\\
_pos_ngram_CARD_PUNC_NN & 1.00000 \nonumber\\
ProductionRule_VP->VBD,NP,,,SBAR, & 1.00000 \nonumber\\
_pos_ngram_CARD_V_V & 1.00000 \nonumber\\
want_its & 1.00000 \nonumber\\
coolio & 1.00000 \nonumber\\
be_coolio & 1.00000 \nonumber\\
coolio_hoolio & 1.00000 \nonumber\\
its_coolio & 1.00000 \nonumber\\
hoolio & 1.00000 \nonumber\\
hoolio_, & 1.00000 \nonumber\\
ProductionRule_NP->DT,NNP,NNPS, & 1.00000 \nonumber\\
job_of & 1.00000 \nonumber\\
run_and & 1.00000 \nonumber\\
the_death & 1.00000 \nonumber\\
other_man & 1.00000 \nonumber\\
trauma_would & 1.00000 \nonumber\\
trauma & 1.00000 \nonumber\\
dont_understand & 1.00000 \nonumber\\
rape_" & 1.00000 \nonumber\\
punish_an & 1.00000 \nonumber\\
good_argument & 1.00000 \nonumber\\
an_innocent & 1.00000 \nonumber\\
the_emotional & 1.00000 \nonumber\\
baby_with & 1.00000 \nonumber\\
however_why & 1.00000 \nonumber\\
innocent_baby & 1.00000 \nonumber\\
woman_do & 1.00000 \nonumber\\
'_crime & 1.00000 \nonumber\\
emotional & 1.00000 \nonumber\\
she_could & 1.00000 \nonumber\\
ProductionRule_VP->VBN,'', & 1.00000 \nonumber\\
penalty_for & 1.00000 \nonumber\\
ProductionRule_S->``,SBAR,VP,., & 1.00000 \nonumber\\
would_happen & 1.00000 \nonumber\\
you_punish & 1.00000 \nonumber\\
would_kill & 1.00000 \nonumber\\
death_penalty & 1.00000 \nonumber\\
happen_without & 1.00000 \nonumber\\
emotional_trauma & 1.00000 \nonumber\\
her_wife & 1.00000 \nonumber\\
guy_her & 1.00000 \nonumber\\
hackman & 1.00000 \nonumber\\
hackman_kill & 1.00000 \nonumber\\
would_trust & 1.00000 \nonumber\\
cheat_with & 1.00000 \nonumber\\
her_for & 1.00000 \nonumber\\
wife_that & 1.00000 \nonumber\\
be_cheat & 1.00000 \nonumber\\
gene_hackman & 1.00000 \nonumber\\
relatively_because & 1.00000 \nonumber\\
marry_her & 1.00000 \nonumber\\
because_murder & 1.00000 \nonumber\\
and_marry & 1.00000 \nonumber\\
still_murder & 1.00000 \nonumber\\
,_relatively & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,ADJP,,,SBAR, & 1.00000 \nonumber\\
lord & 1.00000 \nonumber\\
organize & 1.00000 \nonumber\\
vow & 1.00000 \nonumber\\
stick_by & 1.00000 \nonumber\\
on_our & 1.00000 \nonumber\\
alway_teach & 1.00000 \nonumber\\
spank_child & 1.00000 \nonumber\\
to_hurt & 1.00000 \nonumber\\
will_bid & 1.00000 \nonumber\\
child_not & 1.00000 \nonumber\\
their_development & 1.00000 \nonumber\\
we_alway & 1.00000 \nonumber\\
hurt_other & 1.00000 \nonumber\\
ProductionRule_S->SBAR,ADVP,NP,VP, & 1.00000 \nonumber\\
._bottle & 1.00000 \nonumber\\
._different & 1.00000 \nonumber\\
to_sympathize & 1.00000 \nonumber\\
about_why & 1.00000 \nonumber\\
be_remorseful & 1.00000 \nonumber\\
forgive & 1.00000 \nonumber\\
sympathize_with & 1.00000 \nonumber\\
sympathize & 1.00000 \nonumber\\
could_forgive & 1.00000 \nonumber\\
forgive_her & 1.00000 \nonumber\\
remorseful_for & 1.00000 \nonumber\\
ProductionRule_S->S,,,S,CC,S,., & 1.00000 \nonumber\\
remorseful & 1.00000 \nonumber\\
what_have & 1.00000 \nonumber\\
why_she & 1.00000 \nonumber\\
murder_than & 1.00000 \nonumber\\
than_maybe & 1.00000 \nonumber\\
her_about & 1.00000 \nonumber\\
truly_feel & 1.00000 \nonumber\\
the_story & 1.00000 \nonumber\\
story_and & 1.00000 \nonumber\\
can_sympathize & 1.00000 \nonumber\\
the_origin & 1.00000 \nonumber\\
origin_of & 1.00000 \nonumber\\
origin & 1.00000 \nonumber\\
'_no & 1.00000 \nonumber\\
can_only & 1.00000 \nonumber\\
and_lose & 1.00000 \nonumber\\
better_browser & 1.00000 \nonumber\\
sure_you & 1.00000 \nonumber\\
and_that & 1.00000 \nonumber\\
they_do & 1.00000 \nonumber\\
be_incapable & 1.00000 \nonumber\\
incapable_of & 1.00000 \nonumber\\
incapable & 1.00000 \nonumber\\
!_we & 1.00000 \nonumber\\
class_should & 1.00000 \nonumber\\
stronger & 1.00000 \nonumber\\
,_anyone & 1.00000 \nonumber\\
steve & 1.00000 \nonumber\\
watch_all & 1.00000 \nonumber\\
that_only & 1.00000 \nonumber\\
love_may & 1.00000 \nonumber\\
yes_" & 1.00000 \nonumber\\
rather_them & 1.00000 \nonumber\\
than_my & 1.00000 \nonumber\\
_pos_ngram_O_ADV_O & 1.00000 \nonumber\\
husband_die & 1.00000 \nonumber\\
the_side & 1.00000 \nonumber\\
i_put & 1.00000 \nonumber\\
"_but & 1.00000 \nonumber\\
because_love & 1.00000 \nonumber\\
put_my & 1.00000 \nonumber\\
in_self-defense & 1.00000 \nonumber\\
ProductionRule_S->PP,NP,ADVP,VP, & 1.00000 \nonumber\\
side_say & 1.00000 \nonumber\\
ProductionRule_VP->VBG,``,NP,'', & 1.00000 \nonumber\\
self-defense_, & 1.00000 \nonumber\\
murderer_because & 1.00000 \nonumber\\
them_kill & 1.00000 \nonumber\\
depend_in & 1.00000 \nonumber\\
just_kill & 1.00000 \nonumber\\
person_than & 1.00000 \nonumber\\
strong_but & 1.00000 \nonumber\\
ProductionRule_VP->VBD,NP,PP,S, & 1.00000 \nonumber\\
reality_it & 1.00000 \nonumber\\
cant_even & 1.00000 \nonumber\\
ProductionRule_NP->NNS,NN,NN, & 1.00000 \nonumber\\
you_could & 1.00000 \nonumber\\
put_the & 1.00000 \nonumber\\
ah & 1.00000 \nonumber\\
._otherwise & 1.00000 \nonumber\\
porn_you & 1.00000 \nonumber\\
want_with & 1.00000 \nonumber\\
slippery_slope & 1.00000 \nonumber\\
different_scenario & 1.00000 \nonumber\\
my_rebuttal & 1.00000 \nonumber\\
"_furthermore & 1.00000 \nonumber\\
slope & 1.00000 \nonumber\\
blindly & 1.00000 \nonumber\\
little_relative & 1.00000 \nonumber\\
slippery & 1.00000 \nonumber\\
but_identical & 1.00000 \nonumber\\
relative_impact & 1.00000 \nonumber\\
propose_that & 1.00000 \nonumber\\
blindly_apply & 1.00000 \nonumber\\
relative & 1.00000 \nonumber\\
the_slippery & 1.00000 \nonumber\\
this_line & 1.00000 \nonumber\\
let_any & 1.00000 \nonumber\\
that_law & 1.00000 \nonumber\\
marriage_for & 1.00000 \nonumber\\
be_blindly & 1.00000 \nonumber\\
to_res0ndf7 & 1.00000 \nonumber\\
law_develop & 1.00000 \nonumber\\
demand_a & 1.00000 \nonumber\\
"_... & 1.00000 \nonumber\\
read_my & 1.00000 \nonumber\\
change_with & 1.00000 \nonumber\\
minimal_... & 1.00000 \nonumber\\
res0ndf7 & 1.00000 \nonumber\\
perfectly_to & 1.00000 \nonumber\\
res0ndf7_for & 1.00000 \nonumber\\
apply_perfectly & 1.00000 \nonumber\\
a_change & 1.00000 \nonumber\\
any_small & 1.00000 \nonumber\\
slope_argument & 1.00000 \nonumber\\
scenario_. & 1.00000 \nonumber\\
scenario & 1.00000 \nonumber\\
impact_? & 1.00000 \nonumber\\
of_assumption & 1.00000 \nonumber\\
"_this & 1.00000 \nonumber\\
argument_apply & 1.00000 \nonumber\\
homosexual_relationship & 1.00000 \nonumber\\
assumption_should & 1.00000 \nonumber\\
identical_marriage & 1.00000 \nonumber\\
one_set & 1.00000 \nonumber\\
union_. & 1.00000 \nonumber\\
group_demand & 1.00000 \nonumber\\
small_group & 1.00000 \nonumber\\
with_little & 1.00000 \nonumber\\
a_separate & 1.00000 \nonumber\\
develop_under & 1.00000 \nonumber\\
bottle_of & 1.00000 \nonumber\\
_pos_ngram_NN_ART_NP & 1.00000 \nonumber\\
third & 1.00000 \nonumber\\
this_that & 1.00000 \nonumber\\
doubt_on & 1.00000 \nonumber\\
no_doubt & 1.00000 \nonumber\\
have_power & 1.00000 \nonumber\\
way_you & 1.00000 \nonumber\\
to_create & 1.00000 \nonumber\\
tube & 1.00000 \nonumber\\
tube_. & 1.00000 \nonumber\\
,_spongebob & 1.00000 \nonumber\\
more_imformation & 1.00000 \nonumber\\
._ex & 1.00000 \nonumber\\
news_, & 1.00000 \nonumber\\
imformation & 1.00000 \nonumber\\
tube_, & 1.00000 \nonumber\\
spongebob_, & 1.00000 \nonumber\\
the_tube & 1.00000 \nonumber\\
not_sayin & 1.00000 \nonumber\\
ex_) & 1.00000 \nonumber\\
this_cuz & 1.00000 \nonumber\\
sayin_this & 1.00000 \nonumber\\
,_baseball & 1.00000 \nonumber\\
sayin & 1.00000 \nonumber\\
ex & 1.00000 \nonumber\\
)_news & 1.00000 \nonumber\\
imformation_than & 1.00000 \nonumber\\
,_yes & 1.00000 \nonumber\\
ProductionRule_SBAR->IN,FRAG, & 1.00000 \nonumber\\
lousy_and & 1.00000 \nonumber\\
why_you & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,ADJP,S,SBAR, & 1.00000 \nonumber\\
be_half & 1.00000 \nonumber\\
real_find & 1.00000 \nonumber\\
if_evealution & 1.00000 \nonumber\\
me_someone/something & 1.00000 \nonumber\\
half_way & 1.00000 \nonumber\\
find_me & 1.00000 \nonumber\\
someone/something_that & 1.00000 \nonumber\\
evealution & 1.00000 \nonumber\\
evealution_be & 1.00000 \nonumber\\
someone/something & 1.00000 \nonumber\\
also_recyclable & 1.00000 \nonumber\\
re-use_and & 1.00000 \nonumber\\
it_several & 1.00000 \nonumber\\
re-use_the & 1.00000 \nonumber\\
ProductionRule_VP->VBG,ADVP,NP, & 1.00000 \nonumber\\
bottle_over & 1.00000 \nonumber\\
technically_you & 1.00000 \nonumber\\
economy_if & 1.00000 \nonumber\\
bottle_so & 1.00000 \nonumber\\
over_and & 1.00000 \nonumber\\
can_re-use & 1.00000 \nonumber\\
drink_your & 1.00000 \nonumber\\
reuse_properly & 1.00000 \nonumber\\
youre & 1.00000 \nonumber\\
youre_do & 1.00000 \nonumber\\
and_re-use & 1.00000 \nonumber\\
we_figure & 1.00000 \nonumber\\
recyclable & 1.00000 \nonumber\\
after_youre & 1.00000 \nonumber\\
recyclable_and & 1.00000 \nonumber\\
ProductionRule_VP->VB,NP,NP,S, & 1.00000 \nonumber\\
object_such & 1.00000 \nonumber\\
serval & 1.00000 \nonumber\\
re-use_it & 1.00000 \nonumber\\
same_plastic & 1.00000 \nonumber\\
your_bottle & 1.00000 \nonumber\\
as_more & 1.00000 \nonumber\\
more_plastic & 1.00000 \nonumber\\
have_serval & 1.00000 \nonumber\\
water_you & 1.00000 \nonumber\\
less_plastic & 1.00000 \nonumber\\
so_technically & 1.00000 \nonumber\\
use_less & 1.00000 \nonumber\\
to_reuse & 1.00000 \nonumber\\
re-use & 1.00000 \nonumber\\
because_after & 1.00000 \nonumber\\
do_drink & 1.00000 \nonumber\\
new_object & 1.00000 \nonumber\\
serval_bottle & 1.00000 \nonumber\\
properly_. & 1.00000 \nonumber\\
plastic_. & 1.00000 \nonumber\\
the_rat & 1.00000 \nonumber\\
sense_of & 1.00000 \nonumber\\
unborn_human & 1.00000 \nonumber\\
law_pro-choice & 1.00000 \nonumber\\
murder_their & 1.00000 \nonumber\\
own_unborn & 1.00000 \nonumber\\
human_child & 1.00000 \nonumber\\
._keep & 1.00000 \nonumber\\
allow_woman & 1.00000 \nonumber\\
someone_and & 1.00000 \nonumber\\
pe_be & 1.00000 \nonumber\\
of_expression & 1.00000 \nonumber\\
should_wear & 1.00000 \nonumber\\
feel_free & 1.00000 \nonumber\\
free_about & 1.00000 \nonumber\\
about_their & 1.00000 \nonumber\\
situation_go & 1.00000 \nonumber\\
best_we & 1.00000 \nonumber\\
neither_be & 1.00000 \nonumber\\
useful_we & 1.00000 \nonumber\\
only_live & 1.00000 \nonumber\\
a_mean & 1.00000 \nonumber\\
so_long & 1.00000 \nonumber\\
for_so & 1.00000 \nonumber\\
maybe_your & 1.00000 \nonumber\\
._neither & 1.00000 \nonumber\\
himself_first & 1.00000 \nonumber\\
be_necessarily & 1.00000 \nonumber\\
individual_will & 1.00000 \nonumber\\
will_usually & 1.00000 \nonumber\\
life_for & 1.00000 \nonumber\\
better_but & 1.00000 \nonumber\\
but_an & 1.00000 \nonumber\\
do_advance & 1.00000 \nonumber\\
necessarily_better & 1.00000 \nonumber\\
we_want & 1.00000 \nonumber\\
unfortunately_it & 1.00000 \nonumber\\
mean_person & 1.00000 \nonumber\\
and_alway & 1.00000 \nonumber\\
this_life & 1.00000 \nonumber\\
usually_help & 1.00000 \nonumber\\
good_situation & 1.00000 \nonumber\\
alway_do & 1.00000 \nonumber\\
pursuit_might & 1.00000 \nonumber\\
alway_mean & 1.00000 \nonumber\\
live_this & 1.00000 \nonumber\\
help_himself & 1.00000 \nonumber\\
long_and & 1.00000 \nonumber\\
._time & 1.00000 \nonumber\\
have_change & 1.00000 \nonumber\\
seriously & 1.00000 \nonumber\\
definitely_wrong & 1.00000 \nonumber\\
art & 1.00000 \nonumber\\
visit & 1.00000 \nonumber\\
when_farquar & 1.00000 \nonumber\\
farquar_be & 1.00000 \nonumber\\
a_grander & 1.00000 \nonumber\\
ceremony_before & 1.00000 \nonumber\\
leave_compare & 1.00000 \nonumber\\
fire_by & 1.00000 \nonumber\\
grander_ceremony & 1.00000 \nonumber\\
before_he & 1.00000 \nonumber\\
ProductionRule_WHNP->WRB,JJ, & 1.00000 \nonumber\\
grander & 1.00000 \nonumber\\
which_show & 1.00000 \nonumber\\
people_love & 1.00000 \nonumber\\
be_far & 1.00000 \nonumber\\
childhood_obesity & 1.00000 \nonumber\\
be_fine & 1.00000 \nonumber\\
good_option & 1.00000 \nonumber\\
punish_a & 1.00000 \nonumber\\
child_if & 1.00000 \nonumber\\
believe_spank & 1.00000 \nonumber\\
else_work & 1.00000 \nonumber\\
ProductionRule_SINV->S,,,VP,NP, & 1.00000 \nonumber\\
lol_. & 1.00000 \nonumber\\
population_and & 1.00000 \nonumber\\
diferent_material & 1.00000 \nonumber\\
pupil_it & 1.00000 \nonumber\\
pupil_concentrate & 1.00000 \nonumber\\
make_pupil & 1.00000 \nonumber\\
their_education & 1.00000 \nonumber\\
material_status & 1.00000 \nonumber\\
status_more & 1.00000 \nonumber\\
more_equal & 1.00000 \nonumber\\
very_goooooooood & 1.00000 \nonumber\\
pupil_with & 1.00000 \nonumber\\
equal_: & 1.00000 \nonumber\\
with_diferent & 1.00000 \nonumber\\
diferent & 1.00000 \nonumber\\
goooooooood_idea & 1.00000 \nonumber\\
??_becouse & 1.00000 \nonumber\\
goooooooood & 1.00000 \nonumber\\
instill_discipline & 1.00000 \nonumber\\
becouse & 1.00000 \nonumber\\
instill & 1.00000 \nonumber\\
becouse_the & 1.00000 \nonumber\\
concentrate_on & 1.00000 \nonumber\\
why_?? & 1.00000 \nonumber\\
than_on & 1.00000 \nonumber\\
clothe_and & 1.00000 \nonumber\\
uniform_instill & 1.00000 \nonumber\\
discipline_among & 1.00000 \nonumber\\
constraint & 1.00000 \nonumber\\
?_: & 1.00000 \nonumber\\
god_need & 1.00000 \nonumber\\
time_? & 1.00000 \nonumber\\
constraint_of & 1.00000 \nonumber\\
operate & 1.00000 \nonumber\\
to_operate & 1.00000 \nonumber\\
operate_within & 1.00000 \nonumber\\
waste_his & 1.00000 \nonumber\\
the_constraint & 1.00000 \nonumber\\
when_accuse & 1.00000 \nonumber\\
ProductionRule_ADJP->NP,JJ, & 1.00000 \nonumber\\
longer & 1.00000 \nonumber\\
adhere_to & 1.00000 \nonumber\\
adhere & 1.00000 \nonumber\\
say_no & 1.00000 \nonumber\\
people_can & 1.00000 \nonumber\\
right_from & 1.00000 \nonumber\\
from_wrong & 1.00000 \nonumber\\
ProductionRule_SQ->VBZ,NP,NP, & 1.00000 \nonumber\\
in_society & 1.00000 \nonumber\\
baby_and & 1.00000 \nonumber\\
_pos_ngram_NP_PUNC_ADJ & 1.00000 \nonumber\\
well_be & 1.00000 \nonumber\\
idea_the & 1.00000 \nonumber\\
diet & 1.00000 \nonumber\\
internal & 1.00000 \nonumber\\
christianity_because & 1.00000 \nonumber\\
their_home & 1.00000 \nonumber\\
indian_and & 1.00000 \nonumber\\
ProductionRule_PP->RB,PP, & 1.00000 \nonumber\\
by_debate & 1.00000 \nonumber\\
solve_all & 1.00000 \nonumber\\
show_my & 1.00000 \nonumber\\
ProductionRule_NP->DT,NNP,CC,LS, & 1.00000 \nonumber\\
there_country & 1.00000 \nonumber\\
who_think & 1.00000 \nonumber\\
_pos_ngram_PP_CONJ_ART & 1.00000 \nonumber\\
debate_they & 1.00000 \nonumber\\
only_by & 1.00000 \nonumber\\
will_solve & 1.00000 \nonumber\\
country_down & 1.00000 \nonumber\\
also_know & 1.00000 \nonumber\\
reasonable & 1.00000 \nonumber\\
3rd_, & 1.00000 \nonumber\\
2nd & 1.00000 \nonumber\\
format_if & 1.00000 \nonumber\\
_pos_ngram_NP_PP_O & 1.00000 \nonumber\\
password_with & 1.00000 \nonumber\\
(_rare & 1.00000 \nonumber\\
tool_bar & 1.00000 \nonumber\\
support_ms. & 1.00000 \nonumber\\
add-on_allow & 1.00000 \nonumber\\
with_greater & 1.00000 \nonumber\\
friendlier_and & 1.00000 \nonumber\\
,_gesture & 1.00000 \nonumber\\
ms. & 1.00000 \nonumber\\
display_the & 1.00000 \nonumber\\
sap & 1.00000 \nonumber\\
sap_at & 1.00000 \nonumber\\
friendlier & 1.00000 \nonumber\\
ie_format & 1.00000 \nonumber\\
format & 1.00000 \nonumber\\
tab_that & 1.00000 \nonumber\\
ms._because & 1.00000 \nonumber\\
,_weatherfox & 1.00000 \nonumber\\
password & 1.00000 \nonumber\\
._add-on & 1.00000 \nonumber\\
page_in & 1.00000 \nonumber\\
incompatible_( & 1.00000 \nonumber\\
tab_( & 1.00000 \nonumber\\
remember_them & 1.00000 \nonumber\\
remember_password & 1.00000 \nonumber\\
if_something & 1.00000 \nonumber\\
rock_. & 1.00000 \nonumber\\
personalize & 1.00000 \nonumber\\
product_. & 1.00000 \nonumber\\
personalize_your & 1.00000 \nonumber\\
good_product & 1.00000 \nonumber\\
weatherfox & 1.00000 \nonumber\\
it_remember & 1.00000 \nonumber\\
rare_, & 1.00000 \nonumber\\
weatherfox_, & 1.00000 \nonumber\\
them_when & 1.00000 \nonumber\\
a_tab & 1.00000 \nonumber\\
(_age & 1.00000 \nonumber\\
and_remember & 1.00000 \nonumber\\
the_tool & 1.00000 \nonumber\\
-_tab & 1.00000 \nonumber\\
the_link & 1.00000 \nonumber\\
love_- & 1.00000 \nonumber\\
you_display & 1.00000 \nonumber\\
gusto & 1.00000 \nonumber\\
be_incompatible & 1.00000 \nonumber\\
only_sap & 1.00000 \nonumber\\
gusto_. & 1.00000 \nonumber\\
gesture & 1.00000 \nonumber\\
gesture_, & 1.00000 \nonumber\\
work_) & 1.00000 \nonumber\\
product_be & 1.00000 \nonumber\\
incompatible & 1.00000 \nonumber\\
logo_in & 1.00000 \nonumber\\
link_logo & 1.00000 \nonumber\\
much_friendlier & 1.00000 \nonumber\\
bar_rock & 1.00000 \nonumber\\
you_close & 1.00000 \nonumber\\
greater_gusto & 1.00000 \nonumber\\
to_personalize & 1.00000 \nonumber\\
health_class & 1.00000 \nonumber\\
say_with & 1.00000 \nonumber\\
freak_accent & 1.00000 \nonumber\\
accent & 1.00000 \nonumber\\
ProductionRule_NP->PRP$,VBG,NN, & 1.00000 \nonumber\\
world_as & 1.00000 \nonumber\\
as_no & 1.00000 \nonumber\\
their_freak & 1.00000 \nonumber\\
never_lead & 1.00000 \nonumber\\
ProductionRule_SBAR->IN,S,:, & 1.00000 \nonumber\\
accent_; & 1.00000 \nonumber\\
ProductionRule_PRN->S,-RRB-, & 1.00000 \nonumber\\
ProductionRule_ADJP->JJ,PP,S, & 1.00000 \nonumber\\
use_other & 1.00000 \nonumber\\
not_often & 1.00000 \nonumber\\
belt & 1.00000 \nonumber\\
child_as & 1.00000 \nonumber\\
'_ok & 1.00000 \nonumber\\
often_or & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,RB,ADVP, & 1.00000 \nonumber\\
belt_. & 1.00000 \nonumber\\
a_belt & 1.00000 \nonumber\\
..._why & 1.00000 \nonumber\\
n't_miss & 1.00000 \nonumber\\
his_dad & 1.00000 \nonumber\\
like_his & 1.00000 \nonumber\\
do_absoultly & 1.00000 \nonumber\\
miss_what & 1.00000 \nonumber\\
most_kid & 1.00000 \nonumber\\
lousy_like & 1.00000 \nonumber\\
them_around & 1.00000 \nonumber\\
absoultly & 1.00000 \nonumber\\
absoultly_nothing & 1.00000 \nonumber\\
just_means & 1.00000 \nonumber\\
ProductionRule_VP->VP,CC,VP,NP, & 1.00000 \nonumber\\
ProductionRule_VP->RB,VP,IN,VP, & 1.00000 \nonumber\\
why_have & 1.00000 \nonumber\\
and_over & 1.00000 \nonumber\\
do_as & 1.00000 \nonumber\\
prepare_for & 1.00000 \nonumber\\
percentage & 1.00000 \nonumber\\
evolve & 1.00000 \nonumber\\
bencoolen_. & 1.00000 \nonumber\\
degrade_to & 1.00000 \nonumber\\
raffle_institution & 1.00000 \nonumber\\
some_thing & 1.00000 \nonumber\\
of_waste & 1.00000 \nonumber\\
be_barely & 1.00000 \nonumber\\
seem_selfish & 1.00000 \nonumber\\
time_it & 1.00000 \nonumber\\
but_once & 1.00000 \nonumber\\
your_do & 1.00000 \nonumber\\
may_seem & 1.00000 \nonumber\\
at_what & 1.00000 \nonumber\\
yourself_but & 1.00000 \nonumber\\
same_. & 1.00000 \nonumber\\
important_because & 1.00000 \nonumber\\
too_many & 1.00000 \nonumber\\
can_you & 1.00000 \nonumber\\
n't_in & 1.00000 \nonumber\\
a_lower & 1.00000 \nonumber\\
legalize_homosexual & 1.00000 \nonumber\\
marriage_? & 1.00000 \nonumber\\
union_which & 1.00000 \nonumber\\
be_incestual & 1.00000 \nonumber\\
homosexual_union & 1.00000 \nonumber\\
lower_marriage & 1.00000 \nonumber\\
marriage_include & 1.00000 \nonumber\\
include_incestual & 1.00000 \nonumber\\
country_legalize & 1.00000 \nonumber\\
homosexual_marriage & 1.00000 \nonumber\\
marriage_rate & 1.00000 \nonumber\\
marriage_right & 1.00000 \nonumber\\
incestual_marriage & 1.00000 \nonumber\\
incestual_homosexual & 1.00000 \nonumber\\
incestual & 1.00000 \nonumber\\
"_gay & 1.00000 \nonumber\\
marriage_can & 1.00000 \nonumber\\
_pos_ngram_CARD_ART & 1.00000 \nonumber\\
street_fight & 1.00000 \nonumber\\
mean_if & 1.00000 \nonumber\\
like_street & 1.00000 \nonumber\\
platform_. & 1.00000 \nonumber\\
unless_your & 1.00000 \nonumber\\
ufc & 1.00000 \nonumber\\
ufc_. & 1.00000 \nonumber\\
them_at & 1.00000 \nonumber\\
christianity_but & 1.00000 \nonumber\\
n't_argue & 1.00000 \nonumber\\
of_like & 1.00000 \nonumber\\
._kinda & 1.00000 \nonumber\\
same_subject & 1.00000 \nonumber\\
on_on & 1.00000 \nonumber\\
and_ufc & 1.00000 \nonumber\\
kinda_of & 1.00000 \nonumber\\
all_unless & 1.00000 \nonumber\\
different_platform & 1.00000 \nonumber\\
!_there & 1.00000 \nonumber\\
a_pe & 1.00000 \nonumber\\
ProductionRule_VP->VBP,PP,NP, & 1.00000 \nonumber\\
nearby & 1.00000 \nonumber\\
_pos_ngram_NP_PP_NN & 1.00000 \nonumber\\
wrong_..... & 1.00000 \nonumber\\
be_gay & 1.00000 \nonumber\\
and_creative & 1.00000 \nonumber\\
an_equal & 1.00000 \nonumber\\
ProductionRule_NP->DT,JJ,CC,JJ,JJ,NN, & 1.00000 \nonumber\\
social_life & 1.00000 \nonumber\\
personality_and & 1.00000 \nonumber\\
life_much & 1.00000 \nonumber\\
admit_wear & 1.00000 \nonumber\\
not_look & 1.00000 \nonumber\\
allow_an & 1.00000 \nonumber\\
fun_and & 1.00000 \nonumber\\
want_be & 1.00000 \nonumber\\
fun_if & 1.00000 \nonumber\\
mature_look & 1.00000 \nonumber\\
only_base & 1.00000 \nonumber\\
do_half & 1.00000 \nonumber\\
afford_to & 1.00000 \nonumber\\
only_fun & 1.00000 \nonumber\\
uniform_allow & 1.00000 \nonumber\\
fair_social & 1.00000 \nonumber\\
mature & 1.00000 \nonumber\\
case_and & 1.00000 \nonumber\\
peer_standard & 1.00000 \nonumber\\
look_. & 1.00000 \nonumber\\
equal_and & 1.00000 \nonumber\\
cant_afford & 1.00000 \nonumber\\
ProductionRule_VP->VP,CC,RB,VP, & 1.00000 \nonumber\\
standard_so & 1.00000 \nonumber\\
everyone_can & 1.00000 \nonumber\\
but_its & 1.00000 \nonumber\\
live_up & 1.00000 \nonumber\\
and_fair & 1.00000 \nonumber\\
creative_but & 1.00000 \nonumber\\
on_personality & 1.00000 \nonumber\\
half_to & 1.00000 \nonumber\\
make_social & 1.00000 \nonumber\\
status_only & 1.00000 \nonumber\\
more_mature & 1.00000 \nonumber\\
roof & 1.00000 \nonumber\\
us_. & 1.00000 \nonumber\\
old_lol & 1.00000 \nonumber\\
something_for & 1.00000 \nonumber\\
expensive_, & 1.00000 \nonumber\\
could_n't & 1.00000 \nonumber\\
our_life & 1.00000 \nonumber\\
insult & 1.00000 \nonumber\\
or_acceptable & 1.00000 \nonumber\\
next_move & 1.00000 \nonumber\\
solution_or & 1.00000 \nonumber\\
crazy_in & 1.00000 \nonumber\\
toward_me & 1.00000 \nonumber\\
understand_some & 1.00000 \nonumber\\
not_toward & 1.00000 \nonumber\\
never_the & 1.00000 \nonumber\\
to_crazy & 1.00000 \nonumber\\
take_another & 1.00000 \nonumber\\
move_be & 1.00000 \nonumber\\
person_life & 1.00000 \nonumber\\
if_her & 1.00000 \nonumber\\
information_from & 1.00000 \nonumber\\
expression & 1.00000 \nonumber\\
bleed_. & 1.00000 \nonumber\\
though_people & 1.00000 \nonumber\\
n't_my & 1.00000 \nonumber\\
roof_with & 1.00000 \nonumber\\
of_intention & 1.00000 \nonumber\\
be_schizophrenic & 1.00000 \nonumber\\
intention & 1.00000 \nonumber\\
live_under & 1.00000 \nonumber\\
ProductionRule_NP->NNS,S, & 1.00000 \nonumber\\
alway_commit & 1.00000 \nonumber\\
i_stab & 1.00000 \nonumber\\
a_sharp & 1.00000 \nonumber\\
object_, & 1.00000 \nonumber\\
bleed & 1.00000 \nonumber\\
leg_with & 1.00000 \nonumber\\
that_could & 1.00000 \nonumber\\
could_possibly & 1.00000 \nonumber\\
mistake_if & 1.00000 \nonumber\\
same_roof & 1.00000 \nonumber\\
sharp & 1.00000 \nonumber\\
intention_to & 1.00000 \nonumber\\
the_leg & 1.00000 \nonumber\\
stab & 1.00000 \nonumber\\
sharp_object & 1.00000 \nonumber\\
stab_some & 1.00000 \nonumber\\
schizophrenic & 1.00000 \nonumber\\
schizophrenic_. & 1.00000 \nonumber\\
my_intention & 1.00000 \nonumber\\
ProductionRule_S->TO,VP, & 1.00000 \nonumber\\
him_bleed & 1.00000 \nonumber\\
n't_possibly & 1.00000 \nonumber\\
possibly_be & 1.00000 \nonumber\\
commit_with & 1.00000 \nonumber\\
be_anything & 1.00000 \nonumber\\
behind_intelligent & 1.00000 \nonumber\\
merely_christianity & 1.00000 \nonumber\\
christianity_masquerade & 1.00000 \nonumber\\
design_theory & 1.00000 \nonumber\\
masquerade & 1.00000 \nonumber\\
science_behind & 1.00000 \nonumber\\
be_merely & 1.00000 \nonumber\\
real_science & 1.00000 \nonumber\\
masquerade_as & 1.00000 \nonumber\\
design_. & 1.00000 \nonumber\\
intelligent_design & 1.00000 \nonumber\\
someone_that & 1.00000 \nonumber\\
identical & 1.00000 \nonumber\\
under_one & 1.00000 \nonumber\\
cost & 1.00000 \nonumber\\
by_lousy & 1.00000 \nonumber\\
if_by & 1.00000 \nonumber\\
,_rapist & 1.00000 \nonumber\\
,_unintelligent & 1.00000 \nonumber\\
,_detach & 1.00000 \nonumber\\
,_overwork & 1.00000 \nonumber\\
,_lazy & 1.00000 \nonumber\\
,_murderer & 1.00000 \nonumber\\
,_unavailable & 1.00000 \nonumber\\
dealer_, & 1.00000 \nonumber\\
,_uneducate & 1.00000 \nonumber\\
_pos_ngram_PUNC_PUNC_V & 1.00000 \nonumber\\
non-criminal_version & 1.00000 \nonumber\\
non-criminal & 1.00000 \nonumber\\
overwork_, & 1.00000 \nonumber\\
,_distant & 1.00000 \nonumber\\
overwork & 1.00000 \nonumber\\
mean_unemploy & 1.00000 \nonumber\\
lazy_, & 1.00000 \nonumber\\
ProductionRule_NP->NP,,,UCP, & 1.00000 \nonumber\\
satisfy_with & 1.00000 \nonumber\\
bore_, & 1.00000 \nonumber\\
if_pop & 1.00000 \nonumber\\
be_alive & 1.00000 \nonumber\\
distant & 1.00000 \nonumber\\
say_lousy & 1.00000 \nonumber\\
alive_and & 1.00000 \nonumber\\
unintelligent & 1.00000 \nonumber\\
distant_, & 1.00000 \nonumber\\
uneducate & 1.00000 \nonumber\\
uneducate_, & 1.00000 \nonumber\\
unemploy & 1.00000 \nonumber\\
unemploy_, & 1.00000 \nonumber\\
detach & 1.00000 \nonumber\\
detach_, & 1.00000 \nonumber\\
sperm_donor & 1.00000 \nonumber\\
sperm & 1.00000 \nonumber\\
the_sperm & 1.00000 \nonumber\\
unintelligent_, & 1.00000 \nonumber\\
rapist & 1.00000 \nonumber\\
rapist_, & 1.00000 \nonumber\\
pop_be & 1.00000 \nonumber\\
murderer_, & 1.00000 \nonumber\\
unavailable_, & 1.00000 \nonumber\\
unavailable & 1.00000 \nonumber\\
,_bore & 1.00000 \nonumber\\
ProductionRule_UCP->NP,,,ADJP,,,ADJP,,,ADJP,,,ADJP,,,ADJP,,,ADJP,,,ADJP,,,CC,NP, & 1.00000 \nonumber\\
other_non-criminal & 1.00000 \nonumber\\
donor_. & 1.00000 \nonumber\\
donor & 1.00000 \nonumber\\
tire_, & 1.00000 \nonumber\\
commercial_and & 1.00000 \nonumber\\
can_read & 1.00000 \nonumber\\
your_tire & 1.00000 \nonumber\\
how_annoy & 1.00000 \nonumber\\
case_your & 1.00000 \nonumber\\
ProductionRule_ADVP->IN,NN, & 1.00000 \nonumber\\
annoy_they & 1.00000 \nonumber\\
read_to & 1.00000 \nonumber\\
ever_consider & 1.00000 \nonumber\\
the_commercial & 1.00000 \nonumber\\
consider_about & 1.00000 \nonumber\\
relax_in & 1.00000 \nonumber\\
relax_as & 1.00000 \nonumber\\
plus_have & 1.00000 \nonumber\\
you_relax & 1.00000 \nonumber\\
old_person & 1.00000 \nonumber\\
murder_.... & 1.00000 \nonumber\\
in_kill & 1.00000 \nonumber\\
embroyo_or & 1.00000 \nonumber\\
any_difference & 1.00000 \nonumber\\
an_embroyo & 1.00000 \nonumber\\
a_40 & 1.00000 \nonumber\\
embroyo & 1.00000 \nonumber\\
kill_an & 1.00000 \nonumber\\
40_year & 1.00000 \nonumber\\
...._be & 1.00000 \nonumber\\
feel_uncomfortable & 1.00000 \nonumber\\
for_adoption & 1.00000 \nonumber\\
ProductionRule_NP->NNP,NNP,NNP,NNP,NNP,NNP,NNP, & 1.00000 \nonumber\\
boss_( & 1.00000 \nonumber\\
ProductionRule_S->NP,NP,SBAR, & 1.00000 \nonumber\\
founder_!!!! & 1.00000 \nonumber\\
follow_him & 1.00000 \nonumber\\
fire_!!! & 1.00000 \nonumber\\
!!!!_farquhar & 1.00000 \nonumber\\
change_that & 1.00000 \nonumber\\
for_one & 1.00000 \nonumber\\
unfair_for & 1.00000 \nonumber\\
in_varsity & 1.00000 \nonumber\\
embarrass & 1.00000 \nonumber\\
embarrass_for & 1.00000 \nonumber\\
the_class & 1.00000 \nonumber\\
can_waive & 1.00000 \nonumber\\
because_varsity & 1.00000 \nonumber\\
waive & 1.00000 \nonumber\\
for_ap & 1.00000 \nonumber\\
ap_student & 1.00000 \nonumber\\
varsity_sport & 1.00000 \nonumber\\
ProductionRule_VP->VBP,RB,PP,SBAR, & 1.00000 \nonumber\\
,_unfair & 1.00000 \nonumber\\
ap & 1.00000 \nonumber\\
varsity_athlete & 1.00000 \nonumber\\
varsity & 1.00000 \nonumber\\
sport_because & 1.00000 \nonumber\\
waive_the & 1.00000 \nonumber\\
some_, & 1.00000 \nonumber\\
,_embarrass & 1.00000 \nonumber\\
athlete_can & 1.00000 \nonumber\\
ProductionRule_NP->NP,,,ADJP,,, & 1.00000 \nonumber\\
student_that & 1.00000 \nonumber\\
deserve_the & 1.00000 \nonumber\\
ProductionRule_VP->ADJP,PP, & 1.00000 \nonumber\\
just_have & 1.00000 \nonumber\\
you_for & 1.00000 \nonumber\\
best_for & 1.00000 \nonumber\\
regulate & 1.00000 \nonumber\\
to_marriage & 1.00000 \nonumber\\
like_we & 1.00000 \nonumber\\
being_just & 1.00000 \nonumber\\
do_and & 1.00000 \nonumber\\
muscle_, & 1.00000 \nonumber\\
attack_. & 1.00000 \nonumber\\
diet_) & 1.00000 \nonumber\\
age_( & 1.00000 \nonumber\\
globe & 1.00000 \nonumber\\
then_just & 1.00000 \nonumber\\
globe_and & 1.00000 \nonumber\\
just_run & 1.00000 \nonumber\\
keep_a & 1.00000 \nonumber\\
course_you & 1.00000 \nonumber\\
the_field & 1.00000 \nonumber\\
stronger_, & 1.00000 \nonumber\\
strong_people & 1.00000 \nonumber\\
get_muscle & 1.00000 \nonumber\\
prevent_you & 1.00000 \nonumber\\
and_strong & 1.00000 \nonumber\\
from_have & 1.00000 \nonumber\\
more_fit & 1.00000 \nonumber\\
class_there & 1.00000 \nonumber\\
60-80 & 1.00000 \nonumber\\
further_age & 1.00000 \nonumber\\
useless_because & 1.00000 \nonumber\\
normally & 1.00000 \nonumber\\
would_prevent & 1.00000 \nonumber\\
this_class & 1.00000 \nonumber\\
would_normally & 1.00000 \nonumber\\
60-80_) & 1.00000 \nonumber\\
normally_do & 1.00000 \nonumber\\
fat_( & 1.00000 \nonumber\\
(_of & 1.00000 \nonumber\\
heart_attack & 1.00000 \nonumber\\
run_around & 1.00000 \nonumber\\
have_heart & 1.00000 \nonumber\\
education_you & 1.00000 \nonumber\\
)_it & 1.00000 \nonumber\\
_pos_ngram_PP_CARD_O & 1.00000 \nonumber\\
become_stronger & 1.00000 \nonumber\\
easily_for & 1.00000 \nonumber\\
be_fewer & 1.00000 \nonumber\\
also_need & 1.00000 \nonumber\\
field_for & 1.00000 \nonumber\\
fewer_obese & 1.00000 \nonumber\\
fewer & 1.00000 \nonumber\\
_pos_ngram_CARD_O_PR & 1.00000 \nonumber\\
(_like & 1.00000 \nonumber\\
child_around & 1.00000 \nonumber\\
like_60-80 & 1.00000 \nonumber\\
balance_diet & 1.00000 \nonumber\\
for_further & 1.00000 \nonumber\\
with_physical & 1.00000 \nonumber\\
so_easily & 1.00000 \nonumber\\
completely_useless & 1.00000 \nonumber\\
ProductionRule_S->ADVP,,,NP,VP, & 1.00000 \nonumber\\
short & 1.00000 \nonumber\\
curse_itself & 1.00000 \nonumber\\
into_caste & 1.00000 \nonumber\\
we_compare & 1.00000 \nonumber\\
into_development & 1.00000 \nonumber\\
compare_so & 1.00000 \nonumber\\
ProductionRule_UCP->ADJP,:,NP, & 1.00000 \nonumber\\
itself_first & 1.00000 \nonumber\\
find_difficult & 1.00000 \nonumber\\
,_politics & 1.00000 \nonumber\\
let_have & 1.00000 \nonumber\\
world_when & 1.00000 \nonumber\\
illiterate_country & 1.00000 \nonumber\\
illiterate_( & 1.00000 \nonumber\\
illiterate & 1.00000 \nonumber\\
a_look & 1.00000 \nonumber\\
ProductionRule_VP->VB,NP,ADVP,:,SBAR, & 1.00000 \nonumber\\
percentage_) & 1.00000 \nonumber\\
ProductionRule_UCP->NP,CC,ADVP, & 1.00000 \nonumber\\
still_curse & 1.00000 \nonumber\\
itself_and & 1.00000 \nonumber\\
follow_point & 1.00000 \nonumber\\
itself_!! & 1.00000 \nonumber\\
(_do & 1.00000 \nonumber\\
world_.... & 1.00000 \nonumber\\
far_.... & 1.00000 \nonumber\\
...._but & 1.00000 \nonumber\\
the_percentage & 1.00000 \nonumber\\
point_: & 1.00000 \nonumber\\
thing_be & 1.00000 \nonumber\\
almost_90 & 1.00000 \nonumber\\
manage_itself & 1.00000 \nonumber\\
an_illiterate & 1.00000 \nonumber\\
confidence_on & 1.00000 \nonumber\\
country_ca & 1.00000 \nonumber\\
n't_lead & 1.00000 \nonumber\\
less_into & 1.00000 \nonumber\\
ProductionRule_ADJP->RB,RB,SBAR, & 1.00000 \nonumber\\
so_an & 1.00000 \nonumber\\
...._2 & 1.00000 \nonumber\\
no_question & 1.00000 \nonumber\\
politics & 1.00000 \nonumber\\
politics_, & 1.00000 \nonumber\\
"_indium & 1.00000 \nonumber\\
world_so & 1.00000 \nonumber\\
ProductionRule_VP->VBG,ADJP,UCP, & 1.00000 \nonumber\\
of_lead & 1.00000 \nonumber\\
,_religion & 1.00000 \nonumber\\
on_so & 1.00000 \nonumber\\
have_confidence & 1.00000 \nonumber\\
even_impossible & 1.00000 \nonumber\\
!!_" & 1.00000 \nonumber\\
more_into & 1.00000 \nonumber\\
caste_, & 1.00000 \nonumber\\
difficult_or & 1.00000 \nonumber\\
be_illiterate & 1.00000 \nonumber\\
_pos_ngram_CARD_CONJ_ADV & 1.00000 \nonumber\\
:_1 & 1.00000 \nonumber\\
on_itself & 1.00000 \nonumber\\
lead_itself & 1.00000 \nonumber\\
last_resort & 1.00000 \nonumber\\
believe_this & 1.00000 \nonumber\\
side_help & 1.00000 \nonumber\\
suck_not & 1.00000 \nonumber\\
guy_that & 1.00000 \nonumber\\
to_while & 1.00000 \nonumber\\
start_depend & 1.00000 \nonumber\\
best_be & 1.00000 \nonumber\\
your_grow & 1.00000 \nonumber\\
follow_his & 1.00000 \nonumber\\
know_you & 1.00000 \nonumber\\
because_from & 1.00000 \nonumber\\
step_. & 1.00000 \nonumber\\
people_by & 1.00000 \nonumber\\
nothing_in & 1.00000 \nonumber\\
set_bid & 1.00000 \nonumber\\
bid_example & 1.00000 \nonumber\\
while_your & 1.00000 \nonumber\\
get_through & 1.00000 \nonumber\\
there_alway & 1.00000 \nonumber\\
from_day & 1.00000 \nonumber\\
you_start & 1.00000 \nonumber\\
up_follow & 1.00000 \nonumber\\
his_step & 1.00000 \nonumber\\
just_set & 1.00000 \nonumber\\
through_life & 1.00000 \nonumber\\
ProductionRule_VP->VB,PRT,PP,SBAR, & 1.00000 \nonumber\\
own_with & 1.00000 \nonumber\\
we_watch & 1.00000 \nonumber\\
person_have & 1.00000 \nonumber\\
ProductionRule_FRAG->CC,ADVP,SBAR, & 1.00000 \nonumber\\
believe_some & 1.00000 \nonumber\\
correct_way & 1.00000 \nonumber\\
listen_. & 1.00000 \nonumber\\
way_some & 1.00000 \nonumber\\
nessasary_because & 1.00000 \nonumber\\
kid_but & 1.00000 \nonumber\\
ProductionRule_VP->VB,NP,FRAG, & 1.00000 \nonumber\\
nessasary & 1.00000 \nonumber\\
when_nessasary & 1.00000 \nonumber\\
_pos_ngram_ART_O_PUNC & 1.00000 \nonumber\\
skirt & 1.00000 \nonumber\\
,_love & 1.00000 \nonumber\\
._although & 1.00000 \nonumber\\
true_that & 1.00000 \nonumber\\
need_your & 1.00000 \nonumber\\
resort & 1.00000 \nonumber\\
so_then & 1.00000 \nonumber\\
ProductionRule_VP->VB,ADVP,SBAR, & 1.00000 \nonumber\\
allow_you & 1.00000 \nonumber\\
you_down & 1.00000 \nonumber\\
power_you & 1.00000 \nonumber\\
your_dream & 1.00000 \nonumber\\
and_power & 1.00000 \nonumber\\
dream_and & 1.00000 \nonumber\\
slow & 1.00000 \nonumber\\
ProductionRule_S->ADVP,LS,VP,., & 1.00000 \nonumber\\
picture_if & 1.00000 \nonumber\\
pursuit_your & 1.00000 \nonumber\\
slow_you & 1.00000 \nonumber\\
alway_right & 1.00000 \nonumber\\
help_no & 1.00000 \nonumber\\
wrong_help & 1.00000 \nonumber\\
will_just & 1.00000 \nonumber\\
you_pursuit & 1.00000 \nonumber\\
get_rich & 1.00000 \nonumber\\
big_picture & 1.00000 \nonumber\\
that_matter & 1.00000 \nonumber\\
just_slow & 1.00000 \nonumber\\
what_their & 1.00000 \nonumber\\
the_guilt & 1.00000 \nonumber\\
the_god & 1.00000 \nonumber\\
the_globe & 1.00000 \nonumber\\
people_cant & 1.00000 \nonumber\\
?_indium & 1.00000 \nonumber\\
etc._.... & 1.00000 \nonumber\\
impressionable_... & 1.00000 \nonumber\\
thier_work & 1.00000 \nonumber\\
wear_certain & 1.00000 \nonumber\\
help_student & 1.00000 \nonumber\\
code_. & 1.00000 \nonumber\\
rule_to & 1.00000 \nonumber\\
thier_own & 1.00000 \nonumber\\
on_thier & 1.00000 \nonumber\\
code_, & 1.00000 \nonumber\\
keep_order & 1.00000 \nonumber\\
or_code & 1.00000 \nonumber\\
create_dress & 1.00000 \nonumber\\
specific_rule & 1.00000 \nonumber\\
highly_impressionable & 1.00000 \nonumber\\
order_in & 1.00000 \nonumber\\
one_hand & 1.00000 \nonumber\\
impressionable & 1.00000 \nonumber\\
own_creativity & 1.00000 \nonumber\\
prevent_wear & 1.00000 \nonumber\\
student_focus & 1.00000 \nonumber\\
(_kid & 1.00000 \nonumber\\
focus_more & 1.00000 \nonumber\\
another_, & 1.00000 \nonumber\\
creativity_. & 1.00000 \nonumber\\
..._etc. & 1.00000 \nonumber\\
law_or & 1.00000 \nonumber\\
...._) & 1.00000 \nonumber\\
have_thier & 1.00000 \nonumber\\
with_keep & 1.00000 \nonumber\\
allow_ot & 1.00000 \nonumber\\
but_kid & 1.00000 \nonumber\\
certain_thing & 1.00000 \nonumber\\
uniform_help & 1.00000 \nonumber\\
ot_have & 1.00000 \nonumber\\
have_specific & 1.00000 \nonumber\\
creationist_. & 1.00000 \nonumber\\
uniform_to & 1.00000 \nonumber\\
_pos_ngram_PR_ART_ADV & 1.00000 \nonumber\\
i_assume & 1.00000 \nonumber\\
be_probably & 1.00000 \nonumber\\
other_, & 1.00000 \nonumber\\
could_also & 1.00000 \nonumber\\
account & 1.00000 \nonumber\\
take_on & 1.00000 \nonumber\\
child_she & 1.00000 \nonumber\\
who_would & 1.00000 \nonumber\\
man_to & 1.00000 \nonumber\\
watch_and & 1.00000 \nonumber\\
for_kid & 1.00000 \nonumber\\
have_a & 1.00000 \nonumber\\
yr & 1.00000 \nonumber\\
matter_if & 1.00000 \nonumber\\
so_yea & 1.00000 \nonumber\\
be_guilty & 1.00000 \nonumber\\
same_ever & 1.00000 \nonumber\\
spouse_the & 1.00000 \nonumber\\
under_any & 1.00000 \nonumber\\
commit_the & 1.00000 \nonumber\\
circumstance_be & 1.00000 \nonumber\\
secret_of & 1.00000 \nonumber\\
guilty_. & 1.00000 \nonumber\\
any_circumstance & 1.00000 \nonumber\\
ever_again & 1.00000 \nonumber\\
murder_under & 1.00000 \nonumber\\
act_know & 1.00000 \nonumber\\
ProductionRule_ADJP->ADJP,PRN, & 1.00000 \nonumber\\
believe_book & 1.00000 \nonumber\\
can_fly & 1.00000 \nonumber\\
so_true & 1.00000 \nonumber\\
ProductionRule_SBAR->WHNP,S,:, & 1.00000 \nonumber\\
..._) & 1.00000 \nonumber\\
fly_... & 1.00000 \nonumber\\
ProductionRule_VP->VBP,ADJP,ADVP,ADJP, & 1.00000 \nonumber\\
better_( & 1.00000 \nonumber\\
_pos_ngram_PP_CONJ_PR & 1.00000 \nonumber\\
really_love & 1.00000 \nonumber\\
through_anything & 1.00000 \nonumber\\
back_through & 1.00000 \nonumber\\
anything_good & 1.00000 \nonumber\\
her_back & 1.00000 \nonumber\\
her_then & 1.00000 \nonumber\\
plenty & 1.00000 \nonumber\\
be_plenty & 1.00000 \nonumber\\
plenty_of & 1.00000 \nonumber\\
stop_something & 1.00000 \nonumber\\
already_do & 1.00000 \nonumber\\
pornography_, & 1.00000 \nonumber\\
already_happen & 1.00000 \nonumber\\
ProductionRule_SBARQ->SBAR,,,WHADVP,SQ, & 1.00000 \nonumber\\
it_: & 1.00000 \nonumber\\
,_woman & 1.00000 \nonumber\\
'_already & 1.00000 \nonumber\\
:_p & 1.00000 \nonumber\\
yell & 1.00000 \nonumber\\
even_a & 1.00000 \nonumber\\
ProductionRule_NP->NP,PP,NP, & 1.00000 \nonumber\\
other_option & 1.00000 \nonumber\\
parent_have & 1.00000 \nonumber\\
option_before & 1.00000 \nonumber\\
proper_way & 1.00000 \nonumber\\
before_spank & 1.00000 \nonumber\\
lot_other & 1.00000 \nonumber\\
a_proper & 1.00000 \nonumber\\
happy_? & 1.00000 \nonumber\\
ever_mention & 1.00000 \nonumber\\
unwant_pregnancy & 1.00000 \nonumber\\
over_99 & 1.00000 \nonumber\\
all_abortion & 1.00000 \nonumber\\
prevent_those & 1.00000 \nonumber\\
prevent_abortion & 1.00000 \nonumber\\
side_happy & 1.00000 \nonumber\\
of_over & 1.00000 \nonumber\\
you_prevent & 1.00000 \nonumber\\
be_unwant & 1.00000 \nonumber\\
those_, & 1.00000 \nonumber\\
make_both & 1.00000 \nonumber\\
cause_of & 1.00000 \nonumber\\
ProductionRule_SQ->VBZ,ADJP, & 1.00000 \nonumber\\
let_people & 1.00000 \nonumber\\
ProductionRule_SQ->VBP,NP,S, & 1.00000 \nonumber\\
just_let & 1.00000 \nonumber\\
we_not & 1.00000 \nonumber\\
consequence_? & 1.00000 \nonumber\\
?_can & 1.00000 \nonumber\\
back_and & 1.00000 \nonumber\\
a_class & 1.00000 \nonumber\\
every_couple & 1.00000 \nonumber\\
a_useless & 1.00000 \nonumber\\
join_. & 1.00000 \nonumber\\
mile_without & 1.00000 \nonumber\\
couple_foot & 1.00000 \nonumber\\
get_prepare & 1.00000 \nonumber\\
useless_class & 1.00000 \nonumber\\
without_stop & 1.00000 \nonumber\\
not_run & 1.00000 \nonumber\\
class_time & 1.00000 \nonumber\\
their_career & 1.00000 \nonumber\\
gym_class & 1.00000 \nonumber\\
waste_time & 1.00000 \nonumber\\
just_there & 1.00000 \nonumber\\
for_sport & 1.00000 \nonumber\\
foot_they & 1.00000 \nonumber\\
can_join & 1.00000 \nonumber\\
test_and & 1.00000 \nonumber\\
career_and & 1.00000 \nonumber\\
should_join & 1.00000 \nonumber\\
it_toward & 1.00000 \nonumber\\
stop_every & 1.00000 \nonumber\\
foot & 1.00000 \nonumber\\
fact_people & 1.00000 \nonumber\\
student_waste & 1.00000 \nonumber\\
a_test & 1.00000 \nonumber\\
join_to & 1.00000 \nonumber\\
creationism_be & 1.00000 \nonumber\\
correctly & 1.00000 \nonumber\\
correctly_. & 1.00000 \nonumber\\
could_turn & 1.00000 \nonumber\\
herself_in & 1.00000 \nonumber\\
pupil_be & 1.00000 \nonumber\\
not_rare & 1.00000 \nonumber\\
to_enjoy & 1.00000 \nonumber\\
couple_do & 1.00000 \nonumber\\
benefit_that & 1.00000 \nonumber\\
can_anyone & 1.00000 \nonumber\\
enjoy_all & 1.00000 \nonumber\\
anyone_say & 1.00000 \nonumber\\
that_straight & 1.00000 \nonumber\\
make_from & 1.00000 \nonumber\\
belief_so & 1.00000 \nonumber\\
in_turn & 1.00000 \nonumber\\
public_gamble & 1.00000 \nonumber\\
to_activity & 1.00000 \nonumber\\
as_public & 1.00000 \nonumber\\
in_singapore.this & 1.00000 \nonumber\\
slavery_to & 1.00000 \nonumber\\
be_control & 1.00000 \nonumber\\
gamble_and & 1.00000 \nonumber\\
establish_local & 1.00000 \nonumber\\
magistrate_lead & 1.00000 \nonumber\\
control_farquar & 1.00000 \nonumber\\
magistrate_in & 1.00000 \nonumber\\
singapore.this_local & 1.00000 \nonumber\\
magistrate & 1.00000 \nonumber\\
activity_such & 1.00000 \nonumber\\
and_slavery & 1.00000 \nonumber\\
local_magistrate & 1.00000 \nonumber\\
ushould & 1.00000 \nonumber\\
nobody_tell & 1.00000 \nonumber\\
thier_bid & 1.00000 \nonumber\\
ushould_be & 1.00000 \nonumber\\
thik_thier & 1.00000 \nonumber\\
thik & 1.00000 \nonumber\\
tell_u & 1.00000 \nonumber\\
ProductionRule_NP->ADVP,NN, & 1.00000 \nonumber\\
i_thik & 1.00000 \nonumber\\
out_nobody & 1.00000 \nonumber\\
ProductionRule_ADJP->JJR,NN, & 1.00000 \nonumber\\
think_ushould & 1.00000 \nonumber\\
wat_to & 1.00000 \nonumber\\
u_wat & 1.00000 \nonumber\\
not_start & 1.00000 \nonumber\\
much_for & 1.00000 \nonumber\\
if_farquhar & 1.00000 \nonumber\\
still_found & 1.00000 \nonumber\\
tag_along & 1.00000 \nonumber\\
port_. & 1.00000 \nonumber\\
expedition_in & 1.00000 \nonumber\\
the_expedition & 1.00000 \nonumber\\
expedition & 1.00000 \nonumber\\
that_lead & 1.00000 \nonumber\\
so_even & 1.00000 \nonumber\\
new_trade & 1.00000 \nonumber\\
only_tag & 1.00000 \nonumber\\
have_still & 1.00000 \nonumber\\
come_raffle & 1.00000 \nonumber\\
tag & 1.00000 \nonumber\\
raffle_would & 1.00000 \nonumber\\
raffle_that & 1.00000 \nonumber\\
farquhar_only & 1.00000 \nonumber\\
situation_... & 1.00000 \nonumber\\
deserve_it & 1.00000 \nonumber\\
this_a & 1.00000 \nonumber\\
not_situation & 1.00000 \nonumber\\
scary_to & 1.00000 \nonumber\\
a_maybe & 1.00000 \nonumber\\
scary & 1.00000 \nonumber\\
ProductionRule_NP->RB,DT,ADJP,NN, & 1.00000 \nonumber\\
that_deserve & 1.00000 \nonumber\\
sleep_with & 1.00000 \nonumber\\
_pos_ngram_ART_ART_ADV & 1.00000 \nonumber\\
so_yeah & 1.00000 \nonumber\\
much_depend & 1.00000 \nonumber\\
yeah_im & 1.00000 \nonumber\\
maybe_/ & 1.00000 \nonumber\\
all_pretty & 1.00000 \nonumber\\
so_this & 1.00000 \nonumber\\
well_it & 1.00000 \nonumber\\
depend_.... & 1.00000 \nonumber\\
ProductionRule_ADVP->DT,RB,RB, & 1.00000 \nonumber\\
...._like & 1.00000 \nonumber\\
/_maybe & 1.00000 \nonumber\\
be_scary & 1.00000 \nonumber\\
it_well & 1.00000 \nonumber\\
to_sure & 1.00000 \nonumber\\
cool_skin & 1.00000 \nonumber\\
everything_else & 1.00000 \nonumber\\
my_browser & 1.00000 \nonumber\\
ie_provide & 1.00000 \nonumber\\
check_along & 1.00000 \nonumber\\
in_spell & 1.00000 \nonumber\\
build_in & 1.00000 \nonumber\\
a_build & 1.00000 \nonumber\\
n't_beat & 1.00000 \nonumber\\
pimp & 1.00000 \nonumber\\
spell_check & 1.00000 \nonumber\\
else_that & 1.00000 \nonumber\\
beat_it & 1.00000 \nonumber\\
that_ie & 1.00000 \nonumber\\
amazingly_cool & 1.00000 \nonumber\\
amazingly & 1.00000 \nonumber\\
pimp_my & 1.00000 \nonumber\\
me_pimp & 1.00000 \nonumber\\
skin_that & 1.00000 \nonumber\\
..._would & 1.00000 \nonumber\\
._ca & 1.00000 \nonumber\\
._some & 1.00000 \nonumber\\
not_come & 1.00000 \nonumber\\
straight_couple & 1.00000 \nonumber\\
_pos_ngram_PUNC_PR_ART & 1.00000 \nonumber\\
follow_by & 1.00000 \nonumber\\
the_fatherly & 1.00000 \nonumber\\
by_them & 1.00000 \nonumber\\
sickness & 1.00000 \nonumber\\
sickness_and & 1.00000 \nonumber\\
her_from & 1.00000 \nonumber\\
vow_say & 1.00000 \nonumber\\
to_stick & 1.00000 \nonumber\\
head_but & 1.00000 \nonumber\\
ProductionRule_VP->VP,SBAR, & 1.00000 \nonumber\\
anything_id & 1.00000 \nonumber\\
from_get & 1.00000 \nonumber\\
id_be & 1.00000 \nonumber\\
in_sickness & 1.00000 \nonumber\\
be_sick & 1.00000 \nonumber\\
if_anything & 1.00000 \nonumber\\
and_health & 1.00000 \nonumber\\
keep_her & 1.00000 \nonumber\\
a_vow & 1.00000 \nonumber\\
teach_but & 1.00000 \nonumber\\
want_an & 1.00000 \nonumber\\
less_fat & 1.00000 \nonumber\\
some_health & 1.00000 \nonumber\\
it_offer & 1.00000 \nonumber\\
offer_child & 1.00000 \nonumber\\
obese_anymore & 1.00000 \nonumber\\
ProductionRule_VP->VB,ADJP,S,SBAR, & 1.00000 \nonumber\\
class_would & 1.00000 \nonumber\\
class_in & 1.00000 \nonumber\\
course_also & 1.00000 \nonumber\\
diet_and & 1.00000 \nonumber\\
basic_diet & 1.00000 \nonumber\\
fat_child & 1.00000 \nonumber\\
world_pe & 1.00000 \nonumber\\
child_know & 1.00000 \nonumber\\
be_include & 1.00000 \nonumber\\
every_school & 1.00000 \nonumber\\
school_of & 1.00000 \nonumber\\
a_basic & 1.00000 \nonumber\\
if_in & 1.00000 \nonumber\\
include_so & 1.00000 \nonumber\\
child_a & 1.00000 \nonumber\\
obligatory_to & 1.00000 \nonumber\\
obligatory_there & 1.00000 \nonumber\\
city_.... & 1.00000 \nonumber\\
have_strong & 1.00000 \nonumber\\
..._indium & 1.00000 \nonumber\\
tense & 1.00000 \nonumber\\
have_territorial & 1.00000 \nonumber\\
ProductionRule_NP->NN,NNP,NNP,NNP,NNP,CC,NNP, & 1.00000 \nonumber\\
ProductionRule_S->S,:,S,:,CC,S, & 1.00000 \nonumber\\
relation_with & 1.00000 \nonumber\\
territorial & 1.00000 \nonumber\\
&_pakistan & 1.00000 \nonumber\\
corridor_and & 1.00000 \nonumber\\
pak & 1.00000 \nonumber\\
territorial_dispute & 1.00000 \nonumber\\
(_china & 1.00000 \nonumber\\
interference_in & 1.00000 \nonumber\\
of_territorial & 1.00000 \nonumber\\
also_become & 1.00000 \nonumber\\
war_for & 1.00000 \nonumber\\
fight_4 & 1.00000 \nonumber\\
tense_with & 1.00000 \nonumber\\
rise_of & 1.00000 \nonumber\\
with_pakistan & 1.00000 \nonumber\\
example_pak & 1.00000 \nonumber\\
this_... & 1.00000 \nonumber\\
pakistan_china & 1.00000 \nonumber\\
in_pakistan & 1.00000 \nonumber\\
as_pakistan & 1.00000 \nonumber\\
bid_relation & 1.00000 \nonumber\\
4_war & 1.00000 \nonumber\\
pakistan_as & 1.00000 \nonumber\\
pakistan_.... & 1.00000 \nonumber\\
...._as & 1.00000 \nonumber\\
also_fight & 1.00000 \nonumber\\
...._for & 1.00000 \nonumber\\
plan_.... & 1.00000 \nonumber\\
gawadar_mega & 1.00000 \nonumber\\
neighbor_( & 1.00000 \nonumber\\
mega_oil & 1.00000 \nonumber\\
corridor & 1.00000 \nonumber\\
pakistan_) & 1.00000 \nonumber\\
have_long & 1.00000 \nonumber\\
oil_city & 1.00000 \nonumber\\
pakistan & 1.00000 \nonumber\\
pak_china & 1.00000 \nonumber\\
and_gawadar & 1.00000 \nonumber\\
indium_interference & 1.00000 \nonumber\\
indium_relation & 1.00000 \nonumber\\
gawadar & 1.00000 \nonumber\\
interference & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,NP,PP,SBAR, & 1.00000 \nonumber\\
mega & 1.00000 \nonumber\\
strong_military & 1.00000 \nonumber\\
ProductionRule_S->ADVP,,,NP,ADVP,VP, & 1.00000 \nonumber\\
_pos_ngram_CONJ_NP_ADJ & 1.00000 \nonumber\\
military_neighbor & 1.00000 \nonumber\\
..._due & 1.00000 \nonumber\\
china_& & 1.00000 \nonumber\\
china_economic & 1.00000 \nonumber\\
china_have & 1.00000 \nonumber\\
term_plan & 1.00000 \nonumber\\
)_... & 1.00000 \nonumber\\
as_china & 1.00000 \nonumber\\
economic_corridor & 1.00000 \nonumber\\
relation_also & 1.00000 \nonumber\\
become_tense & 1.00000 \nonumber\\
dispute_and & 1.00000 \nonumber\\
china_... & 1.00000 \nonumber\\
military & 1.00000 \nonumber\\
china_, & 1.00000 \nonumber\\
due_rise & 1.00000 \nonumber\\
_pos_ngram_PP_CARD_CARD & 1.00000 \nonumber\\
stuff_themselve & 1.00000 \nonumber\\
of_kid & 1.00000 \nonumber\\
effect_, & 1.00000 \nonumber\\
barely_take & 1.00000 \nonumber\\
junk_food & 1.00000 \nonumber\\
eat_campaign & 1.00000 \nonumber\\
junk & 1.00000 \nonumber\\
take_any & 1.00000 \nonumber\\
around_since & 1.00000 \nonumber\\
since_more & 1.00000 \nonumber\\
obesity_, & 1.00000 \nonumber\\
the_pe & 1.00000 \nonumber\\
200_year & 1.00000 \nonumber\\
campaign & 1.00000 \nonumber\\
._pe & 1.00000 \nonumber\\
kid_stuff & 1.00000 \nonumber\\
with_junk & 1.00000 \nonumber\\
,_mainly & 1.00000 \nonumber\\
than_200 & 1.00000 \nonumber\\
prevent_obesity & 1.00000 \nonumber\\
healthy_eat & 1.00000 \nonumber\\
campaign_. & 1.00000 \nonumber\\
any_effect & 1.00000 \nonumber\\
in_class & 1.00000 \nonumber\\
-_the & 1.00000 \nonumber\\
"_particle & 1.00000 \nonumber\\
that_cause & 1.00000 \nonumber\\
evolution_theory & 1.00000 \nonumber\\
out_creation & 1.00000 \nonumber\\
particle_" & 1.00000 \nonumber\\
particle & 1.00000 \nonumber\\
accept_truth & 1.00000 \nonumber\\
withstand_the & 1.00000 \nonumber\\
amount_support & 1.00000 \nonumber\\
creation_, & 1.00000 \nonumber\\
creation_. & 1.00000 \nonumber\\
and_quite & 1.00000 \nonumber\\
be_interest & 1.00000 \nonumber\\
interest_, & 1.00000 \nonumber\\
creation_can & 1.00000 \nonumber\\
possible_theory & 1.00000 \nonumber\\
an_evolutionary & 1.00000 \nonumber\\
explanation_provide & 1.00000 \nonumber\\
evolutionary_argument & 1.00000 \nonumber\\
on_convince & 1.00000 \nonumber\\
little_evidence & 1.00000 \nonumber\\
,_creation & 1.00000 \nonumber\\
since_creation & 1.00000 \nonumber\\
withstand & 1.00000 \nonumber\\
that_creation & 1.00000 \nonumber\\
possible_, & 1.00000 \nonumber\\
evolution_can & 1.00000 \nonumber\\
evidence_support & 1.00000 \nonumber\\
evidence_must & 1.00000 \nonumber\\
not_rule & 1.00000 \nonumber\\
false_, & 1.00000 \nonumber\\
best_possible & 1.00000 \nonumber\\
,_evidence & 1.00000 \nonumber\\
be_massive & 1.00000 \nonumber\\
must_withstand & 1.00000 \nonumber\\
"_true & 1.00000 \nonumber\\
no_explanation & 1.00000 \nonumber\\
the_test & 1.00000 \nonumber\\
quite_possible & 1.00000 \nonumber\\
support_creation & 1.00000 \nonumber\\
massive_amount & 1.00000 \nonumber\\
massive & 1.00000 \nonumber\\
support_an & 1.00000 \nonumber\\
convince_evidence & 1.00000 \nonumber\\
rule_out & 1.00000 \nonumber\\
"_debate & 1.00000 \nonumber\\
provide_for & 1.00000 \nonumber\\
although_the & 1.00000 \nonumber\\
n't_say & 1.00000 \nonumber\\
of_accept & 1.00000 \nonumber\\
assist & 1.00000 \nonumber\\
to_assist & 1.00000 \nonumber\\
children & 1.00000 \nonumber\\
ever_lead & 1.00000 \nonumber\\
_pos_ngram_O_ART_PR & 1.00000 \nonumber\\
_pos_ngram_ART_NP_NN & 1.00000 \nonumber\\
demand & 1.00000 \nonumber\\
themselve_up & 1.00000 \nonumber\\
be_? & 1.00000 \nonumber\\
all_about & 1.00000 \nonumber\\
none_... & 1.00000 \nonumber\\
no_proof & 1.00000 \nonumber\\
back_themselve & 1.00000 \nonumber\\
where_atheist & 1.00000 \nonumber\\
religion_proof & 1.00000 \nonumber\\
everyone_know & 1.00000 \nonumber\\
religion_have & 1.00000 \nonumber\\
proof_atheist & 1.00000 \nonumber\\
proof_so & 1.00000 \nonumber\\
know_evolution & 1.00000 \nonumber\\
on_proof & 1.00000 \nonumber\\
?_make & 1.00000 \nonumber\\
though_they & 1.00000 \nonumber\\
atheist_? & 1.00000 \nonumber\\
._where & 1.00000 \nonumber\\
ProductionRule_S->NP,VP,:,SBAR, & 1.00000 \nonumber\\
christian_do & 1.00000 \nonumber\\
atheist_have & 1.00000 \nonumber\\
atheist_rely & 1.00000 \nonumber\\
have_? & 1.00000 \nonumber\\
when_christian & 1.00000 \nonumber\\
with_, & 1.00000 \nonumber\\
proof_even & 1.00000 \nonumber\\
?_evolution & 1.00000 \nonumber\\
to_their & 1.00000 \nonumber\\
water_system & 1.00000 \nonumber\\
divorce & 1.00000 \nonumber\\
to_mention & 1.00000 \nonumber\\
_pos_ngram_PUNC_CONJ_PUNC & 1.00000 \nonumber\\
his_time & 1.00000 \nonumber\\
diverse_culture & 1.00000 \nonumber\\
saare & 1.00000 \nonumber\\
achcha & 1.00000 \nonumber\\
saare_jagah & 1.00000 \nonumber\\
se_achcha & 1.00000 \nonumber\\
good_country & 1.00000 \nonumber\\
in_... & 1.00000 \nonumber\\
se & 1.00000 \nonumber\\
hamara & 1.00000 \nonumber\\
culture_but & 1.00000 \nonumber\\
hamara_... & 1.00000 \nonumber\\
achcha_... & 1.00000 \nonumber\\
jagah_se & 1.00000 \nonumber\\
unite_as & 1.00000 \nonumber\\
._saare & 1.00000 \nonumber\\
have_diverse & 1.00000 \nonumber\\
..._hindustan & 1.00000 \nonumber\\
jagah & 1.00000 \nonumber\\
it_unite & 1.00000 \nonumber\\
still_it & 1.00000 \nonumber\\
hindustan & 1.00000 \nonumber\\
hindustan_hamara & 1.00000 \nonumber\\
the_middle & 1.00000 \nonumber\\
ProductionRule_SQ->MD,RB,NP,VP, & 1.00000 \nonumber\\
essentially & 1.00000 \nonumber\\
be_essentially & 1.00000 \nonumber\\
and_when & 1.00000 \nonumber\\
so_he & 1.00000 \nonumber\\
go_. & 1.00000 \nonumber\\
greedy & 1.00000 \nonumber\\
....._it & 1.00000 \nonumber\\
way_it & 1.00000 \nonumber\\
difficult_to & 1.00000 \nonumber\\
_pos_ngram_PUNC_O_CARD & 1.00000 \nonumber\\
ProductionRule_ADVP->RB,NP,PP, & 1.00000 \nonumber\\
the_place & 1.00000 \nonumber\\
and_establish & 1.00000 \nonumber\\
key_in & 1.00000 \nonumber\\
well_the & 1.00000 \nonumber\\
farquhar_who & 1.00000 \nonumber\\
be_farquhar & 1.00000 \nonumber\\
discuss & 1.00000 \nonumber\\
ProductionRule_VP->VP,CC,VP,:,SBAR, & 1.00000 \nonumber\\
a_global & 1.00000 \nonumber\\
place_and & 1.00000 \nonumber\\
..._although & 1.00000 \nonumber\\
place_but & 1.00000 \nonumber\\
that_founder & 1.00000 \nonumber\\
this_to & 1.00000 \nonumber\\
global_level & 1.00000 \nonumber\\
who_suggest & 1.00000 \nonumber\\
of_founder & 1.00000 \nonumber\\
ProductionRule_NP->ADVP,DT,NN, & 1.00000 \nonumber\\
discuss_in & 1.00000 \nonumber\\
establish_it & 1.00000 \nonumber\\
that_day & 1.00000 \nonumber\\
who_discover & 1.00000 \nonumber\\
suggest & 1.00000 \nonumber\\
ProductionRule_VP->VBD,RB,NP, & 1.00000 \nonumber\\
level_... & 1.00000 \nonumber\\
suggest_this & 1.00000 \nonumber\\
founder_discuss & 1.00000 \nonumber\\
remember_that & 1.00000 \nonumber\\
learn_in & 1.00000 \nonumber\\
something_bid & 1.00000 \nonumber\\
they_remember & 1.00000 \nonumber\\
have_those & 1.00000 \nonumber\\
give_an & 1.00000 \nonumber\\
front_of & 1.00000 \nonumber\\
in_front & 1.00000 \nonumber\\
baby_as & 1.00000 \nonumber\\
its_like & 1.00000 \nonumber\\
a_trade & 1.00000 \nonumber\\
not_want & 1.00000 \nonumber\\
idea!yes & 1.00000 \nonumber\\
as_previous & 1.00000 \nonumber\\
child_at & 1.00000 \nonumber\\
to_wear!because & 1.00000 \nonumber\\
ProductionRule_NP->JJ,FW,FW, & 1.00000 \nonumber\\
say_child & 1.00000 \nonumber\\
teenager_. & 1.00000 \nonumber\\
of_pupil & 1.00000 \nonumber\\
idea!yes_i & 1.00000 \nonumber\\
of_benefit & 1.00000 \nonumber\\
very_big & 1.00000 \nonumber\\
wear!because_it & 1.00000 \nonumber\\
first_do & 1.00000 \nonumber\\
pupil_do & 1.00000 \nonumber\\
previous_people & 1.00000 \nonumber\\
for_teenager & 1.00000 \nonumber\\
good_idea!yes & 1.00000 \nonumber\\
wear!because & 1.00000 \nonumber\\
but_however & 1.00000 \nonumber\\
be_false & 1.00000 \nonumber\\
now_know & 1.00000 \nonumber\\
the_unite & 1.00000 \nonumber\\
unite_state & 1.00000 \nonumber\\
!!!!! & 1.00000 \nonumber\\
uniform_also & 1.00000 \nonumber\\
everything_come & 1.00000 \nonumber\\
gene & 1.00000 \nonumber\\
_pos_ngram_CONJ_NP_NN & 1.00000 \nonumber\\
at_me & 1.00000 \nonumber\\
condone_slavery & 1.00000 \nonumber\\
also_mention & 1.00000 \nonumber\\
christianity_condone & 1.00000 \nonumber\\
jot_i & 1.00000 \nonumber\\
slavery_? & 1.00000 \nonumber\\
jot & 1.00000 \nonumber\\
if_jot & 1.00000 \nonumber\\
look_to & 1.00000 \nonumber\\
education_be & 1.00000 \nonumber\\
a_son & 1.00000 \nonumber\\
result_in & 1.00000 \nonumber\\
ProductionRule_S->NP,VP,'',., & 1.00000 \nonumber\\
in_develop & 1.00000 \nonumber\\
ProductionRule_VP->VBD,NP,PP,PP, & 1.00000 \nonumber\\
selfish_. & 1.00000 \nonumber\\
the_decision & 1.00000 \nonumber\\
then_to & 1.00000 \nonumber\\
stand & 1.00000 \nonumber\\
this_grow & 1.00000 \nonumber\\
grow_condition & 1.00000 \nonumber\\
london_and & 1.00000 \nonumber\\
ProductionRule_NP->NNP,NNP,NNP,JJ,NNS, & 1.00000 \nonumber\\
illitrate_here & 1.00000 \nonumber\\
condition_idium & 1.00000 \nonumber\\
idium & 1.00000 \nonumber\\
illitrate & 1.00000 \nonumber\\
idium_can & 1.00000 \nonumber\\
replace_other & 1.00000 \nonumber\\
indium_cant & 1.00000 \nonumber\\
london & 1.00000 \nonumber\\
think_indium & 1.00000 \nonumber\\
not_replace & 1.00000 \nonumber\\
other_develop & 1.00000 \nonumber\\
think_with & 1.00000 \nonumber\\
usa_london & 1.00000 \nonumber\\
like_usa & 1.00000 \nonumber\\
be_illitrate & 1.00000 \nonumber\\
country_like & 1.00000 \nonumber\\
_pos_ngram_NP_NP_ADJ & 1.00000 \nonumber\\
ProductionRule_NP->DT,VBG,NN,NN, & 1.00000 \nonumber\\
cant_. & 1.00000 \nonumber\\
and_an & 1.00000 \nonumber\\
until_he & 1.00000 \nonumber\\
or_how & 1.00000 \nonumber\\
it_until & 1.00000 \nonumber\\
'_its & 1.00000 \nonumber\\
good_your & 1.00000 \nonumber\\
i_myself & 1.00000 \nonumber\\
like_have & 1.00000 \nonumber\\
reality_you & 1.00000 \nonumber\\
myself_know & 1.00000 \nonumber\\
how_good & 1.00000 \nonumber\\
constitutional_way & 1.00000 \nonumber\\
america_, & 1.00000 \nonumber\\
only_constitutional & 1.00000 \nonumber\\
,_pro-choice & 1.00000 \nonumber\\
elsewhere_in & 1.00000 \nonumber\\
ProductionRule_NP->DT,RB,JJ,NN, & 1.00000 \nonumber\\
._elsewhere & 1.00000 \nonumber\\
constitutional & 1.00000 \nonumber\\
elsewhere & 1.00000 \nonumber\\
put_together & 1.00000 \nonumber\\
as_likely & 1.00000 \nonumber\\
tornado & 1.00000 \nonumber\\
747 & 1.00000 \nonumber\\
747_airplane & 1.00000 \nonumber\\
a_tornado & 1.00000 \nonumber\\
through_a & 1.00000 \nonumber\\
a_junkyard & 1.00000 \nonumber\\
junkyard_and & 1.00000 \nonumber\\
a_747 & 1.00000 \nonumber\\
likely_as & 1.00000 \nonumber\\
airplane & 1.00000 \nonumber\\
tornado_go & 1.00000 \nonumber\\
junkyard & 1.00000 \nonumber\\
airplane_. & 1.00000 \nonumber\\
together_a & 1.00000 \nonumber\\
argument_that & 1.00000 \nonumber\\
test_of & 1.00000 \nonumber\\
ot & 1.00000 \nonumber\\
dasanus_( & 1.00000 \nonumber\\
aquafina_( & 1.00000 \nonumber\\
american_water & 1.00000 \nonumber\\
ProductionRule_NP->DT,NNP,NNP,NNS, & 1.00000 \nonumber\\
provide_job & 1.00000 \nonumber\\
american_citizen & 1.00000 \nonumber\\
which_provide & 1.00000 \nonumber\\
,_perrier & 1.00000 \nonumber\\
perrier & 1.00000 \nonumber\\
(_pepsi & 1.00000 \nonumber\\
nestle_) & 1.00000 \nonumber\\
ProductionRule_NP->NP,PRN,,,NP,PRN,SBAR, & 1.00000 \nonumber\\
(_coke & 1.00000 \nonumber\\
ProductionRule_S->NP,VP,,, & 1.00000 \nonumber\\
,_dasanus & 1.00000 \nonumber\\
coke & 1.00000 \nonumber\\
coke_) & 1.00000 \nonumber\\
be_aquafina & 1.00000 \nonumber\\
pepsi_) & 1.00000 \nonumber\\
(_nestle & 1.00000 \nonumber\\
perrier_( & 1.00000 \nonumber\\
important_thing & 1.00000 \nonumber\\
drink_water & 1.00000 \nonumber\\
oblivious_to & 1.00000 \nonumber\\
oblivious & 1.00000 \nonumber\\
be_oblivious & 1.00000 \nonumber\\
own_planet & 1.00000 \nonumber\\
be_own & 1.00000 \nonumber\\
destroy_be & 1.00000 \nonumber\\
people_drink & 1.00000 \nonumber\\
be_destroy & 1.00000 \nonumber\\
me_believe & 1.00000 \nonumber\\
around_and & 1.00000 \nonumber\\
would_come & 1.00000 \nonumber\\
could_knock & 1.00000 \nonumber\\
even_get & 1.00000 \nonumber\\
father_make & 1.00000 \nonumber\\
would_never & 1.00000 \nonumber\\
atleast & 1.00000 \nonumber\\
never_even & 1.00000 \nonumber\\
lousy_do & 1.00000 \nonumber\\
atleast_you & 1.00000 \nonumber\\
because_atleast & 1.00000 \nonumber\\
participate_in & 1.00000 \nonumber\\
of_right & 1.00000 \nonumber\\
morality_. & 1.00000 \nonumber\\
of_morality & 1.00000 \nonumber\\
choice_not & 1.00000 \nonumber\\
?_absolutley & 1.00000 \nonumber\\
your_the & 1.00000 \nonumber\\
own_definition & 1.00000 \nonumber\\
,_porn & 1.00000 \nonumber\\
porn_or & 1.00000 \nonumber\\
absolutley_not & 1.00000 \nonumber\\
not_!! & 1.00000 \nonumber\\
enjoy_it & 1.00000 \nonumber\\
who_participate & 1.00000 \nonumber\\
probably_enjoy & 1.00000 \nonumber\\
whether_your & 1.00000 \nonumber\\
!!_everyone & 1.00000 \nonumber\\
or_participate & 1.00000 \nonumber\\
person_watch & 1.00000 \nonumber\\
porn_wrong & 1.00000 \nonumber\\
never_come & 1.00000 \nonumber\\
should_alway & 1.00000 \nonumber\\
._after & 1.00000 \nonumber\\
child_for & 1.00000 \nonumber\\
every_little & 1.00000 \nonumber\\
'_some & 1.00000 \nonumber\\
obligatory & 1.00000 \nonumber\\
be_obligatory & 1.00000 \nonumber\\
pe_. & 1.00000 \nonumber\\
example_some & 1.00000 \nonumber\\
some_r & 1.00000 \nonumber\\
train_like & 1.00000 \nonumber\\
alreaddy_train & 1.00000 \nonumber\\
alreaddy & 1.00000 \nonumber\\
already_in & 1.00000 \nonumber\\
simply_can & 1.00000 \nonumber\\
athletics & 1.00000 \nonumber\\
take_pe & 1.00000 \nonumber\\
like_crazy & 1.00000 \nonumber\\
child_simply & 1.00000 \nonumber\\
athletics_and & 1.00000 \nonumber\\
r_already & 1.00000 \nonumber\\
be_alreaddy & 1.00000 \nonumber\\
4_example & 1.00000 \nonumber\\
in_athletics & 1.00000 \nonumber\\
be_leave & 1.00000 \nonumber\\
want_and & 1.00000 \nonumber\\
study_have & 1.00000 \nonumber\\
thing_for & 1.00000 \nonumber\\
need_proof & 1.00000 \nonumber\\
prime & 1.00000 \nonumber\\
or_lousy & 1.00000 \nonumber\\
arm & 1.00000 \nonumber\\
browser_, & 1.00000 \nonumber\\
ProductionRule_ADVP->RBS,RB, & 1.00000 \nonumber\\
baseball & 1.00000 \nonumber\\
baseball_, & 1.00000 \nonumber\\
doubt & 1.00000 \nonumber\\
be_tough & 1.00000 \nonumber\\
challenge_but & 1.00000 \nonumber\\
dependant_on & 1.00000 \nonumber\\
people_struggle & 1.00000 \nonumber\\
hard_but & 1.00000 \nonumber\\
a_challenge & 1.00000 \nonumber\\
down_to & 1.00000 \nonumber\\
come_down & 1.00000 \nonumber\\
and_dependant & 1.00000 \nonumber\\
on_themselve & 1.00000 \nonumber\\
tough_and & 1.00000 \nonumber\\
allow_them & 1.00000 \nonumber\\
dependant & 1.00000 \nonumber\\
they_teach & 1.00000 \nonumber\\
tough & 1.00000 \nonumber\\
expand_. & 1.00000 \nonumber\\
struggle_with & 1.00000 \nonumber\\
to_expand & 1.00000 \nonumber\\
she_make & 1.00000 \nonumber\\
problem_when & 1.00000 \nonumber\\
keep_it & 1.00000 \nonumber\\
one_day & 1.00000 \nonumber\\
good_adopter & 1.00000 \nonumber\\
adopter_but & 1.00000 \nonumber\\
and_leader & 1.00000 \nonumber\\
developer_and & 1.00000 \nonumber\\
great_developer & 1.00000 \nonumber\\
leader_should & 1.00000 \nonumber\\
adopter & 1.00000 \nonumber\\
lousy_but & 1.00000 \nonumber\\
appropriate_spank & 1.00000 \nonumber\\
in_fear & 1.00000 \nonumber\\
appropriate & 1.00000 \nonumber\\
a_line & 1.00000 \nonumber\\
consequence_. & 1.00000 \nonumber\\
n't_cross & 1.00000 \nonumber\\
abuse_line & 1.00000 \nonumber\\
spank_again & 1.00000 \nonumber\\
the_appropriate & 1.00000 \nonumber\\
cross_such & 1.00000 \nonumber\\
line_a & 1.00000 \nonumber\\
a_product & 1.00000 \nonumber\\
we_ban & 1.00000 \nonumber\\
ban_a & 1.00000 \nonumber\\
a_recession & 1.00000 \nonumber\\
product_that & 1.00000 \nonumber\\
people_buy & 1.00000 \nonumber\\
buy_when & 1.00000 \nonumber\\
recession_? & 1.00000 \nonumber\\
that_more & 1.00000 \nonumber\\
ProductionRule_QP->JJR,IN,DT,CD, & 1.00000 \nonumber\\
order_for & 1.00000 \nonumber\\
ProductionRule_S->SBAR,:,NP,VP,., & 1.00000 \nonumber\\
accept_due & 1.00000 \nonumber\\
change_aspect & 1.00000 \nonumber\\
..._creation & 1.00000 \nonumber\\
someone_somewhere & 1.00000 \nonumber\\
universe_in & 1.00000 \nonumber\\
somewhere_have & 1.00000 \nonumber\\
'_your & 1.00000 \nonumber\\
the_consequence & 1.00000 \nonumber\\
operation_, & 1.00000 \nonumber\\
operation & 1.00000 \nonumber\\
_pos_ngram_V_NP_ART & 1.00000 \nonumber\\
holy & 1.00000 \nonumber\\
respect_for & 1.00000 \nonumber\\
and_their & 1.00000 \nonumber\\
would_still & 1.00000 \nonumber\\
mosy & 1.00000 \nonumber\\
believe_gay & 1.00000 \nonumber\\
allow_just & 1.00000 \nonumber\\
homosexuality_all & 1.00000 \nonumber\\
like_homosexuality & 1.00000 \nonumber\\
forever_why & 1.00000 \nonumber\\
marry_?? & 1.00000 \nonumber\\
all_together & 1.00000 \nonumber\\
other_forever & 1.00000 \nonumber\\
mosy_who & 1.00000 \nonumber\\
side_tend & 1.00000 \nonumber\\
allow_. & 1.00000 \nonumber\\
._mosy & 1.00000 \nonumber\\
oppose_side & 1.00000 \nonumber\\
two_man & 1.00000 \nonumber\\
two_woman & 1.00000 \nonumber\\
happy_together & 1.00000 \nonumber\\
be_prejudice & 1.00000 \nonumber\\
and_should & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,NP,NP, & 1.00000 \nonumber\\
and_everything & 1.00000 \nonumber\\
tubby & 1.00000 \nonumber\\
tubby_! & 1.00000 \nonumber\\
tubby_!!!!! & 1.00000 \nonumber\\
not_ok & 1.00000 \nonumber\\
because_kid & 1.00000 \nonumber\\
have_gym & 1.00000 \nonumber\\
and_tubby & 1.00000 \nonumber\\
gym_because & 1.00000 \nonumber\\
get_fat & 1.00000 \nonumber\\
trust_my & 1.00000 \nonumber\\
highly & 1.00000 \nonumber\\
they_r & 1.00000 \nonumber\\
brass & 1.00000 \nonumber\\
of_public & 1.00000 \nonumber\\
brass_ring & 1.00000 \nonumber\\
and_maintenance & 1.00000 \nonumber\\
,_wasteful & 1.00000 \nonumber\\
ProductionRule_NP->DT,NN,CC,NN, & 1.00000 \nonumber\\
and_distract & 1.00000 \nonumber\\
distract & 1.00000 \nonumber\\
of_safe & 1.00000 \nonumber\\
wasteful_and & 1.00000 \nonumber\\
the_construction & 1.00000 \nonumber\\
'_costly & 1.00000 \nonumber\\
ring & 1.00000 \nonumber\\
health_: & 1.00000 \nonumber\\
safe_municipal & 1.00000 \nonumber\\
ring_of & 1.00000 \nonumber\\
distract_from & 1.00000 \nonumber\\
maintenance & 1.00000 \nonumber\\
the_brass & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,ADJP,,,S, & 1.00000 \nonumber\\
public_health & 1.00000 \nonumber\\
construction_and & 1.00000 \nonumber\\
maintenance_of & 1.00000 \nonumber\\
costly_, & 1.00000 \nonumber\\
extension_which & 1.00000 \nonumber\\
base_community & 1.00000 \nonumber\\
it_win & 1.00000 \nonumber\\
therefore_it & 1.00000 \nonumber\\
user_base & 1.00000 \nonumber\\
the_user & 1.00000 \nonumber\\
user_make & 1.00000 \nonumber\\
cater_for & 1.00000 \nonumber\\
community_therefore & 1.00000 \nonumber\\
make_extension & 1.00000 \nonumber\\
cater & 1.00000 \nonumber\\
ProductionRule_PP->VBN,NP, & 1.00000 \nonumber\\
which_cater & 1.00000 \nonumber\\
ProductionRule_NP->NP,VP,SBAR, & 1.00000 \nonumber\\
gamble & 1.00000 \nonumber\\
gange & 1.00000 \nonumber\\
organize_their & 1.00000 \nonumber\\
poor_- & 1.00000 \nonumber\\
,_much & 1.00000 \nonumber\\
down-vote & 1.00000 \nonumber\\
gange_! & 1.00000 \nonumber\\
the_gange & 1.00000 \nonumber\\
own_budget & 1.00000 \nonumber\\
a_planet & 1.00000 \nonumber\\
defecate & 1.00000 \nonumber\\
their_dead & 1.00000 \nonumber\\
their_damn & 1.00000 \nonumber\\
insult_, & 1.00000 \nonumber\\
damn_street & 1.00000 \nonumber\\
get_down-vote & 1.00000 \nonumber\\
nah_, & 1.00000 \nonumber\\
defecate_in & 1.00000 \nonumber\\
even_organize & 1.00000 \nonumber\\
in_- & 1.00000 \nonumber\\
nah & 1.00000 \nonumber\\
even_manage & 1.00000 \nonumber\\
everything_i & 1.00000 \nonumber\\
manage_their & 1.00000 \nonumber\\
dead_and & 1.00000 \nonumber\\
down-vote_and & 1.00000 \nonumber\\
bathe & 1.00000 \nonumber\\
and_insult & 1.00000 \nonumber\\
bathe_in & 1.00000 \nonumber\\
but_everything & 1.00000 \nonumber\\
write_be & 1.00000 \nonumber\\
which_they & 1.00000 \nonumber\\
bury_their & 1.00000 \nonumber\\
same_river & 1.00000 \nonumber\\
bury & 1.00000 \nonumber\\
budget & 1.00000 \nonumber\\
extremely_poor & 1.00000 \nonumber\\
river_in & 1.00000 \nonumber\\
planet_! & 1.00000 \nonumber\\
street_! & 1.00000 \nonumber\\
less_a & 1.00000 \nonumber\\
and_defecate & 1.00000 \nonumber\\
budget_, & 1.00000 \nonumber\\
they_bury & 1.00000 \nonumber\\
they_bathe & 1.00000 \nonumber\\
"_look & 1.00000 \nonumber\\
run_away & 1.00000 \nonumber\\
as_of & 1.00000 \nonumber\\
for_" & 1.00000 \nonumber\\
ProductionRule_PRN->-LRB-,ADJP,-RRB-, & 1.00000 \nonumber\\
now_) & 1.00000 \nonumber\\
able_? & 1.00000 \nonumber\\
(_able & 1.00000 \nonumber\\
be_will & 1.00000 \nonumber\\
ProductionRule_ADJP->JJ,., & 1.00000 \nonumber\\
of_now & 1.00000 \nonumber\\
will_( & 1.00000 \nonumber\\
seven_vote & 1.00000 \nonumber\\
(_as & 1.00000 \nonumber\\
)_seven & 1.00000 \nonumber\\
but_no & 1.00000 \nonumber\\
ProductionRule_S->``,NP,VP,'', & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,PRN, & 1.00000 \nonumber\\
it_tell & 1.00000 \nonumber\\
say_why & 1.00000 \nonumber\\
also_find & 1.00000 \nonumber\\
'_( & 1.00000 \nonumber\\
)_to & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,ADJP,PRN, & 1.00000 \nonumber\\
bid_to & 1.00000 \nonumber\\
government_to & 1.00000 \nonumber\\
marry_to & 1.00000 \nonumber\\
._firefox & 1.00000 \nonumber\\
free_with & 1.00000 \nonumber\\
ProductionRule_S->S,,,CC,SINV,., & 1.00000 \nonumber\\
about_a & 1.00000 \nonumber\\
ProductionRule_NP->VBG,NN, & 1.00000 \nonumber\\
"_may & 1.00000 \nonumber\\
n't_religious & 1.00000 \nonumber\\
to_specific & 1.00000 \nonumber\\
but_everyone & 1.00000 \nonumber\\
or_adhere & 1.00000 \nonumber\\
standpoint_gay & 1.00000 \nonumber\\
different_matter & 1.00000 \nonumber\\
misuse & 1.00000 \nonumber\\
guidance_. & 1.00000 \nonumber\\
be_misuse & 1.00000 \nonumber\\
guidance & 1.00000 \nonumber\\
well_that & 1.00000 \nonumber\\
religious_or & 1.00000 \nonumber\\
define_as & 1.00000 \nonumber\\
as_between & 1.00000 \nonumber\\
religious_standpoint & 1.00000 \nonumber\\
specific_religious & 1.00000 \nonumber\\
let_along & 1.00000 \nonumber\\
religious_guidance & 1.00000 \nonumber\\
even_possible & 1.00000 \nonumber\\
along_right & 1.00000 \nonumber\\
misuse_in & 1.00000 \nonumber\\
be_define & 1.00000 \nonumber\\
stylesheet & 1.00000 \nonumber\\
n't_dig & 1.00000 \nonumber\\
stylesheet_for & 1.00000 \nonumber\\
separate_stylesheet & 1.00000 \nonumber\\
suck_and & 1.00000 \nonumber\\
harder_, & 1.00000 \nonumber\\
ProductionRule_NP->NP,ADJP,,,SBAR, & 1.00000 \nonumber\\
do_separate & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,CC,VBZ,NP, & 1.00000 \nonumber\\
make_development & 1.00000 \nonumber\\
development_harder & 1.00000 \nonumber\\
ie_suck & 1.00000 \nonumber\\
dig_do & 1.00000 \nonumber\\
food_. & 1.00000 \nonumber\\
weird_and & 1.00000 \nonumber\\
limit_for & 1.00000 \nonumber\\
discipline_but & 1.00000 \nonumber\\
everything_so & 1.00000 \nonumber\\
it_every & 1.00000 \nonumber\\
something_wrong & 1.00000 \nonumber\\
ProductionRule_ADJP->NP,RB, & 1.00000 \nonumber\\
where_would & 1.00000 \nonumber\\
more_responsibility & 1.00000 \nonumber\\
on_mankind & 1.00000 \nonumber\\
place_on & 1.00000 \nonumber\\
the_21 & 1.00000 \nonumber\\
21 & 1.00000 \nonumber\\
responsibility_place & 1.00000 \nonumber\\
century_, & 1.00000 \nonumber\\
._creation & 1.00000 \nonumber\\
st & 1.00000 \nonumber\\
st_century & 1.00000 \nonumber\\
21_' & 1.00000 \nonumber\\
to_evolve & 1.00000 \nonumber\\
'_st & 1.00000 \nonumber\\
evolve_be & 1.00000 \nonumber\\
with_more & 1.00000 \nonumber\\
just_with & 1.00000 \nonumber\\
_pos_ngram_CARD_O_PP & 1.00000 \nonumber\\
evolution_just & 1.00000 \nonumber\\
be_or & 1.00000 \nonumber\\
when_help & 1.00000 \nonumber\\
time_have & 1.00000 \nonumber\\
that_tv & 1.00000 \nonumber\\
to_click & 1.00000 \nonumber\\
ProductionRule_FRAG->NP,PP,., & 1.00000 \nonumber\\
right_hand & 1.00000 \nonumber\\
"_link & 1.00000 \nonumber\\
you_seem & 1.00000 \nonumber\\
hand_side & 1.00000 \nonumber\\
"_convince & 1.00000 \nonumber\\
click_this & 1.00000 \nonumber\\
convince_me & 1.00000 \nonumber\\
note_to & 1.00000 \nonumber\\
click_anything & 1.00000 \nonumber\\
everything_on & 1.00000 \nonumber\\
that_creationism & 1.00000 \nonumber\\
_pos_ngram_O_ADJ_PR & 1.00000 \nonumber\\
a_note & 1.00000 \nonumber\\
you_win & 1.00000 \nonumber\\
argument_convince & 1.00000 \nonumber\\
please_use & 1.00000 \nonumber\\
link_correctly & 1.00000 \nonumber\\
this_if & 1.00000 \nonumber\\
debate_by & 1.00000 \nonumber\\
be_click & 1.00000 \nonumber\\
_pos_ngram_ADJ_PR_NN & 1.00000 \nonumber\\
well_personally & 1.00000 \nonumber\\
it_... & 1.00000 \nonumber\\
fall_asleep & 1.00000 \nonumber\\
uno & 1.00000 \nonumber\\
card_. & 1.00000 \nonumber\\
asleep_. & 1.00000 \nonumber\\
asleep & 1.00000 \nonumber\\
uno_card & 1.00000 \nonumber\\
card & 1.00000 \nonumber\\
1995_world & 1.00000 \nonumber\\
sheep_count & 1.00000 \nonumber\\
1995 & 1.00000 \nonumber\\
poker & 1.00000 \nonumber\\
sheep & 1.00000 \nonumber\\
use_uno & 1.00000 \nonumber\\
count_him & 1.00000 \nonumber\\
world_series & 1.00000 \nonumber\\
poker_use & 1.00000 \nonumber\\
of_poker & 1.00000 \nonumber\\
he_win & 1.00000 \nonumber\\
the_1995 & 1.00000 \nonumber\\
testament_i & 1.00000 \nonumber\\
_pos_ngram_ADV_ADJ_NP & 1.00000 \nonumber\\
christianity_so & 1.00000 \nonumber\\
testament & 1.00000 \nonumber\\
than_your & 1.00000 \nonumber\\
refer_to & 1.00000 \nonumber\\
refer & 1.00000 \nonumber\\
history_with & 1.00000 \nonumber\\
of_more & 1.00000 \nonumber\\
account_be & 1.00000 \nonumber\\
ProductionRule_VP->VBN,PP,ADVP,PP, & 1.00000 \nonumber\\
in_existance & 1.00000 \nonumber\\
be_refer & 1.00000 \nonumber\\
in_existence & 1.00000 \nonumber\\
old_testament & 1.00000 \nonumber\\
biblical_account & 1.00000 \nonumber\\
write_of & 1.00000 \nonumber\\
recent_christianity & 1.00000 \nonumber\\
ProductionRule_NP->ADJP,NNP, & 1.00000 \nonumber\\
which_have & 1.00000 \nonumber\\
much_longer & 1.00000 \nonumber\\
the_biblical & 1.00000 \nonumber\\
your_note & 1.00000 \nonumber\\
existance_much & 1.00000 \nonumber\\
the_write & 1.00000 \nonumber\\
existance & 1.00000 \nonumber\\
existence_since & 1.00000 \nonumber\\
gym & 1.00000 \nonumber\\
raffle_see & 1.00000 \nonumber\\
clothe_be & 1.00000 \nonumber\\
scar_them & 1.00000 \nonumber\\
could_mentally & 1.00000 \nonumber\\
think_hit & 1.00000 \nonumber\\
hit_their & 1.00000 \nonumber\\
because_hit & 1.00000 \nonumber\\
mentally_scar & 1.00000 \nonumber\\
alright_. & 1.00000 \nonumber\\
hit_your & 1.00000 \nonumber\\
the_father & 1.00000 \nonumber\\
tell_other & 1.00000 \nonumber\\
couse & 1.00000 \nonumber\\
can_couse & 1.00000 \nonumber\\
gay_marrage & 1.00000 \nonumber\\
marrage_can & 1.00000 \nonumber\\
and_sucy & 1.00000 \nonumber\\
marrage_have & 1.00000 \nonumber\\
people_life & 1.00000 \nonumber\\
extrem & 1.00000 \nonumber\\
extrem_case & 1.00000 \nonumber\\
contriverse_, & 1.00000 \nonumber\\
pepole & 1.00000 \nonumber\\
couse_a & 1.00000 \nonumber\\
much_trouble & 1.00000 \nonumber\\
of_contriverse & 1.00000 \nonumber\\
pepole_have & 1.00000 \nonumber\\
have_result & 1.00000 \nonumber\\
cause_so & 1.00000 \nonumber\\
in_extrem & 1.00000 \nonumber\\
in_murder & 1.00000 \nonumber\\
contriverse & 1.00000 \nonumber\\
put_people & 1.00000 \nonumber\\
risk_in & 1.00000 \nonumber\\
sex_marrage & 1.00000 \nonumber\\
at_risk & 1.00000 \nonumber\\
it_put & 1.00000 \nonumber\\
trouble_pepole & 1.00000 \nonumber\\
trade & 1.00000 \nonumber\\
their_love & 1.00000 \nonumber\\
love_one & 1.00000 \nonumber\\
._love & 1.00000 \nonumber\\
both_moth & 1.00000 \nonumber\\
situation_of & 1.00000 \nonumber\\
,_have & 1.00000 \nonumber\\
leadership & 1.00000 \nonumber\\
learn_good & 1.00000 \nonumber\\
also_lead & 1.00000 \nonumber\\
this_could & 1.00000 \nonumber\\
kid_learn & 1.00000 \nonumber\\
not_push & 1.00000 \nonumber\\
and_discipline & 1.00000 \nonumber\\
activity_. & 1.00000 \nonumber\\
leadership_and & 1.00000 \nonumber\\
that_kid & 1.00000 \nonumber\\
home_to & 1.00000 \nonumber\\
discipline_. & 1.00000 \nonumber\\
quality_like & 1.00000 \nonumber\\
any_physical & 1.00000 \nonumber\\
like_leadership & 1.00000 \nonumber\\
push_in & 1.00000 \nonumber\\
good_quality & 1.00000 \nonumber\\
help_childhood & 1.00000 \nonumber\\
abstract_noun & 1.00000 \nonumber\\
noun & 1.00000 \nonumber\\
noun_, & 1.00000 \nonumber\\
to_proper & 1.00000 \nonumber\\
express_emotion & 1.00000 \nonumber\\
emotion_be & 1.00000 \nonumber\\
school_code & 1.00000 \nonumber\\
proper_school & 1.00000 \nonumber\\
necessary_as & 1.00000 \nonumber\\
follow_to & 1.00000 \nonumber\\
right_but & 1.00000 \nonumber\\
come_school & 1.00000 \nonumber\\
ProductionRule_ADJP->JJ,CC,RB,JJ, & 1.00000 \nonumber\\
code_and & 1.00000 \nonumber\\
what_not & 1.00000 \nonumber\\
of_thing & 1.00000 \nonumber\\
have_. & 1.00000 \nonumber\\
hold_accountable & 1.00000 \nonumber\\
otherwise_people & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,PRT,S, & 1.00000 \nonumber\\
lazy_or & 1.00000 \nonumber\\
kill_baby & 1.00000 \nonumber\\
ignorant_to & 1.00000 \nonumber\\
irresponsible_and & 1.00000 \nonumber\\
or_ignorant & 1.00000 \nonumber\\
accountable & 1.00000 \nonumber\\
abuse_their & 1.00000 \nonumber\\
them_up & 1.00000 \nonumber\\
their_power & 1.00000 \nonumber\\
accountable_for & 1.00000 \nonumber\\
up_pregnant & 1.00000 \nonumber\\
lose_in & 1.00000 \nonumber\\
but_because & 1.00000 \nonumber\\
red_coat & 1.00000 \nonumber\\
red_dot & 1.00000 \nonumber\\
yell_, & 1.00000 \nonumber\\
red_uniform & 1.00000 \nonumber\\
take_over & 1.00000 \nonumber\\
if_indium & 1.00000 \nonumber\\
to_yell & 1.00000 \nonumber\\
the_brit & 1.00000 \nonumber\\
british_soldier & 1.00000 \nonumber\\
brit_wear & 1.00000 \nonumber\\
come_, & 1.00000 \nonumber\\
brit_for & 1.00000 \nonumber\\
american_see & 1.00000 \nonumber\\
brit & 1.00000 \nonumber\\
the_red & 1.00000 \nonumber\\
coat_be & 1.00000 \nonumber\\
would_yell & 1.00000 \nonumber\\
american_would & 1.00000 \nonumber\\
fight_the & 1.00000 \nonumber\\
,_american & 1.00000 \nonumber\\
u.s._fight & 1.00000 \nonumber\\
indium_ever & 1.00000 \nonumber\\
ever_try & 1.00000 \nonumber\\
dot_be & 1.00000 \nonumber\\
dot & 1.00000 \nonumber\\
their_independence & 1.00000 \nonumber\\
independence_, & 1.00000 \nonumber\\
as_yourself & 1.00000 \nonumber\\
he_leave & 1.00000 \nonumber\\
because_those & 1.00000 \nonumber\\
other_side & 1.00000 \nonumber\\
from_tv & 1.00000 \nonumber\\
while_information & 1.00000 \nonumber\\
more_convenient & 1.00000 \nonumber\\
and_useful & 1.00000 \nonumber\\
certain_topic & 1.00000 \nonumber\\
update_with & 1.00000 \nonumber\\
who_can & 1.00000 \nonumber\\
program_on & 1.00000 \nonumber\\
accurate_and & 1.00000 \nonumber\\
topic_while & 1.00000 \nonumber\\
latest_information & 1.00000 \nonumber\\
information_about & 1.00000 \nonumber\\
educational_program & 1.00000 \nonumber\\
more_accurate & 1.00000 \nonumber\\
see_or & 1.00000 \nonumber\\
not_update & 1.00000 \nonumber\\
hear_. & 1.00000 \nonumber\\
also_likely & 1.00000 \nonumber\\
also_easy & 1.00000 \nonumber\\
with_latest & 1.00000 \nonumber\\
the_educational & 1.00000 \nonumber\\
convenient_and & 1.00000 \nonumber\\
useful_. & 1.00000 \nonumber\\
among_pupil & 1.00000 \nonumber\\
change_the & 1.00000 \nonumber\\
time_the & 1.00000 \nonumber\\
so-call_operation & 1.00000 \nonumber\\
raffle_practically & 1.00000 \nonumber\\
'_grand & 1.00000 \nonumber\\
faruhar & 1.00000 \nonumber\\
plan_' & 1.00000 \nonumber\\
grand & 1.00000 \nonumber\\
all_go & 1.00000 \nonumber\\
grand_plan & 1.00000 \nonumber\\
lift_a & 1.00000 \nonumber\\
sit_there & 1.00000 \nonumber\\
practically_just & 1.00000 \nonumber\\
faruhar_carry & 1.00000 \nonumber\\
lift & 1.00000 \nonumber\\
of_raffle & 1.00000 \nonumber\\
a_finger & 1.00000 \nonumber\\
even_lift & 1.00000 \nonumber\\
head_of & 1.00000 \nonumber\\
finger_to & 1.00000 \nonumber\\
if_raffle & 1.00000 \nonumber\\
be_here & 1.00000 \nonumber\\
_pos_ngram_O_O_CARD & 1.00000 \nonumber\\
break_your & 1.00000 \nonumber\\
physiatrist & 1.00000 \nonumber\\
that_expirience & 1.00000 \nonumber\\
you_one & 1.00000 \nonumber\\
thing_!!!! & 1.00000 \nonumber\\
about_rape & 1.00000 \nonumber\\
hand_or & 1.00000 \nonumber\\
a_physiatrist & 1.00000 \nonumber\\
you_cut & 1.00000 \nonumber\\
your_actualy & 1.00000 \nonumber\\
_pos_ngram_ART_CONJ_PP & 1.00000 \nonumber\\
up_break & 1.00000 \nonumber\\
would_remind & 1.00000 \nonumber\\
huge_fight & 1.00000 \nonumber\\
it_off & 1.00000 \nonumber\\
get_in & 1.00000 \nonumber\\
this_subject & 1.00000 \nonumber\\
_pos_ngram_PR_ADV_NP & 1.00000 \nonumber\\
arm_... & 1.00000 \nonumber\\
fight_with & 1.00000 \nonumber\\
for_everyone & 1.00000 \nonumber\\
sane_you & 1.00000 \nonumber\\
sane & 1.00000 \nonumber\\
me_ask & 1.00000 \nonumber\\
yes_you & 1.00000 \nonumber\\
or_arm & 1.00000 \nonumber\\
expirience & 1.00000 \nonumber\\
actualy_sane & 1.00000 \nonumber\\
off_just & 1.00000 \nonumber\\
physiatrist_!!!! & 1.00000 \nonumber\\
cut_it & 1.00000 \nonumber\\
subject_let & 1.00000 \nonumber\\
???_if & 1.00000 \nonumber\\
ProductionRule_VP->VBG,PP,PP, & 1.00000 \nonumber\\
actualy & 1.00000 \nonumber\\
expirience_??? & 1.00000 \nonumber\\
!!!!_if & 1.00000 \nonumber\\
rape_in & 1.00000 \nonumber\\
will_receive & 1.00000 \nonumber\\
they_where & 1.00000 \nonumber\\
receive_consequence & 1.00000 \nonumber\\
where_wrong & 1.00000 \nonumber\\
must_understand & 1.00000 \nonumber\\
agree_because & 1.00000 \nonumber\\
ProductionRule_NP->NP,FRAG, & 1.00000 \nonumber\\
than_him & 1.00000 \nonumber\\
would_alway & 1.00000 \nonumber\\
of_business & 1.00000 \nonumber\\
faster_because & 1.00000 \nonumber\\
still_happy & 1.00000 \nonumber\\
start_be & 1.00000 \nonumber\\
imagine_wonder & 1.00000 \nonumber\\
alway_have & 1.00000 \nonumber\\
empty_void & 1.00000 \nonumber\\
responsible_faster & 1.00000 \nonumber\\
also_cause & 1.00000 \nonumber\\
lousy_it & 1.00000 \nonumber\\
void_feel & 1.00000 \nonumber\\
a_have & 1.00000 \nonumber\\
cant_imagine & 1.00000 \nonumber\\
void & 1.00000 \nonumber\\
out_a & 1.00000 \nonumber\\
that_empty & 1.00000 \nonumber\\
empty & 1.00000 \nonumber\\
cause_you & 1.00000 \nonumber\\
happy_i & 1.00000 \nonumber\\
_pos_ngram_CONJ_V_PUNC & 1.00000 \nonumber\\
sex_will & 1.00000 \nonumber\\
disease_especially & 1.00000 \nonumber\\
sex_... & 1.00000 \nonumber\\
in_morallity & 1.00000 \nonumber\\
free_sex & 1.00000 \nonumber\\
a_free & 1.00000 \nonumber\\
hiv & 1.00000 \nonumber\\
..._free & 1.00000 \nonumber\\
especially_hiv & 1.00000 \nonumber\\
will_bring & 1.00000 \nonumber\\
..._in & 1.00000 \nonumber\\
..._we & 1.00000 \nonumber\\
morallity_it & 1.00000 \nonumber\\
morallity & 1.00000 \nonumber\\
hiv_... & 1.00000 \nonumber\\
wrong_... & 1.00000 \nonumber\\
people_watch & 1.00000 \nonumber\\
absolutley & 1.00000 \nonumber\\
all_have & 1.00000 \nonumber\\
convince_you & 1.00000 \nonumber\\
choose_a & 1.00000 \nonumber\\
love_each & 1.00000 \nonumber\\
describe & 1.00000 \nonumber\\
..._that & 1.00000 \nonumber\\
well_they & 1.00000 \nonumber\\
bore_. & 1.00000 \nonumber\\
same_... & 1.00000 \nonumber\\
that_bore & 1.00000 \nonumber\\
down_the & 1.00000 \nonumber\\
be_thousand & 1.00000 \nonumber\\
from_them & 1.00000 \nonumber\\
come_back & 1.00000 \nonumber\\
2_it & 1.00000 \nonumber\\
not_abuse & 1.00000 \nonumber\\
1_get & 1.00000 \nonumber\\
and_2 & 1.00000 \nonumber\\
you_listen & 1.00000 \nonumber\\
ProductionRule_QP->CC,CD, & 1.00000 \nonumber\\
ProductionRule_ADJP->NN,SBAR, & 1.00000 \nonumber\\
'_get & 1.00000 \nonumber\\
because_1 & 1.00000 \nonumber\\
_pos_ngram_CONJ_CARD_PR & 1.00000 \nonumber\\
hit_help & 1.00000 \nonumber\\
_pos_ngram_PP_CONJ_CARD & 1.00000 \nonumber\\
ProductionRule_S->ADVP,,,SBAR,,,NP,VP,., & 1.00000 \nonumber\\
listen_, & 1.00000 \nonumber\\
abuse_it & 1.00000 \nonumber\\
teach_us & 1.00000 \nonumber\\
manufactor & 1.00000 \nonumber\\
outsource & 1.00000 \nonumber\\
have_ptential & 1.00000 \nonumber\\
manufactor_job & 1.00000 \nonumber\\
ProductionRule_VP->VB,S,S, & 1.00000 \nonumber\\
outsource_good & 1.00000 \nonumber\\
china_! & 1.00000 \nonumber\\
ptential_to & 1.00000 \nonumber\\
!_america & 1.00000 \nonumber\\
america_continue & 1.00000 \nonumber\\
to_these & 1.00000 \nonumber\\
economic_boost & 1.00000 \nonumber\\
these_country & 1.00000 \nonumber\\
ProductionRule_SINV->ADVP,VP,NP, & 1.00000 \nonumber\\
boost_for & 1.00000 \nonumber\\
country_result & 1.00000 \nonumber\\
do_china & 1.00000 \nonumber\\
ptential & 1.00000 \nonumber\\
to_outsource & 1.00000 \nonumber\\
good_manufactor & 1.00000 \nonumber\\
teach_child & 1.00000 \nonumber\\
job_in & 1.00000 \nonumber\\
importhant_job & 1.00000 \nonumber\\
by_porn & 1.00000 \nonumber\\
more_importhant & 1.00000 \nonumber\\
importhant & 1.00000 \nonumber\\
feel_degrade & 1.00000 \nonumber\\
morality_police & 1.00000 \nonumber\\
personal_morality & 1.00000 \nonumber\\
unprotect_sex & 1.00000 \nonumber\\
have_unprotect & 1.00000 \nonumber\\
fastest & 1.00000 \nonumber\\
weight_because & 1.00000 \nonumber\\
be_manditory & 1.00000 \nonumber\\
it_definatley & 1.00000 \nonumber\\
they_eat & 1.00000 \nonumber\\
dont_get & 1.00000 \nonumber\\
street_at & 1.00000 \nonumber\\
on_to & 1.00000 \nonumber\\
over_weight & 1.00000 \nonumber\\
play_they & 1.00000 \nonumber\\
eat_to & 1.00000 \nonumber\\
kid_play & 1.00000 \nonumber\\
definatley & 1.00000 \nonumber\\
definatley_should & 1.00000 \nonumber\\
manditory_. & 1.00000 \nonumber\\
get_enough & 1.00000 \nonumber\\
look_on & 1.00000 \nonumber\\
manditory & 1.00000 \nonumber\\
enough_physical & 1.00000 \nonumber\\
likley_over & 1.00000 \nonumber\\
number_of & 1.00000 \nonumber\\
ProductionRule_NP->NN,NN,NN, & 1.00000 \nonumber\\
once_, & 1.00000 \nonumber\\
recognize_on & 1.00000 \nonumber\\
leave_it & 1.00000 \nonumber\\
they_call & 1.00000 \nonumber\\
together_of & 1.00000 \nonumber\\
allow_this & 1.00000 \nonumber\\
sanctity_of & 1.00000 \nonumber\\
a_marry & 1.00000 \nonumber\\
a_violation & 1.00000 \nonumber\\
sanctity & 1.00000 \nonumber\\
same_rights & 1.00000 \nonumber\\
the_come & 1.00000 \nonumber\\
if_call & 1.00000 \nonumber\\
what_marriage & 1.00000 \nonumber\\
an_amendment & 1.00000 \nonumber\\
rights_that & 1.00000 \nonumber\\
it_- & 1.00000 \nonumber\\
it_" & 1.00000 \nonumber\\
amendment_state & 1.00000 \nonumber\\
violation_to & 1.00000 \nonumber\\
be_recognize & 1.00000 \nonumber\\
offend_people & 1.00000 \nonumber\\
or_violate & 1.00000 \nonumber\\
yet_bush & 1.00000 \nonumber\\
court_wo & 1.00000 \nonumber\\
couple_get & 1.00000 \nonumber\\
constitution_and & 1.00000 \nonumber\\
constitution & 1.00000 \nonumber\\
-_gay & 1.00000 \nonumber\\
offend & 1.00000 \nonumber\\
unfortunate_that & 1.00000 \nonumber\\
the_constitution & 1.00000 \nonumber\\
gay_need & 1.00000 \nonumber\\
"_offend & 1.00000 \nonumber\\
soul_, & 1.00000 \nonumber\\
that_level & 1.00000 \nonumber\\
get_. & 1.00000 \nonumber\\
case_on & 1.00000 \nonumber\\
bush_want & 1.00000 \nonumber\\
marry_couple & 1.00000 \nonumber\\
two_soul & 1.00000 \nonumber\\
bush & 1.00000 \nonumber\\
the_sanctity & 1.00000 \nonumber\\
state_what & 1.00000 \nonumber\\
violation & 1.00000 \nonumber\\
violate_what & 1.00000 \nonumber\\
ProductionRule_VP->VB,CC,VB,PP, & 1.00000 \nonumber\\
download_porn & 1.00000 \nonumber\\
ProductionRule_NP->RB,NP,ADVP, & 1.00000 \nonumber\\
unless_it & 1.00000 \nonumber\\
porn_even & 1.00000 \nonumber\\
smoken_hot & 1.00000 \nonumber\\
smoken & 1.00000 \nonumber\\
hot_lesbian & 1.00000 \nonumber\\
fact_i & 1.00000 \nonumber\\
...._unless & 1.00000 \nonumber\\
have_smoken & 1.00000 \nonumber\\
lesbian_in & 1.00000 \nonumber\\
i_type & 1.00000 \nonumber\\
the_oppose & 1.00000 \nonumber\\
class_of & 1.00000 \nonumber\\
coz & 1.00000 \nonumber\\
other_thing & 1.00000 \nonumber\\
farquhar_even & 1.00000 \nonumber\\
even_take & 1.00000 \nonumber\\
to_resolve & 1.00000 \nonumber\\
resolve_certain & 1.00000 \nonumber\\
ProductionRule_VP->VBD,S,PP, & 1.00000 \nonumber\\
certain_issue & 1.00000 \nonumber\\
sorrow & 1.00000 \nonumber\\
resolve & 1.00000 \nonumber\\
leave_, & 1.00000 \nonumber\\
heart_. & 1.00000 \nonumber\\
sorrow_in & 1.00000 \nonumber\\
money_out & 1.00000 \nonumber\\
off_with & 1.00000 \nonumber\\
take_money & 1.00000 \nonumber\\
'_problem & 1.00000 \nonumber\\
recognize_william & 1.00000 \nonumber\\
pocket_to & 1.00000 \nonumber\\
with_sorrow & 1.00000 \nonumber\\
people_send & 1.00000 \nonumber\\
raffle_fail & 1.00000 \nonumber\\
their_heart & 1.00000 \nonumber\\
ProductionRule_NP->NP,NNS,SBAR, & 1.00000 \nonumber\\
else_, & 1.00000 \nonumber\\
education_than & 1.00000 \nonumber\\
ProductionRule_NP->DT,``,NNP,NNP,'',NN, & 1.00000 \nonumber\\
where_ever & 1.00000 \nonumber\\
ipad_so & 1.00000 \nonumber\\
foxtel & 1.00000 \nonumber\\
"_app & 1.00000 \nonumber\\
your_ipad & 1.00000 \nonumber\\
"_foxtel & 1.00000 \nonumber\\
app_on & 1.00000 \nonumber\\
ever_and & 1.00000 \nonumber\\
whenever_you & 1.00000 \nonumber\\
tv_where & 1.00000 \nonumber\\
ipad & 1.00000 \nonumber\\
foxtel_go & 1.00000 \nonumber\\
go_" & 1.00000 \nonumber\\
and_whenever & 1.00000 \nonumber\\
manmohan_singh & 1.00000 \nonumber\\
prove_its & 1.00000 \nonumber\\
manmohan & 1.00000 \nonumber\\
surely_have & 1.00000 \nonumber\\
its_potential & 1.00000 \nonumber\\
...._indium & 1.00000 \nonumber\\
dr_manmohan & 1.00000 \nonumber\\
indium_surely & 1.00000 \nonumber\\
singh & 1.00000 \nonumber\\
field_and & 1.00000 \nonumber\\
most_qualify & 1.00000 \nonumber\\
and_aspect & 1.00000 \nonumber\\
in_various & 1.00000 \nonumber\\
minister_all & 1.00000 \nonumber\\
ProductionRule_NP->DT,NN,FW,FW, & 1.00000 \nonumber\\
dr & 1.00000 \nonumber\\
consider_as & 1.00000 \nonumber\\
qualify_prime & 1.00000 \nonumber\\
aspect_..... & 1.00000 \nonumber\\
...._dr & 1.00000 \nonumber\\
various_field & 1.00000 \nonumber\\
singh_be & 1.00000 \nonumber\\
potential_in & 1.00000 \nonumber\\
she_should & 1.00000 \nonumber\\
a_wrong & 1.00000 \nonumber\\
be_faster & 1.00000 \nonumber\\
ProductionRule_S->NP,VP,VP, & 1.00000 \nonumber\\
faster_and & 1.00000 \nonumber\\
obesity_if & 1.00000 \nonumber\\
start_at & 1.00000 \nonumber\\
age_? & 1.00000 \nonumber\\
n't_start & 1.00000 \nonumber\\
we_suppose & 1.00000 \nonumber\\
curb_childhood & 1.00000 \nonumber\\
young_age & 1.00000 \nonumber\\
ProductionRule_VP->VBN,S,SBAR, & 1.00000 \nonumber\\
to_curb & 1.00000 \nonumber\\
way_around & 1.00000 \nonumber\\
ProductionRule_NP->NN,S, & 1.00000 \nonumber\\
people_" & 1.00000 \nonumber\\
_pos_ngram_ADJ_V_ART & 1.00000 \nonumber\\
foundation & 1.00000 \nonumber\\
ProductionRule_VP->VBD,PRT,NP, & 1.00000 \nonumber\\
other_choice & 1.00000 \nonumber\\
uniform_would & 1.00000 \nonumber\\
he_get & 1.00000 \nonumber\\
selection & 1.00000 \nonumber\\
the_creature & 1.00000 \nonumber\\
also_an & 1.00000 \nonumber\\
useful_for & 1.00000 \nonumber\\
._fruit & 1.00000 \nonumber\\
about_because & 1.00000 \nonumber\\
survive_because & 1.00000 \nonumber\\
speciation_be & 1.00000 \nonumber\\
speciation & 1.00000 \nonumber\\
mutation_and & 1.00000 \nonumber\\
the_breed & 1.00000 \nonumber\\
so_quickly & 1.00000 \nonumber\\
mutation_have & 1.00000 \nonumber\\
see_evolution & 1.00000 \nonumber\\
._natural & 1.00000 \nonumber\\
..._different & 1.00000 \nonumber\\
actually_see & 1.00000 \nonumber\\
a_slightly & 1.00000 \nonumber\\
come_about & 1.00000 \nonumber\\
happen_because & 1.00000 \nonumber\\
different_species & 1.00000 \nonumber\\
those_mutation & 1.00000 \nonumber\\
creature_to & 1.00000 \nonumber\\
experiment_since & 1.00000 \nonumber\\
._speciation & 1.00000 \nonumber\\
,_live & 1.00000 \nonumber\\
look_you & 1.00000 \nonumber\\
this_experiment & 1.00000 \nonumber\\
can_actually & 1.00000 \nonumber\\
selection_. & 1.00000 \nonumber\\
slightly & 1.00000 \nonumber\\
survive_then & 1.00000 \nonumber\\
they_survive & 1.00000 \nonumber\\
of_mutation & 1.00000 \nonumber\\
slightly_different & 1.00000 \nonumber\\
quite_useful & 1.00000 \nonumber\\
natural_selection & 1.00000 \nonumber\\
die_so & 1.00000 \nonumber\\
breed_, & 1.00000 \nonumber\\
fly_be & 1.00000 \nonumber\\
often_. & 1.00000 \nonumber\\
the_product & 1.00000 \nonumber\\
stunt & 1.00000 \nonumber\\
to_yourselve & 1.00000 \nonumber\\
overly & 1.00000 \nonumber\\
overly_protective & 1.00000 \nonumber\\
be_overrate & 1.00000 \nonumber\\
,_abuse & 1.00000 \nonumber\\
stunt_. & 1.00000 \nonumber\\
liberal_wakoness & 1.00000 \nonumber\\
protective & 1.00000 \nonumber\\
protective_parent & 1.00000 \nonumber\\
another_" & 1.00000 \nonumber\\
yourselve_, & 1.00000 \nonumber\\
of_overly & 1.00000 \nonumber\\
,_nobody & 1.00000 \nonumber\\
product_of & 1.00000 \nonumber\\
call_attention & 1.00000 \nonumber\\
be_another & 1.00000 \nonumber\\
wakoness_( & 1.00000 \nonumber\\
yourselve & 1.00000 \nonumber\\
"_stunt & 1.00000 \nonumber\\
wakoness & 1.00000 \nonumber\\
or_liberal & 1.00000 \nonumber\\
disease_) & 1.00000 \nonumber\\
gay_would & 1.00000 \nonumber\\
you_gay & 1.00000 \nonumber\\
stop_call & 1.00000 \nonumber\\
overrate_. & 1.00000 \nonumber\\
overrate & 1.00000 \nonumber\\
maybe_he & 1.00000 \nonumber\\
teach_at & 1.00000 \nonumber\\
could_toughen & 1.00000 \nonumber\\
saint_or & 1.00000 \nonumber\\
toughen & 1.00000 \nonumber\\
ProductionRule_QP->JJR,IN,DT,NN, & 1.00000 \nonumber\\
to_treat & 1.00000 \nonumber\\
least_know & 1.00000 \nonumber\\
saint & 1.00000 \nonumber\\
toughen_you & 1.00000 \nonumber\\
will_at & 1.00000 \nonumber\\
how_not & 1.00000 \nonumber\\
treat_your & 1.00000 \nonumber\\
no_teach & 1.00000 \nonumber\\
never_wonder & 1.00000 \nonumber\\
teach_what & 1.00000 \nonumber\\
a_saint & 1.00000 \nonumber\\
you_up & 1.00000 \nonumber\\
sex_and & 1.00000 \nonumber\\
america_. & 1.00000 \nonumber\\
life_! & 1.00000 \nonumber\\
win_the & 1.00000 \nonumber\\
but_put & 1.00000 \nonumber\\
mean_sure & 1.00000 \nonumber\\
"_your & 1.00000 \nonumber\\
just_them & 1.00000 \nonumber\\
not_about & 1.00000 \nonumber\\
_pos_ngram_ADV_PR_CONJ & 1.00000 \nonumber\\
about_just & 1.00000 \nonumber\\
can_worry & 1.00000 \nonumber\\
other_first & 1.00000 \nonumber\\
people_where & 1.00000 \nonumber\\
put_yourself & 1.00000 \nonumber\\
world_" & 1.00000 \nonumber\\
important_person & 1.00000 \nonumber\\
everyone_just & 1.00000 \nonumber\\
later_then & 1.00000 \nonumber\\
yourself_later & 1.00000 \nonumber\\
people_bid & 1.00000 \nonumber\\
farewell_on & 1.00000 \nonumber\\
doings_. & 1.00000 \nonumber\\
the_affection & 1.00000 \nonumber\\
his_doings & 1.00000 \nonumber\\
respect_from & 1.00000 \nonumber\\
doings & 1.00000 \nonumber\\
farewell & 1.00000 \nonumber\\
very_important & 1.00000 \nonumber\\
sack_, & 1.00000 \nonumber\\
him_farewell & 1.00000 \nonumber\\
affection_and & 1.00000 \nonumber\\
bid_him & 1.00000 \nonumber\\
farquhar_win & 1.00000 \nonumber\\
,_thousand & 1.00000 \nonumber\\
create_a & 1.00000 \nonumber\\
,_christ & 1.00000 \nonumber\\
real_or & 1.00000 \nonumber\\
short_of & 1.00000 \nonumber\\
must_really & 1.00000 \nonumber\\
fall_way & 1.00000 \nonumber\\
piss_off & 1.00000 \nonumber\\
off_those & 1.00000 \nonumber\\
really_piss & 1.00000 \nonumber\\
ideology & 1.00000 \nonumber\\
better_example & 1.00000 \nonumber\\
?_nothing & 1.00000 \nonumber\\
ideology_to & 1.00000 \nonumber\\
any_human & 1.00000 \nonumber\\
promote_better & 1.00000 \nonumber\\
way_short & 1.00000 \nonumber\\
of_christ & 1.00000 \nonumber\\
and_ethic & 1.00000 \nonumber\\
human_must & 1.00000 \nonumber\\
._real & 1.00000 \nonumber\\
example_to & 1.00000 \nonumber\\
a_ideology & 1.00000 \nonumber\\
what_harm & 1.00000 \nonumber\\
christ_, & 1.00000 \nonumber\\
that_fall & 1.00000 \nonumber\\
christ_be & 1.00000 \nonumber\\
follow_than & 1.00000 \nonumber\\
ethic_. & 1.00000 \nonumber\\
contribute_? & 1.00000 \nonumber\\
ethic & 1.00000 \nonumber\\
do_atheism & 1.00000 \nonumber\\
ProductionRule_VP->VB,ADJP,NP, & 1.00000 \nonumber\\
harm_be & 1.00000 \nonumber\\
any_atheist & 1.00000 \nonumber\\
better_moral & 1.00000 \nonumber\\
atheism_contribute & 1.00000 \nonumber\\
christianity_strive & 1.00000 \nonumber\\
and_keep & 1.00000 \nonumber\\
or_bid & 1.00000 \nonumber\\
minister_anymore & 1.00000 \nonumber\\
farquer_incharge & 1.00000 \nonumber\\
family_time & 1.00000 \nonumber\\
ntu & 1.00000 \nonumber\\
singapore_for & 1.00000 \nonumber\\
lee & 1.00000 \nonumber\\
lee_hsien & 1.00000 \nonumber\\
imagine_sst & 1.00000 \nonumber\\
neglete_us & 1.00000 \nonumber\\
neglete & 1.00000 \nonumber\\
and_ntu & 1.00000 \nonumber\\
if_lee & 1.00000 \nonumber\\
ann & 1.00000 \nonumber\\
ann_poly & 1.00000 \nonumber\\
another_good & 1.00000 \nonumber\\
example_would & 1.00000 \nonumber\\
anymore_? & 1.00000 \nonumber\\
hsien_lioeng & 1.00000 \nonumber\\
hsien & 1.00000 \nonumber\\
back_take & 1.00000 \nonumber\\
be_back & 1.00000 \nonumber\\
?_he & 1.00000 \nonumber\\
time_would & 1.00000 \nonumber\\
lioeng & 1.00000 \nonumber\\
lioeng_take & 1.00000 \nonumber\\
off_for & 1.00000 \nonumber\\
he_neglete & 1.00000 \nonumber\\
be_neglect & 1.00000 \nonumber\\
leave_farquer & 1.00000 \nonumber\\
imply & 1.00000 \nonumber\\
own_school & 1.00000 \nonumber\\
imply_that & 1.00000 \nonumber\\
incharge_therefore & 1.00000 \nonumber\\
ngee & 1.00000 \nonumber\\
poly_and & 1.00000 \nonumber\\
ngee_ann & 1.00000 \nonumber\\
singapore_? & 1.00000 \nonumber\\
incharge & 1.00000 \nonumber\\
sst_ngee & 1.00000 \nonumber\\
for_family & 1.00000 \nonumber\\
sst & 1.00000 \nonumber\\
poly & 1.00000 \nonumber\\
to_imply & 1.00000 \nonumber\\
consider_the & 1.00000 \nonumber\\
_pos_ngram_CONJ_V_O & 1.00000 \nonumber\\
year_and & 1.00000 \nonumber\\
our_prime & 1.00000 \nonumber\\
now_they & 1.00000 \nonumber\\
ntu_have & 1.00000 \nonumber\\
day_off & 1.00000 \nonumber\\
a_mistake & 1.00000 \nonumber\\
to_woman & 1.00000 \nonumber\\
scene_its & 1.00000 \nonumber\\
its_theyre & 1.00000 \nonumber\\
not_degrade & 1.00000 \nonumber\\
theyre_choice & 1.00000 \nonumber\\
the_actor & 1.00000 \nonumber\\
freedom_of & 1.00000 \nonumber\\
open_about & 1.00000 \nonumber\\
about_sex & 1.00000 \nonumber\\
have_freedom & 1.00000 \nonumber\\
actor_do & 1.00000 \nonumber\\
expression_you & 1.00000 \nonumber\\
the_scene & 1.00000 \nonumber\\
your_talk & 1.00000 \nonumber\\
ProductionRule_VP->VBG,PP,NP, & 1.00000 \nonumber\\
woman_they & 1.00000 \nonumber\\
ProductionRule_S->S,,,CC,IN,S,., & 1.00000 \nonumber\\
they_wan & 1.00000 \nonumber\\
on_scientists.most & 1.00000 \nonumber\\
ProductionRule_NP->JJ,S, & 1.00000 \nonumber\\
world.so_, & 1.00000 \nonumber\\
world.so & 1.00000 \nonumber\\
the_world.so & 1.00000 \nonumber\\
scientists.most & 1.00000 \nonumber\\
employee_in & 1.00000 \nonumber\\
scientists.most_of & 1.00000 \nonumber\\
have_potential & 1.00000 \nonumber\\
country_depend & 1.00000 \nonumber\\
every_country & 1.00000 \nonumber\\
,_many & 1.00000 \nonumber\\
of_employee & 1.00000 \nonumber\\
ProductionRule_PP->VBZ,NP, & 1.00000 \nonumber\\
n't_change & 1.00000 \nonumber\\
have_adapt & 1.00000 \nonumber\\
fruit & 1.00000 \nonumber\\
fruit_fly & 1.00000 \nonumber\\
he_or & 1.00000 \nonumber\\
and_choice & 1.00000 \nonumber\\
_pos_ngram_PR_PR_CONJ & 1.00000 \nonumber\\
let_that & 1.00000 \nonumber\\
about_gay & 1.00000 \nonumber\\
she_please & 1.00000 \nonumber\\
free_to & 1.00000 \nonumber\\
way_frown & 1.00000 \nonumber\\
myself_but & 1.00000 \nonumber\\
frown & 1.00000 \nonumber\\
frown_upon & 1.00000 \nonumber\\
thought_, & 1.00000 \nonumber\\
ProductionRule_NP->PRP,CC,PRP, & 1.00000 \nonumber\\
care_much & 1.00000 \nonumber\\
that_influence & 1.00000 \nonumber\\
go_ahead & 1.00000 \nonumber\\
upon_, & 1.00000 \nonumber\\
religion_it & 1.00000 \nonumber\\
upon_it & 1.00000 \nonumber\\
_pos_ngram_CONJ_O_PP & 1.00000 \nonumber\\
but_dont & 1.00000 \nonumber\\
influence_your & 1.00000 \nonumber\\
big_difference & 1.00000 \nonumber\\
it_myself & 1.00000 \nonumber\\
ahead_, & 1.00000 \nonumber\\
be_frown & 1.00000 \nonumber\\
some_religion & 1.00000 \nonumber\\
person_should & 1.00000 \nonumber\\
way_wrong & 1.00000 \nonumber\\
but_for & 1.00000 \nonumber\\
me_if & 1.00000 \nonumber\\
female_who & 1.00000 \nonumber\\
my_boyfriend & 1.00000 \nonumber\\
porn_can & 1.00000 \nonumber\\
no_wrong & 1.00000 \nonumber\\
natural_for & 1.00000 \nonumber\\
love_porn & 1.00000 \nonumber\\
boyfriend_watch & 1.00000 \nonumber\\
the_video & 1.00000 \nonumber\\
its_natural & 1.00000 \nonumber\\
video_they & 1.00000 \nonumber\\
a_female & 1.00000 \nonumber\\
see_no & 1.00000 \nonumber\\
not_bother & 1.00000 \nonumber\\
uncomfortable_with & 1.00000 \nonumber\\
beside_spank & 1.00000 \nonumber\\
option_beside & 1.00000 \nonumber\\
ProductionRule_NP->NP,NN,PP, & 1.00000 \nonumber\\
may_get & 1.00000 \nonumber\\
affect_a & 1.00000 \nonumber\\
get_depress & 1.00000 \nonumber\\
try_a & 1.00000 \nonumber\\
different_option & 1.00000 \nonumber\\
can_affect & 1.00000 \nonumber\\
'_way & 1.00000 \nonumber\\
_pos_ngram_V_O_CARD & 1.00000 \nonumber\\
least_the & 1.00000 \nonumber\\
virtualearth_. & 1.00000 \nonumber\\
aside_, & 1.00000 \nonumber\\
virtualearth & 1.00000 \nonumber\\
window_virtualearth & 1.00000 \nonumber\\
new_wonder & 1.00000 \nonumber\\
it_unusable & 1.00000 \nonumber\\
write_this & 1.00000 \nonumber\\
unusable_for & 1.00000 \nonumber\\
emotion_aside & 1.00000 \nonumber\\
unusable & 1.00000 \nonumber\\
support_. & 1.00000 \nonumber\\
firefox_) & 1.00000 \nonumber\\
wonder_tool & 1.00000 \nonumber\\
activex_support & 1.00000 \nonumber\\
)_emotion & 1.00000 \nonumber\\
ProductionRule_SBAR->PRN,S, & 1.00000 \nonumber\\
through_firefox & 1.00000 \nonumber\\
tool_, & 1.00000 \nonumber\\
this_through & 1.00000 \nonumber\\
,_window & 1.00000 \nonumber\\
no_activex & 1.00000 \nonumber\\
worse_since & 1.00000 \nonumber\\
and/or_the & 1.00000 \nonumber\\
hide_be & 1.00000 \nonumber\\
a_lawful & 1.00000 \nonumber\\
ProductionRule_NP->DT,JJ,,,JJ,NN, & 1.00000 \nonumber\\
._hopefully & 1.00000 \nonumber\\
be_lenient & 1.00000 \nonumber\\
but_nonetheless & 1.00000 \nonumber\\
nonetheless & 1.00000 \nonumber\\
murder_would & 1.00000 \nonumber\\
guilt_and/or & 1.00000 \nonumber\\
prison_except & 1.00000 \nonumber\\
the_sentence & 1.00000 \nonumber\\
harsh & 1.00000 \nonumber\\
harsh_, & 1.00000 \nonumber\\
all_murderer & 1.00000 \nonumber\\
chance_for & 1.00000 \nonumber\\
parole_since & 1.00000 \nonumber\\
parole & 1.00000 \nonumber\\
ProductionRule_NP->DT,JJ,,,JJ,,,NN,NN, & 1.00000 \nonumber\\
much_worse & 1.00000 \nonumber\\
with_any & 1.00000 \nonumber\\
little_chance & 1.00000 \nonumber\\
basically_the & 1.00000 \nonumber\\
spouse_will & 1.00000 \nonumber\\
,_young & 1.00000 \nonumber\\
young_person & 1.00000 \nonumber\\
pleasure/malicious-kill_, & 1.00000 \nonumber\\
pleasure/malicious-kill & 1.00000 \nonumber\\
any_murderer & 1.00000 \nonumber\\
result_of & 1.00000 \nonumber\\
,_hopefully & 1.00000 \nonumber\\
,_homicide & 1.00000 \nonumber\\
an_ambitious & 1.00000 \nonumber\\
a_pleasure/malicious-kill & 1.00000 \nonumber\\
ambitious_, & 1.00000 \nonumber\\
detective & 1.00000 \nonumber\\
midst & 1.00000 \nonumber\\
midst_. & 1.00000 \nonumber\\
since_there & 1.00000 \nonumber\\
lenient_with & 1.00000 \nonumber\\
person_want & 1.00000 \nonumber\\
lenient & 1.00000 \nonumber\\
murderer_must & 1.00000 \nonumber\\
murderer_in & 1.00000 \nonumber\\
successful_, & 1.00000 \nonumber\\
detective_, & 1.00000 \nonumber\\
ambitious & 1.00000 \nonumber\\
nonetheless_, & 1.00000 \nonumber\\
hopefully_, & 1.00000 \nonumber\\
lawful & 1.00000 \nonumber\\
homicide_detective & 1.00000 \nonumber\\
as_harsh & 1.00000 \nonumber\\
hopefully_my & 1.00000 \nonumber\\
my_midst & 1.00000 \nonumber\\
for_parole & 1.00000 \nonumber\\
homicide & 1.00000 \nonumber\\
,_successful & 1.00000 \nonumber\\
except_much & 1.00000 \nonumber\\
in_hide & 1.00000 \nonumber\\
sentence_wo & 1.00000 \nonumber\\
the_result & 1.00000 \nonumber\\
lawful_, & 1.00000 \nonumber\\
and_one & 1.00000 \nonumber\\
efficient_. & 1.00000 \nonumber\\
rebel & 1.00000 \nonumber\\
wear_inappropriate & 1.00000 \nonumber\\
rebel_jeans & 1.00000 \nonumber\\
oh_please & 1.00000 \nonumber\\
inappropriate_clothe & 1.00000 \nonumber\\
we_let & 1.00000 \nonumber\\
if_other & 1.00000 \nonumber\\
hot_pants & 1.00000 \nonumber\\
pants_, & 1.00000 \nonumber\\
indirectly_give & 1.00000 \nonumber\\
as_hot & 1.00000 \nonumber\\
jeans_or & 1.00000 \nonumber\\
inappropriate & 1.00000 \nonumber\\
study_so & 1.00000 \nonumber\\
would_they & 1.00000 \nonumber\\
dress_correctly & 1.00000 \nonumber\\
dress_theirself & 1.00000 \nonumber\\
or_sexy & 1.00000 \nonumber\\
sexy_clothe & 1.00000 \nonumber\\
theirself_, & 1.00000 \nonumber\\
uniform_indirectly & 1.00000 \nonumber\\
clothe_such & 1.00000 \nonumber\\
their_study & 1.00000 \nonumber\\
think_how & 1.00000 \nonumber\\
them_dress & 1.00000 \nonumber\\
could_wear & 1.00000 \nonumber\\
sexy & 1.00000 \nonumber\\
what_would & 1.00000 \nonumber\\
many_thing & 1.00000 \nonumber\\
other_say & 1.00000 \nonumber\\
to_dress & 1.00000 \nonumber\\
more_efficient & 1.00000 \nonumber\\
more_concentrate & 1.00000 \nonumber\\
give_think & 1.00000 \nonumber\\
,_oh & 1.00000 \nonumber\\
concentrate_with & 1.00000 \nonumber\\
,_rebel & 1.00000 \nonumber\\
theirself & 1.00000 \nonumber\\
pretty_lousy & 1.00000 \nonumber\\
she_' & 1.00000 \nonumber\\
you_question & 1.00000 \nonumber\\
evolutionist & 1.00000 \nonumber\\
or_order & 1.00000 \nonumber\\
about_by & 1.00000 \nonumber\\
awe & 1.00000 \nonumber\\
highly_organize & 1.00000 \nonumber\\
evolutionist_need & 1.00000 \nonumber\\
awe_of & 1.00000 \nonumber\\
faith_than & 1.00000 \nonumber\\
complex_than & 1.00000 \nonumber\\
computer_do & 1.00000 \nonumber\\
?_evolutionist & 1.00000 \nonumber\\
tiny_cell & 1.00000 \nonumber\\
circumstance_? & 1.00000 \nonumber\\
more_faith & 1.00000 \nonumber\\
more_complex & 1.00000 \nonumber\\
design_that & 1.00000 \nonumber\\
nurse & 1.00000 \nonumber\\
miracle_of & 1.00000 \nonumber\\
every_tiny & 1.00000 \nonumber\\
miracle & 1.00000 \nonumber\\
machine_come & 1.00000 \nonumber\\
biology_, & 1.00000 \nonumber\\
biology & 1.00000 \nonumber\\
study_biology & 1.00000 \nonumber\\
nurse_and & 1.00000 \nonumber\\
a_nurse & 1.00000 \nonumber\\
this_highly & 1.00000 \nonumber\\
of_circumstance & 1.00000 \nonumber\\
mere_accident & 1.00000 \nonumber\\
than_creationist & 1.00000 \nonumber\\
more_i & 1.00000 \nonumber\\
the_miracle & 1.00000 \nonumber\\
creator_? & 1.00000 \nonumber\\
i_study & 1.00000 \nonumber\\
'_own & 1.00000 \nonumber\\
cell_have & 1.00000 \nonumber\\
ProductionRule_S->SBAR,,,X,NP,VP, & 1.00000 \nonumber\\
in_awe & 1.00000 \nonumber\\
a_computer & 1.00000 \nonumber\\
organize_machine & 1.00000 \nonumber\\
own_design & 1.00000 \nonumber\\
could_be & 1.00000 \nonumber\\
they_take & 1.00000 \nonumber\\
dont_recycle & 1.00000 \nonumber\\
american_on & 1.00000 \nonumber\\
do_! & 1.00000 \nonumber\\
there_bottle & 1.00000 \nonumber\\
than_half & 1.00000 \nonumber\\
average_recycle & 1.00000 \nonumber\\
so_stop & 1.00000 \nonumber\\
recycle_because & 1.00000 \nonumber\\
stop_complain & 1.00000 \nonumber\\
recycle_86-88 & 1.00000 \nonumber\\
on_average & 1.00000 \nonumber\\
complain & 1.00000 \nonumber\\
86-88_% & 1.00000 \nonumber\\
half_! & 1.00000 \nonumber\\
complain_that & 1.00000 \nonumber\\
86-88 & 1.00000 \nonumber\\
!_http://www.treehugger.com/culture/23-percent-of-americans-donatmt-recycle.html & 1.00000 \nonumber\\
manners & 1.00000 \nonumber\\
way.our & 1.00000 \nonumber\\
aim_be & 1.00000 \nonumber\\
_pos_ngram_PUNC_ART_CONJ & 1.00000 \nonumber\\
aim & 1.00000 \nonumber\\
only_aim & 1.00000 \nonumber\\
manners_and & 1.00000 \nonumber\\
any_way.our & 1.00000 \nonumber\\
and_civilization & 1.00000 \nonumber\\
way.our_manners & 1.00000 \nonumber\\
and_reduce & 1.00000 \nonumber\\
fully_fill & 1.00000 \nonumber\\
his_only & 1.00000 \nonumber\\
fully & 1.00000 \nonumber\\
with_corruption & 1.00000 \nonumber\\
reduce_and & 1.00000 \nonumber\\
reduce_every & 1.00000 \nonumber\\
be_reduce & 1.00000 \nonumber\\
money_in & 1.00000 \nonumber\\
civilization & 1.00000 \nonumber\\
corruption_. & 1.00000 \nonumber\\
be_fully & 1.00000 \nonumber\\
civilization_be & 1.00000 \nonumber\\
avid_christian & 1.00000 \nonumber\\
on_christian & 1.00000 \nonumber\\
be_found & 1.00000 \nonumber\\
should_adhere & 1.00000 \nonumber\\
beyond_belief & 1.00000 \nonumber\\
belif & 1.00000 \nonumber\\
belief_, & 1.00000 \nonumber\\
christian_belief & 1.00000 \nonumber\\
the_belif & 1.00000 \nonumber\\
found_on & 1.00000 \nonumber\\
wrong_beyond & 1.00000 \nonumber\\
belif_use & 1.00000 \nonumber\\
_pos_ngram_ART_V_O & 1.00000 \nonumber\\
valid & 1.00000 \nonumber\\
proof_for & 1.00000 \nonumber\\
valid_proof & 1.00000 \nonumber\\
that_that & 1.00000 \nonumber\\
no_valid & 1.00000 \nonumber\\
a_valid & 1.00000 \nonumber\\
ProductionRule_ADJP->JJ,CC,RB, & 1.00000 \nonumber\\
dont_care & 1.00000 \nonumber\\
practically & 1.00000 \nonumber\\
thin & 1.00000 \nonumber\\
and_thin & 1.00000 \nonumber\\
thick_and & 1.00000 \nonumber\\
that_never & 1.00000 \nonumber\\
give_prime & 1.00000 \nonumber\\
porn_not & 1.00000 \nonumber\\
only_teach & 1.00000 \nonumber\\
also_give & 1.00000 \nonumber\\
never_give & 1.00000 \nonumber\\
demonstration_because & 1.00000 \nonumber\\
demonstration & 1.00000 \nonumber\\
accurate_demonstration & 1.00000 \nonumber\\
an_accurate & 1.00000 \nonumber\\
prime_example & 1.00000 \nonumber\\
listen_porn & 1.00000 \nonumber\\
because_to & 1.00000 \nonumber\\
to_listen & 1.00000 \nonumber\\
imagine_your & 1.00000 \nonumber\\
be_whatever & 1.00000 \nonumber\\
me_a & 1.00000 \nonumber\\
to_agree & 1.00000 \nonumber\\
_pos_ngram_ADV_CONJ_PUNC & 1.00000 \nonumber\\
_pos_ngram_V_CONJ_PUNC & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,ADVP,ADVP,S, & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,ADVP,ADVP,SBAR, & 1.00000 \nonumber\\
eye_can & 1.00000 \nonumber\\
alot_if & 1.00000 \nonumber\\
you_blind & 1.00000 \nonumber\\
hurt_alot & 1.00000 \nonumber\\
watch_to & 1.00000 \nonumber\\
only_option & 1.00000 \nonumber\\
stable & 1.00000 \nonumber\\
do_support & 1.00000 \nonumber\\
he_might & 1.00000 \nonumber\\
he_keep & 1.00000 \nonumber\\
figure_around & 1.00000 \nonumber\\
out_sometime & 1.00000 \nonumber\\
me_play & 1.00000 \nonumber\\
stable_throughout & 1.00000 \nonumber\\
thing_stable & 1.00000 \nonumber\\
keep_thing & 1.00000 \nonumber\\
throughout_your & 1.00000 \nonumber\\
you_or & 1.00000 \nonumber\\
around_even & 1.00000 \nonumber\\
your_childhood & 1.00000 \nonumber\\
huge_role & 1.00000 \nonumber\\
childhood_. & 1.00000 \nonumber\\
the_book & 1.00000 \nonumber\\
them_about & 1.00000 \nonumber\\
on_3 & 1.00000 \nonumber\\
3_side & 1.00000 \nonumber\\
by_water & 1.00000 \nonumber\\
big_advantage & 1.00000 \nonumber\\
other_nation & 1.00000 \nonumber\\
bind_by & 1.00000 \nonumber\\
advantage_for & 1.00000 \nonumber\\
ProductionRule_VP->VBN,PP,PP,,,NP, & 1.00000 \nonumber\\
ProductionRule_NP->RBS,JJ,NNS, & 1.00000 \nonumber\\
which_most & 1.00000 \nonumber\\
most_other & 1.00000 \nonumber\\
,_pe & 1.00000 \nonumber\\
ProductionRule_S->NP,ADVP,,,NP,VP, & 1.00000 \nonumber\\
parent_therefore & 1.00000 \nonumber\\
anybody_would & 1.00000 \nonumber\\
by_there & 1.00000 \nonumber\\
spank_by & 1.00000 \nonumber\\
there_parent & 1.00000 \nonumber\\
maybe_in & 1.00000 \nonumber\\
be_lead & 1.00000 \nonumber\\
ProductionRule_VP->VBG,NP,PP,SBAR, & 1.00000 \nonumber\\
ProductionRule_NP->DT,NN,NN,NN,NN, & 1.00000 \nonumber\\
helpful_to & 1.00000 \nonumber\\
specialy & 1.00000 \nonumber\\
layer_quota & 1.00000 \nonumber\\
but_corruption & 1.00000 \nonumber\\
this_quota & 1.00000 \nonumber\\
future_..... & 1.00000 \nonumber\\
anyone_) & 1.00000 \nonumber\\
cream_layer & 1.00000 \nonumber\\
not_helpful & 1.00000 \nonumber\\
cream & 1.00000 \nonumber\\
(_not & 1.00000 \nonumber\\
specialy_help & 1.00000 \nonumber\\
n't_prefer & 1.00000 \nonumber\\
quota & 1.00000 \nonumber\\
quota_system & 1.00000 \nonumber\\
to_anyone & 1.00000 \nonumber\\
indium_to & 1.00000 \nonumber\\
n't_specialy & 1.00000 \nonumber\\
reason_brain & 1.00000 \nonumber\\
the_cream & 1.00000 \nonumber\\
yes_indium & 1.00000 \nonumber\\
system_i & 1.00000 \nonumber\\
help_indium & 1.00000 \nonumber\\
prefer_indium & 1.00000 \nonumber\\
system_( & 1.00000 \nonumber\\
the_main & 1.00000 \nonumber\\
matter_.... & 1.00000 \nonumber\\
form_for & 1.00000 \nonumber\\
-_with & 1.00000 \nonumber\\
bang_" & 1.00000 \nonumber\\
bang_and & 1.00000 \nonumber\\
rest_on & 1.00000 \nonumber\\
apart_in & 1.00000 \nonumber\\
...._another & 1.00000 \nonumber\\
of_proof & 1.00000 \nonumber\\
interest_because & 1.00000 \nonumber\\
mankind_change & 1.00000 \nonumber\\
proof_rest & 1.00000 \nonumber\\
burden_of & 1.00000 \nonumber\\
burden & 1.00000 \nonumber\\
blow_apart & 1.00000 \nonumber\\
n't_notice & 1.00000 \nonumber\\
the_burden & 1.00000 \nonumber\\
question_- & 1.00000 \nonumber\\
notice_mankind & 1.00000 \nonumber\\
have_blow & 1.00000 \nonumber\\
everything_should & 1.00000 \nonumber\\
like_everything & 1.00000 \nonumber\\
year_.... & 1.00000 \nonumber\\
about_anyone & 1.00000 \nonumber\\
"_theory & 1.00000 \nonumber\\
change_form & 1.00000 \nonumber\\
else_but & 1.00000 \nonumber\\
few_thousand & 1.00000 \nonumber\\
whole_" & 1.00000 \nonumber\\
this_whole & 1.00000 \nonumber\\
"_big & 1.00000 \nonumber\\
another_question & 1.00000 \nonumber\\
then_try & 1.00000 \nonumber\\
user_but & 1.00000 \nonumber\\
i_become & 1.00000 \nonumber\\
'cause_it & 1.00000 \nonumber\\
'cause & 1.00000 \nonumber\\
not_any & 1.00000 \nonumber\\
wrong_'cause & 1.00000 \nonumber\\
any_good & 1.00000 \nonumber\\
reuse & 1.00000 \nonumber\\
to_try & 1.00000 \nonumber\\
not_wear & 1.00000 \nonumber\\
marrage & 1.00000 \nonumber\\
career_, & 1.00000 \nonumber\\
most_important & 1.00000 \nonumber\\
couldnt_picture & 1.00000 \nonumber\\
picture_my & 1.00000 \nonumber\\
ProductionRule_NP->PRP$,NN,CC,NNS, & 1.00000 \nonumber\\
away_someone & 1.00000 \nonumber\\
be_wong & 1.00000 \nonumber\\
ProductionRule_PP->IN,PRN,NP, & 1.00000 \nonumber\\
friend_if & 1.00000 \nonumber\\
you_live & 1.00000 \nonumber\\
i_couldnt & 1.00000 \nonumber\\
wong_especialy & 1.00000 \nonumber\\
_pos_ngram_PR_CONJ_O & 1.00000 \nonumber\\
especialy_if & 1.00000 \nonumber\\
anyone_send & 1.00000 \nonumber\\
wong & 1.00000 \nonumber\\
or_my & 1.00000 \nonumber\\
couldnt & 1.00000 \nonumber\\
send_away & 1.00000 \nonumber\\
ProductionRule_PRN->,,CC,NP, & 1.00000 \nonumber\\
someone_they & 1.00000 \nonumber\\
to_close & 1.00000 \nonumber\\
murder_because & 1.00000 \nonumber\\
would_anyone & 1.00000 \nonumber\\
your_proof & 1.00000 \nonumber\\
atheist_' & 1.00000 \nonumber\\
a_fight & 1.00000 \nonumber\\
between_two & 1.00000 \nonumber\\
"_faith & 1.00000 \nonumber\\
point_this & 1.00000 \nonumber\\
army_where & 1.00000 \nonumber\\
truthfully_win & 1.00000 \nonumber\\
n't_need & 1.00000 \nonumber\\
probably_a & 1.00000 \nonumber\\
proof_to & 1.00000 \nonumber\\
side_contradict & 1.00000 \nonumber\\
both_do & 1.00000 \nonumber\\
one_truthfully & 1.00000 \nonumber\\
your_faith & 1.00000 \nonumber\\
mainly_, & 1.00000 \nonumber\\
other_belief & 1.00000 \nonumber\\
case_or & 1.00000 \nonumber\\
,_whatever & 1.00000 \nonumber\\
oh_lol & 1.00000 \nonumber\\
this_out & 1.00000 \nonumber\\
out_believe & 1.00000 \nonumber\\
this_atheist & 1.00000 \nonumber\\
two_army & 1.00000 \nonumber\\
faith_so & 1.00000 \nonumber\\
support_christianity & 1.00000 \nonumber\\
n't_win & 1.00000 \nonumber\\
own_word & 1.00000 \nonumber\\
faith_" & 1.00000 \nonumber\\
contradict_each & 1.00000 \nonumber\\
exist_do & 1.00000 \nonumber\\
my_" & 1.00000 \nonumber\\
where_both & 1.00000 \nonumber\\
win_until & 1.00000 \nonumber\\
ProductionRule_NP->INTJ,NP, & 1.00000 \nonumber\\
false_be & 1.00000 \nonumber\\
or_turn & 1.00000 \nonumber\\
ppl & 1.00000 \nonumber\\
,_would & 1.00000 \nonumber\\
awesome & 1.00000 \nonumber\\
be_awesome & 1.00000 \nonumber\\
easily-distract & 1.00000 \nonumber\\
n't_go & 1.00000 \nonumber\\
be_exaggerate & 1.00000 \nonumber\\
5_minute & 1.00000 \nonumber\\
,_derelict & 1.00000 \nonumber\\
be_underachieve & 1.00000 \nonumber\\
would_cause & 1.00000 \nonumber\\
,_easily-distract & 1.00000 \nonumber\\
minute_in & 1.00000 \nonumber\\
that_allow & 1.00000 \nonumber\\
allow_that & 1.00000 \nonumber\\
attention_for & 1.00000 \nonumber\\
that_ca & 1.00000 \nonumber\\
easily-distract_, & 1.00000 \nonumber\\
ProductionRule_S->SBAR,,,VP,., & 1.00000 \nonumber\\
exaggerate & 1.00000 \nonumber\\
focus_their & 1.00000 \nonumber\\
my_message & 1.00000 \nonumber\\
for_5 & 1.00000 \nonumber\\
derelict & 1.00000 \nonumber\\
cause_. & 1.00000 \nonumber\\
exaggerate_. & 1.00000 \nonumber\\
n't_focus & 1.00000 \nonumber\\
message_be & 1.00000 \nonumber\\
underachieve_, & 1.00000 \nonumber\\
prevent_problem & 1.00000 \nonumber\\
cry_to & 1.00000 \nonumber\\
derelict_that & 1.00000 \nonumber\\
underachieve & 1.00000 \nonumber\\
the_jungle & 1.00000 \nonumber\\
colony_carve & 1.00000 \nonumber\\
own_money & 1.00000 \nonumber\\
colony & 1.00000 \nonumber\\
start_up & 1.00000 \nonumber\\
nothing_of & 1.00000 \nonumber\\
exterminate & 1.00000 \nonumber\\
the_colony & 1.00000 \nonumber\\
fork & 1.00000 \nonumber\\
fork_out & 1.00000 \nonumber\\
ProductionRule_VP->VBD,ADVP,,,SBAR, & 1.00000 \nonumber\\
to_hunt & 1.00000 \nonumber\\
incentive_for & 1.00000 \nonumber\\
jungle_, & 1.00000 \nonumber\\
contribute_significantly & 1.00000 \nonumber\\
jungle & 1.00000 \nonumber\\
ProductionRule_VP->VBG,PRT,NP,S, & 1.00000 \nonumber\\
significantly_, & 1.00000 \nonumber\\
first_offer & 1.00000 \nonumber\\
an_incentive & 1.00000 \nonumber\\
that_sort & 1.00000 \nonumber\\
exterminate_rat & 1.00000 \nonumber\\
offer_money & 1.00000 \nonumber\\
ProductionRule_NP->S,CC,S, & 1.00000 \nonumber\\
farquhar_contribute & 1.00000 \nonumber\\
even_fork & 1.00000 \nonumber\\
to_exterminate & 1.00000 \nonumber\\
hunt & 1.00000 \nonumber\\
carve & 1.00000 \nonumber\\
by_first & 1.00000 \nonumber\\
hunt_and & 1.00000 \nonumber\\
carve_out & 1.00000 \nonumber\\
sort_. & 1.00000 \nonumber\\
centipede_. & 1.00000 \nonumber\\
remove_farquhar & 1.00000 \nonumber\\
unjustly_remove & 1.00000 \nonumber\\
who_contribute & 1.00000 \nonumber\\
ProductionRule_NP->DT,JJ,NN,'', & 1.00000 \nonumber\\
population_' & 1.00000 \nonumber\\
contribute_so & 1.00000 \nonumber\\
ProductionRule_ADVP->RB,RB,PP, & 1.00000 \nonumber\\
and_accuse & 1.00000 \nonumber\\
ProductionRule_VP->VBD,NP,PP,ADVP, & 1.00000 \nonumber\\
unfair_that & 1.00000 \nonumber\\
be_unfair & 1.00000 \nonumber\\
development_be & 1.00000 \nonumber\\
_pos_ngram_PR_PP_O & 1.00000 \nonumber\\
farquhar_from & 1.00000 \nonumber\\
local_population & 1.00000 \nonumber\\
ProductionRule_VP->ADVP,VBD,NP,PP, & 1.00000 \nonumber\\
off_like & 1.00000 \nonumber\\
much_to & 1.00000 \nonumber\\
raffle_unjustly & 1.00000 \nonumber\\
unjustly_send & 1.00000 \nonumber\\
position_in & 1.00000 \nonumber\\
ProductionRule_ADVP->DT,NN, & 1.00000 \nonumber\\
develop_into & 1.00000 \nonumber\\
great_adult & 1.00000 \nonumber\\
unrelate & 1.00000 \nonumber\\
even_great & 1.00000 \nonumber\\
to_how & 1.00000 \nonumber\\
unrelate_to & 1.00000 \nonumber\\
become_good & 1.00000 \nonumber\\
quite_unrelate & 1.00000 \nonumber\\
who_become & 1.00000 \nonumber\\
be_unnecessary & 1.00000 \nonumber\\
unnecessary_, & 1.00000 \nonumber\\
spank_grow & 1.00000 \nonumber\\
who_grow & 1.00000 \nonumber\\
adult_, & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,ADJP,,,ADVP, & 1.00000 \nonumber\\
terrible_adult & 1.00000 \nonumber\\
how_a & 1.00000 \nonumber\\
_pos_ngram_NP_O_ART & 1.00000 \nonumber\\
begin_of & 1.00000 \nonumber\\
think_aid & 1.00000 \nonumber\\
ProductionRule_FRAG->PP,., & 1.00000 \nonumber\\
aid_exist & 1.00000 \nonumber\\
course_its & 1.00000 \nonumber\\
exist_? & 1.00000 \nonumber\\
young_and & 1.00000 \nonumber\\
phy_ed & 1.00000 \nonumber\\
them_different & 1.00000 \nonumber\\
ProductionRule_FRAG->ADJP,,,SBAR,., & 1.00000 \nonumber\\
everything_they & 1.00000 \nonumber\\
spank_for & 1.00000 \nonumber\\
alway_need & 1.00000 \nonumber\\
government_be & 1.00000 \nonumber\\
right_" & 1.00000 \nonumber\\
real_rights & 1.00000 \nonumber\\
ProductionRule_X->DT,ADJP, & 1.00000 \nonumber\\
question_... & 1.00000 \nonumber\\
ProductionRule_NP->PRP$,CD,NN, & 1.00000 \nonumber\\
unborn_when & 1.00000 \nonumber\\
my_one & 1.00000 \nonumber\\
we_argue & 1.00000 \nonumber\\
"_right & 1.00000 \nonumber\\
ProductionRule_SBAR->IN,X, & 1.00000 \nonumber\\
one_question & 1.00000 \nonumber\\
ProductionRule_S->NP,:,ADVP,VP,., & 1.00000 \nonumber\\
away_our & 1.00000 \nonumber\\
rights_? & 1.00000 \nonumber\\
couch_all & 1.00000 \nonumber\\
just_explore & 1.00000 \nonumber\\
explore_the & 1.00000 \nonumber\\
while_sit & 1.00000 \nonumber\\
be_reform & 1.00000 \nonumber\\
child_what & 1.00000 \nonumber\\
have_involve & 1.00000 \nonumber\\
bounce_on & 1.00000 \nonumber\\
n't_require & 1.00000 \nonumber\\
bounce & 1.00000 \nonumber\\
effort_, & 1.00000 \nonumber\\
do_absolutely & 1.00000 \nonumber\\
test_that & 1.00000 \nonumber\\
barely_move & 1.00000 \nonumber\\
ball & 1.00000 \nonumber\\
lack_. & 1.00000 \nonumber\\
class_can & 1.00000 \nonumber\\
involve_barely & 1.00000 \nonumber\\
on_fitness & 1.00000 \nonumber\\
ball_, & 1.00000 \nonumber\\
education_career & 1.00000 \nonumber\\
require_effort & 1.00000 \nonumber\\
unless_public & 1.00000 \nonumber\\
half-heart_volleyball/dodgeball & 1.00000 \nonumber\\
_pos_ngram_CONJ_PUNC_ADV & 1.00000 \nonumber\\
._throughout & 1.00000 \nonumber\\
talk_with & 1.00000 \nonumber\\
art_high & 1.00000 \nonumber\\
watch_sport & 1.00000 \nonumber\\
ddr_, & 1.00000 \nonumber\\
sport_documentary & 1.00000 \nonumber\\
'_health & 1.00000 \nonumber\\
wius & 1.00000 \nonumber\\
mandatory_for & 1.00000 \nonumber\\
._unless & 1.00000 \nonumber\\
can_teach & 1.00000 \nonumber\\
public_education & 1.00000 \nonumber\\
and_nutrition & 1.00000 \nonumber\\
because_pe & 1.00000 \nonumber\\
half-heart & 1.00000 \nonumber\\
health_and/or & 1.00000 \nonumber\\
documentary_and & 1.00000 \nonumber\\
be_severely & 1.00000 \nonumber\\
severely_lack & 1.00000 \nonumber\\
reform_, & 1.00000 \nonumber\\
education_do & 1.00000 \nonumber\\
friend_, & 1.00000 \nonumber\\
stand_talk & 1.00000 \nonumber\\
me_describe & 1.00000 \nonumber\\
fitness_and & 1.00000 \nonumber\\
this_have & 1.00000 \nonumber\\
fitness_ball & 1.00000 \nonumber\\
fitness_test & 1.00000 \nonumber\\
about_fitness & 1.00000 \nonumber\\
my_pe & 1.00000 \nonumber\\
,_health & 1.00000 \nonumber\\
nutrition_, & 1.00000 \nonumber\\
,_half-heart & 1.00000 \nonumber\\
,_stand & 1.00000 \nonumber\\
my_art & 1.00000 \nonumber\\
with_friend & 1.00000 \nonumber\\
most_recently & 1.00000 \nonumber\\
nutrition & 1.00000 \nonumber\\
ProductionRule_NP->NP,NN,NN,NN, & 1.00000 \nonumber\\
describe_my & 1.00000 \nonumber\\
recently_at & 1.00000 \nonumber\\
wius_sport & 1.00000 \nonumber\\
,_yearly & 1.00000 \nonumber\\
move_, & 1.00000 \nonumber\\
throughout_my & 1.00000 \nonumber\\
and/or_lifestyle & 1.00000 \nonumber\\
ddr & 1.00000 \nonumber\\
volleyball/dodgeball & 1.00000 \nonumber\\
yearly & 1.00000 \nonumber\\
absolutely_nothing & 1.00000 \nonumber\\
volleyball/dodgeball_, & 1.00000 \nonumber\\
,_bounce & 1.00000 \nonumber\\
yearly_physical & 1.00000 \nonumber\\
pe_experience & 1.00000 \nonumber\\
,_ddr & 1.00000 \nonumber\\
play_wius & 1.00000 \nonumber\\
restriction_becoz & 1.00000 \nonumber\\
c_d & 1.00000 \nonumber\\
c & 1.00000 \nonumber\\
better_2 & 1.00000 \nonumber\\
r_away & 1.00000 \nonumber\\
than_keep & 1.00000 \nonumber\\
2_b & 1.00000 \nonumber\\
d_othr & 1.00000 \nonumber\\
way_worse & 1.00000 \nonumber\\
_pos_ngram_PR_ADJ_CARD & 1.00000 \nonumber\\
no_morals.so & 1.00000 \nonumber\\
their_personality & 1.00000 \nonumber\\
2_feed & 1.00000 \nonumber\\
people_2 & 1.00000 \nonumber\\
morals.so & 1.00000 \nonumber\\
these_restriction & 1.00000 \nonumber\\
morals.so_alow & 1.00000 \nonumber\\
restriction_, & 1.00000 \nonumber\\
more_hungry & 1.00000 \nonumber\\
becoz_that & 1.00000 \nonumber\\
teens & 1.00000 \nonumber\\
especialy_teens & 1.00000 \nonumber\\
fashion_. & 1.00000 \nonumber\\
teens_more & 1.00000 \nonumber\\
personality_instead & 1.00000 \nonumber\\
alow_people & 1.00000 \nonumber\\
will_c & 1.00000 \nonumber\\
becoz & 1.00000 \nonumber\\
hungry_for & 1.00000 \nonumber\\
alow & 1.00000 \nonumber\\
hungry.and & 1.00000 \nonumber\\
hungry.and_once & 1.00000 \nonumber\\
hungry & 1.00000 \nonumber\\
them_than & 1.00000 \nonumber\\
for_fashion & 1.00000 \nonumber\\
student_especialy & 1.00000 \nonumber\\
b_free & 1.00000 \nonumber\\
them_hungry.and & 1.00000 \nonumber\\
othr_side & 1.00000 \nonumber\\
worse_with & 1.00000 \nonumber\\
of_stop & 1.00000 \nonumber\\
othr & 1.00000 \nonumber\\
keep_restriction & 1.00000 \nonumber\\
feed_them & 1.00000 \nonumber\\
a_series & 1.00000 \nonumber\\
kinda & 1.00000 \nonumber\\
not_care & 1.00000 \nonumber\\
greedy_, & 1.00000 \nonumber\\
selfish_, & 1.00000 \nonumber\\
toward_the & 1.00000 \nonumber\\
really_exist & 1.00000 \nonumber\\
small_feel & 1.00000 \nonumber\\
have_small & 1.00000 \nonumber\\
exist_in & 1.00000 \nonumber\\
would_care & 1.00000 \nonumber\\
best_advance & 1.00000 \nonumber\\
advance_toward & 1.00000 \nonumber\\
ProductionRule_VP->VBP,NP,VP, & 1.00000 \nonumber\\
but_most & 1.00000 \nonumber\\
,_selfish & 1.00000 \nonumber\\
than_anyone & 1.00000 \nonumber\\
._mostly & 1.00000 \nonumber\\
be_greedy & 1.00000 \nonumber\\
other_would & 1.00000 \nonumber\\
ProductionRule_NP->PRP$,JJS, & 1.00000 \nonumber\\
believe_everyone & 1.00000 \nonumber\\
only_would & 1.00000 \nonumber\\
mostly_everyone & 1.00000 \nonumber\\
feel_toward & 1.00000 \nonumber\\
its_best & 1.00000 \nonumber\\
what_other & 1.00000 \nonumber\\
education_reduce & 1.00000 \nonumber\\
obesity_rate & 1.00000 \nonumber\\
the_obesity & 1.00000 \nonumber\\
failure_, & 1.00000 \nonumber\\
stress_reduction & 1.00000 \nonumber\\
go_even & 1.00000 \nonumber\\
than_what & 1.00000 \nonumber\\
onw_of & 1.00000 \nonumber\\
that_onw & 1.00000 \nonumber\\
dicipline_, & 1.00000 \nonumber\\
why_also & 1.00000 \nonumber\\
self_dicipline & 1.00000 \nonumber\\
,_weight & 1.00000 \nonumber\\
a_physical & 1.00000 \nonumber\\
fitness_, & 1.00000 \nonumber\\
,_self & 1.00000 \nonumber\\
education_class & 1.00000 \nonumber\\
onw & 1.00000 \nonumber\\
,_improve & 1.00000 \nonumber\\
reduction_. & 1.00000 \nonumber\\
improve_physical & 1.00000 \nonumber\\
weight_reduction & 1.00000 \nonumber\\
also_stress & 1.00000 \nonumber\\
heart_failure & 1.00000 \nonumber\\
higher_than & 1.00000 \nonumber\\
reduce_heart & 1.00000 \nonumber\\
be_now & 1.00000 \nonumber\\
reduction & 1.00000 \nonumber\\
reduction_, & 1.00000 \nonumber\\
even_higher & 1.00000 \nonumber\\
rate_will & 1.00000 \nonumber\\
also_physical & 1.00000 \nonumber\\
suicidal & 1.00000 \nonumber\\
love_most & 1.00000 \nonumber\\
get_off & 1.00000 \nonumber\\
suicidal_think & 1.00000 \nonumber\\
most_get & 1.00000 \nonumber\\
become_suicidal & 1.00000 \nonumber\\
_pos_ngram_CARD_O_NN & 1.00000 \nonumber\\
ProductionRule_VP->ADVP,VBG,PRT,PP, & 1.00000 \nonumber\\
other_woman & 1.00000 \nonumber\\
sex_? & 1.00000 \nonumber\\
obviously_, & 1.00000 \nonumber\\
make_man & 1.00000 \nonumber\\
?_obviously & 1.00000 \nonumber\\
species_survive & 1.00000 \nonumber\\
populate & 1.00000 \nonumber\\
to_populate & 1.00000 \nonumber\\
populate_the & 1.00000 \nonumber\\
attract_to & 1.00000 \nonumber\\
can_human & 1.00000 \nonumber\\
survive_if & 1.00000 \nonumber\\
human_species & 1.00000 \nonumber\\
only_attract & 1.00000 \nonumber\\
their_same & 1.00000 \nonumber\\
with_surround & 1.00000 \nonumber\\
in_4-d & 1.00000 \nonumber\\
pleasurable_btw & 1.00000 \nonumber\\
special_effect & 1.00000 \nonumber\\
btw_im & 1.00000 \nonumber\\
surround_sound & 1.00000 \nonumber\\
girl_..... & 1.00000 \nonumber\\
ProductionRule_ADJP->RB,RBR, & 1.00000 \nonumber\\
effect_:) & 1.00000 \nonumber\\
jarman & 1.00000 \nonumber\\
sound_and & 1.00000 \nonumber\\
ProductionRule_S->NP,ADJP,PP, & 1.00000 \nonumber\\
4-d & 1.00000 \nonumber\\
surround & 1.00000 \nonumber\\
it_sholud & 1.00000 \nonumber\\
jarman_: & 1.00000 \nonumber\\
more_pleasurable & 1.00000 \nonumber\\
and_special & 1.00000 \nonumber\\
4-d_with & 1.00000 \nonumber\\
sholud_be & 1.00000 \nonumber\\
pleasurable & 1.00000 \nonumber\\
ProductionRule_VP->ADVP,PP, & 1.00000 \nonumber\\
:)_it & 1.00000 \nonumber\\
sholud & 1.00000 \nonumber\\
lead_. & 1.00000 \nonumber\\
defense_and & 1.00000 \nonumber\\
r_talk & 1.00000 \nonumber\\
the_7th & 1.00000 \nonumber\\
people_talk & 1.00000 \nonumber\\
time_2 & 1.00000 \nonumber\\
3rd_. & 1.00000 \nonumber\\
and_arable & 1.00000 \nonumber\\
arable_land & 1.00000 \nonumber\\
moreover_the & 1.00000 \nonumber\\
2nd_or & 1.00000 \nonumber\\
or_3rd & 1.00000 \nonumber\\
land_respectively & 1.00000 \nonumber\\
arable & 1.00000 \nonumber\\
respectively & 1.00000 \nonumber\\
respectively_but & 1.00000 \nonumber\\
cant_rely & 1.00000 \nonumber\\
people_r & 1.00000 \nonumber\\
u_people & 1.00000 \nonumber\\
development_they & 1.00000 \nonumber\\
2nd_rank & 1.00000 \nonumber\\
here_we & 1.00000 \nonumber\\
on_2nd & 1.00000 \nonumber\\
,_3rd & 1.00000 \nonumber\\
at_their & 1.00000 \nonumber\\
rank_of & 1.00000 \nonumber\\
but_here & 1.00000 \nonumber\\
power_we & 1.00000 \nonumber\\
supreme_power & 1.00000 \nonumber\\
area_defense & 1.00000 \nonumber\\
ProductionRule_VP->LS,ADVP,S, & 1.00000 \nonumber\\
r_happy & 1.00000 \nonumber\\
rank & 1.00000 \nonumber\\
r_lazy & 1.00000 \nonumber\\
7th & 1.00000 \nonumber\\
._u & 1.00000 \nonumber\\
lazy_they & 1.00000 \nonumber\\
2_think & 1.00000 \nonumber\\
7th_, & 1.00000 \nonumber\\
about_country & 1.00000 \nonumber\\
happy_at & 1.00000 \nonumber\\
,_2nd & 1.00000 \nonumber\\
ProductionRule_NX->NP,PP, & 1.00000 \nonumber\\
'_in & 1.00000 \nonumber\\
even_consider & 1.00000 \nonumber\\
some_respects & 1.00000 \nonumber\\
'_give & 1.00000 \nonumber\\
etc._to & 1.00000 \nonumber\\
anything_but & 1.00000 \nonumber\\
give_equal & 1.00000 \nonumber\\
form_in & 1.00000 \nonumber\\
equal_gratification & 1.00000 \nonumber\\
but_wrong & 1.00000 \nonumber\\
most_case & 1.00000 \nonumber\\
'_nothing & 1.00000 \nonumber\\
wrong_in & 1.00000 \nonumber\\
art_form & 1.00000 \nonumber\\
bid_taste & 1.00000 \nonumber\\
could_even & 1.00000 \nonumber\\
all_party & 1.00000 \nonumber\\
an_art & 1.00000 \nonumber\\
consider_it & 1.00000 \nonumber\\
respects & 1.00000 \nonumber\\
respects_. & 1.00000 \nonumber\\
taste & 1.00000 \nonumber\\
it_an & 1.00000 \nonumber\\
gratification_, & 1.00000 \nonumber\\
taste_, & 1.00000 \nonumber\\
in_very & 1.00000 \nonumber\\
definattley & 1.00000 \nonumber\\
life_of & 1.00000 \nonumber\\
whloe & 1.00000 \nonumber\\
be_mandortory & 1.00000 \nonumber\\
excersise_and & 1.00000 \nonumber\\
excersise & 1.00000 \nonumber\\
definattley_all & 1.00000 \nonumber\\
whloe_part & 1.00000 \nonumber\\
a_whloe & 1.00000 \nonumber\\
mandortory_. & 1.00000 \nonumber\\
need_excersise & 1.00000 \nonumber\\
those_obese & 1.00000 \nonumber\\
mandortory & 1.00000 \nonumber\\
_pos_ngram_NP_ART_ART & 1.00000 \nonumber\\
toolbar_appear & 1.00000 \nonumber\\
appear_from & 1.00000 \nonumber\\
from_nowhere & 1.00000 \nonumber\\
random_toolbar & 1.00000 \nonumber\\
ask_before & 1.00000 \nonumber\\
before_anything & 1.00000 \nonumber\\
install_for & 1.00000 \nonumber\\
anything_be & 1.00000 \nonumber\\
be_install & 1.00000 \nonumber\\
ie_random & 1.00000 \nonumber\\
be_ask & 1.00000 \nonumber\\
with_just & 1.00000 \nonumber\\
alcohlic & 1.00000 \nonumber\\
together_how & 1.00000 \nonumber\\
to_an & 1.00000 \nonumber\\
with_theirs & 1.00000 \nonumber\\
theirs & 1.00000 \nonumber\\
life_together & 1.00000 \nonumber\\
theirs_. & 1.00000 \nonumber\\
so_basically & 1.00000 \nonumber\\
an_organization & 1.00000 \nonumber\\
basically_you & 1.00000 \nonumber\\
your_still & 1.00000 \nonumber\\
else_with & 1.00000 \nonumber\\
_pos_ngram_CONJ_CARD_V & 1.00000 \nonumber\\
organization_you & 1.00000 \nonumber\\
one_want & 1.00000 \nonumber\\
organization & 1.00000 \nonumber\\
a_job & 1.00000 \nonumber\\
less_and & 1.00000 \nonumber\\
the_m$ & 1.00000 \nonumber\\
welcome & 1.00000 \nonumber\\
best_virus & 1.00000 \nonumber\\
interface_in & 1.00000 \nonumber\\
by_stick & 1.00000 \nonumber\\
ie_? & 1.00000 \nonumber\\
cute_virus & 1.00000 \nonumber\\
welcome_those & 1.00000 \nonumber\\
m$_ie & 1.00000 \nonumber\\
ProductionRule_S->S,,,RB,SBARQ, & 1.00000 \nonumber\\
ProductionRule_NP->DT,$,NN, & 1.00000 \nonumber\\
little_cute & 1.00000 \nonumber\\
hey_ie & 1.00000 \nonumber\\
virus_interface & 1.00000 \nonumber\\
you_welcome & 1.00000 \nonumber\\
virus_by & 1.00000 \nonumber\\
m$ & 1.00000 \nonumber\\
those_little & 1.00000 \nonumber\\
strongly_believe & 1.00000 \nonumber\\
we_to & 1.00000 \nonumber\\
._william & 1.00000 \nonumber\\
addictive & 1.00000 \nonumber\\
smoke_ciggarette & 1.00000 \nonumber\\
addictive_? & 1.00000 \nonumber\\
unhealthy_? & 1.00000 \nonumber\\
be_smoke & 1.00000 \nonumber\\
wrong_do & 1.00000 \nonumber\\
._addictive & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,NP,ADJP, & 1.00000 \nonumber\\
ciggarette & 1.00000 \nonumber\\
._unhealthy & 1.00000 \nonumber\\
ciggarette_. & 1.00000 \nonumber\\
teach_other & 1.00000 \nonumber\\
or_society & 1.00000 \nonumber\\
legacy_behind & 1.00000 \nonumber\\
out_its & 1.00000 \nonumber\\
about_leave & 1.00000 \nonumber\\
that_everything & 1.00000 \nonumber\\
advance_. & 1.00000 \nonumber\\
can_advance & 1.00000 \nonumber\\
learn_or & 1.00000 \nonumber\\
people_help & 1.00000 \nonumber\\
therefore_you & 1.00000 \nonumber\\
behind_by & 1.00000 \nonumber\\
model_by & 1.00000 \nonumber\\
important_when & 1.00000 \nonumber\\
help_each & 1.00000 \nonumber\\
let_other & 1.00000 \nonumber\\
assist_other & 1.00000 \nonumber\\
by_teach & 1.00000 \nonumber\\
society_process & 1.00000 \nonumber\\
other_take & 1.00000 \nonumber\\
yes_personal & 1.00000 \nonumber\\
by_help & 1.00000 \nonumber\\
but_than & 1.00000 \nonumber\\
you_let & 1.00000 \nonumber\\
leave_legacy & 1.00000 \nonumber\\
process_can & 1.00000 \nonumber\\
of_go & 1.00000 \nonumber\\
derrrr & 1.00000 \nonumber\\
firefox_ah & 1.00000 \nonumber\\
ie_invent & 1.00000 \nonumber\\
hey_nobrob & 1.00000 \nonumber\\
derrrr_!!!!!!!! & 1.00000 \nonumber\\
invent_before & 1.00000 \nonumber\\
nobrob & 1.00000 \nonumber\\
wasnt_ie & 1.00000 \nonumber\\
before_firefox & 1.00000 \nonumber\\
ah_derrrr & 1.00000 \nonumber\\
nobrob_wasnt & 1.00000 \nonumber\\
have_... & 1.00000 \nonumber\\
poor_. & 1.00000 \nonumber\\
the_manpower & 1.00000 \nonumber\\
knowledge_, & 1.00000 \nonumber\\
course_indium & 1.00000 \nonumber\\
happen_anytime & 1.00000 \nonumber\\
anytime_soon & 1.00000 \nonumber\\
manpower_, & 1.00000 \nonumber\\
manpower & 1.00000 \nonumber\\
the_resource & 1.00000 \nonumber\\
world_..... & 1.00000 \nonumber\\
replace & 1.00000 \nonumber\\
kid_can & 1.00000 \nonumber\\
but_use & 1.00000 \nonumber\\
decision_kid & 1.00000 \nonumber\\
open_, & 1.00000 \nonumber\\
,_cute & 1.00000 \nonumber\\
process_you & 1.00000 \nonumber\\
easly_. & 1.00000 \nonumber\\
easy_install & 1.00000 \nonumber\\
oh_yeah & 1.00000 \nonumber\\
thanks_to & 1.00000 \nonumber\\
realease_in & 1.00000 \nonumber\\
addon_, & 1.00000 \nonumber\\
you_about & 1.00000 \nonumber\\
one_will & 1.00000 \nonumber\\
realease & 1.00000 \nonumber\\
that_;) & 1.00000 \nonumber\\
that_and & 1.00000 \nonumber\\
thanks & 1.00000 \nonumber\\
addon & 1.00000 \nonumber\\
'_safe & 1.00000 \nonumber\\
linux & 1.00000 \nonumber\\
exist_an & 1.00000 \nonumber\\
use_linux & 1.00000 \nonumber\\
install_, & 1.00000 \nonumber\\
will_process & 1.00000 \nonumber\\
to_linux & 1.00000 \nonumber\\
ie_version & 1.00000 \nonumber\\
in_less & 1.00000 \nonumber\\
linux_, & 1.00000 \nonumber\\
safe_, & 1.00000 \nonumber\\
linux_! & 1.00000 \nonumber\\
have_addon & 1.00000 \nonumber\\
etc_, & 1.00000 \nonumber\\
easly & 1.00000 \nonumber\\
,_easy & 1.00000 \nonumber\\
;)_oh & 1.00000 \nonumber\\
,_patch & 1.00000 \nonumber\\
patch_realease & 1.00000 \nonumber\\
and_thanks & 1.00000 \nonumber\\
cute_, & 1.00000 \nonumber\\
do_offer & 1.00000 \nonumber\\
hope_in & 1.00000 \nonumber\\
christianity_do & 1.00000 \nonumber\\
offer_hope & 1.00000 \nonumber\\
fool_. & 1.00000 \nonumber\\
factual & 1.00000 \nonumber\\
team_seem & 1.00000 \nonumber\\
excrament_. & 1.00000 \nonumber\\
foolish_fool & 1.00000 \nonumber\\
excrament & 1.00000 \nonumber\\
fool & 1.00000 \nonumber\\
bunch_of & 1.00000 \nonumber\\
bunch & 1.00000 \nonumber\\
bull_excrament & 1.00000 \nonumber\\
your_team & 1.00000 \nonumber\\
a_bunch & 1.00000 \nonumber\\
of_foolish & 1.00000 \nonumber\\
factual_and & 1.00000 \nonumber\\
foolish & 1.00000 \nonumber\\
not_factual & 1.00000 \nonumber\\
in_lesson & 1.00000 \nonumber\\
any_important & 1.00000 \nonumber\\
it_time & 1.00000 \nonumber\\
to_constantly & 1.00000 \nonumber\\
on_shop & 1.00000 \nonumber\\
constantly_worry & 1.00000 \nonumber\\
wear_every & 1.00000 \nonumber\\
little_bore & 1.00000 \nonumber\\
less_costly & 1.00000 \nonumber\\
costly_this & 1.00000 \nonumber\\
do_any & 1.00000 \nonumber\\
same_set & 1.00000 \nonumber\\
morn_. & 1.00000 \nonumber\\
so_regularly & 1.00000 \nonumber\\
shop_trip & 1.00000 \nonumber\\
trip & 1.00000 \nonumber\\
regularly_. & 1.00000 \nonumber\\
shop & 1.00000 \nonumber\\
which_help & 1.00000 \nonumber\\
situation_you & 1.00000 \nonumber\\
i_actually & 1.00000 \nonumber\\
trip_so & 1.00000 \nonumber\\
na_wear & 1.00000 \nonumber\\
bore_put & 1.00000 \nonumber\\
'_less & 1.00000 \nonumber\\
hit_than & 1.00000 \nonumber\\
fear_get & 1.00000 \nonumber\\
they_fear & 1.00000 \nonumber\\
ever_right & 1.00000 \nonumber\\
selfish_creature & 1.00000 \nonumber\\
of_views.we & 1.00000 \nonumber\\
different_point & 1.00000 \nonumber\\
to_question & 1.00000 \nonumber\\
different_people & 1.00000 \nonumber\\
so_ever & 1.00000 \nonumber\\
thing_accord & 1.00000 \nonumber\\
views.we_perceive & 1.00000 \nonumber\\
what_so & 1.00000 \nonumber\\
views.we & 1.00000 \nonumber\\
perception_and & 1.00000 \nonumber\\
view_thing & 1.00000 \nonumber\\
have_different & 1.00000 \nonumber\\
only_view & 1.00000 \nonumber\\
who_go & 1.00000 \nonumber\\
creature_we & 1.00000 \nonumber\\
very_selfish & 1.00000 \nonumber\\
no_what & 1.00000 \nonumber\\
way_as & 1.00000 \nonumber\\
'_point & 1.00000 \nonumber\\
and_disgust & 1.00000 \nonumber\\
on_perception & 1.00000 \nonumber\\
individualist_' & 1.00000 \nonumber\\
woman_marriage & 1.00000 \nonumber\\
the_individualist & 1.00000 \nonumber\\
perceive_that & 1.00000 \nonumber\\
weird_. & 1.00000 \nonumber\\
'_perception & 1.00000 \nonumber\\
we_human & 1.00000 \nonumber\\
individualist & 1.00000 \nonumber\\
be_weird & 1.00000 \nonumber\\
question_one & 1.00000 \nonumber\\
disgust_but & 1.00000 \nonumber\\
title_and & 1.00000 \nonumber\\
ie7_' & 1.00000 \nonumber\\
firefox_2.0 & 1.00000 \nonumber\\
hover_over & 1.00000 \nonumber\\
page_title & 1.00000 \nonumber\\
hover & 1.00000 \nonumber\\
7_have & 1.00000 \nonumber\\
the_tooltip & 1.00000 \nonumber\\
title_. & 1.00000 \nonumber\\
ProductionRule_NP->DT,NN,NN,CC,NN, & 1.00000 \nonumber\\
'_tab & 1.00000 \nonumber\\
you_hover & 1.00000 \nonumber\\
over_ie7 & 1.00000 \nonumber\\
_pos_ngram_NP_CARD_ADV & 1.00000 \nonumber\\
2.0 & 1.00000 \nonumber\\
have_title & 1.00000 \nonumber\\
tooltip & 1.00000 \nonumber\\
and_address & 1.00000 \nonumber\\
tooltip_have & 1.00000 \nonumber\\
2.0_just & 1.00000 \nonumber\\
ProductionRule_S->S,CC,,,S, & 1.00000 \nonumber\\
_pos_ngram_CONJ_PUNC_PR & 1.00000 \nonumber\\
!_so & 1.00000 \nonumber\\
however_it & 1.00000 \nonumber\\
when_in & 1.00000 \nonumber\\
themselve_and & 1.00000 \nonumber\\
one_' & 1.00000 \nonumber\\
in_jail & 1.00000 \nonumber\\
husband_commit & 1.00000 \nonumber\\
everybody_make & 1.00000 \nonumber\\
wrong_decision & 1.00000 \nonumber\\
partner_throught & 1.00000 \nonumber\\
he_must & 1.00000 \nonumber\\
throught_the & 1.00000 \nonumber\\
thin_no & 1.00000 \nonumber\\
husband_to & 1.00000 \nonumber\\
throught & 1.00000 \nonumber\\
decision_he & 1.00000 \nonumber\\
._everybody & 1.00000 \nonumber\\
he_take & 1.00000 \nonumber\\
this_would & 1.00000 \nonumber\\
the_thick & 1.00000 \nonumber\\
this_situation & 1.00000 \nonumber\\
ProductionRule_VP->NP,SBAR, & 1.00000 \nonumber\\
sir & 1.00000 \nonumber\\
sir_raffle & 1.00000 \nonumber\\
action_can & 1.00000 \nonumber\\
to_decipher & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,ADJP,PP,S, & 1.00000 \nonumber\\
display_that & 1.00000 \nonumber\\
'_face & 1.00000 \nonumber\\
be_display & 1.00000 \nonumber\\
decipher_from & 1.00000 \nonumber\\
decipher & 1.00000 \nonumber\\
character_' & 1.00000 \nonumber\\
tire_. & 1.00000 \nonumber\\
simply_. & 1.00000 \nonumber\\
compulsory.the_minimum & 1.00000 \nonumber\\
compulsory.the & 1.00000 \nonumber\\
be_compulsory.the & 1.00000 \nonumber\\
why_physical & 1.00000 \nonumber\\
._simply & 1.00000 \nonumber\\
simply_too & 1.00000 \nonumber\\
too_tire & 1.00000 \nonumber\\
their_view & 1.00000 \nonumber\\
in_childhood & 1.00000 \nonumber\\
follower & 1.00000 \nonumber\\
follower_at & 1.00000 \nonumber\\
by_any & 1.00000 \nonumber\\
watch_out & 1.00000 \nonumber\\
atheist_than & 1.00000 \nonumber\\
the_follower & 1.00000 \nonumber\\
atheist_by & 1.00000 \nonumber\\
follow_them & 1.00000 \nonumber\\
no_individual & 1.00000 \nonumber\\
most_religion & 1.00000 \nonumber\\
will_twist & 1.00000 \nonumber\\
any_logic & 1.00000 \nonumber\\
rather_call & 1.00000 \nonumber\\
find_most & 1.00000 \nonumber\\
be_intelligent & 1.00000 \nonumber\\
absolutely_ridiculous & 1.00000 \nonumber\\
allow_for & 1.00000 \nonumber\\
twist_any & 1.00000 \nonumber\\
religion_absolutely & 1.00000 \nonumber\\
and_illogical & 1.00000 \nonumber\\
theist_who & 1.00000 \nonumber\\
;)_i & 1.00000 \nonumber\\
be_theist & 1.00000 \nonumber\\
call_myself & 1.00000 \nonumber\\
who_follow & 1.00000 \nonumber\\
illogical_, & 1.00000 \nonumber\\
means_, & 1.00000 \nonumber\\
think_process & 1.00000 \nonumber\\
brainwash_in & 1.00000 \nonumber\\
logic_in & 1.00000 \nonumber\\
for_;) & 1.00000 \nonumber\\
least_. & 1.00000 \nonumber\\
individual_think & 1.00000 \nonumber\\
myself_an & 1.00000 \nonumber\\
childhood_and & 1.00000 \nonumber\\
only_people & 1.00000 \nonumber\\
logic_to & 1.00000 \nonumber\\
more_logic & 1.00000 \nonumber\\
any_means & 1.00000 \nonumber\\
intelligent_one & 1.00000 \nonumber\\
my_mind & 1.00000 \nonumber\\
not_someone & 1.00000 \nonumber\\
good_role & 1.00000 \nonumber\\
open & 1.00000 \nonumber\\
around_be & 1.00000 \nonumber\\
what_exactly & 1.00000 \nonumber\\
._grow & 1.00000 \nonumber\\
way_your & 1.00000 \nonumber\\
without_that & 1.00000 \nonumber\\
than_he & 1.00000 \nonumber\\
surpass_him & 1.00000 \nonumber\\
to_prefer & 1.00000 \nonumber\\
exactly_make & 1.00000 \nonumber\\
alway_around & 1.00000 \nonumber\\
,_alway & 1.00000 \nonumber\\
or_give & 1.00000 \nonumber\\
the_motivation & 1.00000 \nonumber\\
might_become & 1.00000 \nonumber\\
become_even & 1.00000 \nonumber\\
become_like & 1.00000 \nonumber\\
him_or & 1.00000 \nonumber\\
that_figure & 1.00000 \nonumber\\
become_lose & 1.00000 \nonumber\\
ProductionRule_NP->DT,JJ,NN,S, & 1.00000 \nonumber\\
,_good & 1.00000 \nonumber\\
abortion_should & 1.00000 \nonumber\\
draw_. & 1.00000 \nonumber\\
be_few & 1.00000 \nonumber\\
someone_would & 1.00000 \nonumber\\
somebody_. & 1.00000 \nonumber\\
the_no & 1.00000 \nonumber\\
drive_to & 1.00000 \nonumber\\
ProductionRule_VP->VBG,ADVP,SBAR, & 1.00000 \nonumber\\
about_there & 1.00000 \nonumber\\
commit_. & 1.00000 \nonumber\\
kill_but & 1.00000 \nonumber\\
no_snitch & 1.00000 \nonumber\\
murder_that & 1.00000 \nonumber\\
yea_at & 1.00000 \nonumber\\
act_should & 1.00000 \nonumber\\
snitch_say & 1.00000 \nonumber\\
draw & 1.00000 \nonumber\\
ProductionRule_NP->DT,DT,NN, & 1.00000 \nonumber\\
in_say & 1.00000 \nonumber\\
why_someone & 1.00000 \nonumber\\
be_draw & 1.00000 \nonumber\\
be_drive & 1.00000 \nonumber\\
line_be & 1.00000 \nonumber\\
few_reason & 1.00000 \nonumber\\
im_all & 1.00000 \nonumber\\
._yea & 1.00000 \nonumber\\
she_ever & 1.00000 \nonumber\\
be_commit & 1.00000 \nonumber\\
people_rationalize & 1.00000 \nonumber\\
doesnt_make & 1.00000 \nonumber\\
in_america & 1.00000 \nonumber\\
sense_... & 1.00000 \nonumber\\
dont_undertsand & 1.00000 \nonumber\\
take_life & 1.00000 \nonumber\\
life_it & 1.00000 \nonumber\\
america_how & 1.00000 \nonumber\\
ProductionRule_S->S,SBARQ, & 1.00000 \nonumber\\
be_how & 1.00000 \nonumber\\
rationalize & 1.00000 \nonumber\\
idc_the & 1.00000 \nonumber\\
idc & 1.00000 \nonumber\\
leagal & 1.00000 \nonumber\\
leagal_? & 1.00000 \nonumber\\
ProductionRule_VP->VBP,S,:,S, & 1.00000 \nonumber\\
undertsand & 1.00000 \nonumber\\
undertsand_be & 1.00000 \nonumber\\
kill_leagal & 1.00000 \nonumber\\
..._idc & 1.00000 \nonumber\\
any_sense & 1.00000 \nonumber\\
rationalize_take & 1.00000 \nonumber\\
spouse_, & 1.00000 \nonumber\\
out_there & 1.00000 \nonumber\\
be_ponder & 1.00000 \nonumber\\
better_it & 1.00000 \nonumber\\
your_other & 1.00000 \nonumber\\
bigger_gap & 1.00000 \nonumber\\
dad_could & 1.00000 \nonumber\\
boyfriend_as & 1.00000 \nonumber\\
how_amaze & 1.00000 \nonumber\\
other_half & 1.00000 \nonumber\\
._wonder & 1.00000 \nonumber\\
terrible_they & 1.00000 \nonumber\\
prove_fact & 1.00000 \nonumber\\
than_wonder & 1.00000 \nonumber\\
by_have & 1.00000 \nonumber\\
what_could & 1.00000 \nonumber\\
'_similar & 1.00000 \nonumber\\
a_bigger & 1.00000 \nonumber\\
father_create & 1.00000 \nonumber\\
amaze_your & 1.00000 \nonumber\\
gap_in & 1.00000 \nonumber\\
how_terrible & 1.00000 \nonumber\\
lousy_boyfriend & 1.00000 \nonumber\\
half_that & 1.00000 \nonumber\\
similar & 1.00000 \nonumber\\
similar_to & 1.00000 \nonumber\\
wonder_how & 1.00000 \nonumber\\
a_prove & 1.00000 \nonumber\\
mean_have & 1.00000 \nonumber\\
wonder_what & 1.00000 \nonumber\\
ponder_how & 1.00000 \nonumber\\
existence_of & 1.00000 \nonumber\\
the_existence & 1.00000 \nonumber\\
when_alway & 1.00000 \nonumber\\
lonely_. & 1.00000 \nonumber\\
lonely & 1.00000 \nonumber\\
like_by & 1.00000 \nonumber\\
'_champ & 1.00000 \nonumber\\
jerk_be & 1.00000 \nonumber\\
hole_. & 1.00000 \nonumber\\
alone_and & 1.00000 \nonumber\\
a_rapper & 1.00000 \nonumber\\
when_alone & 1.00000 \nonumber\\
champ_. & 1.00000 \nonumber\\
when_want & 1.00000 \nonumber\\
an_a & 1.00000 \nonumber\\
once_be & 1.00000 \nonumber\\
rapper_who & 1.00000 \nonumber\\
become_lonely & 1.00000 \nonumber\\
successful_sometime & 1.00000 \nonumber\\
a_jerk & 1.00000 \nonumber\\
conceit & 1.00000 \nonumber\\
conceit_and & 1.00000 \nonumber\\
rapper & 1.00000 \nonumber\\
other_become & 1.00000 \nonumber\\
become_conceit & 1.00000 \nonumber\\
you_tend & 1.00000 \nonumber\\
there_once & 1.00000 \nonumber\\
ProductionRule_ADVP->RBR,RB, & 1.00000 \nonumber\\
only_reasonable & 1.00000 \nonumber\\
more_that & 1.00000 \nonumber\\
argument_ie & 1.00000 \nonumber\\
reasonable_argument & 1.00000 \nonumber\\
user_have & 1.00000 \nonumber\\
be_cooler & 1.00000 \nonumber\\
prove_even & 1.00000 \nonumber\\
cooler_or & 1.00000 \nonumber\\
lay_more & 1.00000 \nonumber\\
more_only & 1.00000 \nonumber\\
cheat & 1.00000 \nonumber\\
up_a & 1.00000 \nonumber\\
vote_bid & 1.00000 \nonumber\\
there_young & 1.00000 \nonumber\\
self_there & 1.00000 \nonumber\\
when_there & 1.00000 \nonumber\\
independence_. & 1.00000 \nonumber\\
there_independence & 1.00000 \nonumber\\
find_them & 1.00000 \nonumber\\
spank_them & 1.00000 \nonumber\\
_pos_ngram_CONJ_ART_CARD & 1.00000 \nonumber\\
spouse_' & 1.00000 \nonumber\\
self-defense_they & 1.00000 \nonumber\\
self-defense_or & 1.00000 \nonumber\\
mourn_because & 1.00000 \nonumber\\
would_eat & 1.00000 \nonumber\\
in_whether & 1.00000 \nonumber\\
mourn & 1.00000 \nonumber\\
eat_at & 1.00000 \nonumber\\
an_act & 1.00000 \nonumber\\
it_but & 1.00000 \nonumber\\
of_rage & 1.00000 \nonumber\\
likely_get & 1.00000 \nonumber\\
not_live & 1.00000 \nonumber\\
rage_i & 1.00000 \nonumber\\
rage_. & 1.00000 \nonumber\\
rage & 1.00000 \nonumber\\
conscience_would & 1.00000 \nonumber\\
'_action & 1.00000 \nonumber\\
live_know & 1.00000 \nonumber\\
family_that & 1.00000 \nonumber\\
be_self-defense & 1.00000 \nonumber\\
my_conscience & 1.00000 \nonumber\\
be_mourn & 1.00000 \nonumber\\
uniform_u & 1.00000 \nonumber\\
fashionable_you & 1.00000 \nonumber\\
ProductionRule_VP->VP,,,RB,VP, & 1.00000 \nonumber\\
u_can & 1.00000 \nonumber\\
how_fashionable & 1.00000 \nonumber\\
to_sleep & 1.00000 \nonumber\\
never_go & 1.00000 \nonumber\\
say_this & 1.00000 \nonumber\\
ashame_of & 1.00000 \nonumber\\
go_day & 1.00000 \nonumber\\
that_father & 1.00000 \nonumber\\
of_him & 1.00000 \nonumber\\
especially_for & 1.00000 \nonumber\\
else_for & 1.00000 \nonumber\\
special_, & 1.00000 \nonumber\\
anything_special & 1.00000 \nonumber\\
with_him & 1.00000 \nonumber\\
us_about & 1.00000 \nonumber\\
about_team & 1.00000 \nonumber\\
do_community & 1.00000 \nonumber\\
service_be & 1.00000 \nonumber\\
day_our & 1.00000 \nonumber\\
teacher_have & 1.00000 \nonumber\\
or_our & 1.00000 \nonumber\\
parent_or & 1.00000 \nonumber\\
help_our & 1.00000 \nonumber\\
whole_point & 1.00000 \nonumber\\
the_very & 1.00000 \nonumber\\
very_first & 1.00000 \nonumber\\
team_work & 1.00000 \nonumber\\
our_teacher & 1.00000 \nonumber\\
have_teach & 1.00000 \nonumber\\
anyone_can & 1.00000 \nonumber\\
bite_strict & 1.00000 \nonumber\\
strict_, & 1.00000 \nonumber\\
abuse_a & 1.00000 \nonumber\\
do_again & 1.00000 \nonumber\\
spank_fast & 1.00000 \nonumber\\
fast_, & 1.00000 \nonumber\\
spank_do & 1.00000 \nonumber\\
so_its & 1.00000 \nonumber\\
really_solve & 1.00000 \nonumber\\
_pos_ngram_O_NP_CONJ & 1.00000 \nonumber\\
_pos_ngram_CARD_V_PR & 1.00000 \nonumber\\
can_hurt & 1.00000 \nonumber\\
hurt_and & 1.00000 \nonumber\\
sometime_good & 1.00000 \nonumber\\
use_repeatedly & 1.00000 \nonumber\\
spank_can & 1.00000 \nonumber\\
understand_but & 1.00000 \nonumber\\
ProductionRule_CONJP->CC,RB, & 1.00000 \nonumber\\
be_sometime & 1.00000 \nonumber\\
ProductionRule_PP->PP,CONJP,PP, & 1.00000 \nonumber\\
through_the & 1.00000 \nonumber\\
of_two & 1.00000 \nonumber\\
everyone_take & 1.00000 \nonumber\\
change_you & 1.00000 \nonumber\\
do_change & 1.00000 \nonumber\\
change_to & 1.00000 \nonumber\\
want_change & 1.00000 \nonumber\\
that_know & 1.00000 \nonumber\\
believe_if & 1.00000 \nonumber\\
selfish_thing & 1.00000 \nonumber\\
and_believe & 1.00000 \nonumber\\
people_then & 1.00000 \nonumber\\
no_use & 1.00000 \nonumber\\
only_person & 1.00000 \nonumber\\
to_abuse & 1.00000 \nonumber\\
like_in & 1.00000 \nonumber\\
world_??????????????? & 1.00000 \nonumber\\
indium_don & 1.00000 \nonumber\\
!!!!!!!!!!!!_jaus & 1.00000 \nonumber\\
indian_say & 1.00000 \nonumber\\
world_other-than & 1.00000 \nonumber\\
??????????????? & 1.00000 \nonumber\\
???????????????_indium & 1.00000 \nonumber\\
jaus & 1.00000 \nonumber\\
jaus_hind & 1.00000 \nonumber\\
!!!!!!!!!!!! & 1.00000 \nonumber\\
the_heaven & 1.00000 \nonumber\\
other-than_any & 1.00000 \nonumber\\
other-than & 1.00000 \nonumber\\
country_!!!!!!!!!!!! & 1.00000 \nonumber\\
heaven_in & 1.00000 \nonumber\\
heaven & 1.00000 \nonumber\\
become_potential & 1.00000 \nonumber\\
hardwork_..... & 1.00000 \nonumber\\
believe_yourself & 1.00000 \nonumber\\
and_hardwork & 1.00000 \nonumber\\
surely_indium & 1.00000 \nonumber\\
_pos_ngram_NP_PR_CONJ & 1.00000 \nonumber\\
don_not & 1.00000 \nonumber\\
..._surely & 1.00000 \nonumber\\
don & 1.00000 \nonumber\\
_pos_ngram_NN_ADJ_ART & 1.00000 \nonumber\\
....._believe & 1.00000 \nonumber\\
hardwork & 1.00000 \nonumber\\
can_indian & 1.00000 \nonumber\\
pursuit_you & 1.00000 \nonumber\\
year_be & 1.00000 \nonumber\\
in_high & 1.00000 \nonumber\\
optional_class & 1.00000 \nonumber\\
grade_, & 1.00000 \nonumber\\
because_little & 1.00000 \nonumber\\
yes_phy & 1.00000 \nonumber\\
in_lower & 1.00000 \nonumber\\
especially_not & 1.00000 \nonumber\\
little_kid & 1.00000 \nonumber\\
should_still & 1.00000 \nonumber\\
one_year & 1.00000 \nonumber\\
lower_grade & 1.00000 \nonumber\\
_pos_ngram_ADV_ART_CARD & 1.00000 \nonumber\\
thing_instead & 1.00000 \nonumber\\
a_continuous & 1.00000 \nonumber\\
an_optional & 1.00000 \nonumber\\
mandatory_thing & 1.00000 \nonumber\\
in_weird & 1.00000 \nonumber\\
class_and & 1.00000 \nonumber\\
gain_and & 1.00000 \nonumber\\
(_especially & 1.00000 \nonumber\\
they_shouldnt & 1.00000 \nonumber\\
a_mandatory & 1.00000 \nonumber\\
mandatory_( & 1.00000 \nonumber\\
weight_in & 1.00000 \nonumber\\
continuous & 1.00000 \nonumber\\
while_yes & 1.00000 \nonumber\\
weird_pattern & 1.00000 \nonumber\\
h_) & 1.00000 \nonumber\\
ed_. & 1.00000 \nonumber\\
of_h & 1.00000 \nonumber\\
pattern_. & 1.00000 \nonumber\\
._class & 1.00000 \nonumber\\
h & 1.00000 \nonumber\\
all_4 & 1.00000 \nonumber\\
lose_weight & 1.00000 \nonumber\\
continuous_pe & 1.00000 \nonumber\\
maybe_just & 1.00000 \nonumber\\
or_she & 1.00000 \nonumber\\
100_% & 1.00000 \nonumber\\
ProductionRule_NP->DT,JJS,NN,NN, & 1.00000 \nonumber\\
will_become & 1.00000 \nonumber\\
dont_judge & 1.00000 \nonumber\\
judge_yourself & 1.00000 \nonumber\\
and_forgiveness & 1.00000 \nonumber\\
other_before & 1.00000 \nonumber\\
two_marry & 1.00000 \nonumber\\
judge_other & 1.00000 \nonumber\\
forgiveness & 1.00000 \nonumber\\
gender_love & 1.00000 \nonumber\\
teach_love & 1.00000 \nonumber\\
nutjobe_by & 1.00000 \nonumber\\
you_judge & 1.00000 \nonumber\\
nutjobe & 1.00000 \nonumber\\
way_be & 1.00000 \nonumber\\
forget_dont & 1.00000 \nonumber\\
bible_nutjobe & 1.00000 \nonumber\\
really_teach & 1.00000 \nonumber\\
bible_really & 1.00000 \nonumber\\
people_regardless & 1.00000 \nonumber\\
you_bible & 1.00000 \nonumber\\
_pos_ngram_ART_ART_CARD & 1.00000 \nonumber\\
forgiveness_, & 1.00000 \nonumber\\
let_not & 1.00000 \nonumber\\
follow_what & 1.00000 \nonumber\\
of_gender & 1.00000 \nonumber\\
that_follow & 1.00000 \nonumber\\
matter_? & 1.00000 \nonumber\\
bible_teach & 1.00000 \nonumber\\
bible_have & 1.00000 \nonumber\\
more_sense & 1.00000 \nonumber\\
time_will & 1.00000 \nonumber\\
through_different & 1.00000 \nonumber\\
existence_... & 1.00000 \nonumber\\
evolution_make & 1.00000 \nonumber\\
contradiction_and & 1.00000 \nonumber\\
concrete_evidence & 1.00000 \nonumber\\
._animal & 1.00000 \nonumber\\
convince_in & 1.00000 \nonumber\\
his_existence & 1.00000 \nonumber\\
no_concrete & 1.00000 \nonumber\\
and_change & 1.00000 \nonumber\\
sense_to & 1.00000 \nonumber\\
many_contradiction & 1.00000 \nonumber\\
and_situation & 1.00000 \nonumber\\
survive_through & 1.00000 \nonumber\\
climate_and & 1.00000 \nonumber\\
climate & 1.00000 \nonumber\\
over_huge & 1.00000 \nonumber\\
support_that & 1.00000 \nonumber\\
their_environment & 1.00000 \nonumber\\
different_climate & 1.00000 \nonumber\\
..._evolution & 1.00000 \nonumber\\
animal_adapt & 1.00000 \nonumber\\
less_convince & 1.00000 \nonumber\\
become_less & 1.00000 \nonumber\\
that_support & 1.00000 \nonumber\\
alcohlic_. & 1.00000 \nonumber\\
your_boy & 1.00000 \nonumber\\
about_guy & 1.00000 \nonumber\\
right_if & 1.00000 \nonumber\\
alot_especially & 1.00000 \nonumber\\
be_friend & 1.00000 \nonumber\\
boy_because & 1.00000 \nonumber\\
an_alcohlic & 1.00000 \nonumber\\
view_be & 1.00000 \nonumber\\
would_understand & 1.00000 \nonumber\\
whether_its & 1.00000 \nonumber\\
at_sometime & 1.00000 \nonumber\\
you_at & 1.00000 \nonumber\\
different_then & 1.00000 \nonumber\\
mother_you & 1.00000 \nonumber\\
or_life & 1.00000 \nonumber\\
n't_because & 1.00000 \nonumber\\
means_alot & 1.00000 \nonumber\\
guy_problem & 1.00000 \nonumber\\
father_even & 1.00000 \nonumber\\
job_or & 1.00000 \nonumber\\
most_father & 1.00000 \nonumber\\
father_means & 1.00000 \nonumber\\
live_my & 1.00000 \nonumber\\
her_view & 1.00000 \nonumber\\
father_they & 1.00000 \nonumber\\
just_live & 1.00000 \nonumber\\
no_job & 1.00000 \nonumber\\
friend_to & 1.00000 \nonumber\\
_pos_ngram_ADV_PUNC_CARD & 1.00000 \nonumber\\
and_sure & 1.00000 \nonumber\\
choose_that & 1.00000 \nonumber\\
sure_woman & 1.00000 \nonumber\\
business_, & 1.00000 \nonumber\\
that_business & 1.00000 \nonumber\\
own_desire & 1.00000 \nonumber\\
'_their & 1.00000 \nonumber\\
path_. & 1.00000 \nonumber\\
pornography_but & 1.00000 \nonumber\\
path & 1.00000 \nonumber\\
career_path & 1.00000 \nonumber\\
that_career & 1.00000 \nonumber\\
be_... & 1.00000 \nonumber\\
your_go & 1.00000 \nonumber\\
study_, & 1.00000 \nonumber\\
would_really & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,RB,NP,SBAR, & 1.00000 \nonumber\\
detrimental & 1.00000 \nonumber\\
"_http://www.democraticunderground.com/discuss/duboard.php?az=view & 1.00000 \nonumber\\
their_production & 1.00000 \nonumber\\
other_beverage & 1.00000 \nonumber\\
habit_. & 1.00000 \nonumber\\
consume_huge & 1.00000 \nonumber\\
"_bottle & 1.00000 \nonumber\\
our_biggest & 1.00000 \nonumber\\
beverage_consume & 1.00000 \nonumber\\
detrimental_than & 1.00000 \nonumber\\
during_their & 1.00000 \nonumber\\
make_their & 1.00000 \nonumber\\
energy_during & 1.00000 \nonumber\\
biggest_problem & 1.00000 \nonumber\\
their_ecological & 1.00000 \nonumber\\
impact_far & 1.00000 \nonumber\\
ecological & 1.00000 \nonumber\\
ecological_impact & 1.00000 \nonumber\\
more_detrimental & 1.00000 \nonumber\\
and_energy & 1.00000 \nonumber\\
drink_habit & 1.00000 \nonumber\\
production_process & 1.00000 \nonumber\\
apply & 1.00000 \nonumber\\
that_indian & 1.00000 \nonumber\\
a_role & 1.00000 \nonumber\\
i_cant & 1.00000 \nonumber\\
ProductionRule_VP->VBN,PP,,,SBAR, & 1.00000 \nonumber\\
site_in & 1.00000 \nonumber\\
be_design & 1.00000 \nonumber\\
ie_in & 1.00000 \nonumber\\
design_only & 1.00000 \nonumber\\
government_site & 1.00000 \nonumber\\
ProductionRule_VP->VBP,RB,PP, & 1.00000 \nonumber\\
or_speak & 1.00000 \nonumber\\
country_then & 1.00000 \nonumber\\
specific_language & 1.00000 \nonumber\\
understand_or & 1.00000 \nonumber\\
how_the & 1.00000 \nonumber\\
tv_come & 1.00000 \nonumber\\
also_hear & 1.00000 \nonumber\\
be_pronounce & 1.00000 \nonumber\\
only_understand & 1.00000 \nonumber\\
pronounce_in & 1.00000 \nonumber\\
hear_how & 1.00000 \nonumber\\
your_language & 1.00000 \nonumber\\
move_to & 1.00000 \nonumber\\
different_language & 1.00000 \nonumber\\
language_but & 1.00000 \nonumber\\
speak_a & 1.00000 \nonumber\\
pronounce & 1.00000 \nonumber\\
language_. & 1.00000 \nonumber\\
ProductionRule_VP->VP,,,VP, & 1.00000 \nonumber\\
steal_the & 1.00000 \nonumber\\
,_steal & 1.00000 \nonumber\\
get_extension & 1.00000 \nonumber\\
browse_from & 1.00000 \nonumber\\
scum_, & 1.00000 \nonumber\\
tab_browse & 1.00000 \nonumber\\
be_scum & 1.00000 \nonumber\\
other_browser & 1.00000 \nonumber\\
extension_for & 1.00000 \nonumber\\
scum & 1.00000 \nonumber\\
hmmm_that & 1.00000 \nonumber\\
hmmm & 1.00000 \nonumber\\
my_vow & 1.00000 \nonumber\\
marry_without & 1.00000 \nonumber\\
the_bid & 1.00000 \nonumber\\
ProductionRule_VP->ADVP,VBG,SBAR, & 1.00000 \nonumber\\
definitely_would & 1.00000 \nonumber\\
toughy_. & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,PP,PP, & 1.00000 \nonumber\\
without_truly & 1.00000 \nonumber\\
whatever_reason & 1.00000 \nonumber\\
toughy & 1.00000 \nonumber\\
._hmmm & 1.00000 \nonumber\\
a_toughy & 1.00000 \nonumber\\
marriage_through & 1.00000 \nonumber\\
mean_some & 1.00000 \nonumber\\
who_the & 1.00000 \nonumber\\
for_whatever & 1.00000 \nonumber\\
death_do & 1.00000 \nonumber\\
be_divorce & 1.00000 \nonumber\\
hard_one & 1.00000 \nonumber\\
divorce_that & 1.00000 \nonumber\\
us_part & 1.00000 \nonumber\\
in_thick & 1.00000 \nonumber\\
do_us & 1.00000 \nonumber\\
vow_of & 1.00000 \nonumber\\
thin_till & 1.00000 \nonumber\\
because_for & 1.00000 \nonumber\\
well_if & 1.00000 \nonumber\\
i_definitely & 1.00000 \nonumber\\
a_promise & 1.00000 \nonumber\\
till_death & 1.00000 \nonumber\\
happen_all & 1.00000 \nonumber\\
truly_know & 1.00000 \nonumber\\
love_this & 1.00000 \nonumber\\
all_you & 1.00000 \nonumber\\
equally & 1.00000 \nonumber\\
though_he & 1.00000 \nonumber\\
well_i & 1.00000 \nonumber\\
hobbe & 1.00000 \nonumber\\
ProductionRule_S->RB,VP,., & 1.00000 \nonumber\\
._ever & 1.00000 \nonumber\\
should_look & 1.00000 \nonumber\\
you_state & 1.00000 \nonumber\\
glib_, & 1.00000 \nonumber\\
glib & 1.00000 \nonumber\\
t._hobbe & 1.00000 \nonumber\\
..._? & 1.00000 \nonumber\\
assist_us & 1.00000 \nonumber\\
ever_read & 1.00000 \nonumber\\
our_belief & 1.00000 \nonumber\\
belief_system & 1.00000 \nonumber\\
ProductionRule_VP->VB,PP,S, & 1.00000 \nonumber\\
be_glib & 1.00000 \nonumber\\
t. & 1.00000 \nonumber\\
read_t. & 1.00000 \nonumber\\
hobbe_... & 1.00000 \nonumber\\
abortion_legal & 1.00000 \nonumber\\
keep_abortion & 1.00000 \nonumber\\
tell_him & 1.00000 \nonumber\\
ProductionRule_PP->IN,WHNP, & 1.00000 \nonumber\\
ProductionRule_NP->PRP$,NX, & 1.00000 \nonumber\\
this_point & 1.00000 \nonumber\\
at_this & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,PP,,,S, & 1.00000 \nonumber\\
attest_to & 1.00000 \nonumber\\
attest & 1.00000 \nonumber\\
science_attest & 1.00000 \nonumber\\
school_where & 1.00000 \nonumber\\
ProductionRule_NP->NP,PP,-RRB-, & 1.00000 \nonumber\\
bless & 1.00000 \nonumber\\
amaze_god & 1.00000 \nonumber\\
bless_to & 1.00000 \nonumber\\
definitely_christianity & 1.00000 \nonumber\\
be_bless & 1.00000 \nonumber\\
our_amaze & 1.00000 \nonumber\\
christian_school & 1.00000 \nonumber\\
christianity_:) & 1.00000 \nonumber\\
god_: & 1.00000 \nonumber\\
:)_and & 1.00000 \nonumber\\
ProductionRule_PP->IN,NP,:, & 1.00000 \nonumber\\
;) & 1.00000 \nonumber\\
day_then & 1.00000 \nonumber\\
can_quit & 1.00000 \nonumber\\
get_sick & 1.00000 \nonumber\\
dislike_sport & 1.00000 \nonumber\\
,_play & 1.00000 \nonumber\\
and_healthy & 1.00000 \nonumber\\
better_at & 1.00000 \nonumber\\
unfit_. & 1.00000 \nonumber\\
pe_should & 1.00000 \nonumber\\
and_unfit & 1.00000 \nonumber\\
it_keep & 1.00000 \nonumber\\
healthy_. & 1.00000 \nonumber\\
compulsory_because & 1.00000 \nonumber\\
play_and & 1.00000 \nonumber\\
teamwork_. & 1.00000 \nonumber\\
really_dislike & 1.00000 \nonumber\\
quit & 1.00000 \nonumber\\
constantly_fit & 1.00000 \nonumber\\
at_teamwork & 1.00000 \nonumber\\
us_constantly & 1.00000 \nonumber\\
best_thing & 1.00000 \nonumber\\
keep_us & 1.00000 \nonumber\\
it_when & 1.00000 \nonumber\\
sick_and & 1.00000 \nonumber\\
and_lie & 1.00000 \nonumber\\
lie_on & 1.00000 \nonumber\\
pe_help & 1.00000 \nonumber\\
quit_it & 1.00000 \nonumber\\
be_compulsory & 1.00000 \nonumber\\
part_. & 1.00000 \nonumber\\
to_oregon & 1.00000 \nonumber\\
that_! & 1.00000 \nonumber\\
oregon_? & 1.00000 \nonumber\\
leaf_the & 1.00000 \nonumber\\
ProductionRule_SINV->FRAG,,,VP,S,., & 1.00000 \nonumber\\
oregon & 1.00000 \nonumber\\
decision_with & 1.00000 \nonumber\\
to_enforce & 1.00000 \nonumber\\
her_god & 1.00000 \nonumber\\
pro-choice_and & 1.00000 \nonumber\\
everywhere_( & 1.00000 \nonumber\\
without_force & 1.00000 \nonumber\\
(_ever & 1.00000 \nonumber\\
god_instead & 1.00000 \nonumber\\
legal_leaf & 1.00000 \nonumber\\
power_without & 1.00000 \nonumber\\
enough_power & 1.00000 \nonumber\\
enforce_that & 1.00000 \nonumber\\
enforce & 1.00000 \nonumber\\
not_illegal & 1.00000 \nonumber\\
force_the & 1.00000 \nonumber\\
!_it & 1.00000 \nonumber\\
of_with & 1.00000 \nonumber\\
_pos_ngram_PR_NP_ADV & 1.00000 \nonumber\\
,_try & 1.00000 \nonumber\\
religion_on & 1.00000 \nonumber\\
suicide_everywhere & 1.00000 \nonumber\\
actually_not & 1.00000 \nonumber\\
nobody_to & 1.00000 \nonumber\\
bid_time & 1.00000 \nonumber\\
or_tell & 1.00000 \nonumber\\
have_nobody & 1.00000 \nonumber\\
him_your & 1.00000 \nonumber\\
to_count & 1.00000 \nonumber\\
with_or & 1.00000 \nonumber\\
count_with & 1.00000 \nonumber\\
jesus_, & 1.00000 \nonumber\\
love_jesus & 1.00000 \nonumber\\
individuality_- & 1.00000 \nonumber\\
hinder & 1.00000 \nonumber\\
still-develop_child & 1.00000 \nonumber\\
still-develop & 1.00000 \nonumber\\
ProductionRule_NP->NP,PRN,PP, & 1.00000 \nonumber\\
creative_expression & 1.00000 \nonumber\\
hinder_the & 1.00000 \nonumber\\
ought & 1.00000 \nonumber\\
ought_to & 1.00000 \nonumber\\
school_ought & 1.00000 \nonumber\\
expression_- & 1.00000 \nonumber\\
-_of & 1.00000 \nonumber\\
to_hinder & 1.00000 \nonumber\\
ProductionRule_PRN->:,NP,:, & 1.00000 \nonumber\\
the_individuality & 1.00000 \nonumber\\
their_still-develop & 1.00000 \nonumber\\
the_creative & 1.00000 \nonumber\\
_pos_ngram_ADV_O_CARD & 1.00000 \nonumber\\
refute_my & 1.00000 \nonumber\\
without_one & 1.00000 \nonumber\\
action_be & 1.00000 \nonumber\\
statement_by & 1.00000 \nonumber\\
become_extinct & 1.00000 \nonumber\\
an_action & 1.00000 \nonumber\\
statement & 1.00000 \nonumber\\
benefit_if & 1.00000 \nonumber\\
straight_people & 1.00000 \nonumber\\
because_without & 1.00000 \nonumber\\
._fair & 1.00000 \nonumber\\
like_say & 1.00000 \nonumber\\
marriage_ca & 1.00000 \nonumber\\
who_wo & 1.00000 \nonumber\\
reproduction_and & 1.00000 \nonumber\\
not_benefit & 1.00000 \nonumber\\
say_kill & 1.00000 \nonumber\\
continuation_of & 1.00000 \nonumber\\
extinct & 1.00000 \nonumber\\
continuation & 1.00000 \nonumber\\
if_society & 1.00000 \nonumber\\
no_reproduction & 1.00000 \nonumber\\
fair_enough & 1.00000 \nonumber\\
all_become & 1.00000 \nonumber\\
n't_refute & 1.00000 \nonumber\\
all_do & 1.00000 \nonumber\\
enough_? & 1.00000 \nonumber\\
reproduction & 1.00000 \nonumber\\
extinct_, & 1.00000 \nonumber\\
then_society & 1.00000 \nonumber\\
would_benefit & 1.00000 \nonumber\\
my_statement & 1.00000 \nonumber\\
ethical_. & 1.00000 \nonumber\\
ethical & 1.00000 \nonumber\\
ethical_if & 1.00000 \nonumber\\
society_as & 1.00000 \nonumber\\
be_ethical & 1.00000 \nonumber\\
and_continuation & 1.00000 \nonumber\\
whole_would & 1.00000 \nonumber\\
our_species & 1.00000 \nonumber\\
woman_there & 1.00000 \nonumber\\
one_man & 1.00000 \nonumber\\
drink_on & 1.00000 \nonumber\\
all_even & 1.00000 \nonumber\\
just_how & 1.00000 \nonumber\\
curse_my & 1.00000 \nonumber\\
him_my & 1.00000 \nonumber\\
a_alcohlic & 1.00000 \nonumber\\
alcohlic_father & 1.00000 \nonumber\\
n't_call & 1.00000 \nonumber\\
ProductionRule_S->NP,S,VP,., & 1.00000 \nonumber\\
bid_he & 1.00000 \nonumber\\
he_his & 1.00000 \nonumber\\
who_drink & 1.00000 \nonumber\\
his_still & 1.00000 \nonumber\\
and_curse & 1.00000 \nonumber\\
still_in & 1.00000 \nonumber\\
establish_2000yr & 1.00000 \nonumber\\
ago_where & 1.00000 \nonumber\\
where_other & 1.00000 \nonumber\\
ProductionRule_NP->PRN,NNS, & 1.00000 \nonumber\\
language_be & 1.00000 \nonumber\\
there_languag & 1.00000 \nonumber\\
2000yr_ago & 1.00000 \nonumber\\
2000yr & 1.00000 \nonumber\\
find_there & 1.00000 \nonumber\\
be_establish & 1.00000 \nonumber\\
indian_culture & 1.00000 \nonumber\\
i_turn & 1.00000 \nonumber\\
the_mood & 1.00000 \nonumber\\
release_. & 1.00000 \nonumber\\
for_sex & 1.00000 \nonumber\\
like_simple & 1.00000 \nonumber\\
facilitate & 1.00000 \nonumber\\
facilitate_this & 1.00000 \nonumber\\
mood_for & 1.00000 \nonumber\\
simple_release & 1.00000 \nonumber\\
mood & 1.00000 \nonumber\\
pornography_facilitate & 1.00000 \nonumber\\
._pornography & 1.00000 \nonumber\\
_pos_ngram_PUNC_CARD_ADV & 1.00000 \nonumber\\
job_your & 1.00000 \nonumber\\
better_benifit & 1.00000 \nonumber\\
a_50/50 & 1.00000 \nonumber\\
another_employe & 1.00000 \nonumber\\
50/50_. & 1.00000 \nonumber\\
good_" & 1.00000 \nonumber\\
make_another & 1.00000 \nonumber\\
make_yourself & 1.00000 \nonumber\\
that_evryone & 1.00000 \nonumber\\
benifit_us & 1.00000 \nonumber\\
less_selfish & 1.00000 \nonumber\\
hand_we & 1.00000 \nonumber\\
a_kind & 1.00000 \nonumber\\
good_so & 1.00000 \nonumber\\
50/50 & 1.00000 \nonumber\\
well_for & 1.00000 \nonumber\\
yourself_look & 1.00000 \nonumber\\
evryone_should & 1.00000 \nonumber\\
example_in & 1.00000 \nonumber\\
employe_, & 1.00000 \nonumber\\
evryone & 1.00000 \nonumber\\
employe & 1.00000 \nonumber\\
"_advance & 1.00000 \nonumber\\
to_thing & 1.00000 \nonumber\\
again_on & 1.00000 \nonumber\\
actuality_, & 1.00000 \nonumber\\
package_, & 1.00000 \nonumber\\
,_market & 1.00000 \nonumber\\
the_high & 1.00000 \nonumber\\
ship_, & 1.00000 \nonumber\\
transport_it & 1.00000 \nonumber\\
ProductionRule_UCP->NP,CC,VP, & 1.00000 \nonumber\\
water_but & 1.00000 \nonumber\\
retail & 1.00000 \nonumber\\
retail_and & 1.00000 \nonumber\\
ProductionRule_NP->NP,,,NP,,,NP,,,NP,,,NP, & 1.00000 \nonumber\\
,_ship & 1.00000 \nonumber\\
actuality & 1.00000 \nonumber\\
and_transport & 1.00000 \nonumber\\
high_price & 1.00000 \nonumber\\
in_actuality & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,RB,NP,ADVP,,,PP, & 1.00000 \nonumber\\
,_retail & 1.00000 \nonumber\\
cost_of & 1.00000 \nonumber\\
,_package & 1.00000 \nonumber\\
ProductionRule_S->S,,,CC,SBARQ,., & 1.00000 \nonumber\\
just_me & 1.00000 \nonumber\\
help_at & 1.00000 \nonumber\\
good_i & 1.00000 \nonumber\\
all_just & 1.00000 \nonumber\\
ProductionRule_SBARQ->WHADVP,S, & 1.00000 \nonumber\\
feel_so & 1.00000 \nonumber\\
volunteer_at & 1.00000 \nonumber\\
favor_in & 1.00000 \nonumber\\
so_great & 1.00000 \nonumber\\
volunteer & 1.00000 \nonumber\\
at_some & 1.00000 \nonumber\\
irve_care & 1.00000 \nonumber\\
help_myself & 1.00000 \nonumber\\
help_ourselve & 1.00000 \nonumber\\
irve & 1.00000 \nonumber\\
at_irve & 1.00000 \nonumber\\
return_or & 1.00000 \nonumber\\
a_favor & 1.00000 \nonumber\\
would_our & 1.00000 \nonumber\\
great_that & 1.00000 \nonumber\\
i_volunteer & 1.00000 \nonumber\\
just_help & 1.00000 \nonumber\\
ourselve_where & 1.00000 \nonumber\\
its_sick & 1.00000 \nonumber\\
porn_eg & 1.00000 \nonumber\\
sick_porn & 1.00000 \nonumber\\
eg_child & 1.00000 \nonumber\\
ProductionRule_NP->PRP$,JJ,NX, & 1.00000 \nonumber\\
wrong_unless & 1.00000 \nonumber\\
aslong & 1.00000 \nonumber\\
unless_its & 1.00000 \nonumber\\
_pos_ngram_PR_ADJ_O & 1.00000 \nonumber\\
pornography_be & 1.00000 \nonumber\\
aslong_as & 1.00000 \nonumber\\
or_rape & 1.00000 \nonumber\\
view_in & 1.00000 \nonumber\\
a_discreet & 1.00000 \nonumber\\
discreet & 1.00000 \nonumber\\
ok_aslong & 1.00000 \nonumber\\
as_its & 1.00000 \nonumber\\
animal_or & 1.00000 \nonumber\\
,_animal & 1.00000 \nonumber\\
ProductionRule_NP->NN,,,NN,CC,NN, & 1.00000 \nonumber\\
rape_but & 1.00000 \nonumber\\
its_view & 1.00000 \nonumber\\
discreet_manner & 1.00000 \nonumber\\
other_pornography & 1.00000 \nonumber\\
bring_a & 1.00000 \nonumber\\
tell_not & 1.00000 \nonumber\\
ProductionRule_VP->VB,PP,ADVP,SBAR, & 1.00000 \nonumber\\
ProductionRule_VP->ADVP,VBN,NP, & 1.00000 \nonumber\\
call_for & 1.00000 \nonumber\\
certain_circumstance & 1.00000 \nonumber\\
bastard_child & 1.00000 \nonumber\\
ProductionRule_VP->VBN,CC,VBN,PP, & 1.00000 \nonumber\\
and_severely & 1.00000 \nonumber\\
emotionally_traumatize & 1.00000 \nonumber\\
for_desperate & 1.00000 \nonumber\\
make_and & 1.00000 \nonumber\\
the_bastard & 1.00000 \nonumber\\
._certain & 1.00000 \nonumber\\
traumatize_her & 1.00000 \nonumber\\
that_baby & 1.00000 \nonumber\\
rape_her & 1.00000 \nonumber\\
severely_emotionally & 1.00000 \nonumber\\
circumstance_call & 1.00000 \nonumber\\
who_rape & 1.00000 \nonumber\\
her_' & 1.00000 \nonumber\\
desperate_decision & 1.00000 \nonumber\\
desperate & 1.00000 \nonumber\\
bid_dad & 1.00000 \nonumber\\
ProductionRule_SBAR->WHADJP,S, & 1.00000 \nonumber\\
ProductionRule_WHADJP->WRB,JJ, & 1.00000 \nonumber\\
infront & 1.00000 \nonumber\\
infront_of & 1.00000 \nonumber\\
cause_obesity & 1.00000 \nonumber\\
against_tv & 1.00000 \nonumber\\
..._it & 1.00000 \nonumber\\
us_or & 1.00000 \nonumber\\
add_more & 1.00000 \nonumber\\
unwant_child & 1.00000 \nonumber\\
more_unwant & 1.00000 \nonumber\\
like_drug & 1.00000 \nonumber\\
biblically & 1.00000 \nonumber\\
alcohol_. & 1.00000 \nonumber\\
that_destroy & 1.00000 \nonumber\\
biblically_, & 1.00000 \nonumber\\
why_god & 1.00000 \nonumber\\
god_tell & 1.00000 \nonumber\\
drug_and & 1.00000 \nonumber\\
ProductionRule_S->ADVP,,,RB,NP,VP,., & 1.00000 \nonumber\\
but_aside & 1.00000 \nonumber\\
life_just & 1.00000 \nonumber\\
destroy_life & 1.00000 \nonumber\\
aside_from & 1.00000 \nonumber\\
alcohol & 1.00000 \nonumber\\
addiction_that & 1.00000 \nonumber\\
and_alcohol & 1.00000 \nonumber\\
the_infestation & 1.00000 \nonumber\\
for_farquar & 1.00000 \nonumber\\
weed_out & 1.00000 \nonumber\\
out_many & 1.00000 \nonumber\\
farquar_weed & 1.00000 \nonumber\\
centipede_infestation & 1.00000 \nonumber\\
finish_destroy & 1.00000 \nonumber\\
infestation_. & 1.00000 \nonumber\\
problem_at & 1.00000 \nonumber\\
take_only & 1.00000 \nonumber\\
infestation_, & 1.00000 \nonumber\\
day_for & 1.00000 \nonumber\\
farquar_to & 1.00000 \nonumber\\
weed & 1.00000 \nonumber\\
infestation & 1.00000 \nonumber\\
wealth_of & 1.00000 \nonumber\\
spread_the & 1.00000 \nonumber\\
just_yourself & 1.00000 \nonumber\\
but_have & 1.00000 \nonumber\\
mass_or & 1.00000 \nonumber\\
or_situation & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,ADVP,ADVP, & 1.00000 \nonumber\\
greatest_benefit & 1.00000 \nonumber\\
mass & 1.00000 \nonumber\\
task_but & 1.00000 \nonumber\\
by_advance & 1.00000 \nonumber\\
you_spread & 1.00000 \nonumber\\
around_once & 1.00000 \nonumber\\
improve_the & 1.00000 \nonumber\\
nobility & 1.00000 \nonumber\\
good_only & 1.00000 \nonumber\\
life_or & 1.00000 \nonumber\\
into_consideration & 1.00000 \nonumber\\
of_nobility & 1.00000 \nonumber\\
life_time & 1.00000 \nonumber\\
take_into & 1.00000 \nonumber\\
an_assessable & 1.00000 \nonumber\\
consideration & 1.00000 \nonumber\\
nobility_to & 1.00000 \nonumber\\
consideration_that & 1.00000 \nonumber\\
can_improve & 1.00000 \nonumber\\
assessable & 1.00000 \nonumber\\
assessable_task & 1.00000 \nonumber\\
benefit_yourself & 1.00000 \nonumber\\
ProductionRule_PP->CC,S, & 1.00000 \nonumber\\
alway_an & 1.00000 \nonumber\\
the_mass & 1.00000 \nonumber\\
really_suck & 1.00000 \nonumber\\
obligatory_in & 1.00000 \nonumber\\
clase & 1.00000 \nonumber\\
clase_should & 1.00000 \nonumber\\
of_obecity & 1.00000 \nonumber\\
pe_clase & 1.00000 \nonumber\\
obecity & 1.00000 \nonumber\\
obecity_. & 1.00000 \nonumber\\
ever_wan & 1.00000 \nonumber\\
it_bright & 1.00000 \nonumber\\
breathe & 1.00000 \nonumber\\
apart_i & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,PRT,SBAR, & 1.00000 \nonumber\\
would_surely & 1.00000 \nonumber\\
breathe_life & 1.00000 \nonumber\\
bright_light & 1.00000 \nonumber\\
nightmare & 1.00000 \nonumber\\
n't_ever & 1.00000 \nonumber\\
wake & 1.00000 \nonumber\\
here_like & 1.00000 \nonumber\\
clean_this & 1.00000 \nonumber\\
light_turn & 1.00000 \nonumber\\
nightmare_if & 1.00000 \nonumber\\
like_punch & 1.00000 \nonumber\\
punch_in & 1.00000 \nonumber\\
punch & 1.00000 \nonumber\\
surely_wake & 1.00000 \nonumber\\
_pos_ngram_PR_ADJ_NP & 1.00000 \nonumber\\
turn_me & 1.00000 \nonumber\\
wake_it & 1.00000 \nonumber\\
me_clean & 1.00000 \nonumber\\
dream_breathe & 1.00000 \nonumber\\
it_fall & 1.00000 \nonumber\\
life_into & 1.00000 \nonumber\\
be_worse & 1.00000 \nonumber\\
my_nightmare & 1.00000 \nonumber\\
into_my & 1.00000 \nonumber\\
a_dream & 1.00000 \nonumber\\
fall_apart & 1.00000 \nonumber\\
tiny_bite & 1.00000 \nonumber\\
two_period & 1.00000 \nonumber\\
school_who & 1.00000 \nonumber\\
change_any & 1.00000 \nonumber\\
week_and & 1.00000 \nonumber\\
and_afterschool & 1.00000 \nonumber\\
a_tiny & 1.00000 \nonumber\\
of_pe & 1.00000 \nonumber\\
pe_a & 1.00000 \nonumber\\
not_change & 1.00000 \nonumber\\
afterschool & 1.00000 \nonumber\\
afterschool_sport & 1.00000 \nonumber\\
sport_have & 1.00000 \nonumber\\
help_some & 1.00000 \nonumber\\
love_for & 1.00000 \nonumber\\
murder_by & 1.00000 \nonumber\\
crime_to & 1.00000 \nonumber\\
a_definitely & 1.00000 \nonumber\\
on_stay & 1.00000 \nonumber\\
major_crime & 1.00000 \nonumber\\
ProductionRule_X->ADVP,NP, & 1.00000 \nonumber\\
most_. & 1.00000 \nonumber\\
definitely_no & 1.00000 \nonumber\\
but_although & 1.00000 \nonumber\\
i_plan & 1.00000 \nonumber\\
well_then & 1.00000 \nonumber\\
never_turn & 1.00000 \nonumber\\
with_then & 1.00000 \nonumber\\
ProductionRule_NP->DT,X, & 1.00000 \nonumber\\
drain & 1.00000 \nonumber\\
brain_drain & 1.00000 \nonumber\\
drain_, & 1.00000 \nonumber\\
_pos_ngram_PUNC_PUNC_ADJ & 1.00000 \nonumber\\
what_your & 1.00000 \nonumber\\
n't_kill & 1.00000 \nonumber\\
right_because & 1.00000 \nonumber\\
a_u.s. & 1.00000 \nonumber\\
u.s._decision & 1.00000 \nonumber\\
argue_about & 1.00000 \nonumber\\
canada & 1.00000 \nonumber\\
decision_when & 1.00000 \nonumber\\
canada_? & 1.00000 \nonumber\\
in_canada & 1.00000 \nonumber\\
my_public & 1.00000 \nonumber\\
add_to & 1.00000 \nonumber\\
rely & 1.00000 \nonumber\\
rely_on & 1.00000 \nonumber\\
mac & 1.00000 \nonumber\\
?_there & 1.00000 \nonumber\\
since_when & 1.00000 \nonumber\\
second_paragraph & 1.00000 \nonumber\\
share_? & 1.00000 \nonumber\\
"_original & 1.00000 \nonumber\\
market_share & 1.00000 \nonumber\\
_pos_ngram_ADJ_V_O & 1.00000 \nonumber\\
argument_either & 1.00000 \nonumber\\
fad_? & 1.00000 \nonumber\\
when_be & 1.00000 \nonumber\\
mac_firefox & 1.00000 \nonumber\\
more_window & 1.00000 \nonumber\\
firefox_an & 1.00000 \nonumber\\
even_worth & 1.00000 \nonumber\\
browser_everyone & 1.00000 \nonumber\\
n't_contain & 1.00000 \nonumber\\
worth_rebut & 1.00000 \nonumber\\
apple_fad & 1.00000 \nonumber\\
original_" & 1.00000 \nonumber\\
original_and & 1.00000 \nonumber\\
since_day & 1.00000 \nonumber\\
paragraph & 1.00000 \nonumber\\
else_do & 1.00000 \nonumber\\
contain_a & 1.00000 \nonumber\\
firefox_download & 1.00000 \nonumber\\
an_apple & 1.00000 \nonumber\\
paragraph_of & 1.00000 \nonumber\\
single_fact & 1.00000 \nonumber\\
download_since & 1.00000 \nonumber\\
than_mac & 1.00000 \nonumber\\
fad & 1.00000 \nonumber\\
mind_" & 1.00000 \nonumber\\
and_free & 1.00000 \nonumber\\
58.6 & 1.00000 \nonumber\\
a_58.6 & 1.00000 \nonumber\\
58.6_% & 1.00000 \nonumber\\
be_firefox & 1.00000 \nonumber\\
rebut_the & 1.00000 \nonumber\\
window_than & 1.00000 \nonumber\\
%_market & 1.00000 \nonumber\\
temptation & 1.00000 \nonumber\\
wow_. & 1.00000 \nonumber\\
baby_make & 1.00000 \nonumber\\
temptation_to & 1.00000 \nonumber\\
baby_? & 1.00000 \nonumber\\
next_generation & 1.00000 \nonumber\\
be_sex & 1.00000 \nonumber\\
?_- & 1.00000 \nonumber\\
sex_what & 1.00000 \nonumber\\
generation_... & 1.00000 \nonumber\\
for_? & 1.00000 \nonumber\\
should_you & 1.00000 \nonumber\\
..._conclusion & 1.00000 \nonumber\\
make_why & 1.00000 \nonumber\\
to_control & 1.00000 \nonumber\\
conclusion & 1.00000 \nonumber\\
conclusion_: & 1.00000 \nonumber\\
situation_where & 1.00000 \nonumber\\
_pos_ngram_PUNC_ADJ_ADV & 1.00000 \nonumber\\
make_baby & 1.00000 \nonumber\\
in_porn & 1.00000 \nonumber\\
watch_other & 1.00000 \nonumber\\
porn_? & 1.00000 \nonumber\\
pleasure_what & 1.00000 \nonumber\\
pleasure_? & 1.00000 \nonumber\\
temptation_? & 1.00000 \nonumber\\
control_temptation & 1.00000 \nonumber\\
>_then & 1.00000 \nonumber\\
cause_pleasure & 1.00000 \nonumber\\
>_temptation & 1.00000 \nonumber\\
sex_for & 1.00000 \nonumber\\
>_sex & 1.00000 \nonumber\\
be_temptation & 1.00000 \nonumber\\
>_pleasure & 1.00000 \nonumber\\
>_baby & 1.00000 \nonumber\\
temptation_what & 1.00000 \nonumber\\
> & 1.00000 \nonumber\\
..._wow & 1.00000 \nonumber\\
other_make & 1.00000 \nonumber\\
-_> & 1.00000 \nonumber\\
run_so & 1.00000 \nonumber\\
to_run & 1.00000 \nonumber\\
soooo_much & 1.00000 \nonumber\\
p.e._i & 1.00000 \nonumber\\
much_!!!!! & 1.00000 \nonumber\\
hate_p.e. & 1.00000 \nonumber\\
it_soooo & 1.00000 \nonumber\\
edison & 1.00000 \nonumber\\
edison_, & 1.00000 \nonumber\\
found_father & 1.00000 \nonumber\\
our_found & 1.00000 \nonumber\\
martin & 1.00000 \nonumber\\
huge_advance & 1.00000 \nonumber\\
honor_for & 1.00000 \nonumber\\
thoma_edison & 1.00000 \nonumber\\
martin_luther & 1.00000 \nonumber\\
george_washington & 1.00000 \nonumber\\
make_advancement & 1.00000 \nonumber\\
washington_, & 1.00000 \nonumber\\
have_succede & 1.00000 \nonumber\\
george & 1.00000 \nonumber\\
succede & 1.00000 \nonumber\\
jr_, & 1.00000 \nonumber\\
,_george & 1.00000 \nonumber\\
honor & 1.00000 \nonumber\\
,_thoma & 1.00000 \nonumber\\
thoma & 1.00000 \nonumber\\
allot_of & 1.00000 \nonumber\\
._allot & 1.00000 \nonumber\\
allot & 1.00000 \nonumber\\
in_do & 1.00000 \nonumber\\
jr & 1.00000 \nonumber\\
make_huge & 1.00000 \nonumber\\
luther_king & 1.00000 \nonumber\\
luther & 1.00000 \nonumber\\
king_jr & 1.00000 \nonumber\\
world_forever & 1.00000 \nonumber\\
succede_in & 1.00000 \nonumber\\
be_honor & 1.00000 \nonumber\\
washington & 1.00000 \nonumber\\
while_strive & 1.00000 \nonumber\\
,_martin & 1.00000 \nonumber\\
still_be & 1.00000 \nonumber\\
just_plain & 1.00000 \nonumber\\
all_so & 1.00000 \nonumber\\
after_high & 1.00000 \nonumber\\
dont_go & 1.00000 \nonumber\\
but_personal & 1.00000 \nonumber\\
_pos_ngram_ART_ADV_O & 1.00000 \nonumber\\
wont_go & 1.00000 \nonumber\\
pursuit_will & 1.00000 \nonumber\\
choose_my & 1.00000 \nonumber\\
go_at & 1.00000 \nonumber\\
college_after & 1.00000 \nonumber\\
ProductionRule_NP->DT,ADVP,NN, & 1.00000 \nonumber\\
announce_to & 1.00000 \nonumber\\
power_. & 1.00000 \nonumber\\
little_money & 1.00000 \nonumber\\
truly_advance & 1.00000 \nonumber\\
ever_in & 1.00000 \nonumber\\
of_power & 1.00000 \nonumber\\
a_career & 1.00000 \nonumber\\
will_announce & 1.00000 \nonumber\\
persuit_come & 1.00000 \nonumber\\
donate_a & 1.00000 \nonumber\\
have_money & 1.00000 \nonumber\\
little_bite & 1.00000 \nonumber\\
end_if & 1.00000 \nonumber\\
here_and & 1.00000 \nonumber\\
,_donate & 1.00000 \nonumber\\
donate & 1.00000 \nonumber\\
announce & 1.00000 \nonumber\\
there_really & 1.00000 \nonumber\\
that_focus & 1.00000 \nonumber\\
reach_a & 1.00000 \nonumber\\
your_ever & 1.00000 \nonumber\\
could_truly & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,ADVP,,,S,,,S, & 1.00000 \nonumber\\
and_reach & 1.00000 \nonumber\\
money_you & 1.00000 \nonumber\\
enough_to & 1.00000 \nonumber\\
and_her & 1.00000 \nonumber\\
to_god & 1.00000 \nonumber\\
historical & 1.00000 \nonumber\\
save_life & 1.00000 \nonumber\\
by_eliminate & 1.00000 \nonumber\\
do_legalize & 1.00000 \nonumber\\
illegaly_abort & 1.00000 \nonumber\\
?_keep & 1.00000 \nonumber\\
drug_have & 1.00000 \nonumber\\
ProductionRule_SQ->VBZ,VP, & 1.00000 \nonumber\\
legal_will & 1.00000 \nonumber\\
illegaly & 1.00000 \nonumber\\
with_save & 1.00000 \nonumber\\
kill_themselve & 1.00000 \nonumber\\
themselve_at & 1.00000 \nonumber\\
life_by & 1.00000 \nonumber\\
to_illegaly & 1.00000 \nonumber\\
help_save & 1.00000 \nonumber\\
legalize_drug & 1.00000 \nonumber\\
_pos_ngram_CONJ_ADV_CONJ & 1.00000 \nonumber\\
whoop-de-doo_. & 1.00000 \nonumber\\
be_neccisary & 1.00000 \nonumber\\
little_hypocritical & 1.00000 \nonumber\\
be_convince & 1.00000 \nonumber\\
in_creationism & 1.00000 \nonumber\\
debate_it & 1.00000 \nonumber\\
in_evolutionism & 1.00000 \nonumber\\
the_opponent & 1.00000 \nonumber\\
'_great & 1.00000 \nonumber\\
see_why & 1.00000 \nonumber\\
neccisary & 1.00000 \nonumber\\
neccisary_. & 1.00000 \nonumber\\
why_even & 1.00000 \nonumber\\
post_this & 1.00000 \nonumber\\
xd_sorry & 1.00000 \nonumber\\
so_go & 1.00000 \nonumber\\
._whoop-de-doo & 1.00000 \nonumber\\
hypocritical & 1.00000 \nonumber\\
everything_, & 1.00000 \nonumber\\
whoop-de-doo & 1.00000 \nonumber\\
._xd & 1.00000 \nonumber\\
._yet & 1.00000 \nonumber\\
evolutionism & 1.00000 \nonumber\\
creationism_, & 1.00000 \nonumber\\
yet_with & 1.00000 \nonumber\\
hypocritical_of & 1.00000 \nonumber\\
evolutionism_, & 1.00000 \nonumber\\
!_if & 1.00000 \nonumber\\
convince_of & 1.00000 \nonumber\\
xd & 1.00000 \nonumber\\
say_... & 1.00000 \nonumber\\
even_debate & 1.00000 \nonumber\\
..._maybe & 1.00000 \nonumber\\
matter_so & 1.00000 \nonumber\\
live_your & 1.00000 \nonumber\\
opponent_to & 1.00000 \nonumber\\
listen & 1.00000 \nonumber\\
sometime_, & 1.00000 \nonumber\\
ProductionRule_VP->VB,PRT,NP,SBAR, & 1.00000 \nonumber\\
tell_but & 1.00000 \nonumber\\
police_be & 1.00000 \nonumber\\
still_wrong & 1.00000 \nonumber\\
want_her & 1.00000 \nonumber\\
person_but & 1.00000 \nonumber\\
her_to & 1.00000 \nonumber\\
accident_but & 1.00000 \nonumber\\
out_who & 1.00000 \nonumber\\
wrong_to & 1.00000 \nonumber\\
wife_because & 1.00000 \nonumber\\
time_so & 1.00000 \nonumber\\
leave_me & 1.00000 \nonumber\\
not_show & 1.00000 \nonumber\\
and_dug & 1.00000 \nonumber\\
start_would & 1.00000 \nonumber\\
shld_not & 1.00000 \nonumber\\
dosage_, & 1.00000 \nonumber\\
dug_. & 1.00000 \nonumber\\
almost_kill & 1.00000 \nonumber\\
have_start & 1.00000 \nonumber\\
its_as & 1.00000 \nonumber\\
waste_energy & 1.00000 \nonumber\\
totally_crap & 1.00000 \nonumber\\
not_devote & 1.00000 \nonumber\\
increase_one & 1.00000 \nonumber\\
future_sexual & 1.00000 \nonumber\\
waste_effort & 1.00000 \nonumber\\
maturity_and & 1.00000 \nonumber\\
population_. & 1.00000 \nonumber\\
face_an & 1.00000 \nonumber\\
an_age & 1.00000 \nonumber\\
porn_would & 1.00000 \nonumber\\
and_regret & 1.00000 \nonumber\\
assault_, & 1.00000 \nonumber\\
sexual_assault & 1.00000 \nonumber\\
assault & 1.00000 \nonumber\\
most_develop & 1.00000 \nonumber\\
'_maturity & 1.00000 \nonumber\\
road_that & 1.00000 \nonumber\\
the_reality & 1.00000 \nonumber\\
a_dosage & 1.00000 \nonumber\\
urself & 1.00000 \nonumber\\
dosage & 1.00000 \nonumber\\
smoke_and & 1.00000 \nonumber\\
effort_and & 1.00000 \nonumber\\
thus_increase & 1.00000 \nonumber\\
possible_future & 1.00000 \nonumber\\
shld & 1.00000 \nonumber\\
as_smoke & 1.00000 \nonumber\\
devote_urself & 1.00000 \nonumber\\
ban_in & 1.00000 \nonumber\\
reason_its & 1.00000 \nonumber\\
expose_one & 1.00000 \nonumber\\
waste_ur & 1.00000 \nonumber\\
energy_, & 1.00000 \nonumber\\
would_expose & 1.00000 \nonumber\\
ur_time & 1.00000 \nonumber\\
,_waste & 1.00000 \nonumber\\
regret_that & 1.00000 \nonumber\\
regret & 1.00000 \nonumber\\
reality_in & 1.00000 \nonumber\\
not_ban & 1.00000 \nonumber\\
prevent_possible & 1.00000 \nonumber\\
and_prevent & 1.00000 \nonumber\\
would_almost & 1.00000 \nonumber\\
dug & 1.00000 \nonumber\\
age_population & 1.00000 \nonumber\\
urself_to & 1.00000 \nonumber\\
that_shld & 1.00000 \nonumber\\
receive & 1.00000 \nonumber\\
of_common & 1.00000 \nonumber\\
,_watch & 1.00000 \nonumber\\
_pos_ngram_PR_ADV_PUNC & 1.00000 \nonumber\\
be_her & 1.00000 \nonumber\\
an_adult & 1.00000 \nonumber\\
just_think & 1.00000 \nonumber\\
creative & 1.00000 \nonumber\\
go_both & 1.00000 \nonumber\\
accurate & 1.00000 \nonumber\\
alive_should & 1.00000 \nonumber\\
by_billion & 1.00000 \nonumber\\
it_; & 1.00000 \nonumber\\
your_merely & 1.00000 \nonumber\\
over_advance & 1.00000 \nonumber\\
be_planet & 1.00000 \nonumber\\
_pos_ngram_ADJ_O_CONJ & 1.00000 \nonumber\\
billion_, & 1.00000 \nonumber\\
greedy_and & 1.00000 \nonumber\\
share_by & 1.00000 \nonumber\\
hear_" & 1.00000 \nonumber\\
'_human & 1.00000 \nonumber\\
,_share & 1.00000 \nonumber\\
gain_over & 1.00000 \nonumber\\
live_together & 1.00000 \nonumber\\
ProductionRule_CONJP->RB,RB, & 1.00000 \nonumber\\
should_take & 1.00000 \nonumber\\
ot_hear & 1.00000 \nonumber\\
want_ot & 1.00000 \nonumber\\
ProductionRule_NP->NP,,,VP,,, & 1.00000 \nonumber\\
your_surroundings & 1.00000 \nonumber\\
up_space & 1.00000 \nonumber\\
ProductionRule_NP->NN,NNP, & 1.00000 \nonumber\\
merely_take & 1.00000 \nonumber\\
personal_gain & 1.00000 \nonumber\\
other_lame & 1.00000 \nonumber\\
individual_around & 1.00000 \nonumber\\
race_, & 1.00000 \nonumber\\
lame_excuse & 1.00000 \nonumber\\
person_alive & 1.00000 \nonumber\\
self-center & 1.00000 \nonumber\\
;_choose & 1.00000 \nonumber\\
and_self-center & 1.00000 \nonumber\\
selfish_" & 1.00000 \nonumber\\
surroundings_and & 1.00000 \nonumber\\
all_live & 1.00000 \nonumber\\
excuse_. & 1.00000 \nonumber\\
take_up & 1.00000 \nonumber\\
no_other & 1.00000 \nonumber\\
around_it & 1.00000 \nonumber\\
if_give & 1.00000 \nonumber\\
too_greedy & 1.00000 \nonumber\\
self-center_to & 1.00000 \nonumber\\
allow_some & 1.00000 \nonumber\\
fox_do & 1.00000 \nonumber\\
novanet_. & 1.00000 \nonumber\\
on_some & 1.00000 \nonumber\\
need_internet & 1.00000 \nonumber\\
novanet & 1.00000 \nonumber\\
to_install & 1.00000 \nonumber\\
like_novanet & 1.00000 \nonumber\\
such_website & 1.00000 \nonumber\\
some_website & 1.00000 \nonumber\\
website_like & 1.00000 \nonumber\\
pop-up_on & 1.00000 \nonumber\\
install_such & 1.00000 \nonumber\\
some_pop-up & 1.00000 \nonumber\\
fire_fox & 1.00000 \nonumber\\
explorer_to & 1.00000 \nonumber\\
why_million & 1.00000 \nonumber\\
damn_bloody & 1.00000 \nonumber\\
god_damn & 1.00000 \nonumber\\
aunt_or & 1.00000 \nonumber\\
and_definately & 1.00000 \nonumber\\
aunt & 1.00000 \nonumber\\
definately_a & 1.00000 \nonumber\\
why_your & 1.00000 \nonumber\\
super_great & 1.00000 \nonumber\\
girlfriend_( & 1.00000 \nonumber\\
not_sleep & 1.00000 \nonumber\\
your_girlfriend & 1.00000 \nonumber\\
your_aunt & 1.00000 \nonumber\\
uncle_be & 1.00000 \nonumber\\
uncle & 1.00000 \nonumber\\
sleep_properly & 1.00000 \nonumber\\
in_hospital & 1.00000 \nonumber\\
fat_. & 1.00000 \nonumber\\
properly_at & 1.00000 \nonumber\\
girlfriend & 1.00000 \nonumber\\
great_sex & 1.00000 \nonumber\\
bloody_yes & 1.00000 \nonumber\\
or_uncle & 1.00000 \nonumber\\
._lack & 1.00000 \nonumber\\
at_time & 1.00000 \nonumber\\
have_super & 1.00000 \nonumber\\
from_work & 1.00000 \nonumber\\
alway_agree & 1.00000 \nonumber\\
in_so & 1.00000 \nonumber\\
me_which & 1.00000 \nonumber\\
and_wait & 1.00000 \nonumber\\
ProductionRule_ADVP->RB,RB,S, & 1.00000 \nonumber\\
'_live & 1.00000 \nonumber\\
ProductionRule_VP->MD,ADVP,ADVP,VP, & 1.00000 \nonumber\\
nerve_sometime & 1.00000 \nonumber\\
own_kind & 1.00000 \nonumber\\
alway_get & 1.00000 \nonumber\\
lousy_in & 1.00000 \nonumber\\
every_dad & 1.00000 \nonumber\\
wait_for & 1.00000 \nonumber\\
get_home & 1.00000 \nonumber\\
get_along & 1.00000 \nonumber\\
do_without & 1.00000 \nonumber\\
my_nerve & 1.00000 \nonumber\\
lousy_to & 1.00000 \nonumber\\
mom_to & 1.00000 \nonumber\\
couch_, & 1.00000 \nonumber\\
a_be & 1.00000 \nonumber\\
that_pretty & 1.00000 \nonumber\\
than_me & 1.00000 \nonumber\\
wiser_in & 1.00000 \nonumber\\
home_from & 1.00000 \nonumber\\
along_, & 1.00000 \nonumber\\
dad_out & 1.00000 \nonumber\\
him_food & 1.00000 \nonumber\\
many_different & 1.00000 \nonumber\\
him_wiser & 1.00000 \nonumber\\
it_must & 1.00000 \nonumber\\
school_cloth & 1.00000 \nonumber\\
so_weird & 1.00000 \nonumber\\
there_dumb & 1.00000 \nonumber\\
more_bull & 1.00000 \nonumber\\
bull_and & 1.00000 \nonumber\\
their_so & 1.00000 \nonumber\\
also_there & 1.00000 \nonumber\\
and_gay & 1.00000 \nonumber\\
dumb_stupid & 1.00000 \nonumber\\
cloth_because & 1.00000 \nonumber\\
stupid_and & 1.00000 \nonumber\\
ProductionRule_FRAG->FRAG,CC,FRAG, & 1.00000 \nonumber\\
ProductionRule_VP->VB,IN,S, & 1.00000 \nonumber\\
instead_they & 1.00000 \nonumber\\
book_to & 1.00000 \nonumber\\
._study & 1.00000 \nonumber\\
have_telvision & 1.00000 \nonumber\\
that_telivision & 1.00000 \nonumber\\
more_stimulate & 1.00000 \nonumber\\
stimulate & 1.00000 \nonumber\\
stimulate_than & 1.00000 \nonumber\\
telvision & 1.00000 \nonumber\\
a_run & 1.00000 \nonumber\\
telvision_. & 1.00000 \nonumber\\
tv_then & 1.00000 \nonumber\\
in_gym & 1.00000 \nonumber\\
tv_keep & 1.00000 \nonumber\\
book_infront & 1.00000 \nonumber\\
gym_people & 1.00000 \nonumber\\
telivision_be & 1.00000 \nonumber\\
have_book & 1.00000 \nonumber\\
exercise_watch & 1.00000 \nonumber\\
telivision & 1.00000 \nonumber\\
on_say & 1.00000 \nonumber\\
keep_on & 1.00000 \nonumber\\
read_on & 1.00000 \nonumber\\
an_indian & 1.00000 \nonumber\\
him_he & 1.00000 \nonumber\\
better_step & 1.00000 \nonumber\\
_pos_ngram_PR_PR_ADJ & 1.00000 \nonumber\\
go_fatherless & 1.00000 \nonumber\\
teach_his & 1.00000 \nonumber\\
rather_go & 1.00000 \nonumber\\
his_kid & 1.00000 \nonumber\\
he_better & 1.00000 \nonumber\\
husband_be & 1.00000 \nonumber\\
house_a & 1.00000 \nonumber\\
okay_to & 1.00000 \nonumber\\
should_set & 1.00000 \nonumber\\
dad_i & 1.00000 \nonumber\\
lousy_? & 1.00000 \nonumber\\
a_never & 1.00000 \nonumber\\
the_dad & 1.00000 \nonumber\\
father_should & 1.00000 \nonumber\\
to_much & 1.00000 \nonumber\\
and_pe & 1.00000 \nonumber\\
our_private & 1.00000 \nonumber\\
those_so & 1.00000 \nonumber\\
gay_coach & 1.00000 \nonumber\\
be_100 & 1.00000 \nonumber\\
stupid_outfit & 1.00000 \nonumber\\
%_right & 1.00000 \nonumber\\
coach_can & 1.00000 \nonumber\\
these_stupid & 1.00000 \nonumber\\
wear_those & 1.00000 \nonumber\\
the_gay & 1.00000 \nonumber\\
outfit_. & 1.00000 \nonumber\\
wear_these & 1.00000 \nonumber\\
see_our & 1.00000 \nonumber\\
just_stupid & 1.00000 \nonumber\\
pe_and & 1.00000 \nonumber\\
coach & 1.00000 \nonumber\\
private_part & 1.00000 \nonumber\\
us_wear & 1.00000 \nonumber\\
ProductionRule_NP->DT,JJ,NNP,,,NNP, & 1.00000 \nonumber\\
that_then & 1.00000 \nonumber\\
the_quickness & 1.00000 \nonumber\\
heck_yes & 1.00000 \nonumber\\
next_victim & 1.00000 \nonumber\\
,_loco & 1.00000 \nonumber\\
insane_in & 1.00000 \nonumber\\
insane & 1.00000 \nonumber\\
brain_, & 1.00000 \nonumber\\
its_illegal & 1.00000 \nonumber\\
ProductionRule_VP->RB,VBG,S, & 1.00000 \nonumber\\
ProductionRule_NP->DT,NN,,,CC,NN, & 1.00000 \nonumber\\
then_she & 1.00000 \nonumber\\
loco & 1.00000 \nonumber\\
,_insane & 1.00000 \nonumber\\
in_with & 1.00000 \nonumber\\
illegal_and & 1.00000 \nonumber\\
loco_, & 1.00000 \nonumber\\
crazy_, & 1.00000 \nonumber\\
quickness_because & 1.00000 \nonumber\\
quickness & 1.00000 \nonumber\\
little_crazy & 1.00000 \nonumber\\
you_fall & 1.00000 \nonumber\\
wife_to & 1.00000 \nonumber\\
n't_fall & 1.00000 \nonumber\\
love_a & 1.00000 \nonumber\\
love_with & 1.00000 \nonumber\\
fall_in & 1.00000 \nonumber\\
ProductionRule_NP->DT,JJS,NNS, & 1.00000 \nonumber\\
daily & 1.00000 \nonumber\\
the_biggest & 1.00000 \nonumber\\
only_ponder & 1.00000 \nonumber\\
it_from & 1.00000 \nonumber\\
hardship_, & 1.00000 \nonumber\\
would_frustrate & 1.00000 \nonumber\\
probably_one & 1.00000 \nonumber\\
basis_would & 1.00000 \nonumber\\
to_time & 1.00000 \nonumber\\
ponder_on & 1.00000 \nonumber\\
who_on & 1.00000 \nonumber\\
by_all & 1.00000 \nonumber\\
thought_forever & 1.00000 \nonumber\\
daily_basis & 1.00000 \nonumber\\
no_knowledge & 1.00000 \nonumber\\
from_time & 1.00000 \nonumber\\
undesire & 1.00000 \nonumber\\
undesire_by & 1.00000 \nonumber\\
you_only & 1.00000 \nonumber\\
a_daily & 1.00000 \nonumber\\
,_undesire & 1.00000 \nonumber\\
frustrate_me & 1.00000 \nonumber\\
biggest_hardship & 1.00000 \nonumber\\
although_be & 1.00000 \nonumber\\
hardship & 1.00000 \nonumber\\
least_when & 1.00000 \nonumber\\
change_some & 1.00000 \nonumber\\
love_everyone & 1.00000 \nonumber\\
ProductionRule_NP->``,NN,'', & 1.00000 \nonumber\\
god_love & 1.00000 \nonumber\\
ever_wonder & 1.00000 \nonumber\\
make_" & 1.00000 \nonumber\\
one_cardinal & 1.00000 \nonumber\\
cardinal_who & 1.00000 \nonumber\\
cardinal & 1.00000 \nonumber\\
wonder_that & 1.00000 \nonumber\\
y_do & 1.00000 \nonumber\\
then_y & 1.00000 \nonumber\\
it_change & 1.00000 \nonumber\\
everyone_then & 1.00000 \nonumber\\
y & 1.00000 \nonumber\\
gay_and & 1.00000 \nonumber\\
translate_it & 1.00000 \nonumber\\
translate & 1.00000 \nonumber\\
who_translate & 1.00000 \nonumber\\
hate_gay & 1.00000 \nonumber\\
mistake.thats & 1.00000 \nonumber\\
nobody_say & 1.00000 \nonumber\\
nothing_should & 1.00000 \nonumber\\
_pos_ngram_ART_NP_ADV & 1.00000 \nonumber\\
a_mistake.thats & 1.00000 \nonumber\\
_pos_ngram_CONJ_PR_PUNC & 1.00000 \nonumber\\
ProductionRule_NP->NNP,RB,JJ,NN,NN, & 1.00000 \nonumber\\
mistake.thats_not & 1.00000 \nonumber\\
any_one & 1.00000 \nonumber\\
what_nobody & 1.00000 \nonumber\\
would_because & 1.00000 \nonumber\\
say_if & 1.00000 \nonumber\\
mistake_or & 1.00000 \nonumber\\
what_nothing & 1.00000 \nonumber\\
right_i & 1.00000 \nonumber\\
ProductionRule_NP->DT,NP,NN, & 1.00000 \nonumber\\
kill_any & 1.00000 \nonumber\\
choice_for & 1.00000 \nonumber\\
ProductionRule_VP->TO,RB,VP, & 1.00000 \nonumber\\
economize & 1.00000 \nonumber\\
for_read & 1.00000 \nonumber\\
your_money & 1.00000 \nonumber\\
economize_your & 1.00000 \nonumber\\
buy_any & 1.00000 \nonumber\\
any_device & 1.00000 \nonumber\\
device & 1.00000 \nonumber\\
you_economize & 1.00000 \nonumber\\
device_for & 1.00000 \nonumber\\
you_watch & 1.00000 \nonumber\\
but_so & 1.00000 \nonumber\\
jeans & 1.00000 \nonumber\\
amaze & 1.00000 \nonumber\\
cloth & 1.00000 \nonumber\\
especialy & 1.00000 \nonumber\\
betray_her & 1.00000 \nonumber\\
angry_and & 1.00000 \nonumber\\
betray & 1.00000 \nonumber\\
divorce_her & 1.00000 \nonumber\\
self_defence & 1.00000 \nonumber\\
what_type & 1.00000 \nonumber\\
extremely_angry & 1.00000 \nonumber\\
defence & 1.00000 \nonumber\\
n't_betray & 1.00000 \nonumber\\
murder_whether & 1.00000 \nonumber\\
wife_confide & 1.00000 \nonumber\\
her_depend & 1.00000 \nonumber\\
support_and & 1.00000 \nonumber\\
a_self & 1.00000 \nonumber\\
murder_or & 1.00000 \nonumber\\
her_trust & 1.00000 \nonumber\\
me_than & 1.00000 \nonumber\\
fun_. & 1.00000 \nonumber\\
defence_murder & 1.00000 \nonumber\\
ProductionRule_VP->VBD,PP,ADVP, & 1.00000 \nonumber\\
even_divorce & 1.00000 \nonumber\\
than_i & 1.00000 \nonumber\\
of_murder & 1.00000 \nonumber\\
ProductionRule_S->RB,ADVP,NP,VP,:, & 1.00000 \nonumber\\
then_accord & 1.00000 \nonumber\\
and_survive & 1.00000 \nonumber\\
really_sure & 1.00000 \nonumber\\
fly_would & 1.00000 \nonumber\\
the_fruit & 1.00000 \nonumber\\
ProductionRule_PP->PP,PP, & 1.00000 \nonumber\\
that_argument & 1.00000 \nonumber\\
argument_work & 1.00000 \nonumber\\
theory_the & 1.00000 \nonumber\\
work_... & 1.00000 \nonumber\\
ProductionRule_ADVP->PP,IN, & 1.00000 \nonumber\\
your_theory & 1.00000 \nonumber\\
adapt_and & 1.00000 \nonumber\\
survive_so & 1.00000 \nonumber\\
ProductionRule_PP->TO,SBAR, & 1.00000 \nonumber\\
look_good & 1.00000 \nonumber\\
physical_punishment & 1.00000 \nonumber\\
obey & 1.00000 \nonumber\\
strong_healthy & 1.00000 \nonumber\\
obey_if & 1.00000 \nonumber\\
will_soon & 1.00000 \nonumber\\
have_gain & 1.00000 \nonumber\\
gain_their & 1.00000 \nonumber\\
ProductionRule_NP->NN,PRP$,NN, & 1.00000 \nonumber\\
believe_parent & 1.00000 \nonumber\\
like_spank & 1.00000 \nonumber\\
what_best & 1.00000 \nonumber\\
agree_to & 1.00000 \nonumber\\
decide_although & 1.00000 \nonumber\\
use_physical & 1.00000 \nonumber\\
a_friendly & 1.00000 \nonumber\\
punishment_like & 1.00000 \nonumber\\
healthy_relationship & 1.00000 \nonumber\\
their_respect & 1.00000 \nonumber\\
soon_respect & 1.00000 \nonumber\\
a_strong & 1.00000 \nonumber\\
respect_them & 1.00000 \nonumber\\
parent_know & 1.00000 \nonumber\\
friendly & 1.00000 \nonumber\\
will_obey & 1.00000 \nonumber\\
although_they & 1.00000 \nonumber\\
friendly_relationship & 1.00000 \nonumber\\
parent_decide & 1.00000 \nonumber\\
though_i & 1.00000 \nonumber\\
legal_because & 1.00000 \nonumber\\
purpose_only & 1.00000 \nonumber\\
only_filter & 1.00000 \nonumber\\
1000_% & 1.00000 \nonumber\\
like_katrina & 1.00000 \nonumber\\
that_water & 1.00000 \nonumber\\
1000 & 1.00000 \nonumber\\
profit_. & 1.00000 \nonumber\\
in_emergency & 1.00000 \nonumber\\
it_pollute & 1.00000 \nonumber\\
and_unnecessary & 1.00000 \nonumber\\
emergency_situation & 1.00000 \nonumber\\
unnecessary_. & 1.00000 \nonumber\\
big_company & 1.00000 \nonumber\\
emergency_purpose & 1.00000 \nonumber\\
the_land & 1.00000 \nonumber\\
be_pollute & 1.00000 \nonumber\\
the_profit & 1.00000 \nonumber\\
katrina & 1.00000 \nonumber\\
katrina_no & 1.00000 \nonumber\\
bottle_to & 1.00000 \nonumber\\
land_and & 1.00000 \nonumber\\
only_. & 1.00000 \nonumber\\
pollute_the & 1.00000 \nonumber\\
this_water & 1.00000 \nonumber\\
believe_plastic & 1.00000 \nonumber\\
situation_like & 1.00000 \nonumber\\
have_access & 1.00000 \nonumber\\
company_get & 1.00000 \nonumber\\
those_plastic & 1.00000 \nonumber\\
pollute_land & 1.00000 \nonumber\\
bid_? & 1.00000 \nonumber\\
._other & 1.00000 \nonumber\\
?_many & 1.00000 \nonumber\\
and_big & 1.00000 \nonumber\\
people_believe & 1.00000 \nonumber\\
it_provide & 1.00000 \nonumber\\
get_1000 & 1.00000 \nonumber\\
to_tap & 1.00000 \nonumber\\
certain_limit & 1.00000 \nonumber\\
off_material & 1.00000 \nonumber\\
stressful & 1.00000 \nonumber\\
have_' & 1.00000 \nonumber\\
less_stressful & 1.00000 \nonumber\\
prevent_people & 1.00000 \nonumber\\
cool_' & 1.00000 \nonumber\\
good_within & 1.00000 \nonumber\\
non-uniform & 1.00000 \nonumber\\
wealth_/ & 1.00000 \nonumber\\
allow_colour & 1.00000 \nonumber\\
'_cool & 1.00000 \nonumber\\
within_certain & 1.00000 \nonumber\\
from_show & 1.00000 \nonumber\\
'_good & 1.00000 \nonumber\\
colour_sock & 1.00000 \nonumber\\
-_prevent & 1.00000 \nonumber\\
leveler & 1.00000 \nonumber\\
leveler_- & 1.00000 \nonumber\\
sock & 1.00000 \nonumber\\
too_far & 1.00000 \nonumber\\
sock_, & 1.00000 \nonumber\\
material_wealth & 1.00000 \nonumber\\
a_leveler & 1.00000 \nonumber\\
stressful_than & 1.00000 \nonumber\\
/_make & 1.00000 \nonumber\\
'_stuff & 1.00000 \nonumber\\
non-uniform_college & 1.00000 \nonumber\\
stuff_. & 1.00000 \nonumber\\
'd_argue & 1.00000 \nonumber\\
end_, & 1.00000 \nonumber\\
far_less & 1.00000 \nonumber\\
than_non-uniform & 1.00000 \nonumber\\
"_t & 1.00000 \nonumber\\
ProductionRule_NP->ADVP,JJ,``,NN, & 1.00000 \nonumber\\
extensive & 1.00000 \nonumber\\
fit_2 & 1.00000 \nonumber\\
_pos_ngram_CARD_NP_ART & 1.00000 \nonumber\\
coz_sme & 1.00000 \nonumber\\
ProductionRule_SINV->PP,VP,NP, & 1.00000 \nonumber\\
cz_phy & 1.00000 \nonumber\\
ed_must & 1.00000 \nonumber\\
_pos_ngram_ADV_ADJ_CARD & 1.00000 \nonumber\\
_pos_ngram_ADJ_CARD_NP & 1.00000 \nonumber\\
b_compulsory & 1.00000 \nonumber\\
cz & 1.00000 \nonumber\\
ProductionRule_NP->CD,NNP, & 1.00000 \nonumber\\
the_extensive & 1.00000 \nonumber\\
of_cz & 1.00000 \nonumber\\
but_mustn & 1.00000 \nonumber\\
du_the & 1.00000 \nonumber\\
compulsory_coz & 1.00000 \nonumber\\
not_fit & 1.00000 \nonumber\\
2_du & 1.00000 \nonumber\\
extensive_exersise & 1.00000 \nonumber\\
exersise_perfome & 1.00000 \nonumber\\
exersise & 1.00000 \nonumber\\
mustn_" & 1.00000 \nonumber\\
mustn & 1.00000 \nonumber\\
sme & 1.00000 \nonumber\\
sme_of & 1.00000 \nonumber\\
du & 1.00000 \nonumber\\
t_b & 1.00000 \nonumber\\
that_let & 1.00000 \nonumber\\
back_you & 1.00000 \nonumber\\
whack_help & 1.00000 \nonumber\\
whack & 1.00000 \nonumber\\
of_whack & 1.00000 \nonumber\\
before_other & 1.00000 \nonumber\\
singapore_from & 1.00000 \nonumber\\
_pos_ngram_NN_NN_NP & 1.00000 \nonumber\\
good_one & 1.00000 \nonumber\\
have_me & 1.00000 \nonumber\\
name_, & 1.00000 \nonumber\\
one_btw & 1.00000 \nonumber\\
btw_. & 1.00000 \nonumber\\
_pos_ngram_PUNC_ADJ_CARD & 1.00000 \nonumber\\
,_seriously & 1.00000 \nonumber\\
adrian & 1.00000 \nonumber\\
you_my & 1.00000 \nonumber\\
peterson_? & 1.00000 \nonumber\\
peterson & 1.00000 \nonumber\\
adrian_peterson & 1.00000 \nonumber\\
seriously_? & 1.00000 \nonumber\\
not_then & 1.00000 \nonumber\\
your_name & 1.00000 \nonumber\\
your_speech & 1.00000 \nonumber\\
._good & 1.00000 \nonumber\\
me_convince & 1.00000 \nonumber\\
etc_. & 1.00000 \nonumber\\
unnecessary & 1.00000 \nonumber\\
wat & 1.00000 \nonumber\\
close_friend & 1.00000 \nonumber\\
for_do & 1.00000 \nonumber\\
your_consequence & 1.00000 \nonumber\\
friend_? & 1.00000 \nonumber\\
better_you & 1.00000 \nonumber\\
somebody_kill & 1.00000 \nonumber\\
explain_" & 1.00000 \nonumber\\
plain_wrong & 1.00000 \nonumber\\
member_or & 1.00000 \nonumber\\
punish_? & 1.00000 \nonumber\\
so_for & 1.00000 \nonumber\\
would_explain & 1.00000 \nonumber\\
if_somebody & 1.00000 \nonumber\\
a_close & 1.00000 \nonumber\\
consequence_' & 1.00000 \nonumber\\
me_the & 1.00000 \nonumber\\
ProductionRule_PP->IN,NP,NP, & 1.00000 \nonumber\\
never_there & 1.00000 \nonumber\\
(_anyway & 1.00000 \nonumber\\
kill_herself & 1.00000 \nonumber\\
in_attempt & 1.00000 \nonumber\\
'_choice & 1.00000 \nonumber\\
control_her & 1.00000 \nonumber\\
her_baby & 1.00000 \nonumber\\
u_know & 1.00000 \nonumber\\
anyway_how & 1.00000 \nonumber\\
not_control & 1.00000 \nonumber\\
know_she & 1.00000 \nonumber\\
although_it & 1.00000 \nonumber\\
complex & 1.00000 \nonumber\\
be_" & 1.00000 \nonumber\\
and_really & 1.00000 \nonumber\\
to_birth & 1.00000 \nonumber\\
ignore_fact & 1.00000 \nonumber\\
best_choice & 1.00000 \nonumber\\
ProductionRule_VP->VBD,NP,PRT,PP, & 1.00000 \nonumber\\
:_adoption & 1.00000 \nonumber\\
be_absolutley & 1.00000 \nonumber\\
then_put & 1.00000 \nonumber\\
could_continue & 1.00000 \nonumber\\
far_the & 1.00000 \nonumber\\
by_far & 1.00000 \nonumber\\
commonly_ignore & 1.00000 \nonumber\\
continue_through & 1.00000 \nonumber\\
one_word & 1.00000 \nonumber\\
fact_in & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,ADVP,NP,S, & 1.00000 \nonumber\\
abortion_when & 1.00000 \nonumber\\
through_to & 1.00000 \nonumber\\
receive_an & 1.00000 \nonumber\\
birth_and & 1.00000 \nonumber\\
abortion_debate & 1.00000 \nonumber\\
absolutley_no & 1.00000 \nonumber\\
adoption_there & 1.00000 \nonumber\\
actually_believe & 1.00000 \nonumber\\
same_sex & 1.00000 \nonumber\\
definition & 1.00000 \nonumber\\
live_longer & 1.00000 \nonumber\\
really_good & 1.00000 \nonumber\\
would_stick & 1.00000 \nonumber\\
ProductionRule_VP->VB,NP,,,S, & 1.00000 \nonumber\\
again_regard & 1.00000 \nonumber\\
or_dont & 1.00000 \nonumber\\
mean_each & 1.00000 \nonumber\\
wish_whether & 1.00000 \nonumber\\
once_again & 1.00000 \nonumber\\
regard_the & 1.00000 \nonumber\\
think_each & 1.00000 \nonumber\\
therus & 1.00000 \nonumber\\
think_once & 1.00000 \nonumber\\
own_wish & 1.00000 \nonumber\\
have_therus & 1.00000 \nonumber\\
to_or & 1.00000 \nonumber\\
therus_own & 1.00000 \nonumber\\
each_principal & 1.00000 \nonumber\\
each_person & 1.00000 \nonumber\\
should_think & 1.00000 \nonumber\\
principal & 1.00000 \nonumber\\
principal_should & 1.00000 \nonumber\\
girl/woman & 1.00000 \nonumber\\
girl/woman_get & 1.00000 \nonumber\\
'_her & 1.00000 \nonumber\\
a_girl/woman & 1.00000 \nonumber\\
fault_for & 1.00000 \nonumber\\
prepare_. & 1.00000 \nonumber\\
;_if & 1.00000 \nonumber\\
young_teen & 1.00000 \nonumber\\
fair_that & 1.00000 \nonumber\\
teen_have & 1.00000 \nonumber\\
her_fault & 1.00000 \nonumber\\
situation_; & 1.00000 \nonumber\\
teen & 1.00000 \nonumber\\
not_fair & 1.00000 \nonumber\\
depend_the & 1.00000 \nonumber\\
community_. & 1.00000 \nonumber\\
see_what & 1.00000 \nonumber\\
believe_its & 1.00000 \nonumber\\
_pos_ngram_CONJ_ART_PUNC & 1.00000 \nonumber\\
people_i & 1.00000 \nonumber\\
my_goal & 1.00000 \nonumber\\
if_im & 1.00000 \nonumber\\
give_my & 1.00000 \nonumber\\
about_most & 1.00000 \nonumber\\
alway_dream & 1.00000 \nonumber\\
me_even & 1.00000 \nonumber\\
just_feel & 1.00000 \nonumber\\
i_may & 1.00000 \nonumber\\
someday & 1.00000 \nonumber\\
family_what & 1.00000 \nonumber\\
then_someday & 1.00000 \nonumber\\
myself_instead & 1.00000 \nonumber\\
ProductionRule_S->RB,ADVP,NP,VP,., & 1.00000 \nonumber\\
i_care & 1.00000 \nonumber\\
return_help & 1.00000 \nonumber\\
i_focus & 1.00000 \nonumber\\
about_in & 1.00000 \nonumber\\
reason_really & 1.00000 \nonumber\\
for_myself & 1.00000 \nonumber\\
goal_then & 1.00000 \nonumber\\
someday_i & 1.00000 \nonumber\\
im_look & 1.00000 \nonumber\\
choice_that & 1.00000 \nonumber\\
can_just & 1.00000 \nonumber\\
discipline_it & 1.00000 \nonumber\\
get_mad & 1.00000 \nonumber\\
mad_than & 1.00000 \nonumber\\
profit_ha & 1.00000 \nonumber\\
longer_well & 1.00000 \nonumber\\
fun_with & 1.00000 \nonumber\\
money_or & 1.00000 \nonumber\\
want_money & 1.00000 \nonumber\\
water_have & 1.00000 \nonumber\\
ha_you & 1.00000 \nonumber\\
well_without & 1.00000 \nonumber\\
without_water & 1.00000 \nonumber\\
that_better & 1.00000 \nonumber\\
child_just & 1.00000 \nonumber\\
ProductionRule_S->ADVP,ADVP,NP,VP,., & 1.00000 \nonumber\\
take_, & 1.00000 \nonumber\\
uncomfortable_, & 1.00000 \nonumber\\
express_his/her & 1.00000 \nonumber\\
n't_force & 1.00000 \nonumber\\
very_uncomfortable & 1.00000 \nonumber\\
also_very & 1.00000 \nonumber\\
that_wear & 1.00000 \nonumber\\
during_winter & 1.00000 \nonumber\\
and_during & 1.00000 \nonumber\\
time_might & 1.00000 \nonumber\\
winter & 1.00000 \nonumber\\
cold_as & 1.00000 \nonumber\\
force_student & 1.00000 \nonumber\\
might_very & 1.00000 \nonumber\\
winter_time & 1.00000 \nonumber\\
very_cold & 1.00000 \nonumber\\
his/her_individuality & 1.00000 \nonumber\\
hand_out & 1.00000 \nonumber\\
hold_your & 1.00000 \nonumber\\
receive_. & 1.00000 \nonumber\\
endeavor_, & 1.00000 \nonumber\\
help_then & 1.00000 \nonumber\\
give_other & 1.00000 \nonumber\\
in_help & 1.00000 \nonumber\\
give_then & 1.00000 \nonumber\\
you_hold & 1.00000 \nonumber\\
pursuit_of & 1.00000 \nonumber\\
seem_like & 1.00000 \nonumber\\
world_doesnt & 1.00000 \nonumber\\
say_like & 1.00000 \nonumber\\
it_!!!!!!! & 1.00000 \nonumber\\
this_..... & 1.00000 \nonumber\\
ProductionRule_FRAG->NP,:,S, & 1.00000 \nonumber\\
produce_more & 1.00000 \nonumber\\
r_say & 1.00000 \nonumber\\
....._do & 1.00000 \nonumber\\
be_utillise & 1.00000 \nonumber\\
and_blame & 1.00000 \nonumber\\
....._the & 1.00000 \nonumber\\
ProductionRule_FRAG->FRAG,:,FRAG, & 1.00000 \nonumber\\
ProductionRule_FRAG->X,NP, & 1.00000 \nonumber\\
....._other & 1.00000 \nonumber\\
seem_as & 1.00000 \nonumber\\
ProductionRule_X->X,PP, & 1.00000 \nonumber\\
more_pollution & 1.00000 \nonumber\\
of_food & 1.00000 \nonumber\\
for_feed & 1.00000 \nonumber\\
waste_can & 1.00000 \nonumber\\
population_... & 1.00000 \nonumber\\
pollution_and & 1.00000 \nonumber\\
america_which & 1.00000 \nonumber\\
eat_less & 1.00000 \nonumber\\
food_they & 1.00000 \nonumber\\
feed_whole & 1.00000 \nonumber\\
aah_... & 1.00000 \nonumber\\
blame_us & 1.00000 \nonumber\\
it_eat & 1.00000 \nonumber\\
quality_..... & 1.00000 \nonumber\\
as_lead & 1.00000 \nonumber\\
have_this & 1.00000 \nonumber\\
utillise_for & 1.00000 \nonumber\\
aah & 1.00000 \nonumber\\
waste_more & 1.00000 \nonumber\\
it_produce & 1.00000 \nonumber\\
whole_indian & 1.00000 \nonumber\\
doesnt_have & 1.00000 \nonumber\\
indian_population & 1.00000 \nonumber\\
us_... & 1.00000 \nonumber\\
bid_quality & 1.00000 \nonumber\\
utillise & 1.00000 \nonumber\\
thing_..... & 1.00000 \nonumber\\
u_r & 1.00000 \nonumber\\
ProductionRule_NP->VBG,JJ,JJ,NN, & 1.00000 \nonumber\\
country_donot & 1.00000 \nonumber\\
which_seem & 1.00000 \nonumber\\
be_easily & 1.00000 \nonumber\\
of_site & 1.00000 \nonumber\\
the_breadth & 1.00000 \nonumber\\
element & 1.00000 \nonumber\\
to_suit & 1.00000 \nonumber\\
more_involve & 1.00000 \nonumber\\
extension_i & 1.00000 \nonumber\\
easily_to & 1.00000 \nonumber\\
easily_remodel & 1.00000 \nonumber\\
element_of & 1.00000 \nonumber\\
suit_my & 1.00000 \nonumber\\
critical_advantage & 1.00000 \nonumber\\
firefox_very & 1.00000 \nonumber\\
need_as & 1.00000 \nonumber\\
an_html & 1.00000 \nonumber\\
ProductionRule_VP->NN,NP,ADVP, & 1.00000 \nonumber\\
picker & 1.00000 \nonumber\\
picker_instead & 1.00000 \nonumber\\
get_them & 1.00000 \nonumber\\
of_ff & 1.00000 \nonumber\\
great_seo & 1.00000 \nonumber\\
my_need & 1.00000 \nonumber\\
my_new & 1.00000 \nonumber\\
site_development & 1.00000 \nonumber\\
need_great & 1.00000 \nonumber\\
html_color & 1.00000 \nonumber\\
html & 1.00000 \nonumber\\
seo_extension & 1.00000 \nonumber\\
seo & 1.00000 \nonumber\\
browse_need & 1.00000 \nonumber\\
critical & 1.00000 \nonumber\\
breadth & 1.00000 \nonumber\\
ff_add-on & 1.00000 \nonumber\\
other_element & 1.00000 \nonumber\\
new_browse & 1.00000 \nonumber\\
a_critical & 1.00000 \nonumber\\
and_variety & 1.00000 \nonumber\\
reconfigure & 1.00000 \nonumber\\
need_an & 1.00000 \nonumber\\
reconfigure_firefox & 1.00000 \nonumber\\
color_picker & 1.00000 \nonumber\\
can_reconfigure & 1.00000 \nonumber\\
very_easily & 1.00000 \nonumber\\
remodel_to & 1.00000 \nonumber\\
add-on_be & 1.00000 \nonumber\\
breadth_and & 1.00000 \nonumber\\
instead_when & 1.00000 \nonumber\\
ProductionRule_ADVP->RB,RB,SBAR, & 1.00000 \nonumber\\
,_ff & 1.00000 \nonumber\\
life_change & 1.00000 \nonumber\\
and/or & 1.00000 \nonumber\\
ProductionRule_PP->NP,IN,NP, & 1.00000 \nonumber\\
life_without & 1.00000 \nonumber\\
without_any & 1.00000 \nonumber\\
or_get & 1.00000 \nonumber\\
law_. & 1.00000 \nonumber\\
me_gay & 1.00000 \nonumber\\
opinion_but & 1.00000 \nonumber\\
my_moral & 1.00000 \nonumber\\
an_unnatural & 1.00000 \nonumber\\
against_my & 1.00000 \nonumber\\
other_opinion & 1.00000 \nonumber\\
moral_law & 1.00000 \nonumber\\
unnatural_way & 1.00000 \nonumber\\
i_respect & 1.00000 \nonumber\\
but_woppen & 1.00000 \nonumber\\
woppen_then & 1.00000 \nonumber\\
it_show & 1.00000 \nonumber\\
woppen & 1.00000 \nonumber\\
_pos_ngram_ART_CONJ_NN & 1.00000 \nonumber\\
show_then & 1.00000 \nonumber\\
the_feel & 1.00000 \nonumber\\
mistake_twice & 1.00000 \nonumber\\
you_child & 1.00000 \nonumber\\
spank_you & 1.00000 \nonumber\\
a_but & 1.00000 \nonumber\\
ProductionRule_NP->DT,VP,NN, & 1.00000 \nonumber\\
wont_make & 1.00000 \nonumber\\
insecure & 1.00000 \nonumber\\
low_level & 1.00000 \nonumber\\
of_lousy & 1.00000 \nonumber\\
just_fine & 1.00000 \nonumber\\
me_) & 1.00000 \nonumber\\
a_insecure & 1.00000 \nonumber\\
topic_in & 1.00000 \nonumber\\
like_would & 1.00000 \nonumber\\
it_better & 1.00000 \nonumber\\
would_( & 1.00000 \nonumber\\
consider_my & 1.00000 \nonumber\\
exist_would & 1.00000 \nonumber\\
level_of & 1.00000 \nonumber\\
insecure_topic & 1.00000 \nonumber\\
modern & 1.00000 \nonumber\\
._uniform & 1.00000 \nonumber\\
to_another & 1.00000 \nonumber\\
much_about & 1.00000 \nonumber\\
pepsi & 1.00000 \nonumber\\
aquafina & 1.00000 \nonumber\\
another_700 & 1.00000 \nonumber\\
worth_make & 1.00000 \nonumber\\
ProductionRule_NP->DT,VBG,JJ,NN, & 1.00000 \nonumber\\
industry_, & 1.00000 \nonumber\\
usage & 1.00000 \nonumber\\
lead_corporate & 1.00000 \nonumber\\
these_bottle & 1.00000 \nonumber\\
although_maybe & 1.00000 \nonumber\\
decompose_for & 1.00000 \nonumber\\
maybe_a & 1.00000 \nonumber\\
it_already & 1.00000 \nonumber\\
corporate_industry & 1.00000 \nonumber\\
environment_worse & 1.00000 \nonumber\\
ProductionRule_S->NP,,,SBAR,,,VP,., & 1.00000 \nonumber\\
corporate & 1.00000 \nonumber\\
usage_, & 1.00000 \nonumber\\
bottle_will & 1.00000 \nonumber\\
bottle_usage & 1.00000 \nonumber\\
like_and & 1.00000 \nonumber\\
teenager & 1.00000 \nonumber\\
_pos_ngram_PR_ART_NP & 1.00000 \nonumber\\
,_your & 1.00000 \nonumber\\
then_1 & 1.00000 \nonumber\\
can_change & 1.00000 \nonumber\\
compulsory & 1.00000 \nonumber\\
thing_easier & 1.00000 \nonumber\\
a_sleeker & 1.00000 \nonumber\\
ie_because & 1.00000 \nonumber\\
internet_user & 1.00000 \nonumber\\
it_my & 1.00000 \nonumber\\
after_my & 1.00000 \nonumber\\
a_casual & 1.00000 \nonumber\\
again_after & 1.00000 \nonumber\\
brother_make & 1.00000 \nonumber\\
bookmark & 1.00000 \nonumber\\
firefox_though & 1.00000 \nonumber\\
bookmark/history & 1.00000 \nonumber\\
my_bookmark & 1.00000 \nonumber\\
prefer_ie & 1.00000 \nonumber\\
transfer_my & 1.00000 \nonumber\\
transfer & 1.00000 \nonumber\\
sleeker_design & 1.00000 \nonumber\\
design_, & 1.00000 \nonumber\\
the_bookmark/history & 1.00000 \nonumber\\
user_, & 1.00000 \nonumber\\
,_cuz & 1.00000 \nonumber\\
to_transfer & 1.00000 \nonumber\\
bookmark/history_thing & 1.00000 \nonumber\\
bookmark_again & 1.00000 \nonumber\\
my_default & 1.00000 \nonumber\\
casual_internet & 1.00000 \nonumber\\
maybe_it & 1.00000 \nonumber\\
ProductionRule_NP->NN,NN,NNS, & 1.00000 \nonumber\\
natural & 1.00000 \nonumber\\
not_need & 1.00000 \nonumber\\
great_argument & 1.00000 \nonumber\\
browser_... & 1.00000 \nonumber\\
argument_why & 1.00000 \nonumber\\
why_ie & 1.00000 \nonumber\\
..._not & 1.00000 \nonumber\\
really_great & 1.00000 \nonumber\\
model_to & 1.00000 \nonumber\\
both_. & 1.00000 \nonumber\\
of_both & 1.00000 \nonumber\\
bestow & 1.00000 \nonumber\\
bestow_death & 1.00000 \nonumber\\
ProductionRule_NP->NP,SBAR,,, & 1.00000 \nonumber\\
whom_bestow & 1.00000 \nonumber\\
bestow_life & 1.00000 \nonumber\\
one_whom & 1.00000 \nonumber\\
'_population & 1.00000 \nonumber\\
be_indirectly & 1.00000 \nonumber\\
farquhar_when & 1.00000 \nonumber\\
be_adopt & 1.00000 \nonumber\\
best_interest & 1.00000 \nonumber\\
interest_of & 1.00000 \nonumber\\
believe_farquhar & 1.00000 \nonumber\\
population_at & 1.00000 \nonumber\\
raffle_sack & 1.00000 \nonumber\\
sack_him & 1.00000 \nonumber\\
sack_farquhar & 1.00000 \nonumber\\
at_heart & 1.00000 \nonumber\\
measure_that & 1.00000 \nonumber\\
harmful_to & 1.00000 \nonumber\\
indirectly_harmful & 1.00000 \nonumber\\
die_. & 1.00000 \nonumber\\
'_other & 1.00000 \nonumber\\
them_behave & 1.00000 \nonumber\\
behave_. & 1.00000 \nonumber\\
a_couple & 1.00000 \nonumber\\
theyre_not & 1.00000 \nonumber\\
keep_you & 1.00000 \nonumber\\
not_expensive & 1.00000 \nonumber\\
recycle_to & 1.00000 \nonumber\\
buck_for & 1.00000 \nonumber\\
like_more & 1.00000 \nonumber\\
big_pack & 1.00000 \nonumber\\
3_buck & 1.00000 \nonumber\\
shaw & 1.00000 \nonumber\\
pack & 1.00000 \nonumber\\
pack_at & 1.00000 \nonumber\\
shaw_. & 1.00000 \nonumber\\
at_shaw & 1.00000 \nonumber\\
company_rich & 1.00000 \nonumber\\
._theyre & 1.00000 \nonumber\\
will_keep & 1.00000 \nonumber\\
buck & 1.00000 \nonumber\\
more_water & 1.00000 \nonumber\\
for_pocket & 1.00000 \nonumber\\
also_make & 1.00000 \nonumber\\
you_un-thirsty & 1.00000 \nonumber\\
un-thirsty_for & 1.00000 \nonumber\\
pocket_change & 1.00000 \nonumber\\
un-thirsty & 1.00000 \nonumber\\
like_3 & 1.00000 \nonumber\\
week_for & 1.00000 \nonumber\\
couple_week & 1.00000 \nonumber\\
huge_amount & 1.00000 \nonumber\\
be_sorry & 1.00000 \nonumber\\
less_time & 1.00000 \nonumber\\
an_ie & 1.00000 \nonumber\\
that_when & 1.00000 \nonumber\\
look_unatrel & 1.00000 \nonumber\\
unatrel & 1.00000 \nonumber\\
unatrel_and & 1.00000 \nonumber\\
ProductionRule_ADJP->JJ,JJ, & 1.00000 \nonumber\\
band_school & 1.00000 \nonumber\\
not_express & 1.00000 \nonumber\\
yourself_enough & 1.00000 \nonumber\\
enough_so & 1.00000 \nonumber\\
so_band & 1.00000 \nonumber\\
uniform_because & 1.00000 \nonumber\\
band & 1.00000 \nonumber\\
uniform_ok & 1.00000 \nonumber\\
expand & 1.00000 \nonumber\\
their_act & 1.00000 \nonumber\\
use_way & 1.00000 \nonumber\\
better_get & 1.00000 \nonumber\\
gut_. & 1.00000 \nonumber\\
system_' & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,ADJP,ADVP, & 1.00000 \nonumber\\
once_everyone & 1.00000 \nonumber\\
to_switch & 1.00000 \nonumber\\
pc_, & 1.00000 \nonumber\\
new_pc & 1.00000 \nonumber\\
so_bloat & 1.00000 \nonumber\\
a_web & 1.00000 \nonumber\\
gut_from & 1.00000 \nonumber\\
it_use & 1.00000 \nonumber\\
all_my & 1.00000 \nonumber\\
bloat & 1.00000 \nonumber\\
excuse_to & 1.00000 \nonumber\\
bloat_now & 1.00000 \nonumber\\
bloat_netscape & 1.00000 \nonumber\\
more_memory & 1.00000 \nonumber\\
mozillium & 1.00000 \nonumber\\
'_memory & 1.00000 \nonumber\\
web_browser & 1.00000 \nonumber\\
get_get & 1.00000 \nonumber\\
everyone_buy & 1.00000 \nonumber\\
get_gut & 1.00000 \nonumber\\
netscape & 1.00000 \nonumber\\
netscape_. & 1.00000 \nonumber\\
firefox_better & 1.00000 \nonumber\\
firefox_need & 1.00000 \nonumber\\
get_ie7 & 1.00000 \nonumber\\
act_together & 1.00000 \nonumber\\
way_more & 1.00000 \nonumber\\
a_bloat & 1.00000 \nonumber\\
_pos_ngram_PP_NP_PR & 1.00000 \nonumber\\
ie7_, & 1.00000 \nonumber\\
like_mozillium & 1.00000 \nonumber\\
use_a & 1.00000 \nonumber\\
gut & 1.00000 \nonumber\\
no_excuse & 1.00000 \nonumber\\
mozillium_who & 1.00000 \nonumber\\
opera_it & 1.00000 \nonumber\\
as_adobe & 1.00000 \nonumber\\
browser_i & 1.00000 \nonumber\\
opera_which & 1.00000 \nonumber\\
smoothly & 1.00000 \nonumber\\
load_from & 1.00000 \nonumber\\
smoothly_. & 1.00000 \nonumber\\
opera & 1.00000 \nonumber\\
use_opera & 1.00000 \nonumber\\
fx & 1.00000 \nonumber\\
but_ffx & 1.00000 \nonumber\\
fx_unlike & 1.00000 \nonumber\\
the_flash & 1.00000 \nonumber\\
unlike & 1.00000 \nonumber\\
unlike_in & 1.00000 \nonumber\\
i_frequently & 1.00000 \nonumber\\
use_such & 1.00000 \nonumber\\
unlike_the & 1.00000 \nonumber\\
opera_be & 1.00000 \nonumber\\
which_play & 1.00000 \nonumber\\
plug-in_i & 1.00000 \nonumber\\
3_yr & 1.00000 \nonumber\\
seconds & 1.00000 \nonumber\\
start_. & 1.00000 \nonumber\\
start_fast & 1.00000 \nonumber\\
start_it & 1.00000 \nonumber\\
ffx_have & 1.00000 \nonumber\\
ffx_. & 1.00000 \nonumber\\
ffx & 1.00000 \nonumber\\
often_stop & 1.00000 \nonumber\\
my_3 & 1.00000 \nonumber\\
in_ffx & 1.00000 \nonumber\\
in_fx & 1.00000 \nonumber\\
disk & 1.00000 \nonumber\\
disk_. & 1.00000 \nonumber\\
still_young & 1.00000 \nonumber\\
fast_when & 1.00000 \nonumber\\
perfrom_well & 1.00000 \nonumber\\
perfrom & 1.00000 \nonumber\\
stop_in & 1.00000 \nonumber\\
in_opera & 1.00000 \nonumber\\
adobe & 1.00000 \nonumber\\
adobe_flash & 1.00000 \nonumber\\
more_seconds & 1.00000 \nonumber\\
lastly_, & 1.00000 \nonumber\\
lastly & 1.00000 \nonumber\\
young_. & 1.00000 \nonumber\\
not_perfrom & 1.00000 \nonumber\\
movie_smoothly & 1.00000 \nonumber\\
movie_often & 1.00000 \nonumber\\
yr_old & 1.00000 \nonumber\\
,_unlike & 1.00000 \nonumber\\
seconds_to & 1.00000 \nonumber\\
me_opera & 1.00000 \nonumber\\
of_issue & 1.00000 \nonumber\\
frequently_use & 1.00000 \nonumber\\
._plug-in & 1.00000 \nonumber\\
take_about & 1.00000 \nonumber\\
flash_player & 1.00000 \nonumber\\
computer_, & 1.00000 \nonumber\\
flash_movie & 1.00000 \nonumber\\
flash & 1.00000 \nonumber\\
._lastly & 1.00000 \nonumber\\
plug-in & 1.00000 \nonumber\\
frequently & 1.00000 \nonumber\\
player_do & 1.00000 \nonumber\\
about_10 & 1.00000 \nonumber\\
player & 1.00000 \nonumber\\
play_flash & 1.00000 \nonumber\\
issue_first & 1.00000 \nonumber\\
10_or & 1.00000 \nonumber\\
old_computer & 1.00000 \nonumber\\
the_disk & 1.00000 \nonumber\\
the_view & 1.00000 \nonumber\\
very_comfortable & 1.00000 \nonumber\\
comfortable_. & 1.00000 \nonumber\\
every_teenager & 1.00000 \nonumber\\
the_type & 1.00000 \nonumber\\
_pos_ngram_V_NP_CARD & 1.00000 \nonumber\\
and_waste & 1.00000 \nonumber\\
or_3 & 1.00000 \nonumber\\
2_or & 1.00000 \nonumber\\
3_week & 1.00000 \nonumber\\
ProductionRule_NP->CD,CC,CD,NNS, & 1.00000 \nonumber\\
week_or & 1.00000 \nonumber\\
spank_would & 1.00000 \nonumber\\
could_last & 1.00000 \nonumber\\
but_punish & 1.00000 \nonumber\\
maybe_more & 1.00000 \nonumber\\
minute_, & 1.00000 \nonumber\\
a_minute & 1.00000 \nonumber\\
ProductionRule_NP->RB,JJR, & 1.00000 \nonumber\\
or_maybe & 1.00000 \nonumber\\
would_last & 1.00000 \nonumber\\
last_just & 1.00000 \nonumber\\
to_2 & 1.00000 \nonumber\\
necessary_, & 1.00000 \nonumber\\
punish_could & 1.00000 \nonumber\\
last_up & 1.00000 \nonumber\\
ProductionRule_NP->PDT,DT,JJ,NNS, & 1.00000 \nonumber\\
just_karma & 1.00000 \nonumber\\
somehow_, & 1.00000 \nonumber\\
karma & 1.00000 \nonumber\\
will_eventually & 1.00000 \nonumber\\
world_somehow & 1.00000 \nonumber\\
karma_. & 1.00000 \nonumber\\
you_out & 1.00000 \nonumber\\
fame_or & 1.00000 \nonumber\\
_pos_ngram_PR_ADJ_ART & 1.00000 \nonumber\\
some_way & 1.00000 \nonumber\\
ProductionRule_VP->VB,ADVP,PP,ADVP, & 1.00000 \nonumber\\
be_money & 1.00000 \nonumber\\
somehow & 1.00000 \nonumber\\
eventually_come & 1.00000 \nonumber\\
you_anyway & 1.00000 \nonumber\\
a_young & 1.00000 \nonumber\\
suffer & 1.00000 \nonumber\\
ProductionRule_NP->RB,JJ, & 1.00000 \nonumber\\
ff_come & 1.00000 \nonumber\\
preinstall & 1.00000 \nonumber\\
ie_will & 1.00000 \nonumber\\
in_pc & 1.00000 \nonumber\\
dominate_. & 1.00000 \nonumber\\
ProductionRule_SINV->PP,VP,NP,., & 1.00000 \nonumber\\
pc_.... & 1.00000 \nonumber\\
preinstall_in & 1.00000 \nonumber\\
till_there & 1.00000 \nonumber\\
enuff_say & 1.00000 \nonumber\\
enuff & 1.00000 \nonumber\\
...._ie & 1.00000 \nonumber\\
._enuff & 1.00000 \nonumber\\
to_dominate & 1.00000 \nonumber\\
come_preinstall & 1.00000 \nonumber\\
there_come & 1.00000 \nonumber\\
point_that & 1.00000 \nonumber\\
ProductionRule_SBAR->IN,S,., & 1.00000 \nonumber\\
those_we & 1.00000 \nonumber\\
bottle_all & 1.00000 \nonumber\\
without_those & 1.00000 \nonumber\\
block_with & 1.00000 \nonumber\\
safe_suply & 1.00000 \nonumber\\
suply & 1.00000 \nonumber\\
day_guy & 1.00000 \nonumber\\
comfortabley & 1.00000 \nonumber\\
guy_, & 1.00000 \nonumber\\
the_block & 1.00000 \nonumber\\
could_comfortabley & 1.00000 \nonumber\\
comfortabley_walk & 1.00000 \nonumber\\
day_every & 1.00000 \nonumber\\
ProductionRule_NP->NP,NP,,,PP, & 1.00000 \nonumber\\
suply_of & 1.00000 \nonumber\\
our_hand & 1.00000 \nonumber\\
_pos_ngram_NN_CONJ_CONJ & 1.00000 \nonumber\\
ever & 1.00000 \nonumber\\
deal_! & 1.00000 \nonumber\\
no_bid & 1.00000 \nonumber\\
water_next & 1.00000 \nonumber\\
its_no & 1.00000 \nonumber\\
ProductionRule_ADVP->JJ,PP, & 1.00000 \nonumber\\
ProductionRule_S->S,., & 1.00000 \nonumber\\
a_bottle & 1.00000 \nonumber\\
bid_deal & 1.00000 \nonumber\\
yeah_i & 1.00000 \nonumber\\
,_parent & 1.00000 \nonumber\\
which_a & 1.00000 \nonumber\\
weaker & 1.00000 \nonumber\\
idea_, & 1.00000 \nonumber\\
the_damage & 1.00000 \nonumber\\
imagine_thing & 1.00000 \nonumber\\
reduce_learn & 1.00000 \nonumber\\
ProductionRule_VP->ADVP,VBP,NP, & 1.00000 \nonumber\\
and_creativity & 1.00000 \nonumber\\
obesity_as & 1.00000 \nonumber\\
someone_imagination & 1.00000 \nonumber\\
tv_but & 1.00000 \nonumber\\
cause_violence & 1.00000 \nonumber\\
book_for & 1.00000 \nonumber\\
amount_and & 1.00000 \nonumber\\
imagination_and & 1.00000 \nonumber\\
people_http://www.echoworld.com/b05/b0510/b0510tvbad.htm & 1.00000 \nonumber\\
as_tv & 1.00000 \nonumber\\
violence_and & 1.00000 \nonumber\\
bid_in & 1.00000 \nonumber\\
increase_someone & 1.00000 \nonumber\\
large_amount & 1.00000 \nonumber\\
not_completely & 1.00000 \nonumber\\
it_reduce & 1.00000 \nonumber\\
learn_. & 1.00000 \nonumber\\
in_large & 1.00000 \nonumber\\
creativity_as & 1.00000 \nonumber\\
to_cause & 1.00000 \nonumber\\
book_increase & 1.00000 \nonumber\\
sit_infront & 1.00000 \nonumber\\
completely_against & 1.00000 \nonumber\\
by_give & 1.00000 \nonumber\\
give_to & 1.00000 \nonumber\\
of_high & 1.00000 \nonumber\\
beverage_be & 1.00000 \nonumber\\
47_million & 1.00000 \nonumber\\
47 & 1.00000 \nonumber\\
water_produce & 1.00000 \nonumber\\
to_47 & 1.00000 \nonumber\\
waste_per & 1.00000 \nonumber\\
plastic_require & 1.00000 \nonumber\\
plastic_use & 1.00000 \nonumber\\
plastic_waste & 1.00000 \nonumber\\
80 & 1.00000 \nonumber\\
80_percent & 1.00000 \nonumber\\
to_bottle & 1.00000 \nonumber\\
quality_and & 1.00000 \nonumber\\
high_quality & 1.00000 \nonumber\\
per_year & 1.00000 \nonumber\\
to_produce & 1.00000 \nonumber\\
recycler & 1.00000 \nonumber\\
recycler_, & 1.00000 \nonumber\\
million_ton & 1.00000 \nonumber\\
in_demand & 1.00000 \nonumber\\
simply_throw & 1.00000 \nonumber\\
oil_per & 1.00000 \nonumber\\
bottle_beverage & 1.00000 \nonumber\\
throw_away & 1.00000 \nonumber\\
require_up & 1.00000 \nonumber\\
by_recycler & 1.00000 \nonumber\\
over_80 & 1.00000 \nonumber\\
to_1.5 & 1.00000 \nonumber\\
produce_. & 1.00000 \nonumber\\
ProductionRule_QP->IN,TO,CD,CD, & 1.00000 \nonumber\\
demand_by & 1.00000 \nonumber\\
produce_up & 1.00000 \nonumber\\
only_if & 1.00000 \nonumber\\
with_violence & 1.00000 \nonumber\\
discipline_, & 1.00000 \nonumber\\
n't_hit & 1.00000 \nonumber\\
everything_begin & 1.00000 \nonumber\\
not_everything & 1.00000 \nonumber\\
for_discipline & 1.00000 \nonumber\\
hit_kid & 1.00000 \nonumber\\
its_necessary & 1.00000 \nonumber\\
wouldnt_turn & 1.00000 \nonumber\\
ProductionRule_NP->NP,:,NP,., & 1.00000 \nonumber\\
the_competitiveness & 1.00000 \nonumber\\
important_. & 1.00000 \nonumber\\
kid_should & 1.00000 \nonumber\\
learn_, & 1.00000 \nonumber\\
competitiveness_can & 1.00000 \nonumber\\
competitiveness & 1.00000 \nonumber\\
on_learn & 1.00000 \nonumber\\
core & 1.00000 \nonumber\\
core_class & 1.00000 \nonumber\\
cause_bully & 1.00000 \nonumber\\
to_implement & 1.00000 \nonumber\\
require_action & 1.00000 \nonumber\\
which_would & 1.00000 \nonumber\\
implement_the & 1.00000 \nonumber\\
farquhar_implement & 1.00000 \nonumber\\
implement_those & 1.00000 \nonumber\\
implement & 1.00000 \nonumber\\
would_or & 1.00000 \nonumber\\
those_idea & 1.00000 \nonumber\\
ProductionRule_VP->VBD,PRT,PP, & 1.00000 \nonumber\\
action_require & 1.00000 \nonumber\\
actual_operation & 1.00000 \nonumber\\
or_would & 1.00000 \nonumber\\
knowledge_than & 1.00000 \nonumber\\
tv_do & 1.00000 \nonumber\\
tv_coz & 1.00000 \nonumber\\
book_give & 1.00000 \nonumber\\
give_more & 1.00000 \nonumber\\
more_knowledge & 1.00000 \nonumber\\
coz_. & 1.00000 \nonumber\\
ProductionRule_VP->VBP,ADVP,ADJP, & 1.00000 \nonumber\\
do_their & 1.00000 \nonumber\\
homework & 1.00000 \nonumber\\
homework_they & 1.00000 \nonumber\\
-_) & 1.00000 \nonumber\\
for_young & 1.00000 \nonumber\\
read_than & 1.00000 \nonumber\\
their_homework & 1.00000 \nonumber\\
young_kid & 1.00000 \nonumber\\
eye_. & 1.00000 \nonumber\\
their_eye & 1.00000 \nonumber\\
healthier_for & 1.00000 \nonumber\\
more_read & 1.00000 \nonumber\\
than_watch & 1.00000 \nonumber\\
:_- & 1.00000 \nonumber\\
its_healthier & 1.00000 \nonumber\\
when_kid & 1.00000 \nonumber\\
no_time & 1.00000 \nonumber\\
ProductionRule_VP->NP,NP,PP, & 1.00000 \nonumber\\
citizen_of & 1.00000 \nonumber\\
more_citizen & 1.00000 \nonumber\\
help_more & 1.00000 \nonumber\\
just_more & 1.00000 \nonumber\\
maybe_even & 1.00000 \nonumber\\
just_an & 1.00000 \nonumber\\
their_life & 1.00000 \nonumber\\
gas & 1.00000 \nonumber\\
universe_come & 1.00000 \nonumber\\
'_, & 1.00000 \nonumber\\
then_where & 1.00000 \nonumber\\
by_certain & 1.00000 \nonumber\\
those_gas & 1.00000 \nonumber\\
in_' & 1.00000 \nonumber\\
bang_' & 1.00000 \nonumber\\
gas_come & 1.00000 \nonumber\\
appear_. & 1.00000 \nonumber\\
gas_react & 1.00000 \nonumber\\
do_those & 1.00000 \nonumber\\
certain_gas & 1.00000 \nonumber\\
you_believe & 1.00000 \nonumber\\
cause_it & 1.00000 \nonumber\\
just_appear & 1.00000 \nonumber\\
_pos_ngram_PP_O_ART & 1.00000 \nonumber\\
react_with & 1.00000 \nonumber\\
from_? & 1.00000 \nonumber\\
this_universe & 1.00000 \nonumber\\
think_this & 1.00000 \nonumber\\
there_must & 1.00000 \nonumber\\
then_please & 1.00000 \nonumber\\
average_organ & 1.00000 \nonumber\\
characteristic_? & 1.00000 \nonumber\\
japanese_woman & 1.00000 \nonumber\\
japanese & 1.00000 \nonumber\\
a_japanese & 1.00000 \nonumber\\
hair & 1.00000 \nonumber\\
organ_size & 1.00000 \nonumber\\
fact_an & 1.00000 \nonumber\\
an_asian & 1.00000 \nonumber\\
believe_anyhow & 1.00000 \nonumber\\
?_speak & 1.00000 \nonumber\\
?_heart & 1.00000 \nonumber\\
?_hair & 1.00000 \nonumber\\
have_brain & 1.00000 \nonumber\\
pattern_? & 1.00000 \nonumber\\
organ & 1.00000 \nonumber\\
these_factor & 1.00000 \nonumber\\
scan_of & 1.00000 \nonumber\\
there_in & 1.00000 \nonumber\\
scan & 1.00000 \nonumber\\
different_racial & 1.00000 \nonumber\\
we_look & 1.00000 \nonumber\\
your_fact & 1.00000 \nonumber\\
asian_garden & 1.00000 \nonumber\\
asian & 1.00000 \nonumber\\
anyhow_? & 1.00000 \nonumber\\
sabrejimmy_account & 1.00000 \nonumber\\
record_? & 1.00000 \nonumber\\
!_do & 1.00000 \nonumber\\
garden_of & 1.00000 \nonumber\\
human_? & 1.00000 \nonumber\\
of_modern & 1.00000 \nonumber\\
account_for & 1.00000 \nonumber\\
an_african & 1.00000 \nonumber\\
modern_human & 1.00000 \nonumber\\
the_different & 1.00000 \nonumber\\
rate_record & 1.00000 \nonumber\\
about_average & 1.00000 \nonumber\\
hair_pattern & 1.00000 \nonumber\\
you_sabrejimmy & 1.00000 \nonumber\\
racial_characteristic & 1.00000 \nonumber\\
heart_rate & 1.00000 \nonumber\\
eden_? & 1.00000 \nonumber\\
look_so & 1.00000 \nonumber\\
._illuminate & 1.00000 \nonumber\\
racial & 1.00000 \nonumber\\
illuminate_us & 1.00000 \nonumber\\
illuminate & 1.00000 \nonumber\\
facial & 1.00000 \nonumber\\
please_do & 1.00000 \nonumber\\
speak_of & 1.00000 \nonumber\\
brain_scan & 1.00000 \nonumber\\
first_human & 1.00000 \nonumber\\
a_... & 1.00000 \nonumber\\
so_different & 1.00000 \nonumber\\
?_facial & 1.00000 \nonumber\\
size_? & 1.00000 \nonumber\\
african_garden & 1.00000 \nonumber\\
african & 1.00000 \nonumber\\
facial_characteristic & 1.00000 \nonumber\\
ProductionRule_S->SBAR,,,ADVP,VP,., & 1.00000 \nonumber\\
fact_! & 1.00000 \nonumber\\
_pos_ngram_CARD_NN_CARD & 1.00000 \nonumber\\
pursue_personal & 1.00000 \nonumber\\
goal_i & 1.00000 \nonumber\\
pursuit_and & 1.00000 \nonumber\\
responsible_and & 1.00000 \nonumber\\
best_pole & 1.00000 \nonumber\\
and_personal & 1.00000 \nonumber\\
pursue_a & 1.00000 \nonumber\\
mine_have & 1.00000 \nonumber\\
endeavor_simply & 1.00000 \nonumber\\
anything_you & 1.00000 \nonumber\\
learn_so & 1.00000 \nonumber\\
while_try & 1.00000 \nonumber\\
best_at & 1.00000 \nonumber\\
vaulter_that & 1.00000 \nonumber\\
from_my & 1.00000 \nonumber\\
achieve_this & 1.00000 \nonumber\\
vaulter & 1.00000 \nonumber\\
of_mine & 1.00000 \nonumber\\
pole & 1.00000 \nonumber\\
this_personal & 1.00000 \nonumber\\
goal_have & 1.00000 \nonumber\\
pole_vaulter & 1.00000 \nonumber\\
in_pursue & 1.00000 \nonumber\\
more_obedient & 1.00000 \nonumber\\
about_try & 1.00000 \nonumber\\
at_anything & 1.00000 \nonumber\\
obedient & 1.00000 \nonumber\\
more_responsible & 1.00000 \nonumber\\
,_pursue & 1.00000 \nonumber\\
obedient_. & 1.00000 \nonumber\\
me_its & 1.00000 \nonumber\\
it_a & 1.00000 \nonumber\\
be_religious & 1.00000 \nonumber\\
anymore & 1.00000 \nonumber\\
browse & 1.00000 \nonumber\\
chemical & 1.00000 \nonumber\\
have_bacterium & 1.00000 \nonumber\\
._water & 1.00000 \nonumber\\
bottle_also & 1.00000 \nonumber\\
judge & 1.00000 \nonumber\\
drug & 1.00000 \nonumber\\
if_evolution & 1.00000 \nonumber\\
*_if & 1.00000 \nonumber\\
true_.... & 1.00000 \nonumber\\
ProductionRule_S->NP,SBAR,NP,VP,., & 1.00000 \nonumber\\
...._how & 1.00000 \nonumber\\
singapore_' & 1.00000 \nonumber\\
!_in & 1.00000 \nonumber\\
a_life & 1.00000 \nonumber\\
its_wrong & 1.00000 \nonumber\\
guess_it & 1.00000 \nonumber\\
to_college & 1.00000 \nonumber\\
even_an & 1.00000 \nonumber\\
he_probaly & 1.00000 \nonumber\\
will_come & 1.00000 \nonumber\\
probaly_wont & 1.00000 \nonumber\\
he_need & 1.00000 \nonumber\\
have_and & 1.00000 \nonumber\\
assurance & 1.00000 \nonumber\\
probaly & 1.00000 \nonumber\\
assurance_that & 1.00000 \nonumber\\
way_about & 1.00000 \nonumber\\
that_assurance & 1.00000 \nonumber\\
will_realize & 1.00000 \nonumber\\
beileve & 1.00000 \nonumber\\
somebody_for & 1.00000 \nonumber\\
about_somebody & 1.00000 \nonumber\\
no_chance & 1.00000 \nonumber\\
that_at & 1.00000 \nonumber\\
yo_have & 1.00000 \nonumber\\
yo & 1.00000 \nonumber\\
beileve_that & 1.00000 \nonumber\\
i_beileve & 1.00000 \nonumber\\
least_yo & 1.00000 \nonumber\\
never_feel & 1.00000 \nonumber\\
pattern & 1.00000 \nonumber\\
all_tv & 1.00000 \nonumber\\
as_script & 1.00000 \nonumber\\
)_first & 1.00000 \nonumber\\
ProductionRule_VP->VBN,PRT,PP,ADVP, & 1.00000 \nonumber\\
ProductionRule_NP->NP,-LRB-,NP,-RRB-, & 1.00000 \nonumber\\
down_as & 1.00000 \nonumber\\
write_down & 1.00000 \nonumber\\
script_( & 1.00000 \nonumber\\
book_) & 1.00000 \nonumber\\
script & 1.00000 \nonumber\\
easier_. & 1.00000 \nonumber\\
_pos_ngram_NN_CONJ_PUNC & 1.00000 \nonumber\\
playstation & 1.00000 \nonumber\\
watch_what & 1.00000 \nonumber\\
ever_i & 1.00000 \nonumber\\
playstation_. & 1.00000 \nonumber\\
tv_sooooooo & 1.00000 \nonumber\\
_pos_ngram_PR_ADV_O & 1.00000 \nonumber\\
much_i & 1.00000 \nonumber\\
love_tv & 1.00000 \nonumber\\
dvd_and & 1.00000 \nonumber\\
sooooooo & 1.00000 \nonumber\\
play_on & 1.00000 \nonumber\\
dvd & 1.00000 \nonumber\\
on_playstation & 1.00000 \nonumber\\
watch_dvd & 1.00000 \nonumber\\
sooooooo_much & 1.00000 \nonumber\\
of_think & 1.00000 \nonumber\\
on_a & 1.00000 \nonumber\\
so_uniform & 1.00000 \nonumber\\
afford & 1.00000 \nonumber\\
us_to & 1.00000 \nonumber\\
fat & 1.00000 \nonumber\\
_pos_ngram_PR_NP_PP & 1.00000 \nonumber\\
a_situation & 1.00000 \nonumber\\
the_victim & 1.00000 \nonumber\\
stranger_. & 1.00000 \nonumber\\
be_harm & 1.00000 \nonumber\\
person_like & 1.00000 \nonumber\\
will_say & 1.00000 \nonumber\\
harm_us & 1.00000 \nonumber\\
consider_him & 1.00000 \nonumber\\
victim_or & 1.00000 \nonumber\\
situation_it & 1.00000 \nonumber\\
afraid_to & 1.00000 \nonumber\\
a_stranger & 1.00000 \nonumber\\
ProductionRule_VP->VBD,UCP, & 1.00000 \nonumber\\
'_most & 1.00000 \nonumber\\
depend_whether & 1.00000 \nonumber\\
ProductionRule_UCP->NP,CC,SBAR, & 1.00000 \nonumber\\
_pos_ngram_CONJ_PR_PP & 1.00000 \nonumber\\
a_psycho & 1.00000 \nonumber\\
a_random & 1.00000 \nonumber\\
psycho_and & 1.00000 \nonumber\\
psycho & 1.00000 \nonumber\\
that_consider & 1.00000 \nonumber\\
also_what & 1.00000 \nonumber\\
stranger_, & 1.00000 \nonumber\\
random_stranger & 1.00000 \nonumber\\
sit_them & 1.00000 \nonumber\\
need_that & 1.00000 \nonumber\\
possibility_they & 1.00000 \nonumber\\
the_punishment & 1.00000 \nonumber\\
because_depend & 1.00000 \nonumber\\
punishment_its & 1.00000 \nonumber\\
in_punishment & 1.00000 \nonumber\\
because_just & 1.00000 \nonumber\\
you_give & 1.00000 \nonumber\\
need_need & 1.00000 \nonumber\\
him_as & 1.00000 \nonumber\\
ProductionRule_S->NP,PP, & 1.00000 \nonumber\\
ProductionRule_ADJP->JJR,SBAR, & 1.00000 \nonumber\\
_pos_ngram_ADJ_O_NN & 1.00000 \nonumber\\
n't_feel & 1.00000 \nonumber\\
few_people & 1.00000 \nonumber\\
ProductionRule_NP->RB,DT,JJ,NNS, & 1.00000 \nonumber\\
life_' & 1.00000 \nonumber\\
apply_physical & 1.00000 \nonumber\\
people_apply & 1.00000 \nonumber\\
exercise_in & 1.00000 \nonumber\\
'_! & 1.00000 \nonumber\\
drink_bottle & 1.00000 \nonumber\\
watch_anything & 1.00000 \nonumber\\
win_hopefully & 1.00000 \nonumber\\
!!!!_tv & 1.00000 \nonumber\\
hopefully_lol & 1.00000 \nonumber\\
!!!!!! & 1.00000 \nonumber\\
!!!!!!_go & 1.00000 \nonumber\\
tv_!!!!!! & 1.00000 \nonumber\\
go_tv & 1.00000 \nonumber\\
great_to & 1.00000 \nonumber\\
lol_tv & 1.00000 \nonumber\\
will_win & 1.00000 \nonumber\\
tv_!!!! & 1.00000 \nonumber\\
tv_will & 1.00000 \nonumber\\
worse_than & 1.00000 \nonumber\\
not_take & 1.00000 \nonumber\\
be_botherd & 1.00000 \nonumber\\
ProductionRule_PP->TO,PP, & 1.00000 \nonumber\\
ProductionRule_NP->NP,CC,NP,CC,NP, & 1.00000 \nonumber\\
botherd_to & 1.00000 \nonumber\\
botherd & 1.00000 \nonumber\\
to_to & 1.00000 \nonumber\\
some_crisp & 1.00000 \nonumber\\
tv_when & 1.00000 \nonumber\\
crisp_or & 1.00000 \nonumber\\
sweet_and & 1.00000 \nonumber\\
sweet & 1.00000 \nonumber\\
with_some & 1.00000 \nonumber\\
a_burger & 1.00000 \nonumber\\
couch_with & 1.00000 \nonumber\\
or_sweet & 1.00000 \nonumber\\
burger & 1.00000 \nonumber\\
burger_or & 1.00000 \nonumber\\
parent_be & 1.00000 \nonumber\\
snake & 1.00000 \nonumber\\
infanticide_, & 1.00000 \nonumber\\
talk_donkey & 1.00000 \nonumber\\
snake_, & 1.00000 \nonumber\\
,_hell & 1.00000 \nonumber\\
talk_snake & 1.00000 \nonumber\\
:_belief & 1.00000 \nonumber\\
matricide & 1.00000 \nonumber\\
,_unscientific & 1.00000 \nonumber\\
,_talk & 1.00000 \nonumber\\
,_superstition & 1.00000 \nonumber\\
,_pedophilia & 1.00000 \nonumber\\
logic_, & 1.00000 \nonumber\\
,_observation & 1.00000 \nonumber\\
,_matricide & 1.00000 \nonumber\\
,_infanticide & 1.00000 \nonumber\\
,_incest & 1.00000 \nonumber\\
,_genocide & 1.00000 \nonumber\\
,_eternal & 1.00000 \nonumber\\
superstition_, & 1.00000 \nonumber\\
superstition & 1.00000 \nonumber\\
,_bestiality & 1.00000 \nonumber\\
ProductionRule_NP->NP,,,NP,,,NP,,,NP,,,NP,,,NP,,,NP,,,NP,,,NP,,,NP,,,NP,,,NP,,,NP,,,NP,,,NP,,,CC,NP, & 1.00000 \nonumber\\
these_claim & 1.00000 \nonumber\\
ProductionRule_NP->NP,:,NP,X, & 1.00000 \nonumber\\
ProductionRule_X->IN,NP, & 1.00000 \nonumber\\
infanticide & 1.00000 \nonumber\\
the_rejection & 1.00000 \nonumber\\
matricide_, & 1.00000 \nonumber\\
observation_, & 1.00000 \nonumber\\
bestiality_, & 1.00000 \nonumber\\
claim_, & 1.00000 \nonumber\\
pedophilia & 1.00000 \nonumber\\
torture & 1.00000 \nonumber\\
pedophilia_, & 1.00000 \nonumber\\
atheism_: & 1.00000 \nonumber\\
unscientific & 1.00000 \nonumber\\
etc_atheism & 1.00000 \nonumber\\
genocide_, & 1.00000 \nonumber\\
eternal & 1.00000 \nonumber\\
claim_base & 1.00000 \nonumber\\
eternal_torture & 1.00000 \nonumber\\
bestiality & 1.00000 \nonumber\\
rejection & 1.00000 \nonumber\\
and_common & 1.00000 \nonumber\\
genocide & 1.00000 \nonumber\\
fire_, & 1.00000 \nonumber\\
rejection_of & 1.00000 \nonumber\\
donkey_, & 1.00000 \nonumber\\
incest & 1.00000 \nonumber\\
donkey & 1.00000 \nonumber\\
torture_, & 1.00000 \nonumber\\
hell_fire & 1.00000 \nonumber\\
incest_, & 1.00000 \nonumber\\
on_logic & 1.00000 \nonumber\\
unscientific_claim & 1.00000 \nonumber\\
ProductionRule_ADJP->JJR,S, & 1.00000 \nonumber\\
today_, & 1.00000 \nonumber\\
be_pro-life & 1.00000 \nonumber\\
of_those & 1.00000 \nonumber\\
proof_that & 1.00000 \nonumber\\
people_here & 1.00000 \nonumber\\
that_man & 1.00000 \nonumber\\
many_more & 1.00000 \nonumber\\
website & 1.00000 \nonumber\\
time_on & 1.00000 \nonumber\\
ProductionRule_X->NP,NP,NP, & 1.00000 \nonumber\\
maybe_i & 1.00000 \nonumber\\
a_christianity & 1.00000 \nonumber\\
._each & 1.00000 \nonumber\\
you_'d & 1.00000 \nonumber\\
'd_accept & 1.00000 \nonumber\\
it_!!! & 1.00000 \nonumber\\
or_adopt & 1.00000 \nonumber\\
adopt_mother/father & 1.00000 \nonumber\\
accept_it & 1.00000 \nonumber\\
child_or & 1.00000 \nonumber\\
marry_let & 1.00000 \nonumber\\
mother/father_you & 1.00000 \nonumber\\
mother/father & 1.00000 \nonumber\\
belief_in & 1.00000 \nonumber\\
hospital_. & 1.00000 \nonumber\\
add_any & 1.00000 \nonumber\\
safer & 1.00000 \nonumber\\
safer_, & 1.00000 \nonumber\\
customize_it & 1.00000 \nonumber\\
name_! & 1.00000 \nonumber\\
more_original & 1.00000 \nonumber\\
of_. & 1.00000 \nonumber\\
functionality_you & 1.00000 \nonumber\\
sleeker_. & 1.00000 \nonumber\\
original_name & 1.00000 \nonumber\\
look_any & 1.00000 \nonumber\\
and_sleeker & 1.00000 \nonumber\\
any_functionality & 1.00000 \nonumber\\
reason_at & 1.00000 \nonumber\\
customize & 1.00000 \nonumber\\
all_why & 1.00000 \nonumber\\
,_faster & 1.00000 \nonumber\\
be_safer & 1.00000 \nonumber\\
can_think & 1.00000 \nonumber\\
can_customize & 1.00000 \nonumber\\
could_say & 1.00000 \nonumber\\
say_ie & 1.00000 \nonumber\\
can_add & 1.00000 \nonumber\\
anyone_could & 1.00000 \nonumber\\
why_anyone & 1.00000 \nonumber\\
dichotomy_in & 1.00000 \nonumber\\
"_theism & 1.00000 \nonumber\\
option_be & 1.00000 \nonumber\\
atheism_or & 1.00000 \nonumber\\
other_" & 1.00000 \nonumber\\
or_atheism & 1.00000 \nonumber\\
a_false & 1.00000 \nonumber\\
debate_present & 1.00000 \nonumber\\
theism_or & 1.00000 \nonumber\\
theism & 1.00000 \nonumber\\
present_a & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,ADVP,NP,SBAR, & 1.00000 \nonumber\\
these_people & 1.00000 \nonumber\\
television_' & 1.00000 \nonumber\\
!!!_:) & 1.00000 \nonumber\\
eye_bid & 1.00000 \nonumber\\
dhal & 1.00000 \nonumber\\
dhal_you & 1.00000 \nonumber\\
than_t.v. & 1.00000 \nonumber\\
dead_! & 1.00000 \nonumber\\
'_by & 1.00000 \nonumber\\
roald & 1.00000 \nonumber\\
roald_dhal & 1.00000 \nonumber\\
you_eye & 1.00000 \nonumber\\
all_!!! & 1.00000 \nonumber\\
t.v._make & 1.00000 \nonumber\\
imagination_dead & 1.00000 \nonumber\\
ProductionRule_NP->VBZ,NP, & 1.00000 \nonumber\\
t.v._because & 1.00000 \nonumber\\
'_television & 1.00000 \nonumber\\
by_roald & 1.00000 \nonumber\\
:)_: & 1.00000 \nonumber\\
because_t.v. & 1.00000 \nonumber\\
read_' & 1.00000 \nonumber\\
!_read & 1.00000 \nonumber\\
kill_imagination & 1.00000 \nonumber\\
bid_be & 1.00000 \nonumber\\
:)_:) & 1.00000 \nonumber\\
the_evolution & 1.00000 \nonumber\\
father_either & 1.00000 \nonumber\\
n't_teach & 1.00000 \nonumber\\
respectable_father & 1.00000 \nonumber\\
best_he & 1.00000 \nonumber\\
case_its & 1.00000 \nonumber\\
a_respectable & 1.00000 \nonumber\\
still_lose & 1.00000 \nonumber\\
all_if & 1.00000 \nonumber\\
you_anything & 1.00000 \nonumber\\
comman_good & 1.00000 \nonumber\\
that_advence & 1.00000 \nonumber\\
do_wont & 1.00000 \nonumber\\
advence & 1.00000 \nonumber\\
advence_the & 1.00000 \nonumber\\
little_good & 1.00000 \nonumber\\
wont_really & 1.00000 \nonumber\\
difference_. & 1.00000 \nonumber\\
see_very & 1.00000 \nonumber\\
comman & 1.00000 \nonumber\\
bid_thing & 1.00000 \nonumber\\
more_for & 1.00000 \nonumber\\
world_where & 1.00000 \nonumber\\
persuit_do & 1.00000 \nonumber\\
do_good & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,ADVP,ADVP,NP, & 1.00000 \nonumber\\
the_comman & 1.00000 \nonumber\\
to_myself & 1.00000 \nonumber\\
union_, & 1.00000 \nonumber\\
i_also & 1.00000 \nonumber\\
depict_that & 1.00000 \nonumber\\
goal_for & 1.00000 \nonumber\\
class_they & 1.00000 \nonumber\\
uniform_signify & 1.00000 \nonumber\\
fidelity_in & 1.00000 \nonumber\\
of_peace & 1.00000 \nonumber\\
that_whether & 1.00000 \nonumber\\
wall_of & 1.00000 \nonumber\\
roof_. & 1.00000 \nonumber\\
high_or & 1.00000 \nonumber\\
nice_to & 1.00000 \nonumber\\
from_high & 1.00000 \nonumber\\
its_goal & 1.00000 \nonumber\\
,_white & 1.00000 \nonumber\\
fidelity & 1.00000 \nonumber\\
i_wear & 1.00000 \nonumber\\
or_low & 1.00000 \nonumber\\
low_class & 1.00000 \nonumber\\
child_come & 1.00000 \nonumber\\
shirt_and & 1.00000 \nonumber\\
identical_uniform & 1.00000 \nonumber\\
color_be & 1.00000 \nonumber\\
of_status & 1.00000 \nonumber\\
relationship_moreover & 1.00000 \nonumber\\
one_roof & 1.00000 \nonumber\\
depict & 1.00000 \nonumber\\
and_blue & 1.00000 \nonumber\\
'_uniform & 1.00000 \nonumber\\
skirt_in & 1.00000 \nonumber\\
the_wall & 1.00000 \nonumber\\
signify & 1.00000 \nonumber\\
signify_its & 1.00000 \nonumber\\
moreover_identical & 1.00000 \nonumber\\
white_shirt & 1.00000 \nonumber\\
for_instant & 1.00000 \nonumber\\
blue & 1.00000 \nonumber\\
equally_under & 1.00000 \nonumber\\
blue_of & 1.00000 \nonumber\\
blue_skirt & 1.00000 \nonumber\\
in_relationship & 1.00000 \nonumber\\
of_fidelity & 1.00000 \nonumber\\
each_school & 1.00000 \nonumber\\
also_remove & 1.00000 \nonumber\\
instant & 1.00000 \nonumber\\
wear_white & 1.00000 \nonumber\\
instant_i & 1.00000 \nonumber\\
also_depict & 1.00000 \nonumber\\
indication & 1.00000 \nonumber\\
white_color & 1.00000 \nonumber\\
indication_of & 1.00000 \nonumber\\
an_indication & 1.00000 \nonumber\\
'_nice & 1.00000 \nonumber\\
treat_equally & 1.00000 \nonumber\\
punishment & 1.00000 \nonumber\\
water_use & 1.00000 \nonumber\\
will_learn & 1.00000 \nonumber\\
be_other & 1.00000 \nonumber\\
,_etc. & 1.00000 \nonumber\\
unform & 1.00000 \nonumber\\
kid_expression & 1.00000 \nonumber\\
unform_dose & 1.00000 \nonumber\\
and_unform & 1.00000 \nonumber\\
expression_and & 1.00000 \nonumber\\
dose_not & 1.00000 \nonumber\\
it_dose & 1.00000 \nonumber\\
show_kid & 1.00000 \nonumber\\
long_term & 1.00000 \nonumber\\
transport & 1.00000 \nonumber\\
will_once & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,RB,NP,,,SBAR, & 1.00000 \nonumber\\
ProductionRule_S->S,S,S,,,S, & 1.00000 \nonumber\\
all_wont & 1.00000 \nonumber\\
y'_all & 1.00000 \nonumber\\
good_technique & 1.00000 \nonumber\\
technique_they & 1.00000 \nonumber\\
ProductionRule_VP->MD,ADVP, & 1.00000 \nonumber\\
good_relationship & 1.00000 \nonumber\\
wont_have & 1.00000 \nonumber\\
then_y' & 1.00000 \nonumber\\
they_grow & 1.00000 \nonumber\\
not_grow & 1.00000 \nonumber\\
up_it & 1.00000 \nonumber\\
y' & 1.00000 \nonumber\\
relationship_will & 1.00000 \nonumber\\
a_creator & 1.00000 \nonumber\\
full_person & 1.00000 \nonumber\\
citizenship & 1.00000 \nonumber\\
..._america & 1.00000 \nonumber\\
conceive_here & 1.00000 \nonumber\\
life_begin & 1.00000 \nonumber\\
at_conception & 1.00000 \nonumber\\
bear_" & 1.00000 \nonumber\\
who_believe & 1.00000 \nonumber\\
grant & 1.00000 \nonumber\\
citizenship_to & 1.00000 \nonumber\\
should_also & 1.00000 \nonumber\\
"_begin & 1.00000 \nonumber\\
those_conceive & 1.00000 \nonumber\\
"_bear & 1.00000 \nonumber\\
begin_at & 1.00000 \nonumber\\
a_full & 1.00000 \nonumber\\
grant_citizenship & 1.00000 \nonumber\\
ProductionRule_S->``,NP,'',VP, & 1.00000 \nonumber\\
conception_and & 1.00000 \nonumber\\
also_grant & 1.00000 \nonumber\\
no_? & 1.00000 \nonumber\\
birth_... & 1.00000 \nonumber\\
believe_life & 1.00000 \nonumber\\
america_grant & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,PP,:,S, & 1.00000 \nonumber\\
think_for & 1.00000 \nonumber\\
conception_rather & 1.00000 \nonumber\\
person_with & 1.00000 \nonumber\\
interest_think & 1.00000 \nonumber\\
perhap_if & 1.00000 \nonumber\\
ProductionRule_PP->PP,,,CC,RB,PP, & 1.00000 \nonumber\\
ProductionRule_VP->``,VBN,'',PP, & 1.00000 \nonumber\\
with_rights & 1.00000 \nonumber\\
than_birth & 1.00000 \nonumber\\
._perhap & 1.00000 \nonumber\\
an_interest & 1.00000 \nonumber\\
adrenalin & 1.00000 \nonumber\\
adrenalin_rush & 1.00000 \nonumber\\
raise_it & 1.00000 \nonumber\\
the_adrenalin & 1.00000 \nonumber\\
they_obviously & 1.00000 \nonumber\\
that_less & 1.00000 \nonumber\\
rape_get & 1.00000 \nonumber\\
1_% & 1.00000 \nonumber\\
'_biological & 1.00000 \nonumber\\
own_because & 1.00000 \nonumber\\
you_otherwise & 1.00000 \nonumber\\
pregnant_because & 1.00000 \nonumber\\
of_adoption & 1.00000 \nonumber\\
their_family & 1.00000 \nonumber\\
the_wait & 1.00000 \nonumber\\
rush & 1.00000 \nonumber\\
_pos_ngram_ART_ADV_ART & 1.00000 \nonumber\\
biological_mother & 1.00000 \nonumber\\
obviously_hav & 1.00000 \nonumber\\
or_abortion & 1.00000 \nonumber\\
another_baby & 1.00000 \nonumber\\
the_still & 1.00000 \nonumber\\
otherwise_because & 1.00000 \nonumber\\
take_an & 1.00000 \nonumber\\
wait_list & 1.00000 \nonumber\\
statistics_prove & 1.00000 \nonumber\\
statistics & 1.00000 \nonumber\\
list_for & 1.00000 \nonumber\\
baby_to & 1.00000 \nonumber\\
of_woman & 1.00000 \nonumber\\
anyone_tell & 1.00000 \nonumber\\
or_raise & 1.00000 \nonumber\\
avoid_the & 1.00000 \nonumber\\
rush_. & 1.00000 \nonumber\\
ProductionRule_NP->JJ,JJ,NN,NNS, & 1.00000 \nonumber\\
drink_from & 1.00000 \nonumber\\
you_guy & 1.00000 \nonumber\\
for_water & 1.00000 \nonumber\\
heat_and & 1.00000 \nonumber\\
waste_the & 1.00000 \nonumber\\
all_dehydrate & 1.00000 \nonumber\\
sick/in_the & 1.00000 \nonumber\\
water_bottlee & 1.00000 \nonumber\\
sick/in & 1.00000 \nonumber\\
convenient_to & 1.00000 \nonumber\\
or_drink & 1.00000 \nonumber\\
guy_but & 1.00000 \nonumber\\
but_water & 1.00000 \nonumber\\
two_option & 1.00000 \nonumber\\
the_heat & 1.00000 \nonumber\\
so_convenient & 1.00000 \nonumber\\
summer_day & 1.00000 \nonumber\\
my_day & 1.00000 \nonumber\\
drink_out & 1.00000 \nonumber\\
the_hospital & 1.00000 \nonumber\\
option_for & 1.00000 \nonumber\\
the_beach & 1.00000 \nonumber\\
summer & 1.00000 \nonumber\\
,_pass & 1.00000 \nonumber\\
dehydrate_and & 1.00000 \nonumber\\
dehydrate & 1.00000 \nonumber\\
ocean_that & 1.00000 \nonumber\\
n't_drink & 1.00000 \nonumber\\
._or & 1.00000 \nonumber\\
hot_summer & 1.00000 \nonumber\\
pass_out & 1.00000 \nonumber\\
a_water & 1.00000 \nonumber\\
my_only & 1.00000 \nonumber\\
beach & 1.00000 \nonumber\\
beach_on & 1.00000 \nonumber\\
and_lack & 1.00000 \nonumber\\
day_sick/in & 1.00000 \nonumber\\
everybody_have & 1.00000 \nonumber\\
america & 1.00000 \nonumber\\
alway_work & 1.00000 \nonumber\\
figure_. & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,NP,S, & 1.00000 \nonumber\\
have_so & 1.00000 \nonumber\\
unsuitable & 1.00000 \nonumber\\
unsuitable_clothe & 1.00000 \nonumber\\
wear_later & 1.00000 \nonumber\\
they_ensure & 1.00000 \nonumber\\
the_clothe & 1.00000 \nonumber\\
no_unsuitable & 1.00000 \nonumber\\
prepare_people & 1.00000 \nonumber\\
clothe_they & 1.00000 \nonumber\\
they_prepare & 1.00000 \nonumber\\
oil & 1.00000 \nonumber\\
country_' & 1.00000 \nonumber\\
only_indium & 1.00000 \nonumber\\
water_company & 1.00000 \nonumber\\
hub & 1.00000 \nonumber\\
_pos_ngram_V_CARD_PP & 1.00000 \nonumber\\
if_there & 1.00000 \nonumber\\
way_the & 1.00000 \nonumber\\
hurt_, & 1.00000 \nonumber\\
this_from & 1.00000 \nonumber\\
again_because & 1.00000 \nonumber\\
really_hurt & 1.00000 \nonumber\\
ProductionRule_VP->VP,,,CC,ADVP,VP, & 1.00000 \nonumber\\
from_experience & 1.00000 \nonumber\\
ProductionRule_S->ADVP,PP,NP,VP,., & 1.00000 \nonumber\\
_pos_ngram_CARD_ADV_V & 1.00000 \nonumber\\
after_all & 1.00000 \nonumber\\
'_behavior & 1.00000 \nonumber\\
book_will & 1.00000 \nonumber\\
_pos_ngram_ADJ_ART_ART & 1.00000 \nonumber\\
alway_great & 1.00000 \nonumber\\
ProductionRule_NP->PRP$,VBN,NN, & 1.00000 \nonumber\\
whatever_the & 1.00000 \nonumber\\
emerge_book & 1.00000 \nonumber\\
new_technological & 1.00000 \nonumber\\
human_heart & 1.00000 \nonumber\\
development_emerge & 1.00000 \nonumber\\
great_whatever & 1.00000 \nonumber\\
fix_place & 1.00000 \nonumber\\
have_its & 1.00000 \nonumber\\
its_fix & 1.00000 \nonumber\\
every_human & 1.00000 \nonumber\\
goodness_, & 1.00000 \nonumber\\
advance_a & 1.00000 \nonumber\\
just_assume & 1.00000 \nonumber\\
goodness & 1.00000 \nonumber\\
this_goodness & 1.00000 \nonumber\\
your_common & 1.00000 \nonumber\\
your_good & 1.00000 \nonumber\\
great_person & 1.00000 \nonumber\\
to_then & 1.00000 \nonumber\\
must_first & 1.00000 \nonumber\\
know_when & 1.00000 \nonumber\\
start_the & 1.00000 \nonumber\\
spread_your & 1.00000 \nonumber\\
that_start & 1.00000 \nonumber\\
show_it & 1.00000 \nonumber\\
world_full & 1.00000 \nonumber\\
then_spread & 1.00000 \nonumber\\
you_desire & 1.00000 \nonumber\\
spark & 1.00000 \nonumber\\
first_realize & 1.00000 \nonumber\\
that_spark & 1.00000 \nonumber\\
the_fire & 1.00000 \nonumber\\
realize_what & 1.00000 \nonumber\\
spark_that & 1.00000 \nonumber\\
to_achieve & 1.00000 \nonumber\\
cute_little & 1.00000 \nonumber\\
popup_window & 1.00000 \nonumber\\
popup & 1.00000 \nonumber\\
those_with & 1.00000 \nonumber\\
those_cute & 1.00000 \nonumber\\
little_popup & 1.00000 \nonumber\\
get_those & 1.00000 \nonumber\\
like_those & 1.00000 \nonumber\\
presence_be & 1.00000 \nonumber\\
british_presence & 1.00000 \nonumber\\
take_charge & 1.00000 \nonumber\\
be_introduce & 1.00000 \nonumber\\
presence & 1.00000 \nonumber\\
new_settlement & 1.00000 \nonumber\\
settlement_and & 1.00000 \nonumber\\
odds_after & 1.00000 \nonumber\\
after_british & 1.00000 \nonumber\\
all_odds & 1.00000 \nonumber\\
run_against & 1.00000 \nonumber\\
introduce_, & 1.00000 \nonumber\\
to_return & 1.00000 \nonumber\\
against_all & 1.00000 \nonumber\\
active & 1.00000 \nonumber\\
us_with & 1.00000 \nonumber\\
get_here & 1.00000 \nonumber\\
we_here & 1.00000 \nonumber\\
here_but & 1.00000 \nonumber\\
ProductionRule_VP->VBD,ADVP,PRN, & 1.00000 \nonumber\\
ProductionRule_PRN->CC,SBAR, & 1.00000 \nonumber\\
how_we & 1.00000 \nonumber\\
percent_. & 1.00000 \nonumber\\
worldwide_bottle & 1.00000 \nonumber\\
_pos_ngram_CARD_CONJ_O & 1.00000 \nonumber\\
worldwide & 1.00000 \nonumber\\
startle_annual & 1.00000 \nonumber\\
billion_each & 1.00000 \nonumber\\
variously & 1.00000 \nonumber\\
startle & 1.00000 \nonumber\\
7_percent & 1.00000 \nonumber\\
dry & 1.00000 \nonumber\\
dry_well & 1.00000 \nonumber\\
rate_of & 1.00000 \nonumber\\
estimate_variously & 1.00000 \nonumber\\
market_expand & 1.00000 \nonumber\\
at_between & 1.00000 \nonumber\\
of_sustainability & 1.00000 \nonumber\\
50_and & 1.00000 \nonumber\\
sale_at & 1.00000 \nonumber\\
sustainability & 1.00000 \nonumber\\
sustainability_, & 1.00000 \nonumber\\
100_billion & 1.00000 \nonumber\\
ProductionRule_VP->VBP,NP,PP,,,PP, & 1.00000 \nonumber\\
the_startle & 1.00000 \nonumber\\
place_worldwide & 1.00000 \nonumber\\
expand_at & 1.00000 \nonumber\\
in_term & 1.00000 \nonumber\\
_pos_ngram_CARD_CARD_ART & 1.00000 \nonumber\\
and_$ & 1.00000 \nonumber\\
annual_rate & 1.00000 \nonumber\\
term_of & 1.00000 \nonumber\\
$_100 & 1.00000 \nonumber\\
$_50 & 1.00000 \nonumber\\
annual & 1.00000 \nonumber\\
ProductionRule_QP->IN,$,CD,CC,$,CD,CD, & 1.00000 \nonumber\\
between_$ & 1.00000 \nonumber\\
variously_place & 1.00000 \nonumber\\
a_dry & 1.00000 \nonumber\\
be_big & 1.00000 \nonumber\\
water_sale & 1.00000 \nonumber\\
spouse_kill & 1.00000 \nonumber\\
and_or & 1.00000 \nonumber\\
should_enjoy & 1.00000 \nonumber\\
preserve_for & 1.00000 \nonumber\\
preserve & 1.00000 \nonumber\\
enjoy_and & 1.00000 \nonumber\\
atheist_because & 1.00000 \nonumber\\
future_generation & 1.00000 \nonumber\\
one_life & 1.00000 \nonumber\\
all_future & 1.00000 \nonumber\\
and_preserve & 1.00000 \nonumber\\
(_20 & 1.00000 \nonumber\\
(_flexible & 1.00000 \nonumber\\
the_advantage & 1.00000 \nonumber\\
weakness & 1.00000 \nonumber\\
weakness_. & 1.00000 \nonumber\\
button_? & 1.00000 \nonumber\\
)_or & 1.00000 \nonumber\\
ie7_in & 1.00000 \nonumber\\
issue_i & 1.00000 \nonumber\\
once_) & 1.00000 \nonumber\\
em & 1.00000 \nonumber\\
restart_will & 1.00000 \nonumber\\
a_know & 1.00000 \nonumber\\
ie_7 & 1.00000 \nonumber\\
and_argue & 1.00000 \nonumber\\
more_at & 1.00000 \nonumber\\
only_memory & 1.00000 \nonumber\\
across_be & 1.00000 \nonumber\\
multiple_window & 1.00000 \nonumber\\
earlier & 1.00000 \nonumber\\
obviously_have & 1.00000 \nonumber\\
earlier_version & 1.00000 \nonumber\\
when_leave & 1.00000 \nonumber\\
know_issue & 1.00000 \nonumber\\
active_for & 1.00000 \nonumber\\
will_fix & 1.00000 \nonumber\\
memory_issue & 1.00000 \nonumber\\
memory_leak & 1.00000 \nonumber\\
simple_restart & 1.00000 \nonumber\\
feature_they & 1.00000 \nonumber\\
window_( & 1.00000 \nonumber\\
to_ie & 1.00000 \nonumber\\
they_add & 1.00000 \nonumber\\
time_( & 1.00000 \nonumber\\
actually_use & 1.00000 \nonumber\\
20_or & 1.00000 \nonumber\\
for_three & 1.00000 \nonumber\\
firefox_2 & 1.00000 \nonumber\\
leak_obviously & 1.00000 \nonumber\\
advantage_earlier & 1.00000 \nonumber\\
fix_) & 1.00000 \nonumber\\
who_need & 1.00000 \nonumber\\
firefox_... & 1.00000 \nonumber\\
toolbar_? & 1.00000 \nonumber\\
need_em & 1.00000 \nonumber\\
firefox_active & 1.00000 \nonumber\\
or_when & 1.00000 \nonumber\\
on_open & 1.00000 \nonumber\\
7_they & 1.00000 \nonumber\\
remove_one & 1.00000 \nonumber\\
..._weakness & 1.00000 \nonumber\\
flexible_toolbar & 1.00000 \nonumber\\
for_ie7 & 1.00000 \nonumber\\
customizable & 1.00000 \nonumber\\
?_customizable & 1.00000 \nonumber\\
come_across & 1.00000 \nonumber\\
they_remove & 1.00000 \nonumber\\
customizable_button & 1.00000 \nonumber\\
have_major & 1.00000 \nonumber\\
every_feature & 1.00000 \nonumber\\
open_multiple & 1.00000 \nonumber\\
say_firefox & 1.00000 \nonumber\\
2_have & 1.00000 \nonumber\\
major_memory & 1.00000 \nonumber\\
hour_or & 1.00000 \nonumber\\
em_! & 1.00000 \nonumber\\
version_have & 1.00000 \nonumber\\
three_hour & 1.00000 \nonumber\\
leave_firefox & 1.00000 \nonumber\\
at_once & 1.00000 \nonumber\\
biggest & 1.00000 \nonumber\\
their_be & 1.00000 \nonumber\\
child_who & 1.00000 \nonumber\\
_pos_ngram_PUNC_ADJ_CONJ & 1.00000 \nonumber\\
a_form & 1.00000 \nonumber\\
help_advance & 1.00000 \nonumber\\
"_life & 1.00000 \nonumber\\
life_" & 1.00000 \nonumber\\
than_any & 1.00000 \nonumber\\
someone_you & 1.00000 \nonumber\\
love_someone & 1.00000 \nonumber\\
be_rich & 1.00000 \nonumber\\
desire_. & 1.00000 \nonumber\\
will_want & 1.00000 \nonumber\\
ProductionRule_X->X,NP, & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,ADJP,PP,SBAR, & 1.00000 \nonumber\\
give_moment & 1.00000 \nonumber\\
the_personal & 1.00000 \nonumber\\
rather_do & 1.00000 \nonumber\\
my_give & 1.00000 \nonumber\\
._right & 1.00000 \nonumber\\
be_feel & 1.00000 \nonumber\\
believe_a & 1.00000 \nonumber\\
better_my & 1.00000 \nonumber\\
every_once & 1.00000 \nonumber\\
the_if & 1.00000 \nonumber\\
ProductionRule_PP->RB,IN,SBAR, & 1.00000 \nonumber\\
right_after & 1.00000 \nonumber\\
t_would & 1.00000 \nonumber\\
fine_? & 1.00000 \nonumber\\
after_than & 1.00000 \nonumber\\
than_t & 1.00000 \nonumber\\
abortion_right & 1.00000 \nonumber\\
_pos_ngram_NP_NP_ART & 1.00000 \nonumber\\
ProductionRule_VP->VB,NP,PP,,,S, & 1.00000 \nonumber\\
bed & 1.00000 \nonumber\\
my_bed & 1.00000 \nonumber\\
murderer_on & 1.00000 \nonumber\\
bed_. & 1.00000 \nonumber\\
right_, & 1.00000 \nonumber\\
ProductionRule_S->S,,,CC,ADVP,S,., & 1.00000 \nonumber\\
,_kill & 1.00000 \nonumber\\
one_else & 1.00000 \nonumber\\
ProductionRule_NP->PRP$,ADJP,NNS, & 1.00000 \nonumber\\
too_great & 1.00000 \nonumber\\
the_caste & 1.00000 \nonumber\\
ProductionRule_S->NP,VP,CC,S, & 1.00000 \nonumber\\
they_still & 1.00000 \nonumber\\
still_heavily & 1.00000 \nonumber\\
caste_system & 1.00000 \nonumber\\
poor_be & 1.00000 \nonumber\\
ProductionRule_NP->DT,JJ,CC,JJ, & 1.00000 \nonumber\\
heavily & 1.00000 \nonumber\\
heavily_believe & 1.00000 \nonumber\\
great_and & 1.00000 \nonumber\\
municipal_water & 1.00000 \nonumber\\
municipal & 1.00000 \nonumber\\
come_a & 1.00000 \nonumber\\
report & 1.00000 \nonumber\\
bmw_. & 1.00000 \nonumber\\
existence_be & 1.00000 \nonumber\\
you_fail & 1.00000 \nonumber\\
"_order & 1.00000 \nonumber\\
"_existence & 1.00000 \nonumber\\
bmw & 1.00000 \nonumber\\
aggressive & 1.00000 \nonumber\\
aggressive_as & 1.00000 \nonumber\\
good_read & 1.00000 \nonumber\\
equally_well & 1.00000 \nonumber\\
within_a & 1.00000 \nonumber\\
well_write & 1.00000 \nonumber\\
fall_for & 1.00000 \nonumber\\
significance_of & 1.00000 \nonumber\\
'_watch & 1.00000 \nonumber\\
god_dilusion & 1.00000 \nonumber\\
old_' & 1.00000 \nonumber\\
as_his & 1.00000 \nonumber\\
dilusion & 1.00000 \nonumber\\
a_naturally & 1.00000 \nonumber\\
his_more & 1.00000 \nonumber\\
order_and & 1.00000 \nonumber\\
a_bmw & 1.00000 \nonumber\\
replicate & 1.00000 \nonumber\\
be_fall & 1.00000 \nonumber\\
gene_" & 1.00000 \nonumber\\
dawkin & 1.00000 \nonumber\\
detail_. & 1.00000 \nonumber\\
select_environment & 1.00000 \nonumber\\
replicate_system & 1.00000 \nonumber\\
dawkin_. & 1.00000 \nonumber\\
maker & 1.00000 \nonumber\\
ProductionRule_FRAG->``,ADJP,.,'', & 1.00000 \nonumber\\
self_replicate & 1.00000 \nonumber\\
recent_" & 1.00000 \nonumber\\
not_as & 1.00000 \nonumber\\
richard_dawkin & 1.00000 \nonumber\\
richard & 1.00000 \nonumber\\
define_" & 1.00000 \nonumber\\
selfish_gene & 1.00000 \nonumber\\
write_. & 1.00000 \nonumber\\
to_recognize & 1.00000 \nonumber\\
the_significance & 1.00000 \nonumber\\
ProductionRule_ADJP->NP,CC,ADJP, & 1.00000 \nonumber\\
the_selfish & 1.00000 \nonumber\\
dilusion_, & 1.00000 \nonumber\\
naturally & 1.00000 \nonumber\\
watch_maker & 1.00000 \nonumber\\
recognize_the & 1.00000 \nonumber\\
maker_' & 1.00000 \nonumber\\
and_equally & 1.00000 \nonumber\\
system_within & 1.00000 \nonumber\\
as_aggressive & 1.00000 \nonumber\\
_pos_ngram_PUNC_O_CONJ & 1.00000 \nonumber\\
naturally_select & 1.00000 \nonumber\\
by_richard & 1.00000 \nonumber\\
and_detail & 1.00000 \nonumber\\
_pos_ngram_ADJ_V_PR & 1.00000 \nonumber\\
whether_or & 1.00000 \nonumber\\
_pos_ngram_PP_CONJ_ADV & 1.00000 \nonumber\\
that_work & 1.00000 \nonumber\\
those_that & 1.00000 \nonumber\\
although_i & 1.00000 \nonumber\\
i_still & 1.00000 \nonumber\\
life_then & 1.00000 \nonumber\\
group_. & 1.00000 \nonumber\\
ProductionRule_ADJP->NP,JJR, & 1.00000 \nonumber\\
the_couch & 1.00000 \nonumber\\
judge_what & 1.00000 \nonumber\\
_pos_ngram_O_CONJ_NP & 1.00000 \nonumber\\
in_to & 1.00000 \nonumber\\
turn_on & 1.00000 \nonumber\\
dont_like & 1.00000 \nonumber\\
think_we & 1.00000 \nonumber\\
most_certainly & 1.00000 \nonumber\\
baby_would & 1.00000 \nonumber\\
baby_whoever & 1.00000 \nonumber\\
baby_' & 1.00000 \nonumber\\
excuse_in & 1.00000 \nonumber\\
there_isnt & 1.00000 \nonumber\\
woman_with & 1.00000 \nonumber\\
whoever_they & 1.00000 \nonumber\\
speak_for & 1.00000 \nonumber\\
certainly_be & 1.00000 \nonumber\\
isnt & 1.00000 \nonumber\\
fetus_, & 1.00000 \nonumber\\
should_speak & 1.00000 \nonumber\\
be_should & 1.00000 \nonumber\\
it_most & 1.00000 \nonumber\\
isnt_an & 1.00000 \nonumber\\
ProductionRule_NP->NP,PP,S, & 1.00000 \nonumber\\
a_single & 1.00000 \nonumber\\
your_cat & 1.00000 \nonumber\\
tax_report & 1.00000 \nonumber\\
ProductionRule_NP->PRP$,NN,CC,NN, & 1.00000 \nonumber\\
or_dog & 1.00000 \nonumber\\
income_tax & 1.00000 \nonumber\\
!_evolution & 1.00000 \nonumber\\
dog_try & 1.00000 \nonumber\\
your_income & 1.00000 \nonumber\\
understand_god & 1.00000 \nonumber\\
ProductionRule_SBAR->IN,S,,, & 1.00000 \nonumber\\
income & 1.00000 \nonumber\\
and_creation & 1.00000 \nonumber\\
cat & 1.00000 \nonumber\\
cat_or & 1.00000 \nonumber\\
creation_go & 1.00000 \nonumber\\
report_! & 1.00000 \nonumber\\
hand_! & 1.00000 \nonumber\\
understand_your & 1.00000 \nonumber\\
some_parent & 1.00000 \nonumber\\
myself_. & 1.00000 \nonumber\\
uniform_make & 1.00000 \nonumber\\
how_much & 1.00000 \nonumber\\
fastest_and & 1.00000 \nonumber\\
source_like & 1.00000 \nonumber\\
plus_its & 1.00000 \nonumber\\
like_firefox & 1.00000 \nonumber\\
safest & 1.00000 \nonumber\\
the_safest & 1.00000 \nonumber\\
_pos_ngram_ART_PR_ART & 1.00000 \nonumber\\
all_its & 1.00000 \nonumber\\
open_source & 1.00000 \nonumber\\
chorme & 1.00000 \nonumber\\
also_open & 1.00000 \nonumber\\
the_fastest & 1.00000 \nonumber\\
safest_plus & 1.00000 \nonumber\\
beat_all & 1.00000 \nonumber\\
chorme_beat & 1.00000 \nonumber\\
5_year & 1.00000 \nonumber\\
of_firefox & 1.00000 \nonumber\\
credit & 1.00000 \nonumber\\
each_year & 1.00000 \nonumber\\
let_' & 1.00000 \nonumber\\
ProductionRule_SBAR->RB,S, & 1.00000 \nonumber\\
ProductionRule_NP->NP,ADVP,SBAR, & 1.00000 \nonumber\\
ProductionRule_INTJ->JJ,., & 1.00000 \nonumber\\
so_take & 1.00000 \nonumber\\
one_for & 1.00000 \nonumber\\
to_explain & 1.00000 \nonumber\\
lazy_to & 1.00000 \nonumber\\
for_4 & 1.00000 \nonumber\\
take_my & 1.00000 \nonumber\\
explain_why & 1.00000 \nonumber\\
why_so & 1.00000 \nonumber\\
year_at & 1.00000 \nonumber\\
scar & 1.00000 \nonumber\\
christian_or & 1.00000 \nonumber\\
a_guy & 1.00000 \nonumber\\
understand_evolution & 1.00000 \nonumber\\
i_rather & 1.00000 \nonumber\\
way_that & 1.00000 \nonumber\\
ProductionRule_VP->VBP,NP,,,SBAR, & 1.00000 \nonumber\\
_pos_ngram_CONJ_PUNC & 1.00000 \nonumber\\
supernatural_as & 1.00000 \nonumber\\
natural_world & 1.00000 \nonumber\\
call_pseudo-science & 1.00000 \nonumber\\
the_supernatural & 1.00000 \nonumber\\
supernatural & 1.00000 \nonumber\\
)_have & 1.00000 \nonumber\\
claim_be & 1.00000 \nonumber\\
method_deal & 1.00000 \nonumber\\
sneak_the & 1.00000 \nonumber\\
their_claim & 1.00000 \nonumber\\
._creationism & 1.00000 \nonumber\\
let_first & 1.00000 \nonumber\\
sneak & 1.00000 \nonumber\\
to_sneak & 1.00000 \nonumber\\
first_know & 1.00000 \nonumber\\
deal_only & 1.00000 \nonumber\\
only_with & 1.00000 \nonumber\\
explanation_. & 1.00000 \nonumber\\
theological_claim & 1.00000 \nonumber\\
creationism_try & 1.00000 \nonumber\\
the_refute & 1.00000 \nonumber\\
know_through & 1.00000 \nonumber\\
will_rebuttal & 1.00000 \nonumber\\
a_science & 1.00000 \nonumber\\
after_this & 1.00000 \nonumber\\
rebuttal_after & 1.00000 \nonumber\\
the_natural & 1.00000 \nonumber\\
this_) & 1.00000 \nonumber\\
refute_i & 1.00000 \nonumber\\
what_science & 1.00000 \nonumber\\
see_( & 1.00000 \nonumber\\
a_scientific & 1.00000 \nonumber\\
scientific_explanation & 1.00000 \nonumber\\
be_theological & 1.00000 \nonumber\\
and_die & 1.00000 \nonumber\\
ProductionRule_VP->VBP,NP,ADVP, & 1.00000 \nonumber\\
self_. & 1.00000 \nonumber\\
buy_a & 1.00000 \nonumber\\
can_cause & 1.00000 \nonumber\\
of_anger & 1.00000 \nonumber\\
ProductionRule_ADVP->DT,RP, & 1.00000 \nonumber\\
do_like & 1.00000 \nonumber\\
if_some & 1.00000 \nonumber\\
mostly_out & 1.00000 \nonumber\\
ProductionRule_ADJP->IN,PP, & 1.00000 \nonumber\\
thy_let & 1.00000 \nonumber\\
thy & 1.00000 \nonumber\\
else_make & 1.00000 \nonumber\\
make_thm & 1.00000 \nonumber\\
more_then & 1.00000 \nonumber\\
thm_mad & 1.00000 \nonumber\\
on_thm & 1.00000 \nonumber\\
thm & 1.00000 \nonumber\\
kid_have & 1.00000 \nonumber\\
mad_thy & 1.00000 \nonumber\\
from_all & 1.00000 \nonumber\\
fat_and & 1.00000 \nonumber\\
and_many & 1.00000 \nonumber\\
strive_to & 1.00000 \nonumber\\
strive & 1.00000 \nonumber\\
while_the & 1.00000 \nonumber\\
person_if & 1.00000 \nonumber\\
feel_if & 1.00000 \nonumber\\
so_you & 1.00000 \nonumber\\
._be & 1.00000 \nonumber\\
book_can & 1.00000 \nonumber\\
dear_and & 1.00000 \nonumber\\
violent_or & 1.00000 \nonumber\\
the_stuff & 1.00000 \nonumber\\
ProductionRule_ADJP->CC,ADJP,CC,ADJP, & 1.00000 \nonumber\\
tv_licence & 1.00000 \nonumber\\
licence_book & 1.00000 \nonumber\\
really_dear & 1.00000 \nonumber\\
kid_so & 1.00000 \nonumber\\
well_better & 1.00000 \nonumber\\
licence & 1.00000 \nonumber\\
tv_it & 1.00000 \nonumber\\
ProductionRule_VP->VB,ADVP,ADJP, & 1.00000 \nonumber\\
either_violent & 1.00000 \nonumber\\
cheaper & 1.00000 \nonumber\\
stuff_on & 1.00000 \nonumber\\
dear & 1.00000 \nonumber\\
be_cheaper & 1.00000 \nonumber\\
cheaper_to & 1.00000 \nonumber\\
learn_a & 1.00000 \nonumber\\
a_tv & 1.00000 \nonumber\\
package & 1.00000 \nonumber\\
ProductionRule_SBAR->UCP,S, & 1.00000 \nonumber\\
ProductionRule_VP->VBN,CC,VBN, & 1.00000 \nonumber\\
way_this & 1.00000 \nonumber\\
i_truly & 1.00000 \nonumber\\
if_our & 1.00000 \nonumber\\
alway_their & 1.00000 \nonumber\\
that_protect & 1.00000 \nonumber\\
trust_that & 1.00000 \nonumber\\
to_throw & 1.00000 \nonumber\\
even_trust & 1.00000 \nonumber\\
our_father & 1.00000 \nonumber\\
you_how & 1.00000 \nonumber\\
baseball_game & 1.00000 \nonumber\\
protect_you & 1.00000 \nonumber\\
and_spend & 1.00000 \nonumber\\
then_how & 1.00000 \nonumber\\
game_. & 1.00000 \nonumber\\
you_trust & 1.00000 \nonumber\\
his_room & 1.00000 \nonumber\\
throw_a & 1.00000 \nonumber\\
room_, & 1.00000 \nonumber\\
spend_most & 1.00000 \nonumber\\
the_evil & 1.00000 \nonumber\\
time_trust & 1.00000 \nonumber\\
a_baseball & 1.00000 \nonumber\\
that_teach & 1.00000 \nonumber\\
you_baseball & 1.00000 \nonumber\\
and_come & 1.00000 \nonumber\\
evil_of & 1.00000 \nonumber\\
stick_with & 1.00000 \nonumber\\
ProductionRule_VP->VBG,NP,SBAR, & 1.00000 \nonumber\\
inside & 1.00000 \nonumber\\
life_if & 1.00000 \nonumber\\
._actually & 1.00000 \nonumber\\
be_hell & 1.00000 \nonumber\\
hell_. & 1.00000 \nonumber\\
ProductionRule_ADJP->ADJP,PP,., & 1.00000 \nonumber\\
christianity_of & 1.00000 \nonumber\\
imagine_life & 1.00000 \nonumber\\
actually_i & 1.00000 \nonumber\\
with_murder & 1.00000 \nonumber\\
_pos_ngram_PR_CARD & 1.00000 \nonumber\\
but_book & 1.00000 \nonumber\\
of_information & 1.00000 \nonumber\\
from_different & 1.00000 \nonumber\\
resource_in & 1.00000 \nonumber\\
,_!! & 1.00000 \nonumber\\
different_resource & 1.00000 \nonumber\\
a_short & 1.00000 \nonumber\\
!!_because & 1.00000 \nonumber\\
short_time & 1.00000 \nonumber\\
ProductionRule_FRAG->,,NP, & 1.00000 \nonumber\\
get_information & 1.00000 \nonumber\\
get_that & 1.00000 \nonumber\\
ProductionRule_NP->NP,,,FRAG, & 1.00000 \nonumber\\
must_read & 1.00000 \nonumber\\
information_!! & 1.00000 \nonumber\\
pc & 1.00000 \nonumber\\
_pos_ngram_CONJ_ADJ_V & 1.00000 \nonumber\\
a_puzzle & 1.00000 \nonumber\\
wand_. & 1.00000 \nonumber\\
_pos_ngram_CONJ_O_NP & 1.00000 \nonumber\\
wand & 1.00000 \nonumber\\
magic_wand & 1.00000 \nonumber\\
in_" & 1.00000 \nonumber\\
godly & 1.00000 \nonumber\\
a_magic & 1.00000 \nonumber\\
godly_finger & 1.00000 \nonumber\\
and_" & 1.00000 \nonumber\\
your_line & 1.00000 \nonumber\\
along_your & 1.00000 \nonumber\\
piece_with & 1.00000 \nonumber\\
god_would & 1.00000 \nonumber\\
,_believe & 1.00000 \nonumber\\
creationism_" & 1.00000 \nonumber\\
his_godly & 1.00000 \nonumber\\
by_wave & 1.00000 \nonumber\\
finger_would & 1.00000 \nonumber\\
you_clearly & 1.00000 \nonumber\\
book_or & 1.00000 \nonumber\\
touch_the & 1.00000 \nonumber\\
actually_touch & 1.00000 \nonumber\\
but_along & 1.00000 \nonumber\\
"_creationism & 1.00000 \nonumber\\
wave_a & 1.00000 \nonumber\\
he_? & 1.00000 \nonumber\\
clearly_do & 1.00000 \nonumber\\
and_find & 1.00000 \nonumber\\
claim_to & 1.00000 \nonumber\\
not_spank & 1.00000 \nonumber\\
way_they & 1.00000 \nonumber\\
oppose & 1.00000 \nonumber\\
at_it & 1.00000 \nonumber\\
_pos_ngram_ADJ_CARD_V & 1.00000 \nonumber\\
them_but & 1.00000 \nonumber\\
dont_need & 1.00000 \nonumber\\
best_. & 1.00000 \nonumber\\
stop_singapore & 1.00000 \nonumber\\
upset_that & 1.00000 \nonumber\\
stop_the & 1.00000 \nonumber\\
upset & 1.00000 \nonumber\\
ProductionRule_ADJP->VBN,SBAR, & 1.00000 \nonumber\\
dutch_be & 1.00000 \nonumber\\
be_upset & 1.00000 \nonumber\\
from_take & 1.00000 \nonumber\\
take_by & 1.00000 \nonumber\\
dutch_would & 1.00000 \nonumber\\
dutch_from & 1.00000 \nonumber\\
raffle_stop & 1.00000 \nonumber\\
from_be & 1.00000 \nonumber\\
dutch_, & 1.00000 \nonumber\\
take_singapore & 1.00000 \nonumber\\
who_stop & 1.00000 \nonumber\\
2012 & 1.00000 \nonumber\\
2012_. & 1.00000 \nonumber\\
world_after & 1.00000 \nonumber\\
after_2012 & 1.00000 \nonumber\\
grow_faster & 1.00000 \nonumber\\
ProductionRule_PP->IN,NP,PP, & 1.00000 \nonumber\\
will_grow & 1.00000 \nonumber\\
country_of & 1.00000 \nonumber\\
publicly_distribute & 1.00000 \nonumber\\
much_money & 1.00000 \nonumber\\
girl_to & 1.00000 \nonumber\\
would_feel & 1.00000 \nonumber\\
the_younger & 1.00000 \nonumber\\
only_here & 1.00000 \nonumber\\
jack & 1.00000 \nonumber\\
make_so & 1.00000 \nonumber\\
be_buy & 1.00000 \nonumber\\
off_' & 1.00000 \nonumber\\
king_sense & 1.00000 \nonumber\\
nake_girl & 1.00000 \nonumber\\
common_f & 1.00000 \nonumber\\
and_stupid & 1.00000 \nonumber\\
younger_youth & 1.00000 \nonumber\\
wtf & 1.00000 \nonumber\\
and_our & 1.00000 \nonumber\\
inside_we & 1.00000 \nonumber\\
try_watch & 1.00000 \nonumber\\
,_friend & 1.00000 \nonumber\\
know_why & 1.00000 \nonumber\\
to_publicly & 1.00000 \nonumber\\
conscience_deep & 1.00000 \nonumber\\
can_jack & 1.00000 \nonumber\\
jack_off & 1.00000 \nonumber\\
uncomfortable_and & 1.00000 \nonumber\\
here_because & 1.00000 \nonumber\\
wtf_. & 1.00000 \nonumber\\
mean_wtf & 1.00000 \nonumber\\
distribute_it & 1.00000 \nonumber\\
sense_and & 1.00000 \nonumber\\
hell_yeah & 1.00000 \nonumber\\
yeah_porn & 1.00000 \nonumber\\
our_conscience & 1.00000 \nonumber\\
yeah_you & 1.00000 \nonumber\\
why_? & 1.00000 \nonumber\\
youth_. & 1.00000 \nonumber\\
family_, & 1.00000 \nonumber\\
deep_inside & 1.00000 \nonumber\\
publicly & 1.00000 \nonumber\\
so_jerk & 1.00000 \nonumber\\
film_nake & 1.00000 \nonumber\\
into_it & 1.00000 \nonumber\\
stupid_people & 1.00000 \nonumber\\
'_can & 1.00000 \nonumber\\
buy_into & 1.00000 \nonumber\\
._film & 1.00000 \nonumber\\
internet_so & 1.00000 \nonumber\\
instance_, & 1.00000 \nonumber\\
for_instance & 1.00000 \nonumber\\
supporter_. & 1.00000 \nonumber\\
some_straight & 1.00000 \nonumber\\
and_care & 1.00000 \nonumber\\
i.e_have & 1.00000 \nonumber\\
get_kid & 1.00000 \nonumber\\
marriage_if & 1.00000 \nonumber\\
marry_for & 1.00000 \nonumber\\
its_benefit & 1.00000 \nonumber\\
develop_society & 1.00000 \nonumber\\
benefit_? & 1.00000 \nonumber\\
gay_rights & 1.00000 \nonumber\\
only_get & 1.00000 \nonumber\\
this_matter & 1.00000 \nonumber\\
marriage_of & 1.00000 \nonumber\\
case_? & 1.00000 \nonumber\\
have_kid & 1.00000 \nonumber\\
couple_just & 1.00000 \nonumber\\
way_do & 1.00000 \nonumber\\
to_reap & 1.00000 \nonumber\\
agnostic_so & 1.00000 \nonumber\\
ProductionRule_NP->NP,VP,., & 1.00000 \nonumber\\
i.e & 1.00000 \nonumber\\
?_i.e & 1.00000 \nonumber\\
term_and & 1.00000 \nonumber\\
?_as & 1.00000 \nonumber\\
rights_supporter & 1.00000 \nonumber\\
avid_gay & 1.00000 \nonumber\\
religion_conflict & 1.00000 \nonumber\\
of_2 & 1.00000 \nonumber\\
an_agnostic & 1.00000 \nonumber\\
a_develop & 1.00000 \nonumber\\
if_2 & 1.00000 \nonumber\\
people_only & 1.00000 \nonumber\\
about_each & 1.00000 \nonumber\\
reap_its & 1.00000 \nonumber\\
2_people & 1.00000 \nonumber\\
to_term & 1.00000 \nonumber\\
reap & 1.00000 \nonumber\\
kid_? & 1.00000 \nonumber\\
also_it & 1.00000 \nonumber\\
against_gay & 1.00000 \nonumber\\
10_, & 1.00000 \nonumber\\
load_time & 1.00000 \nonumber\\
just_install & 1.00000 \nonumber\\
load_up & 1.00000 \nonumber\\
will_experience & 1.00000 \nonumber\\
ff_load & 1.00000 \nonumber\\
load_faster & 1.00000 \nonumber\\
ff_will & 1.00000 \nonumber\\
_pos_ngram_PUNC_CONJ_CARD & 1.00000 \nonumber\\
say_ff & 1.00000 \nonumber\\
time_than & 1.00000 \nonumber\\
they_say & 1.00000 \nonumber\\
program_load & 1.00000 \nonumber\\
slower_program & 1.00000 \nonumber\\
ProductionRule_VP->VBD,ADVP,VP, & 1.00000 \nonumber\\
up_ie & 1.00000 \nonumber\\
ProductionRule_NP->JJR,NN,NN,NNS, & 1.00000 \nonumber\\
experience_slower & 1.00000 \nonumber\\
slower & 1.00000 \nonumber\\
but_9 & 1.00000 \nonumber\\
than_load & 1.00000 \nonumber\\
install_ff & 1.00000 \nonumber\\
trust_. & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,ADVP,SBAR, & 1.00000 \nonumber\\
i_beleive & 1.00000 \nonumber\\
beleive_that & 1.00000 \nonumber\\
and_less & 1.00000 \nonumber\\
..._" & 1.00000 \nonumber\\
nature_to & 1.00000 \nonumber\\
5_cent & 1.00000 \nonumber\\
two_brand & 1.00000 \nonumber\\
-_and & 1.00000 \nonumber\\
from_vend & 1.00000 \nonumber\\
coca-cola & 1.00000 \nonumber\\
water_cost & 1.00000 \nonumber\\
._assume & 1.00000 \nonumber\\
assume_you & 1.00000 \nonumber\\
aquafina_or & 1.00000 \nonumber\\
a_$ & 1.00000 \nonumber\\
1_machine & 1.00000 \nonumber\\
dasanus_bottle & 1.00000 \nonumber\\
machine_, & 1.00000 \nonumber\\
cost_less & 1.00000 \nonumber\\
20_ounce & 1.00000 \nonumber\\
1_cent & 1.00000 \nonumber\\
sell_in & 1.00000 \nonumber\\
for_something & 1.00000 \nonumber\\
_pos_ngram_O_NP_ADJ & 1.00000 \nonumber\\
gallon_. & 1.00000 \nonumber\\
machine_alongside & 1.00000 \nonumber\\
or_coca-cola & 1.00000 \nonumber\\
coca-cola_' & 1.00000 \nonumber\\
to_5 & 1.00000 \nonumber\\
brand_be & 1.00000 \nonumber\\
distribution & 1.00000 \nonumber\\
your_sink & 1.00000 \nonumber\\
bottle_close & 1.00000 \nonumber\\
distribution_point & 1.00000 \nonumber\\
ProductionRule_VP->VB,,,FRAG, & 1.00000 \nonumber\\
'_dasanus & 1.00000 \nonumber\\
alongside & 1.00000 \nonumber\\
ProductionRule_NP->NP,NNP,JJ,NN, & 1.00000 \nonumber\\
be_sell & 1.00000 \nonumber\\
drink_- & 1.00000 \nonumber\\
most_municipal & 1.00000 \nonumber\\
alongside_soft & 1.00000 \nonumber\\
vend_machine & 1.00000 \nonumber\\
vend & 1.00000 \nonumber\\
size_and & 1.00000 \nonumber\\
their_distribution & 1.00000 \nonumber\\
be_purchase & 1.00000 \nonumber\\
essentially_filter & 1.00000 \nonumber\\
pepsi_' & 1.00000 \nonumber\\
ounce_. & 1.00000 \nonumber\\
ounce_size & 1.00000 \nonumber\\
per_gallon & 1.00000 \nonumber\\
in_20 & 1.00000 \nonumber\\
can_find & 1.00000 \nonumber\\
an_ounce & 1.00000 \nonumber\\
cent_per & 1.00000 \nonumber\\
_pos_ngram_ART_O_CARD & 1.00000 \nonumber\\
cent_an & 1.00000 \nonumber\\
cent & 1.00000 \nonumber\\
,_pepsi & 1.00000 \nonumber\\
ProductionRule_FRAG->PP,,,NP,., & 1.00000 \nonumber\\
'_aquafina & 1.00000 \nonumber\\
you_pay & 1.00000 \nonumber\\
price_. & 1.00000 \nonumber\\
same_price & 1.00000 \nonumber\\
$_1 & 1.00000 \nonumber\\
soft_drink & 1.00000 \nonumber\\
purchase_from & 1.00000 \nonumber\\
make_him & 1.00000 \nonumber\\
matter_where & 1.00000 \nonumber\\
to_understand & 1.00000 \nonumber\\
and_without & 1.00000 \nonumber\\
(_s & 1.00000 \nonumber\\
s_) & 1.00000 \nonumber\\
wrong_" & 1.00000 \nonumber\\
any_country & 1.00000 \nonumber\\
myself_to & 1.00000 \nonumber\\
healp & 1.00000 \nonumber\\
laptop_then & 1.00000 \nonumber\\
god_will & 1.00000 \nonumber\\
school_laptop & 1.00000 \nonumber\\
laptop & 1.00000 \nonumber\\
god_help & 1.00000 \nonumber\\
themselve_! & 1.00000 \nonumber\\
who_help & 1.00000 \nonumber\\
healp_myself & 1.00000 \nonumber\\
and_healp & 1.00000 \nonumber\\
then_god & 1.00000 \nonumber\\
help_themselve & 1.00000 \nonumber\\
help_those & 1.00000 \nonumber\\
firefox_. & 1.00000 \nonumber\\
still_the & 1.00000 \nonumber\\
_pos_ngram_PR_PR_ART & 1.00000 \nonumber\\
cute & 1.00000 \nonumber\\
kid_do & 1.00000 \nonumber\\
people_like & 1.00000 \nonumber\\
marriage_in & 1.00000 \nonumber\\
sin_to & 1.00000 \nonumber\\
the_hell & 1.00000 \nonumber\\
marriage_kill & 1.00000 \nonumber\\
hell_do & 1.00000 \nonumber\\
._bottom & 1.00000 \nonumber\\
straight_ppl & 1.00000 \nonumber\\
offensive_? & 1.00000 \nonumber\\
accept_everyone & 1.00000 \nonumber\\
offensive & 1.00000 \nonumber\\
._enough & 1.00000 \nonumber\\
in_anyway & 1.00000 \nonumber\\
enough_say & 1.00000 \nonumber\\
affect_anyone & 1.00000 \nonumber\\
marriage_go & 1.00000 \nonumber\\
end_the & 1.00000 \nonumber\\
follow_that & 1.00000 \nonumber\\
bottom_line & 1.00000 \nonumber\\
bottom & 1.00000 \nonumber\\
to_kep & 1.00000 \nonumber\\
marrage_to & 1.00000 \nonumber\\
hurt_anyone & 1.00000 \nonumber\\
ppl_get & 1.00000 \nonumber\\
marriage_hurt & 1.00000 \nonumber\\
else_to & 1.00000 \nonumber\\
between_you & 1.00000 \nonumber\\
to_end & 1.00000 \nonumber\\
line_, & 1.00000 \nonumber\\
other_apart & 1.00000 \nonumber\\
show_they & 1.00000 \nonumber\\
world_? & 1.00000 \nonumber\\
his_people & 1.00000 \nonumber\\
so_offensive & 1.00000 \nonumber\\
you_fine & 1.00000 \nonumber\\
kep_two & 1.00000 \nonumber\\
two_get & 1.00000 \nonumber\\
fine_let & 1.00000 \nonumber\\
anyone_but & 1.00000 \nonumber\\
kep & 1.00000 \nonumber\\
anyone_? & 1.00000 \nonumber\\
god_accept & 1.00000 \nonumber\\
marry_? & 1.00000 \nonumber\\
do_straight & 1.00000 \nonumber\\
anyway_affect & 1.00000 \nonumber\\
apart_. & 1.00000 \nonumber\\
ProductionRule_SQ->VBP,NP,ADJP,., & 1.00000 \nonumber\\
why_the & 1.00000 \nonumber\\
something_else & 1.00000 \nonumber\\
want_marrage & 1.00000 \nonumber\\
gold & 1.00000 \nonumber\\
_pos_ngram_O_CARD_PR & 1.00000 \nonumber\\
language & 1.00000 \nonumber\\
be_reuse & 1.00000 \nonumber\\
that_bottle & 1.00000 \nonumber\\
waste_, & 1.00000 \nonumber\\
reuse_! & 1.00000 \nonumber\\
but_bottle & 1.00000 \nonumber\\
other_way & 1.00000 \nonumber\\
fiber_material & 1.00000 \nonumber\\
fill_cup & 1.00000 \nonumber\\
or_carpet & 1.00000 \nonumber\\
re_use & 1.00000 \nonumber\\
re & 1.00000 \nonumber\\
fiber & 1.00000 \nonumber\\
carpet_. & 1.00000 \nonumber\\
clothe_or & 1.00000 \nonumber\\
and_re & 1.00000 \nonumber\\
make_into & 1.00000 \nonumber\\
cup_with & 1.00000 \nonumber\\
cup & 1.00000 \nonumber\\
just_fill & 1.00000 \nonumber\\
material_, & 1.00000 \nonumber\\
ProductionRule_VP->ADVP,VB,VP, & 1.00000 \nonumber\\
like_clothe & 1.00000 \nonumber\\
into_long & 1.00000 \nonumber\\
carpet & 1.00000 \nonumber\\
term_fiber & 1.00000 \nonumber\\
ProductionRule_NP->LS,RB, & 1.00000 \nonumber\\
conscience & 1.00000 \nonumber\\
or_two & 1.00000 \nonumber\\
react & 1.00000 \nonumber\\
creation_be & 1.00000 \nonumber\\
make_new & 1.00000 \nonumber\\
frustrate & 1.00000 \nonumber\\
alimony & 1.00000 \nonumber\\
roomate_to & 1.00000 \nonumber\\
roomate & 1.00000 \nonumber\\
say_let & 1.00000 \nonumber\\
of_asset & 1.00000 \nonumber\\
it_too & 1.00000 \nonumber\\
custody & 1.00000 \nonumber\\
split_of & 1.00000 \nonumber\\
,_alimony & 1.00000 \nonumber\\
,_custody & 1.00000 \nonumber\\
illegal_; & 1.00000 \nonumber\\
alimony_, & 1.00000 \nonumber\\
,_regardless & 1.00000 \nonumber\\
custody_, & 1.00000 \nonumber\\
divorce_, & 1.00000 \nonumber\\
"_from & 1.00000 \nonumber\\
joy & 1.00000 \nonumber\\
"_walk & 1.00000 \nonumber\\
marraige & 1.00000 \nonumber\\
encourage_roomate & 1.00000 \nonumber\\
joy_of & 1.00000 \nonumber\\
marraige_, & 1.00000 \nonumber\\
people_know & 1.00000 \nonumber\\
"_couple & 1.00000 \nonumber\\
a_buddy & 1.00000 \nonumber\\
yard_! & 1.00000 \nonumber\\
orientation_, & 1.00000 \nonumber\\
couple_" & 1.00000 \nonumber\\
too_easy & 1.00000 \nonumber\\
miserable_. & 1.00000 \nonumber\\
miserable & 1.00000 \nonumber\\
yard & 1.00000 \nonumber\\
,_split & 1.00000 \nonumber\\
of_divorce & 1.00000 \nonumber\\
nine_yard & 1.00000 \nonumber\\
buddy_out & 1.00000 \nonumber\\
let_gay & 1.00000 \nonumber\\
buddy & 1.00000 \nonumber\\
be_miserable & 1.00000 \nonumber\\
benefits.civil_union & 1.00000 \nonumber\\
with_benefits.civil & 1.00000 \nonumber\\
asset_, & 1.00000 \nonumber\\
whole_nine & 1.00000 \nonumber\\
asset & 1.00000 \nonumber\\
the_joy & 1.00000 \nonumber\\
walk_away & 1.00000 \nonumber\\
away_" & 1.00000 \nonumber\\
make_civil & 1.00000 \nonumber\\
child_support & 1.00000 \nonumber\\
union_illegal & 1.00000 \nonumber\\
benefits.civil & 1.00000 \nonumber\\
gay_marraige & 1.00000 \nonumber\\
marriage_as & 1.00000 \nonumber\\
:_it & 1.00000 \nonumber\\
on_them & 1.00000 \nonumber\\
wife_or & 1.00000 \nonumber\\
us_have & 1.00000 \nonumber\\
prevert & 1.00000 \nonumber\\
be_lustful & 1.00000 \nonumber\\
lustful_before & 1.00000 \nonumber\\
,_count & 1.00000 \nonumber\\
marry_because & 1.00000 \nonumber\\
lustful & 1.00000 \nonumber\\
prevert_way & 1.00000 \nonumber\\
count_as & 1.00000 \nonumber\\
before_, & 1.00000 \nonumber\\
not_judge & 1.00000 \nonumber\\
which_believe & 1.00000 \nonumber\\
a_prevert & 1.00000 \nonumber\\
it_or & 1.00000 \nonumber\\
lustful_: & 1.00000 \nonumber\\
at_another & 1.00000 \nonumber\\
cheat_on & 1.00000 \nonumber\\
stop_. & 1.00000 \nonumber\\
your_wife & 1.00000 \nonumber\\
or_husband & 1.00000 \nonumber\\
judge_you & 1.00000 \nonumber\\
as_cheat & 1.00000 \nonumber\\
mother_do & 1.00000 \nonumber\\
bum_for & 1.00000 \nonumber\\
be_set & 1.00000 \nonumber\\
can_raise & 1.00000 \nonumber\\
well_at & 1.00000 \nonumber\\
why_keep & 1.00000 \nonumber\\
keep_him & 1.00000 \nonumber\\
better_fatherless & 1.00000 \nonumber\\
father_your & 1.00000 \nonumber\\
lousy_just & 1.00000 \nonumber\\
fatherless_the & 1.00000 \nonumber\\
mother_can & 1.00000 \nonumber\\
him_? & 1.00000 \nonumber\\
least_my & 1.00000 \nonumber\\
a_bum & 1.00000 \nonumber\\
him_so & 1.00000 \nonumber\\
set_example & 1.00000 \nonumber\\
that_type & 1.00000 \nonumber\\
son_the & 1.00000 \nonumber\\
teach_to & 1.00000 \nonumber\\
bum & 1.00000 \nonumber\\
_pos_ngram_O_CARD_CONJ & 1.00000 \nonumber\\
would_hope & 1.00000 \nonumber\\
anybody_. & 1.00000 \nonumber\\
police_catch & 1.00000 \nonumber\\
catch_them & 1.00000 \nonumber\\
turn_their & 1.00000 \nonumber\\
to_weird & 1.00000 \nonumber\\
weird_for & 1.00000 \nonumber\\
tell_anybody & 1.00000 \nonumber\\
the_word & 1.00000 \nonumber\\
,_by & 1.00000 \nonumber\\
go_figure & 1.00000 \nonumber\\
be_wayyyyy & 1.00000 \nonumber\\
wayyyyy & 1.00000 \nonumber\\
._go & 1.00000 \nonumber\\
wayyyyy_better & 1.00000 \nonumber\\
ProductionRule_S->S,S,., & 1.00000 \nonumber\\
figure_why & 1.00000 \nonumber\\
more_focus & 1.00000 \nonumber\\
make_money & 1.00000 \nonumber\\
biblical & 1.00000 \nonumber\\
come_out & 1.00000 \nonumber\\
exploitation_. & 1.00000 \nonumber\\
exploitation & 1.00000 \nonumber\\
expression_that & 1.00000 \nonumber\\
for_exploitation & 1.00000 \nonumber\\
ProductionRule_NP->NN,SBAR, & 1.00000 \nonumber\\
wrong_than & 1.00000 \nonumber\\
most_if & 1.00000 \nonumber\\
water_in & 1.00000 \nonumber\\
alawy_feel & 1.00000 \nonumber\\
and_terror & 1.00000 \nonumber\\
beat_your & 1.00000 \nonumber\\
anything_for & 1.00000 \nonumber\\
alcoholic & 1.00000 \nonumber\\
mother_, & 1.00000 \nonumber\\
ProductionRule_S->S,,,RB,S,., & 1.00000 \nonumber\\
family.imagine & 1.00000 \nonumber\\
father.he & 1.00000 \nonumber\\
and_beat & 1.00000 \nonumber\\
alcoholic_and & 1.00000 \nonumber\\
you_alawy & 1.00000 \nonumber\\
terror_in & 1.00000 \nonumber\\
the_family.imagine & 1.00000 \nonumber\\
alawy & 1.00000 \nonumber\\
no_mean & 1.00000 \nonumber\\
father.he_create & 1.00000 \nonumber\\
violance & 1.00000 \nonumber\\
a_father.he & 1.00000 \nonumber\\
be_alcoholic & 1.00000 \nonumber\\
family.imagine_a & 1.00000 \nonumber\\
feel_ashame & 1.00000 \nonumber\\
violance_and & 1.00000 \nonumber\\
terror & 1.00000 \nonumber\\
mean_of & 1.00000 \nonumber\\
create_violance & 1.00000 \nonumber\\
rich_, & 1.00000 \nonumber\\
ProductionRule_VP->MD,S, & 1.00000 \nonumber\\
ProductionRule_VP->VP,,,ADVP,VP, & 1.00000 \nonumber\\
our_industrial & 1.00000 \nonumber\\
sector_. & 1.00000 \nonumber\\
ProductionRule_NP->PRP$,NN,,,NN,CC,JJ,NN, & 1.00000 \nonumber\\
,_suitable & 1.00000 \nonumber\\
salary.so_its & 1.00000 \nonumber\\
work_environment & 1.00000 \nonumber\\
be_qualify & 1.00000 \nonumber\\
superbrain.if_indium & 1.00000 \nonumber\\
will_definetly & 1.00000 \nonumber\\
of_open & 1.00000 \nonumber\\
superbrain.if & 1.00000 \nonumber\\
,_value & 1.00000 \nonumber\\
qualify_iit & 1.00000 \nonumber\\
and_astronomical & 1.00000 \nonumber\\
isro_then & 1.00000 \nonumber\\
iitian_, & 1.00000 \nonumber\\
isro & 1.00000 \nonumber\\
know_to & 1.00000 \nonumber\\
their_level.we & 1.00000 \nonumber\\
iitian & 1.00000 \nonumber\\
scientist_will & 1.00000 \nonumber\\
status_, & 1.00000 \nonumber\\
iit_, & 1.00000 \nonumber\\
iit & 1.00000 \nonumber\\
to_brain & 1.00000 \nonumber\\
proper_salary.so & 1.00000 \nonumber\\
,_lack & 1.00000 \nonumber\\
education.then & 1.00000 \nonumber\\
be_superbrain.if & 1.00000 \nonumber\\
suitable_work & 1.00000 \nonumber\\
education.then_why & 1.00000 \nonumber\\
the_hour & 1.00000 \nonumber\\
imagine_that & 1.00000 \nonumber\\
think_abt & 1.00000 \nonumber\\
recent_report & 1.00000 \nonumber\\
a_recent & 1.00000 \nonumber\\
our_status & 1.00000 \nonumber\\
international_status & 1.00000 \nonumber\\
give_international & 1.00000 \nonumber\\
salary.so & 1.00000 \nonumber\\
will_join & 1.00000 \nonumber\\
provide_them & 1.00000 \nonumber\\
definetly_increase & 1.00000 \nonumber\\
perfect_job & 1.00000 \nonumber\\
just_imagine & 1.00000 \nonumber\\
industrial_sector & 1.00000 \nonumber\\
level.we & 1.00000 \nonumber\\
value_and & 1.00000 \nonumber\\
indian_iitian & 1.00000 \nonumber\\
join_isro & 1.00000 \nonumber\\
increase_. & 1.00000 \nonumber\\
why_unable & 1.00000 \nonumber\\
advantage_from & 1.00000 \nonumber\\
of_education.then & 1.00000 \nonumber\\
hitech_institution & 1.00000 \nonumber\\
astronomical_knowledge & 1.00000 \nonumber\\
take_best & 1.00000 \nonumber\\
those_scientist & 1.00000 \nonumber\\
unable_provide & 1.00000 \nonumber\\
report_50 & 1.00000 \nonumber\\
open_hitech & 1.00000 \nonumber\\
hitech & 1.00000 \nonumber\\
them.this_be & 1.00000 \nonumber\\
hour_to & 1.00000 \nonumber\\
industrial_development & 1.00000 \nonumber\\
from_them.this & 1.00000 \nonumber\\
level.we_be & 1.00000 \nonumber\\
as_proper & 1.00000 \nonumber\\
._iitian & 1.00000 \nonumber\\
of_industrial & 1.00000 \nonumber\\
then_our & 1.00000 \nonumber\\
them.this & 1.00000 \nonumber\\
best_advantage & 1.00000 \nonumber\\
un & 1.00000 \nonumber\\
bible_, & 1.00000 \nonumber\\
or_be & 1.00000 \nonumber\\
tell_a & 1.00000 \nonumber\\
if_later & 1.00000 \nonumber\\
intentional_so & 1.00000 \nonumber\\
and_intentional & 1.00000 \nonumber\\
intentional & 1.00000 \nonumber\\
on_down & 1.00000 \nonumber\\
ProductionRule_FRAG->INTJ,,,ADVP,NP, & 1.00000 \nonumber\\
ProductionRule_VP->VBD,CC,VBD,PP, & 1.00000 \nonumber\\
premeditate_and & 1.00000 \nonumber\\
line_they & 1.00000 \nonumber\\
premeditate & 1.00000 \nonumber\\
ProductionRule_NP->VBN,NN,RB, & 1.00000 \nonumber\\
be_premeditate & 1.00000 \nonumber\\
ProductionRule_NP->NP,SBAR,., & 1.00000 \nonumber\\
lot_to & 1.00000 \nonumber\\
ie_, & 1.00000 \nonumber\\
their_dad & 1.00000 \nonumber\\
different_enviroment & 1.00000 \nonumber\\
have_like & 1.00000 \nonumber\\
_pos_ngram_PP_PUNC_PUNC & 1.00000 \nonumber\\
for_help & 1.00000 \nonumber\\
be_lazy & 1.00000 \nonumber\\
lazy_and & 1.00000 \nonumber\\
and_there & 1.00000 \nonumber\\
first_and & 1.00000 \nonumber\\
example_for & 1.00000 \nonumber\\
not_allow & 1.00000 \nonumber\\
classify_under & 1.00000 \nonumber\\
science_? & 1.00000 \nonumber\\
be_creation & 1.00000 \nonumber\\
?_2 & 1.00000 \nonumber\\
you_disillusion & 1.00000 \nonumber\\
disillusion_ppl & 1.00000 \nonumber\\
disillusion & 1.00000 \nonumber\\
the_religion & 1.00000 \nonumber\\
ppl_think & 1.00000 \nonumber\\
this_classify & 1.00000 \nonumber\\
classify & 1.00000 \nonumber\\
?_3 & 1.00000 \nonumber\\
category & 1.00000 \nonumber\\
category_? & 1.00000 \nonumber\\
creation_not & 1.00000 \nonumber\\
not_science & 1.00000 \nonumber\\
religion_category & 1.00000 \nonumber\\
like_monkey & 1.00000 \nonumber\\
i_watch & 1.00000 \nonumber\\
raffle_establish & 1.00000 \nonumber\\
arrest & 1.00000 \nonumber\\
goldilock_" & 1.00000 \nonumber\\
amphibian & 1.00000 \nonumber\\
,_dense & 1.00000 \nonumber\\
the_burst & 1.00000 \nonumber\\
now_nearby & 1.00000 \nonumber\\
the_creation & 1.00000 \nonumber\\
burst_of & 1.00000 \nonumber\\
hotter_and & 1.00000 \nonumber\\
hotter & 1.00000 \nonumber\\
from_molecule & 1.00000 \nonumber\\
hot_, & 1.00000 \nonumber\\
goldilock & 1.00000 \nonumber\\
begin_the & 1.00000 \nonumber\\
nearby_galaxy & 1.00000 \nonumber\\
move_further & 1.00000 \nonumber\\
molecule & 1.00000 \nonumber\\
._scientist & 1.00000 \nonumber\\
form_from & 1.00000 \nonumber\\
then_amphibian & 1.00000 \nonumber\\
monkey_, & 1.00000 \nonumber\\
scientist_know & 1.00000 \nonumber\\
which_form & 1.00000 \nonumber\\
molecule_that & 1.00000 \nonumber\\
amphibian_, & 1.00000 \nonumber\\
condition_. & 1.00000 \nonumber\\
into_fish & 1.00000 \nonumber\\
be_hotter & 1.00000 \nonumber\\
and_further & 1.00000 \nonumber\\
be_move & 1.00000 \nonumber\\
perfect_candidate & 1.00000 \nonumber\\
molecule_, & 1.00000 \nonumber\\
form_into & 1.00000 \nonumber\\
to_describe & 1.00000 \nonumber\\
land_animal & 1.00000 \nonumber\\
cooler_, & 1.00000 \nonumber\\
that_begin & 1.00000 \nonumber\\
._earth & 1.00000 \nonumber\\
fish_, & 1.00000 \nonumber\\
life_because & 1.00000 \nonumber\\
bacterium_start & 1.00000 \nonumber\\
describe_the & 1.00000 \nonumber\\
then_land & 1.00000 \nonumber\\
start_out & 1.00000 \nonumber\\
dense_space & 1.00000 \nonumber\\
dense_. & 1.00000 \nonumber\\
creation_of & 1.00000 \nonumber\\
then_monkey & 1.00000 \nonumber\\
further_and & 1.00000 \nonumber\\
then_human & 1.00000 \nonumber\\
"_goldilock & 1.00000 \nonumber\\
further_away & 1.00000 \nonumber\\
universe_. & 1.00000 \nonumber\\
universe_must & 1.00000 \nonumber\\
"_condition & 1.00000 \nonumber\\
universe_start & 1.00000 \nonumber\\
of_molecule & 1.00000 \nonumber\\
bang_theory & 1.00000 \nonumber\\
galaxy_be & 1.00000 \nonumber\\
the_perfect & 1.00000 \nonumber\\
expand_and & 1.00000 \nonumber\\
galaxy & 1.00000 \nonumber\\
become_cooler & 1.00000 \nonumber\\
to_form & 1.00000 \nonumber\\
dense & 1.00000 \nonumber\\
more_dense & 1.00000 \nonumber\\
term_use & 1.00000 \nonumber\\
earth_be & 1.00000 \nonumber\\
away_and & 1.00000 \nonumber\\
be_expand & 1.00000 \nonumber\\
science_can & 1.00000 \nonumber\\
a_term & 1.00000 \nonumber\\
._bacterium & 1.00000 \nonumber\\
candidate & 1.00000 \nonumber\\
candidate_for & 1.00000 \nonumber\\
burst & 1.00000 \nonumber\\
him_the & 1.00000 \nonumber\\
that_firefox & 1.00000 \nonumber\\
happen_to & 1.00000 \nonumber\\
apply_to & 1.00000 \nonumber\\
because_then & 1.00000 \nonumber\\
good_example & 1.00000 \nonumber\\
to_ever & 1.00000 \nonumber\\
guilty & 1.00000 \nonumber\\
much_brainwash & 1.00000 \nonumber\\
brainwash_as & 1.00000 \nonumber\\
ProductionRule_ADVP->RB,ADVP, & 1.00000 \nonumber\\
be_except & 1.00000 \nonumber\\
except_you & 1.00000 \nonumber\\
make_an & 1.00000 \nonumber\\
down_and & 1.00000 \nonumber\\
religion_they & 1.00000 \nonumber\\
they_come & 1.00000 \nonumber\\
else_accept & 1.00000 \nonumber\\
what_religion & 1.00000 \nonumber\\
accept_each & 1.00000 \nonumber\\
because_this & 1.00000 \nonumber\\
physical_fitness & 1.00000 \nonumber\\
fitness & 1.00000 \nonumber\\
ProductionRule_ADJP->JJ,,,JJ,,,JJ,CC,JJ, & 1.00000 \nonumber\\
dissappoint & 1.00000 \nonumber\\
orderly & 1.00000 \nonumber\\
toward_it & 1.00000 \nonumber\\
modern_and & 1.00000 \nonumber\\
elegant_, & 1.00000 \nonumber\\
feel_dissappoint & 1.00000 \nonumber\\
singapore_poorly & 1.00000 \nonumber\\
dissappoint_. & 1.00000 \nonumber\\
he_work & 1.00000 \nonumber\\
,_rational & 1.00000 \nonumber\\
and_modern & 1.00000 \nonumber\\
rational_and & 1.00000 \nonumber\\
a_vision & 1.00000 \nonumber\\
vision_for & 1.00000 \nonumber\\
singapore_that & 1.00000 \nonumber\\
orderly_, & 1.00000 \nonumber\\
work_toward & 1.00000 \nonumber\\
cause_raffle & 1.00000 \nonumber\\
an_orderly & 1.00000 \nonumber\\
_pos_ngram_CONJ_PP_NP & 1.00000 \nonumber\\
poorly_cause & 1.00000 \nonumber\\
elegant & 1.00000 \nonumber\\
,_elegant & 1.00000 \nonumber\\
overal_for & 1.00000 \nonumber\\
they_require & 1.00000 \nonumber\\
better_overal & 1.00000 \nonumber\\
be_benifit & 1.00000 \nonumber\\
to_tv & 1.00000 \nonumber\\
ProductionRule_VP->VBP,NP,PP,,,NP, & 1.00000 \nonumber\\
learn_as & 1.00000 \nonumber\\
overal & 1.00000 \nonumber\\
focus_. & 1.00000 \nonumber\\
require_more & 1.00000 \nonumber\\
benifit_to & 1.00000 \nonumber\\
person_i & 1.00000 \nonumber\\
ProductionRule_NP->JJ,JJ,JJ,NNS, & 1.00000 \nonumber\\
ProductionRule_ADJP->NN,PP, & 1.00000 \nonumber\\
side_be & 1.00000 \nonumber\\
_pos_ngram_PUNC_NN_O & 1.00000 \nonumber\\
not_our & 1.00000 \nonumber\\
._plastic & 1.00000 \nonumber\\
benifit & 1.00000 \nonumber\\
adapt & 1.00000 \nonumber\\
phy_. & 1.00000 \nonumber\\
._ed & 1.00000 \nonumber\\
yourself_as & 1.00000 \nonumber\\
filter_tap & 1.00000 \nonumber\\
filter & 1.00000 \nonumber\\
because_, & 1.00000 \nonumber\\
the_universe & 1.00000 \nonumber\\
so_that & 1.00000 \nonumber\\
anymore_. & 1.00000 \nonumber\\
valuable_away & 1.00000 \nonumber\\
learn_by & 1.00000 \nonumber\\
_pos_ngram_PR_PUNC_PUNC & 1.00000 \nonumber\\
alway_take & 1.00000 \nonumber\\
take_something & 1.00000 \nonumber\\
n't_learn & 1.00000 \nonumber\\
why_waste & 1.00000 \nonumber\\
something_valuable & 1.00000 \nonumber\\
by_spank & 1.00000 \nonumber\\
valuable & 1.00000 \nonumber\\
ProductionRule_PP->IN,NP,., & 1.00000 \nonumber\\
ProductionRule_S->ADVP,,,SBAR,NP,VP,., & 1.00000 \nonumber\\
we_wo & 1.00000 \nonumber\\
have_just & 1.00000 \nonumber\\
would_hate & 1.00000 \nonumber\\
same_clothe & 1.00000 \nonumber\\
for_ie & 1.00000 \nonumber\\
thing_which & 1.00000 \nonumber\\
prize & 1.00000 \nonumber\\
a_nobel & 1.00000 \nonumber\\
who_come & 1.00000 \nonumber\\
rule_" & 1.00000 \nonumber\\
nobel_prize & 1.00000 \nonumber\\
"_rule & 1.00000 \nonumber\\
prize_while & 1.00000 \nonumber\\
ProductionRule_ADVP->RB,IN, & 1.00000 \nonumber\\
succeed_. & 1.00000 \nonumber\\
,_down & 1.00000 \nonumber\\
actually_let & 1.00000 \nonumber\\
good_mind & 1.00000 \nonumber\\
nobody_actually & 1.00000 \nonumber\\
why_! & 1.00000 \nonumber\\
with_good & 1.00000 \nonumber\\
country_get & 1.00000 \nonumber\\
some_foreign & 1.00000 \nonumber\\
just_stick & 1.00000 \nonumber\\
anyone_succeed & 1.00000 \nonumber\\
push_the & 1.00000 \nonumber\\
nobel & 1.00000 \nonumber\\
good_indian & 1.00000 \nonumber\\
ProductionRule_VP->``,VB,'',NP, & 1.00000 \nonumber\\
?_good & 1.00000 \nonumber\\
mind_be & 1.00000 \nonumber\\
centipede_and & 1.00000 \nonumber\\
pest_like & 1.00000 \nonumber\\
he_solve & 1.00000 \nonumber\\
pest_hurt & 1.00000 \nonumber\\
pest_. & 1.00000 \nonumber\\
reward_be & 1.00000 \nonumber\\
tiger & 1.00000 \nonumber\\
kill_these & 1.00000 \nonumber\\
solve_it & 1.00000 \nonumber\\
threat_to & 1.00000 \nonumber\\
island_. & 1.00000 \nonumber\\
like_centipede & 1.00000 \nonumber\\
threat & 1.00000 \nonumber\\
be_pest & 1.00000 \nonumber\\
food_supplies & 1.00000 \nonumber\\
the_food & 1.00000 \nonumber\\
hurt_some & 1.00000 \nonumber\\
._tiger & 1.00000 \nonumber\\
give_reward & 1.00000 \nonumber\\
tiger_be & 1.00000 \nonumber\\
these_pest & 1.00000 \nonumber\\
also_destroy & 1.00000 \nonumber\\
rat_also & 1.00000 \nonumber\\
supplies_. & 1.00000 \nonumber\\
a_threat & 1.00000 \nonumber\\
and_rat & 1.00000 \nonumber\\
rat_all & 1.00000 \nonumber\\
....._yes & 1.00000 \nonumber\\
different_way & 1.00000 \nonumber\\
together_to & 1.00000 \nonumber\\
yes_and & 1.00000 \nonumber\\
sustain & 1.00000 \nonumber\\
and_leave & 1.00000 \nonumber\\
this_do & 1.00000 \nonumber\\
it_even & 1.00000 \nonumber\\
take_much & 1.00000 \nonumber\\
n't_actually & 1.00000 \nonumber\\
know_this & 1.00000 \nonumber\\
a_way & 1.00000 \nonumber\\
wiser & 1.00000 \nonumber\\
logic & 1.00000 \nonumber\\
to_earn & 1.00000 \nonumber\\
he_exist & 1.00000 \nonumber\\
well_in & 1.00000 \nonumber\\
cooler & 1.00000 \nonumber\\
but_why & 1.00000 \nonumber\\
goal_before & 1.00000 \nonumber\\
both_, & 1.00000 \nonumber\\
color & 1.00000 \nonumber\\
in_book & 1.00000 \nonumber\\
kill_the & 1.00000 \nonumber\\
accept & 1.00000 \nonumber\\
them_accomplish & 1.00000 \nonumber\\
i_" & 1.00000 \nonumber\\
set_and & 1.00000 \nonumber\\
goal_set & 1.00000 \nonumber\\
_pos_ngram_O_PR_PR & 1.00000 \nonumber\\
help_first & 1.00000 \nonumber\\
do_enjoy & 1.00000 \nonumber\\
accomplish_before & 1.00000 \nonumber\\
the_moment & 1.00000 \nonumber\\
must_help & 1.00000 \nonumber\\
christianity_( & 1.00000 \nonumber\\
even_that & 1.00000 \nonumber\\
in_almost & 1.00000 \nonumber\\
precede_christianity & 1.00000 \nonumber\\
touch_by & 1.00000 \nonumber\\
argue_to & 1.00000 \nonumber\\
of_christian & 1.00000 \nonumber\\
prove_. & 1.00000 \nonumber\\
that_precede & 1.00000 \nonumber\\
precede & 1.00000 \nonumber\\
every_society & 1.00000 \nonumber\\
never_touch & 1.00000 \nonumber\\
christian_marriage & 1.00000 \nonumber\\
society_that & 1.00000 \nonumber\\
judaism_) & 1.00000 \nonumber\\
,_include & 1.00000 \nonumber\\
bible_can & 1.00000 \nonumber\\
and_judaism & 1.00000 \nonumber\\
by_christianity & 1.00000 \nonumber\\
include_those & 1.00000 \nonumber\\
or_judaism & 1.00000 \nonumber\\
how_i & 1.00000 \nonumber\\
prevent & 1.00000 \nonumber\\
ProductionRule_VP->VB,NP,ADJP, & 1.00000 \nonumber\\
ProductionRule_S->ADVP,,,PP,NP,VP,., & 1.00000 \nonumber\\
farquhar_do & 1.00000 \nonumber\\
come_true & 1.00000 \nonumber\\
even_weaker & 1.00000 \nonumber\\
human_or & 1.00000 \nonumber\\
humanity_about & 1.00000 \nonumber\\
everything_it & 1.00000 \nonumber\\
or_hallucination & 1.00000 \nonumber\\
replace_it & 1.00000 \nonumber\\
single_prophecy & 1.00000 \nonumber\\
to_humanity & 1.00000 \nonumber\\
have_lie & 1.00000 \nonumber\\
prophecy_in & 1.00000 \nonumber\\
prophecy & 1.00000 \nonumber\\
about_literally & 1.00000 \nonumber\\
and_certainly & 1.00000 \nonumber\\
weaker_be & 1.00000 \nonumber\\
with_one & 1.00000 \nonumber\\
give_deity & 1.00000 \nonumber\\
wiser_. & 1.00000 \nonumber\\
ProductionRule_NP->DT,VBN,NN, & 1.00000 \nonumber\\
can_replace & 1.00000 \nonumber\\
literally_everything & 1.00000 \nonumber\\
unreasonable_be & 1.00000 \nonumber\\
unreasonable & 1.00000 \nonumber\\
deity_unreasonable & 1.00000 \nonumber\\
the_wiser & 1.00000 \nonumber\\
any_give & 1.00000 \nonumber\\
no_a & 1.00000 \nonumber\\
lie_of & 1.00000 \nonumber\\
of_lie & 1.00000 \nonumber\\
hallucination & 1.00000 \nonumber\\
none_that & 1.00000 \nonumber\\
greatest_reason & 1.00000 \nonumber\\
also_replace & 1.00000 \nonumber\\
it_with & 1.00000 \nonumber\\
hallucination_. & 1.00000 \nonumber\\
certainly_none & 1.00000 \nonumber\\
,_yet & 1.00000 \nonumber\\
god_" & 1.00000 \nonumber\\
to_just & 1.00000 \nonumber\\
singapore_into & 1.00000 \nonumber\\
about_our & 1.00000 \nonumber\\
up_hurt & 1.00000 \nonumber\\
woulld_end & 1.00000 \nonumber\\
world_if & 1.00000 \nonumber\\
to_pursue & 1.00000 \nonumber\\
woulld & 1.00000 \nonumber\\
that_woulld & 1.00000 \nonumber\\
that_good & 1.00000 \nonumber\\
hurt_someone & 1.00000 \nonumber\\
like_hurt & 1.00000 \nonumber\\
be_before & 1.00000 \nonumber\\
about_everyone & 1.00000 \nonumber\\
pursue_my & 1.00000 \nonumber\\
better_world & 1.00000 \nonumber\\
else_well & 1.00000 \nonumber\\
selfish_choice & 1.00000 \nonumber\\
ProductionRule_NP->PDT,NP, & 1.00000 \nonumber\\
hurt_people & 1.00000 \nonumber\\
_pos_ngram_PR_NP_NP & 1.00000 \nonumber\\
singapore.he_contribute & 1.00000 \nonumber\\
a_' & 1.00000 \nonumber\\
contribute_more & 1.00000 \nonumber\\
role_of & 1.00000 \nonumber\\
that_play & 1.00000 \nonumber\\
raffle_support & 1.00000 \nonumber\\
the_role & 1.00000 \nonumber\\
to_singapore.he & 1.00000 \nonumber\\
tax & 1.00000 \nonumber\\
many_liberal & 1.00000 \nonumber\\
theologian & 1.00000 \nonumber\\
theologian_and & 1.00000 \nonumber\\
halfway & 1.00000 \nonumber\\
halfway_point & 1.00000 \nonumber\\
even_agnostic & 1.00000 \nonumber\\
idea_) & 1.00000 \nonumber\\
ProductionRule_ADJP->ADVP,NN, & 1.00000 \nonumber\\
ProductionRule_NP->DT,JJ,JJ,JJ,NNS, & 1.00000 \nonumber\\
most_you & 1.00000 \nonumber\\
that_idea & 1.00000 \nonumber\\
can_co-exist & 1.00000 \nonumber\\
speak_in & 1.00000 \nonumber\\
may_easily & 1.00000 \nonumber\\
faith/science_where & 1.00000 \nonumber\\
ProductionRule_NP->CD,CD,NN, & 1.00000 \nonumber\\
ProductionRule_S->PP,NP,PP,VP, & 1.00000 \nonumber\\
_pos_ngram_PR_CARD_CARD & 1.00000 \nonumber\\
lose_me & 1.00000 \nonumber\\
faith/science & 1.00000 \nonumber\\
great_many & 1.00000 \nonumber\\
real_problem & 1.00000 \nonumber\\
between_faith/science & 1.00000 \nonumber\\
creationism_--- & 1.00000 \nonumber\\
(_no & 1.00000 \nonumber\\
co-exist & 1.00000 \nonumber\\
be_halfway & 1.00000 \nonumber\\
creationism_can & 1.00000 \nonumber\\
answer_( & 1.00000 \nonumber\\
me_--- & 1.00000 \nonumber\\
ProductionRule_VP->VB,PRN, & 1.00000 \nonumber\\
one_) & 1.00000 \nonumber\\
and_creationism & 1.00000 \nonumber\\
to_counter & 1.00000 \nonumber\\
---_99 & 1.00000 \nonumber\\
scientist_would & 1.00000 \nonumber\\
ProductionRule_VP->VBP,PRT,NP, & 1.00000 \nonumber\\
where_evolution & 1.00000 \nonumber\\
science_do & 1.00000 \nonumber\\
---_at & 1.00000 \nonumber\\
there_may & 1.00000 \nonumber\\
ProductionRule_NP->RB,NNS, & 1.00000 \nonumber\\
no_scientist & 1.00000 \nonumber\\
agnostic_would & 1.00000 \nonumber\\
you_lose & 1.00000 \nonumber\\
say_speak & 1.00000 \nonumber\\
liberal_theologian & 1.00000 \nonumber\\
against_creationism & 1.00000 \nonumber\\
point_between & 1.00000 \nonumber\\
--- & 1.00000 \nonumber\\
that_science & 1.00000 \nonumber\\
counter_you & 1.00000 \nonumber\\
_pos_ngram_CARD_O_CONJ & 1.00000 \nonumber\\
co-exist_( & 1.00000 \nonumber\\
at_most & 1.00000 \nonumber\\
logical_at & 1.00000 \nonumber\\
world_we & 1.00000 \nonumber\\
there_way & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,ADVP,RB,ADJP,ADVP, & 1.00000 \nonumber\\
end_and & 1.00000 \nonumber\\
not_logical & 1.00000 \nonumber\\
sense_no & 1.00000 \nonumber\\
together_and & 1.00000 \nonumber\\
should_end & 1.00000 \nonumber\\
one_country & 1.00000 \nonumber\\
should_lead & 1.00000 \nonumber\\
even_make & 1.00000 \nonumber\\
country_should & 1.00000 \nonumber\\
have_there & 1.00000 \nonumber\\
start_together & 1.00000 \nonumber\\
have_notice & 1.00000 \nonumber\\
usually_my & 1.00000 \nonumber\\
"_better & 1.00000 \nonumber\\
end_be & 1.00000 \nonumber\\
happy_predicament & 1.00000 \nonumber\\
endeavor_have & 1.00000 \nonumber\\
"_us & 1.00000 \nonumber\\
my_decision & 1.00000 \nonumber\\
yourself_will & 1.00000 \nonumber\\
be_advance & 1.00000 \nonumber\\
help_? & 1.00000 \nonumber\\
or_go & 1.00000 \nonumber\\
some_not & 1.00000 \nonumber\\
ProductionRule_ADVP->RB,CC,RB, & 1.00000 \nonumber\\
into_some & 1.00000 \nonumber\\
really_help & 1.00000 \nonumber\\
all_want & 1.00000 \nonumber\\
notice_personal & 1.00000 \nonumber\\
decision_in & 1.00000 \nonumber\\
wherea_, & 1.00000 \nonumber\\
so_happy & 1.00000 \nonumber\\
run_who & 1.00000 \nonumber\\
us_" & 1.00000 \nonumber\\
better_place & 1.00000 \nonumber\\
be_yes & 1.00000 \nonumber\\
predicament_. & 1.00000 \nonumber\\
place_" & 1.00000 \nonumber\\
will_it & 1.00000 \nonumber\\
predicament & 1.00000 \nonumber\\
?_wherea & 1.00000 \nonumber\\
ProductionRule_SINV->VP,NP, & 1.00000 \nonumber\\
_pos_ngram_PR_CONJ_ADJ & 1.00000 \nonumber\\
better_suit & 1.00000 \nonumber\\
personal_endeavor & 1.00000 \nonumber\\
get_" & 1.00000 \nonumber\\
an_advancement & 1.00000 \nonumber\\
suit_yourself & 1.00000 \nonumber\\
refute & 1.00000 \nonumber\\
of_there & 1.00000 \nonumber\\
world_country & 1.00000 \nonumber\\
absolute_or & 1.00000 \nonumber\\
womb_? & 1.00000 \nonumber\\
premature & 1.00000 \nonumber\\
,_let & 1.00000 \nonumber\\
upon_position & 1.00000 \nonumber\\
premature_baby & 1.00000 \nonumber\\
absolute & 1.00000 \nonumber\\
personhood & 1.00000 \nonumber\\
be_inside & 1.00000 \nonumber\\
personhood_absolute & 1.00000 \nonumber\\
be_personhood & 1.00000 \nonumber\\
situation_change & 1.00000 \nonumber\\
so_drastically & 1.00000 \nonumber\\
a_premature & 1.00000 \nonumber\\
predicate & 1.00000 \nonumber\\
gallon_pail & 1.00000 \nonumber\\
inside_the & 1.00000 \nonumber\\
say_for & 1.00000 \nonumber\\
position_? & 1.00000 \nonumber\\
sake_of & 1.00000 \nonumber\\
sake & 1.00000 \nonumber\\
an_incubator & 1.00000 \nonumber\\
incubator_or & 1.00000 \nonumber\\
predicate_upon & 1.00000 \nonumber\\
incubator & 1.00000 \nonumber\\
drastically_just & 1.00000 \nonumber\\
lie_in & 1.00000 \nonumber\\
change_so & 1.00000 \nonumber\\
a_5 & 1.00000 \nonumber\\
it_predicate & 1.00000 \nonumber\\
'_say & 1.00000 \nonumber\\
ProductionRule_SQ->VBZ,NP,NP,., & 1.00000 \nonumber\\
pail & 1.00000 \nonumber\\
the_sake & 1.00000 \nonumber\\
pail_, & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,NP,VP, & 1.00000 \nonumber\\
5_gallon & 1.00000 \nonumber\\
kill_it & 1.00000 \nonumber\\
machine & 1.00000 \nonumber\\
smoother & 1.00000 \nonumber\\
everyone_would & 1.00000 \nonumber\\
god-give_talent & 1.00000 \nonumber\\
of_humanity & 1.00000 \nonumber\\
just_that & 1.00000 \nonumber\\
appeal & 1.00000 \nonumber\\
also_combine & 1.00000 \nonumber\\
job_that & 1.00000 \nonumber\\
improve_society & 1.00000 \nonumber\\
talent & 1.00000 \nonumber\\
smoother_. & 1.00000 \nonumber\\
two_if & 1.00000 \nonumber\\
doesnt_sound & 1.00000 \nonumber\\
would_run & 1.00000 \nonumber\\
a_god-give & 1.00000 \nonumber\\
of_job & 1.00000 \nonumber\\
everyone_put & 1.00000 \nonumber\\
combine_the & 1.00000 \nonumber\\
good_doesnt & 1.00000 \nonumber\\
appeal_to & 1.00000 \nonumber\\
sound_appeal & 1.00000 \nonumber\\
effort_into & 1.00000 \nonumber\\
nor_will & 1.00000 \nonumber\\
world_nor & 1.00000 \nonumber\\
lot_smoother & 1.00000 \nonumber\\
ProductionRule_NP->PRP$,NNS,CC,NNS, & 1.00000 \nonumber\\
talent_and & 1.00000 \nonumber\\
humanity_, & 1.00000 \nonumber\\
ability_for & 1.00000 \nonumber\\
talent_that & 1.00000 \nonumber\\
their_talent & 1.00000 \nonumber\\
god-give & 1.00000 \nonumber\\
into_improve & 1.00000 \nonumber\\
will_we & 1.00000 \nonumber\\
we_ever & 1.00000 \nonumber\\
if_advance & 1.00000 \nonumber\\
would_use & 1.00000 \nonumber\\
little_effort & 1.00000 \nonumber\\
n't_matter & 1.00000 \nonumber\\
them_do & 1.00000 \nonumber\\
important_than & 1.00000 \nonumber\\
like_any & 1.00000 \nonumber\\
,_sometime & 1.00000 \nonumber\\
though_there & 1.00000 \nonumber\\
work_so & 1.00000 \nonumber\\
other_different & 1.00000 \nonumber\\
ProductionRule_VP->VP,,,S, & 1.00000 \nonumber\\
ProductionRule_SBAR->IN,SBAR, & 1.00000 \nonumber\\
'_bid & 1.00000 \nonumber\\
it_wo & 1.00000 \nonumber\\
because_even & 1.00000 \nonumber\\
ProductionRule_S->ADVP,PRN,ADVP,NP,VP,., & 1.00000 \nonumber\\
discipline_kid & 1.00000 \nonumber\\
them_learn & 1.00000 \nonumber\\
learn_they & 1.00000 \nonumber\\
little_spank & 1.00000 \nonumber\\
ProductionRule_PRN->,,SBAR,,, & 1.00000 \nonumber\\
good_because & 1.00000 \nonumber\\
win_. & 1.00000 \nonumber\\
*_. & 1.00000 \nonumber\\
porn_* & 1.00000 \nonumber\\
'n' & 1.00000 \nonumber\\
they_focus & 1.00000 \nonumber\\
count_? & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,PRT,PP, & 1.00000 \nonumber\\
*_actor & 1.00000 \nonumber\\
*_t. & 1.00000 \nonumber\\
note_that & 1.00000 \nonumber\\
spiel & 1.00000 \nonumber\\
be_ebil & 1.00000 \nonumber\\
exclusively & 1.00000 \nonumber\\
actor_* & 1.00000 \nonumber\\
whenever_someone & 1.00000 \nonumber\\
ProductionRule_NP->DT,``,S,'',NN, & 1.00000 \nonumber\\
as_if & 1.00000 \nonumber\\
on_woman & 1.00000 \nonumber\\
(_what & 1.00000 \nonumber\\
arguement_otherwise & 1.00000 \nonumber\\
n't_count & 1.00000 \nonumber\\
in_on & 1.00000 \nonumber\\
exclusively_on & 1.00000 \nonumber\\
feminist & 1.00000 \nonumber\\
as_porn & 1.00000 \nonumber\\
degrade_" & 1.00000 \nonumber\\
)_porn & 1.00000 \nonumber\\
start_in & 1.00000 \nonumber\\
bullsh_* & 1.00000 \nonumber\\
"_bullsh & 1.00000 \nonumber\\
bullsh & 1.00000 \nonumber\\
that_whenever & 1.00000 \nonumber\\
less_. & 1.00000 \nonumber\\
_pos_ngram_ADV_O_NP & 1.00000 \nonumber\\
no_less & 1.00000 \nonumber\\
focus_exclusively & 1.00000 \nonumber\\
feminist_" & 1.00000 \nonumber\\
otherwise_be & 1.00000 \nonumber\\
just_" & 1.00000 \nonumber\\
ebil & 1.00000 \nonumber\\
any_arguement & 1.00000 \nonumber\\
i_note & 1.00000 \nonumber\\
ebil_'n' & 1.00000 \nonumber\\
man_do & 1.00000 \nonumber\\
someone_start & 1.00000 \nonumber\\
spiel_, & 1.00000 \nonumber\\
"_spiel & 1.00000 \nonumber\\
'n'_degrade & 1.00000 \nonumber\\
"_feminist & 1.00000 \nonumber\\
with_firefox & 1.00000 \nonumber\\
hard_for & 1.00000 \nonumber\\
that_every & 1.00000 \nonumber\\
space & 1.00000 \nonumber\\
space_. & 1.00000 \nonumber\\
so_when & 1.00000 \nonumber\\
to_speak & 1.00000 \nonumber\\
church_. & 1.00000 \nonumber\\
that_one & 1.00000 \nonumber\\
fill_with & 1.00000 \nonumber\\
be_illegal & 1.00000 \nonumber\\
in_europe & 1.00000 \nonumber\\
again_the & 1.00000 \nonumber\\
china_who & 1.00000 \nonumber\\
of_chaos & 1.00000 \nonumber\\
order_out & 1.00000 \nonumber\\
alway_make & 1.00000 \nonumber\\
way_indium & 1.00000 \nonumber\\
be_china & 1.00000 \nonumber\\
indium_run & 1.00000 \nonumber\\
make_order & 1.00000 \nonumber\\
potential_? & 1.00000 \nonumber\\
only_competition & 1.00000 \nonumber\\
ProductionRule_SQ->VBP,NP,VP,., & 1.00000 \nonumber\\
better_job & 1.00000 \nonumber\\
competition_we & 1.00000 \nonumber\\
school_with & 1.00000 \nonumber\\
really_easy & 1.00000 \nonumber\\
all_they & 1.00000 \nonumber\\
easy_. & 1.00000 \nonumber\\
pe_teacher & 1.00000 \nonumber\\
teacher_job & 1.00000 \nonumber\\
be_yell & 1.00000 \nonumber\\
ProductionRule_NP->DT,NNP,NNS,NN, & 1.00000 \nonumber\\
job_must & 1.00000 \nonumber\\
yell_at & 1.00000 \nonumber\\
different_? & 1.00000 \nonumber\\
hot & 1.00000 \nonumber\\
4_year & 1.00000 \nonumber\\
on_his & 1.00000 \nonumber\\
can_even & 1.00000 \nonumber\\
_pos_ngram_ADV_PP_PUNC & 1.00000 \nonumber\\
much_. & 1.00000 \nonumber\\
platform & 1.00000 \nonumber\\
and_, & 1.00000 \nonumber\\
it_the & 1.00000 \nonumber\\
_pos_ngram_PP_ADJ_O & 1.00000 \nonumber\\
kid_lose & 1.00000 \nonumber\\
feel_comfortable & 1.00000 \nonumber\\
lose_their & 1.00000 \nonumber\\
individuality_and & 1.00000 \nonumber\\
no_sense & 1.00000 \nonumber\\
'd_rather & 1.00000 \nonumber\\
ProductionRule_VP->ADVP,VB,PP, & 1.00000 \nonumber\\
western_education & 1.00000 \nonumber\\
a_language & 1.00000 \nonumber\\
education_and & 1.00000 \nonumber\\
nothing_compare & 1.00000 \nonumber\\
indium_' & 1.00000 \nonumber\\
world_ca & 1.00000 \nonumber\\
doubt_indium & 1.00000 \nonumber\\
..._where & 1.00000 \nonumber\\
to_western & 1.00000 \nonumber\\
understand_? & 1.00000 \nonumber\\
understand_and & 1.00000 \nonumber\\
indium_... & 1.00000 \nonumber\\
leave_that & 1.00000 \nonumber\\
i_highly & 1.00000 \nonumber\\
education_quality & 1.00000 \nonumber\\
will_ever & 1.00000 \nonumber\\
highly_doubt & 1.00000 \nonumber\\
opress & 1.00000 \nonumber\\
ProductionRule_S->NP,:,NP,., & 1.00000 \nonumber\\
'_education & 1.00000 \nonumber\\
superpower_that & 1.00000 \nonumber\\
whole_class & 1.00000 \nonumber\\
superpower_. & 1.00000 \nonumber\\
that_control & 1.00000 \nonumber\\
wealth_difference & 1.00000 \nonumber\\
should_leave & 1.00000 \nonumber\\
quality_have & 1.00000 \nonumber\\
of_opress & 1.00000 \nonumber\\
the_superpower & 1.00000 \nonumber\\
opress_people & 1.00000 \nonumber\\
ProductionRule_NP->SBAR,CC,NP, & 1.00000 \nonumber\\
control_the & 1.00000 \nonumber\\
huge_wealth & 1.00000 \nonumber\\
language_that & 1.00000 \nonumber\\
child_be & 1.00000 \nonumber\\
party_, & 1.00000 \nonumber\\
party & 1.00000 \nonumber\\
_pos_ngram_CARD_CONJ_CARD & 1.00000 \nonumber\\
memory & 1.00000 \nonumber\\
thing_in & 1.00000 \nonumber\\
away_in & 1.00000 \nonumber\\
hope_nobody & 1.00000 \nonumber\\
we_pro-choicer & 1.00000 \nonumber\\
seam & 1.00000 \nonumber\\
seam_to & 1.00000 \nonumber\\
face_it & 1.00000 \nonumber\\
a_sad & 1.00000 \nonumber\\
some_man & 1.00000 \nonumber\\
awful_thing & 1.00000 \nonumber\\
d.c. & 1.00000 \nonumber\\
d.c._that & 1.00000 \nonumber\\
something_a & 1.00000 \nonumber\\
would_take & 1.00000 \nonumber\\
woman_would & 1.00000 \nonumber\\
the_obama & 1.00000 \nonumber\\
not_some & 1.00000 \nonumber\\
difficult_and & 1.00000 \nonumber\\
decision_should & 1.00000 \nonumber\\
pro-choicer_hope & 1.00000 \nonumber\\
we_also & 1.00000 \nonumber\\
mile_away & 1.00000 \nonumber\\
in_d.c. & 1.00000 \nonumber\\
never_something & 1.00000 \nonumber\\
even_pray & 1.00000 \nonumber\\
life_alter & 1.00000 \nonumber\\
n't_seam & 1.00000 \nonumber\\
pray_involve & 1.00000 \nonumber\\
and_awful & 1.00000 \nonumber\\
make_this & 1.00000 \nonumber\\
obama_approach & 1.00000 \nonumber\\
this_abortion & 1.00000 \nonumber\\
lightly_there & 1.00000 \nonumber\\
pro-choicer & 1.00000 \nonumber\\
with_make & 1.00000 \nonumber\\
alter_situation & 1.00000 \nonumber\\
think_ask & 1.00000 \nonumber\\
ask_for & 1.00000 \nonumber\\
man_mile & 1.00000 \nonumber\\
and_life & 1.00000 \nonumber\\
never_face & 1.00000 \nonumber\\
ever_have & 1.00000 \nonumber\\
pro-life_people & 1.00000 \nonumber\\
approach_to & 1.00000 \nonumber\\
take_lightly & 1.00000 \nonumber\\
sad_and & 1.00000 \nonumber\\
this_decision & 1.00000 \nonumber\\
this_difficult & 1.00000 \nonumber\\
ProductionRule_VP->VB,ADVP,ADVP, & 1.00000 \nonumber\\
think_in & 1.00000 \nonumber\\
beacuse & 1.00000 \nonumber\\
centry & 1.00000 \nonumber\\
the_21st & 1.00000 \nonumber\\
centry_! & 1.00000 \nonumber\\
21st_centry & 1.00000 \nonumber\\
would_u & 1.00000 \nonumber\\
be_deny & 1.00000 \nonumber\\
beacuse_there & 1.00000 \nonumber\\
gay_do & 1.00000 \nonumber\\
marry_so & 1.00000 \nonumber\\
they_! & 1.00000 \nonumber\\
just_beacuse & 1.00000 \nonumber\\
!_everyone & 1.00000 \nonumber\\
happy_! & 1.00000 \nonumber\\
u_feel & 1.00000 \nonumber\\
there_gay & 1.00000 \nonumber\\
!_how & 1.00000 \nonumber\\
else_be & 1.00000 \nonumber\\
ProductionRule_S->S,NP,VP,., & 1.00000 \nonumber\\
deny_! & 1.00000 \nonumber\\
ProductionRule_ADVP->DT,NN,SBAR, & 1.00000 \nonumber\\
call_him & 1.00000 \nonumber\\
an_economic & 1.00000 \nonumber\\
_pos_ngram_CARD_V_O & 1.00000 \nonumber\\
a_case & 1.00000 \nonumber\\
as_complex & 1.00000 \nonumber\\
,_personal & 1.00000 \nonumber\\
who_create & 1.00000 \nonumber\\
reasonable_before & 1.00000 \nonumber\\
so_complex & 1.00000 \nonumber\\
be_reasonable & 1.00000 \nonumber\\
all-know & 1.00000 \nonumber\\
merciful & 1.00000 \nonumber\\
that_belief & 1.00000 \nonumber\\
all-know_all-powerful & 1.00000 \nonumber\\
argument_seem & 1.00000 \nonumber\\
the_creator & 1.00000 \nonumber\\
complex_life & 1.00000 \nonumber\\
explain_by & 1.00000 \nonumber\\
all-powerful_love & 1.00000 \nonumber\\
imagine_, & 1.00000 \nonumber\\
,_merciful & 1.00000 \nonumber\\
merciful_, & 1.00000 \nonumber\\
to_apply & 1.00000 \nonumber\\
complex_creator & 1.00000 \nonumber\\
personal_god & 1.00000 \nonumber\\
a_complex & 1.00000 \nonumber\\
apply_here & 1.00000 \nonumber\\
life_can & 1.00000 \nonumber\\
creator_" & 1.00000 \nonumber\\
creature_as & 1.00000 \nonumber\\
an_all-know & 1.00000 \nonumber\\
complex_a & 1.00000 \nonumber\\
a_creature & 1.00000 \nonumber\\
front & 1.00000 \nonumber\\
from_school & 1.00000 \nonumber\\
candy & 1.00000 \nonumber\\
ProductionRule_NP->NP,'',PP, & 1.00000 \nonumber\\
advancement_for & 1.00000 \nonumber\\
advance_for & 1.00000 \nonumber\\
and_while & 1.00000 \nonumber\\
to_begin & 1.00000 \nonumber\\
pro-choice & 1.00000 \nonumber\\
battle & 1.00000 \nonumber\\
to_add & 1.00000 \nonumber\\
student_equal & 1.00000 \nonumber\\
policy_be & 1.00000 \nonumber\\
level_this & 1.00000 \nonumber\\
a_policy & 1.00000 \nonumber\\
that_such & 1.00000 \nonumber\\
envy_and & 1.00000 \nonumber\\
jealousy & 1.00000 \nonumber\\
equal_on & 1.00000 \nonumber\\
economic_level & 1.00000 \nonumber\\
jealousy_. & 1.00000 \nonumber\\
and_jealousy & 1.00000 \nonumber\\
prevent_envy & 1.00000 \nonumber\\
be_prevent & 1.00000 \nonumber\\
let_anyone & 1.00000 \nonumber\\
speed & 1.00000 \nonumber\\
do_much & 1.00000 \nonumber\\
human_being & 1.00000 \nonumber\\
being & 1.00000 \nonumber\\
_pos_ngram_PR_O_V & 1.00000 \nonumber\\
_pos_ngram_ART_ART_V & 1.00000 \nonumber\\
truly_love & 1.00000 \nonumber\\
fir & 1.00000 \nonumber\\
wrongly_as & 1.00000 \nonumber\\
singapore_on & 1.00000 \nonumber\\
fir_journey & 1.00000 \nonumber\\
be_later & 1.00000 \nonumber\\
his_discovery & 1.00000 \nonumber\\
29_february & 1.00000 \nonumber\\
29 & 1.00000 \nonumber\\
ProductionRule_VP->VBN,NP,ADVP,PP,NP, & 1.00000 \nonumber\\
wrongly & 1.00000 \nonumber\\
as_29 & 1.00000 \nonumber\\
write_his & 1.00000 \nonumber\\
later_correct & 1.00000 \nonumber\\
discovery_wrongly & 1.00000 \nonumber\\
discover_singapore & 1.00000 \nonumber\\
have_discover & 1.00000 \nonumber\\
his_fir & 1.00000 \nonumber\\
1819_. & 1.00000 \nonumber\\
settlement_. & 1.00000 \nonumber\\
evolution_and & 1.00000 \nonumber\\
firefox_, & 1.00000 \nonumber\\
want_a & 1.00000 \nonumber\\
patch & 1.00000 \nonumber\\
then_a & 1.00000 \nonumber\\
baby_because & 1.00000 \nonumber\\
good_of & 1.00000 \nonumber\\
mostly & 1.00000 \nonumber\\
no_real & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,RB,ADVP,VP, & 1.00000 \nonumber\\
you_strive & 1.00000 \nonumber\\
?_you & 1.00000 \nonumber\\
to_murder & 1.00000 \nonumber\\
the_america & 1.00000 \nonumber\\
field & 1.00000 \nonumber\\
ProductionRule_S->ADVP,NP, & 1.00000 \nonumber\\
ProductionRule_WHADVP->WRB,ADJP, & 1.00000 \nonumber\\
a_hot & 1.00000 \nonumber\\
want_. & 1.00000 \nonumber\\
?_yes & 1.00000 \nonumber\\
and_so & 1.00000 \nonumber\\
by_definition & 1.00000 \nonumber\\
"_test & 1.00000 \nonumber\\
-_argumentum & 1.00000 \nonumber\\
ad_populum & 1.00000 \nonumber\\
predate & 1.00000 \nonumber\\
predate_christianity & 1.00000 \nonumber\\
ad & 1.00000 \nonumber\\
_pos_ngram_PUNC_CARD_PR & 1.00000 \nonumber\\
with_- & 1.00000 \nonumber\\
also_like & 1.00000 \nonumber\\
definition_, & 1.00000 \nonumber\\
dichotomy_. & 1.00000 \nonumber\\
._---------------------------------------------------------------------------------------------------- & 1.00000 \nonumber\\
bullshit_to & 1.00000 \nonumber\\
destroy_your & 1.00000 \nonumber\\
---------------------------------------------------------------------------------------------------- & 1.00000 \nonumber\\
predate_religion & 1.00000 \nonumber\\
----------------------------------------------------------------------------------------------------_i & 1.00000 \nonumber\\
that_atheism & 1.00000 \nonumber\\
populum & 1.00000 \nonumber\\
be_bullshit & 1.00000 \nonumber\\
argumentum_ad & 1.00000 \nonumber\\
your_" & 1.00000 \nonumber\\
argumentum & 1.00000 \nonumber\\
argument_( & 1.00000 \nonumber\\
populum_) & 1.00000 \nonumber\\
atheism_predate & 1.00000 \nonumber\\
,_destroy & 1.00000 \nonumber\\
time_" & 1.00000 \nonumber\\
law_that & 1.00000 \nonumber\\
be_straight & 1.00000 \nonumber\\
the_rich & 1.00000 \nonumber\\
_pos_ngram_ART_ADJ_ADV & 1.00000 \nonumber\\
marriage_should & 1.00000 \nonumber\\
like_, & 1.00000 \nonumber\\
throw_and & 1.00000 \nonumber\\
and_polute & 1.00000 \nonumber\\
recycle_the & 1.00000 \nonumber\\
people_recycle & 1.00000 \nonumber\\
company_fault & 1.00000 \nonumber\\
polute & 1.00000 \nonumber\\
as_people & 1.00000 \nonumber\\
evironment_, & 1.00000 \nonumber\\
evironment & 1.00000 \nonumber\\
be_throw & 1.00000 \nonumber\\
the_evironment & 1.00000 \nonumber\\
polute_. & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,ADVP,NP, & 1.00000 \nonumber\\
the_shoe & 1.00000 \nonumber\\
effort_to & 1.00000 \nonumber\\
father_do & 1.00000 \nonumber\\
deeper_. & 1.00000 \nonumber\\
._during & 1.00000 \nonumber\\
deeper & 1.00000 \nonumber\\
those_vital & 1.00000 \nonumber\\
fill_the & 1.00000 \nonumber\\
the_characteristic & 1.00000 \nonumber\\
be_poisonous & 1.00000 \nonumber\\
shoe_of & 1.00000 \nonumber\\
brand_those & 1.00000 \nonumber\\
to_fill & 1.00000 \nonumber\\
externally & 1.00000 \nonumber\\
of_childhood & 1.00000 \nonumber\\
poisonous_. & 1.00000 \nonumber\\
go_much & 1.00000 \nonumber\\
scar_externally & 1.00000 \nonumber\\
poisonous & 1.00000 \nonumber\\
an_unfit & 1.00000 \nonumber\\
leaf_bump & 1.00000 \nonumber\\
,_scrape & 1.00000 \nonumber\\
scrape & 1.00000 \nonumber\\
scrape_and & 1.00000 \nonumber\\
alter_self & 1.00000 \nonumber\\
ProductionRule_NP->NNS,,,NNS,CC,NNS, & 1.00000 \nonumber\\
unfit_parent & 1.00000 \nonumber\\
easily_. & 1.00000 \nonumber\\
the_miss & 1.00000 \nonumber\\
self_confidence & 1.00000 \nonumber\\
and_scar & 1.00000 \nonumber\\
childhood_have & 1.00000 \nonumber\\
and_self & 1.00000 \nonumber\\
ProductionRule_VP->ADVP,VBZ,NP,ADVP, & 1.00000 \nonumber\\
bid_habit & 1.00000 \nonumber\\
n't_something & 1.00000 \nonumber\\
those_bid & 1.00000 \nonumber\\
self_worth & 1.00000 \nonumber\\
it_alter & 1.00000 \nonumber\\
bump_, & 1.00000 \nonumber\\
one_forget & 1.00000 \nonumber\\
vital_year & 1.00000 \nonumber\\
can_covertly & 1.00000 \nonumber\\
bump & 1.00000 \nonumber\\
habit_in & 1.00000 \nonumber\\
forget_easily & 1.00000 \nonumber\\
covertly_brand & 1.00000 \nonumber\\
miss_party & 1.00000 \nonumber\\
much_deeper & 1.00000 \nonumber\\
just_leaf & 1.00000 \nonumber\\
worth_, & 1.00000 \nonumber\\
externally_. & 1.00000 \nonumber\\
much_effort & 1.00000 \nonumber\\
will_take & 1.00000 \nonumber\\
damage_go & 1.00000 \nonumber\\
covertly & 1.00000 \nonumber\\
fortune & 1.00000 \nonumber\\
this_mutation & 1.00000 \nonumber\\
the_darkness & 1.00000 \nonumber\\
darkness_be & 1.00000 \nonumber\\
observation_- & 1.00000 \nonumber\\
select_for & 1.00000 \nonumber\\
present_at & 1.00000 \nonumber\\
who_select & 1.00000 \nonumber\\
happen_by & 1.00000 \nonumber\\
with_... & 1.00000 \nonumber\\
-_who & 1.00000 \nonumber\\
situation_, & 1.00000 \nonumber\\
-_both & 1.00000 \nonumber\\
the_observation & 1.00000 \nonumber\\
color_moth & 1.00000 \nonumber\\
_pos_ngram_O_ADV_ART & 1.00000 \nonumber\\
by_good & 1.00000 \nonumber\\
tree_to & 1.00000 \nonumber\\
select_this & 1.00000 \nonumber\\
change_during & 1.00000 \nonumber\\
ProductionRule_S->PP,,,S,:,S, & 1.00000 \nonumber\\
for_when & 1.00000 \nonumber\\
mutation_to & 1.00000 \nonumber\\
ProductionRule_S->SBAR,:,``,ADVP,NP,VP,.,'', & 1.00000 \nonumber\\
good_fortune & 1.00000 \nonumber\\
fortune_? & 1.00000 \nonumber\\
environment_change & 1.00000 \nonumber\\
be_select & 1.00000 \nonumber\\
both_color & 1.00000 \nonumber\\
be_present & 1.00000 \nonumber\\
just_happen & 1.00000 \nonumber\\
ProductionRule_VP->VP,,,CONJP,VP, & 1.00000 \nonumber\\
out_he & 1.00000 \nonumber\\
die_believe & 1.00000 \nonumber\\
rather_die & 1.00000 \nonumber\\
you_rather & 1.00000 \nonumber\\
exist_! & 1.00000 \nonumber\\
believe_and & 1.00000 \nonumber\\
to_school & 1.00000 \nonumber\\
colour & 1.00000 \nonumber\\
grow_as & 1.00000 \nonumber\\
record_, & 1.00000 \nonumber\\
individual_refuse & 1.00000 \nonumber\\
first_point & 1.00000 \nonumber\\
you_! & 1.00000 \nonumber\\
share_the & 1.00000 \nonumber\\
..._or & 1.00000 \nonumber\\
,_yeah & 1.00000 \nonumber\\
my_first & 1.00000 \nonumber\\
christian_... & 1.00000 \nonumber\\
refuse & 1.00000 \nonumber\\
refuse_to & 1.00000 \nonumber\\
._unfortunately & 1.00000 \nonumber\\
same_belief & 1.00000 \nonumber\\
anything_? & 1.00000 \nonumber\\
than_hey & 1.00000 \nonumber\\
ProductionRule_FRAG->S,:,FRAG,., & 1.00000 \nonumber\\
!_for & 1.00000 \nonumber\\
yeah_it & 1.00000 \nonumber\\
hey_who & 1.00000 \nonumber\\
hence_, & 1.00000 \nonumber\\
oppose_individual & 1.00000 \nonumber\\
ProductionRule_S->S,:,S, & 1.00000 \nonumber\\
ProductionRule_VP->ADVP,VB, & 1.00000 \nonumber\\
_pos_ngram_O_NP_PP & 1.00000 \nonumber\\
so_how & 1.00000 \nonumber\\
exist_during & 1.00000 \nonumber\\
during_biblical & 1.00000 \nonumber\\
porn_because & 1.00000 \nonumber\\
sin_? & 1.00000 \nonumber\\
mench & 1.00000 \nonumber\\
say_god & 1.00000 \nonumber\\
against_porn & 1.00000 \nonumber\\
not_mench & 1.00000 \nonumber\\
mench_porn & 1.00000 \nonumber\\
biblical_time & 1.00000 \nonumber\\
bible_do & 1.00000 \nonumber\\
a_difference & 1.00000 \nonumber\\
people_have & 1.00000 \nonumber\\
something_that & 1.00000 \nonumber\\
_pos_ngram_CONJ_PR_NP & 1.00000 \nonumber\\
other_religion & 1.00000 \nonumber\\
those_people & 1.00000 \nonumber\\
up_have & 1.00000 \nonumber\\
can_better & 1.00000 \nonumber\\
down_or & 1.00000 \nonumber\\
or_you & 1.00000 \nonumber\\
opinion_if & 1.00000 \nonumber\\
run_you & 1.00000 \nonumber\\
break_down & 1.00000 \nonumber\\
fix_them & 1.00000 \nonumber\\
ProductionRule_NP->PRP$,JJ,NN,SBAR, & 1.00000 \nonumber\\
to_fix & 1.00000 \nonumber\\
a_break & 1.00000 \nonumber\\
rich_and & 1.00000 \nonumber\\
gap_between & 1.00000 \nonumber\\
and_poor & 1.00000 \nonumber\\
_pos_ngram_CARD_ADV & 1.00000 \nonumber\\
community_and & 1.00000 \nonumber\\
recognition_for & 1.00000 \nonumber\\
a_reward & 1.00000 \nonumber\\
accomplish_in & 1.00000 \nonumber\\
surely_live & 1.00000 \nonumber\\
will_most & 1.00000 \nonumber\\
really_think & 1.00000 \nonumber\\
most_surely & 1.00000 \nonumber\\
themselve_will & 1.00000 \nonumber\\
win-win_situation & 1.00000 \nonumber\\
,_advance & 1.00000 \nonumber\\
win-win & 1.00000 \nonumber\\
a_win-win & 1.00000 \nonumber\\
the_support & 1.00000 \nonumber\\
better_life & 1.00000 \nonumber\\
get_recognition & 1.00000 \nonumber\\
ProductionRule_PP->TO,ADJP, & 1.00000 \nonumber\\
me_it & 1.00000 \nonumber\\
devote & 1.00000 \nonumber\\
a_thing & 1.00000 \nonumber\\
it_we & 1.00000 \nonumber\\
explorer_suck & 1.00000 \nonumber\\
could_spawn & 1.00000 \nonumber\\
multiple_svchost.exe & 1.00000 \nonumber\\
extreme_memory & 1.00000 \nonumber\\
those_as & 1.00000 \nonumber\\
a_blind & 1.00000 \nonumber\\
memory_when & 1.00000 \nonumber\\
when_run & 1.00000 \nonumber\\
extreme & 1.00000 \nonumber\\
multiple_tab & 1.00000 \nonumber\\
more_; & 1.00000 \nonumber\\
instance_and & 1.00000 \nonumber\\
use_those & 1.00000 \nonumber\\
spawn_multiple & 1.00000 \nonumber\\
suck_extreme & 1.00000 \nonumber\\
and_probably & 1.00000 \nonumber\\
svchost.exe & 1.00000 \nonumber\\
svchost.exe_instance & 1.00000 \nonumber\\
run_multiple & 1.00000 \nonumber\\
spawn & 1.00000 \nonumber\\
probably_more & 1.00000 \nonumber\\
say_something & 1.00000 \nonumber\\
ProductionRule_NP->PRP$,ADJP, & 1.00000 \nonumber\\
whole_hour & 1.00000 \nonumber\\
ed_be & 1.00000 \nonumber\\
payer & 1.00000 \nonumber\\
responsible_with & 1.00000 \nonumber\\
go_swim & 1.00000 \nonumber\\
car_, & 1.00000 \nonumber\\
the_tax & 1.00000 \nonumber\\
tax_payer & 1.00000 \nonumber\\
another_class & 1.00000 \nonumber\\
swim_or & 1.00000 \nonumber\\
should_start & 1.00000 \nonumber\\
time_they & 1.00000 \nonumber\\
for_student & 1.00000 \nonumber\\
a_car & 1.00000 \nonumber\\
their_health & 1.00000 \nonumber\\
just_another & 1.00000 \nonumber\\
swim & 1.00000 \nonumber\\
dont_realize & 1.00000 \nonumber\\
payer_also & 1.00000 \nonumber\\
also_dont & 1.00000 \nonumber\\
in_highschool & 1.00000 \nonumber\\
highschool_. & 1.00000 \nonumber\\
or_play & 1.00000 \nonumber\\
highschool & 1.00000 \nonumber\\
hardly & 1.00000 \nonumber\\
ProductionRule_NP->NP,X, & 1.00000 \nonumber\\
n't_imagine & 1.00000 \nonumber\\
_pos_ngram_PR_PR_PP & 1.00000 \nonumber\\
ProductionRule_FRAG->SBAR,., & 1.00000 \nonumber\\
nobody_would & 1.00000 \nonumber\\
or_anything & 1.00000 \nonumber\\
out_into & 1.00000 \nonumber\\
because_one & 1.00000 \nonumber\\
can_go & 1.00000 \nonumber\\
no_happiness & 1.00000 \nonumber\\
themselve_happy & 1.00000 \nonumber\\
ProductionRule_VP->MD,ADVP,S,SBAR, & 1.00000 \nonumber\\
must_themselve & 1.00000 \nonumber\\
happiness_in & 1.00000 \nonumber\\
people_find & 1.00000 \nonumber\\
happy_before & 1.00000 \nonumber\\
leave_no & 1.00000 \nonumber\\
own_pursuit & 1.00000 \nonumber\\
a_wreak & 1.00000 \nonumber\\
you_leave & 1.00000 \nonumber\\
wreak & 1.00000 \nonumber\\
wreak_and & 1.00000 \nonumber\\
else_happy & 1.00000 \nonumber\\
one_must & 1.00000 \nonumber\\
need_more & 1.00000 \nonumber\\
version & 1.00000 \nonumber\\
last_thing & 1.00000 \nonumber\\
)_so & 1.00000 \nonumber\\
usually & 1.00000 \nonumber\\
be_prove & 1.00000 \nonumber\\
one_because & 1.00000 \nonumber\\
could_hide & 1.00000 \nonumber\\
accident_more & 1.00000 \nonumber\\
than_once & 1.00000 \nonumber\\
once_. & 1.00000 \nonumber\\
ProductionRule_NP->DT,QP, & 1.00000 \nonumber\\
hide_the & 1.00000 \nonumber\\
never_happen & 1.00000 \nonumber\\
unless_he & 1.00000 \nonumber\\
person_enough & 1.00000 \nonumber\\
in_unless & 1.00000 \nonumber\\
enough_i & 1.00000 \nonumber\\
up_who & 1.00000 \nonumber\\
your_mother & 1.00000 \nonumber\\
alive & 1.00000 \nonumber\\
whole_world & 1.00000 \nonumber\\
a_much & 1.00000 \nonumber\\
stress_on & 1.00000 \nonumber\\
its_celebration & 1.00000 \nonumber\\
nature_. & 1.00000 \nonumber\\
restrict & 1.00000 \nonumber\\
deprive_the & 1.00000 \nonumber\\
unity_in & 1.00000 \nonumber\\
the_stress & 1.00000 \nonumber\\
to_restrict & 1.00000 \nonumber\\
they_deprive & 1.00000 \nonumber\\
the_spirit & 1.00000 \nonumber\\
vital_aspect & 1.00000 \nonumber\\
celebration_. & 1.00000 \nonumber\\
deprive & 1.00000 \nonumber\\
diversity & 1.00000 \nonumber\\
in_diversity & 1.00000 \nonumber\\
code_in & 1.00000 \nonumber\\
school_oppose & 1.00000 \nonumber\\
uniform_dress & 1.00000 \nonumber\\
a_vital & 1.00000 \nonumber\\
oppose_the & 1.00000 \nonumber\\
celebration & 1.00000 \nonumber\\
even_claim & 1.00000 \nonumber\\
diversity_and & 1.00000 \nonumber\\
against_school & 1.00000 \nonumber\\
restrict_socialization & 1.00000 \nonumber\\
socialization_, & 1.00000 \nonumber\\
of_unity & 1.00000 \nonumber\\
reason_argue & 1.00000 \nonumber\\
socialization & 1.00000 \nonumber\\
spirit_of & 1.00000 \nonumber\\
3_some & 1.00000 \nonumber\\
actually_like & 1.00000 \nonumber\\
._sex & 1.00000 \nonumber\\
compensate_well & 1.00000 \nonumber\\
compensate & 1.00000 \nonumber\\
say_porn & 1.00000 \nonumber\\
1_they & 1.00000 \nonumber\\
sex_= & 1.00000 \nonumber\\
4_without & 1.00000 \nonumber\\
2_they & 1.00000 \nonumber\\
_pos_ngram_CARD_PP_NN & 1.00000 \nonumber\\
porn_degrade & 1.00000 \nonumber\\
girl_actually & 1.00000 \nonumber\\
whoever_say & 1.00000 \nonumber\\
get_compensate & 1.00000 \nonumber\\
some_girl & 1.00000 \nonumber\\
ProductionRule_S->SBARQ,NP,VP,., & 1.00000 \nonumber\\
._= & 1.00000 \nonumber\\
without_sex & 1.00000 \nonumber\\
degrade_woman & 1.00000 \nonumber\\
=_) & 1.00000 \nonumber\\
=_life & 1.00000 \nonumber\\
_pos_ngram_O_CARD_ART & 1.00000 \nonumber\\
#_4 & 1.00000 \nonumber\\
= & 1.00000 \nonumber\\
_pos_ngram_ADJ_NN_NP & 1.00000 \nonumber\\
childhood & 1.00000 \nonumber\\
appreciate & 1.00000 \nonumber\\
on_myself & 1.00000 \nonumber\\
spend_time & 1.00000 \nonumber\\
ProductionRule_S->SBAR,,,ADVP,VP, & 1.00000 \nonumber\\
best_to & 1.00000 \nonumber\\
or_people & 1.00000 \nonumber\\
by_that & 1.00000 \nonumber\\
i_wo & 1.00000 \nonumber\\
my_best & 1.00000 \nonumber\\
feel_better & 1.00000 \nonumber\\
appreciate_by & 1.00000 \nonumber\\
it_appreciate & 1.00000 \nonumber\\
accomplish_that & 1.00000 \nonumber\\
myself_, & 1.00000 \nonumber\\
to_reproduce & 1.00000 \nonumber\\
issue_. & 1.00000 \nonumber\\
._over & 1.00000 \nonumber\\
suit_us & 1.00000 \nonumber\\
we_adapt & 1.00000 \nonumber\\
best_otherwise & 1.00000 \nonumber\\
us_best & 1.00000 \nonumber\\
_pos_ngram_ADV_PR_CARD & 1.00000 \nonumber\\
there_so & 1.00000 \nonumber\\
what_suit & 1.00000 \nonumber\\
otherwise_why & 1.00000 \nonumber\\
to_adapt & 1.00000 \nonumber\\
we_one & 1.00000 \nonumber\\
one_skin & 1.00000 \nonumber\\
why_ar & 1.00000 \nonumber\\
ar_n't & 1.00000 \nonumber\\
ar & 1.00000 \nonumber\\
of_animal & 1.00000 \nonumber\\
its_simple & 1.00000 \nonumber\\
skin_colour & 1.00000 \nonumber\\
ProductionRule_S->NP,,,ADVP,VP,., & 1.00000 \nonumber\\
over_time & 1.00000 \nonumber\\
time_we & 1.00000 \nonumber\\
colour_, & 1.00000 \nonumber\\
self-opinion & 1.00000 \nonumber\\
interaction_, & 1.00000 \nonumber\\
myself_for & 1.00000 \nonumber\\
half_a & 1.00000 \nonumber\\
fatherly_interaction & 1.00000 \nonumber\\
would_rub & 1.00000 \nonumber\\
essential_time & 1.00000 \nonumber\\
man_, & 1.00000 \nonumber\\
i_live & 1.00000 \nonumber\\
model_and & 1.00000 \nonumber\\
major_male & 1.00000 \nonumber\\
(_self-opinion & 1.00000 \nonumber\\
up_completely & 1.00000 \nonumber\\
mold_me & 1.00000 \nonumber\\
first_thirteen & 1.00000 \nonumber\\
,_albeit & 1.00000 \nonumber\\
around_his/her & 1.00000 \nonumber\\
ProductionRule_SBAR->IN,NP, & 1.00000 \nonumber\\
albeit_a & 1.00000 \nonumber\\
albeit & 1.00000 \nonumber\\
his/her_father & 1.00000 \nonumber\\
self-opinion_) & 1.00000 \nonumber\\
example_; & 1.00000 \nonumber\\
great_( & 1.00000 \nonumber\\
into_half & 1.00000 \nonumber\\
as_oppose & 1.00000 \nonumber\\
rub_off & 1.00000 \nonumber\\
the_essential & 1.00000 \nonumber\\
rub & 1.00000 \nonumber\\
take_myself & 1.00000 \nonumber\\
so_yes & 1.00000 \nonumber\\
completely_fatherless & 1.00000 \nonumber\\
oppose_to & 1.00000 \nonumber\\
any_major & 1.00000 \nonumber\\
thirteen_year & 1.00000 \nonumber\\
me_into & 1.00000 \nonumber\\
successful_. & 1.00000 \nonumber\\
any_fatherly & 1.00000 \nonumber\\
to_that & 1.00000 \nonumber\\
the_age & 1.00000 \nonumber\\
ProductionRule_NP->PRP$,NN,NN,NN, & 1.00000 \nonumber\\
option_, & 1.00000 \nonumber\\
crime_and & 1.00000 \nonumber\\
less_land & 1.00000 \nonumber\\
medal & 1.00000 \nonumber\\
land_, & 1.00000 \nonumber\\
the_increase & 1.00000 \nonumber\\
gold_medal & 1.00000 \nonumber\\
of_corrosion & 1.00000 \nonumber\\
increase_population & 1.00000 \nonumber\\
means_a & 1.00000 \nonumber\\
means_less & 1.00000 \nonumber\\
corrosion_, & 1.00000 \nonumber\\
medal_of & 1.00000 \nonumber\\
terrorism_, & 1.00000 \nonumber\\
crowd_on & 1.00000 \nonumber\\
crowd & 1.00000 \nonumber\\
every_place & 1.00000 \nonumber\\
land_means & 1.00000 \nonumber\\
corrosion & 1.00000 \nonumber\\
population_means & 1.00000 \nonumber\\
big_crowd & 1.00000 \nonumber\\
,_illeteracy & 1.00000 \nonumber\\
win_gold & 1.00000 \nonumber\\
,_violence & 1.00000 \nonumber\\
illeteracy & 1.00000 \nonumber\\
illeteracy_, & 1.00000 \nonumber\\
be_equal & 1.00000 \nonumber\\
too_lazy & 1.00000 \nonumber\\
indium_and & 1.00000 \nonumber\\
and_china & 1.00000 \nonumber\\
one_in & 1.00000 \nonumber\\
ProductionRule_VP->TO,NP, & 1.00000 \nonumber\\
africa_, & 1.00000 \nonumber\\
africa & 1.00000 \nonumber\\
ProductionRule_NP->NP,NN,S, & 1.00000 \nonumber\\
condemn_consensual-cannibalism & 1.00000 \nonumber\\
consensual-cannibalism & 1.00000 \nonumber\\
consensual-cannibalism_in & 1.00000 \nonumber\\
body_? & 1.00000 \nonumber\\
should_abortion & 1.00000 \nonumber\\
people_condemn & 1.00000 \nonumber\\
do_they & 1.00000 \nonumber\\
ProductionRule_SQ->VBD,NP,VP, & 1.00000 \nonumber\\
ProductionRule_SBARQ->WHADVP,PRN,SQ,., & 1.00000 \nonumber\\
condemn & 1.00000 \nonumber\\
in_africa & 1.00000 \nonumber\\
any_different & 1.00000 \nonumber\\
to_receive & 1.00000 \nonumber\\
religon & 1.00000 \nonumber\\
religon_and & 1.00000 \nonumber\\
up_my & 1.00000 \nonumber\\
ProductionRule_VP->LS,ADVP,VP, & 1.00000 \nonumber\\
ProductionRule_FRAG->ADJP,SBAR,., & 1.00000 \nonumber\\
my_religon & 1.00000 \nonumber\\
christian_so & 1.00000 \nonumber\\
down_. & 1.00000 \nonumber\\
,_without & 1.00000 \nonumber\\
gimmick & 1.00000 \nonumber\\
own_tongue & 1.00000 \nonumber\\
some_sush102 & 1.00000 \nonumber\\
nd_run & 1.00000 \nonumber\\
between_chatng & 1.00000 \nonumber\\
dnt & 1.00000 \nonumber\\
dnt_" & 1.00000 \nonumber\\
dnt_teach & 1.00000 \nonumber\\
will_b & 1.00000 \nonumber\\
no_difference & 1.00000 \nonumber\\
me_wat & 1.00000 \nonumber\\
quote_some & 1.00000 \nonumber\\
be_quote & 1.00000 \nonumber\\
wat_da & 1.00000 \nonumber\\
sush102_" & 1.00000 \nonumber\\
chatng_nd & 1.00000 \nonumber\\
better_dnt & 1.00000 \nonumber\\
indian_at & 1.00000 \nonumber\\
indian_be & 1.00000 \nonumber\\
still_remains & 1.00000 \nonumber\\
"_hey & 1.00000 \nonumber\\
....._if & 1.00000 \nonumber\\
manage_to & 1.00000 \nonumber\\
...._" & 1.00000 \nonumber\\
these_mongrel & 1.00000 \nonumber\\
b_4ce & 1.00000 \nonumber\\
away_.... & 1.00000 \nonumber\\
den_u & 1.00000 \nonumber\\
sush102 & 1.00000 \nonumber\\
start_my & 1.00000 \nonumber\\
we_indian & 1.00000 \nonumber\\
nd_debatng & 1.00000 \nonumber\\
'_language & 1.00000 \nonumber\\
gimmick_stumble & 1.00000 \nonumber\\
di_" & 1.00000 \nonumber\\
it_still & 1.00000 \nonumber\\
di_site & 1.00000 \nonumber\\
difference_what & 1.00000 \nonumber\\
crap_? & 1.00000 \nonumber\\
crap_be & 1.00000 \nonumber\\
u_bloody & 1.00000 \nonumber\\
ma & 1.00000 \nonumber\\
ma_" & 1.00000 \nonumber\\
"_dnt & 1.00000 \nonumber\\
tongue & 1.00000 \nonumber\\
site_nd & 1.00000 \nonumber\\
tongue_. & 1.00000 \nonumber\\
mongrel_' & 1.00000 \nonumber\\
mongrel & 1.00000 \nonumber\\
4ce_to & 1.00000 \nonumber\\
english_gimmick & 1.00000 \nonumber\\
"_ma & 1.00000 \nonumber\\
differnce & 1.00000 \nonumber\\
na_den & 1.00000 \nonumber\\
da_differnce & 1.00000 \nonumber\\
pretty_good & 1.00000 \nonumber\\
debatng_..... & 1.00000 \nonumber\\
ProductionRule_NP->PRP,NNPS, & 1.00000 \nonumber\\
my_say & 1.00000 \nonumber\\
teach_me & 1.00000 \nonumber\\
debatng & 1.00000 \nonumber\\
debate_na & 1.00000 \nonumber\\
"_di & 1.00000 \nonumber\\
differnce_between & 1.00000 \nonumber\\
chatng & 1.00000 \nonumber\\
bloody_will & 1.00000 \nonumber\\
my_debate & 1.00000 \nonumber\\
4ce & 1.00000 \nonumber\\
???_it & 1.00000 \nonumber\\
you_english & 1.00000 \nonumber\\
already_have & 1.00000 \nonumber\\
stumble_in & 1.00000 \nonumber\\
hey_its & 1.00000 \nonumber\\
best_!!!! & 1.00000 \nonumber\\
that_??? & 1.00000 \nonumber\\
learn_these & 1.00000 \nonumber\\
what_crap & 1.00000 \nonumber\\
_pos_ngram_NN_ADV_CARD & 1.00000 \nonumber\\
_pos_ngram_O_PR_ADJ & 1.00000 \nonumber\\
remains_that & 1.00000 \nonumber\\
i_already & 1.00000 \nonumber\\
leave_di & 1.00000 \nonumber\\
least_manage & 1.00000 \nonumber\\
stumble & 1.00000 \nonumber\\
like_marriage & 1.00000 \nonumber\\
drive_through & 1.00000 \nonumber\\
do_when & 1.00000 \nonumber\\
holy_thing & 1.00000 \nonumber\\
be_fake & 1.00000 \nonumber\\
high_holy & 1.00000 \nonumber\\
fake_love & 1.00000 \nonumber\\
-_we & 1.00000 \nonumber\\
ProductionRule_FRAG->ADVP,:,SBAR,., & 1.00000 \nonumber\\
some_high & 1.00000 \nonumber\\
we_sell & 1.00000 \nonumber\\
sell_it & 1.00000 \nonumber\\
will_you & 1.00000 \nonumber\\
what_will & 1.00000 \nonumber\\
care_- & 1.00000 \nonumber\\
thing_- & 1.00000 \nonumber\\
in_drive & 1.00000 \nonumber\\
etc._and & 1.00000 \nonumber\\
people_really & 1.00000 \nonumber\\
their_friend & 1.00000 \nonumber\\
plus_what & 1.00000 \nonumber\\
together_so & 1.00000 \nonumber\\
through_, & 1.00000 \nonumber\\
together_then & 1.00000 \nonumber\\
honestly_who & 1.00000 \nonumber\\
be_way & 1.00000 \nonumber\\
_pos_ngram_NP_NN_CONJ & 1.00000 \nonumber\\
school_they & 1.00000 \nonumber\\
yet_you & 1.00000 \nonumber\\
list_them & 1.00000 \nonumber\\
be_last & 1.00000 \nonumber\\
pop_up & 1.00000 \nonumber\\
website_( & 1.00000 \nonumber\\
virus_ie & 1.00000 \nonumber\\
new_browser & 1.00000 \nonumber\\
two_website & 1.00000 \nonumber\\
restart_or & 1.00000 \nonumber\\
search_two & 1.00000 \nonumber\\
to_list & 1.00000 \nonumber\\
at_in & 1.00000 \nonumber\\
get_up & 1.00000 \nonumber\\
tab_option & 1.00000 \nonumber\\
website_at & 1.00000 \nonumber\\
_pos_ngram_PUNC_PUNC_CARD & 1.00000 \nonumber\\
annoy_load & 1.00000 \nonumber\\
and_virus & 1.00000 \nonumber\\
/_oh & 1.00000 \nonumber\\
whole_new & 1.00000 \nonumber\\
last_at & 1.00000 \nonumber\\
?!_main & 1.00000 \nonumber\\
feature_i & 1.00000 \nonumber\\
the_website & 1.00000 \nonumber\\
require_you & 1.00000 \nonumber\\
you_continue & 1.00000 \nonumber\\
ie_require & 1.00000 \nonumber\\
cool_feature & 1.00000 \nonumber\\
oh_and & 1.00000 \nonumber\\
check_ie & 1.00000 \nonumber\\
the_annoy & 1.00000 \nonumber\\
a_restart & 1.00000 \nonumber\\
pointlessss_. & 1.00000 \nonumber\\
it_?! & 1.00000 \nonumber\\
order_search & 1.00000 \nonumber\\
many_cool & 1.00000 \nonumber\\
i_pity & 1.00000 \nonumber\\
pointlessss & 1.00000 \nonumber\\
and_. & 1.00000 \nonumber\\
of_pop & 1.00000 \nonumber\\
firefox_save & 1.00000 \nonumber\\
pity & 1.00000 \nonumber\\
pity_those & 1.00000 \nonumber\\
have_, & 1.00000 \nonumber\\
'_pointlessss & 1.00000 \nonumber\\
about_that & 1.00000 \nonumber\\
i_grow & 1.00000 \nonumber\\
a_sible & 1.00000 \nonumber\\
ProductionRule_SBAR->RB,RB,S, & 1.00000 \nonumber\\
she_tend & 1.00000 \nonumber\\
10_than & 1.00000 \nonumber\\
even_now & 1.00000 \nonumber\\
spank_along & 1.00000 \nonumber\\
ProductionRule_S->PP,S,CC,S, & 1.00000 \nonumber\\
least_because & 1.00000 \nonumber\\
mistake_even & 1.00000 \nonumber\\
sible & 1.00000 \nonumber\\
sible_of & 1.00000 \nonumber\\
hand_our & 1.00000 \nonumber\\
youngest_sister & 1.00000 \nonumber\\
youngest & 1.00000 \nonumber\\
now_that & 1.00000 \nonumber\\
discipline_and & 1.00000 \nonumber\\
she_10 & 1.00000 \nonumber\\
sister_have & 1.00000 \nonumber\\
resort_at & 1.00000 \nonumber\\
my_sister & 1.00000 \nonumber\\
our_youngest & 1.00000 \nonumber\\
believe_so & 1.00000 \nonumber\\
ProductionRule_VP->S,,,VP, & 1.00000 \nonumber\\
of_three & 1.00000 \nonumber\\
ProductionRule_S->S,RB,,,S,CC,S,., & 1.00000 \nonumber\\
more_mistake & 1.00000 \nonumber\\
because_researcher & 1.00000 \nonumber\\
researcher & 1.00000 \nonumber\\
failure_to & 1.00000 \nonumber\\
same_billion & 1.00000 \nonumber\\
be_purely & 1.00000 \nonumber\\
recreate_it & 1.00000 \nonumber\\
a_laboratory & 1.00000 \nonumber\\
laboratory & 1.00000 \nonumber\\
devote_those & 1.00000 \nonumber\\
have_fail & 1.00000 \nonumber\\
laboratory_be & 1.00000 \nonumber\\
to_devote & 1.00000 \nonumber\\
researcher_have & 1.00000 \nonumber\\
any_failure & 1.00000 \nonumber\\
those_same & 1.00000 \nonumber\\
around_for & 1.00000 \nonumber\\
year_try & 1.00000 \nonumber\\
purely_because & 1.00000 \nonumber\\
to_recreate & 1.00000 \nonumber\\
for_billion & 1.00000 \nonumber\\
recreate & 1.00000 \nonumber\\
girl_, & 1.00000 \nonumber\\
adapt_to & 1.00000 \nonumber\\
$_7.7 & 1.00000 \nonumber\\
company_produce & 1.00000 \nonumber\\
roughly_35,000 & 1.00000 \nonumber\\
company_in & 1.00000 \nonumber\\
2002_. & 1.00000 \nonumber\\
for_bottle & 1.00000 \nonumber\\
market_corporation & 1.00000 \nonumber\\
_pos_ngram_CARD_CARD_PUNC & 1.00000 \nonumber\\
billion_. & 1.00000 \nonumber\\
research_and & 1.00000 \nonumber\\
corporation_, & 1.00000 \nonumber\\
alone_pay & 1.00000 \nonumber\\
pay_$ & 1.00000 \nonumber\\
beverage_market & 1.00000 \nonumber\\
the_beverage & 1.00000 \nonumber\\
consult_do & 1.00000 \nonumber\\
to_over & 1.00000 \nonumber\\
$_35 & 1.00000 \nonumber\\
'_thousand & 1.00000 \nonumber\\
_pos_ngram_CARD_CARD_PP & 1.00000 \nonumber\\
have_explode & 1.00000 \nonumber\\
billion_for & 1.00000 \nonumber\\
roughly & 1.00000 \nonumber\\
7.7 & 1.00000 \nonumber\\
liter_of & 1.00000 \nonumber\\
liter & 1.00000 \nonumber\\
the_global & 1.00000 \nonumber\\
%_. & 1.00000 \nonumber\\
by_over & 1.00000 \nonumber\\
._american & 1.00000 \nonumber\\
example_globally & 1.00000 \nonumber\\
this_produce & 1.00000 \nonumber\\
dollar_in & 1.00000 \nonumber\\
over_130,000 & 1.00000 \nonumber\\
explode_to & 1.00000 \nonumber\\
in_revenue & 1.00000 \nonumber\\
revenue_for & 1.00000 \nonumber\\
in_2002 & 1.00000 \nonumber\\
13_% & 1.00000 \nonumber\\
american_alone & 1.00000 \nonumber\\
130,000_million & 1.00000 \nonumber\\
in_2001 & 1.00000 \nonumber\\
revenue & 1.00000 \nonumber\\
to_research & 1.00000 \nonumber\\
13 & 1.00000 \nonumber\\
million_dollar & 1.00000 \nonumber\\
million_liter & 1.00000 \nonumber\\
global_bottle & 1.00000 \nonumber\\
alone_grow & 1.00000 \nonumber\\
produce_roughly & 1.00000 \nonumber\\
130,000 & 1.00000 \nonumber\\
2001_. & 1.00000 \nonumber\\
35 & 1.00000 \nonumber\\
over_13 & 1.00000 \nonumber\\
over_$ & 1.00000 \nonumber\\
do_by & 1.00000 \nonumber\\
7.7_billion & 1.00000 \nonumber\\
u.s._alone & 1.00000 \nonumber\\
produce_over & 1.00000 \nonumber\\
2002 & 1.00000 \nonumber\\
grow_by & 1.00000 \nonumber\\
35_billion & 1.00000 \nonumber\\
explode & 1.00000 \nonumber\\
globally_bottle & 1.00000 \nonumber\\
35,000 & 1.00000 \nonumber\\
2001 & 1.00000 \nonumber\\
2001_, & 1.00000 \nonumber\\
35,000_million & 1.00000 \nonumber\\
and_consult & 1.00000 \nonumber\\
for_yourself & 1.00000 \nonumber\\
much_or & 1.00000 \nonumber\\
grow_and & 1.00000 \nonumber\\
kid_the & 1.00000 \nonumber\\
kid_just & 1.00000 \nonumber\\
be_grow & 1.00000 \nonumber\\
eventually_they & 1.00000 \nonumber\\
just_eat & 1.00000 \nonumber\\
ProductionRule_NP->RB,RB, & 1.00000 \nonumber\\
help_fat & 1.00000 \nonumber\\
and_eventually & 1.00000 \nonumber\\
p.e_do & 1.00000 \nonumber\\
all_in & 1.00000 \nonumber\\
stop_you & 1.00000 \nonumber\\
be_stricter & 1.00000 \nonumber\\
stricter & 1.00000 \nonumber\\
experience_. & 1.00000 \nonumber\\
you_grow & 1.00000 \nonumber\\
_pos_ngram_CARD_CONJ_ADJ & 1.00000 \nonumber\\
,_me & 1.00000 \nonumber\\
be_the & 1.00000 \nonumber\\
i_agree & 1.00000 \nonumber\\
a_british & 1.00000 \nonumber\\
that_cant & 1.00000 \nonumber\\
war & 1.00000 \nonumber\\
ProductionRule_SBAR->RB,IN,S,., & 1.00000 \nonumber\\
no_evidence & 1.00000 \nonumber\\
sky & 1.00000 \nonumber\\
for_which & 1.00000 \nonumber\\
history_weve & 1.00000 \nonumber\\
which_no & 1.00000 \nonumber\\
in_sky & 1.00000 \nonumber\\
since_record & 1.00000 \nonumber\\
evidence_exist & 1.00000 \nonumber\\
sky_spirit & 1.00000 \nonumber\\
ProductionRule_NP->VBN,NN,NN, & 1.00000 \nonumber\\
exist_at & 1.00000 \nonumber\\
ever_since & 1.00000 \nonumber\\
weve & 1.00000 \nonumber\\
weve_believe & 1.00000 \nonumber\\
spirit_for & 1.00000 \nonumber\\
,_uniform & 1.00000 \nonumber\\
herself_pregnant & 1.00000 \nonumber\\
they_believe & 1.00000 \nonumber\\
when_rape & 1.00000 \nonumber\\
woman_have & 1.00000 \nonumber\\
mother_fault & 1.00000 \nonumber\\
she_get & 1.00000 \nonumber\\
she_more & 1.00000 \nonumber\\
fault_but & 1.00000 \nonumber\\
!_when & 1.00000 \nonumber\\
be_children & 1.00000 \nonumber\\
die_? & 1.00000 \nonumber\\
it_wasnt & 1.00000 \nonumber\\
,_defenceless & 1.00000 \nonumber\\
be_innocent & 1.00000 \nonumber\\
wasnt_the & 1.00000 \nonumber\\
defenceless_baby & 1.00000 \nonumber\\
be_concern & 1.00000 \nonumber\\
selfish_where & 1.00000 \nonumber\\
defenceless & 1.00000 \nonumber\\
child_? & 1.00000 \nonumber\\
rape_occur & 1.00000 \nonumber\\
choice_and & 1.00000 \nonumber\\
have_become & 1.00000 \nonumber\\
pregnant_! & 1.00000 \nonumber\\
innocent_, & 1.00000 \nonumber\\
life_we & 1.00000 \nonumber\\
get_herself & 1.00000 \nonumber\\
pregnant_and & 1.00000 \nonumber\\
circumstance_a & 1.00000 \nonumber\\
concern_. & 1.00000 \nonumber\\
there_body & 1.00000 \nonumber\\
in_she & 1.00000 \nonumber\\
get_no & 1.00000 \nonumber\\
children_life & 1.00000 \nonumber\\
become_selfish & 1.00000 \nonumber\\
body_be & 1.00000 \nonumber\\
occur_why & 1.00000 \nonumber\\
baby_who & 1.00000 \nonumber\\
n't_stop & 1.00000 \nonumber\\
ProductionRule_NP->NNP,NNP,., & 1.00000 \nonumber\\
not_! & 1.00000 \nonumber\\
bloody & 1.00000 \nonumber\\
third_world & 1.00000 \nonumber\\
simultaneously_. & 1.00000 \nonumber\\
country_simultaneously & 1.00000 \nonumber\\
china_could & 1.00000 \nonumber\\
be_first & 1.00000 \nonumber\\
country_means & 1.00000 \nonumber\\
could_redefine & 1.00000 \nonumber\\
simultaneously & 1.00000 \nonumber\\
both_will & 1.00000 \nonumber\\
redefine_what & 1.00000 \nonumber\\
ProductionRule_NP->ADJP,NN,NNS, & 1.00000 \nonumber\\
what_third & 1.00000 \nonumber\\
and_third & 1.00000 \nonumber\\
means_because & 1.00000 \nonumber\\
their_mind & 1.00000 \nonumber\\
turn_his & 1.00000 \nonumber\\
regardless_of & 1.00000 \nonumber\\
regardless & 1.00000 \nonumber\\
something_i & 1.00000 \nonumber\\
back_this & 1.00000 \nonumber\\
person_at & 1.00000 \nonumber\\
,_9 & 1.00000 \nonumber\\
in_share & 1.00000 \nonumber\\
think_advancement & 1.00000 \nonumber\\
guess_because & 1.00000 \nonumber\\
advance_of & 1.00000 \nonumber\\
me_personally & 1.00000 \nonumber\\
personally_for & 1.00000 \nonumber\\
all_when & 1.00000 \nonumber\\
10_i & 1.00000 \nonumber\\
well_me & 1.00000 \nonumber\\
the_topic & 1.00000 \nonumber\\
to_sacrifice & 1.00000 \nonumber\\
the_advance & 1.00000 \nonumber\\
sacrifice_personally & 1.00000 \nonumber\\
._4 & 1.00000 \nonumber\\
to_those & 1.00000 \nonumber\\
exact_opposite & 1.00000 \nonumber\\
attention_again & 1.00000 \nonumber\\
help_him & 1.00000 \nonumber\\
will_move & 1.00000 \nonumber\\
a_cost & 1.00000 \nonumber\\
hide_all & 1.00000 \nonumber\\
his_attention & 1.00000 \nonumber\\
opposite_i & 1.00000 \nonumber\\
never_bring & 1.00000 \nonumber\\
if_any & 1.00000 \nonumber\\
cost_. & 1.00000 \nonumber\\
bring_it & 1.00000 \nonumber\\
any_, & 1.00000 \nonumber\\
him_hide & 1.00000 \nonumber\\
move_if & 1.00000 \nonumber\\
_pos_ngram_NP_PUNC_CONJ & 1.00000 \nonumber\\
our_self & 1.00000 \nonumber\\
mother_. & 1.00000 \nonumber\\
,_maybe & 1.00000 \nonumber\\
again_. & 1.00000 \nonumber\\
want_your & 1.00000 \nonumber\\
would_also & 1.00000 \nonumber\\
note & 1.00000 \nonumber\\
man_or & 1.00000 \nonumber\\
where_there & 1.00000 \nonumber\\
-- & 1.00000 \nonumber\\
?_that & 1.00000 \nonumber\\
ProductionRule_PP->CC,NP, & 1.00000 \nonumber\\
get_on & 1.00000 \nonumber\\
itself_... & 1.00000 \nonumber\\
on_society & 1.00000 \nonumber\\
furthermore_, & 1.00000 \nonumber\\
any_assumption & 1.00000 \nonumber\\
assumption & 1.00000 \nonumber\\
with_semantics & 1.00000 \nonumber\\
be_minimal & 1.00000 \nonumber\\
essentially_play & 1.00000 \nonumber\\
"_civil & 1.00000 \nonumber\\
challenge_any & 1.00000 \nonumber\\
assumption_? & 1.00000 \nonumber\\
why_challenge & 1.00000 \nonumber\\
semantics & 1.00000 \nonumber\\
bind_to & 1.00000 \nonumber\\
society_be & 1.00000 \nonumber\\
law_should & 1.00000 \nonumber\\
play_with & 1.00000 \nonumber\\
semantics_. & 1.00000 \nonumber\\
furthermore & 1.00000 \nonumber\\
lie_to & 1.00000 \nonumber\\
longer_than & 1.00000 \nonumber\\
characteristic_of & 1.00000 \nonumber\\
teach_them & 1.00000 \nonumber\\
its_completely & 1.00000 \nonumber\\
get_ta & 1.00000 \nonumber\\
fact_be & 1.00000 \nonumber\\
ProductionRule_ADJP->RB,NN, & 1.00000 \nonumber\\
ta_pick & 1.00000 \nonumber\\
ProductionRule_S->S,,,RB,S, & 1.00000 \nonumber\\
until_its & 1.00000 \nonumber\\
mainstream_i & 1.00000 \nonumber\\
pick_ie & 1.00000 \nonumber\\
completely_mainstream & 1.00000 \nonumber\\
mainstream & 1.00000 \nonumber\\
all_site & 1.00000 \nonumber\\
site_work & 1.00000 \nonumber\\
ta & 1.00000 \nonumber\\
work_well & 1.00000 \nonumber\\
_pos_ngram_PUNC_PUNC_PUNC & 1.00000 \nonumber\\
learn_malay & 1.00000 \nonumber\\
initiative_to & 1.00000 \nonumber\\
make_conversation & 1.00000 \nonumber\\
conversation & 1.00000 \nonumber\\
he_even & 1.00000 \nonumber\\
initiative & 1.00000 \nonumber\\
conversation_easier & 1.00000 \nonumber\\
malay_just & 1.00000 \nonumber\\
local_and & 1.00000 \nonumber\\
william_make & 1.00000 \nonumber\\
the_initiative & 1.00000 \nonumber\\
even_learn & 1.00000 \nonumber\\
to_communicate & 1.00000 \nonumber\\
army & 1.00000 \nonumber\\
singapore.this & 1.00000 \nonumber\\
their_self & 1.00000 \nonumber\\
be_create & 1.00000 \nonumber\\
anyway_. & 1.00000 \nonumber\\
me_to & 1.00000 \nonumber\\
make_no & 1.00000 \nonumber\\
meet_my & 1.00000 \nonumber\\
to_meet & 1.00000 \nonumber\\
_pos_ngram_PUNC_O_NP & 1.00000 \nonumber\\
ProductionRule_SBAR->IN,,,S, & 1.00000 \nonumber\\
or_negative & 1.00000 \nonumber\\
ya & 1.00000 \nonumber\\
to_remind & 1.00000 \nonumber\\
a_punishment & 1.00000 \nonumber\\
we_go & 1.00000 \nonumber\\
they_gon & 1.00000 \nonumber\\
_pos_ngram_CONJ_ADJ_CARD & 1.00000 \nonumber\\
ya_, & 1.00000 \nonumber\\
punishment_and & 1.00000 \nonumber\\
will_see & 1.00000 \nonumber\\
logo_for & 1.00000 \nonumber\\
teacher_give & 1.00000 \nonumber\\
teacher_will & 1.00000 \nonumber\\
discipline_student & 1.00000 \nonumber\\
we_from & 1.00000 \nonumber\\
for_our & 1.00000 \nonumber\\
use_our & 1.00000 \nonumber\\
see_we & 1.00000 \nonumber\\
school_thankyou & 1.00000 \nonumber\\
school_than & 1.00000 \nonumber\\
us_a & 1.00000 \nonumber\\
important_1 & 1.00000 \nonumber\\
uniform_basically & 1.00000 \nonumber\\
school_2 & 1.00000 \nonumber\\
a_discipline & 1.00000 \nonumber\\
uniform_so & 1.00000 \nonumber\\
student_use & 1.00000 \nonumber\\
us_that & 1.00000 \nonumber\\
basically_student & 1.00000 \nonumber\\
our_uniform & 1.00000 \nonumber\\
a_logo & 1.00000 \nonumber\\
student_5 & 1.00000 \nonumber\\
school_3 & 1.00000 \nonumber\\
._school & 1.00000 \nonumber\\
_pos_ngram_PR_NN_CARD & 1.00000 \nonumber\\
negative_4 & 1.00000 \nonumber\\
remind_us & 1.00000 \nonumber\\
positive_or & 1.00000 \nonumber\\
ProductionRule_FRAG->ADVP,,,PP,., & 1.00000 \nonumber\\
it_positive & 1.00000 \nonumber\\
the_teacher & 1.00000 \nonumber\\
morn_we & 1.00000 \nonumber\\
wasnt & 1.00000 \nonumber\\
hate_it & 1.00000 \nonumber\\
already_be & 1.00000 \nonumber\\
or_, & 1.00000 \nonumber\\
time_when & 1.00000 \nonumber\\
out_with & 1.00000 \nonumber\\
support_me & 1.00000 \nonumber\\
as_me & 1.00000 \nonumber\\
have_many & 1.00000 \nonumber\\
uniform_prove & 1.00000 \nonumber\\
and_wasteful & 1.00000 \nonumber\\
_pos_ngram_CONJ_ADJ_ADV & 1.00000 \nonumber\\
in_comparison & 1.00000 \nonumber\\
civil_dress & 1.00000 \nonumber\\
comparison & 1.00000 \nonumber\\
be_futile & 1.00000 \nonumber\\
wasteful_once & 1.00000 \nonumber\\
to_civil & 1.00000 \nonumber\\
once_the & 1.00000 \nonumber\\
dress_, & 1.00000 \nonumber\\
futile_and & 1.00000 \nonumber\\
futile & 1.00000 \nonumber\\
comparison_to & 1.00000 \nonumber\\
give_them & 1.00000 \nonumber\\
a_solution & 1.00000 \nonumber\\
miss_wear & 1.00000 \nonumber\\
!!_so & 1.00000 \nonumber\\
!!_though & 1.00000 \nonumber\\
miss_the & 1.00000 \nonumber\\
wear_their & 1.00000 \nonumber\\
a_student & 1.00000 \nonumber\\
bid_!! & 1.00000 \nonumber\\
student_i & 1.00000 \nonumber\\
!!_: & 1.00000 \nonumber\\
very_very & 1.00000 \nonumber\\
to_miss & 1.00000 \nonumber\\
know_im & 1.00000 \nonumber\\
their_uniform & 1.00000 \nonumber\\
a_college & 1.00000 \nonumber\\
i_miss & 1.00000 \nonumber\\
when_im & 1.00000 \nonumber\\
college_student & 1.00000 \nonumber\\
uniform_!! & 1.00000 \nonumber\\
hate_wear & 1.00000 \nonumber\\
your_partner & 1.00000 \nonumber\\
dad & 1.00000 \nonumber\\
thousand_year & 1.00000 \nonumber\\
a_mile & 1.00000 \nonumber\\
it_just & 1.00000 \nonumber\\
_pos_ngram_ART_ADV_ADV & 1.00000 \nonumber\\
make_, & 1.00000 \nonumber\\
a_little & 1.00000 \nonumber\\
ponder & 1.00000 \nonumber\\
_pos_ngram_CARD_ART_NN & 1.00000 \nonumber\\
sense_. & 1.00000 \nonumber\\
to_occur & 1.00000 \nonumber\\
occur_? & 1.00000 \nonumber\\
ProductionRule_ADVP->IN,DT, & 1.00000 \nonumber\\
then_be & 1.00000 \nonumber\\
and_step & 1.00000 \nonumber\\
standard_for & 1.00000 \nonumber\\
i_look & 1.00000 \nonumber\\
lousy_person & 1.00000 \nonumber\\
and_set & 1.00000 \nonumber\\
or_sister & 1.00000 \nonumber\\
example_so & 1.00000 \nonumber\\
fatherless_" & 1.00000 \nonumber\\
have_younger & 1.00000 \nonumber\\
"_lousy & 1.00000 \nonumber\\
sister_. & 1.00000 \nonumber\\
house_especially & 1.00000 \nonumber\\
brother_or & 1.00000 \nonumber\\
"_father & 1.00000 \nonumber\\
family_can & 1.00000 \nonumber\\
ProductionRule_VP->VB,``,ADJP,'',ADVP,S, & 1.00000 \nonumber\\
will_set & 1.00000 \nonumber\\
ProductionRule_NP->DT,``,JJ,NN,'', & 1.00000 \nonumber\\
might_then & 1.00000 \nonumber\\
"_fatherless & 1.00000 \nonumber\\
the_standard & 1.00000 \nonumber\\
father_" & 1.00000 \nonumber\\
younger_brother & 1.00000 \nonumber\\
up_at & 1.00000 \nonumber\\
man_of & 1.00000 \nonumber\\
i_vote & 1.00000 \nonumber\\
she_just & 1.00000 \nonumber\\
what_happen & 1.00000 \nonumber\\
and_itll & 1.00000 \nonumber\\
!!_1 & 1.00000 \nonumber\\
fat_these & 1.00000 \nonumber\\
p.e._help & 1.00000 \nonumber\\
lame_ass & 1.00000 \nonumber\\
itll_help & 1.00000 \nonumber\\
itll & 1.00000 \nonumber\\
ass_future & 1.00000 \nonumber\\
ProductionRule_VP->VBP,ADJP,NP, & 1.00000 \nonumber\\
._p.e. & 1.00000 \nonumber\\
!!!!!_one & 1.00000 \nonumber\\
heath_be & 1.00000 \nonumber\\
future_lol & 1.00000 \nonumber\\
heath & 1.00000 \nonumber\\
_pos_ngram_V_NN_CARD & 1.00000 \nonumber\\
relize_heath & 1.00000 \nonumber\\
1_!!!!! & 1.00000 \nonumber\\
them_relize & 1.00000 \nonumber\\
these_day & 1.00000 \nonumber\\
help_!! & 1.00000 \nonumber\\
one_!!!! & 1.00000 \nonumber\\
relize & 1.00000 \nonumber\\
there_lame & 1.00000 \nonumber\\
relation & 1.00000 \nonumber\\
10 & 1.00000 \nonumber\\
your_whole & 1.00000 \nonumber\\
hit_somebody & 1.00000 \nonumber\\
a_candy & 1.00000 \nonumber\\
the_saame & 1.00000 \nonumber\\
your_favorite & 1.00000 \nonumber\\
by_get & 1.00000 \nonumber\\
then_tell & 1.00000 \nonumber\\
this_make & 1.00000 \nonumber\\
hm & 1.00000 \nonumber\\
get_something & 1.00000 \nonumber\\
you_hit & 1.00000 \nonumber\\
candy_bar & 1.00000 \nonumber\\
you_steal & 1.00000 \nonumber\\
steal_. & 1.00000 \nonumber\\
saame & 1.00000 \nonumber\\
favorite_toy & 1.00000 \nonumber\\
ProductionRule_SINV->VBZ,NP,VP, & 1.00000 \nonumber\\
steal_a & 1.00000 \nonumber\\
steal_something & 1.00000 \nonumber\\
steal_your & 1.00000 \nonumber\\
hit_, & 1.00000 \nonumber\\
get_tell & 1.00000 \nonumber\\
bar_from & 1.00000 \nonumber\\
saame_person & 1.00000 \nonumber\\
then_your & 1.00000 \nonumber\\
discipline_by & 1.00000 \nonumber\\
hit_by & 1.00000 \nonumber\\
._same & 1.00000 \nonumber\\
somebody_then & 1.00000 \nonumber\\
._hm & 1.00000 \nonumber\\
ProductionRule_S->SINV,:,S,., & 1.00000 \nonumber\\
parent_steal & 1.00000 \nonumber\\
your_parent & 1.00000 \nonumber\\
then_hit & 1.00000 \nonumber\\
thing_apply & 1.00000 \nonumber\\
something_steal & 1.00000 \nonumber\\
somebody_, & 1.00000 \nonumber\\
sense_: & 1.00000 \nonumber\\
hm_. & 1.00000 \nonumber\\
it_have & 1.00000 \nonumber\\
ProductionRule_NP->NP,PRN, & 1.00000 \nonumber\\
look_out & 1.00000 \nonumber\\
world_to & 1.00000 \nonumber\\
two_piece & 1.00000 \nonumber\\
darwinism_and & 1.00000 \nonumber\\
ProductionRule_VP->VBG,``,NP,'',PP, & 1.00000 \nonumber\\
by_pour & 1.00000 \nonumber\\
ProductionRule_VP->VBG,NP,PRT,PP, & 1.00000 \nonumber\\
"_evolution & 1.00000 \nonumber\\
pour_the & 1.00000 \nonumber\\
evolution_" & 1.00000 \nonumber\\
ProductionRule_NP->NP,CC,NP,,, & 1.00000 \nonumber\\
in_darwinism & 1.00000 \nonumber\\
"_as & 1.00000 \nonumber\\
stick_together & 1.00000 \nonumber\\
pour & 1.00000 \nonumber\\
out_because & 1.00000 \nonumber\\
ProductionRule_VP->ADVP,VBN,ADVP, & 1.00000 \nonumber\\
darwinism & 1.00000 \nonumber\\
piece_kind & 1.00000 \nonumber\\
of_stick & 1.00000 \nonumber\\
as_in & 1.00000 \nonumber\\
piece_out & 1.00000 \nonumber\\
the_puzzle & 1.00000 \nonumber\\
because_two & 1.00000 \nonumber\\
the_like & 1.00000 \nonumber\\
trade_route & 1.00000 \nonumber\\
trade_with & 1.00000 \nonumber\\
he_increase & 1.00000 \nonumber\\
to_trade & 1.00000 \nonumber\\
he_establish & 1.00000 \nonumber\\
,_boost & 1.00000 \nonumber\\
free_trade & 1.00000 \nonumber\\
malacca_as & 1.00000 \nonumber\\
route_. & 1.00000 \nonumber\\
by_use & 1.00000 \nonumber\\
route & 1.00000 \nonumber\\
thus_many & 1.00000 \nonumber\\
economy_of & 1.00000 \nonumber\\
singapore_by & 1.00000 \nonumber\\
boost_singapore & 1.00000 \nonumber\\
establish_free & 1.00000 \nonumber\\
how_bid & 1.00000 \nonumber\\
_pos_ngram_NP_CARD_V & 1.00000 \nonumber\\
a_muslim & 1.00000 \nonumber\\
best_religion & 1.00000 \nonumber\\
religion_... & 1.00000 \nonumber\\
muslim_, & 1.00000 \nonumber\\
in_christianity & 1.00000 \nonumber\\
christianity_nor & 1.00000 \nonumber\\
nor_atheism & 1.00000 \nonumber\\
ProductionRule_VP->VBP,ADVP,NP,PP, & 1.00000 \nonumber\\
_pos_ngram_ADV_NP_PP & 1.00000 \nonumber\\
boost & 1.00000 \nonumber\\
bastard & 1.00000 \nonumber\\
?_it & 1.00000 \nonumber\\
a_loan & 1.00000 \nonumber\\
endeavor_than & 1.00000 \nonumber\\
who_only & 1.00000 \nonumber\\
a_charity & 1.00000 \nonumber\\
pursuit_however & 1.00000 \nonumber\\
selfish_people & 1.00000 \nonumber\\
an_orphanage & 1.00000 \nonumber\\
for_college & 1.00000 \nonumber\\
example_there & 1.00000 \nonumber\\
charity & 1.00000 \nonumber\\
loan & 1.00000 \nonumber\\
charity_for & 1.00000 \nonumber\\
good_happen & 1.00000 \nonumber\\
some_from & 1.00000 \nonumber\\
those_selfish & 1.00000 \nonumber\\
orphanage & 1.00000 \nonumber\\
orphanage_, & 1.00000 \nonumber\\
loan_for & 1.00000 \nonumber\\
about_themselve & 1.00000 \nonumber\\
i_only & 1.00000 \nonumber\\
skin & 1.00000 \nonumber\\
sleeker & 1.00000 \nonumber\\
..._so & 1.00000 \nonumber\\
more_wrong & 1.00000 \nonumber\\
to_accept & 1.00000 \nonumber\\
wrong_because & 1.00000 \nonumber\\
also_fun & 1.00000 \nonumber\\
their_sunday & 1.00000 \nonumber\\
sunday_go & 1.00000 \nonumber\\
!!!!_hahaha & 1.00000 \nonumber\\
fun_to & 1.00000 \nonumber\\
waste_half & 1.00000 \nonumber\\
half_of & 1.00000 \nonumber\\
lawl_at & 1.00000 \nonumber\\
lawl & 1.00000 \nonumber\\
to_lawl & 1.00000 \nonumber\\
at_because & 1.00000 \nonumber\\
ProductionRule_VP->VBP,ADVP,NP,PP,PP, & 1.00000 \nonumber\\
waste_!!!! & 1.00000 \nonumber\\
hour_in & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,ADVP,RB,ADJP,SBAR, & 1.00000 \nonumber\\
in_not & 1.00000 \nonumber\\
a_classroom & 1.00000 \nonumber\\
not_comfortable & 1.00000 \nonumber\\
you_sit & 1.00000 \nonumber\\
sit_for & 1.00000 \nonumber\\
comfortable_when & 1.00000 \nonumber\\
classroom_. & 1.00000 \nonumber\\
_pos_ngram_PR_PP_CARD & 1.00000 \nonumber\\
force_that & 1.00000 \nonumber\\
and_win & 1.00000 \nonumber\\
win_by & 1.00000 \nonumber\\
percentage_be & 1.00000 \nonumber\\
be_down & 1.00000 \nonumber\\
not_vote & 1.00000 \nonumber\\
than_of & 1.00000 \nonumber\\
of_force & 1.00000 \nonumber\\
vote_. & 1.00000 \nonumber\\
population_or & 1.00000 \nonumber\\
win_you & 1.00000 \nonumber\\
do_vote & 1.00000 \nonumber\\
yourself_to & 1.00000 \nonumber\\
make_as & 1.00000 \nonumber\\
vote_they & 1.00000 \nonumber\\
difference_and & 1.00000 \nonumber\\
or_percentage & 1.00000 \nonumber\\
whole_the & 1.00000 \nonumber\\
same_view & 1.00000 \nonumber\\
bigger_than & 1.00000 \nonumber\\
other_with & 1.00000 \nonumber\\
by_look & 1.00000 \nonumber\\
whole_group & 1.00000 \nonumber\\
be_bigger & 1.00000 \nonumber\\
ProductionRule_S->S,,,S, & 1.00000 \nonumber\\
previous & 1.00000 \nonumber\\
although_we & 1.00000 \nonumber\\
be_new & 1.00000 \nonumber\\
be_obvious & 1.00000 \nonumber\\
two_men/women & 1.00000 \nonumber\\
two_human & 1.00000 \nonumber\\
new_idea & 1.00000 \nonumber\\
men/women & 1.00000 \nonumber\\
men/women_together & 1.00000 \nonumber\\
not_seem & 1.00000 \nonumber\\
bible_but & 1.00000 \nonumber\\
this_so & 1.00000 \nonumber\\
reproduce_and & 1.00000 \nonumber\\
take_from & 1.00000 \nonumber\\
seem_ironic & 1.00000 \nonumber\\
together_be & 1.00000 \nonumber\\
seem_natural & 1.00000 \nonumber\\
approve_of & 1.00000 \nonumber\\
ironic_in & 1.00000 \nonumber\\
obvious_that & 1.00000 \nonumber\\
together_do & 1.00000 \nonumber\\
technology_be & 1.00000 \nonumber\\
this_nation & 1.00000 \nonumber\\
unite_kingdom & 1.00000 \nonumber\\
not_yet & 1.00000 \nonumber\\
%_sure & 1.00000 \nonumber\\
technology_like & 1.00000 \nonumber\\
sophisticate & 1.00000 \nonumber\\
if_because & 1.00000 \nonumber\\
essential_invention & 1.00000 \nonumber\\
ever_create & 1.00000 \nonumber\\
lead_us & 1.00000 \nonumber\\
sustain_the & 1.00000 \nonumber\\
future_that & 1.00000 \nonumber\\
and_essential & 1.00000 \nonumber\\
invention_ever & 1.00000 \nonumber\\
to_sustain & 1.00000 \nonumber\\
russium & 1.00000 \nonumber\\
that_full & 1.00000 \nonumber\\
russium_, & 1.00000 \nonumber\\
potential_and & 1.00000 \nonumber\\
progressive_, & 1.00000 \nonumber\\
progressive & 1.00000 \nonumber\\
enought & 1.00000 \nonumber\\
sure_if & 1.00000 \nonumber\\
enought_potential & 1.00000 \nonumber\\
sophisticate_and & 1.00000 \nonumber\\
of_technology & 1.00000 \nonumber\\
indium_could & 1.00000 \nonumber\\
literate & 1.00000 \nonumber\\
yet_that & 1.00000 \nonumber\\
could_lead & 1.00000 \nonumber\\
,_russium & 1.00000 \nonumber\\
country_who & 1.00000 \nonumber\\
yet_enought & 1.00000 \nonumber\\
could_fail & 1.00000 \nonumber\\
nation_itself & 1.00000 \nonumber\\
fact_technology & 1.00000 \nonumber\\
the_usa & 1.00000 \nonumber\\
literate_, & 1.00000 \nonumber\\
powerful_than & 1.00000 \nonumber\\
most_sophisticate & 1.00000 \nonumber\\
ProductionRule_VP->VBP,RB,ADVP,ADJP, & 1.00000 \nonumber\\
ProductionRule_ADJP->NP,JJ,SBAR, & 1.00000 \nonumber\\
still_other & 1.00000 \nonumber\\
big_if & 1.00000 \nonumber\\
more_progressive & 1.00000 \nonumber\\
ProductionRule_S->NP,VP,SBAR,., & 1.00000 \nonumber\\
than_indium & 1.00000 \nonumber\\
more_literate & 1.00000 \nonumber\\
know_maybe & 1.00000 \nonumber\\
,_unite & 1.00000 \nonumber\\
itself_could & 1.00000 \nonumber\\
indium_, & 1.00000 \nonumber\\
technology & 1.00000 \nonumber\\
yet_100 & 1.00000 \nonumber\\
kingdom_, & 1.00000 \nonumber\\
kingdom & 1.00000 \nonumber\\
,_japan & 1.00000 \nonumber\\
country_, & 1.00000 \nonumber\\
morality_, & 1.00000 \nonumber\\
violence_, & 1.00000 \nonumber\\
do_need & 1.00000 \nonumber\\
get_their & 1.00000 \nonumber\\
ProductionRule_NP->NP,PP,NN, & 1.00000 \nonumber\\
firefox_of & 1.00000 \nonumber\\
why_school & 1.00000 \nonumber\\
bigger_picture & 1.00000 \nonumber\\
picture_) & 1.00000 \nonumber\\
not_purely & 1.00000 \nonumber\\
toward_spank & 1.00000 \nonumber\\
unruliest_there & 1.00000 \nonumber\\
near_as & 1.00000 \nonumber\\
the_unruliest & 1.00000 \nonumber\\
'_kid & 1.00000 \nonumber\\
resentment_toward & 1.00000 \nonumber\\
ProductionRule_SBAR->SBAR,:,PRN, & 1.00000 \nonumber\\
much_resentment & 1.00000 \nonumber\\
year_with & 1.00000 \nonumber\\
today_' & 1.00000 \nonumber\\
and_today & 1.00000 \nonumber\\
the_bigger & 1.00000 \nonumber\\
a_trend & 1.00000 \nonumber\\
ProductionRule_VP->VBN,PP,PP,SBAR, & 1.00000 \nonumber\\
do_admit & 1.00000 \nonumber\\
trend_... & 1.00000 \nonumber\\
small_part & 1.00000 \nonumber\\
cause_but & 1.00000 \nonumber\\
not_near & 1.00000 \nonumber\\
..._there & 1.00000 \nonumber\\
unruliest & 1.00000 \nonumber\\
purely_spank & 1.00000 \nonumber\\
..._( & 1.00000 \nonumber\\
raise_for & 1.00000 \nonumber\\
one_at & 1.00000 \nonumber\\
everyone_, & 1.00000 \nonumber\\
be_fat & 1.00000 \nonumber\\
who_get & 1.00000 \nonumber\\
dichotomy & 1.00000 \nonumber\\
false_dichotomy & 1.00000 \nonumber\\
language_and & 1.00000 \nonumber\\
and_answer & 1.00000 \nonumber\\
important_that & 1.00000 \nonumber\\
young_man & 1.00000 \nonumber\\
question_you & 1.00000 \nonumber\\
young_boy & 1.00000 \nonumber\\
successful_in & 1.00000 \nonumber\\
hope_and & 1.00000 \nonumber\\
there_life & 1.00000 \nonumber\\
grow_hope & 1.00000 \nonumber\\
answer_question & 1.00000 \nonumber\\
in_there & 1.00000 \nonumber\\
support_you & 1.00000 \nonumber\\
man_it & 1.00000 \nonumber\\
be_need & 1.00000 \nonumber\\
boy_you & 1.00000 \nonumber\\
who_life & 1.00000 \nonumber\\
push_you & 1.00000 \nonumber\\
finger & 1.00000 \nonumber\\
a_learn & 1.00000 \nonumber\\
read_a & 1.00000 \nonumber\\
this_for & 1.00000 \nonumber\\
be_rule & 1.00000 \nonumber\\
spend_all & 1.00000 \nonumber\\
and_time & 1.00000 \nonumber\\
perspective_of & 1.00000 \nonumber\\
there_money & 1.00000 \nonumber\\
friend_happy & 1.00000 \nonumber\\
would_spend & 1.00000 \nonumber\\
the_perspective & 1.00000 \nonumber\\
than_themselve & 1.00000 \nonumber\\
"_for & 1.00000 \nonumber\\
nation_do & 1.00000 \nonumber\\
also_get & 1.00000 \nonumber\\
week_, & 1.00000 \nonumber\\
at_kid & 1.00000 \nonumber\\
very_bid & 1.00000 \nonumber\\
father_grow & 1.00000 \nonumber\\
not_really & 1.00000 \nonumber\\
by_talk & 1.00000 \nonumber\\
im_guess & 1.00000 \nonumber\\
speech_) & 1.00000 \nonumber\\
(_by & 1.00000 \nonumber\\
._monkey & 1.00000 \nonumber\\
guess_you & 1.00000 \nonumber\\
branch_on & 1.00000 \nonumber\\
ProductionRule_ADVP->RB,SBAR, & 1.00000 \nonumber\\
from_exist & 1.00000 \nonumber\\
a_dead & 1.00000 \nonumber\\
a_branch & 1.00000 \nonumber\\
of_speech & 1.00000 \nonumber\\
monkey_have & 1.00000 \nonumber\\
branch & 1.00000 \nonumber\\
monkey_from & 1.00000 \nonumber\\
talk_im & 1.00000 \nonumber\\
talk_monkey & 1.00000 \nonumber\\
dead_end & 1.00000 \nonumber\\
monkey_that & 1.00000 \nonumber\\
n't_evolve & 1.00000 \nonumber\\
mean_speech & 1.00000 \nonumber\\
yes_if & 1.00000 \nonumber\\
we_on & 1.00000 \nonumber\\
)_because & 1.00000 \nonumber\\
ProductionRule_S->``,ADVP,NP,VP,.,'', & 1.00000 \nonumber\\
descend & 1.00000 \nonumber\\
speech_. & 1.00000 \nonumber\\
descend_from & 1.00000 \nonumber\\
stop_monkey & 1.00000 \nonumber\\
herring_. & 1.00000 \nonumber\\
be_descend & 1.00000 \nonumber\\
have_evolve & 1.00000 \nonumber\\
tree_of & 1.00000 \nonumber\\
have_talk & 1.00000 \nonumber\\
hand_have & 1.00000 \nonumber\\
talk_. & 1.00000 \nonumber\\
talk_( & 1.00000 \nonumber\\
friend_or & 1.00000 \nonumber\\
"_so & 1.00000 \nonumber\\
that_too & 1.00000 \nonumber\\
have_hear & 1.00000 \nonumber\\
hear_, & 1.00000 \nonumber\\
have_go & 1.00000 \nonumber\\
thing_ie & 1.00000 \nonumber\\
firefox_win & 1.00000 \nonumber\\
it_pre-install & 1.00000 \nonumber\\
speed_to & 1.00000 \nonumber\\
add-on_, & 1.00000 \nonumber\\
to_add-on & 1.00000 \nonumber\\
window_have & 1.00000 \nonumber\\
that_window & 1.00000 \nonumber\\
._everything & 1.00000 \nonumber\\
argue_? & 1.00000 \nonumber\\
from_speed & 1.00000 \nonumber\\
pre-install_, & 1.00000 \nonumber\\
pre-install & 1.00000 \nonumber\\
everything_from & 1.00000 \nonumber\\
ProductionRule_SBAR->RB,RB,IN,S, & 1.00000 \nonumber\\
pose_. & 1.00000 \nonumber\\
who_choose & 1.00000 \nonumber\\
behind_your & 1.00000 \nonumber\\
'_only & 1.00000 \nonumber\\
partner_' & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,RB,ADJP,,,SBAR, & 1.00000 \nonumber\\
it_behind & 1.00000 \nonumber\\
pose & 1.00000 \nonumber\\
to_pose & 1.00000 \nonumber\\
monkey_? & 1.00000 \nonumber\\
spank_that & 1.00000 \nonumber\\
set_a & 1.00000 \nonumber\\
step_up & 1.00000 \nonumber\\
idiotic_. & 1.00000 \nonumber\\
be_idiotic & 1.00000 \nonumber\\
ProductionRule_ADJP->JJ,JJS, & 1.00000 \nonumber\\
me_for & 1.00000 \nonumber\\
something_. & 1.00000 \nonumber\\
not_just & 1.00000 \nonumber\\
dig & 1.00000 \nonumber\\
birth_certificate & 1.00000 \nonumber\\
certificate_. & 1.00000 \nonumber\\
certificate & 1.00000 \nonumber\\
because_honestly & 1.00000 \nonumber\\
school_will & 1.00000 \nonumber\\
billionaire & 1.00000 \nonumber\\
billionaire_or & 1.00000 \nonumber\\
bastard_legally & 1.00000 \nonumber\\
should_grow & 1.00000 \nonumber\\
in_touch & 1.00000 \nonumber\\
ask_about & 1.00000 \nonumber\\
will_ask & 1.00000 \nonumber\\
mess_with & 1.00000 \nonumber\\
even_on & 1.00000 \nonumber\\
legally_because & 1.00000 \nonumber\\
whether_he & 1.00000 \nonumber\\
mother_anymore & 1.00000 \nonumber\\
lousy_or & 1.00000 \nonumber\\
dad_and & 1.00000 \nonumber\\
a_bastard & 1.00000 \nonumber\\
my_birth & 1.00000 \nonumber\\
a_billionaire & 1.00000 \nonumber\\
it_mess & 1.00000 \nonumber\\
_pos_ngram_PUNC_PR_PUNC & 1.00000 \nonumber\\
touch_with & 1.00000 \nonumber\\
'd_choose & 1.00000 \nonumber\\
n't_with & 1.00000 \nonumber\\
kid_in & 1.00000 \nonumber\\
be_write & 1.00000 \nonumber\\
ie_have & 1.00000 \nonumber\\
,_boo & 1.00000 \nonumber\\
ProductionRule_RRC->ADVP,ADJP, & 1.00000 \nonumber\\
actually_really & 1.00000 \nonumber\\
they_actually & 1.00000 \nonumber\\
stupid_indium & 1.00000 \nonumber\\
indium_they & 1.00000 \nonumber\\
indium_boo & 1.00000 \nonumber\\
boo_indium & 1.00000 \nonumber\\
boo & 1.00000 \nonumber\\
boo_! & 1.00000 \nonumber\\
_pos_ngram_ART_CARD_PR & 1.00000 \nonumber\\
like_when & 1.00000 \nonumber\\
unacceptable_. & 1.00000 \nonumber\\
woman_as & 1.00000 \nonumber\\
man_ca & 1.00000 \nonumber\\
as_gay & 1.00000 \nonumber\\
anybody_should & 1.00000 \nonumber\\
his_feeling & 1.00000 \nonumber\\
acceptable_or & 1.00000 \nonumber\\
say_most & 1.00000 \nonumber\\
unacceptable & 1.00000 \nonumber\\
come_we & 1.00000 \nonumber\\
other_secuality & 1.00000 \nonumber\\
sexuality_i & 1.00000 \nonumber\\
one_they & 1.00000 \nonumber\\
sexuality & 1.00000 \nonumber\\
feeling_to & 1.00000 \nonumber\\
love_so & 1.00000 \nonumber\\
of_britain & 1.00000 \nonumber\\
however_a & 1.00000 \nonumber\\
like_!! & 1.00000 \nonumber\\
marriage_acceptable & 1.00000 \nonumber\\
secuality_however & 1.00000 \nonumber\\
gay_sexuality & 1.00000 \nonumber\\
wrong_however & 1.00000 \nonumber\\
express_his & 1.00000 \nonumber\\
secuality & 1.00000 \nonumber\\
express_there & 1.00000 \nonumber\\
britain_would & 1.00000 \nonumber\\
or_unacceptable & 1.00000 \nonumber\\
myself & 1.00000 \nonumber\\
school_then & 1.00000 \nonumber\\
decision_? & 1.00000 \nonumber\\
_pos_ngram_PR_ART_PUNC & 1.00000 \nonumber\\
a_choice & 1.00000 \nonumber\\
project & 1.00000 \nonumber\\
project_. & 1.00000 \nonumber\\
the_creationist & 1.00000 \nonumber\\
that_? & 1.00000 \nonumber\\
daughter & 1.00000 \nonumber\\
feature_. & 1.00000 \nonumber\\
prefer_to & 1.00000 \nonumber\\
more_flexible & 1.00000 \nonumber\\
more_lazy & 1.00000 \nonumber\\
teacher_should & 1.00000 \nonumber\\
._teacher & 1.00000 \nonumber\\
strengthen_their & 1.00000 \nonumber\\
mussel_and & 1.00000 \nonumber\\
exercise_so & 1.00000 \nonumber\\
mussel & 1.00000 \nonumber\\
their_mussel & 1.00000 \nonumber\\
get_thinner & 1.00000 \nonumber\\
can_strengthen & 1.00000 \nonumber\\
flexible_instead & 1.00000 \nonumber\\
obvious_. & 1.00000 \nonumber\\
thinner & 1.00000 \nonumber\\
thinner_and & 1.00000 \nonumber\\
lazy_so & 1.00000 \nonumber\\
answer_be & 1.00000 \nonumber\\
should_let & 1.00000 \nonumber\\
of_fatter & 1.00000 \nonumber\\
so_obvious & 1.00000 \nonumber\\
everyone_exercise & 1.00000 \nonumber\\
fatter_and & 1.00000 \nonumber\\
let_everyone & 1.00000 \nonumber\\
bully_as & 1.00000 \nonumber\\
,_, & 1.00000 \nonumber\\
face_and & 1.00000 \nonumber\\
that_say & 1.00000 \nonumber\\
)_which & 1.00000 \nonumber\\
about_wear & 1.00000 \nonumber\\
serious_problem & 1.00000 \nonumber\\
misunderstanding_with & 1.00000 \nonumber\\
make_trouble & 1.00000 \nonumber\\
misunderstanding & 1.00000 \nonumber\\
_pos_ngram_NN_ADJ_CARD & 1.00000 \nonumber\\
within_student & 1.00000 \nonumber\\
people_age & 1.00000 \nonumber\\
their_freedom & 1.00000 \nonumber\\
problem_follow & 1.00000 \nonumber\\
relation_. & 1.00000 \nonumber\\
age_16-18 & 1.00000 \nonumber\\
sense_, & 1.00000 \nonumber\\
very_serious & 1.00000 \nonumber\\
become_adult & 1.00000 \nonumber\\
become_very & 1.00000 \nonumber\\
behavior_- & 1.00000 \nonumber\\
mention_about & 1.00000 \nonumber\\
16-18 & 1.00000 \nonumber\\
teacher_relation & 1.00000 \nonumber\\
school_student & 1.00000 \nonumber\\
by_high & 1.00000 \nonumber\\
by_misunderstanding & 1.00000 \nonumber\\
limit_and & 1.00000 \nonumber\\
like_parent & 1.00000 \nonumber\\
age_when & 1.00000 \nonumber\\
limit_their & 1.00000 \nonumber\\
freedom_can & 1.00000 \nonumber\\
opposite_, & 1.00000 \nonumber\\
when_student & 1.00000 \nonumber\\
the_control & 1.00000 \nonumber\\
any_limit & 1.00000 \nonumber\\
trouble_within & 1.00000 \nonumber\\
uniform_by & 1.00000 \nonumber\\
the_childhood & 1.00000 \nonumber\\
16-18_do & 1.00000 \nonumber\\
childhood_, & 1.00000 \nonumber\\
sometime_limit & 1.00000 \nonumber\\
-_it & 1.00000 \nonumber\\
control_person & 1.00000 \nonumber\\
gay_should & 1.00000 \nonumber\\
but_since & 1.00000 \nonumber\\
help_them & 1.00000 \nonumber\\
for_what & 1.00000 \nonumber\\
i_hate & 1.00000 \nonumber\\
of_clothe & 1.00000 \nonumber\\
dream & 1.00000 \nonumber\\
else_in & 1.00000 \nonumber\\
believe_i & 1.00000 \nonumber\\
_pos_ngram_O_O_ADV & 1.00000 \nonumber\\
be_away & 1.00000 \nonumber\\
singapore_while & 1.00000 \nonumber\\
legally & 1.00000 \nonumber\\
_pos_ngram_ADV_O_PP & 1.00000 \nonumber\\
?_if & 1.00000 \nonumber\\
comfortable & 1.00000 \nonumber\\
future.so_just & 1.00000 \nonumber\\
a_lie & 1.00000 \nonumber\\
future.so & 1.00000 \nonumber\\
clean_and & 1.00000 \nonumber\\
arrest_, & 1.00000 \nonumber\\
a_murderer?he & 1.00000 \nonumber\\
me_do & 1.00000 \nonumber\\
the_future.so & 1.00000 \nonumber\\
innocent_. & 1.00000 \nonumber\\
and_innocent & 1.00000 \nonumber\\
can_i & 1.00000 \nonumber\\
also_how & 1.00000 \nonumber\\
feel_guilty & 1.00000 \nonumber\\
maybe_if & 1.00000 \nonumber\\
definately_i & 1.00000 \nonumber\\
just_by & 1.00000 \nonumber\\
murderer?he_can & 1.00000 \nonumber\\
sin_. & 1.00000 \nonumber\\
murderer?he & 1.00000 \nonumber\\
try_not & 1.00000 \nonumber\\
him_clean & 1.00000 \nonumber\\
i_trust & 1.00000 \nonumber\\
yes_definately & 1.00000 \nonumber\\
maybe_can & 1.00000 \nonumber\\
confide_to & 1.00000 \nonumber\\
get_arrest & 1.00000 \nonumber\\
guilty_for & 1.00000 \nonumber\\
repeat_it & 1.00000 \nonumber\\
by_confide & 1.00000 \nonumber\\
police_because & 1.00000 \nonumber\\
trust_a & 1.00000 \nonumber\\
through_creation & 1.00000 \nonumber\\
it_himself & 1.00000 \nonumber\\
answer_: & 1.00000 \nonumber\\
?_final & 1.00000 \nonumber\\
or_evolution & 1.00000 \nonumber\\
n't_cause & 1.00000 \nonumber\\
both_? & 1.00000 \nonumber\\
_pos_ngram_PR_PR_PUNC & 1.00000 \nonumber\\
not_both & 1.00000 \nonumber\\
bang_or & 1.00000 \nonumber\\
n't_god & 1.00000 \nonumber\\
final & 1.00000 \nonumber\\
himself_? & 1.00000 \nonumber\\
ProductionRule_WHADVP->WRB,RB, & 1.00000 \nonumber\\
evolution_through & 1.00000 \nonumber\\
final_answer & 1.00000 \nonumber\\
ProductionRule_FRAG->WHADVP,NP,., & 1.00000 \nonumber\\
such_thing & 1.00000 \nonumber\\
no_such & 1.00000 \nonumber\\
conceive & 1.00000 \nonumber\\
invite & 1.00000 \nonumber\\
)_be & 1.00000 \nonumber\\
their_to & 1.00000 \nonumber\\
somebody_their & 1.00000 \nonumber\\
ProductionRule_VP->VBG,PRT,PP, & 1.00000 \nonumber\\
support_your & 1.00000 \nonumber\\
dad_to & 1.00000 \nonumber\\
need_dad & 1.00000 \nonumber\\
father_no & 1.00000 \nonumber\\
force_us & 1.00000 \nonumber\\
w3c & 1.00000 \nonumber\\
to_force & 1.00000 \nonumber\\
more_respectful & 1.00000 \nonumber\\
monopoly_. & 1.00000 \nonumber\\
own_standard & 1.00000 \nonumber\\
monopoly & 1.00000 \nonumber\\
internet_standard & 1.00000 \nonumber\\
respectful_of & 1.00000 \nonumber\\
suck_by & 1.00000 \nonumber\\
standard_to & 1.00000 \nonumber\\
their_monopoly & 1.00000 \nonumber\\
keep_their & 1.00000 \nonumber\\
of_w3c & 1.00000 \nonumber\\
soft_suck & 1.00000 \nonumber\\
by_try & 1.00000 \nonumber\\
w3c_internet & 1.00000 \nonumber\\
standard_while & 1.00000 \nonumber\\
while_soft & 1.00000 \nonumber\\
though_, & 1.00000 \nonumber\\
means_take & 1.00000 \nonumber\\
this_horrible & 1.00000 \nonumber\\
secret_to & 1.00000 \nonumber\\
my_love & 1.00000 \nonumber\\
whatever_whenever & 1.00000 \nonumber\\
whenever_to & 1.00000 \nonumber\\
survival_mechanism & 1.00000 \nonumber\\
fabricate_with & 1.00000 \nonumber\\
be_fabricate & 1.00000 \nonumber\\
tell_be & 1.00000 \nonumber\\
fabricate & 1.00000 \nonumber\\
the_grave & 1.00000 \nonumber\\
a_survival & 1.00000 \nonumber\\
everything_in & 1.00000 \nonumber\\
my_power & 1.00000 \nonumber\\
grave_. & 1.00000 \nonumber\\
mechanism & 1.00000 \nonumber\\
being_, & 1.00000 \nonumber\\
horrible_secret & 1.00000 \nonumber\\
mechanism_that & 1.00000 \nonumber\\
that_tell & 1.00000 \nonumber\\
take_this & 1.00000 \nonumber\\
protect_my & 1.00000 \nonumber\\
and_play & 1.00000 \nonumber\\
make_more & 1.00000 \nonumber\\
consequence & 1.00000 \nonumber\\
moreover & 1.00000 \nonumber\\
your_help & 1.00000 \nonumber\\
people_choose & 1.00000 \nonumber\\
will_benefit & 1.00000 \nonumber\\
if_every & 1.00000 \nonumber\\
benefit_from & 1.00000 \nonumber\\
then_every & 1.00000 \nonumber\\
person_decide & 1.00000 \nonumber\\
from_it & 1.00000 \nonumber\\
person_would & 1.00000 \nonumber\\
effect_of & 1.00000 \nonumber\\
would_see & 1.00000 \nonumber\\
ProductionRule_VP->VBP,PRT, & 1.00000 \nonumber\\
would_tell & 1.00000 \nonumber\\
if_one & 1.00000 \nonumber\\
her_life & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,NP,,,SBAR, & 1.00000 \nonumber\\
long_period & 1.00000 \nonumber\\
believe_personal & 1.00000 \nonumber\\
nice_and & 1.00000 \nonumber\\
that_uniform & 1.00000 \nonumber\\
a_more & 1.00000 \nonumber\\
time_for & 1.00000 \nonumber\\
_pos_ngram_ADJ_O_ADV & 1.00000 \nonumber\\
crime_, & 1.00000 \nonumber\\
mutation & 1.00000 \nonumber\\
of_human & 1.00000 \nonumber\\
_pos_ngram_NN_CARD_PR & 1.00000 \nonumber\\
be_next & 1.00000 \nonumber\\
out_from & 1.00000 \nonumber\\
_pos_ngram_PP_PUNC_CONJ & 1.00000 \nonumber\\
ProductionRule_NP->FW,FW,FW,FW, & 1.00000 \nonumber\\
would_most & 1.00000 \nonumber\\
social_status & 1.00000 \nonumber\\
social & 1.00000 \nonumber\\
_pos_ngram_PP_O_CARD & 1.00000 \nonumber\\
of_get & 1.00000 \nonumber\\
do_? & 1.00000 \nonumber\\
support_this & 1.00000 \nonumber\\
all_start & 1.00000 \nonumber\\
truly_believe & 1.00000 \nonumber\\
an_abomination & 1.00000 \nonumber\\
._secular & 1.00000 \nonumber\\
all_man & 1.00000 \nonumber\\
._leviticus & 1.00000 \nonumber\\
freedom_. & 1.00000 \nonumber\\
secular_law & 1.00000 \nonumber\\
thereof & 1.00000 \nonumber\\
both_commit & 1.00000 \nonumber\\
with_mankind & 1.00000 \nonumber\\
infect & 1.00000 \nonumber\\
unite_if & 1.00000 \nonumber\\
of_freedom & 1.00000 \nonumber\\
a_love & 1.00000 \nonumber\\
in_place & 1.00000 \nonumber\\
,_their & 1.00000 \nonumber\\
infect_this & 1.00000 \nonumber\\
only_law & 1.00000 \nonumber\\
or_lack & 1.00000 \nonumber\\
over_another & 1.00000 \nonumber\\
if_law & 1.00000 \nonumber\\
abomination & 1.00000 \nonumber\\
abomination_, & 1.00000 \nonumber\\
blood_be & 1.00000 \nonumber\\
only_remain & 1.00000 \nonumber\\
commit_an & 1.00000 \nonumber\\
the_religious & 1.00000 \nonumber\\
create_with & 1.00000 \nonumber\\
thereof_, & 1.00000 \nonumber\\
leviticus & 1.00000 \nonumber\\
leviticus_20:13 & 1.00000 \nonumber\\
lie_with & 1.00000 \nonumber\\
law_, & 1.00000 \nonumber\\
love_god & 1.00000 \nonumber\\
lack_thereof & 1.00000 \nonumber\\
man_lie & 1.00000 \nonumber\\
mankind_as & 1.00000 \nonumber\\
marriage_ban & 1.00000 \nonumber\\
womankind & 1.00000 \nonumber\\
womankind_, & 1.00000 \nonumber\\
they_shall & 1.00000 \nonumber\\
their_blood & 1.00000 \nonumber\\
with_womankind & 1.00000 \nonumber\\
the_bane & 1.00000 \nonumber\\
place_because & 1.00000 \nonumber\\
america_can & 1.00000 \nonumber\\
that_favor & 1.00000 \nonumber\\
be_both & 1.00000 \nonumber\\
put_to & 1.00000 \nonumber\\
20:13 & 1.00000 \nonumber\\
right_that & 1.00000 \nonumber\\
be_infect & 1.00000 \nonumber\\
religious_right & 1.00000 \nonumber\\
favor_one & 1.00000 \nonumber\\
remain_unite & 1.00000 \nonumber\\
20:13_: & 1.00000 \nonumber\\
bane_of & 1.00000 \nonumber\\
ban_, & 1.00000 \nonumber\\
bane & 1.00000 \nonumber\\
that_seem & 1.00000 \nonumber\\
,_eh & 1.00000 \nonumber\\
want_that & 1.00000 \nonumber\\
finally_realize & 1.00000 \nonumber\\
create_sierious & 1.00000 \nonumber\\
issue_to & 1.00000 \nonumber\\
the_envirnment & 1.00000 \nonumber\\
human_maybe & 1.00000 \nonumber\\
envirnment_. & 1.00000 \nonumber\\
that_plastic & 1.00000 \nonumber\\
hurt_us & 1.00000 \nonumber\\
people_finally & 1.00000 \nonumber\\
sierious_issue & 1.00000 \nonumber\\
maybe_they & 1.00000 \nonumber\\
to_as & 1.00000 \nonumber\\
sierious & 1.00000 \nonumber\\
turn_hurt & 1.00000 \nonumber\\
plastic_after & 1.00000 \nonumber\\
envirnment & 1.00000 \nonumber\\
_pos_ngram_O_ADV_V & 1.00000 \nonumber\\
self_and & 1.00000 \nonumber\\
_pos_ngram_NP_O_O & 1.00000 \nonumber\\
best_of & 1.00000 \nonumber\\
but_that & 1.00000 \nonumber\\
one_should & 1.00000 \nonumber\\
you_read & 1.00000 \nonumber\\
that_by & 1.00000 \nonumber\\
bacterium & 1.00000 \nonumber\\
be_give & 1.00000 \nonumber\\
_pos_ngram_NN_ART_ART & 1.00000 \nonumber\\
challenge & 1.00000 \nonumber\\
_pos_ngram_PR_ADJ_V & 1.00000 \nonumber\\
_pos_ngram_O_NP_V & 1.00000 \nonumber\\
you_use & 1.00000 \nonumber\\
other_to & 1.00000 \nonumber\\
of_america & 1.00000 \nonumber\\
i_in & 1.00000 \nonumber\\
it_seem & 1.00000 \nonumber\\
world_be & 1.00000 \nonumber\\
ProductionRule_NP->NP,POS, & 1.00000 \nonumber\\
beter & 1.00000 \nonumber\\
watch_t.v & 1.00000 \nonumber\\
its_common & 1.00000 \nonumber\\
liv_wdout & 1.00000 \nonumber\\
ix & 1.00000 \nonumber\\
bookxx_.... & 1.00000 \nonumber\\
bookxx & 1.00000 \nonumber\\
...._t.v & 1.00000 \nonumber\\
...._evrybdy & 1.00000 \nonumber\\
all_... & 1.00000 \nonumber\\
than_bookxx & 1.00000 \nonumber\\
beter_than & 1.00000 \nonumber\\
so_..... & 1.00000 \nonumber\\
ix_beter & 1.00000 \nonumber\\
common_to & 1.00000 \nonumber\\
vot_for & 1.00000 \nonumber\\
wdout_t.v. & 1.00000 \nonumber\\
evrybdy & 1.00000 \nonumber\\
vot & 1.00000 \nonumber\\
t.v & 1.00000 \nonumber\\
nowadayz_no & 1.00000 \nonumber\\
t.v._... & 1.00000 \nonumber\\
can_liv & 1.00000 \nonumber\\
t.v_ix & 1.00000 \nonumber\\
liv & 1.00000 \nonumber\\
for_t.v. & 1.00000 \nonumber\\
t.v._. & 1.00000 \nonumber\\
t.v_to & 1.00000 \nonumber\\
evrybdy_vot & 1.00000 \nonumber\\
nowadayz & 1.00000 \nonumber\\
wdout & 1.00000 \nonumber\\
creation & 1.00000 \nonumber\\
one_religion & 1.00000 \nonumber\\
the_cost & 1.00000 \nonumber\\
the_lord & 1.00000 \nonumber\\
the_womb & 1.00000 \nonumber\\
singapore_than & 1.00000 \nonumber\\
crime_that & 1.00000 \nonumber\\
little_thing & 1.00000 \nonumber\\
dutch_attack & 1.00000 \nonumber\\
attract_trader & 1.00000 \nonumber\\
trader_to & 1.00000 \nonumber\\
and_attract & 1.00000 \nonumber\\
attack_and & 1.00000 \nonumber\\
farquar_protect & 1.00000 \nonumber\\
protect_singapore & 1.00000 \nonumber\\
_pos_ngram_CONJ_ADJ_O & 1.00000 \nonumber\\
self_in & 1.00000 \nonumber\\
window_. & 1.00000 \nonumber\\
can_begin & 1.00000 \nonumber\\
lame & 1.00000 \nonumber\\
marriage_and & 1.00000 \nonumber\\
make_the & 1.00000 \nonumber\\
choose_personal & 1.00000 \nonumber\\
aspect & 1.00000 \nonumber\\
_pos_ngram_O_PP_PP & 1.00000 \nonumber\\
end_. & 1.00000 \nonumber\\
tab_, & 1.00000 \nonumber\\
rock & 1.00000 \nonumber\\
wont_do & 1.00000 \nonumber\\
argue_that & 1.00000 \nonumber\\
policy & 1.00000 \nonumber\\
will_get & 1.00000 \nonumber\\
fake & 1.00000 \nonumber\\
to_put & 1.00000 \nonumber\\
where_they & 1.00000 \nonumber\\
aspect_of & 1.00000 \nonumber\\
other_law & 1.00000 \nonumber\\
year_to & 1.00000 \nonumber\\
word_be & 1.00000 \nonumber\\
from_dutch & 1.00000 \nonumber\\
ProductionRule_NP->FW,FW,NN, & 1.00000 \nonumber\\
that_if & 1.00000 \nonumber\\
say_. & 1.00000 \nonumber\\
the_tree & 1.00000 \nonumber\\
alter & 1.00000 \nonumber\\
fault_. & 1.00000 \nonumber\\
them_with & 1.00000 \nonumber\\
a_friend & 1.00000 \nonumber\\
with_get & 1.00000 \nonumber\\
awesome_, & 1.00000 \nonumber\\
survive_life & 1.00000 \nonumber\\
rather_help & 1.00000 \nonumber\\
thing_can & 1.00000 \nonumber\\
can_impact & 1.00000 \nonumber\\
impact_someone & 1.00000 \nonumber\\
their_need & 1.00000 \nonumber\\
can_. & 1.00000 \nonumber\\
the_ability & 1.00000 \nonumber\\
both_would & 1.00000 \nonumber\\
choose_i & 1.00000 \nonumber\\
to_feed & 1.00000 \nonumber\\
all_student & 1.00000 \nonumber\\
child_will & 1.00000 \nonumber\\
nearly & 1.00000 \nonumber\\
dirty_, & 1.00000 \nonumber\\
five_test & 1.00000 \nonumber\\
be_dirty & 1.00000 \nonumber\\
recycle_, & 1.00000 \nonumber\\
._nearly & 1.00000 \nonumber\\
usually_tap & 1.00000 \nonumber\\
with_leaf & 1.00000 \nonumber\\
decompose_. & 1.00000 \nonumber\\
almost_never & 1.00000 \nonumber\\
our_environment & 1.00000 \nonumber\\
take_700 & 1.00000 \nonumber\\
dirty & 1.00000 \nonumber\\
consumption_of & 1.00000 \nonumber\\
allow_anywhere & 1.00000 \nonumber\\
be_usually & 1.00000 \nonumber\\
five & 1.00000 \nonumber\\
test_water & 1.00000 \nonumber\\
to_pollution & 1.00000 \nonumber\\
some_water & 1.00000 \nonumber\\
regulate_. & 1.00000 \nonumber\\
do_feel & 1.00000 \nonumber\\
,_moss & 1.00000 \nonumber\\
never_recycle & 1.00000 \nonumber\\
chemical_after & 1.00000 \nonumber\\
nearly_one & 1.00000 \nonumber\\
moss_, & 1.00000 \nonumber\\
leak_chemical & 1.00000 \nonumber\\
pollution_of & 1.00000 \nonumber\\
bacterium_anyway & 1.00000 \nonumber\\
bottle_have & 1.00000 \nonumber\\
not_regulate & 1.00000 \nonumber\\
easily_clean & 1.00000 \nonumber\\
bottle_itself & 1.00000 \nonumber\\
water_cleanser & 1.00000 \nonumber\\
in_five & 1.00000 \nonumber\\
moss & 1.00000 \nonumber\\
anywhere_unless & 1.00000 \nonumber\\
if_tap & 1.00000 \nonumber\\
cleanser & 1.00000 \nonumber\\
clean_it & 1.00000 \nonumber\\
cleanser_. & 1.00000 \nonumber\\
ProductionRule_VP->VBN,ADVP,SBAR, & 1.00000 \nonumber\\
the_consumption & 1.00000 \nonumber\\
landfill_which & 1.00000 \nonumber\\
of_emergency & 1.00000 \nonumber\\
leaf_, & 1.00000 \nonumber\\
cost_be & 1.00000 \nonumber\\
._90 & 1.00000 \nonumber\\
unless_in & 1.00000 \nonumber\\
can_leak & 1.00000 \nonumber\\
have_show & 1.00000 \nonumber\\
envy & 1.00000 \nonumber\\
ProductionRule_ADVP->NN,IN, & 1.00000 \nonumber\\
help_kid & 1.00000 \nonumber\\
than_1 & 1.00000 \nonumber\\
can_, & 1.00000 \nonumber\\
dad_. & 1.00000 \nonumber\\
first_sign & 1.00000 \nonumber\\
away_at & 1.00000 \nonumber\\
then_" & 1.00000 \nonumber\\
longer_yours & 1.00000 \nonumber\\
of_pain & 1.00000 \nonumber\\
outside_your & 1.00000 \nonumber\\
ProductionRule_VP->VBZ,ADVP,NP,,,SBAR, & 1.00000 \nonumber\\
own_. & 1.00000 \nonumber\\
off_move & 1.00000 \nonumber\\
rid_off & 1.00000 \nonumber\\
pain_, & 1.00000 \nonumber\\
sign_of & 1.00000 \nonumber\\
feel_outside & 1.00000 \nonumber\\
nobody_have & 1.00000 \nonumber\\
no_longer & 1.00000 \nonumber\\
which_you & 1.00000 \nonumber\\
without_you & 1.00000 \nonumber\\
to_rid & 1.00000 \nonumber\\
your_body & 1.00000 \nonumber\\
ProductionRule_VP->VB,PRT,NP,ADVP,,,PP, & 1.00000 \nonumber\\
that_which & 1.00000 \nonumber\\
make_that & 1.00000 \nonumber\\
dont_want & 1.00000 \nonumber\\
._read & 1.00000 \nonumber\\
express_yourself & 1.00000 \nonumber\\
stratum & 1.00000 \nonumber\\
rock_stratum & 1.00000 \nonumber\\
because_there & 1.00000 \nonumber\\
concern_about & 1.00000 \nonumber\\
people_be & 1.00000 \nonumber\\
list & 1.00000 \nonumber\\
be_such & 1.00000 \nonumber\\
aside & 1.00000 \nonumber\\
to_hold & 1.00000 \nonumber\\
rule_, & 1.00000 \nonumber\\
off_in & 1.00000 \nonumber\\
liquidate & 1.00000 \nonumber\\
poorer & 1.00000 \nonumber\\
can_start & 1.00000 \nonumber\\
start_row & 1.00000 \nonumber\\
uniform_liquidate & 1.00000 \nonumber\\
action_will & 1.00000 \nonumber\\
boy_. & 1.00000 \nonumber\\
liquidate_all & 1.00000 \nonumber\\
poorer_. & 1.00000 \nonumber\\
this_action & 1.00000 \nonumber\\
will_create & 1.00000 \nonumber\\
atmosphere_in & 1.00000 \nonumber\\
both_pupil & 1.00000 \nonumber\\
make_impossible & 1.00000 \nonumber\\
all_conflict & 1.00000 \nonumber\\
be_richer & 1.00000 \nonumber\\
occur_between & 1.00000 \nonumber\\
rich_can & 1.00000 \nonumber\\
row_between & 1.00000 \nonumber\\
pupil_. & 1.00000 \nonumber\\
richer_than & 1.00000 \nonumber\\
one_pupil & 1.00000 \nonumber\\
the_race & 1.00000 \nonumber\\
fashion_among & 1.00000 \nonumber\\
negative_atmosphere & 1.00000 \nonumber\\
richer & 1.00000 \nonumber\\
be_poorer & 1.00000 \nonumber\\
it_often & 1.00000 \nonumber\\
between_both & 1.00000 \nonumber\\
rare_between & 1.00000 \nonumber\\
than_another & 1.00000 \nonumber\\
the_boy & 1.00000 \nonumber\\
row & 1.00000 \nonumber\\
a_rule & 1.00000 \nonumber\\
._rich & 1.00000 \nonumber\\
hold_the & 1.00000 \nonumber\\
conflict_. & 1.00000 \nonumber\\
race_for & 1.00000 \nonumber\\
of_memory & 1.00000 \nonumber\\
increase_the & 1.00000 \nonumber\\
will_do & 1.00000 \nonumber\\
this_case & 1.00000 \nonumber\\
be_take & 1.00000 \nonumber\\
them_all & 1.00000 \nonumber\\
._physical & 1.00000 \nonumber\\
_pos_ngram_CARD_V_NN & 1.00000 \nonumber\\
necessarily & 1.00000 \nonumber\\
like_for & 1.00000 \nonumber\\
example_at & 1.00000 \nonumber\\
else_back & 1.00000 \nonumber\\
abusive_to & 1.00000 \nonumber\\
hit_there & 1.00000 \nonumber\\
and_abusive & 1.00000 \nonumber\\
there_kid & 1.00000 \nonumber\\
up_fight & 1.00000 \nonumber\\
hit_someone & 1.00000 \nonumber\\
back_like & 1.00000 \nonumber\\
not_hit & 1.00000 \nonumber\\
ok_to & 1.00000 \nonumber\\
ProductionRule_VP->VB,PRT,UCP, & 1.00000 \nonumber\\
adult_. & 1.00000 \nonumber\\
it_shouldnt & 1.00000 \nonumber\\
._though & 1.00000 \nonumber\\
the_learn & 1.00000 \nonumber\\
to_feel & 1.00000 \nonumber\\
do_everything & 1.00000 \nonumber\\
nd & 1.00000 \nonumber\\
together_. & 1.00000 \nonumber\\
and_this & 1.00000 \nonumber\\
fair_all-around & 1.00000 \nonumber\\
%_effective & 1.00000 \nonumber\\
all-around & 1.00000 \nonumber\\
all-around_. & 1.00000 \nonumber\\
"_they & 1.00000 \nonumber\\
be_) & 1.00000 \nonumber\\
patch_, & 1.00000 \nonumber\\
75_% & 1.00000 \nonumber\\
morning-after & 1.00000 \nonumber\\
rape_) & 1.00000 \nonumber\\
,_pill & 1.00000 \nonumber\\
with_exception & 1.00000 \nonumber\\
morning-after_pill & 1.00000 \nonumber\\
be_ton & 1.00000 \nonumber\\
pill_( & 1.00000 \nonumber\\
maybe_instead & 1.00000 \nonumber\\
effective_) & 1.00000 \nonumber\\
have_pro-life & 1.00000 \nonumber\\
pregnant_. & 1.00000 \nonumber\\
the_patch & 1.00000 \nonumber\\
_pos_ngram_PUNC_PR_O & 1.00000 \nonumber\\
'_fair & 1.00000 \nonumber\\
be_morning-after & 1.00000 \nonumber\\
they_( & 1.00000 \nonumber\\
ProductionRule_VP->TO,ADVP,VP, & 1.00000 \nonumber\\
they_" & 1.00000 \nonumber\\
of_pro-choice & 1.00000 \nonumber\\
condom & 1.00000 \nonumber\\
)_should & 1.00000 \nonumber\\
)_for & 1.00000 \nonumber\\
(_99 & 1.00000 \nonumber\\
(_i.e. & 1.00000 \nonumber\\
way_not & 1.00000 \nonumber\\
exception & 1.00000 \nonumber\\
(_75 & 1.00000 \nonumber\\
i.e._woman & 1.00000 \nonumber\\
pro-choice_v. & 1.00000 \nonumber\\
i.e. & 1.00000 \nonumber\\
v._pro-life & 1.00000 \nonumber\\
but_with & 1.00000 \nonumber\\
exception_( & 1.00000 \nonumber\\
condom_( & 1.00000 \nonumber\\
be_condom & 1.00000 \nonumber\\
75 & 1.00000 \nonumber\\
evidence_. & 1.00000 \nonumber\\
to_our & 1.00000 \nonumber\\
creator_. & 1.00000 \nonumber\\
woman_in & 1.00000 \nonumber\\
ProductionRule_X->DT,RBR, & 1.00000 \nonumber\\
ProductionRule_X->DT,JJR, & 1.00000 \nonumber\\
(_which & 1.00000 \nonumber\\
_pos_ngram_CARD_PP_CARD & 1.00000 \nonumber\\
not_because & 1.00000 \nonumber\\
unborn & 1.00000 \nonumber\\
ProductionRule_VP->VBP,PP,PP, & 1.00000 \nonumber\\
herself & 1.00000 \nonumber\\
as_that & 1.00000 \nonumber\\
computer & 1.00000 \nonumber\\
_pos_ngram_ADJ_ADJ_CONJ & 1.00000 \nonumber\\
i_take & 1.00000 \nonumber\\
come_. & 1.00000 \nonumber\\
'_unfortunate & 1.00000 \nonumber\\
mistake_and & 1.00000 \nonumber\\
his_accomplice & 1.00000 \nonumber\\
bid_it & 1.00000 \nonumber\\
worst_. & 1.00000 \nonumber\\
me_his & 1.00000 \nonumber\\
heart_to & 1.00000 \nonumber\\
accomplice_. & 1.00000 \nonumber\\
accomplice & 1.00000 \nonumber\\
or_for & 1.00000 \nonumber\\
ProductionRule_VP->MD,ADVP,RB,VP, & 1.00000 \nonumber\\
for_better & 1.00000 \nonumber\\
better_or & 1.00000 \nonumber\\
_pos_ngram_PP_CONJ_O & 1.00000 \nonumber\\
the_heart & 1.00000 \nonumber\\
for_worst & 1.00000 \nonumber\\
that_but & 1.00000 \nonumber\\
protect_each & 1.00000 \nonumber\\
likely_not & 1.00000 \nonumber\\
yes_he & 1.00000 \nonumber\\
man_i & 1.00000 \nonumber\\
big_mistake & 1.00000 \nonumber\\
husband_where & 1.00000 \nonumber\\
life_to & 1.00000 \nonumber\\
_pos_ngram_V_ART_CONJ & 1.00000 \nonumber\\
economy_. & 1.00000 \nonumber\\
they_waste & 1.00000 \nonumber\\
_pos_ngram_O_NN_ART & 1.00000 \nonumber\\
super & 1.00000 \nonumber\\
be_part & 1.00000 \nonumber\\
yes_to & 1.00000 \nonumber\\
book_do & 1.00000 \nonumber\\
want_it & 1.00000 \nonumber\\
_pos_ngram_NP_ART_NP & 1.00000 \nonumber\\
_pos_ngram_V_O_ADV & 1.00000 \nonumber\\
page & 1.00000 \nonumber\\
ProductionRule_NP->PRP,NNS, & 1.00000 \nonumber\\
toolbar & 1.00000 \nonumber\\
in_we & 1.00000 \nonumber\\
not_insult & 1.00000 \nonumber\\
just_wrong & 1.00000 \nonumber\\
wrong_we & 1.00000 \nonumber\\
ProductionRule_VP->MD,RB,S, & 1.00000 \nonumber\\
we_believe & 1.00000 \nonumber\\
you_people & 1.00000 \nonumber\\
insult_who & 1.00000 \nonumber\\
electricity_bill & 1.00000 \nonumber\\
even_reduce & 1.00000 \nonumber\\
which_use & 1.00000 \nonumber\\
reduce_our & 1.00000 \nonumber\\
our_electricity & 1.00000 \nonumber\\
bill & 1.00000 \nonumber\\
book_even & 1.00000 \nonumber\\
our_spend & 1.00000 \nonumber\\
use_much & 1.00000 \nonumber\\
bill_! & 1.00000 \nonumber\\
!_which & 1.00000 \nonumber\\
spend_money & 1.00000 \nonumber\\
resentment_among & 1.00000 \nonumber\\
equal_status & 1.00000 \nonumber\\
afford_and & 1.00000 \nonumber\\
that_rich & 1.00000 \nonumber\\
provide_equal & 1.00000 \nonumber\\
essential_especially & 1.00000 \nonumber\\
rich_student & 1.00000 \nonumber\\
dress_everyday & 1.00000 \nonumber\\
be_essential & 1.00000 \nonumber\\
mock_other & 1.00000 \nonumber\\
not_afford & 1.00000 \nonumber\\
student_may & 1.00000 \nonumber\\
student_will & 1.00000 \nonumber\\
mock & 1.00000 \nonumber\\
to_resentment & 1.00000 \nonumber\\
among_them & 1.00000 \nonumber\\
uniform_provide & 1.00000 \nonumber\\
also_mock & 1.00000 \nonumber\\
same_financial & 1.00000 \nonumber\\
gap_among & 1.00000 \nonumber\\
child_may & 1.00000 \nonumber\\
other_student & 1.00000 \nonumber\\
some_insensitive & 1.00000 \nonumber\\
wear_old & 1.00000 \nonumber\\
cloth_. & 1.00000 \nonumber\\
school_all & 1.00000 \nonumber\\
insensitive & 1.00000 \nonumber\\
will_wear & 1.00000 \nonumber\\
belong_to & 1.00000 \nonumber\\
no_uniform & 1.00000 \nonumber\\
no_gap & 1.00000 \nonumber\\
everyday_which & 1.00000 \nonumber\\
not_belong & 1.00000 \nonumber\\
old_cloth & 1.00000 \nonumber\\
may_lead & 1.00000 \nonumber\\
status_to & 1.00000 \nonumber\\
financial_status & 1.00000 \nonumber\\
financial & 1.00000 \nonumber\\
insensitive_child & 1.00000 \nonumber\\
new_dress & 1.00000 \nonumber\\
wear_new & 1.00000 \nonumber\\
innocent & 1.00000 \nonumber\\
that_right & 1.00000 \nonumber\\
._teenager & 1.00000 \nonumber\\
to_church & 1.00000 \nonumber\\
idea_of & 1.00000 \nonumber\\
_pos_ngram_V_O_PR & 1.00000 \nonumber\\
bottle_should & 1.00000 \nonumber\\
you_like & 1.00000 \nonumber\\
700 & 1.00000 \nonumber\\
700_year & 1.00000 \nonumber\\
to_decompose & 1.00000 \nonumber\\
poor & 1.00000 \nonumber\\
size & 1.00000 \nonumber\\
support_evolution & 1.00000 \nonumber\\
ProductionRule_VP->VBP,NP,ADVP,SBAR, & 1.00000 \nonumber\\
would_stop & 1.00000 \nonumber\\
of_one & 1.00000 \nonumber\\
,_both & 1.00000 \nonumber\\
fox & 1.00000 \nonumber\\
_pos_ngram_ADV_CARD_PP & 1.00000 \nonumber\\
with_our & 1.00000 \nonumber\\
think_book & 1.00000 \nonumber\\
that_student & 1.00000 \nonumber\\
family_and & 1.00000 \nonumber\\
and_friend & 1.00000 \nonumber\\
sad & 1.00000 \nonumber\\
mile_in & 1.00000 \nonumber\\
may_stand & 1.00000 \nonumber\\
ProductionRule_NP->CD,NP,NNS, & 1.00000 \nonumber\\
'_story & 1.00000 \nonumber\\
._until & 1.00000 \nonumber\\
firm_with & 1.00000 \nonumber\\
until_then & 1.00000 \nonumber\\
walk_a & 1.00000 \nonumber\\
speak_on & 1.00000 \nonumber\\
to_like & 1.00000 \nonumber\\
your_opinion & 1.00000 \nonumber\\
their_behalf & 1.00000 \nonumber\\
?_until & 1.00000 \nonumber\\
stand_firm & 1.00000 \nonumber\\
can_or & 1.00000 \nonumber\\
these_girl & 1.00000 \nonumber\\
'_/ & 1.00000 \nonumber\\
opinion_on & 1.00000 \nonumber\\
audacity_to & 1.00000 \nonumber\\
then_, & 1.00000 \nonumber\\
in_these & 1.00000 \nonumber\\
to_respect & 1.00000 \nonumber\\
behalf_. & 1.00000 \nonumber\\
the_subject & 1.00000 \nonumber\\
'_shoe & 1.00000 \nonumber\\
have_walk & 1.00000 \nonumber\\
subject_matter & 1.00000 \nonumber\\
the_audacity & 1.00000 \nonumber\\
shoe_, & 1.00000 \nonumber\\
audacity & 1.00000 \nonumber\\
or_ca & 1.00000 \nonumber\\
'_opinion & 1.00000 \nonumber\\
know_these & 1.00000 \nonumber\\
/_woman & 1.00000 \nonumber\\
believe_" & 1.00000 \nonumber\\
which_will & 1.00000 \nonumber\\
life_have & 1.00000 \nonumber\\
our_body & 1.00000 \nonumber\\
quite_often & 1.00000 \nonumber\\
clear-cut_winner & 1.00000 \nonumber\\
of_every & 1.00000 \nonumber\\
of_toolbar & 1.00000 \nonumber\\
a_design & 1.00000 \nonumber\\
design_standpoint & 1.00000 \nonumber\\
ProductionRule_NP->DT,NNP,NNP,NN, & 1.00000 \nonumber\\
uus_like & 1.00000 \nonumber\\
uus_customization & 1.00000 \nonumber\\
uus & 1.00000 \nonumber\\
'_fox & 1.00000 \nonumber\\
customization_that & 1.00000 \nonumber\\
customization & 1.00000 \nonumber\\
7_be & 1.00000 \nonumber\\
people_debate & 1.00000 \nonumber\\
criminal_of & 1.00000 \nonumber\\
pretty_browser & 1.00000 \nonumber\\
their_browser & 1.00000 \nonumber\\
ProductionRule_S->PP,,,NP,ADVP,VP,., & 1.00000 \nonumber\\
most_criminal & 1.00000 \nonumber\\
ugly & 1.00000 \nonumber\\
absolutely_win & 1.00000 \nonumber\\
ugly_uus & 1.00000 \nonumber\\
the_clear-cut & 1.00000 \nonumber\\
the_superiority & 1.00000 \nonumber\\
beautiful_skin & 1.00000 \nonumber\\
beautiful & 1.00000 \nonumber\\
browser_battle & 1.00000 \nonumber\\
browser_or & 1.00000 \nonumber\\
browser_quite & 1.00000 \nonumber\\
or_another & 1.00000 \nonumber\\
one_browser & 1.00000 \nonumber\\
the_pretty & 1.00000 \nonumber\\
clear-cut & 1.00000 \nonumber\\
of_beautiful & 1.00000 \nonumber\\
(_7 & 1.00000 \nonumber\\
junkie_, & 1.00000 \nonumber\\
intraweb_junkie & 1.00000 \nonumber\\
ie_( & 1.00000 \nonumber\\
you_add & 1.00000 \nonumber\\
all_) & 1.00000 \nonumber\\
array & 1.00000 \nonumber\\
everyone_use & 1.00000 \nonumber\\
array_of & 1.00000 \nonumber\\
firefox_support & 1.00000 \nonumber\\
every_ie & 1.00000 \nonumber\\
assume_most & 1.00000 \nonumber\\
know_everyone & 1.00000 \nonumber\\
fox_be & 1.00000 \nonumber\\
winner_. & 1.00000 \nonumber\\
intraweb & 1.00000 \nonumber\\
superiority_of & 1.00000 \nonumber\\
and_since & 1.00000 \nonumber\\
be_intraweb & 1.00000 \nonumber\\
skin_out & 1.00000 \nonumber\\
an_array & 1.00000 \nonumber\\
at_an & 1.00000 \nonumber\\
firefox_absolutely & 1.00000 \nonumber\\
)_? & 1.00000 \nonumber\\
superiority & 1.00000 \nonumber\\
battle_. & 1.00000 \nonumber\\
junkie & 1.00000 \nonumber\\
and_uus & 1.00000 \nonumber\\
an_ugly & 1.00000 \nonumber\\
power_have & 1.00000 \nonumber\\
old_? & 1.00000 \nonumber\\
have_exist & 1.00000 \nonumber\\
ProductionRule_SQ->MD,NP,VP,., & 1.00000 \nonumber\\
when_really & 1.00000 \nonumber\\
_pos_ngram_CARD_CARD_CARD & 1.00000 \nonumber\\
only_1 & 1.00000 \nonumber\\
higher_power & 1.00000 \nonumber\\
unproven_higher & 1.00000 \nonumber\\
ProductionRule_QP->RB,CD,CD, & 1.00000 \nonumber\\
exist_for & 1.00000 \nonumber\\
appear_to & 1.00000 \nonumber\\
year_when & 1.00000 \nonumber\\
10_million & 1.00000 \nonumber\\
a_unproven & 1.00000 \nonumber\\
could_a & 1.00000 \nonumber\\
1_hundr & 1.00000 \nonumber\\
million_year & 1.00000 \nonumber\\
hundr_thousand & 1.00000 \nonumber\\
that_appear & 1.00000 \nonumber\\
unproven & 1.00000 \nonumber\\
ProductionRule_QP->JJR,IN,CD,CD, & 1.00000 \nonumber\\
hundr & 1.00000 \nonumber\\
ProductionRule_NP->DT,JJ,JJR,NN, & 1.00000 \nonumber\\
rich_. & 1.00000 \nonumber\\
woman_who & 1.00000 \nonumber\\
_pos_ngram_O_PR_O & 1.00000 \nonumber\\
ProductionRule_SBAR->CC,S, & 1.00000 \nonumber\\
_pos_ngram_PR_ADJ_PR & 1.00000 \nonumber\\
give_it & 1.00000 \nonumber\\
_pos_ngram_ART_V_PUNC & 1.00000 \nonumber\\
leak & 1.00000 \nonumber\\
whoever & 1.00000 \nonumber\\
something_and & 1.00000 \nonumber\\
institute & 1.00000 \nonumber\\
"_porn & 1.00000 \nonumber\\
and_respect & 1.00000 \nonumber\\
him_a & 1.00000 \nonumber\\
status_. & 1.00000 \nonumber\\
_pos_ngram_ADV_ART_NP & 1.00000 \nonumber\\
yours_, & 1.00000 \nonumber\\
yours & 1.00000 \nonumber\\
involve_with & 1.00000 \nonumber\\
code & 1.00000 \nonumber\\
fill & 1.00000 \nonumber\\
be_discipline & 1.00000 \nonumber\\
much_of & 1.00000 \nonumber\\
show_off & 1.00000 \nonumber\\
definitely_turn & 1.00000 \nonumber\\
also_hurt & 1.00000 \nonumber\\
tell_anyone & 1.00000 \nonumber\\
really_make & 1.00000 \nonumber\\
spam & 1.00000 \nonumber\\
not_approve & 1.00000 \nonumber\\
to_read & 1.00000 \nonumber\\
cover & 1.00000 \nonumber\\
basically_a & 1.00000 \nonumber\\
nope & 1.00000 \nonumber\\
but_as & 1.00000 \nonumber\\
who_give & 1.00000 \nonumber\\
think_spank & 1.00000 \nonumber\\
land & 1.00000 \nonumber\\
kid_a & 1.00000 \nonumber\\
reason_not & 1.00000 \nonumber\\
yes_so & 1.00000 \nonumber\\
ProductionRule_ADVP->ADVP,IN, & 1.00000 \nonumber\\
other_no & 1.00000 \nonumber\\
choose_to & 1.00000 \nonumber\\
nothing_wrong & 1.00000 \nonumber\\
have_goal & 1.00000 \nonumber\\
and_end & 1.00000 \nonumber\\
sell & 1.00000 \nonumber\\
temenggong & 1.00000 \nonumber\\
the_temenggong & 1.00000 \nonumber\\
not_up & 1.00000 \nonumber\\
have_come & 1.00000 \nonumber\\
to_exercise & 1.00000 \nonumber\\
think_school & 1.00000 \nonumber\\
help_me & 1.00000 \nonumber\\
$ & 1.00000 \nonumber\\
and_at & 1.00000 \nonumber\\
properly & 1.00000 \nonumber\\
im_go & 1.00000 \nonumber\\
not_it & 1.00000 \nonumber\\
that_just & 1.00000 \nonumber\\
shirt_, & 1.00000 \nonumber\\
flexible & 1.00000 \nonumber\\
,_grow & 1.00000 \nonumber\\
that_no & 1.00000 \nonumber\\
ProductionRule_VP->VB,FRAG, & 1.00000 \nonumber\\
think_, & 1.00000 \nonumber\\
middle_of & 1.00000 \nonumber\\
ProductionRule_NP->DT,ADJP,JJ,NN, & 1.00000 \nonumber\\
your_decision & 1.00000 \nonumber\\
_pos_ngram_PUNC_PP & 1.00000 \nonumber\\
4 & 1.00000 \nonumber\\
wrong_action & 1.00000 \nonumber\\
really_a & 1.00000 \nonumber\\
their_lesson & 1.00000 \nonumber\\
physically_. & 1.00000 \nonumber\\
could_just & 1.00000 \nonumber\\
just_scold & 1.00000 \nonumber\\
scold_their & 1.00000 \nonumber\\
just_scare & 1.00000 \nonumber\\
value_of & 1.00000 \nonumber\\
the_value & 1.00000 \nonumber\\
parent_could & 1.00000 \nonumber\\
scold & 1.00000 \nonumber\\
child_emotionally & 1.00000 \nonumber\\
because_aside & 1.00000 \nonumber\\
next_time & 1.00000 \nonumber\\
hurt_them & 1.00000 \nonumber\\
scare_that & 1.00000 \nonumber\\
lesson_, & 1.00000 \nonumber\\
of_respect & 1.00000 \nonumber\\
them_physically & 1.00000 \nonumber\\
would_hit & 1.00000 \nonumber\\
learn_their & 1.00000 \nonumber\\
hit_be & 1.00000 \nonumber\\
solution_because & 1.00000 \nonumber\\
scare_. & 1.00000 \nonumber\\
kid_wouldnt & 1.00000 \nonumber\\
parent_because & 1.00000 \nonumber\\
only_learn & 1.00000 \nonumber\\
._hit & 1.00000 \nonumber\\
wouldnt_learn & 1.00000 \nonumber\\
again_next & 1.00000 \nonumber\\
stop_what & 1.00000 \nonumber\\
hurt_a & 1.00000 \nonumber\\
action_again & 1.00000 \nonumber\\
aside_hurt & 1.00000 \nonumber\\
of_way & 1.00000 \nonumber\\
brother_, & 1.00000 \nonumber\\
all_compare & 1.00000 \nonumber\\
farquar_stay & 1.00000 \nonumber\\
farquar_. & 1.00000 \nonumber\\
much_at & 1.00000 \nonumber\\
,_return & 1.00000 \nonumber\\
solve_many & 1.00000 \nonumber\\
to_farquar & 1.00000 \nonumber\\
ProductionRule_VP->VBD,CC,VBD,NP,,,S, & 1.00000 \nonumber\\
here_all & 1.00000 \nonumber\\
stay_here & 1.00000 \nonumber\\
._farquar & 1.00000 \nonumber\\
return_after & 1.00000 \nonumber\\
"_undermine & 1.00000 \nonumber\\
will_still & 1.00000 \nonumber\\
will_drastically & 1.00000 \nonumber\\
overpopulate_earth & 1.00000 \nonumber\\
union_" & 1.00000 \nonumber\\
ability_of & 1.00000 \nonumber\\
not_satisfy & 1.00000 \nonumber\\
of_law & 1.00000 \nonumber\\
an_overpopulate & 1.00000 \nonumber\\
an_issue & 1.00000 \nonumber\\
should_revert & 1.00000 \nonumber\\
of_nature & 1.00000 \nonumber\\
year_" & 1.00000 \nonumber\\
"_might & 1.00000 \nonumber\\
if_" & 1.00000 \nonumber\\
slavery_- & 1.00000 \nonumber\\
over_hundred & 1.00000 \nonumber\\
overtax & 1.00000 \nonumber\\
feed_us & 1.00000 \nonumber\\
so_call & 1.00000 \nonumber\\
overtax_ability & 1.00000 \nonumber\\
never_change & 1.00000 \nonumber\\
._furthermore & 1.00000 \nonumber\\
undermine & 1.00000 \nonumber\\
undermine_the & 1.00000 \nonumber\\
but_will & 1.00000 \nonumber\\
already_overtax & 1.00000 \nonumber\\
shut & 1.00000 \nonumber\\
overpopulate & 1.00000 \nonumber\\
mouth_, & 1.00000 \nonumber\\
where_global & 1.00000 \nonumber\\
shut_their & 1.00000 \nonumber\\
revert_back & 1.00000 \nonumber\\
tribe_& & 1.00000 \nonumber\\
satisfy_them & 1.00000 \nonumber\\
to_tribe & 1.00000 \nonumber\\
their_mouth & 1.00000 \nonumber\\
the_already & 1.00000 \nonumber\\
warm_will & 1.00000 \nonumber\\
than_law & 1.00000 \nonumber\\
drastically_reduce & 1.00000 \nonumber\\
really_an & 1.00000 \nonumber\\
develop_over & 1.00000 \nonumber\\
&_slavery & 1.00000 \nonumber\\
really_against & 1.00000 \nonumber\\
assumption_of & 1.00000 \nonumber\\
might_shut & 1.00000 \nonumber\\
earth_where & 1.00000 \nonumber\\
the_assumption & 1.00000 \nonumber\\
revert & 1.00000 \nonumber\\
minimal_on & 1.00000 \nonumber\\
be_strong & 1.00000 \nonumber\\
ProductionRule_PP->DT,IN,NP, & 1.00000 \nonumber\\
or_they & 1.00000 \nonumber\\
a_sin & 1.00000 \nonumber\\
economy_he & 1.00000 \nonumber\\
'_boost & 1.00000 \nonumber\\
boost_of & 1.00000 \nonumber\\
of_economy & 1.00000 \nonumber\\
survive & 1.00000 \nonumber\\
to_increase & 1.00000 \nonumber\\
!_( & 1.00000 \nonumber\\
?_) & 1.00000 \nonumber\\
college_. & 1.00000 \nonumber\\
with_out & 1.00000 \nonumber\\
ProductionRule_NP->NP,,,NP, & 1.00000 \nonumber\\
standpoint & 1.00000 \nonumber\\
you_on & 1.00000 \nonumber\\
the_tab & 1.00000 \nonumber\\
be_drink & 1.00000 \nonumber\\
still_not & 1.00000 \nonumber\\
they_all & 1.00000 \nonumber\\
of_global & 1.00000 \nonumber\\
_pos_ngram_ADJ_PR_PP & 1.00000 \nonumber\\
flinch & 1.00000 \nonumber\\
keep_obtain & 1.00000 \nonumber\\
its_what & 1.00000 \nonumber\\
thier_. & 1.00000 \nonumber\\
our_instinc & 1.00000 \nonumber\\
instinc_have & 1.00000 \nonumber\\
we_see & 1.00000 \nonumber\\
our_desire & 1.00000 \nonumber\\
post_modern & 1.00000 \nonumber\\
our_animal & 1.00000 \nonumber\\
state_change & 1.00000 \nonumber\\
today_post & 1.00000 \nonumber\\
keep_ous & 1.00000 \nonumber\\
but_our & 1.00000 \nonumber\\
wen_we & 1.00000 \nonumber\\
into_keep & 1.00000 \nonumber\\
something_come & 1.00000 \nonumber\\
our_mental & 1.00000 \nonumber\\
animal_insctinc & 1.00000 \nonumber\\
come_at & 1.00000 \nonumber\\
above_other & 1.00000 \nonumber\\
ProductionRule_NP->PRP$,JJ,NN,NNS, & 1.00000 \nonumber\\
time_change & 1.00000 \nonumber\\
survive_above & 1.00000 \nonumber\\
flinch_wen & 1.00000 \nonumber\\
survival_, & 1.00000 \nonumber\\
us_flinch & 1.00000 \nonumber\\
ous_it & 1.00000 \nonumber\\
insctinc_be & 1.00000 \nonumber\\
be_survival & 1.00000 \nonumber\\
mental_state & 1.00000 \nonumber\\
change_but & 1.00000 \nonumber\\
ous_alive & 1.00000 \nonumber\\
change_into & 1.00000 \nonumber\\
ous & 1.00000 \nonumber\\
ProductionRule_VP->VB,ADVP,,,NP, & 1.00000 \nonumber\\
at_ous & 1.00000 \nonumber\\
in_today & 1.00000 \nonumber\\
us_react & 1.00000 \nonumber\\
obtain & 1.00000 \nonumber\\
alive_. & 1.00000 \nonumber\\
obtain_money & 1.00000 \nonumber\\
react_faster & 1.00000 \nonumber\\
instinc & 1.00000 \nonumber\\
wen & 1.00000 \nonumber\\
modern_world & 1.00000 \nonumber\\
insctinc & 1.00000 \nonumber\\
still_thier & 1.00000 \nonumber\\
easier_and & 1.00000 \nonumber\\
you_argue & 1.00000 \nonumber\\
that_happen & 1.00000 \nonumber\\
_pos_ngram_PUNC_PR_PR & 1.00000 \nonumber\\
do_both & 1.00000 \nonumber\\
like_what & 1.00000 \nonumber\\
can_become & 1.00000 \nonumber\\
become_more & 1.00000 \nonumber\\
me_too & 1.00000 \nonumber\\
their_for & 1.00000 \nonumber\\
younger & 1.00000 \nonumber\\
stay_with & 1.00000 \nonumber\\
learn_the & 1.00000 \nonumber\\
sleep_next & 1.00000 \nonumber\\
_pos_ngram_ART_PR_ADV & 1.00000 \nonumber\\
the_fact & 1.00000 \nonumber\\
;_i & 1.00000 \nonumber\\
people_? & 1.00000 \nonumber\\
ProductionRule_VP->VB,S,,,SBAR, & 1.00000 \nonumber\\
to_win & 1.00000 \nonumber\\
while_raffle & 1.00000 \nonumber\\
have_write & 1.00000 \nonumber\\
no_more & 1.00000 \nonumber\\
the_moral & 1.00000 \nonumber\\
puzzle & 1.00000 \nonumber\\
like_believe & 1.00000 \nonumber\\
solve_by & 1.00000 \nonumber\\
be_solve & 1.00000 \nonumber\\
puzzle_can & 1.00000 \nonumber\\
the_piece & 1.00000 \nonumber\\
feel_and & 1.00000 \nonumber\\
right_way & 1.00000 \nonumber\\
us_smart & 1.00000 \nonumber\\
ProductionRule_VP->VB,CC,VB, & 1.00000 \nonumber\\
and_express & 1.00000 \nonumber\\
learn_which & 1.00000 \nonumber\\
express_but & 1.00000 \nonumber\\
need_him & 1.00000 \nonumber\\
._take & 1.00000 \nonumber\\
have_never & 1.00000 \nonumber\\
"_to & 1.00000 \nonumber\\
what_right & 1.00000 \nonumber\\
(_a & 1.00000 \nonumber\\
"_argument & 1.00000 \nonumber\\
,_over & 1.00000 \nonumber\\
,_although & 1.00000 \nonumber\\
uncomfortable_. & 1.00000 \nonumber\\
acceptance_and & 1.00000 \nonumber\\
respecful_of & 1.00000 \nonumber\\
away_because & 1.00000 \nonumber\\
please_be & 1.00000 \nonumber\\
respecful & 1.00000 \nonumber\\
consider_" & 1.00000 \nonumber\\
constantly_be & 1.00000 \nonumber\\
lifestyle_choice & 1.00000 \nonumber\\
and_his/her & 1.00000 \nonumber\\
harrass_and & 1.00000 \nonumber\\
be_harrass & 1.00000 \nonumber\\
between_that & 1.00000 \nonumber\\
harrass & 1.00000 \nonumber\\
interest_. & 1.00000 \nonumber\\
happy_or & 1.00000 \nonumber\\
n't_choose & 1.00000 \nonumber\\
and_cruel & 1.00000 \nonumber\\
you_uncomfortable & 1.00000 \nonumber\\
"_unnatural & 1.00000 \nonumber\\
all_some & 1.00000 \nonumber\\
want_acceptance & 1.00000 \nonumber\\
live_that & 1.00000 \nonumber\\
ignore_it & 1.00000 \nonumber\\
gay_either & 1.00000 \nonumber\\
unfortunate_and & 1.00000 \nonumber\\
a_lifestyle & 1.00000 \nonumber\\
one_give & 1.00000 \nonumber\\
be_respecful & 1.00000 \nonumber\\
love_interest & 1.00000 \nonumber\\
his/her_love & 1.00000 \nonumber\\
create_them & 1.00000 \nonumber\\
right_away & 1.00000 \nonumber\\
cruel_. & 1.00000 \nonumber\\
give_right & 1.00000 \nonumber\\
take_that & 1.00000 \nonumber\\
unnatural_" & 1.00000 \nonumber\\
cruel & 1.00000 \nonumber\\
ProductionRule_VP->VB,NP,ADVP,SBAR, & 1.00000 \nonumber\\
control & 1.00000 \nonumber\\
than_you & 1.00000 \nonumber\\
perspective & 1.00000 \nonumber\\
where_he & 1.00000 \nonumber\\
be_scare & 1.00000 \nonumber\\
kid_for & 1.00000 \nonumber\\
a_last & 1.00000 \nonumber\\
then_there & 1.00000 \nonumber\\
earn_the & 1.00000 \nonumber\\
trust_of & 1.00000 \nonumber\\
ProductionRule_VP->VBD,PP,ADVP,,,SBAR,,,S, & 1.00000 \nonumber\\
so_farquhar & 1.00000 \nonumber\\
farquhar_stay & 1.00000 \nonumber\\
ProductionRule_NP->JJR,NN,S, & 1.00000 \nonumber\\
the_trust & 1.00000 \nonumber\\
singapore_longer & 1.00000 \nonumber\\
ProductionRule_VP->VP,,,VP,CC,VP, & 1.00000 \nonumber\\
people_more & 1.00000 \nonumber\\
those_problem & 1.00000 \nonumber\\
solve_those & 1.00000 \nonumber\\
see_something & 1.00000 \nonumber\\
to_start & 1.00000 \nonumber\\
ProductionRule_VP->ADVP,VBN,SBAR, & 1.00000 \nonumber\\
the_future & 1.00000 \nonumber\\
choice_, & 1.00000 \nonumber\\
understand_him & 1.00000 \nonumber\\
father_not & 1.00000 \nonumber\\
case_i & 1.00000 \nonumber\\
not_here & 1.00000 \nonumber\\
great_reason & 1.00000 \nonumber\\
here_in & 1.00000 \nonumber\\
two_choice & 1.00000 \nonumber\\
will_prefer & 1.00000 \nonumber\\
him_here & 1.00000 \nonumber\\
leave_back & 1.00000 \nonumber\\
depress_. & 1.00000 \nonumber\\
be_depress & 1.00000 \nonumber\\
depress & 1.00000 \nonumber\\
this_two & 1.00000 \nonumber\\
can_pair & 1.00000 \nonumber\\
._guy & 1.00000 \nonumber\\
wether_its & 1.00000 \nonumber\\
reproductive & 1.00000 \nonumber\\
wether & 1.00000 \nonumber\\
that_why & 1.00000 \nonumber\\
attract_, & 1.00000 \nonumber\\
pair_up & 1.00000 \nonumber\\
and_male & 1.00000 \nonumber\\
only_work & 1.00000 \nonumber\\
,_wether & 1.00000 \nonumber\\
reproductive_system & 1.00000 \nonumber\\
opposite_attract & 1.00000 \nonumber\\
and_girl & 1.00000 \nonumber\\
atom & 1.00000 \nonumber\\
atom_, & 1.00000 \nonumber\\
where_, & 1.00000 \nonumber\\
._opposite & 1.00000 \nonumber\\
,_atom & 1.00000 \nonumber\\
why_there & 1.00000 \nonumber\\
electricity_, & 1.00000 \nonumber\\
guy_( & 1.00000 \nonumber\\
magnet & 1.00000 \nonumber\\
two_guy & 1.00000 \nonumber\\
magnet_, & 1.00000 \nonumber\\
work_with & 1.00000 \nonumber\\
doesnt_work & 1.00000 \nonumber\\
make_for & 1.00000 \nonumber\\
girl_! & 1.00000 \nonumber\\
in_magnet & 1.00000 \nonumber\\
male_reproductive & 1.00000 \nonumber\\
with_two & 1.00000 \nonumber\\
female_reproductive & 1.00000 \nonumber\\
its_in & 1.00000 \nonumber\\
with_opposite & 1.00000 \nonumber\\
_pos_ngram_PUNC_PUNC_NP & 1.00000 \nonumber\\
this_reason & 1.00000 \nonumber\\
genitals_) & 1.00000 \nonumber\\
guy_and & 1.00000 \nonumber\\
genitals & 1.00000 \nonumber\\
every_where & 1.00000 \nonumber\\
(_genitals & 1.00000 \nonumber\\
,_electricity & 1.00000 \nonumber\\
._on & 1.00000 \nonumber\\
money_and & 1.00000 \nonumber\\
and_put & 1.00000 \nonumber\\
,_indium & 1.00000 \nonumber\\
think_the & 1.00000 \nonumber\\
his/her & 1.00000 \nonumber\\
now_you & 1.00000 \nonumber\\
ProductionRule_ADVP->RB,RBR, & 1.00000 \nonumber\\
reward_for & 1.00000 \nonumber\\
as_far & 1.00000 \nonumber\\
far_as & 1.00000 \nonumber\\
;_it & 1.00000 \nonumber\\
worse & 1.00000 \nonumber\\
other_channel & 1.00000 \nonumber\\
smarter & 1.00000 \nonumber\\
adult_get & 1.00000 \nonumber\\
,_grammar & 1.00000 \nonumber\\
or_adult & 1.00000 \nonumber\\
history_channel & 1.00000 \nonumber\\
smarter_i & 1.00000 \nonumber\\
imagination_so & 1.00000 \nonumber\\
more_you & 1.00000 \nonumber\\
kid_or & 1.00000 \nonumber\\
write_skill & 1.00000 \nonumber\\
ProductionRule_S->X,NP,VP, & 1.00000 \nonumber\\
ProductionRule_S->S,CC,S,,,CC,S, & 1.00000 \nonumber\\
!!!_also & 1.00000 \nonumber\\
pb_kid & 1.00000 \nonumber\\
pb & 1.00000 \nonumber\\
improve_read & 1.00000 \nonumber\\
skill_!!! & 1.00000 \nonumber\\
improve_and & 1.00000 \nonumber\\
bob_!!! & 1.00000 \nonumber\\
use_your & 1.00000 \nonumber\\
sponge & 1.00000 \nonumber\\
more_your & 1.00000 \nonumber\\
imagination_improve & 1.00000 \nonumber\\
your_imagination & 1.00000 \nonumber\\
,_history & 1.00000 \nonumber\\
bob & 1.00000 \nonumber\\
sponge_bob & 1.00000 \nonumber\\
say_pb & 1.00000 \nonumber\\
channel_, & 1.00000 \nonumber\\
read_the & 1.00000 \nonumber\\
read_, & 1.00000 \nonumber\\
get_smarter & 1.00000 \nonumber\\
grammar_, & 1.00000 \nonumber\\
commercial_!!! & 1.00000 \nonumber\\
hate_sponge & 1.00000 \nonumber\\
hate_commercial & 1.00000 \nonumber\\
channel_that & 1.00000 \nonumber\\
your_write & 1.00000 \nonumber\\
connection & 1.00000 \nonumber\\
to_yourself & 1.00000 \nonumber\\
both_student & 1.00000 \nonumber\\
approach_with & 1.00000 \nonumber\\
and_approach & 1.00000 \nonumber\\
properly_and & 1.00000 \nonumber\\
_pos_ngram_O_PUNC_ADJ & 1.00000 \nonumber\\
attitude_, & 1.00000 \nonumber\\
if_teach & 1.00000 \nonumber\\
,_will & 1.00000 \nonumber\\
right_attitude & 1.00000 \nonumber\\
teach_and & 1.00000 \nonumber\\
encourage_properly & 1.00000 \nonumber\\
for_both & 1.00000 \nonumber\\
largest_army & 1.00000 \nonumber\\
largest & 1.00000 \nonumber\\
army_in & 1.00000 \nonumber\\
begin_with & 1.00000 \nonumber\\
the_mind & 1.00000 \nonumber\\
._yeah & 1.00000 \nonumber\\
easily_be & 1.00000 \nonumber\\
alot & 1.00000 \nonumber\\
not_the & 1.00000 \nonumber\\
anything_, & 1.00000 \nonumber\\
sunday & 1.00000 \nonumber\\
because_now & 1.00000 \nonumber\\
concentrate & 1.00000 \nonumber\\
_pos_ngram_PR_CARD_NN & 1.00000 \nonumber\\
darkness & 1.00000 \nonumber\\
define & 1.00000 \nonumber\\
self_, & 1.00000 \nonumber\\
here_to & 1.00000 \nonumber\\
woman_to & 1.00000 \nonumber\\
nut & 1.00000 \nonumber\\
go_nut & 1.00000 \nonumber\\
little_different & 1.00000 \nonumber\\
_pos_ngram_ART_CARD_ADV & 1.00000 \nonumber\\
he_feel & 1.00000 \nonumber\\
kill_some & 1.00000 \nonumber\\
accident_. & 1.00000 \nonumber\\
_pos_ngram_CARD_ADV_PP & 1.00000 \nonumber\\
somone & 1.00000 \nonumber\\
like_kill & 1.00000 \nonumber\\
somone_it & 1.00000 \nonumber\\
nut_and & 1.00000 \nonumber\\
kill_somone & 1.00000 \nonumber\\
._parent & 1.00000 \nonumber\\
rape_, & 1.00000 \nonumber\\
understand_. & 1.00000 \nonumber\\
be_we & 1.00000 \nonumber\\
spirit & 1.00000 \nonumber\\
on_and & 1.00000 \nonumber\\
self_because & 1.00000 \nonumber\\
quarterback & 1.00000 \nonumber\\
quarterback_to & 1.00000 \nonumber\\
quarterback_, & 1.00000 \nonumber\\
the_super & 1.00000 \nonumber\\
in_each & 1.00000 \nonumber\\
super_bowl & 1.00000 \nonumber\\
ProductionRule_SBAR->``,S, & 1.00000 \nonumber\\
because_like & 1.00000 \nonumber\\
good_reward & 1.00000 \nonumber\\
drive_in & 1.00000 \nonumber\\
and_depend & 1.00000 \nonumber\\
block_for & 1.00000 \nonumber\\
pass_. & 1.00000 \nonumber\\
last_2 & 1.00000 \nonumber\\
"_two & 1.00000 \nonumber\\
bowl_the & 1.00000 \nonumber\\
bowl & 1.00000 \nonumber\\
team_" & 1.00000 \nonumber\\
team_sport & 1.00000 \nonumber\\
the_win & 1.00000 \nonumber\\
on_each & 1.00000 \nonumber\\
lineman_block & 1.00000 \nonumber\\
minute_with & 1.00000 \nonumber\\
in_team & 1.00000 \nonumber\\
steeler_could & 1.00000 \nonumber\\
2_minute & 1.00000 \nonumber\\
receiver_believe & 1.00000 \nonumber\\
no_" & 1.00000 \nonumber\\
night_in & 1.00000 \nonumber\\
score & 1.00000 \nonumber\\
the_receiver & 1.00000 \nonumber\\
the_quarterback & 1.00000 \nonumber\\
sport_they & 1.00000 \nonumber\\
football_be & 1.00000 \nonumber\\
labor & 1.00000 \nonumber\\
the_lineman & 1.00000 \nonumber\\
labor_. & 1.00000 \nonumber\\
need_each & 1.00000 \nonumber\\
win_drive & 1.00000 \nonumber\\
quarterback_believe & 1.00000 \nonumber\\
receiver & 1.00000 \nonumber\\
the_steeler & 1.00000 \nonumber\\
,_quarterback & 1.00000 \nonumber\\
good_pass & 1.00000 \nonumber\\
,_football & 1.00000 \nonumber\\
their_labor & 1.00000 \nonumber\\
lineman_, & 1.00000 \nonumber\\
n't_score & 1.00000 \nonumber\\
lineman & 1.00000 \nonumber\\
steeler & 1.00000 \nonumber\\
other_night & 1.00000 \nonumber\\
score_the & 1.00000 \nonumber\\
to_train & 1.00000 \nonumber\\
basketball_in & 1.00000 \nonumber\\
basketball & 1.00000 \nonumber\\
play_basketball & 1.00000 \nonumber\\
go_hike & 1.00000 \nonumber\\
please_with & 1.00000 \nonumber\\
exercise_on & 1.00000 \nonumber\\
not_please & 1.00000 \nonumber\\
choose_whether & 1.00000 \nonumber\\
train_our & 1.00000 \nonumber\\
exercise_, & 1.00000 \nonumber\\
increase_p.e. & 1.00000 \nonumber\\
any_p.e. & 1.00000 \nonumber\\
p.e._requirement & 1.00000 \nonumber\\
to_require & 1.00000 \nonumber\\
i_add & 1.00000 \nonumber\\
my_neighborhood & 1.00000 \nonumber\\
hike_and & 1.00000 \nonumber\\
hike & 1.00000 \nonumber\\
college_be & 1.00000 \nonumber\\
college_to & 1.00000 \nonumber\\
requirement_in & 1.00000 \nonumber\\
requirement_. & 1.00000 \nonumber\\
require_student & 1.00000 \nonumber\\
the_responsible & 1.00000 \nonumber\\
need_exercise & 1.00000 \nonumber\\
neighborhood & 1.00000 \nonumber\\
neighborhood_. & 1.00000 \nonumber\\
can_exercise & 1.00000 \nonumber\\
the_college & 1.00000 \nonumber\\
brain_not & 1.00000 \nonumber\\
our_brain & 1.00000 \nonumber\\
own_as & 1.00000 \nonumber\\
responsible_to & 1.00000 \nonumber\\
variety & 1.00000 \nonumber\\
variety_of & 1.00000 \nonumber\\
big_contribution & 1.00000 \nonumber\\
be_indirect & 1.00000 \nonumber\\
murder_if & 1.00000 \nonumber\\
indirect & 1.00000 \nonumber\\
that_may & 1.00000 \nonumber\\
indirect_murder & 1.00000 \nonumber\\
be_deal & 1.00000 \nonumber\\
woman_decide & 1.00000 \nonumber\\
to_abort & 1.00000 \nonumber\\
n't_take & 1.00000 \nonumber\\
....._..... & 1.00000 \nonumber\\
._please & 1.00000 \nonumber\\
idea_to & 1.00000 \nonumber\\
matter_. & 1.00000 \nonumber\\
in_nasa & 1.00000 \nonumber\\
%_scientist & 1.00000 \nonumber\\
nasa_be & 1.00000 \nonumber\\
nasa & 1.00000 \nonumber\\
scientist_in & 1.00000 \nonumber\\
_pos_ngram_PP_CARD_PP & 1.00000 \nonumber\\
adoption_or & 1.00000 \nonumber\\
bottle_can & 1.00000 \nonumber\\
either_. & 1.00000 \nonumber\\
simple_reason & 1.00000 \nonumber\\
could.for & 1.00000 \nonumber\\
certainly_would & 1.00000 \nonumber\\
i_could.for & 1.00000 \nonumber\\
ProductionRule_VP->VB,ADVP,ADVP,,,SBAR, & 1.00000 \nonumber\\
her_; & 1.00000 \nonumber\\
her_as & 1.00000 \nonumber\\
i_certainly & 1.00000 \nonumber\\
love.but & 1.00000 \nonumber\\
not_stay & 1.00000 \nonumber\\
ProductionRule_S->S,ADVP,VP, & 1.00000 \nonumber\\
dont_believe & 1.00000 \nonumber\\
would_move & 1.00000 \nonumber\\
the_simple & 1.00000 \nonumber\\
of_love.but & 1.00000 \nonumber\\
could.for_the & 1.00000 \nonumber\\
invole & 1.00000 \nonumber\\
from_her & 1.00000 \nonumber\\
love.but_i & 1.00000 \nonumber\\
be_invole & 1.00000 \nonumber\\
invole_with & 1.00000 \nonumber\\
world_in & 1.00000 \nonumber\\
especially_in & 1.00000 \nonumber\\
some_kid & 1.00000 \nonumber\\
!_its & 1.00000 \nonumber\\
world_that & 1.00000 \nonumber\\
dress_code & 1.00000 \nonumber\\
and_push & 1.00000 \nonumber\\
ProductionRule_ADJP->``,JJ,'', & 1.00000 \nonumber\\
which_make & 1.00000 \nonumber\\
ProductionRule_ADJP->JJ,CC,JJ,S, & 1.00000 \nonumber\\
that_" & 1.00000 \nonumber\\
someone_. & 1.00000 \nonumber\\
respect_other & 1.00000 \nonumber\\
day_!!! & 1.00000 \nonumber\\
_pos_ngram_NP_ADV_ADJ & 1.00000 \nonumber\\
begin_to & 1.00000 \nonumber\\
shouldnt_be & 1.00000 \nonumber\\
just_the & 1.00000 \nonumber\\
_pos_ngram_PR_NN_NP & 1.00000 \nonumber\\
rich_" & 1.00000 \nonumber\\
3_time & 1.00000 \nonumber\\
consumption_on & 1.00000 \nonumber\\
ProductionRule_NP->ADJP,NNPS, & 1.00000 \nonumber\\
the_planet & 1.00000 \nonumber\\
could_that & 1.00000 \nonumber\\
_pos_ngram_CARD_NP_PUNC & 1.00000 \nonumber\\
bottle_consumption & 1.00000 \nonumber\\
could_cover & 1.00000 \nonumber\\
mind_mexican & 1.00000 \nonumber\\
_pos_ngram_NN_CARD_NP & 1.00000 \nonumber\\
"_rich & 1.00000 \nonumber\\
of_mexico & 1.00000 \nonumber\\
mexico_3 & 1.00000 \nonumber\\
cover_all & 1.00000 \nonumber\\
ProductionRule_NP->NN,CD,NNP, & 1.00000 \nonumber\\
of_could & 1.00000 \nonumber\\
mexico & 1.00000 \nonumber\\
mexican_. & 1.00000 \nonumber\\
mexican & 1.00000 \nonumber\\
browser_and & 1.00000 \nonumber\\
cache & 1.00000 \nonumber\\
top_feature & 1.00000 \nonumber\\
previous_browser & 1.00000 \nonumber\\
surf & 1.00000 \nonumber\\
net_even & 1.00000 \nonumber\\
surf_the & 1.00000 \nonumber\\
all_previous & 1.00000 \nonumber\\
firefox_take & 1.00000 \nonumber\\
neat_package & 1.00000 \nonumber\\
net & 1.00000 \nonumber\\
_pos_ngram_ART_PP_CARD & 1.00000 \nonumber\\
one_neat & 1.00000 \nonumber\\
cache_if & 1.00000 \nonumber\\
ff_seem & 1.00000 \nonumber\\
and_stick & 1.00000 \nonumber\\
cache_so & 1.00000 \nonumber\\
the_cache & 1.00000 \nonumber\\
stick_it & 1.00000 \nonumber\\
memory_? & 1.00000 \nonumber\\
of_its & 1.00000 \nonumber\\
even_faster & 1.00000 \nonumber\\
its_top & 1.00000 \nonumber\\
security_and & 1.00000 \nonumber\\
to_surf & 1.00000 \nonumber\\
the_net & 1.00000 \nonumber\\
package_. & 1.00000 \nonumber\\
extendibility & 1.00000 \nonumber\\
extendibility_be & 1.00000 \nonumber\\
neat & 1.00000 \nonumber\\
and_extendibility & 1.00000 \nonumber\\
eat_up & 1.00000 \nonumber\\
eat_so & 1.00000 \nonumber\\
just_lower & 1.00000 \nonumber\\
lower_the & 1.00000 \nonumber\\
._security & 1.00000 \nonumber\\
_pos_ngram_O_O_PP & 1.00000 \nonumber\\
and_against & 1.00000 \nonumber\\
ProductionRule_ADVP->IN,PP, & 1.00000 \nonumber\\
sink_. & 1.00000 \nonumber\\
._science & 1.00000 \nonumber\\
because_have & 1.00000 \nonumber\\
have_lousy & 1.00000 \nonumber\\
express_them & 1.00000 \nonumber\\
the_region & 1.00000 \nonumber\\
region & 1.00000 \nonumber\\
value & 1.00000 \nonumber\\
train & 1.00000 \nonumber\\
not_let & 1.00000 \nonumber\\
lay & 1.00000 \nonumber\\
?_the & 1.00000 \nonumber\\
love_firefox & 1.00000 \nonumber\\
the_atheist & 1.00000 \nonumber\\
_pos_ngram_O_PP_O & 1.00000 \nonumber\\
not_have & 1.00000 \nonumber\\
house_and & 1.00000 \nonumber\\
efficient & 1.00000 \nonumber\\
they_wear & 1.00000 \nonumber\\
just_doesnt & 1.00000 \nonumber\\
internet_be & 1.00000 \nonumber\\
the_american & 1.00000 \nonumber\\
block & 1.00000 \nonumber\\
mean_i & 1.00000 \nonumber\\
off_on & 1.00000 \nonumber\\
essential & 1.00000 \nonumber\\
recognize_farquhar & 1.00000 \nonumber\\
when_farquhar & 1.00000 \nonumber\\
not_raffle & 1.00000 \nonumber\\
their_founder & 1.00000 \nonumber\\
farquhar_leave & 1.00000 \nonumber\\
founder_, & 1.00000 \nonumber\\
to_care & 1.00000 \nonumber\\
be_with & 1.00000 \nonumber\\
just_my & 1.00000 \nonumber\\
have_aa & 1.00000 \nonumber\\
father_figuer & 1.00000 \nonumber\\
respectable_, & 1.00000 \nonumber\\
,_honest & 1.00000 \nonumber\\
you_life & 1.00000 \nonumber\\
someone_respectable & 1.00000 \nonumber\\
figuer & 1.00000 \nonumber\\
figuer_in & 1.00000 \nonumber\\
alway_tought & 1.00000 \nonumber\\
,_nd & 1.00000 \nonumber\\
tought_that & 1.00000 \nonumber\\
tought & 1.00000 \nonumber\\
hard_work & 1.00000 \nonumber\\
in_you & 1.00000 \nonumber\\
man_should & 1.00000 \nonumber\\
n't_deserve & 1.00000 \nonumber\\
man_then & 1.00000 \nonumber\\
a_that & 1.00000 \nonumber\\
true_man & 1.00000 \nonumber\\
nd_hard & 1.00000 \nonumber\\
a_true & 1.00000 \nonumber\\
aa & 1.00000 \nonumber\\
aa_father & 1.00000 \nonumber\\
natural_. & 1.00000 \nonumber\\
as_your & 1.00000 \nonumber\\
would_change & 1.00000 \nonumber\\
view_the & 1.00000 \nonumber\\
just_see & 1.00000 \nonumber\\
bid_person & 1.00000 \nonumber\\
relationship_would & 1.00000 \nonumber\\
life_know & 1.00000 \nonumber\\
somebody_else & 1.00000 \nonumber\\
something_to & 1.00000 \nonumber\\
with_life & 1.00000 \nonumber\\
person_as & 1.00000 \nonumber\\
as_somebody & 1.00000 \nonumber\\
change_because & 1.00000 \nonumber\\
you_view & 1.00000 \nonumber\\
same_it & 1.00000 \nonumber\\
spouse_any & 1.00000 \nonumber\\
have_murder & 1.00000 \nonumber\\
global_warm & 1.00000 \nonumber\\
warm & 1.00000 \nonumber\\
crazy_enough & 1.00000 \nonumber\\
listen_to & 1.00000 \nonumber\\
biological & 1.00000 \nonumber\\
earth_, & 1.00000 \nonumber\\
planet_earth & 1.00000 \nonumber\\
on_it & 1.00000 \nonumber\\
much_easier & 1.00000 \nonumber\\
correct & 1.00000 \nonumber\\
another_be & 1.00000 \nonumber\\
standpoint_, & 1.00000 \nonumber\\
compatible_with & 1.00000 \nonumber\\
ProductionRule_ADJP->RB,ADVP,JJ, & 1.00000 \nonumber\\
with_ie & 1.00000 \nonumber\\
adware_seem & 1.00000 \nonumber\\
more_compatible & 1.00000 \nonumber\\
and_adware & 1.00000 \nonumber\\
adware & 1.00000 \nonumber\\
spam_and & 1.00000 \nonumber\\
50_% & 1.00000 \nonumber\\
ProductionRule_S->S,CC,S,CC,S, & 1.00000 \nonumber\\
say_, & 1.00000 \nonumber\\
some_one & 1.00000 \nonumber\\
make_us & 1.00000 \nonumber\\
than_they & 1.00000 \nonumber\\
leaf & 1.00000 \nonumber\\
ProductionRule_NP->DT,``,NN,'', & 1.00000 \nonumber\\
teenager_be & 1.00000 \nonumber\\
belong_. & 1.00000 \nonumber\\
poor_student & 1.00000 \nonumber\\
inferior_. & 1.00000 \nonumber\\
inferior & 1.00000 \nonumber\\
about_my & 1.00000 \nonumber\\
about_clothe & 1.00000 \nonumber\\
plain_clothe & 1.00000 \nonumber\\
sensible & 1.00000 \nonumber\\
brand_and & 1.00000 \nonumber\\
cheap_better & 1.00000 \nonumber\\
cheap & 1.00000 \nonumber\\
wear_to & 1.00000 \nonumber\\
student_day & 1.00000 \nonumber\\
of_kinship & 1.00000 \nonumber\\
although_school & 1.00000 \nonumber\\
case_, & 1.00000 \nonumber\\
also_they & 1.00000 \nonumber\\
clothe_by & 1.00000 \nonumber\\
sensible_so & 1.00000 \nonumber\\
clothe_during & 1.00000 \nonumber\\
and_sense & 1.00000 \nonumber\\
by_brand & 1.00000 \nonumber\\
to_plain & 1.00000 \nonumber\\
feel_sense & 1.00000 \nonumber\\
convenient_. & 1.00000 \nonumber\\
my_student & 1.00000 \nonumber\\
my_clothe & 1.00000 \nonumber\\
feel_inferior & 1.00000 \nonumber\\
my_case & 1.00000 \nonumber\\
and_quantity & 1.00000 \nonumber\\
very_expensive & 1.00000 \nonumber\\
of_belong & 1.00000 \nonumber\\
be_efficient & 1.00000 \nonumber\\
be_cheap & 1.00000 \nonumber\\
kinship & 1.00000 \nonumber\\
be_sensible & 1.00000 \nonumber\\
efficient_in & 1.00000 \nonumber\\
during_my & 1.00000 \nonumber\\
quantity & 1.00000 \nonumber\\
quantity_of & 1.00000 \nonumber\\
kinship_and & 1.00000 \nonumber\\
than_plain & 1.00000 \nonumber\\
they_concern & 1.00000 \nonumber\\
be_convenient & 1.00000 \nonumber\\
would_choose & 1.00000 \nonumber\\
then_he & 1.00000 \nonumber\\
a_murderer & 1.00000 \nonumber\\
from_. & 1.00000 \nonumber\\
ProductionRule_NP->DT,ADJP, & 1.00000 \nonumber\\
belong & 1.00000 \nonumber\\
if_two & 1.00000 \nonumber\\
toolbar_and & 1.00000 \nonumber\\
learn_not & 1.00000 \nonumber\\
determine & 1.00000 \nonumber\\
suck_. & 1.00000 \nonumber\\
found & 1.00000 \nonumber\\
own_hand & 1.00000 \nonumber\\
for_singapore & 1.00000 \nonumber\\
._let & 1.00000 \nonumber\\
ProductionRule_VP->VB,PRT,PP, & 1.00000 \nonumber\\
of_would & 1.00000 \nonumber\\
support_her & 1.00000 \nonumber\\
,_something & 1.00000 \nonumber\\
mistake_she & 1.00000 \nonumber\\
keep_to & 1.00000 \nonumber\\
absolutely_not & 1.00000 \nonumber\\
what_! & 1.00000 \nonumber\\
definitely_learn & 1.00000 \nonumber\\
definitely_support & 1.00000 \nonumber\\
its_something & 1.00000 \nonumber\\
easy_for & 1.00000 \nonumber\\
strongly_doubt & 1.00000 \nonumber\\
not_easy & 1.00000 \nonumber\\
._anyone & 1.00000 \nonumber\\
to_themselve & 1.00000 \nonumber\\
doubt_, & 1.00000 \nonumber\\
strong_enough & 1.00000 \nonumber\\
something_not & 1.00000 \nonumber\\
of_just & 1.00000 \nonumber\\
would_of & 1.00000 \nonumber\\
and_something & 1.00000 \nonumber\\
!_absolutely & 1.00000 \nonumber\\
ever_happen & 1.00000 \nonumber\\
something_she & 1.00000 \nonumber\\
argument_, & 1.00000 \nonumber\\
time_in & 1.00000 \nonumber\\
pollution & 1.00000 \nonumber\\
bind & 1.00000 \nonumber\\
not_wrong & 1.00000 \nonumber\\
requirement & 1.00000 \nonumber\\
great_. & 1.00000 \nonumber\\
think_if & 1.00000 \nonumber\\
_pos_ngram_PR_ADV_NN & 1.00000 \nonumber\\
'_just & 1.00000 \nonumber\\
supporter & 1.00000 \nonumber\\
i_could & 1.00000 \nonumber\\
when_ff & 1.00000 \nonumber\\
them_self & 1.00000 \nonumber\\
push & 1.00000 \nonumber\\
a_gay & 1.00001 \nonumber\\
be_overlook & 1.00001 \nonumber\\
you_as & 1.00001 \nonumber\\
ProductionRule_VP->VBG,IN, & 1.00001 \nonumber\\
commit_this & 1.00001 \nonumber\\
ProductionRule_VP->VB,,,S, & 1.00001 \nonumber\\
this_crime & 1.00001 \nonumber\\
responsible_as & 1.00001 \nonumber\\
overlook & 1.00001 \nonumber\\
ProductionRule_ADJP->RB,RB,JJ,PP, & 1.00001 \nonumber\\
much_responsible & 1.00001 \nonumber\\
murder_of & 1.00001 \nonumber\\
about_make & 1.00001 \nonumber\\
overlook_, & 1.00001 \nonumber\\
sound & 1.00001 \nonumber\\
'_come & 1.00001 \nonumber\\
legal_to & 1.00001 \nonumber\\
against_that & 1.00001 \nonumber\\
baby_while & 1.00001 \nonumber\\
nebraska & 1.00001 \nonumber\\
'_legal & 1.00001 \nonumber\\
by_kill & 1.00001 \nonumber\\
abortion_by & 1.00001 \nonumber\\
womb_. & 1.00001 \nonumber\\
in_nebraska & 1.00001 \nonumber\\
nebraska_, & 1.00001 \nonumber\\
be_impossible & 1.00001 \nonumber\\
largest_man & 1.00001 \nonumber\\
proud_to & 1.00001 \nonumber\\
of_hope & 1.00001 \nonumber\\
power_n & 1.00001 \nonumber\\
n_be & 1.00001 \nonumber\\
n_for & 1.00001 \nonumber\\
n_we & 1.00001 \nonumber\\
ProductionRule_PP->JJ,IN,SQ, & 1.00001 \nonumber\\
country_full & 1.00001 \nonumber\\
n_third & 1.00001 \nonumber\\
r_proud & 1.00001 \nonumber\\
the_king & 1.00001 \nonumber\\
n_it & 1.00001 \nonumber\\
every_manner & 1.00001 \nonumber\\
even_34 & 1.00001 \nonumber\\
impossible_, & 1.00001 \nonumber\\
aspiration & 1.00001 \nonumber\\
hope_n & 1.00001 \nonumber\\
third_largest & 1.00001 \nonumber\\
second_largest & 1.00001 \nonumber\\
34_% & 1.00001 \nonumber\\
for_indian & 1.00001 \nonumber\\
king_of & 1.00001 \nonumber\\
man_power & 1.00001 \nonumber\\
aspiration_n & 1.00001 \nonumber\\
lead_because & 1.00001 \nonumber\\
indian_n & 1.00001 \nonumber\\
34 & 1.00001 \nonumber\\
n_aspiration & 1.00001 \nonumber\\
indian_nothing & 1.00001 \nonumber\\
,_n & 1.00001 \nonumber\\
ProductionRule_ADJP->NN,S, & 1.00001 \nonumber\\
world_n & 1.00001 \nonumber\\
ProductionRule_NP->DT,ADJP,NN,NN,NN,ADJP,NN, & 1.00001 \nonumber\\
ProductionRule_SQ->VP,NP,PRN,SBAR, & 1.00001 \nonumber\\
every_father & 1.00001 \nonumber\\
as_an & 1.00001 \nonumber\\
be_bind & 1.00001 \nonumber\\
firstly & 1.00001 \nonumber\\
._firstly & 1.00001 \nonumber\\
try_. & 1.00001 \nonumber\\
_pos_ngram_ART_CARD_O & 1.00001 \nonumber\\
bar & 1.00001 \nonumber\\
that_their & 1.00001 \nonumber\\
!!!! & 1.00001 \nonumber\\
_pos_ngram_ADV_ART_PUNC & 1.00001 \nonumber\\
who_love & 1.00001 \nonumber\\
life_that & 1.00001 \nonumber\\
proper & 1.00001 \nonumber\\
beside_just & 1.00001 \nonumber\\
it_go & 1.00001 \nonumber\\
be_know & 1.00001 \nonumber\\
_pos_ngram_V_PP_O & 1.00001 \nonumber\\
the_murder & 1.00001 \nonumber\\
be_this & 1.00001 \nonumber\\
ProductionRule_ADVP->NP,RB, & 1.00001 \nonumber\\
_pos_ngram_PR_PP_NP & 1.00001 \nonumber\\
ProductionRule_NP->NP,JJ,NN, & 1.00001 \nonumber\\
to_follow & 1.00001 \nonumber\\
than_not & 1.00001 \nonumber\\
memory_. & 1.00001 \nonumber\\
the_singapore & 1.00001 \nonumber\\
girl & 1.00001 \nonumber\\
city & 1.00001 \nonumber\\
respectable & 1.00001 \nonumber\\
_pos_ngram_PR_ART_O & 1.00001 \nonumber\\
restart & 1.00001 \nonumber\\
yes_it & 1.00001 \nonumber\\
condition & 1.00001 \nonumber\\
child_that & 1.00001 \nonumber\\
faster_, & 1.00001 \nonumber\\
_pos_ngram_PUNC_NN_ADJ & 1.00001 \nonumber\\
we_need & 1.00001 \nonumber\\
,_my & 1.00001 \nonumber\\
to_keep & 1.00001 \nonumber\\
site & 1.00001 \nonumber\\
farquhar_as & 1.00001 \nonumber\\
people_recognize & 1.00001 \nonumber\\
clear & 1.00001 \nonumber\\
out_great & 1.00001 \nonumber\\
commercial & 1.00001 \nonumber\\
ProductionRule_NP->QP,NNS, & 1.00001 \nonumber\\
ProductionRule_NP->NNS,NN, & 1.00001 \nonumber\\
have_an & 1.00001 \nonumber\\
a_founder & 1.00001 \nonumber\\
the_man & 1.00001 \nonumber\\
not_how & 1.00001 \nonumber\\
week & 1.00001 \nonumber\\
one_just & 1.00001 \nonumber\\
,_our & 1.00001 \nonumber\\
pretty_much & 1.00001 \nonumber\\
couple & 1.00001 \nonumber\\
i_use & 1.00001 \nonumber\\
recognize & 1.00001 \nonumber\\
to_student & 1.00001 \nonumber\\
on_other & 1.00001 \nonumber\\
ProductionRule_SBAR->X,S, & 1.00001 \nonumber\\
tv_, & 1.00001 \nonumber\\
problem_of & 1.00001 \nonumber\\
protection & 1.00001 \nonumber\\
take_away & 1.00001 \nonumber\\
be_find & 1.00001 \nonumber\\
subject & 1.00001 \nonumber\\
_pos_ngram_CONJ_PR_ADJ & 1.00001 \nonumber\\
way_bigger & 1.00001 \nonumber\\
membership_of & 1.00001 \nonumber\\
membership & 1.00001 \nonumber\\
atheist_here & 1.00001 \nonumber\\
the_congregation & 1.00001 \nonumber\\
the_underdog & 1.00001 \nonumber\\
root_for & 1.00001 \nonumber\\
bigger_. & 1.00001 \nonumber\\
congregation & 1.00001 \nonumber\\
just_look & 1.00001 \nonumber\\
underdog & 1.00001 \nonumber\\
underdog_. & 1.00001 \nonumber\\
alway_root & 1.00001 \nonumber\\
congregation_of & 1.00001 \nonumber\\
the_membership & 1.00001 \nonumber\\
root & 1.00001 \nonumber\\
they_must & 1.00001 \nonumber\\
just_so & 1.00001 \nonumber\\
better_as & 1.00001 \nonumber\\
of_physical & 1.00001 \nonumber\\
btw & 1.00001 \nonumber\\
murder_and & 1.00001 \nonumber\\
work_, & 1.00001 \nonumber\\
agnostic & 1.00001 \nonumber\\
n't_good & 1.00001 \nonumber\\
to_hide & 1.00001 \nonumber\\
this_common & 1.00001 \nonumber\\
must_at & 1.00001 \nonumber\\
say_have & 1.00001 \nonumber\\
all_pseudo-science & 1.00001 \nonumber\\
._none & 1.00001 \nonumber\\
sean & 1.00001 \nonumber\\
what_sean & 1.00001 \nonumber\\
to_debate & 1.00001 \nonumber\\
._http://pasadena.wr.usgs.gov/office/ganderson/es10/lectures/lecture01/sci.method.jpg & 1.00001 \nonumber\\
method_down & 1.00001 \nonumber\\
a_theological & 1.00001 \nonumber\\
science_never & 1.00001 \nonumber\\
science_of & 1.00001 \nonumber\\
about_theology & 1.00001 \nonumber\\
sean_say & 1.00001 \nonumber\\
theology_. & 1.00001 \nonumber\\
dont_try & 1.00001 \nonumber\\
understand_if & 1.00001 \nonumber\\
theology & 1.00001 \nonumber\\
creationist_argument & 1.00001 \nonumber\\
hide_it & 1.00001 \nonumber\\
least_get & 1.00001 \nonumber\\
common_view & 1.00001 \nonumber\\
theological_view & 1.00001 \nonumber\\
the_science & 1.00001 \nonumber\\
of_water & 1.00001 \nonumber\\
to_judge & 1.00001 \nonumber\\
they_feel & 1.00001 \nonumber\\
poor_, & 1.00001 \nonumber\\
live_with & 1.00001 \nonumber\\
jobs/apple_? & 1.00001 \nonumber\\
?_seperate & 1.00001 \nonumber\\
do_or & 1.00001 \nonumber\\
enitity_, & 1.00001 \nonumber\\
,_ie & 1.00001 \nonumber\\
ie_ever & 1.00001 \nonumber\\
consortium_standard & 1.00001 \nonumber\\
when_make & 1.00001 \nonumber\\
with_steve & 1.00001 \nonumber\\
!_btw & 1.00001 \nonumber\\
ie_blow & 1.00001 \nonumber\\
look_right & 1.00001 \nonumber\\
much_closer & 1.00001 \nonumber\\
or_will & 1.00001 \nonumber\\
page_and & 1.00001 \nonumber\\
jobs/apple & 1.00001 \nonumber\\
get_thing & 1.00001 \nonumber\\
make_page & 1.00001 \nonumber\\
enitity & 1.00001 \nonumber\\
ff/mozilla & 1.00001 \nonumber\\
wide_web & 1.00001 \nonumber\\
about_ff/mozilla & 1.00001 \nonumber\\
standard_much & 1.00001 \nonumber\\
world_wide & 1.00001 \nonumber\\
bite_attach & 1.00001 \nonumber\\
wide & 1.00001 \nonumber\\
ff/mozilla_have & 1.00001 \nonumber\\
web_consortium & 1.00001 \nonumber\\
blow_when & 1.00001 \nonumber\\
attach & 1.00001 \nonumber\\
attach_! & 1.00001 \nonumber\\
seperate & 1.00001 \nonumber\\
to_world & 1.00001 \nonumber\\
closer_than & 1.00001 \nonumber\\
ff_stick & 1.00001 \nonumber\\
steve_jobs/apple & 1.00001 \nonumber\\
seperate_enitity & 1.00001 \nonumber\\
closer & 1.00001 \nonumber\\
btw_, & 1.00001 \nonumber\\
stick_to & 1.00001 \nonumber\\
least_bite & 1.00001 \nonumber\\
consortium & 1.00001 \nonumber\\
and_sometime & 1.00001 \nonumber\\
better_the & 1.00001 \nonumber\\
ProductionRule_S->NP,,,ADVP,,,VP,., & 1.00001 \nonumber\\
approach & 1.00001 \nonumber\\
be_porn & 1.00001 \nonumber\\
run_. & 1.00001 \nonumber\\
environment_as & 1.00001 \nonumber\\
scale & 1.00001 \nonumber\\
lead_" & 1.00001 \nonumber\\
i_ca & 1.00001 \nonumber\\
not_itself & 1.00001 \nonumber\\
country_must & 1.00001 \nonumber\\
tension_between & 1.00001 \nonumber\\
conflict_, & 1.00001 \nonumber\\
tension & 1.00001 \nonumber\\
scale_internal & 1.00001 \nonumber\\
but_right & 1.00001 \nonumber\\
nation_that & 1.00001 \nonumber\\
muslim_and & 1.00001 \nonumber\\
internal_conflict & 1.00001 \nonumber\\
between_muslim & 1.00001 \nonumber\\
itself_. & 1.00001 \nonumber\\
large_scale & 1.00001 \nonumber\\
current_religious & 1.00001 \nonumber\\
religious_tension & 1.00001 \nonumber\\
and_resource & 1.00001 \nonumber\\
lead_nation & 1.00001 \nonumber\\
the_current & 1.00001 \nonumber\\
"_lead & 1.00001 \nonumber\\
now_the & 1.00001 \nonumber\\
hindu_would & 1.00001 \nonumber\\
potential_, & 1.00001 \nonumber\\
hindu & 1.00001 \nonumber\\
prevent_this & 1.00001 \nonumber\\
probably_prevent & 1.00001 \nonumber\\
and_hindu & 1.00001 \nonumber\\
have_large & 1.00001 \nonumber\\
ProductionRule_NP->NNPS,CC,NNPS, & 1.00001 \nonumber\\
wouldnt_want & 1.00001 \nonumber\\
drastically & 1.00001 \nonumber\\
ProductionRule_NP->DT,NN,POS, & 1.00001 \nonumber\\
web & 1.00001 \nonumber\\
to_survive & 1.00001 \nonumber\\
then_yes & 1.00001 \nonumber\\
ProductionRule_NP->NNP,CD, & 1.00001 \nonumber\\
catholic & 1.00001 \nonumber\\
'_? & 1.00001 \nonumber\\
_pos_ngram_PUNC_V_PUNC & 1.00001 \nonumber\\
create_in & 1.00001 \nonumber\\
christian_. & 1.00001 \nonumber\\
call_it & 1.00001 \nonumber\\
_pos_ngram_PR_ADV_CONJ & 1.00001 \nonumber\\
lazy & 1.00001 \nonumber\\
person_' & 1.00001 \nonumber\\
course_it & 1.00001 \nonumber\\
you_feel & 1.00001 \nonumber\\
faster_than & 1.00001 \nonumber\\
a_small & 1.00001 \nonumber\\
wrong_then & 1.00001 \nonumber\\
becasue_it & 1.00001 \nonumber\\
becasue & 1.00001 \nonumber\\
_pos_ngram_NN_PR_ART & 1.00001 \nonumber\\
child_should & 1.00001 \nonumber\\
look_up & 1.00001 \nonumber\\
will_lead & 1.00001 \nonumber\\
?_no & 1.00001 \nonumber\\
find_the & 1.00001 \nonumber\\
important_then & 1.00001 \nonumber\\
world_you & 1.00001 \nonumber\\
plus_not & 1.00001 \nonumber\\
_pos_ngram_NP_ADV_ART & 1.00001 \nonumber\\
yourself_then & 1.00001 \nonumber\\
need_, & 1.00001 \nonumber\\
its_easier & 1.00001 \nonumber\\
pursuit_first & 1.00001 \nonumber\\
other_need & 1.00001 \nonumber\\
fight_for & 1.00001 \nonumber\\
all_people & 1.00001 \nonumber\\
out_the & 1.00001 \nonumber\\
there_or & 1.00001 \nonumber\\
abort_a & 1.00001 \nonumber\\
dutch & 1.00001 \nonumber\\
absolutely & 1.00001 \nonumber\\
interaction & 1.00001 \nonumber\\
they_wont & 1.00001 \nonumber\\
spank_their & 1.00001 \nonumber\\
view_of & 1.00001 \nonumber\\
lead_to & 1.00001 \nonumber\\
not_all & 1.00001 \nonumber\\
den & 1.00001 \nonumber\\
girl_' & 1.00001 \nonumber\\
,_this & 1.00001 \nonumber\\
firefox_user & 1.00001 \nonumber\\
people_will & 1.00001 \nonumber\\
be_indian & 1.00001 \nonumber\\
._farquhar & 1.00001 \nonumber\\
_pos_ngram_PUNC_NP_ADV & 1.00001 \nonumber\\
positive & 1.00001 \nonumber\\
_pos_ngram_ART_O_NP & 1.00001 \nonumber\\
but_when & 1.00001 \nonumber\\
their_own & 1.00001 \nonumber\\
woman_that & 1.00001 \nonumber\\
_pos_ngram_ADJ_PP_O & 1.00001 \nonumber\\
as_human & 1.00001 \nonumber\\
ProductionRule_S->ADVP,NP,VP, & 1.00001 \nonumber\\
._secondly & 1.00001 \nonumber\\
secondly & 1.00001 \nonumber\\
i_spend & 1.00001 \nonumber\\
resource_to & 1.00001 \nonumber\\
but_every & 1.00001 \nonumber\\
a_good & 1.00001 \nonumber\\
be_spank & 1.00001 \nonumber\\
manner_. & 1.00001 \nonumber\\
manner & 1.00001 \nonumber\\
consumption & 1.00001 \nonumber\\
good_when & 1.00001 \nonumber\\
issue_be & 1.00001 \nonumber\\
this_issue & 1.00001 \nonumber\\
"_in & 1.00001 \nonumber\\
'_economy & 1.00001 \nonumber\\
_pos_ngram_PP_O_NP & 1.00001 \nonumber\\
can_use & 1.00001 \nonumber\\
ProductionRule_PP->TO,S, & 1.00001 \nonumber\\
toy_. & 1.00001 \nonumber\\
toy & 1.00001 \nonumber\\
in_this & 1.00001 \nonumber\\
what_i & 1.00001 \nonumber\\
one_, & 1.00001 \nonumber\\
he_look & 1.00001 \nonumber\\
tell_that & 1.00001 \nonumber\\
_pos_ngram_CONJ_O_ADV & 1.00001 \nonumber\\
kid_to & 1.00001 \nonumber\\
yourself_before & 1.00001 \nonumber\\
pursuit_because & 1.00001 \nonumber\\
freedom & 1.00001 \nonumber\\
read_: & 1.00001 \nonumber\\
he_think & 1.00001 \nonumber\\
her_. & 1.00001 \nonumber\\
catch & 1.00001 \nonumber\\
right_thing & 1.00001 \nonumber\\
ProductionRule_VP->VB,PRT,NP, & 1.00001 \nonumber\\
_pos_ngram_NN_ADJ_V & 1.00001 \nonumber\\
support_, & 1.00001 \nonumber\\
the_two & 1.00001 \nonumber\\
but_in & 1.00001 \nonumber\\
do_just & 1.00001 \nonumber\\
spouse_commit & 1.00001 \nonumber\\
usa & 1.00001 \nonumber\\
english & 1.00001 \nonumber\\
action_. & 1.00001 \nonumber\\
_pos_ngram_V_O_NP & 1.00001 \nonumber\\
may_not & 1.00001 \nonumber\\
ProductionRule_VP->VBD,ADVP, & 1.00001 \nonumber\\
thought & 1.00001 \nonumber\\
your_thought & 1.00001 \nonumber\\
cuz_i & 1.00001 \nonumber\\
and_cram & 1.00001 \nonumber\\
for_morality & 1.00001 \nonumber\\
a_platform & 1.00001 \nonumber\\
fly_) & 1.00001 \nonumber\\
(_think & 1.00001 \nonumber\\
'_throat & 1.00001 \nonumber\\
the_fly & 1.00001 \nonumber\\
kid_' & 1.00001 \nonumber\\
if_morality & 1.00001 \nonumber\\
reward_with & 1.00001 \nonumber\\
cram_it & 1.00001 \nonumber\\
cram & 1.00001 \nonumber\\
do_society & 1.00001 \nonumber\\
to_spew & 1.00001 \nonumber\\
(_lord & 1.00001 \nonumber\\
the_homosexual & 1.00001 \nonumber\\
public_exposure/support & 1.00001 \nonumber\\
platform_to & 1.00001 \nonumber\\
exposure/support_of & 1.00001 \nonumber\\
exposure/support & 1.00001 \nonumber\\
their_garbage & 1.00001 \nonumber\\
this_public & 1.00001 \nonumber\\
in_sin & 1.00001 \nonumber\\
since_homosexuality & 1.00001 \nonumber\\
throat & 1.00001 \nonumber\\
sin_together & 1.00001 \nonumber\\
it_) & 1.00001 \nonumber\\
with_tax & 1.00001 \nonumber\\
sin_( & 1.00001 \nonumber\\
learn_sin & 1.00001 \nonumber\\
garbage & 1.00001 \nonumber\\
spew_their & 1.00001 \nonumber\\
spew & 1.00001 \nonumber\\
garbage_and & 1.00001 \nonumber\\
morality_go & 1.00001 \nonumber\\
throat_. & 1.00001 \nonumber\\
lord_of & 1.00001 \nonumber\\
i_sure & 1.00001 \nonumber\\
down_my & 1.00001 \nonumber\\
civil_union & 1.00001 \nonumber\\
cross & 1.00001 \nonumber\\
way_? & 1.00001 \nonumber\\
he_kill & 1.00001 \nonumber\\
survival & 1.00001 \nonumber\\
one_have & 1.00001 \nonumber\\
_pos_ngram_CARD_CARD_NN & 1.00001 \nonumber\\
get_pregnant & 1.00001 \nonumber\\
soft & 1.00001 \nonumber\\
well_with & 1.00001 \nonumber\\
,_of & 1.00001 \nonumber\\
education_, & 1.00001 \nonumber\\
be_waste & 1.00001 \nonumber\\
union & 1.00001 \nonumber\\
compare_to & 1.00001 \nonumber\\
scare & 1.00001 \nonumber\\
me_have & 1.00001 \nonumber\\
seven & 1.00001 \nonumber\\
not_go & 1.00001 \nonumber\\
father_in & 1.00001 \nonumber\\
yu & 1.00001 \nonumber\\
atheism & 1.00001 \nonumber\\
a_long & 1.00001 \nonumber\\
the_long & 1.00001 \nonumber\\
ProductionRule_NP->NP,,,NP,,,NP,,,NP, & 1.00001 \nonumber\\
country_. & 1.00001 \nonumber\\
be_crazy & 1.00001 \nonumber\\
who_be & 1.00001 \nonumber\\
ProductionRule_PP->IN,ADVP, & 1.00001 \nonumber\\
send_him & 1.00001 \nonumber\\
him_off & 1.00001 \nonumber\\
leave_to & 1.00001 \nonumber\\
_pos_ngram_NN_ADJ_ADJ & 1.00001 \nonumber\\
intelligently & 1.00001 \nonumber\\
intelligently_, & 1.00001 \nonumber\\
east & 1.00001 \nonumber\\
you_truly & 1.00001 \nonumber\\
and_encourage & 1.00001 \nonumber\\
_pos_ngram_PP_NP_CARD & 1.00001 \nonumber\\
that_much & 1.00001 \nonumber\\
clothe_for & 1.00001 \nonumber\\
ready & 1.00001 \nonumber\\
indian_. & 1.00001 \nonumber\\
want_them & 1.00001 \nonumber\\
uniform_, & 1.00001 \nonumber\\
other_hand & 1.00001 \nonumber\\
add_that & 1.00001 \nonumber\\
convenient & 1.00001 \nonumber\\
ProductionRule_SQ->VBZ,NP,ADJP,., & 1.00001 \nonumber\\
have_all & 1.00001 \nonumber\\
_pos_ngram_PUNC_ART_PUNC & 1.00001 \nonumber\\
_pos_ngram_ADV_CARD_CARD & 1.00001 \nonumber\\
two_people & 1.00001 \nonumber\\
they_wo & 1.00001 \nonumber\\
book_. & 1.00001 \nonumber\\
really_want & 1.00001 \nonumber\\
feel_. & 1.00001 \nonumber\\
kill_because & 1.00001 \nonumber\\
convince_him & 1.00001 \nonumber\\
also_depend & 1.00001 \nonumber\\
reason_behind & 1.00001 \nonumber\\
just_cant & 1.00001 \nonumber\\
random_kill & 1.00001 \nonumber\\
behind_him & 1.00001 \nonumber\\
my_place & 1.00001 \nonumber\\
dont_see & 1.00001 \nonumber\\
get_kill & 1.00001 \nonumber\\
him_kill & 1.00001 \nonumber\\
some_random & 1.00001 \nonumber\\
purely & 1.00001 \nonumber\\
to_protect & 1.00001 \nonumber\\
finally & 1.00001 \nonumber\\
the_name & 1.00001 \nonumber\\
t.v. & 1.00001 \nonumber\\
only_one & 1.00001 \nonumber\\
'_fault & 1.00001 \nonumber\\
do_to & 1.00001 \nonumber\\
_pos_ngram_CONJ_PP_ADV & 1.00001 \nonumber\\
a_lead & 1.00001 \nonumber\\
_pos_ngram_CONJ_PP_O & 1.00001 \nonumber\\
ProductionRule_S->NP,NP,VP,., & 1.00001 \nonumber\\
,_than & 1.00001 \nonumber\\
muslim & 1.00001 \nonumber\\
on_an & 1.00001 \nonumber\\
_pos_ngram_ADV_ART_ART & 1.00001 \nonumber\\
spouse_in & 1.00001 \nonumber\\
an_hour & 1.00001 \nonumber\\
_pos_ngram_ART_PUNC_CONJ & 1.00001 \nonumber\\
"_that & 1.00001 \nonumber\\
than_one & 1.00001 \nonumber\\
indirectly & 1.00001 \nonumber\\
someone_, & 1.00001 \nonumber\\
be_quite & 1.00001 \nonumber\\
thing_they & 1.00001 \nonumber\\
let_it & 1.00001 \nonumber\\
* & 1.00001 \nonumber\\
police_. & 1.00001 \nonumber\\
can_feel & 1.00001 \nonumber\\
know_i & 1.00001 \nonumber\\
otherwise & 1.00001 \nonumber\\
correct_. & 1.00001 \nonumber\\
._whether & 1.00001 \nonumber\\
body_, & 1.00001 \nonumber\\
perhap & 1.00001 \nonumber\\
but_at & 1.00001 \nonumber\\
and_take & 1.00001 \nonumber\\
_pos_ngram_PR_ADV_ART & 1.00001 \nonumber\\
survey & 1.00001 \nonumber\\
suit & 1.00001 \nonumber\\
resentment & 1.00001 \nonumber\\
ProductionRule_VP->VB,NP,NP,SBAR, & 1.00001 \nonumber\\
would_definitely & 1.00001 \nonumber\\
accompany & 1.00001 \nonumber\\
between_raffle & 1.00001 \nonumber\\
singapore_treaty & 1.00001 \nonumber\\
accompany_seven & 1.00001 \nonumber\\
seven_ship & 1.00001 \nonumber\\
ship_witness & 1.00001 \nonumber\\
sign_between & 1.00001 \nonumber\\
commandant & 1.00001 \nonumber\\
the_event & 1.00001 \nonumber\\
commandant_under & 1.00001 \nonumber\\
the_accompany & 1.00001 \nonumber\\
with_commandant & 1.00001 \nonumber\\
temenggong_with & 1.00001 \nonumber\\
ProductionRule_NP->NP,,,NP,CC,NP, & 1.00001 \nonumber\\
hussein_and & 1.00001 \nonumber\\
treaty_be & 1.00001 \nonumber\\
event_. & 1.00001 \nonumber\\
be_sign & 1.00001 \nonumber\\
,_sultan & 1.00001 \nonumber\\
event & 1.00001 \nonumber\\
witness_the & 1.00001 \nonumber\\
three & 1.00001 \nonumber\\
against_the & 1.00001 \nonumber\\
,_god & 1.00001 \nonumber\\
contradiction & 1.00001 \nonumber\\
do_believe & 1.00001 \nonumber\\
,_every & 1.00001 \nonumber\\
the_' & 1.00001 \nonumber\\
with_not & 1.00001 \nonumber\\
my_opinion & 1.00001 \nonumber\\
decision_and & 1.00001 \nonumber\\
need_a & 1.00001 \nonumber\\
body_. & 1.00001 \nonumber\\
keep_them & 1.00001 \nonumber\\
detail & 1.00001 \nonumber\\
and_teacher & 1.00001 \nonumber\\
teacher_. & 1.00001 \nonumber\\
student_and & 1.00001 \nonumber\\
this_view & 1.00001 \nonumber\\
firstly_, & 1.00001 \nonumber\\
into_social & 1.00001 \nonumber\\
,_divide & 1.00001 \nonumber\\
show_student & 1.00001 \nonumber\\
when_all & 1.00001 \nonumber\\
in_choose & 1.00001 \nonumber\\
secondly_, & 1.00001 \nonumber\\
any_discrimination & 1.00001 \nonumber\\
problem_what & 1.00001 \nonumber\\
university_.... & 1.00001 \nonumber\\
one_uniform & 1.00001 \nonumber\\
ProductionRule_FRAG->ADJP,,,NP,., & 1.00001 \nonumber\\
me_be & 1.00001 \nonumber\\
uniform_show & 1.00001 \nonumber\\
waste_a & 1.00001 \nonumber\\
ProductionRule_NP->NN,DT,NN, & 1.00001 \nonumber\\
...._i & 1.00001 \nonumber\\
discrimination & 1.00001 \nonumber\\
equality & 1.00001 \nonumber\\
student_equality & 1.00001 \nonumber\\
divide & 1.00001 \nonumber\\
discrimination_, & 1.00001 \nonumber\\
divide_into & 1.00001 \nonumber\\
equality_. & 1.00001 \nonumber\\
status_group & 1.00001 \nonumber\\
spend_too & 1.00001 \nonumber\\
the_university & 1.00001 \nonumber\\
more_, & 1.00001 \nonumber\\
a_very & 1.00001 \nonumber\\
and_thing & 1.00001 \nonumber\\
fly & 1.00001 \nonumber\\
_pos_ngram_ART_CARD_PUNC & 1.00001 \nonumber\\
to_all & 1.00001 \nonumber\\
than_book & 1.00001 \nonumber\\
,_archaeological & 1.00001 \nonumber\\
,_astronomical & 1.00001 \nonumber\\
ProductionRule_ADJP->JJ,,,JJ,,,JJ,,,CC,JJ,JJ, & 1.00001 \nonumber\\
perfect_, & 1.00001 \nonumber\\
an_all & 1.00001 \nonumber\\
(_bar & 1.00001 \nonumber\\
,_creator & 1.00001 \nonumber\\
grind_( & 1.00001 \nonumber\\
powerful_, & 1.00001 \nonumber\\
_pos_ngram_NN_CARD_CONJ & 1.00001 \nonumber\\
,_biological & 1.00001 \nonumber\\
archaeological & 1.00001 \nonumber\\
impartial_common & 1.00001 \nonumber\\
two_, & 1.00001 \nonumber\\
by_an & 1.00001 \nonumber\\
teaching_, & 1.00001 \nonumber\\
impartial & 1.00001 \nonumber\\
with_historical & 1.00001 \nonumber\\
ProductionRule_NP->NP,PP,., & 1.00001 \nonumber\\
&_impartial & 1.00001 \nonumber\\
write_by & 1.00001 \nonumber\\
universe_, & 1.00001 \nonumber\\
not_perfect & 1.00001 \nonumber\\
all_know & 1.00001 \nonumber\\
with_contradiction & 1.00001 \nonumber\\
christianity_conflict & 1.00001 \nonumber\\
christianity_just & 1.00001 \nonumber\\
close_) & 1.00001 \nonumber\\
logical_position & 1.00001 \nonumber\\
creator_of & 1.00001 \nonumber\\
biological_, & 1.00001 \nonumber\\
contradiction_. & 1.00001 \nonumber\\
bar_one & 1.00001 \nonumber\\
archaeological_, & 1.00001 \nonumber\\
deny_rational & 1.00001 \nonumber\\
its_teaching & 1.00001 \nonumber\\
all_powerful & 1.00001 \nonumber\\
more_logical & 1.00001 \nonumber\\
be_fill & 1.00001 \nonumber\\
rational_& & 1.00001 \nonumber\\
be_close & 1.00001 \nonumber\\
ProductionRule_NP->JJ,,,ADJP,NNS, & 1.00001 \nonumber\\
hold_grind & 1.00001 \nonumber\\
it_deny & 1.00001 \nonumber\\
historical_, & 1.00001 \nonumber\\
astronomical_, & 1.00001 \nonumber\\
fault_that & 1.00001 \nonumber\\
more_important & 1.00001 \nonumber\\
their_opinion & 1.00001 \nonumber\\
lack_of & 1.00001 \nonumber\\
topic & 1.00001 \nonumber\\
effect & 1.00001 \nonumber\\
and_other & 1.00001 \nonumber\\
violent & 1.00001 \nonumber\\
_pos_ngram_PP_CONJ_NN & 1.00001 \nonumber\\
electricity & 1.00001 \nonumber\\
_pos_ngram_O_NP_PUNC & 1.00001 \nonumber\\
much_and & 1.00001 \nonumber\\
they_only & 1.00001 \nonumber\\
mile & 1.00001 \nonumber\\
or_just & 1.00001 \nonumber\\
raffle_. & 1.00001 \nonumber\\
_pos_ngram_NP_NN_PR & 1.00001 \nonumber\\
would_you & 1.00001 \nonumber\\
,_firefox & 1.00001 \nonumber\\
http://aynrandlexicon.com/lexicon/religion.html & 1.00001 \nonumber\\
use_, & 1.00001 \nonumber\\
motive_, & 1.00001 \nonumber\\
motive & 1.00001 \nonumber\\
vile & 1.00001 \nonumber\\
vile_ideal & 1.00001 \nonumber\\
be_perhap & 1.00001 \nonumber\\
3956 & 1.00001 \nonumber\\
3956_. & 1.00001 \nonumber\\
._christopher & 1.00001 \nonumber\\
to_poison & 1.00001 \nonumber\\
fictional & 1.00001 \nonumber\\
fictional_story & 1.00001 \nonumber\\
quite_plainly & 1.00001 \nonumber\\
'_use & 1.00001 \nonumber\\
and_fictional & 1.00001 \nonumber\\
most_vile & 1.00001 \nonumber\\
http://aynrandlexicon.com/lexicon/religion.html_) & 1.00001 \nonumber\\
plainly_immoral & 1.00001 \nonumber\\
,_motive & 1.00001 \nonumber\\
http://www.infidels.org/library/modern/richard_) & 1.00001 \nonumber\\
http://www.infidels.org/library/modern/richard & 1.00001 \nonumber\\
christopher_) & 1.00001 \nonumber\\
ideal & 1.00001 \nonumber\\
(_http://www.infidels.org/library/modern/richard & 1.00001 \nonumber\\
ideal_to & 1.00001 \nonumber\\
poison_the & 1.00001 \nonumber\\
immoral & 1.00001 \nonumber\\
(_http://aynrandlexicon.com/lexicon/religion.html & 1.00001 \nonumber\\
http://www.goodreads.com/author/quotes/_3956 & 1.00001 \nonumber\\
perhap_the & 1.00001 \nonumber\\
ProductionRule_NP->DT,ADJP,NN,S, & 1.00001 \nonumber\\
(_http://www.goodreads.com/author/quotes/ & 1.00001 \nonumber\\
poison & 1.00001 \nonumber\\
immoral_. & 1.00001 \nonumber\\
http://www.goodreads.com/author/quotes/ & 1.00001 \nonumber\\
plainly & 1.00001 \nonumber\\
christopher & 1.00001 \nonumber\\
_pos_ngram_CONJ_V_CARD & 1.00001 \nonumber\\
_pos_ngram_ART_CONJ_ART & 1.00001 \nonumber\\
_pos_ngram_O_CONJ_PP & 1.00001 \nonumber\\
add & 1.00001 \nonumber\\
_pos_ngram_CARD_NP & 1.00001 \nonumber\\
mind_of & 1.00001 \nonumber\\
_pos_ngram_PP_PP_O & 1.00001 \nonumber\\
best & 1.00001 \nonumber\\
search & 1.00001 \nonumber\\
debate_the & 1.00001 \nonumber\\
also_i & 1.00001 \nonumber\\
pants & 1.00001 \nonumber\\
and_the & 1.00001 \nonumber\\
other_form & 1.00001 \nonumber\\
day_. & 1.00001 \nonumber\\
n't_spend & 1.00001 \nonumber\\
black & 1.00001 \nonumber\\
be_explain & 1.00001 \nonumber\\
where_to & 1.00001 \nonumber\\
and_maybe & 1.00001 \nonumber\\
wear_one & 1.00001 \nonumber\\
we_could & 1.00001 \nonumber\\
have_kill & 1.00001 \nonumber\\
ProductionRule_VP->VBD,NP,SBAR, & 1.00001 \nonumber\\
have_time & 1.00001 \nonumber\\
case_of & 1.00001 \nonumber\\
just_dont & 1.00001 \nonumber\\
_pos_ngram_NP_PUNC_CARD & 1.00001 \nonumber\\
if_people & 1.00001 \nonumber\\
story_be & 1.00001 \nonumber\\
sit & 1.00001 \nonumber\\
drink_! & 1.00001 \nonumber\\
liquid & 1.00001 \nonumber\\
fat_! & 1.00001 \nonumber\\
portable_drink & 1.00001 \nonumber\\
if_bottle & 1.00001 \nonumber\\
only_portable & 1.00001 \nonumber\\
drink_sweeten & 1.00001 \nonumber\\
liquid_becasue & 1.00001 \nonumber\\
sweeten & 1.00001 \nonumber\\
water_do & 1.00001 \nonumber\\
portable & 1.00001 \nonumber\\
sweeten_liquid & 1.00001 \nonumber\\
ProductionRule_VP->VBG,CC,VBG,NP,PP, & 1.00001 \nonumber\\
and_buy & 1.00001 \nonumber\\
ProductionRule_NP->NN,,,JJ,NNS, & 1.00001 \nonumber\\
attendance & 1.00001 \nonumber\\
girl_. & 1.00001 \nonumber\\
,_espeacilly & 1.00001 \nonumber\\
spend_a & 1.00001 \nonumber\\
buy_clothe & 1.00001 \nonumber\\
espeacilly & 1.00001 \nonumber\\
because_school & 1.00001 \nonumber\\
attendance_and & 1.00001 \nonumber\\
student_attendance & 1.00001 \nonumber\\
for_school & 1.00001 \nonumber\\
uniform_improve & 1.00001 \nonumber\\
improve_student & 1.00001 \nonumber\\
espeacilly_girl & 1.00001 \nonumber\\
_pos_ngram_PUNC_PP_PUNC & 1.00001 \nonumber\\
you_better & 1.00001 \nonumber\\
the_gap & 1.00001 \nonumber\\
fatherless_and & 1.00001 \nonumber\\
into_a & 1.00001 \nonumber\\
say_yes & 1.00001 \nonumber\\
child_do & 1.00001 \nonumber\\
light & 1.00001 \nonumber\\
work_out & 1.00001 \nonumber\\
woman_, & 1.00001 \nonumber\\
_pos_ngram_V_PUNC_PUNC & 1.00001 \nonumber\\
and_may & 1.00001 \nonumber\\
they_try & 1.00001 \nonumber\\
_pos_ngram_O_CARD_CARD & 1.00001 \nonumber\\
)_( & 1.00001 \nonumber\\
brain & 1.00001 \nonumber\\
ProductionRule_ADJP->RB,DT, & 1.00001 \nonumber\\
each_and & 1.00001 \nonumber\\
and_every & 1.00001 \nonumber\\
people_would & 1.00001 \nonumber\\
people_make & 1.00001 \nonumber\\
be_reward & 1.00001 \nonumber\\
together_, & 1.00001 \nonumber\\
pair & 1.00001 \nonumber\\
when_it & 1.00001 \nonumber\\
the_opportunity & 1.00001 \nonumber\\
i_might & 1.00001 \nonumber\\
moment_, & 1.00001 \nonumber\\
ProductionRule_ADVP->ADVP,SBAR, & 1.00001 \nonumber\\
ProductionRule_VP->VB,PRT,S, & 1.00001 \nonumber\\
someone_to & 1.00001 \nonumber\\
choose_and & 1.00001 \nonumber\\
tell_you & 1.00001 \nonumber\\
ProductionRule_NP->NNS,POS, & 1.00001 \nonumber\\
ProductionRule_NP->DT,FW,FW, & 1.00001 \nonumber\\
_pos_ngram_O_V_ADJ & 1.00001 \nonumber\\
harmful & 1.00001 \nonumber\\
casual & 1.00001 \nonumber\\
_pos_ngram_O_ADV_PP & 1.00001 \nonumber\\
ProductionRule_S->S,,,NP,VP, & 1.00001 \nonumber\\
as_science & 1.00001 \nonumber\\
_pos_ngram_PP_ADV_O & 1.00001 \nonumber\\
and_mold & 1.00001 \nonumber\\
mold & 1.00001 \nonumber\\
both & 1.00001 \nonumber\\
if_be & 1.00001 \nonumber\\
_pos_ngram_NP_NN_NN & 1.00001 \nonumber\\
make_student & 1.00001 \nonumber\\
hard_to & 1.00001 \nonumber\\
destroy & 1.00001 \nonumber\\
know_the & 1.00001 \nonumber\\
the_health & 1.00001 \nonumber\\
the_kid & 1.00001 \nonumber\\
rational & 1.00001 \nonumber\\
to_commit & 1.00001 \nonumber\\
student_wear & 1.00001 \nonumber\\
most_likely & 1.00001 \nonumber\\
other_country & 1.00001 \nonumber\\
to_jesus & 1.00001 \nonumber\\
have_happen & 1.00001 \nonumber\\
,_some & 1.00001 \nonumber\\
then_read & 1.00001 \nonumber\\
child_' & 1.00001 \nonumber\\
_pos_ngram_NN_NP_PUNC & 1.00001 \nonumber\\
of_, & 1.00001 \nonumber\\
not_exist & 1.00001 \nonumber\\
rest & 1.00001 \nonumber\\
because_in & 1.00001 \nonumber\\
time_to & 1.00001 \nonumber\\
_pos_ngram_PUNC_PUNC_CONJ & 1.00001 \nonumber\\
one_or & 1.00001 \nonumber\\
international & 1.00001 \nonumber\\
deep & 1.00001 \nonumber\\
_pos_ngram_ART_O_ADJ & 1.00001 \nonumber\\
,_she & 1.00001 \nonumber\\
_pos_ngram_V_PP_CARD & 1.00001 \nonumber\\
my_brother & 1.00001 \nonumber\\
violence & 1.00001 \nonumber\\
move_away & 1.00001 \nonumber\\
..._its & 1.00001 \nonumber\\
i_understand & 1.00001 \nonumber\\
"_god & 1.00001 \nonumber\\
clothe_every & 1.00001 \nonumber\\
choose_clothe & 1.00001 \nonumber\\
use_it & 1.00001 \nonumber\\
already & 1.00001 \nonumber\\
appear & 1.00001 \nonumber\\
ProductionRule_VP->VBD,ADJP, & 1.00001 \nonumber\\
kill_a & 1.00001 \nonumber\\
ProductionRule_PRN->S,,, & 1.00001 \nonumber\\
order & 1.00001 \nonumber\\
the_position & 1.00001 \nonumber\\
position_of & 1.00001 \nonumber\\
singapore_, & 1.00001 \nonumber\\
harm_to & 1.00001 \nonumber\\
change_other & 1.00001 \nonumber\\
couple_make & 1.00001 \nonumber\\
feeling_and & 1.00001 \nonumber\\
._meanwhile & 1.00001 \nonumber\\
like_gay & 1.00001 \nonumber\\
meanwhile_, & 1.00001 \nonumber\\
change_there & 1.00001 \nonumber\\
other_base & 1.00001 \nonumber\\
tell_people & 1.00001 \nonumber\\
your_belief & 1.00001 \nonumber\\
be_entitle & 1.00001 \nonumber\\
meanwhile & 1.00001 \nonumber\\
their_veiw & 1.00001 \nonumber\\
apparently & 1.00001 \nonumber\\
but_keep & 1.00001 \nonumber\\
incorrect & 1.00001 \nonumber\\
entitle & 1.00001 \nonumber\\
entitle_to & 1.00001 \nonumber\\
self_rights & 1.00001 \nonumber\\
veiw_be & 1.00001 \nonumber\\
be_incorrect & 1.00001 \nonumber\\
that_apparently & 1.00001 \nonumber\\
must_change & 1.00001 \nonumber\\
veiw & 1.00001 \nonumber\\
not_watch & 1.00001 \nonumber\\
away_self & 1.00001 \nonumber\\
apparently_they & 1.00001 \nonumber\\
incorrect_and & 1.00001 \nonumber\\
watch_a & 1.00001 \nonumber\\
than_ie & 1.00001 \nonumber\\
can_watch & 1.00001 \nonumber\\
sin & 1.00001 \nonumber\\
the_poor & 1.00001 \nonumber\\
know_about & 1.00001 \nonumber\\
life_? & 1.00001 \nonumber\\
especially_if & 1.00001 \nonumber\\
on_their & 1.00001 \nonumber\\
n't_really & 1.00001 \nonumber\\
:_you & 1.00001 \nonumber\\
ff & 1.00001 \nonumber\\
as_much & 1.00001 \nonumber\\
_pos_ngram_NN_PUNC_ADJ & 1.00001 \nonumber\\
shoe & 1.00001 \nonumber\\
produce & 1.00001 \nonumber\\
so_do & 1.00001 \nonumber\\
them_as & 1.00001 \nonumber\\
theological & 1.00001 \nonumber\\
pseudo-science & 1.00001 \nonumber\\
pseudo-science_. & 1.00001 \nonumber\\
method & 1.00001 \nonumber\\
with_science & 1.00001 \nonumber\\
scientific_method & 1.00001 \nonumber\\
method_. & 1.00001 \nonumber\\
woman_' & 1.00001 \nonumber\\
_pos_ngram_NP_PUNC_O & 1.00001 \nonumber\\
._kid & 1.00001 \nonumber\\
only_thing & 1.00001 \nonumber\\
porn_. & 1.00001 \nonumber\\
school_. & 1.00001 \nonumber\\
tv_because & 1.00001 \nonumber\\
ProductionRule_NP->DT,PRP, & 1.00001 \nonumber\\
never_have & 1.00001 \nonumber\\
to_live & 1.00001 \nonumber\\
would_do & 1.00001 \nonumber\\
my_personal & 1.00001 \nonumber\\
_pos_ngram_CARD_PP_ADJ & 1.00001 \nonumber\\
compatible & 1.00001 \nonumber\\
still_evolve & 1.00001 \nonumber\\
different_, & 1.00001 \nonumber\\
just_ca & 1.00001 \nonumber\\
to_better & 1.00001 \nonumber\\
fatherly & 1.00001 \nonumber\\
day_i & 1.00001 \nonumber\\
'_life & 1.00001 \nonumber\\
brand & 1.00001 \nonumber\\
be_about & 1.00001 \nonumber\\
what_to & 1.00001 \nonumber\\
still_a & 1.00001 \nonumber\\
book_have & 1.00001 \nonumber\\
ghost_story & 1.00001 \nonumber\\
explain_and & 1.00001 \nonumber\\
these_book & 1.00001 \nonumber\\
ghost & 1.00001 \nonumber\\
last_i & 1.00001 \nonumber\\
anything_we & 1.00001 \nonumber\\
detail_briefly & 1.00001 \nonumber\\
every_detail & 1.00001 \nonumber\\
at_last & 1.00001 \nonumber\\
etc_these & 1.00001 \nonumber\\
,_fairy & 1.00001 \nonumber\\
sometime_we & 1.00001 \nonumber\\
power_in & 1.00001 \nonumber\\
because_book & 1.00001 \nonumber\\
it_easily & 1.00001 \nonumber\\
book_like & 1.00001 \nonumber\\
tale & 1.00001 \nonumber\\
forget_anything & 1.00001 \nonumber\\
and_much & 1.00001 \nonumber\\
we_forget & 1.00001 \nonumber\\
imaginary & 1.00001 \nonumber\\
imaginary_power & 1.00001 \nonumber\\
ProductionRule_ADJP->DT,CC,DT, & 1.00001 \nonumber\\
cant_remember & 1.00001 \nonumber\\
story_etc & 1.00001 \nonumber\\
can_now & 1.00001 \nonumber\\
only_want & 1.00001 \nonumber\\
remember_it & 1.00001 \nonumber\\
like_story & 1.00001 \nonumber\\
,_ghost & 1.00001 \nonumber\\
us_in & 1.00001 \nonumber\\
only_some & 1.00001 \nonumber\\
bring_imaginary & 1.00001 \nonumber\\
in_bring & 1.00001 \nonumber\\
briefly_. & 1.00001 \nonumber\\
briefly & 1.00001 \nonumber\\
tv_only & 1.00001 \nonumber\\
story_book & 1.00001 \nonumber\\
in_tv & 1.00001 \nonumber\\
now_and & 1.00001 \nonumber\\
in_us & 1.00001 \nonumber\\
fairy_tale & 1.00001 \nonumber\\
have_each & 1.00001 \nonumber\\
book_help & 1.00001 \nonumber\\
tale_, & 1.00001 \nonumber\\
fairy & 1.00001 \nonumber\\
easily_but & 1.00001 \nonumber\\
._raffle & 1.00001 \nonumber\\
them_be & 1.00001 \nonumber\\
the_more & 1.00001 \nonumber\\
respect & 1.00001 \nonumber\\
model & 1.00001 \nonumber\\
role_model & 1.00001 \nonumber\\
be_between & 1.00001 \nonumber\\
ProductionRule_NP->DT,NNP,NN, & 1.00001 \nonumber\\
of_evidence & 1.00001 \nonumber\\
one_that & 1.00001 \nonumber\\
and_do & 1.00001 \nonumber\\
'_very & 1.00001 \nonumber\\
do_more & 1.00001 \nonumber\\
'_like & 1.00001 \nonumber\\
2 & 1.00001 \nonumber\\
creator & 1.00001 \nonumber\\
an_abortion & 1.00001 \nonumber\\
parent_and & 1.00001 \nonumber\\
the_house & 1.00001 \nonumber\\
but_abuse & 1.00001 \nonumber\\
deed_. & 1.00001 \nonumber\\
while_for & 1.00001 \nonumber\\
honest_. & 1.00001 \nonumber\\
do_its & 1.00001 \nonumber\\
touch_fire & 1.00001 \nonumber\\
and_kid & 1.00001 \nonumber\\
than_harm & 1.00001 \nonumber\\
never_good & 1.00001 \nonumber\\
may_do & 1.00001 \nonumber\\
like_touch & 1.00001 \nonumber\\
for_worse & 1.00001 \nonumber\\
fire_to & 1.00001 \nonumber\\
abuse_be & 1.00001 \nonumber\\
be_honest & 1.00001 \nonumber\\
on_parent & 1.00001 \nonumber\\
more_good & 1.00001 \nonumber\\
job_it & 1.00001 \nonumber\\
worse_deed & 1.00001 \nonumber\\
its_job & 1.00001 \nonumber\\
good_than & 1.00001 \nonumber\\
use_protection & 1.00001 \nonumber\\
protection_. & 1.00001 \nonumber\\
ProductionRule_NP->DT,NN,RB, & 1.00001 \nonumber\\
everyone_be & 1.00001 \nonumber\\
cant_be & 1.00001 \nonumber\\
to_society & 1.00001 \nonumber\\
along_with & 1.00001 \nonumber\\
hate & 1.00001 \nonumber\\
if_that & 1.00001 \nonumber\\
_pos_ngram_ADV_NP_V & 1.00001 \nonumber\\
to_study & 1.00001 \nonumber\\
so_if & 1.00001 \nonumber\\
ari & 1.00001 \nonumber\\
duty & 1.00001 \nonumber\\
be_around & 1.00001 \nonumber\\
that_have & 1.00001 \nonumber\\
quite & 1.00001 \nonumber\\
not_so & 1.00001 \nonumber\\
_pos_ngram_NN_V_NN & 1.00001 \nonumber\\
bigger & 1.00001 \nonumber\\
"_be & 1.00001 \nonumber\\
)_and & 1.00001 \nonumber\\
more_time & 1.00001 \nonumber\\
base_on & 1.00001 \nonumber\\
ProductionRule_VP->VBG,PRT, & 1.00001 \nonumber\\
with_them & 1.00001 \nonumber\\
become_fat & 1.00001 \nonumber\\
free & 1.00001 \nonumber\\
have_anything & 1.00001 \nonumber\\
person_, & 1.00001 \nonumber\\
ProductionRule_NP->DT,NNP,CC,NNP, & 1.00001 \nonumber\\
people_while & 1.00001 \nonumber\\
revive_the & 1.00001 \nonumber\\
the_chinese & 1.00001 \nonumber\\
region_by & 1.00001 \nonumber\\
revive & 1.00001 \nonumber\\
the_cultural & 1.00001 \nonumber\\
through_his & 1.00001 \nonumber\\
chinese & 1.00001 \nonumber\\
just_want & 1.00001 \nonumber\\
his_action & 1.00001 \nonumber\\
gain_control & 1.00001 \nonumber\\
heritage_of & 1.00001 \nonumber\\
while_farquhar & 1.00001 \nonumber\\
and_malay & 1.00001 \nonumber\\
cultural & 1.00001 \nonumber\\
cultural_heritage & 1.00001 \nonumber\\
up_school & 1.00001 \nonumber\\
he_revive & 1.00001 \nonumber\\
control_through & 1.00001 \nonumber\\
malay_and & 1.00001 \nonumber\\
heritage & 1.00001 \nonumber\\
by_set & 1.00001 \nonumber\\
lot_for & 1.00001 \nonumber\\
farquhar_just & 1.00001 \nonumber\\
chinese_and & 1.00001 \nonumber\\
_pos_ngram_NP_PUNC_ADV & 1.00001 \nonumber\\
teacher & 1.00001 \nonumber\\
be_any & 1.00001 \nonumber\\
_pos_ngram_PUNC_ADV_CARD & 1.00001 \nonumber\\
spell & 1.00001 \nonumber\\
_pos_ngram_NP_O_NP & 1.00001 \nonumber\\
woman_. & 1.00001 \nonumber\\
stick & 1.00001 \nonumber\\
ie_. & 1.00001 \nonumber\\
ProductionRule_VP->VBG,PRT,NP, & 1.00001 \nonumber\\
when_the & 1.00001 \nonumber\\
discipline_their & 1.00001 \nonumber\\
but_a & 1.00001 \nonumber\\
_pos_ngram_ART_ART_ADJ & 1.00001 \nonumber\\
two_. & 1.00001 \nonumber\\
last_time & 1.00001 \nonumber\\
_pos_ngram_ADJ_V_ADJ & 1.00001 \nonumber\\
astronomical & 1.00001 \nonumber\\
lack & 1.00001 \nonumber\\
_pos_ngram_PUNC_PP_NP & 1.00001 \nonumber\\
book_if & 1.00001 \nonumber\\
create_. & 1.00001 \nonumber\\
a_uniform & 1.00001 \nonumber\\
_pos_ngram_CARD_V_ADV & 1.00001 \nonumber\\
pay & 1.00001 \nonumber\\
child_up & 1.00001 \nonumber\\
those_be & 1.00001 \nonumber\\
student_do & 1.00001 \nonumber\\
_pos_ngram_NP_CONJ_ART & 1.00001 \nonumber\\
_pos_ngram_NP_CONJ_NN & 1.00001 \nonumber\\
ProductionRule_PRN->-LRB-,NP,-RRB-, & 1.00001 \nonumber\\
have_sex & 1.00001 \nonumber\\
conflict & 1.00001 \nonumber\\
be_still & 1.00001 \nonumber\\
_pos_ngram_ADV_ADJ_V & 1.00001 \nonumber\\
once & 1.00001 \nonumber\\
ProductionRule_VP->VBZ,NP,PP, & 1.00001 \nonumber\\
than_raffle & 1.00001 \nonumber\\
real & 1.00001 \nonumber\\
enjoy & 1.00001 \nonumber\\
do_i & 1.00001 \nonumber\\
school_for & 1.00001 \nonumber\\
that_get & 1.00001 \nonumber\\
and_its & 1.00001 \nonumber\\
ProductionRule_NP->NN,CC,NN,NN, & 1.00001 \nonumber\\
a_live & 1.00001 \nonumber\\
._yeh & 1.00001 \nonumber\\
change_what & 1.00001 \nonumber\\
yeh_there & 1.00001 \nonumber\\
the_gore & 1.00001 \nonumber\\
;_t & 1.00001 \nonumber\\
preggo & 1.00001 \nonumber\\
preggo_in & 1.00001 \nonumber\\
fate_or & 1.00001 \nonumber\\
yeh & 1.00001 \nonumber\\
pay_the & 1.00001 \nonumber\\
fetus_... & 1.00001 \nonumber\\
didn_; & 1.00001 \nonumber\\
_pos_ngram_PUNC_NP_ART & 1.00001 \nonumber\\
have_decide & 1.00001 \nonumber\\
didn & 1.00001 \nonumber\\
you_didn & 1.00001 \nonumber\\
or_use & 1.00001 \nonumber\\
or_fate & 1.00001 \nonumber\\
decide_for & 1.00001 \nonumber\\
get_preggo & 1.00001 \nonumber\\
ultimate_price & 1.00001 \nonumber\\
gore & 1.00001 \nonumber\\
gore_be & 1.00001 \nonumber\\
unfortunate_but & 1.00001 \nonumber\\
form_that & 1.00001 \nonumber\\
really_... & 1.00001 \nonumber\\
place_... & 1.00001 \nonumber\\
sex_or & 1.00001 \nonumber\\
t_wannna & 1.00001 \nonumber\\
ProductionRule_WHADVP->WDT,NN, & 1.00001 \nonumber\\
ProductionRule_VP->VP,:,SBAR, & 1.00001 \nonumber\\
ProductionRule_SBAR->SBAR,:,CC,SBAR, & 1.00001 \nonumber\\
live_form & 1.00001 \nonumber\\
ProductionRule_NP->WP,NN, & 1.00001 \nonumber\\
be_have & 1.00001 \nonumber\\
some_woman & 1.00001 \nonumber\\
wannna & 1.00001 \nonumber\\
you_... & 1.00001 \nonumber\\
intimate & 1.00001 \nonumber\\
wannna_get & 1.00001 \nonumber\\
way_yu & 1.00001 \nonumber\\
mothernature_or & 1.00001 \nonumber\\
mothernature & 1.00001 \nonumber\\
its_still & 1.00001 \nonumber\\
..._whatever & 1.00001 \nonumber\\
yu_see & 1.00001 \nonumber\\
ProductionRule_S->NP,:,VP, & 1.00001 \nonumber\\
argument_in & 1.00001 \nonumber\\
intimate_way & 1.00001 \nonumber\\
ProductionRule_NP->PRP$,ADJP,JJ,NN, & 1.00001 \nonumber\\
way_... & 1.00001 \nonumber\\
whatever_way & 1.00001 \nonumber\\
whatever_have & 1.00001 \nonumber\\
what_mothernature & 1.00001 \nonumber\\
should_the & 1.00001 \nonumber\\
should_give & 1.00001 \nonumber\\
ProductionRule_NP->NP,:,NP,:,SBAR, & 1.00001 \nonumber\\
this_really & 1.00001 \nonumber\\
very_intimate & 1.00001 \nonumber\\
very_unfortunate & 1.00001 \nonumber\\
_pos_ngram_NP_NP_PR & 1.00001 \nonumber\\
,_school & 1.00001 \nonumber\\
establish & 1.00001 \nonumber\\
and_turn & 1.00001 \nonumber\\
people_who & 1.00001 \nonumber\\
god_or & 1.00001 \nonumber\\
environment & 1.00001 \nonumber\\
_pos_ngram_PUNC_PP_CARD & 1.00001 \nonumber\\
name & 1.00001 \nonumber\\
as_my & 1.00001 \nonumber\\
..._and & 1.00001 \nonumber\\
t & 1.00001 \nonumber\\
study_in & 1.00001 \nonumber\\
unborn_child & 1.00001 \nonumber\\
ProductionRule_FRAG->CC,NP, & 1.00001 \nonumber\\
_pos_ngram_CARD_NN_NP & 1.00001 \nonumber\\
fail_to & 1.00001 \nonumber\\
say_anything & 1.00001 \nonumber\\
no_one & 1.00001 \nonumber\\
there_feeling & 1.00001 \nonumber\\
read_book & 1.00001 \nonumber\\
basically & 1.00001 \nonumber\\
encourage & 1.00001 \nonumber\\
what_they & 1.00001 \nonumber\\
'_development & 1.00001 \nonumber\\
police & 1.00001 \nonumber\\
_pos_ngram_CARD_NN_NN & 1.00001 \nonumber\\
price_of & 1.00001 \nonumber\\
_pos_ngram_V_NN_NP & 1.00001 \nonumber\\
_pos_ngram_ADV_ADJ_ART & 1.00001 \nonumber\\
doesnt & 1.00001 \nonumber\\
well & 1.00001 \nonumber\\
_pos_ngram_O_ADV_ADJ & 1.00001 \nonumber\\
once_in & 1.00001 \nonumber\\
EndingIve & 1.00001 \nonumber\\
etc & 1.00001 \nonumber\\
n't_be & 1.00001 \nonumber\\
it_depend & 1.00001 \nonumber\\
like_a & 1.00001 \nonumber\\
of_god & 1.00001 \nonumber\\
malay & 1.00001 \nonumber\\
be_study & 1.00001 \nonumber\\
people_want & 1.00001 \nonumber\\
a_while & 1.00001 \nonumber\\
in_for & 1.00001 \nonumber\\
of_evolution & 1.00001 \nonumber\\
order_to & 1.00002 \nonumber\\
_pos_ngram_ADV_CARD_NN & 1.00002 \nonumber\\
_pos_ngram_ADJ_ADV_PR & 1.00002 \nonumber\\
can_say & 1.00002 \nonumber\\
_pos_ngram_CONJ_V_CONJ & 1.00002 \nonumber\\
gap & 1.00002 \nonumber\\
._any & 1.00002 \nonumber\\
99_% & 1.00002 \nonumber\\
99 & 1.00002 \nonumber\\
dress & 1.00002 \nonumber\\
ProductionRule_NP->ADJP,NN, & 1.00002 \nonumber\\
up_to & 1.00002 \nonumber\\
adoption_. & 1.00002 \nonumber\\
i_dont & 1.00002 \nonumber\\
global & 1.00002 \nonumber\\
..._do & 1.00002 \nonumber\\
crime & 1.00002 \nonumber\\
there_for & 1.00002 \nonumber\\
to_choose & 1.00002 \nonumber\\
'_better & 1.00002 \nonumber\\
_pos_ngram_V_PR_ADJ & 1.00002 \nonumber\\
ProductionRule_SBAR->IN,NN,S, & 1.00002 \nonumber\\
_pos_ngram_V_NP_NN & 1.00002 \nonumber\\
year_old & 1.00002 \nonumber\\
ProductionRule_NP->NP,CONJP,NP, & 1.00002 \nonumber\\
touch & 1.00002 \nonumber\\
long_run & 1.00002 \nonumber\\
seem_to & 1.00002 \nonumber\\
_pos_ngram_ART_ADV_PUNC & 1.00002 \nonumber\\
_pos_ngram_ART_ADJ_ART & 1.00002 \nonumber\\
part_of & 1.00002 \nonumber\\
this_. & 1.00002 \nonumber\\
murderer & 1.00002 \nonumber\\
be_their & 1.00002 \nonumber\\
them_in & 1.00002 \nonumber\\
start & 1.00002 \nonumber\\
feel_like & 1.00002 \nonumber\\
honest & 1.00002 \nonumber\\
honest_, & 1.00002 \nonumber\\
first_place & 1.00002 \nonumber\\
so_in & 1.00002 \nonumber\\
..._you & 1.00002 \nonumber\\
because_i & 1.00002 \nonumber\\
_pos_ngram_O_PP_PR & 1.00002 \nonumber\\
go_, & 1.00002 \nonumber\\
next_to & 1.00002 \nonumber\\
be_only & 1.00002 \nonumber\\
a_great & 1.00002 \nonumber\\
more & 1.00002 \nonumber\\
be_change & 1.00002 \nonumber\\
_pos_ngram_ART_ADJ_V & 1.00002 \nonumber\\
_pos_ngram_PUNC_ART_NP & 1.00002 \nonumber\\
fatherless_, & 1.00002 \nonumber\\
be_extremely & 1.00002 \nonumber\\
extremely & 1.00002 \nonumber\\
?_and & 1.00002 \nonumber\\
boy & 1.00002 \nonumber\\
not_, & 1.00002 \nonumber\\
we_have & 1.00002 \nonumber\\
crazy & 1.00002 \nonumber\\
_pos_ngram_ADV_PUNC_NP & 1.00002 \nonumber\\
be_all & 1.00002 \nonumber\\
ProductionRule_VP->VBG,SBAR, & 1.00002 \nonumber\\
and_try & 1.00002 \nonumber\\
better_father & 1.00002 \nonumber\\
_pos_ngram_ADV_ADJ_ADJ & 1.00002 \nonumber\\
to_look & 1.00002 \nonumber\\
would_turn & 1.00002 \nonumber\\
a_fetus & 1.00002 \nonumber\\
book_be & 1.00002 \nonumber\\
either & 1.00002 \nonumber\\
a_" & 1.00002 \nonumber\\
_pos_ngram_V_O_ART & 1.00002 \nonumber\\
the_woman & 1.00002 \nonumber\\
it_as & 1.00002 \nonumber\\
_pos_ngram_V_PUNC_ADJ & 1.00002 \nonumber\\
rape_and & 1.00002 \nonumber\\
hide & 1.00002 \nonumber\\
to_take & 1.00002 \nonumber\\
of_them & 1.00002 \nonumber\\
there_would & 1.00002 \nonumber\\
internet & 1.00002 \nonumber\\
"_the & 1.00002 \nonumber\\
EndingIc & 1.00002 \nonumber\\
ProductionRule_S->S,CC,S, & 1.00002 \nonumber\\
to_change & 1.00002 \nonumber\\
place_to & 1.00002 \nonumber\\
anything_to & 1.00002 \nonumber\\
good_for & 1.00002 \nonumber\\
in_because & 1.00002 \nonumber\\
you_to & 1.00002 \nonumber\\
away_with & 1.00002 \nonumber\\
get_away & 1.00002 \nonumber\\
_pos_ngram_O_NN_CARD & 1.00002 \nonumber\\
murder_i & 1.00002 \nonumber\\
_pos_ngram_ADV_ADV_CONJ & 1.00002 \nonumber\\
time_i & 1.00002 \nonumber\\
_pos_ngram_ADJ_CONJ_PP & 1.00002 \nonumber\\
ProductionRule_S->NP,ADJP, & 1.00002 \nonumber\\
be_good & 1.00002 \nonumber\\
as_you & 1.00002 \nonumber\\
responsible & 1.00002 \nonumber\\
_pos_ngram_O_ADV & 1.00002 \nonumber\\
role & 1.00002 \nonumber\\
_pos_ngram_ADV_ADV_CARD & 1.00002 \nonumber\\
drink & 1.00002 \nonumber\\
use_to & 1.00002 \nonumber\\
so_it & 1.00002 \nonumber\\
than_to & 1.00002 \nonumber\\
need_be & 1.00002 \nonumber\\
unfortunate & 1.00002 \nonumber\\
follow & 1.00002 \nonumber\\
what_a & 1.00002 \nonumber\\
the_best & 1.00002 \nonumber\\
_pos_ngram_CONJ_PP_ADJ & 1.00002 \nonumber\\
u & 1.00002 \nonumber\\
see_a & 1.00002 \nonumber\\
as_well & 1.00002 \nonumber\\
powerful & 1.00002 \nonumber\\
ProductionRule_VP->VB,NP,PRT, & 1.00002 \nonumber\\
_pos_ngram_PP_ADV_V & 1.00002 \nonumber\\
turn_them & 1.00002 \nonumber\\
where & 1.00002 \nonumber\\
off & 1.00002 \nonumber\\
in_, & 1.00002 \nonumber\\
to_what & 1.00002 \nonumber\\
until & 1.00002 \nonumber\\
fault & 1.00002 \nonumber\\
be_wrong & 1.00002 \nonumber\\
_pos_ngram_PUNC_ART_PR & 1.00002 \nonumber\\
_pos_ngram_PR_NN_O & 1.00002 \nonumber\\
ProductionRule_S->PP,NP,VP, & 1.00002 \nonumber\\
ProductionRule_VP->VBD,NP,PP,SBAR, & 1.00002 \nonumber\\
with_be & 1.00002 \nonumber\\
own & 1.00002 \nonumber\\
instead & 1.00002 \nonumber\\
ProductionRule_VP->VBD,NP,PP, & 1.00002 \nonumber\\
_pos_ngram_NN_ADV_O & 1.00002 \nonumber\\
its & 1.00002 \nonumber\\
in_order & 1.00002 \nonumber\\
admit & 1.00002 \nonumber\\
,_more & 1.00002 \nonumber\\
_pos_ngram_CONJ_ADV_PP & 1.00002 \nonumber\\
definitely & 1.00002 \nonumber\\
_pos_ngram_CONJ_ADV_ADV & 1.00002 \nonumber\\
_pos_ngram_ADV_ADV_O & 1.00002 \nonumber\\
that_not & 1.00002 \nonumber\\
get_rape & 1.00002 \nonumber\\
so_the & 1.00002 \nonumber\\
abortion & 1.00002 \nonumber\\
why_be & 1.00002 \nonumber\\
_pos_ngram_PP_ART_O & 1.00002 \nonumber\\
ProductionRule_VP->VB,ADVP,PP, & 1.00003 \nonumber\\
god & 1.00003 \nonumber\\
_pos_ngram_NP_O_CONJ & 1.00003 \nonumber\\
_pos_ngram_NN_PUNC_PUNC & 1.00003 \nonumber\\
during & 1.00003 \nonumber\\
ModalVerbWill & 1.00003 \nonumber\\
instead_of & 1.00003 \nonumber\\
._do & 1.00003 \nonumber\\
just_do & 1.00003 \nonumber\\
long_as & 1.00003 \nonumber\\
as_long & 1.00003 \nonumber\\
i_love & 1.00003 \nonumber\\
opinion & 1.00003 \nonumber\\
not_to & 1.00003 \nonumber\\
your_life & 1.00003 \nonumber\\
up_. & 1.00003 \nonumber\\
the_world & 1.00003 \nonumber\\
seem & 1.00003 \nonumber\\
worry_about & 1.00003 \nonumber\\
worry & 1.00003 \nonumber\\
more_people & 1.00003 \nonumber\\
solve & 1.00003 \nonumber\\
person_who & 1.00003 \nonumber\\
choose & 1.00003 \nonumber\\
_pos_ngram_O_V_ART & 1.00003 \nonumber\\
bring & 1.00003 \nonumber\\
whole & 1.00003 \nonumber\\
_pos_ngram_NN_ADV_NN & 1.00003 \nonumber\\
come & 1.00003 \nonumber\\
the_last & 1.00003 \nonumber\\
._its & 1.00003 \nonumber\\
its_just & 1.00003 \nonumber\\
ProductionRule_NP->DT,JJS, & 1.00003 \nonumber\\
anyone_. & 1.00003 \nonumber\\
_pos_ngram_V_PP_CONJ & 1.00003 \nonumber\\
_pos_ngram_PP_PP_ADJ & 1.00003 \nonumber\\
._maybe & 1.00003 \nonumber\\
_pos_ngram_V_O_ADJ & 1.00003 \nonumber\\
many & 1.00003 \nonumber\\
study & 1.00003 \nonumber\\
everything & 1.00003 \nonumber\\
user & 1.00003 \nonumber\\
EndingAl & 1.00003 \nonumber\\
_pos_ngram_PP_ADJ_CONJ & 1.00003 \nonumber\\
_pos_ngram_ADV_NN_ART & 1.00003 \nonumber\\
_pos_ngram_CARD_O & 1.00003 \nonumber\\
ProductionRule_VP->VBP,NP,SBAR, & 1.00003 \nonumber\\
_pos_ngram_CARD_PP & 1.00003 \nonumber\\
_pos_ngram_O_V_ADV & 1.00003 \nonumber\\
_pos_ngram_NN_CONJ_ADJ & 1.00003 \nonumber\\
mother & 1.00003 \nonumber\\
_pos_ngram_ADJ_CARD_PUNC & 1.00003 \nonumber\\
_pos_ngram_ART_ADV & 1.00003 \nonumber\\
for_you & 1.00003 \nonumber\\
_pos_ngram_V_PP_PUNC & 1.00003 \nonumber\\
_pos_ngram_NN_ADV_CONJ & 1.00003 \nonumber\\
improve & 1.00003 \nonumber\\
fight & 1.00003 \nonumber\\
and_even & 1.00003 \nonumber\\
little & 1.00003 \nonumber\\
exist & 1.00003 \nonumber\\
_pos_ngram_ADV_PUNC_CONJ & 1.00003 \nonumber\\
_pos_ngram_PP_V_CARD & 1.00003 \nonumber\\
easily & 1.00003 \nonumber\\
_pos_ngram_PP_CARD_PUNC & 1.00003 \nonumber\\
_pos_ngram_ART_NN_ADJ & 1.00003 \nonumber\\
harm & 1.00003 \nonumber\\
_pos_ngram_CONJ_PP_NN & 1.00003 \nonumber\\
..... & 1.00003 \nonumber\\
._you & 1.00003 \nonumber\\
man & 1.00003 \nonumber\\
_pos_ngram_CARD_NN_ADJ & 1.00004 \nonumber\\
be_fatherless & 1.00004 \nonumber\\
_pos_ngram_PUNC_V_NN & 1.00004 \nonumber\\
hope & 1.00004 \nonumber\\
_pos_ngram_PP_ADV_ADV & 1.00004 \nonumber\\
_pos_ngram_PP_NP_CONJ & 1.00004 \nonumber\\
all & 1.00004 \nonumber\\
to_tell & 1.00004 \nonumber\\
and_not & 1.00004 \nonumber\\
you_must & 1.00004 \nonumber\\
change & 1.00004 \nonumber\\
suck & 1.00004 \nonumber\\
_pos_ngram_O_CARD & 1.00004 \nonumber\\
_pos_ngram_NN_PP_CARD & 1.00004 \nonumber\\
,_but & 1.00004 \nonumber\\
a_lot & 1.00004 \nonumber\\
_pos_ngram_V_V_O & 1.00004 \nonumber\\
tv & 1.00004 \nonumber\\
_pos_ngram_O_NP_O & 1.00004 \nonumber\\
our & 1.00004 \nonumber\\
ProductionRule_NP->NP,NN, & 1.00004 \nonumber\\
that_we & 1.00004 \nonumber\\
book & 1.00004 \nonumber\\
_pos_ngram_PR_ADJ_CONJ & 1.00004 \nonumber\\
_pos_ngram_O_V_PP & 1.00004 \nonumber\\
less & 1.00004 \nonumber\\
money & 1.00004 \nonumber\\
ProductionRule_VP->VBG,NP,PP, & 1.00004 \nonumber\\
spouse & 1.00004 \nonumber\\
,_they & 1.00004 \nonumber\\
_pos_ngram_V_ADJ_PR & 1.00004 \nonumber\\
_pos_ngram_ADV_PP_NP & 1.00004 \nonumber\\
one_of & 1.00004 \nonumber\\
a_murder & 1.00004 \nonumber\\
sense & 1.00004 \nonumber\\
be_some & 1.00004 \nonumber\\
but_it & 1.00004 \nonumber\\
_pos_ngram_PUNC_O & 1.00004 \nonumber\\
uniform & 1.00004 \nonumber\\
teach & 1.00004 \nonumber\\
_pos_ngram_CARD_PUNC_PR & 1.00004 \nonumber\\
) & 1.00005 \nonumber\\
_pos_ngram_CONJ_ART_ADJ & 1.00005 \nonumber\\
ProductionRule_VP->VBD,S, & 1.00005 \nonumber\\
_pos_ngram_ADJ_NN_O & 1.00005 \nonumber\\
how & 1.00005 \nonumber\\
whatever & 1.00005 \nonumber\\
pursuit_be & 1.00005 \nonumber\\
me & 1.00005 \nonumber\\
likely & 1.00005 \nonumber\\
,_not & 1.00005 \nonumber\\
_pos_ngram_PR_ADV_ADJ & 1.00005 \nonumber\\
._we & 1.00005 \nonumber\\
long & 1.00005 \nonumber\\
_pos_ngram_CARD_NN_O & 1.00005 \nonumber\\
de.tudarmstadt.ukp.dkpro.core.api.ner.type.Organization & 1.00005 \nonumber\\
them_to & 1.00005 \nonumber\\
_pos_ngram_CONJ_ADJ_ADJ & 1.00005 \nonumber\\
_pos_ngram_CARD_PP_ART & 1.00005 \nonumber\\
_pos_ngram_NN_CONJ_V & 1.00005 \nonumber\\
and_if & 1.00005 \nonumber\\
_pos_ngram_ART_NP_V & 1.00005 \nonumber\\
_pos_ngram_ADJ_CARD_NN & 1.00005 \nonumber\\
that_the & 1.00005 \nonumber\\
_pos_ngram_PP_NP_ADV & 1.00005 \nonumber\\
cant & 1.00005 \nonumber\\
the_child & 1.00005 \nonumber\\
_pos_ngram_NN_O_O & 1.00005 \nonumber\\
commit_a & 1.00005 \nonumber\\
ProductionRule_NP->DT,JJ,NN,NN, & 1.00005 \nonumber\\
_pos_ngram_PUNC_CONJ_ART & 1.00005 \nonumber\\
be_there & 1.00005 \nonumber\\
fatherless & 1.00005 \nonumber\\
_pos_ngram_PUNC_CONJ_V & 1.00005 \nonumber\\
the_other & 1.00005 \nonumber\\
ProductionRule_NP->DT,NNP, & 1.00005 \nonumber\\
marriage_be & 1.00005 \nonumber\\
_pos_ngram_PP_O_V & 1.00005 \nonumber\\
_pos_ngram_V_ADJ_O & 1.00005 \nonumber\\
to_get & 1.00005 \nonumber\\
_pos_ngram_PUNC_ADV_ADV & 1.00005 \nonumber\\
last & 1.00006 \nonumber\\
uniform_be & 1.00006 \nonumber\\
_pos_ngram_PUNC_ADV_ART & 1.00006 \nonumber\\
._" & 1.00006 \nonumber\\
ProductionRule_NP->NP,VP, & 1.00006 \nonumber\\
_pos_ngram_PUNC_ADV_PR & 1.00006 \nonumber\\
maybe & 1.00006 \nonumber\\
_pos_ngram_PP_ART_V & 1.00006 \nonumber\\
_pos_ngram_PP_O_O & 1.00006 \nonumber\\
_pos_ngram_ADV_NP & 1.00006 \nonumber\\
ProductionRule_PRN->-LRB-,S,-RRB-, & 1.00006 \nonumber\\
_pos_ngram_ADJ_O & 1.00006 \nonumber\\
ModalVerbMust & 1.00006 \nonumber\\
_pos_ngram_NN_O_PUNC & 1.00006 \nonumber\\
depend_on & 1.00006 \nonumber\\
could & 1.00006 \nonumber\\
_pos_ngram_NP_PUNC_PP & 1.00006 \nonumber\\
_pos_ngram_O_O_PUNC & 1.00006 \nonumber\\
marriage & 1.00006 \nonumber\\
_pos_ngram_CARD_CARD & 1.00006 \nonumber\\
_pos_ngram_V_NN_PUNC & 1.00006 \nonumber\\
option & 1.00007 \nonumber\\
_pos_ngram_NN_CARD_PUNC & 1.00007 \nonumber\\
lot & 1.00007 \nonumber\\
depend & 1.00007 \nonumber\\
they_can & 1.00007 \nonumber\\
ProductionRule_VP->VBZ,VP, & 1.00007 \nonumber\\
yes & 1.00007 \nonumber\\
ProductionRule_NP->NP,NP, & 1.00007 \nonumber\\
try_to & 1.00007 \nonumber\\
life_. & 1.00007 \nonumber\\
too & 1.00007 \nonumber\\
_pos_ngram_NN_PP_PP & 1.00007 \nonumber\\
if_they & 1.00007 \nonumber\\
_pos_ngram_V_ART_NP & 1.00007 \nonumber\\
if_you & 1.00007 \nonumber\\
to_be & 1.00007 \nonumber\\
_pos_ngram_ART_ADJ_PUNC & 1.00007 \nonumber\\
_pos_ngram_PP_ART_ADV & 1.00008 \nonumber\\
ProductionRule_NP->NN,CC,NN, & 1.00008 \nonumber\\
if_i & 1.00008 \nonumber\\
_pos_ngram_PUNC_O_PUNC & 1.00008 \nonumber\\
ProductionRule_S->S,,,CC,S,., & 1.00008 \nonumber\\
_pos_ngram_PP_NN_PR & 1.00008 \nonumber\\
i_think & 1.00008 \nonumber\\
_pos_ngram_PR_PP_NN & 1.00008 \nonumber\\
._this & 1.00008 \nonumber\\
school & 1.00008 \nonumber\\
._in & 1.00008 \nonumber\\
_pos_ngram_V_V_CONJ & 1.00008 \nonumber\\
that_be & 1.00009 \nonumber\\
_pos_ngram_NN_ADV_PP & 1.00009 \nonumber\\
_pos_ngram_NN_NN_PP & 1.00009 \nonumber\\
_pos_ngram_PUNC_O_V & 1.00009 \nonumber\\
_pos_ngram_ADJ_CARD & 1.00009 \nonumber\\
will & 1.00009 \nonumber\\
_pos_ngram_O_ART & 1.00009 \nonumber\\
do_n't & 1.00009 \nonumber\\
_pos_ngram_V_NN_PR & 1.00009 \nonumber\\
to_have & 1.00009 \nonumber\\
_pos_ngram_PUNC_NN_PUNC & 1.00010 \nonumber\\
_pos_ngram_NN_V_ART & 1.00010 \nonumber\\
dont & 1.00010 \nonumber\\
_pos_ngram_PUNC_V_PR & 1.00010 \nonumber\\
away & 1.00010 \nonumber\\
_pos_ngram_CARD_PUNC_PP & 1.00010 \nonumber\\
really & 1.00010 \nonumber\\
_pos_ngram_O_NP & 1.00010 \nonumber\\
turn & 1.00011 \nonumber\\
_pos_ngram_NN_ADJ_PP & 1.00011 \nonumber\\
_pos_ngram_V_PUNC_ADV & 1.00011 \nonumber\\
_pos_ngram_PP_PR_ADJ & 1.00011 \nonumber\\
reason & 1.00011 \nonumber\\
_pos_ngram_CONJ_NN_PP & 1.00011 \nonumber\\
every & 1.00011 \nonumber\\
_pos_ngram_PUNC_NP_NP & 1.00011 \nonumber\\
in_the & 1.00011 \nonumber\\
thing & 1.00011 \nonumber\\
_pos_ngram_ADJ_ADJ_NN & 1.00011 \nonumber\\
ModalVerbWould & 1.00011 \nonumber\\
must & 1.00012 \nonumber\\
_pos_ngram_ADJ_PP_PR & 1.00012 \nonumber\\
( & 1.00012 \nonumber\\
_pos_ngram_ADV_CARD & 1.00012 \nonumber\\
ModalVerbCould & 1.00012 \nonumber\\
_pos_ngram_V_PUNC_ART & 1.00012 \nonumber\\
life & 1.00012 \nonumber\\
ProductionRule_NP->JJ,NNS, & 1.00013 \nonumber\\
_pos_ngram_ADJ_CONJ & 1.00013 \nonumber\\
i_be & 1.00013 \nonumber\\
person & 1.00014 \nonumber\\
right & 1.00014 \nonumber\\
_pos_ngram_V_PR_PR & 1.00014 \nonumber\\
_pos_ngram_ADV_ADJ_PUNC & 1.00014 \nonumber\\
world & 1.00015 \nonumber\\
ProductionRule_VP->VBZ,S, & 1.00015 \nonumber\\
fog & 1.00015 \nonumber\\
_pos_ngram_NN_CARD & 1.00016 \nonumber\\
ProductionRule_VP->VB,S, & 1.00016 \nonumber\\
_pos_ngram_ADV_O & 1.00016 \nonumber\\
_pos_ngram_V_ADJ_PUNC & 1.00017 \nonumber\\
_pos_ngram_ADJ_ADJ & 1.00017 \nonumber\\
_pos_ngram_NN_ART_V & 1.00017 \nonumber\\
ProductionRule_VP->VB,ADJP, & 1.00018 \nonumber\\
_pos_ngram_NN_V_ADJ & 1.00018 \nonumber\\
ModalVerbShould & 1.00018 \nonumber\\
ProductionRule_VP->VBP,SBAR, & 1.00018 \nonumber\\
i_would & 1.00019 \nonumber\\
_pos_ngram_PR_PP_V & 1.00019 \nonumber\\
_pos_ngram_PUNC_CONJ_PR & 1.00019 \nonumber\\
ProductionRule_NP->NN,NN, & 1.00020 \nonumber\\
_pos_ngram_PR_PR_V & 1.00020 \nonumber\\
_pos_ngram_PR_V_PP & 1.00020 \nonumber\\
_pos_ngram_ART_PR_V & 1.00020 \nonumber\\
_pos_ngram_O_NN_O & 1.00020 \nonumber\\
_pos_ngram_NP_O & 1.00020 \nonumber\\
_pos_ngram_ADV_ART & 1.00020 \nonumber\\
_pos_ngram_V_ART_V & 1.00020 \nonumber\\
use & 1.00021 \nonumber\\
_pos_ngram_ADV_V_ADV & 1.00021 \nonumber\\
_pos_ngram_NN_PUNC_PR & 1.00022 \nonumber\\
_pos_ngram_NN_ADV_V & 1.00023 \nonumber\\
ProductionRule_VP->MD,RB,VP, & 1.00023 \nonumber\\
_pos_ngram_ART_PR & 1.00024 \nonumber\\
so & 1.00024 \nonumber\\
people & 1.00024 \nonumber\\
_pos_ngram_PR_NN_V & 1.00024 \nonumber\\
_pos_ngram_ART_NN_NN & 1.00025 \nonumber\\
_pos_ngram_V_V_PUNC & 1.00026 \nonumber\\
,_and & 1.00028 \nonumber\\
_pos_ngram_PR_ADJ & 1.00028 \nonumber\\
_pos_ngram_PP_NN_PP & 1.00030 \nonumber\\
_pos_ngram_ADJ_PUNC_PR & 1.00030 \nonumber\\
_pos_ngram_PP_NN_V & 1.00030 \nonumber\\
_pos_ngram_NP_NN & 1.00034 \nonumber\\
_pos_ngram_NN_PUNC_PP & 1.00034 \nonumber\\
_pos_ngram_PP_V_NN & 1.00039 \nonumber\\
then & 1.00040 \nonumber\\
_pos_ngram_O_NN & 1.00040 \nonumber\\
at & 1.00041 \nonumber\\
make & 1.00041 \nonumber\\
flesch & 1.00044 \nonumber\\
think & 1.00045 \nonumber\\
_pos_ngram_NP_PUNC & 1.00046 \nonumber\\
_pos_ngram_V_ADV_ADJ & 1.00047 \nonumber\\
kincaid & 1.00048 \nonumber\\
_pos_ngram_V_PR_V & 1.00048 \nonumber\\
_pos_ngram_ADJ_PP_ART & 1.00048 \nonumber\\
have & 1.00051 \nonumber\\
_pos_ngram_ADV_ART_NN & 1.00052 \nonumber\\
_pos_ngram_O & 1.00052 \nonumber\\
they & 1.00053 \nonumber\\
_pos_ngram_V_PR_PP & 1.00056 \nonumber\\
_pos_ngram_V_PP_NN & 1.00056 \nonumber\\
on & 1.00060 \nonumber\\
ProductionRule_NP->DT,JJ,NN, & 1.00063 \nonumber\\
ExclamationRatio & 1.00064 \nonumber\\
DependencyTreeDepth & 1.00068 \nonumber\\
_pos_ngram_ADV_V_PR & 1.00069 \nonumber\\
_pos_ngram_ADV_PR & 1.00072 \nonumber\\
_pos_ngram_ADV_PR_V & 1.00076 \nonumber\\
_pos_ngram_ADV_ADJ & 1.00076 \nonumber\\
_pos_ngram_V_PR_NN & 1.00077 \nonumber\\
_pos_ngram_NN_ART & 1.00077 \nonumber\\
_pos_ngram_PP_ART & 1.00080 \nonumber\\
ProductionRule_NP->NP,SBAR, & 1.00082 \nonumber\\
_pos_ngram_PP_ART_ADJ & 1.00084 \nonumber\\
_pos_ngram_PP_V_PP & 1.00088 \nonumber\\
that & 1.00094 \nonumber\\
ProductionRule_VP->VB,NP, & 1.00095 \nonumber\\
_pos_ngram_ART_NN_PUNC & 1.00095 \nonumber\\
ProductionRule_SBAR->WHNP,S, & 1.00097 \nonumber\\
_pos_ngram_NN_PP_ART & 1.00103 \nonumber\\
Emb_dimension_159 & 1.00104 \nonumber\\
_pos_ngram_ADJ_NN_V & 1.00135 \nonumber\\
_pos_ngram_PR_PP & 1.00135 \nonumber\\
_pos_ngram_PUNC_ADV & 1.00139 \nonumber\\
_pos_ngram_PUNC_CONJ & 1.00155 \nonumber\\
ProductionRule_NP->NP,PP, & 1.00170 \nonumber\\
_pos_ngram_NN_PP_NN & 1.00172 \nonumber\\
_pos_ngram_PR_V_ADV & 1.00204 \nonumber\\
_pos_ngram_V_PP_V & 1.00210 \nonumber\\
_pos_ngram_PR_V_V & 1.00222 \nonumber\\
_pos_ngram_V_PUNC & 1.00229 \nonumber\\
Emb_dimension_254 & 1.00229 \nonumber\\
ProductionRule_PP->IN,NP, & 1.00250 \nonumber\\
_pos_ngram_V_ADV_V & 1.00261 \nonumber\\
Emb_dimension_268 & 1.00271 \nonumber\\
_pos_ngram_PP_ART_NN & 1.00272 \nonumber\\
_pos_ngram_PUNC_PR_V & 1.00283 \nonumber\\
_pos_ngram_NN_NN & 1.00301 \nonumber\\
ProductionRule_NP->DT,NN, & 1.00304 \nonumber\\
lix & 1.00307 \nonumber\\
_pos_ngram_PR_NN & 1.00308 \nonumber\\
_pos_ngram_PUNC_PR & 1.00323 \nonumber\\
Emb_dimension_56 & 1.00330 \nonumber\\
coleman_liau & 1.00339 \nonumber\\
_pos_ngram_PP_NN & 1.00346 \nonumber\\
Emb_dimension_274 & 1.00433 \nonumber\\
Emb_dimension_298 & 1.00481 \nonumber\\
Emb_dimension_142 & 1.00488 \nonumber\\
Emb_dimension_29 & 1.00494 \nonumber\\
Emb_dimension_102 & 1.00495 \nonumber\\
Emb_dimension_98 & 1.00504 \nonumber\\
Emb_dimension_247 & 1.00545 \nonumber\\
Emb_dimension_151 & 1.00585 \nonumber\\
Emb_dimension_124 & 1.00763 \nonumber\\
Emb_dimension_138 & 1.00820 \nonumber\\
Emb_dimension_195 & 1.00868 \nonumber\\
Emb_dimension_125 & 1.00893 \nonumber\\
Emb_dimension_37 & 1.01037 \nonumber\\
Emb_dimension_242 & 1.01130 \nonumber\\
Emb_dimension_176 & 1.01159 \nonumber\\
Emb_dimension_34 & 1.01167 \nonumber\\
PronounRate & 1.01207 \nonumber\\
Emb_dimension_246 & 1.01296 \nonumber\\
Emb_dimension_68 & 1.01421 \nonumber\\
Emb_dimension_76 & 1.01444 \nonumber\\
Emb_dimension_106 & 1.01466 \nonumber\\
Emb_dimension_261 & 1.01472 \nonumber\\
CONTEXTUALITY_MEASURE_FN & 1.01517 \nonumber\\
Emb_dimension_230 & 1.01527 \nonumber\\
Emb_dimension_145 & 1.01553 \nonumber\\
Emb_dimension_269 & 1.01574 \nonumber\\
Emb_dimension_39 & 1.01578 \nonumber\\
Emb_dimension_281 & 1.01596 \nonumber\\
Emb_dimension_53 & 1.01596 \nonumber\\
Emb_dimension_4 & 1.01603 \nonumber\\
Emb_dimension_213 & 1.01603 \nonumber\\
Emb_dimension_139 & 1.01711 \nonumber\\
Emb_dimension_67 & 1.01715 \nonumber\\
Emb_dimension_287 & 1.01722 \nonumber\\
Emb_dimension_95 & 1.01803 \nonumber\\
Emb_dimension_141 & 1.01863 \nonumber\\
ArticleRate & 1.01898 \nonumber\\
Emb_dimension_88 & 1.01959 \nonumber\\
Emb_dimension_77 & 1.01978 \nonumber\\
Emb_dimension_41 & 1.01990 \nonumber\\
Emb_dimension_280 & 1.02079 \nonumber\\
Emb_dimension_263 & 1.02117 \nonumber\\
Emb_dimension_51 & 1.02135 \nonumber\\
Emb_dimension_21 & 1.02153 \nonumber\\
Emb_dimension_78 & 1.02203 \nonumber\\
NounRate & 1.02227 \nonumber\\
Emb_dimension_72 & 1.02331 \nonumber\\
Emb_dimension_272 & 1.02342 \nonumber\\
Emb_dimension_198 & 1.02351 \nonumber\\
Emb_dimension_157 & 1.02499 \nonumber\\
Emb_dimension_161 & 1.02551 \nonumber\\
Emb_dimension_81 & 1.02602 \nonumber\\
Emb_dimension_264 & 1.02615 \nonumber\\
Emb_dimension_255 & 1.02666 \nonumber\\
Emb_dimension_243 & 1.02697 \nonumber\\
Emb_dimension_147 & 1.02717 \nonumber\\
Emb_dimension_18 & 1.02784 \nonumber\\
Emb_dimension_135 & 1.02785 \nonumber\\
Emb_dimension_203 & 1.03005 \nonumber\\
Emb_dimension_112 & 1.03041 \nonumber\\
Emb_dimension_58 & 1.03113 \nonumber\\
Emb_dimension_188 & 1.03143 \nonumber\\
Emb_dimension_33 & 1.03151 \nonumber\\
Emb_dimension_92 & 1.03329 \nonumber\\
Emb_dimension_69 & 1.03343 \nonumber\\
Emb_dimension_208 & 1.03356 \nonumber\\
Emb_dimension_286 & 1.03365 \nonumber\\
Emb_dimension_179 & 1.03422 \nonumber\\
Emb_dimension_202 & 1.03509 \nonumber\\
Emb_dimension_52 & 1.03594 \nonumber\\
Emb_dimension_93 & 1.03616 \nonumber\\
Emb_dimension_45 & 1.03627 \nonumber\\
Emb_dimension_129 & 1.03662 \nonumber\\
Emb_dimension_12 & 1.03664 \nonumber\\
PrepositionRate & 1.03697 \nonumber\\
Emb_dimension_35 & 1.03792 \nonumber\\
Emb_dimension_117 & 1.03797 \nonumber\\
Emb_dimension_164 & 1.04007 \nonumber\\
Emb_dimension_183 & 1.04007 \nonumber\\
VerbRate & 1.04135 \nonumber\\
Emb_dimension_25 & 1.04169 \nonumber\\
Emb_dimension_82 & 1.04204 \nonumber\\
Emb_dimension_126 & 1.04250 \nonumber\\
Emb_dimension_94 & 1.04264 \nonumber\\
Emb_dimension_6 & 1.04290 \nonumber\\
Emb_dimension_240 & 1.04355 \nonumber\\
Emb_dimension_103 & 1.04383 \nonumber\\
Emb_dimension_59 & 1.04403 \nonumber\\
Emb_dimension_200 & 1.04507 \nonumber\\
Emb_dimension_14 & 1.04574 \nonumber\\
Emb_dimension_66 & 1.04595 \nonumber\\
Emb_dimension_0 & 1.04648 \nonumber\\
Emb_dimension_90 & 1.04736 \nonumber\\
Emb_dimension_209 & 1.04787 \nonumber\\
Emb_dimension_50 & 1.04850 \nonumber\\
Emb_dimension_91 & 1.04943 \nonumber\\
Emb_dimension_262 & 1.04948 \nonumber\\
Emb_dimension_234 & 1.05034 \nonumber\\
Emb_dimension_23 & 1.05125 \nonumber\\
Emb_dimension_119 & 1.05145 \nonumber\\
Emb_dimension_190 & 1.05160 \nonumber\\
Emb_dimension_223 & 1.05259 \nonumber\\
Emb_dimension_30 & 1.05288 \nonumber\\
Emb_dimension_160 & 1.05413 \nonumber\\
Emb_dimension_120 & 1.05465 \nonumber\\
Emb_dimension_295 & 1.05468 \nonumber\\
Emb_dimension_100 & 1.05541 \nonumber\\
Emb_dimension_210 & 1.05647 \nonumber\\
Emb_dimension_201 & 1.05660 \nonumber\\
Emb_dimension_185 & 1.05731 \nonumber\\
Emb_dimension_143 & 1.05758 \nonumber\\
Emb_dimension_136 & 1.05810 \nonumber\\
Emb_dimension_42 & 1.05825 \nonumber\\
Emb_dimension_123 & 1.05829 \nonumber\\
Emb_dimension_236 & 1.05867 \nonumber\\
Emb_dimension_187 & 1.05899 \nonumber\\
Emb_dimension_273 & 1.05969 \nonumber\\
Emb_dimension_74 & 1.05971 \nonumber\\
Emb_dimension_182 & 1.06050 \nonumber\\
Emb_dimension_221 & 1.06062 \nonumber\\
Emb_dimension_178 & 1.06062 \nonumber\\
Emb_dimension_215 & 1.06079 \nonumber\\
Emb_dimension_293 & 1.06145 \nonumber\\
AdverbRate & 1.06176 \nonumber\\
Emb_dimension_196 & 1.06239 \nonumber\\
Emb_dimension_214 & 1.06288 \nonumber\\
Emb_dimension_134 & 1.06321 \nonumber\\
Emb_dimension_24 & 1.06436 \nonumber\\
Emb_dimension_75 & 1.06495 \nonumber\\
Emb_dimension_128 & 1.06514 \nonumber\\
Emb_dimension_253 & 1.06687 \nonumber\\
Emb_dimension_219 & 1.06888 \nonumber\\
Emb_dimension_46 & 1.07131 \nonumber\\
Emb_dimension_131 & 1.07171 \nonumber\\
Emb_dimension_231 & 1.07226 \nonumber\\
Emb_dimension_207 & 1.07269 \nonumber\\
Emb_dimension_97 & 1.07343 \nonumber\\
Emb_dimension_184 & 1.07446 \nonumber\\
AdjectiveRate & 1.07469 \nonumber\\
Emb_dimension_278 & 1.08253 \nonumber\\
Emb_dimension_206 & 1.08895 \nonumber\\
Emb_dimension_276 & 1.08921 \nonumber\\
Emb_dimension_167 & 1.10825 \nonumber\\
Emb_dimension_225 & 1.11211 \nonumber\\
sentimentVeryPositive & 3.00134 \nonumber\\

